Vision-based Safe Autonomous UAV Docking with Panoramic Sensors

The remarkable growth of unmanned aerial vehicles (UAVs) has also sparked concerns about safety measures during their missions. To advance towards safer autonomous aerial robots, this work presents a vision-based solution to ensuring safe autonomous UAV landings with minimal infrastructure. During docking maneuvers, UAVs pose a hazard to people in the vicinity. In this paper, we propose the use of a single omnidirectional panoramic camera pointing upwards from a landing pad to detect and estimate the position of people around the landing area. The images are processed in real-time in an embedded computer, which communicates with the onboard computer of approaching UAVs to transition between landing, hovering or emergency landing states. While landing, the ground camera also aids in finding an optimal position, which can be required in case of low-battery or when hovering is no longer possible. We use a YOLOv7-based object detection model and a XGBooxt model for localizing nearby people, and the open-source ROS and PX4 frameworks for communication, interfacing, and control of the UAV. We present both simulation and real-world indoor experimental results to show the efficiency of our methods.

==> tikz/ap_example/ap_example.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
	\tikzstyle{every node}=[font=\scriptsize]
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkorange25512714}{RGB}{255,127,14}
	\definecolor{lightgray204}{RGB}{204,204,204}
	\definecolor{steelblue31119180}{RGB}{31,119,180}

	\begin{axis}[
			axis line style = {draw=none},
			legend cell align={left},
			legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
			tick align=outside,
			tick pos=left,
			xlabel={Recall},
			xmin=-0.05, xmax=1.05,
			xtick style={draw=none},
			ylabel={Precision},
			ymin=-0.05, ymax=1.03,
			ytick style={draw=none},
			x grid style = {lightgray204, dashed},
			xmajorgrids,
			y grid style = {lightgray204, dashed},
			ymajorgrids,
		]
		\addplot [line width = 1.2pt, darkorange25512714]
		table {%
				0 1
				0.2 1
				0.4 1
				0.4 0.67
				0.4 0.5
				0.4 0.4
				0.6 0.5
				0.8 0.57
				0.8 0.5
				0.8 0.44
				1 0.5
			};
		\addlegendentry{precision}
		\addplot [name path = pinterp, line width = 1.2pt, steelblue31119180]
		table {%
				0 1
				0.4 1
				0.4 0.57
				0.8 0.57
				0.8 0.5
				1 0.5
			};
		\addlegendentry{$p_{interp}$}
		\path[name path=axis] (0,0) -- (1,0);
		\addplot[steelblue31119180!30, opacity=0.2]
		fill between[
				of=pinterp and axis,
			];
	\end{axis}

\end{tikzpicture}


==> tikz/dist_data/dist_area.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\definecolor{brown1926061}{RGB}{192,60,61}
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkslategray61}{RGB}{61,61,61}
	\definecolor{darkslategray63}{RGB}{63,63,63}
	\definecolor{dimgray1319183}{RGB}{131,91,83}
	\definecolor{mediumpurple147113178}{RGB}{147,113,178}
	\definecolor{peru22412844}{RGB}{224,128,44}
	\definecolor{seagreen5814558}{RGB}{58,145,58}
	\definecolor{steelblue49115161}{RGB}{49,115,161}

	\begin{groupplot}[group style={group size=2 by 1}]
		\nextgroupplot[
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			xlabel={Distance (m)},
			xmin=-0.5, xmax=0.5,
			xtick style={color=black},
			y grid style={darkgray176},
			ylabel={Normalized bounding box area (0-1)},
			ymin=0, ymax=0.4,
			ytick style={color=black}
		]
		\path [draw=darkslategray63, fill=steelblue49115161, semithick]
		(axis cs:-0.4,0.033617827704)
		--(axis cs:0.4,0.033617827704)
		--(axis cs:0.4,0.058813954726)
		--(axis cs:-0.4,0.058813954726)
		--(axis cs:-0.4,0.033617827704)
		--cycle;
		\addplot [semithick, darkslategray63]
		table {%
				0 0.033617827704
				0 0.016562781625
			};
		\addplot [semithick, darkslategray63]
		table {%
				0 0.058813954726
				0 0.095247787726
			};
		\addplot [semithick, darkslategray63]
		table {%
				-0.2 0.016562781625
				0.2 0.016562781625
			};
		\addplot [semithick, darkslategray63]
		table {%
				-0.2 0.095247787726
				0.2 0.095247787726
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray63}, only marks]
		table {%
				0 0.097405518864
				0 0.099598810311
				0 0.101792787768
				0 0.113330045326
				0 0.113749333726
			};
		\addplot [semithick, darkslategray63]
		table {%
				-0.4 0.04528639024
				0.4 0.04528639024
			};

		\nextgroupplot[
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			xlabel={Distance (m)},
			xmin=-0.5, xmax=5.5,
			xtick style={color=black},
			xtick={0,1,2,3,4,5},
			xticklabels={0-1,1-2,2-3,3-4,4-5,>5},
			y grid style={darkgray176},
			ylabel={Normalized bounding box area (0-1)},
			ymin=0, ymax=0.4,
			ytick style={color=black}
		]
		\path [draw=darkslategray61, fill=steelblue49115161, semithick]
		(axis cs:-0.4,0.0967599909195)
		--(axis cs:0.4,0.0967599909195)
		--(axis cs:0.4,0.1874507467025)
		--(axis cs:-0.4,0.1874507467025)
		--(axis cs:-0.4,0.0967599909195)
		--cycle;
		\path [draw=darkslategray61, fill=peru22412844, semithick]
		(axis cs:0.6,0.033617827704)
		--(axis cs:1.4,0.033617827704)
		--(axis cs:1.4,0.058813954726)
		--(axis cs:0.6,0.058813954726)
		--(axis cs:0.6,0.033617827704)
		--cycle;
		\path [draw=darkslategray61, fill=seagreen5814558, semithick]
		(axis cs:1.6,0.0138808959225)
		--(axis cs:2.4,0.0138808959225)
		--(axis cs:2.4,0.01907584615)
		--(axis cs:1.6,0.01907584615)
		--(axis cs:1.6,0.0138808959225)
		--cycle;
		\path [draw=darkslategray61, fill=brown1926061, semithick]
		(axis cs:2.6,0.0095421836495)
		--(axis cs:3.4,0.0095421836495)
		--(axis cs:3.4,0.0134332242025)
		--(axis cs:2.6,0.0134332242025)
		--(axis cs:2.6,0.0095421836495)
		--cycle;
		\path [draw=darkslategray61, fill=mediumpurple147113178, semithick]
		(axis cs:3.6,0.0056776)
		--(axis cs:4.4,0.0056776)
		--(axis cs:4.4,0.0070453476695)
		--(axis cs:3.6,0.0070453476695)
		--(axis cs:3.6,0.0056776)
		--cycle;
		\path [draw=darkslategray61, fill=dimgray1319183, semithick]
		(axis cs:4.6,0.0047448723885)
		--(axis cs:5.4,0.0047448723885)
		--(axis cs:5.4,0.005646809153)
		--(axis cs:4.6,0.005646809153)
		--(axis cs:4.6,0.0047448723885)
		--cycle;
		\addplot [semithick, darkslategray61]
		table {%
				0 0.0967599909195
				0 0.039972175664
			};
		\addplot [semithick, darkslategray61]
		table {%
				0 0.1874507467025
				0 0.322831111736
			};
		\addplot [semithick, darkslategray61]
		table {%
				-0.2 0.039972175664
				0.2 0.039972175664
			};
		\addplot [semithick, darkslategray61]
		table {%
				-0.2 0.322831111736
				0.2 0.322831111736
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
		table {%
				0 0.3309731289
				0 0.344103644173
				0 0.357357756084
				0 0.370773441104
				0 0.384326027463
				0 0.33891145484
				0 0.36567339011
				0 0.365181820243
				0 0.366758262724
				0 0.367105245908
				0 0.36153812674
				0 0.354838531502
				0 0.35222668168
				0 0.368208912512
				0 0.353576220985
				0 0.3576248389
				0 0.35492576029
				0 0.353484174176
				0 0.357258368768
				0 0.361726369544
				0 0.360255960806
				0 0.36153812674
				0 0.366912285936
				0 0.356192888828
				0 0.36273364064
				0 0.35066470642
				0 0.36273364064
				0 0.359089844091
				0 0.345782329762
				0 0.35251545602
				0 0.349046085136
				0 0.34682852446
				0 0.3438694385
				0 0.347677267168
				0 0.346452941604
				0 0.357692212271
				0 0.37105236952
				0 0.36572170214
				0 0.343551202429
				0 0.32738077099
				0 0.348684
				0 0.349421102198
				0 0.380335312059
				0 0.368131900906
				0 0.338095541392
				0 0.340081188664
				0 0.354511562782
				0 0.365408593792
				0 0.369500122118
				0 0.37039713382
				0 0.37728411872
				0 0.3691197881
				0 0.374358619414
				0 0.37469145548
				0 0.363909294737
				0 0.371004279198
				0 0.365384624542
				0 0.36528775094
				0 0.35714279545
				0 0.364102458608
				0 0.350968616816
				0 0.362964675458
				0 0.353484174176
				0 0.368449964999
				0 0.360255960806
				0 0.366840094544
				0 0.365471276576
				0 0.351908310642
				0 0.356192888828
				0 0.375053002352
				0 0.356000303904
				0 0.350125361278
				0 0.361263709996
				0 0.35714279545
				0 0.365384624542
				0 0.354395519086
				0 0.369505539088
				0 0.373481478745
				0 0.36969319198
				0 0.365471276576
				0 0.362964675458
				0 0.355769157268
				0 0.347677267168
				0 0.351648869096
				0 0.374936944361
				0 0.361263709996
				0 0.36289730428
				0 0.367948373077
				0 0.364102458608
				0 0.35881977166
				0 0.3454408369
				0 0.373481478745
				0 0.36528775094
				0 0.35658417166
				0 0.332205430639
				0 0.351503817481
				0 0.356462959066
				0 0.360497006714
				0 0.332793885136
				0 0.32666311769
				0 0.32604754259
				0 0.32917833518
				0 0.344481253655
				0 0.328331909549
				0 0.323839518352
				0 0.332256223838
				0 0.335102680825
				0 0.432209624346
				0 0.345336674977
				0 0.457260794052
				0 0.421667838258
			};
		\addplot [semithick, darkslategray61]
		table {%
				1 0.033617827704
				1 0.016562781625
			};
		\addplot [semithick, darkslategray61]
		table {%
				1 0.058813954726
				1 0.095247787726
			};
		\addplot [semithick, darkslategray61]
		table {%
				0.8 0.016562781625
				1.2 0.016562781625
			};
		\addplot [semithick, darkslategray61]
		table {%
				0.8 0.095247787726
				1.2 0.095247787726
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
		table {%
				1 0.097405518864
				1 0.099598810311
				1 0.101792787768
				1 0.113330045326
				1 0.113749333726
			};
		\addplot [semithick, darkslategray61]
		table {%
				2 0.0138808959225
				2 0.008590737116
			};
		\addplot [semithick, darkslategray61]
		table {%
				2 0.01907584615
				2 0.026802696554
			};
		\addplot [semithick, darkslategray61]
		table {%
				1.8 0.008590737116
				2.2 0.008590737116
			};
		\addplot [semithick, darkslategray61]
		table {%
				1.8 0.026802696554
				2.2 0.026802696554
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
		table {%
				2 0.027519049586
				2 0.027396750726
				2 0.028188846559
				2 0.031044021925
				2 0.032340473048
				2 0.02955481284
				2 0.03161761658
				2 0.030460771814
				2 0.027106282273
				2 0.027106282273
				2 0.027091852328
				2 0.03369787046
				2 0.035232016505
				2 0.036915240497
				2 0.042013011542
				2 0.042931571522
				2 0.032654280971
				2 0.029792808518
				2 0.03220222253
				2 0.027469960988
				2 0.0279605
				2 0.040252611496
				2 0.0402333745
				2 0.0273182246
				2 0.02855700441
				2 0.02779558824
				2 0.02927997072
				2 0.028532872643
				2 0.027414793532
				2 0.027327972672
				2 0.037334512949
				2 0.042079504915
				2 0.041209902741
				2 0.0283695
				2 0.038109767864
				2 0.037712775898
				2 0.041758105104
				2 0.0430434
				2 0.049650244707
				2 0.041814668242
				2 0.032552062949
				2 0.032552062949
				2 0.028929549792
				2 0.028964734414
				2 0.027715753242
				2 0.036365839414
				2 0.036275870605
				2 0.03427222741
			};
		\addplot [semithick, darkslategray61]
		table {%
				3 0.0095421836495
				3 0.005751811365
			};
		\addplot [semithick, darkslategray61]
		table {%
				3 0.0134332242025
				3 0.019236005528
			};
		\addplot [semithick, darkslategray61]
		table {%
				2.8 0.005751811365
				3.2 0.005751811365
			};
		\addplot [semithick, darkslategray61]
		table {%
				2.8 0.019236005528
				3.2 0.019236005528
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
		table {%
				3 0.019297631031
				3 0.019355588251
				3 0.019413039807
				3 0.01947324205
				3 0.019532975
				3 0.019585944384
				3 0.019647608196
				3 0.019699753884
				3 0.01975426758
				3 0.01981148946
				3 0.019865156597
				3 0.019918453797
				3 0.01972364255
				3 0.019529589838
				3 0.01933965939
				3 0.019621455217
				3 0.019948481956
				3 0.020241843952
				3 0.024199829563
				3 0.023084088181
				3 0.023084088181
				3 0.021275821522
				3 0.021756744229
				3 0.021756744229
				3 0.021708653932
				3 0.023468825908
				3 0.032894637435
				3 0.026720726605
				3 0.030964095085
				3 0.025836466068
				3 0.025387489414
				3 0.035916860586
			};
		\addplot [semithick, darkslategray61]
		table {%
				4 0.0056776
				4 0.003846162348
			};
		\addplot [semithick, darkslategray61]
		table {%
				4 0.0070453476695
				4 0.009091352685
			};
		\addplot [semithick, darkslategray61]
		table {%
				3.8 0.003846162348
				4.2 0.003846162348
			};
		\addplot [semithick, darkslategray61]
		table {%
				3.8 0.009091352685
				4.2 0.009091352685
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
		table {%
				4 0.009273605138
				4 0.009464221468
				4 0.009166093943
				4 0.009574637784
				4 0.01011455472
				4 0.01066521716
				4 0.010499590336
				4 0.010337688177
				4 0.01017452565
				4 0.010017168768
				4 0.00985635882
				4 0.009696841614
				4 0.009544885182
				4 0.00938769747
				4 0.00923159604
				4 0.0092771725
				4 0.01034340747
				4 0.010126468184
				4 0.009915405669
				4 0.00970350237
				4 0.0094955481
				4 0.009280593465
				4 0.009159339956
				4 0.0091949692
				4 0.009230159484
				4 0.009263137442
				4 0.00929747973
				4 0.009331383058
				4 0.009367196784
				4 0.009400490112
				4 0.00943311524
				4 0.009463303896
				4 0.009495162858
				4 0.009526728181
				4 0.009557627703
				4 0.00959055007
				4 0.009618623532
				4 0.009648656628
				4 0.009677954925
				4 0.009706705855
				4 0.00969602838
				4 0.009688833492
				4 0.009674650281
				4 0.009661959384
				4 0.009653111869
				4 0.00963998868
				4 0.009625879056
				4 0.0096136436
				4 0.009600912378
				4 0.009582546823
				4 0.00956880216
				4 0.009554677638
				4 0.009401516912
				4 0.00925402934
				4 0.009103831373
				4 0.009476597844
				4 0.01030944024
				4 0.010309793384
				4 0.010307376288
				4 0.010309793384
				4 0.01030944024
				4 0.01031185782
				4 0.010309793384
				4 0.010307376288
				4 0.010307376288
				4 0.01031185782
				4 0.010309793384
				4 0.010307376288
				4 0.010307376288
				4 0.010309793384
				4 0.01030944024
				4 0.010309793384
				4 0.01030944024
				4 0.009733722607
				4 0.01039739239
				4 0.010839838912
				4 0.010132885888
				4 0.00971929486
				4 0.009858760888
				4 0.011037015928
				4 0.011972183237
				4 0.012724086177
				4 0.011972183237
				4 0.012145730668
				4 0.0123626381
				4 0.01279635428
				4 0.01279635428
				4 0.011342236295
			};
		\addplot [semithick, darkslategray61]
		table {%
				5 0.0047448723885
				5 0.003474052296
			};
		\addplot [semithick, darkslategray61]
		table {%
				5 0.005646809153
				5 0.006752021122
			};
		\addplot [semithick, darkslategray61]
		table {%
				4.8 0.003474052296
				5.2 0.003474052296
			};
		\addplot [semithick, darkslategray61]
		table {%
				4.8 0.006752021122
				5.2 0.006752021122
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
		table {%
				5 0.040699867267
				5 0.039358099954
			};
		\addplot [semithick, darkslategray61]
		table {%
				-0.4 0.13826402008
				0.4 0.13826402008
			};
		\addplot [semithick, darkslategray61]
		table {%
				0.6 0.04528639024
				1.4 0.04528639024
			};
		\addplot [semithick, darkslategray61]
		table {%
				1.6 0.01695233518
				2.4 0.01695233518
			};
		\addplot [semithick, darkslategray61]
		table {%
				2.6 0.011215693573
				3.4 0.011215693573
			};
		\addplot [semithick, darkslategray61]
		table {%
				3.6 0.0062491891825
				4.4 0.0062491891825
			};
		\addplot [semithick, darkslategray61]
		table {%
				4.6 0.00538621195
				5.4 0.00538621195
			};
	\end{groupplot}

\end{tikzpicture}


==> tikz/dist_data/dist_area_boxplot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\tikzstyle{every node}=[font=\scriptsize]
	\definecolor{brown1926061}{RGB}{192,60,61}
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkslategray61}{RGB}{61,61,61}
	\definecolor{dimgray1319183}{RGB}{131,91,83}
	\definecolor{mediumpurple147113178}{RGB}{147,113,178}
	\definecolor{peru22412844}{RGB}{224,128,44}
	\definecolor{seagreen5814558}{RGB}{58,145,58}
	\definecolor{steelblue49115161}{RGB}{49,115,161}
	\definecolor{lightgray235}{RGB}{235,235,235}
	\definecolor{lightgray204}{RGB}{204,204,204}

	\begin{axis}[
			width=0.7\textwidth,
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			xlabel={Distance to camera (m)},
			xmin=-0.5, xmax=5.5,
			xtick style={draw=none},
			xtick={0,1,2,3,4,5},
			% ytick={0,0.1, 0.2, 0.3, 0.4},
			xticklabels={0-1,1-2,2-3,3-4,4-5,$>$5},
			ylabel={Normalized bounding box area (0-1)},
			ymin=-0.0192152847918, ymax=0.4799501311398,
			ytick style={draw=none},
			y grid style = {dashed, lightgray204},
			ymajorgrids,
			axis line style = {draw=none},
			yticklabel style={
					/pgf/number format/fixed,
				},
			scaled y ticks=false
    ]
		\path [draw=darkslategray61, fill=steelblue49115161, semithick]
		(axis cs:-0.4,0.0967599909195)
		--(axis cs:0.4,0.0967599909195)
		--(axis cs:0.4,0.1874507467025)
		--(axis cs:-0.4,0.1874507467025)
		--(axis cs:-0.4,0.0967599909195)
		--cycle;
		\path [draw=darkslategray61, fill=peru22412844, semithick]
		(axis cs:0.6,0.033617827704)
		--(axis cs:1.4,0.033617827704)
		--(axis cs:1.4,0.058813954726)
		--(axis cs:0.6,0.058813954726)
		--(axis cs:0.6,0.033617827704)
		--cycle;
		\path [draw=darkslategray61, fill=seagreen5814558, semithick]
		(axis cs:1.6,0.0138808959225)
		--(axis cs:2.4,0.0138808959225)
		--(axis cs:2.4,0.01907584615)
		--(axis cs:1.6,0.01907584615)
		--(axis cs:1.6,0.0138808959225)
		--cycle;
		\path [draw=darkslategray61, fill=brown1926061, semithick]
		(axis cs:2.6,0.0095421836495)
		--(axis cs:3.4,0.0095421836495)
		--(axis cs:3.4,0.0134332242025)
		--(axis cs:2.6,0.0134332242025)
		--(axis cs:2.6,0.0095421836495)
		--cycle;
		\path [draw=darkslategray61, fill=mediumpurple147113178, semithick]
		(axis cs:3.6,0.0056776)
		--(axis cs:4.4,0.0056776)
		--(axis cs:4.4,0.0070453476695)
		--(axis cs:3.6,0.0070453476695)
		--(axis cs:3.6,0.0056776)
		--cycle;
		\path [draw=darkslategray61, fill=dimgray1319183, semithick]
		(axis cs:4.6,0.0047448723885)
		--(axis cs:5.4,0.0047448723885)
		--(axis cs:5.4,0.005646809153)
		--(axis cs:4.6,0.005646809153)
		--(axis cs:4.6,0.0047448723885)
		--cycle;
		\addplot [semithick, darkslategray61]
		table {%
				0 0.0967599909195
				0 0.039972175664
			};
		\addplot [semithick, darkslategray61]
		table {%
				0 0.1874507467025
				0 0.322831111736
			};
		\addplot [semithick, darkslategray61]
		table {%
				-0.2 0.039972175664
				0.2 0.039972175664
			};
		\addplot [semithick, darkslategray61]
		table {%
				-0.2 0.322831111736
				0.2 0.322831111736
			};
		\addplot [semithick, darkslategray61]
		table {%
				1 0.033617827704
				1 0.016562781625
			};
		\addplot [semithick, darkslategray61]
		table {%
				1 0.058813954726
				1 0.095247787726
			};
		\addplot [semithick, darkslategray61]
		table {%
				0.8 0.016562781625
				1.2 0.016562781625
			};
		\addplot [semithick, darkslategray61]
		table {%
				0.8 0.095247787726
				1.2 0.095247787726
			};
		\addplot [semithick, darkslategray61]
		table {%
				2 0.0138808959225
				2 0.008590737116
			};
		\addplot [semithick, darkslategray61]
		table {%
				2 0.01907584615
				2 0.026802696554
			};
		\addplot [semithick, darkslategray61]
		table {%
				1.8 0.008590737116
				2.2 0.008590737116
			};
		\addplot [semithick, darkslategray61]
		table {%
				1.8 0.026802696554
				2.2 0.026802696554
			};
		\addplot [semithick, darkslategray61]
		table {%
				3 0.0095421836495
				3 0.005751811365
			};
		\addplot [semithick, darkslategray61]
		table {%
				3 0.0134332242025
				3 0.019236005528
			};
		\addplot [semithick, darkslategray61]
		table {%
				2.8 0.005751811365
				3.2 0.005751811365
			};
		\addplot [semithick, darkslategray61]
		table {%
				2.8 0.019236005528
				3.2 0.019236005528
			};
		\addplot [semithick, darkslategray61]
		table {%
				4 0.0056776
				4 0.003846162348
			};
		\addplot [semithick, darkslategray61]
		table {%
				4 0.0070453476695
				4 0.009091352685
			};
		\addplot [semithick, darkslategray61]
		table {%
				3.8 0.003846162348
				4.2 0.003846162348
			};
		\addplot [semithick, darkslategray61]
		table {%
				3.8 0.009091352685
				4.2 0.009091352685
			};
		\addplot [semithick, darkslategray61]
		table {%
				5 0.0047448723885
				5 0.003474052296
			};
		\addplot [semithick, darkslategray61]
		table {%
				5 0.005646809153
				5 0.006752021122
			};
		\addplot [semithick, darkslategray61]
		table {%
				4.8 0.003474052296
				5.2 0.003474052296
			};
		\addplot [semithick, darkslategray61]
		table {%
				4.8 0.006752021122
				5.2 0.006752021122
			};
		\addplot [semithick, darkslategray61]
		table {%
				-0.4 0.13826402008
				0.4 0.13826402008
			};
		\addplot [semithick, darkslategray61]
		table {%
				0.6 0.04528639024
				1.4 0.04528639024
			};
		\addplot [semithick, darkslategray61]
		table {%
				1.6 0.01695233518
				2.4 0.01695233518
			};
		\addplot [semithick, darkslategray61]
		table {%
				2.6 0.011215693573
				3.4 0.011215693573
			};
		\addplot [semithick, darkslategray61]
		table {%
				3.6 0.0062491891825
				4.4 0.0062491891825
			};
		\addplot [semithick, darkslategray61]
		table {%
				4.6 0.00538621195
				5.4 0.00538621195
			};
		\addplot [lightgray204, mark=+, mark size=1.5, only marks]
		table {%
				0 0.3309731289
				0 0.344103644173
				0 0.357357756084
				0 0.370773441104
				0 0.384326027463
				0 0.33891145484
				0 0.36567339011
				0 0.365181820243
				0 0.366758262724
				0 0.367105245908
				0 0.36153812674
				0 0.354838531502
				0 0.35222668168
				0 0.368208912512
				0 0.353576220985
				0 0.3576248389
				0 0.35492576029
				0 0.353484174176
				0 0.357258368768
				0 0.361726369544
				0 0.360255960806
				0 0.36153812674
				0 0.366912285936
				0 0.356192888828
				0 0.36273364064
				0 0.35066470642
				0 0.36273364064
				0 0.359089844091
				0 0.345782329762
				0 0.35251545602
				0 0.349046085136
				0 0.34682852446
				0 0.3438694385
				0 0.347677267168
				0 0.346452941604
				0 0.357692212271
				0 0.37105236952
				0 0.36572170214
				0 0.343551202429
				0 0.32738077099
				0 0.348684
				0 0.349421102198
				0 0.380335312059
				0 0.368131900906
				0 0.338095541392
				0 0.340081188664
				0 0.354511562782
				0 0.365408593792
				0 0.369500122118
				0 0.37039713382
				0 0.37728411872
				0 0.3691197881
				0 0.374358619414
				0 0.37469145548
				0 0.363909294737
				0 0.371004279198
				0 0.365384624542
				0 0.36528775094
				0 0.35714279545
				0 0.364102458608
				0 0.350968616816
				0 0.362964675458
				0 0.353484174176
				0 0.368449964999
				0 0.360255960806
				0 0.366840094544
				0 0.365471276576
				0 0.351908310642
				0 0.356192888828
				0 0.375053002352
				0 0.356000303904
				0 0.350125361278
				0 0.361263709996
				0 0.35714279545
				0 0.365384624542
				0 0.354395519086
				0 0.369505539088
				0 0.373481478745
				0 0.36969319198
				0 0.365471276576
				0 0.362964675458
				0 0.355769157268
				0 0.347677267168
				0 0.351648869096
				0 0.374936944361
				0 0.361263709996
				0 0.36289730428
				0 0.367948373077
				0 0.364102458608
				0 0.35881977166
				0 0.3454408369
				0 0.373481478745
				0 0.36528775094
				0 0.35658417166
				0 0.332205430639
				0 0.351503817481
				0 0.356462959066
				0 0.360497006714
				0 0.332793885136
				0 0.32666311769
				0 0.32604754259
				0 0.32917833518
				0 0.344481253655
				0 0.328331909549
				0 0.323839518352
				0 0.332256223838
				0 0.335102680825
				0 0.432209624346
				0 0.345336674977
				0 0.457260794052
				0 0.421667838258
			};
		\addplot [lightgray204, mark=+, mark size=1.5, only marks]
		table {%
				1 0.097405518864
				1 0.099598810311
				1 0.101792787768
				1 0.113330045326
				1 0.113749333726
			};
		\addplot [lightgray204, mark=+, mark size=1.5, only marks]
		table {%
				2 0.027519049586
				2 0.027396750726
				2 0.028188846559
				2 0.031044021925
				2 0.032340473048
				2 0.02955481284
				2 0.03161761658
				2 0.030460771814
				2 0.027106282273
				2 0.027106282273
				2 0.027091852328
				2 0.03369787046
				2 0.035232016505
				2 0.036915240497
				2 0.042013011542
				2 0.042931571522
				2 0.032654280971
				2 0.029792808518
				2 0.03220222253
				2 0.027469960988
				2 0.0279605
				2 0.040252611496
				2 0.0402333745
				2 0.0273182246
				2 0.02855700441
				2 0.02779558824
				2 0.02927997072
				2 0.028532872643
				2 0.027414793532
				2 0.027327972672
				2 0.037334512949
				2 0.042079504915
				2 0.041209902741
				2 0.0283695
				2 0.038109767864
				2 0.037712775898
				2 0.041758105104
				2 0.0430434
				2 0.049650244707
				2 0.041814668242
				2 0.032552062949
				2 0.032552062949
				2 0.028929549792
				2 0.028964734414
				2 0.027715753242
				2 0.036365839414
				2 0.036275870605
				2 0.03427222741
			};
		\addplot [lightgray204, mark=+, mark size=1.5, only marks]
		table {%
				3 0.019297631031
				3 0.019355588251
				3 0.019413039807
				3 0.01947324205
				3 0.019532975
				3 0.019585944384
				3 0.019647608196
				3 0.019699753884
				3 0.01975426758
				3 0.01981148946
				3 0.019865156597
				3 0.019918453797
				3 0.01972364255
				3 0.019529589838
				3 0.01933965939
				3 0.019621455217
				3 0.019948481956
				3 0.020241843952
				3 0.024199829563
				3 0.023084088181
				3 0.023084088181
				3 0.021275821522
				3 0.021756744229
				3 0.021756744229
				3 0.021708653932
				3 0.023468825908
				3 0.032894637435
				3 0.026720726605
				3 0.030964095085
				3 0.025836466068
				3 0.025387489414
				3 0.035916860586
			};
		\addplot [lightgray204, mark=+, mark size=1.5, only marks]
		table {%
				4 0.009273605138
				4 0.009464221468
				4 0.009166093943
				4 0.009574637784
				4 0.01011455472
				4 0.01066521716
				4 0.010499590336
				4 0.010337688177
				4 0.01017452565
				4 0.010017168768
				4 0.00985635882
				4 0.009696841614
				4 0.009544885182
				4 0.00938769747
				4 0.00923159604
				4 0.0092771725
				4 0.01034340747
				4 0.010126468184
				4 0.009915405669
				4 0.00970350237
				4 0.0094955481
				4 0.009280593465
				4 0.009159339956
				4 0.0091949692
				4 0.009230159484
				4 0.009263137442
				4 0.00929747973
				4 0.009331383058
				4 0.009367196784
				4 0.009400490112
				4 0.00943311524
				4 0.009463303896
				4 0.009495162858
				4 0.009526728181
				4 0.009557627703
				4 0.00959055007
				4 0.009618623532
				4 0.009648656628
				4 0.009677954925
				4 0.009706705855
				4 0.00969602838
				4 0.009688833492
				4 0.009674650281
				4 0.009661959384
				4 0.009653111869
				4 0.00963998868
				4 0.009625879056
				4 0.0096136436
				4 0.009600912378
				4 0.009582546823
				4 0.00956880216
				4 0.009554677638
				4 0.009401516912
				4 0.00925402934
				4 0.009103831373
				4 0.009476597844
				4 0.01030944024
				4 0.010309793384
				4 0.010307376288
				4 0.010309793384
				4 0.01030944024
				4 0.01031185782
				4 0.010309793384
				4 0.010307376288
				4 0.010307376288
				4 0.01031185782
				4 0.010309793384
				4 0.010307376288
				4 0.010307376288
				4 0.010309793384
				4 0.01030944024
				4 0.010309793384
				4 0.01030944024
				4 0.009733722607
				4 0.01039739239
				4 0.010839838912
				4 0.010132885888
				4 0.00971929486
				4 0.009858760888
				4 0.011037015928
				4 0.011972183237
				4 0.012724086177
				4 0.011972183237
				4 0.012145730668
				4 0.0123626381
				4 0.01279635428
				4 0.01279635428
				4 0.011342236295
			};
		\addplot [lightgray204, mark=+, mark size=1.5, only marks]
		table {%
				5 0.040699867267
				5 0.039358099954
			};
	\end{axis}

\end{tikzpicture}


==> tikz/dist_data/dist_data_freq.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\tikzstyle{every node}=[font=\scriptsize]
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{steelblue31119180}{RGB}{31,119,180}
	\definecolor{lightgray204}{RGB}{204,204,204}

	\begin{axis}[
			axis line style = {draw=none},
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			xlabel={Distance (m)},
			xmin=-0.8, xmax=5.8,
			xtick style={draw=none},
			y grid style={lightgray204, dashed},
			ylabel={Number of observations},
			ymin=0, ymax=3921.75,
			ytick style={draw=none},
			y grid style = {lightgray204},
			ymajorgrids,
		]
		\draw[draw=black,fill=steelblue31119180,fill opacity=0.75] (axis cs:-0.5,0) rectangle (axis cs:0.5,3735);
		\draw[draw=black,fill=steelblue31119180,fill opacity=0.75] (axis cs:0.5,0) rectangle (axis cs:1.5,2357);
		\draw[draw=black,fill=steelblue31119180,fill opacity=0.75] (axis cs:1.5,0) rectangle (axis cs:2.5,1299);
		\draw[draw=black,fill=steelblue31119180,fill opacity=0.75] (axis cs:2.5,0) rectangle (axis cs:3.5,1087);
		\draw[draw=black,fill=steelblue31119180,fill opacity=0.75] (axis cs:3.5,0) rectangle (axis cs:4.5,860);
		\draw[draw=black,fill=steelblue31119180,fill opacity=0.75] (axis cs:4.5,0) rectangle (axis cs:5.5,322);
	\end{axis}

\end{tikzpicture}


==> tikz/dist_data/dist_data_freq_close2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\tikzstyle{every node}=[font=\scriptsize]
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkslategray63}{RGB}{63,63,63}
	\definecolor{steelblue49115161}{RGB}{49,115,161}

	\begin{axis}[
			width=0.4\textwidth,
			height=\axisdefaultheight,
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			xmin=-0.5, xmax=0.5,
			xtick style={color=black},
      xticklabels={1.8-2.2},
			y grid style={darkgray176},
			ylabel={Normalized bounding box area (0-1)},
			ymin=0.01170345401995, ymax=0.11860866133105,
			ytick style={color=black}
		]
		\path [draw=darkslategray63, fill=steelblue49115161, semithick]
		(axis cs:-0.4,0.033617827704)
		--(axis cs:0.4,0.033617827704)
		--(axis cs:0.4,0.058813954726)
		--(axis cs:-0.4,0.058813954726)
		--(axis cs:-0.4,0.033617827704)
		--cycle;
		\addplot [semithick, darkslategray63]
		table {%
				0 0.033617827704
				0 0.016562781625
			};
		\addplot [semithick, darkslategray63]
		table {%
				0 0.058813954726
				0 0.095247787726
			};
		\addplot [semithick, darkslategray63]
		table {%
				-0.2 0.016562781625
				0.2 0.016562781625
			};
		\addplot [semithick, darkslategray63]
		table {%
				-0.2 0.095247787726
				0.2 0.095247787726
			};
		\addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray63}, only marks]
		table {%
				0 0.097405518864
				0 0.099598810311
				0 0.101792787768
				0 0.113330045326
				0 0.113749333726
			};
		\addplot [semithick, darkslategray63]
		table {%
				-0.4 0.04528639024
				0.4 0.04528639024
			};
	\end{axis}

\end{tikzpicture}


==> tikz/finetuned_pr/augtest_normal_aug_far.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkorange25512714}{RGB}{255,127,14}
	\definecolor{forestgreen4416044}{RGB}{44,160,44}
	\definecolor{lightgray204}{RGB}{204,204,204}
	\definecolor{lightgray235}{RGB}{235,235,235}
	\definecolor{steelblue31119180}{RGB}{31,119,180}
	\definecolor{darkgray}{RGB}{77,77,77}
	\definecolor{darkred}{RGB}{180,96,96}
	\definecolor{beige}{RGB}{255,191,155}

	\begin{axis}[
			axis line style = {draw=none},
			legend cell align={left},
			legend style={
					draw opacity=0.75,
					text opacity=1,
					anchor=south west,
					at={(0.03,0.03)},
					draw=gray,
				},
			tick align=outside,
			tick pos=left,
			xlabel={Recall},
			xmin=-0.05, xmax=1.05,
			xtick style={draw=none},
			ylabel={Precision},
			ymin=-0.05, ymax=1.05,
			ytick style={draw=none},
			x grid style = {lightgray204, dashed},
			xmajorgrids,
			y grid style = {lightgray204, dashed},
			ymajorgrids,
			% axis background/.style={fill=lightgray235},
		]
		\addplot [name path = ap50, line width = 1.2pt, forestgreen4416044]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 0.993690851735016
				0.08 0.993690851735016
				0.09 0.993690851735016
				0.1 0.993690851735016
				0.11 0.993690851735016
				0.12 0.986636971046771
				0.13 0.986636971046771
				0.14 0.986636971046771
				0.15 0.986636971046771
				0.16 0.986636971046771
				0.17 0.983402489626556
				0.18 0.982300884955752
				0.19 0.982300884955752
				0.2 0.982300884955752
				0.21 0.982300884955752
				0.22 0.982300884955752
				0.23 0.982300884955752
				0.24 0.982300884955752
				0.25 0.981958762886598
				0.26 0.981958762886598
				0.27 0.981958762886598
				0.28 0.981549815498155
				0.29 0.979616306954436
				0.3 0.978991596638655
				0.31 0.978991596638655
				0.32 0.978991596638655
				0.33 0.978991596638655
				0.34 0.977800201816347
				0.35 0.977800201816347
				0.36 0.977229601518027
				0.37 0.977229601518027
				0.38 0.976058931860037
				0.39 0.972296693476318
				0.4 0.970434782608696
				0.41 0.970313825275657
				0.42 0.967768595041322
				0.43 0.963836477987421
				0.44 0.963836477987421
				0.45 0.963706563706564
				0.46 0.959429000751315
				0.47 0.958853783982366
				0.48 0.954967834167262
				0.49 0.951014695591323
				0.5 0.946866485013624
				0.51 0.943257676902537
				0.52 0.935672514619883
				0.53 0.931472081218274
				0.54 0.920049200492005
				0.55 0.912522468544038
				0.56 0.90337601862631
				0.57 0.899202733485194
				0.58 0.878075451066156
				0.59 0.85856992639327
				0.6 0.820969337289812
				0.61 0.796698113207547
				0.62 0.746951219512195
				0.63 0.589448765640852
				0.64 0.502839295854628
				0.65 0.448602794411178
				0.66 0.378681045209457
				0.67 0.329717232793882
				0.68 0.291673127616685
				0.69 0.24228963066379
				0.7 0.203082407213252
				0.71 0
				0.72 0
				0.73 0
				0.74 0
				0.75 0
				0.76 0
				0.77 0
				0.78 0
				0.79 0
				0.8 0
				0.81 0
				0.82 0
				0.83 0
				0.84 0
				0.85 0
				0.86 0
				0.87 0
				0.88 0
				0.89 0
				0.9 0
				0.91 0
				0.92 0
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{F}_{50}$}
		\addplot [name path = ap60, line width = 1.2pt, darkorange25512714]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 0.990536277602524
				0.08 0.990536277602524
				0.09 0.990536277602524
				0.1 0.990536277602524
				0.11 0.990536277602524
				0.12 0.984409799554566
				0.13 0.984409799554566
				0.14 0.984409799554566
				0.15 0.984409799554566
				0.16 0.982905982905983
				0.17 0.981327800829875
				0.18 0.979351032448378
				0.19 0.979351032448378
				0.2 0.979351032448378
				0.21 0.979351032448378
				0.22 0.979351032448378
				0.23 0.979351032448378
				0.24 0.979351032448378
				0.25 0.978319783197832
				0.26 0.978319783197832
				0.27 0.978092783505155
				0.28 0.977556109725686
				0.29 0.974820143884892
				0.3 0.974789915966387
				0.31 0.974789915966387
				0.32 0.974789915966387
				0.33 0.974789915966387
				0.34 0.973763874873865
				0.35 0.973384030418251
				0.36 0.973384030418251
				0.37 0.973384030418251
				0.38 0.970534069981584
				0.39 0.966934763181412
				0.4 0.965217391304348
				0.41 0.964376590330789
				0.42 0.961157024793388
				0.43 0.957547169811321
				0.44 0.957547169811321
				0.45 0.955555555555556
				0.46 0.953159851301115
				0.47 0.952415812591508
				0.48 0.947894361170592
				0.49 0.94244105409154
				0.5 0.938941655359566
				0.51 0.936507936507937
				0.52 0.927190721649485
				0.53 0.913965087281795
				0.54 0.906553398058252
				0.55 0.899527186761229
				0.56 0.890867317633544
				0.57 0.87375415282392
				0.58 0.858288770053476
				0.59 0.824658918645781
				0.6 0.791051880057116
				0.61 0.756611385029135
				0.62 0.550208533846647
				0.63 0.386903440621532
				0.64 0.308536585365854
				0.65 0.227289955780164
				0.66 0.167124290682775
				0.67 0
				0.68 0
				0.69 0
				0.7 0
				0.71 0
				0.72 0
				0.73 0
				0.74 0
				0.75 0
				0.76 0
				0.77 0
				0.78 0
				0.79 0
				0.8 0
				0.81 0
				0.82 0
				0.83 0
				0.84 0
				0.85 0
				0.86 0
				0.87 0
				0.88 0
				0.89 0
				0.9 0
				0.91 0
				0.92 0
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{F}_{60}$}
		\addplot [name path = ap70, line width = 1.2pt, steelblue31119180]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 0.990536277602524
				0.08 0.990536277602524
				0.09 0.990536277602524
				0.1 0.990536277602524
				0.11 0.990536277602524
				0.12 0.984409799554566
				0.13 0.984409799554566
				0.14 0.984409799554566
				0.15 0.984409799554566
				0.16 0.982905982905983
				0.17 0.981327800829875
				0.18 0.979351032448378
				0.19 0.979351032448378
				0.2 0.979351032448378
				0.21 0.979351032448378
				0.22 0.979351032448378
				0.23 0.979351032448378
				0.24 0.979351032448378
				0.25 0.978319783197832
				0.26 0.978319783197832
				0.27 0.978092783505155
				0.28 0.977556109725686
				0.29 0.973621103117506
				0.3 0.972796517954298
				0.31 0.972796517954298
				0.32 0.972796517954298
				0.33 0.972689075630252
				0.34 0.971745711402624
				0.35 0.971144278606965
				0.36 0.97090203685742
				0.37 0.968045112781955
				0.38 0.962828649138713
				0.39 0.961675579322638
				0.4 0.957758620689655
				0.41 0.954583683767872
				0.42 0.950527169505272
				0.43 0.949206349206349
				0.44 0.948262548262548
				0.45 0.943609022556391
				0.46 0.942689199118295
				0.47 0.938040345821326
				0.48 0.933895921237693
				0.49 0.928474114441417
				0.5 0.923898531375167
				0.51 0.914082687338501
				0.52 0.899437851342911
				0.53 0.891793313069909
				0.54 0.88
				0.55 0.871794871794872
				0.56 0.85485651214128
				0.57 0.832189973614776
				0.58 0.796921549155909
				0.59 0.761904761904762
				0.6 0.572413793103448
				0.61 0.419796070629197
				0.62 0.255056513979774
				0.63 0.1875
				0.64 0
				0.65 0
				0.66 0
				0.67 0
				0.68 0
				0.69 0
				0.7 0
				0.71 0
				0.72 0
				0.73 0
				0.74 0
				0.75 0
				0.76 0
				0.77 0
				0.78 0
				0.79 0
				0.8 0
				0.81 0
				0.82 0
				0.83 0
				0.84 0
				0.85 0
				0.86 0
				0.87 0
				0.88 0
				0.89 0
				0.9 0
				0.91 0
				0.92 0
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{F}_{70}$}
		\path[name path=axis] (0,1) -- (0,0) -- (1,0);
		\addplot[forestgreen4416044!30, opacity=0.2]
		fill between[
				of=ap50 and ap60,
				split,
			];
		\addplot[darkorange25512714!30, opacity=0.2]
		fill between[
				of=ap60 and ap70,
				split,
			];
		\addplot[steelblue31119180!30, opacity=0.3]
		fill between[
				of=ap70 and axis,
				split,
			];
	\end{axis}

\end{tikzpicture}


==> tikz/finetuned_pr/augtest_normal_aug_near.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkorange25512714}{RGB}{255,127,14}
	\definecolor{forestgreen4416044}{RGB}{44,160,44}
	\definecolor{lightgray204}{RGB}{204,204,204}
	\definecolor{lightgray235}{RGB}{235,235,235}
	\definecolor{steelblue31119180}{RGB}{31,119,180}
	\definecolor{darkgray}{RGB}{77,77,77}
	\definecolor{darkred}{RGB}{180,96,96}
	\definecolor{beige}{RGB}{255,191,155}

	\begin{axis}[
			axis line style = {draw=none},
			legend cell align={left},
			legend style={
					draw opacity=0.75,
					text opacity=1,
					anchor=south west,
					at={(0.03,0.03)},
					draw=gray,
				},
			tick align=outside,
			tick pos=left,
			xlabel={Recall},
			xmin=-0.05, xmax=1.05,
			xtick style={draw=none},
			ylabel={Precision},
			ymin=-0.05, ymax=1.05,
			ytick style={draw=none},
			x grid style = {lightgray204, dashed},
			xmajorgrids,
			y grid style = {lightgray204, dashed},
			ymajorgrids,
			% axis background/.style={fill=lightgray235},
		]
		\addplot [name path = ap50, line width = 1.2pt, forestgreen4416044]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 1
				0.08 1
				0.09 1
				0.1 1
				0.11 0.998330550918197
				0.12 0.998330550918197
				0.13 0.998330550918197
				0.14 0.998330550918197
				0.15 0.998330550918197
				0.16 0.998330550918197
				0.17 0.998330550918197
				0.18 0.998330550918197
				0.19 0.998330550918197
				0.2 0.998330550918197
				0.21 0.998330550918197
				0.22 0.998330550918197
				0.23 0.998330550918197
				0.24 0.998330550918197
				0.25 0.998330550918197
				0.26 0.998330550918197
				0.27 0.998330550918197
				0.28 0.998330550918197
				0.29 0.998330550918197
				0.3 0.998330550918197
				0.31 0.998330550918197
				0.32 0.998330550918197
				0.33 0.998330550918197
				0.34 0.998330550918197
				0.35 0.998330550918197
				0.36 0.998330550918197
				0.37 0.998330550918197
				0.38 0.998330550918197
				0.39 0.998330550918197
				0.4 0.998330550918197
				0.41 0.998330550918197
				0.42 0.998330550918197
				0.43 0.998330550918197
				0.44 0.998330550918197
				0.45 0.998330550918197
				0.46 0.998330550918197
				0.47 0.998330550918197
				0.48 0.997155049786629
				0.49 0.997155049786629
				0.5 0.997155049786629
				0.51 0.997155049786629
				0.52 0.997155049786629
				0.53 0.997155049786629
				0.54 0.997155049786629
				0.55 0.997155049786629
				0.56 0.994771241830065
				0.57 0.994771241830065
				0.58 0.994771241830065
				0.59 0.994771241830065
				0.6 0.994771241830065
				0.61 0.993678887484197
				0.62 0.993678887484197
				0.63 0.992518703241895
				0.64 0.991556091676719
				0.65 0.991556091676719
				0.66 0.988452655889146
				0.67 0.988452655889146
				0.68 0.988452655889146
				0.69 0.987556561085973
				0.7 0.986984815618221
				0.71 0.986984815618221
				0.72 0.986984815618221
				0.73 0.986707566462168
				0.74 0.986707566462168
				0.75 0.986707566462168
				0.76 0.986707566462168
				0.77 0.986013986013986
				0.78 0.986013986013986
				0.79 0.985265225933202
				0.8 0.984659635666347
				0.81 0.984659635666347
				0.82 0.983778625954199
				0.83 0.983193277310924
				0.84 0.982600732600733
				0.85 0.982600732600733
				0.86 0.981916817359855
				0.87 0.98125
				0.88 0.980650835532102
				0.89 0.978373702422145
				0.9 0.978373702422145
				0.91 0.976411120471778
				0.92 0.976411120471778
				0.93 0.97504159733777
				0.94 0.972085385878489
				0.95 0.96677471636953
				0.96 0.957074721780604
				0.97 0.910246821241586
				0.98 0.705916140149339
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{N}_{50}$}
		\addplot [name path = ap60, line width = 1.2pt, darkorange25512714]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 1
				0.08 1
				0.09 1
				0.1 1
				0.11 0.997455470737914
				0.12 0.997455470737914
				0.13 0.997455470737914
				0.14 0.997455470737914
				0.15 0.997455470737914
				0.16 0.997455470737914
				0.17 0.997455470737914
				0.18 0.997455470737914
				0.19 0.997455470737914
				0.2 0.997455470737914
				0.21 0.997455470737914
				0.22 0.997455470737914
				0.23 0.997455470737914
				0.24 0.997455470737914
				0.25 0.997455470737914
				0.26 0.997455470737914
				0.27 0.997455470737914
				0.28 0.997455470737914
				0.29 0.997455470737914
				0.3 0.997455470737914
				0.31 0.997455470737914
				0.32 0.996138996138996
				0.33 0.996138996138996
				0.34 0.996138996138996
				0.35 0.996138996138996
				0.36 0.996138996138996
				0.37 0.996138996138996
				0.38 0.996138996138996
				0.39 0.996138996138996
				0.4 0.996138996138996
				0.41 0.996138996138996
				0.42 0.994991652754591
				0.43 0.994991652754591
				0.44 0.994991652754591
				0.45 0.994991652754591
				0.46 0.994991652754591
				0.47 0.994991652754591
				0.48 0.994310099573257
				0.49 0.994310099573257
				0.5 0.994310099573257
				0.51 0.994310099573257
				0.52 0.994310099573257
				0.53 0.994310099573257
				0.54 0.994310099573257
				0.55 0.994310099573257
				0.56 0.991537376586742
				0.57 0.990849673202614
				0.58 0.990849673202614
				0.59 0.990849673202614
				0.6 0.990849673202614
				0.61 0.989677419354839
				0.62 0.988621997471555
				0.63 0.987531172069825
				0.64 0.986731001206273
				0.65 0.986731001206273
				0.66 0.983833718244804
				0.67 0.983833718244804
				0.68 0.983031674208145
				0.69 0.983031674208145
				0.7 0.982646420824295
				0.71 0.982646420824295
				0.72 0.982646420824295
				0.73 0.982365145228216
				0.74 0.982365145228216
				0.75 0.982365145228216
				0.76 0.98159509202454
				0.77 0.981018981018981
				0.78 0.981018981018981
				0.79 0.980353634577603
				0.8 0.979552093476144
				0.81 0.978906999041227
				0.82 0.977591036414566
				0.83 0.977591036414566
				0.84 0.976894639556377
				0.85 0.976212259835316
				0.86 0.975587703435805
				0.87 0.974130240856378
				0.88 0.971830985915493
				0.89 0.967937608318891
				0.9 0.964556962025316
				0.91 0.964556962025316
				0.92 0.961762261014131
				0.93 0.958162428219852
				0.94 0.946987951807229
				0.95 0.93563579277865
				0.96 0.861230329041488
				0.97 0.627643115007736
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{N}_{60}$}
		\addplot [name path = ap70, line width = 1.2pt, steelblue31119180]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 1
				0.08 1
				0.09 1
				0.1 1
				0.11 0.997101449275362
				0.12 0.997101449275362
				0.13 0.997101449275362
				0.14 0.997101449275362
				0.15 0.997101449275362
				0.16 0.997101449275362
				0.17 0.997101449275362
				0.18 0.997101449275362
				0.19 0.997101449275362
				0.2 0.997101449275362
				0.21 0.997101449275362
				0.22 0.997101449275362
				0.23 0.997101449275362
				0.24 0.997101449275362
				0.25 0.997101449275362
				0.26 0.997101449275362
				0.27 0.997101449275362
				0.28 0.994832041343669
				0.29 0.994832041343669
				0.3 0.994832041343669
				0.31 0.99236641221374
				0.32 0.988416988416988
				0.33 0.988416988416988
				0.34 0.988416988416988
				0.35 0.988416988416988
				0.36 0.988416988416988
				0.37 0.988416988416988
				0.38 0.988416988416988
				0.39 0.988416988416988
				0.4 0.988416988416988
				0.41 0.987249544626594
				0.42 0.987249544626594
				0.43 0.987249544626594
				0.44 0.984873949579832
				0.45 0.984873949579832
				0.46 0.984873949579832
				0.47 0.982456140350877
				0.48 0.982456140350877
				0.49 0.982456140350877
				0.5 0.978755690440061
				0.51 0.978755690440061
				0.52 0.978662873399715
				0.53 0.978662873399715
				0.54 0.978662873399715
				0.55 0.976284584980237
				0.56 0.976284584980237
				0.57 0.976284584980237
				0.58 0.976284584980237
				0.59 0.976284584980237
				0.6 0.974126778783959
				0.61 0.972187104930468
				0.62 0.971321695760598
				0.63 0.970909090909091
				0.64 0.969843184559711
				0.65 0.966512702078522
				0.66 0.966512702078522
				0.67 0.965714285714286
				0.68 0.964932126696833
				0.69 0.964562569213732
				0.7 0.964013086150491
				0.71 0.963002114164905
				0.72 0.963002114164905
				0.73 0.962655601659751
				0.74 0.962655601659751
				0.75 0.962167689161554
				0.76 0.962037962037962
				0.77 0.961386138613861
				0.78 0.958904109589041
				0.79 0.956855225311601
				0.8 0.956115779645191
				0.81 0.956115779645191
				0.82 0.955637707948244
				0.83 0.954254345837146
				0.84 0.953887884267631
				0.85 0.951828724353256
				0.86 0.948154657293497
				0.87 0.94295592048401
				0.88 0.938879456706282
				0.89 0.934166666666667
				0.9 0.930270713699754
				0.91 0.924696356275304
				0.92 0.910094637223975
				0.93 0.848727272727273
				0.94 0.608045384218669
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{N}_{70}$}
		\path[name path=axis] (0,1) -- (0,0) -- (1,0);
		\addplot[forestgreen4416044!30, opacity=0.2]
		fill between[
				of=ap50 and ap60,
				split,
			];
		\addplot[darkorange25512714!30, opacity=0.2]
		fill between[
				of=ap60 and ap70,
				split,
			];
		\addplot[steelblue31119180!30, opacity=0.3]
		fill between[
				of=ap70 and axis,
				split,
			];
	\end{axis}

\end{tikzpicture}


==> tikz/finetuned_pr/augtest_tiny_aug_far.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkorange25512714}{RGB}{255,127,14}
	\definecolor{forestgreen4416044}{RGB}{44,160,44}
	\definecolor{lightgray204}{RGB}{204,204,204}
	\definecolor{lightgray235}{RGB}{235,235,235}
	\definecolor{steelblue31119180}{RGB}{31,119,180}
	\definecolor{darkgray}{RGB}{77,77,77}
	\definecolor{darkred}{RGB}{180,96,96}
	\definecolor{beige}{RGB}{255,191,155}

	\begin{axis}[
			axis line style = {draw=none},
			legend cell align={left},
			legend style={
					draw opacity=0.75,
					text opacity=1,
					anchor=south west,
					at={(0.03,0.03)},
					draw=gray,
				},
			tick align=outside,
			tick pos=left,
			xlabel={Recall},
			xmin=-0.05, xmax=1.05,
			xtick style={draw=none},
			ylabel={Precision},
			ymin=-0.05, ymax=1.05,
			ytick style={draw=none},
			x grid style = {lightgray204, dashed},
			xmajorgrids,
			y grid style = {lightgray204, dashed},
			ymajorgrids,
			% axis background/.style={fill=lightgray235},
		]
		\addplot [name path = ap50, line width = 1.2pt, forestgreen4416044]
		table {%
				0 1
				0.01 0.981132075471698
				0.02 0.977777777777778
				0.03 0.977777777777778
				0.04 0.977777777777778
				0.05 0.977777777777778
				0.06 0.977777777777778
				0.07 0.977777777777778
				0.08 0.975988700564972
				0.09 0.975988700564972
				0.1 0.975988700564972
				0.11 0.975988700564972
				0.12 0.975988700564972
				0.13 0.975988700564972
				0.14 0.975988700564972
				0.15 0.975988700564972
				0.16 0.975988700564972
				0.17 0.975988700564972
				0.18 0.975988700564972
				0.19 0.975988700564972
				0.2 0.975988700564972
				0.21 0.975988700564972
				0.22 0.975988700564972
				0.23 0.975988700564972
				0.24 0.975988700564972
				0.25 0.974719101123595
				0.26 0.973544973544973
				0.27 0.972762645914397
				0.28 0.970037453183521
				0.29 0.966547192353644
				0.3 0.965947786606129
				0.31 0.9652466367713
				0.32 0.964247020585049
				0.33 0.962224554039874
				0.34 0.961689587426326
				0.35 0.961689587426326
				0.36 0.958693563880884
				0.37 0.952073732718894
				0.38 0.951557093425606
				0.39 0.951557093425606
				0.4 0.94957264957265
				0.41 0.948376353039134
				0.42 0.944178628389155
				0.43 0.942564909520063
				0.44 0.93960244648318
				0.45 0.937547027840482
				0.46 0.930707512764406
				0.47 0.927556818181818
				0.48 0.925034387895461
				0.49 0.922448979591837
				0.5 0.919258769027134
				0.51 0.915693904020752
				0.52 0.906742281033396
				0.53 0.902214022140221
				0.54 0.894799760908548
				0.55 0.886495925494761
				0.56 0.882185543540125
				0.57 0.873200442967885
				0.58 0.86871961102107
				0.59 0.851929092805005
				0.6 0.82390873015873
				0.61 0.787313432835821
				0.62 0.73416095890411
				0.63 0.479372937293729
				0.64 0.371590432228284
				0.65 0.255542922114838
				0.66 0.166241806263656
				0.67 0
				0.68 0
				0.69 0
				0.7 0
				0.71 0
				0.72 0
				0.73 0
				0.74 0
				0.75 0
				0.76 0
				0.77 0
				0.78 0
				0.79 0
				0.8 0
				0.81 0
				0.82 0
				0.83 0
				0.84 0
				0.85 0
				0.86 0
				0.87 0
				0.88 0
				0.89 0
				0.9 0
				0.91 0
				0.92 0
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{F}_{50}$}
		\addplot [name path = ap60, line width = 1.2pt, darkorange25512714]
		table {%
				0 1
				0.01 0.968888888888889
				0.02 0.968888888888889
				0.03 0.968888888888889
				0.04 0.968888888888889
				0.05 0.968888888888889
				0.06 0.968888888888889
				0.07 0.968888888888889
				0.08 0.965811965811966
				0.09 0.965732087227414
				0.1 0.965732087227414
				0.11 0.965732087227414
				0.12 0.965367965367965
				0.13 0.965367965367965
				0.14 0.965367965367965
				0.15 0.965367965367965
				0.16 0.965367965367965
				0.17 0.965367965367965
				0.18 0.965367965367965
				0.19 0.965367965367965
				0.2 0.965367965367965
				0.21 0.965367965367965
				0.22 0.965367965367965
				0.23 0.965367965367965
				0.24 0.965367965367965
				0.25 0.961538461538462
				0.26 0.960159362549801
				0.27 0.955414012738854
				0.28 0.953374233128834
				0.29 0.952046783625731
				0.3 0.951191827468786
				0.31 0.950162513542795
				0.32 0.949732620320856
				0.33 0.947095435684647
				0.34 0.946954813359528
				0.35 0.946393762183236
				0.36 0.938248847926267
				0.37 0.938125568698817
				0.38 0.936851211072664
				0.39 0.936851211072664
				0.4 0.935075885328836
				0.41 0.930024410089504
				0.42 0.929824561403509
				0.43 0.927513639906469
				0.44 0.924528301886792
				0.45 0.919675755342668
				0.46 0.916189111747851
				0.47 0.912133891213389
				0.48 0.910335386721424
				0.49 0.90612516644474
				0.5 0.904046997389034
				0.51 0.896573604060914
				0.52 0.891223733003708
				0.53 0.882140709561034
				0.54 0.873831775700935
				0.55 0.868721461187215
				0.56 0.861512791991101
				0.57 0.851971907077256
				0.58 0.834719334719335
				0.59 0.807121661721068
				0.6 0.772093023255814
				0.61 0.631973043803819
				0.62 0.37363834422658
				0.63 0.134480364169431
				0.64 0
				0.65 0
				0.66 0
				0.67 0
				0.68 0
				0.69 0
				0.7 0
				0.71 0
				0.72 0
				0.73 0
				0.74 0
				0.75 0
				0.76 0
				0.77 0
				0.78 0
				0.79 0
				0.8 0
				0.81 0
				0.82 0
				0.83 0
				0.84 0
				0.85 0
				0.86 0
				0.87 0
				0.88 0
				0.89 0
				0.9 0
				0.91 0
				0.92 0
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{F}_{60}$}
		\addplot [name path = ap70, line width = 1.2pt, steelblue31119180]
		table {%
				0 1
				0.01 0.959459459459459
				0.02 0.959459459459459
				0.03 0.959459459459459
				0.04 0.959459459459459
				0.05 0.959459459459459
				0.06 0.959459459459459
				0.07 0.959459459459459
				0.08 0.956656346749226
				0.09 0.956656346749226
				0.1 0.956656346749226
				0.11 0.956656346749226
				0.12 0.955654101995565
				0.13 0.955654101995565
				0.14 0.955654101995565
				0.15 0.955654101995565
				0.16 0.954838709677419
				0.17 0.954697986577181
				0.18 0.954697986577181
				0.19 0.954697986577181
				0.2 0.954697986577181
				0.21 0.954616588419405
				0.22 0.954616588419405
				0.23 0.953956834532374
				0.24 0.953125
				0.25 0.950684931506849
				0.26 0.946959896507115
				0.27 0.945205479452055
				0.28 0.941034897713598
				0.29 0.939323220536756
				0.3 0.937360178970917
				0.31 0.936681222707424
				0.32 0.932984293193717
				0.33 0.932254802831143
				0.34 0.931372549019608
				0.35 0.925118483412322
				0.36 0.92188919164396
				0.37 0.920863309352518
				0.38 0.920552677029361
				0.39 0.917508417508417
				0.4 0.912828947368421
				0.41 0.910756972111554
				0.42 0.908807482462977
				0.43 0.905703422053232
				0.44 0.900960827790096
				0.45 0.896995708154506
				0.46 0.894035087719298
				0.47 0.891319207108681
				0.48 0.884973404255319
				0.49 0.881818181818182
				0.5 0.874368686868687
				0.51 0.867854947756607
				0.52 0.855614973262032
				0.53 0.847663012117715
				0.54 0.841189674523008
				0.55 0.829625610417797
				0.56 0.811943425877423
				0.57 0.783904619970194
				0.58 0.752108716026242
				0.59 0.711421098517873
				0.6 0.433986928104575
				0.61 0.169460897500251
				0.62 0
				0.63 0
				0.64 0
				0.65 0
				0.66 0
				0.67 0
				0.68 0
				0.69 0
				0.7 0
				0.71 0
				0.72 0
				0.73 0
				0.74 0
				0.75 0
				0.76 0
				0.77 0
				0.78 0
				0.79 0
				0.8 0
				0.81 0
				0.82 0
				0.83 0
				0.84 0
				0.85 0
				0.86 0
				0.87 0
				0.88 0
				0.89 0
				0.9 0
				0.91 0
				0.92 0
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{F}_{70}$}
		\path[name path=axis] (0,1) -- (0,0) -- (1,0);
		\addplot[forestgreen4416044!30, opacity=0.2]
		fill between[
				of=ap50 and ap60,
				split,
			];
		\addplot[darkorange25512714!30, opacity=0.2]
		fill between[
				of=ap60 and ap70,
				split,
			];
		\addplot[steelblue31119180!30, opacity=0.3]
		fill between[
				of=ap70 and axis,
				split,
			];
	\end{axis}

\end{tikzpicture}


==> tikz/finetuned_pr/augtest_tiny_aug_near.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{darkorange25512714}{RGB}{255,127,14}
	\definecolor{forestgreen4416044}{RGB}{44,160,44}
	\definecolor{lightgray204}{RGB}{204,204,204}
	\definecolor{lightgray235}{RGB}{235,235,235}
	\definecolor{steelblue31119180}{RGB}{31,119,180}
	\definecolor{darkgray}{RGB}{77,77,77}
	\definecolor{darkred}{RGB}{180,96,96}
	\definecolor{beige}{RGB}{255,191,155}

	\begin{axis}[
			axis line style = {draw=none},
			legend cell align={left},
			legend style={
					draw opacity=0.75,
					text opacity=1,
					anchor=south west,
					at={(0.03,0.03)},
					draw=gray,
				},
			tick align=outside,
			tick pos=left,
			xlabel={Recall},
			xmin=-0.05, xmax=1.05,
			xtick style={draw=none},
			ylabel={Precision},
			ymin=-0.05, ymax=1.05,
			ytick style={draw=none},
			x grid style = {lightgray204, dashed},
			xmajorgrids,
			y grid style = {lightgray204, dashed},
			ymajorgrids,
			% axis background/.style={fill=lightgray235},
		]
		\addplot [name path = ap50, line width = 1.2pt, forestgreen4416044]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 1
				0.08 1
				0.09 1
				0.1 1
				0.11 1
				0.12 1
				0.13 1
				0.14 1
				0.15 1
				0.16 1
				0.17 1
				0.18 1
				0.19 1
				0.2 1
				0.21 1
				0.22 1
				0.23 1
				0.24 1
				0.25 1
				0.26 1
				0.27 1
				0.28 1
				0.29 0.998319327731092
				0.3 0.998319327731092
				0.31 0.998319327731092
				0.32 0.998319327731092
				0.33 0.998319327731092
				0.34 0.998319327731092
				0.35 0.998319327731092
				0.36 0.998319327731092
				0.37 0.998319327731092
				0.38 0.998319327731092
				0.39 0.998319327731092
				0.4 0.998319327731092
				0.41 0.998319327731092
				0.42 0.998319327731092
				0.43 0.998319327731092
				0.44 0.998319327731092
				0.45 0.998319327731092
				0.46 0.998319327731092
				0.47 0.998319327731092
				0.48 0.996974281391831
				0.49 0.996974281391831
				0.5 0.996974281391831
				0.51 0.996974281391831
				0.52 0.996974281391831
				0.53 0.99554234769688
				0.54 0.994194484760523
				0.55 0.993016759776536
				0.56 0.993016759776536
				0.57 0.993006993006993
				0.58 0.993006993006993
				0.59 0.993006993006993
				0.6 0.993006993006993
				0.61 0.993006993006993
				0.62 0.993006993006993
				0.63 0.993006993006993
				0.64 0.993006993006993
				0.65 0.993006993006993
				0.66 0.993006993006993
				0.67 0.993006993006993
				0.68 0.991916859122402
				0.69 0.991370010787487
				0.7 0.991370010787487
				0.71 0.991370010787487
				0.72 0.991370010787487
				0.73 0.991370010787487
				0.74 0.990654205607477
				0.75 0.990654205607477
				0.76 0.990654205607477
				0.77 0.989795918367347
				0.78 0.989632422243167
				0.79 0.989632422243167
				0.8 0.989632422243167
				0.81 0.989632422243167
				0.82 0.989632422243167
				0.83 0.989632422243167
				0.84 0.988940092165899
				0.85 0.988940092165899
				0.86 0.988256549232159
				0.87 0.988256549232159
				0.88 0.986099044309296
				0.89 0.986099044309296
				0.9 0.986099044309296
				0.91 0.984496124031008
				0.92 0.981340118744699
				0.93 0.979882648784577
				0.94 0.974380165289256
				0.95 0.950558213716108
				0.96 0.901197604790419
				0.97 0.757311761045426
				0.98 0.435661113080468
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{N}_{50}$}
		\addplot [name path = ap60, line width = 1.2pt, darkorange25512714]
		table {%
				0 1
				0.01 1
				0.02 1
				0.03 1
				0.04 1
				0.05 1
				0.06 1
				0.07 1
				0.08 1
				0.09 1
				0.1 0.997183098591549
				0.11 0.997183098591549
				0.12 0.997183098591549
				0.13 0.997183098591549
				0.14 0.997183098591549
				0.15 0.997183098591549
				0.16 0.997183098591549
				0.17 0.997183098591549
				0.18 0.997183098591549
				0.19 0.997183098591549
				0.2 0.997183098591549
				0.21 0.997183098591549
				0.22 0.997183098591549
				0.23 0.997183098591549
				0.24 0.997183098591549
				0.25 0.997183098591549
				0.26 0.997183098591549
				0.27 0.997183098591549
				0.28 0.997183098591549
				0.29 0.996396396396396
				0.3 0.996396396396396
				0.31 0.996396396396396
				0.32 0.996396396396396
				0.33 0.996396396396396
				0.34 0.996396396396396
				0.35 0.996396396396396
				0.36 0.996396396396396
				0.37 0.996396396396396
				0.38 0.996396396396396
				0.39 0.996396396396396
				0.4 0.996396396396396
				0.41 0.996396396396396
				0.42 0.996396396396396
				0.43 0.996396396396396
				0.44 0.996396396396396
				0.45 0.994957983193277
				0.46 0.994957983193277
				0.47 0.994957983193277
				0.48 0.993620414673046
				0.49 0.993620414673046
				0.5 0.992211838006231
				0.51 0.990922844175492
				0.52 0.990922844175492
				0.53 0.989583333333333
				0.54 0.986937590711176
				0.55 0.985795454545455
				0.56 0.984723854289072
				0.57 0.984723854289072
				0.58 0.984723854289072
				0.59 0.984723854289072
				0.6 0.984723854289072
				0.61 0.984723854289072
				0.62 0.984723854289072
				0.63 0.984723854289072
				0.64 0.984723854289072
				0.65 0.984723854289072
				0.66 0.984723854289072
				0.67 0.983682983682984
				0.68 0.982551799345692
				0.69 0.982551799345692
				0.7 0.982551799345692
				0.71 0.982551799345692
				0.72 0.981661272923409
				0.73 0.980728051391863
				0.74 0.979978925184405
				0.75 0.979231568016615
				0.76 0.978571428571429
				0.77 0.978
				0.78 0.977379830348728
				0.79 0.977379830348728
				0.8 0.977379830348728
				0.81 0.977379830348728
				0.82 0.977379830348728
				0.83 0.976958525345622
				0.84 0.976958525345622
				0.85 0.976427923844062
				0.86 0.975609756097561
				0.87 0.972590627763042
				0.88 0.972198088618593
				0.89 0.972198088618593
				0.9 0.969957081545064
				0.91 0.967060810810811
				0.92 0.960865945045795
				0.93 0.948178137651822
				0.94 0.919656786271451
				0.95 0.817558299039781
				0.96 0.67075208913649
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{N}_{60}$}
		\addplot [name path = ap70, line width = 1.2pt, steelblue31119180]
		table {%
				0 1
				0.01 0.978260869565217
				0.02 0.978260869565217
				0.03 0.978260869565217
				0.04 0.976744186046512
				0.05 0.976744186046512
				0.06 0.976744186046512
				0.07 0.976744186046512
				0.08 0.976744186046512
				0.09 0.976744186046512
				0.1 0.976744186046512
				0.11 0.976744186046512
				0.12 0.976744186046512
				0.13 0.976744186046512
				0.14 0.976331360946746
				0.15 0.976331360946746
				0.16 0.976331360946746
				0.17 0.976331360946746
				0.18 0.976331360946746
				0.19 0.976331360946746
				0.2 0.976331360946746
				0.21 0.976331360946746
				0.22 0.976331360946746
				0.23 0.976331360946746
				0.24 0.976331360946746
				0.25 0.976331360946746
				0.26 0.976331360946746
				0.27 0.974683544303797
				0.28 0.974683544303797
				0.29 0.974683544303797
				0.3 0.974683544303797
				0.31 0.974683544303797
				0.32 0.974683544303797
				0.33 0.974683544303797
				0.34 0.974683544303797
				0.35 0.974683544303797
				0.36 0.974683544303797
				0.37 0.974683544303797
				0.38 0.974683544303797
				0.39 0.974683544303797
				0.4 0.974683544303797
				0.41 0.974683544303797
				0.42 0.974683544303797
				0.43 0.973498233215548
				0.44 0.972555746140652
				0.45 0.972555746140652
				0.46 0.970345963756178
				0.47 0.9696
				0.48 0.9696
				0.49 0.96875
				0.5 0.96793893129771
				0.51 0.965671641791045
				0.52 0.963609898107715
				0.53 0.96264367816092
				0.54 0.959383753501401
				0.55 0.956175298804781
				0.56 0.956175298804781
				0.57 0.956175298804781
				0.58 0.955901426718547
				0.59 0.955445544554455
				0.6 0.955445544554455
				0.61 0.955445544554455
				0.62 0.954712362301102
				0.63 0.954707985697259
				0.64 0.954063604240283
				0.65 0.953271028037383
				0.66 0.949616648411829
				0.67 0.949616648411829
				0.68 0.949616648411829
				0.69 0.949616648411829
				0.7 0.946351931330472
				0.71 0.943974630021142
				0.72 0.94258872651357
				0.73 0.940881763527054
				0.74 0.940881763527054
				0.75 0.940711462450593
				0.76 0.939901477832512
				0.77 0.938894277400582
				0.78 0.937440758293839
				0.79 0.935849056603774
				0.8 0.935424354243542
				0.81 0.935395814376706
				0.82 0.934723481414325
				0.83 0.9319606087735
				0.84 0.930313588850174
				0.85 0.930313588850174
				0.86 0.927835051546392
				0.87 0.923141891891892
				0.88 0.916182572614108
				0.89 0.900080580177276
				0.9 0.86579754601227
				0.91 0.738202973497091
				0.92 0.555341674687199
				0.93 0
				0.94 0
				0.95 0
				0.96 0
				0.97 0
				0.98 0
				0.99 0
				1 0
			};
		\addlegendentry{$AP^{N}_{70}$}
		\path[name path=axis] (0,1) -- (0,0) -- (1,0);
		\addplot[forestgreen4416044!30, opacity=0.2]
		fill between[
				of=ap50 and ap60,
				split,
			];
		\addplot[darkorange25512714!30, opacity=0.2]
		fill between[
				of=ap60 and ap70,
				split,
			];
		\addplot[steelblue31119180!30, opacity=0.3]
		fill between[
				of=ap70 and axis,
				split,
			];
	\end{axis}

\end{tikzpicture}


==> tikz/vis_localize/vis_loc_test1.tex <==
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, mark size = 0.5, only marks]
table{%
		x  y
		-0.475712776184082 0.139563798904419
		-0.48016357421875 0.13003134727478
		-0.484662771224976 0.120531320571899
		-0.488897800445557 0.11302661895752
		-0.492714405059814 0.10748553276062
		-0.49623441696167 0.103432655334473
		-0.498867750167847 0.100691318511963
		-0.500219106674194 0.099339485168457
		-0.501091718673706 0.0987460613250732
		-0.501281499862671 0.0983812808990479
		-0.500238180160522 0.0990939140319824
		-0.498081684112549 0.10090160369873
		-0.494987010955811 0.10337495803833
		-0.490299224853516 0.107610464096069
		-0.484137296676636 0.113415718078613
		-0.476642370223999 0.11933422088623
		-0.467615127563477 0.125444412231445
		-0.448736906051636 0.139361143112183
		-0.440921068191528 0.145599126815796
		-0.434382915496826 0.151087760925293
		-0.428848266601562 0.154041290283203
		-0.422903537750244 0.154541969299316
		-0.41616678237915 0.151306629180908
		-0.408305883407593 0.146421194076538
		-0.398385524749756 0.13956618309021
		-0.386202573776245 0.130125284194946
		-0.373197555541992 0.119078874588013
		-0.360451459884644 0.10615611076355
		-0.350766658782959 0.0905110836029053
		-0.346651315689087 0.0725741386413574
		-0.346630573272705 0.0540013313293457
		-0.34872579574585 0.0342636108398438
		-0.351482629776001 0.0158054828643799
		-0.354551792144775 -0.000281810760498047
		-0.370930194854736 -0.0325417518615723
		-0.377519130706787 -0.0319318771362305
		-0.385736465454102 -0.0293605327606201
		-0.39378809928894 -0.0262100696563721
		-0.401523590087891 -0.0218305587768555
		-0.405033111572266 -0.017491340637207
		-0.405186414718628 -0.0147974491119385
		-0.404563903808594 -0.0129768848419189
		-0.403174161911011 -0.00988960266113281
		-0.40070366859436 -0.0061955451965332
		-0.396726369857788 -0.00256896018981934
		-0.391418933868408 -0.000899791717529297
		-0.384414911270142 -0.00140118598937988
		-0.378307580947876 -0.00747132301330566
		-0.372807741165161 -0.0177080631256104
		-0.367538690567017 -0.032109260559082
		-0.361993312835693 -0.0495333671569824
		-0.352928876876831 -0.090815544128418
		-0.349136352539062 -0.111238241195679
		-0.345038414001465 -0.12778377532959
		-0.340015172958374 -0.140910148620605
		-0.332670927047729 -0.15178108215332
		-0.325768947601318 -0.16033673286438
		-0.320273637771606 -0.166346549987793
		-0.318015575408936 -0.170641660690308
		-0.31784462928772 -0.173107147216797
		-0.31738805770874 -0.172533512115479
		-0.316419839859009 -0.169675588607788
		-0.31549859046936 -0.164752721786499
		-0.312368869781494 -0.155733108520508
		-0.305740118026733 -0.142026424407959
		-0.29944920539856 -0.13015341758728
		-0.293302536010742 -0.120808362960815
		-0.286153316497803 -0.111964702606201
		-0.458095788955688 0.132659435272217
		-0.36111044883728 -0.0232803821563721
		-0.357597589492798 -0.0695714950561523
		-0.277831077575684 -0.103550910949707
		-0.079371452331543 -0.218852281570435
		-0.0664448738098145 -0.21781587600708
		0.140823364257812 -0.300868034362793
		0.196993350982666 -0.285125255584717
		0.288749694824219 -0.290963411331177
		0.373701572418213 -0.261462926864624
		0.237928867340088 -0.298861026763916
		0.411582946777344 -0.1285240650177
		0.548575401306152 -0.101940393447876
		0.428156852722168 -0.144186019897461
		0.452932834625244 0.0648679733276367
		0.500128269195557 0.150605916976929
		-0.269028186798096 -0.0956037044525146
		-0.259313583374023 -0.089726448059082
		-0.251208305358887 -0.084907054901123
		-0.244046688079834 -0.0823824405670166
		-0.237510681152344 -0.0842549800872803
		-0.231042385101318 -0.0903100967407227
		-0.224717617034912 -0.10001802444458
		-0.218066692352295 -0.113818645477295
		-0.209716320037842 -0.130792617797852
		-0.199263095855713 -0.148705244064331
		-0.184657573699951 -0.168038845062256
		-0.166447162628174 -0.187976121902466
		-0.149294853210449 -0.205202341079712
		-0.13410758972168 -0.215509176254272
		-0.117977142333984 -0.218178272247314
		-0.100935459136963 -0.217293262481689
		-0.0872626304626465 -0.216602325439453
		-0.0756235122680664 -0.226210594177246
		-0.0734786987304688 -0.237581968307495
		-0.0733661651611328 -0.250401496887207
		-0.0741291046142578 -0.26203179359436
		-0.0754437446594238 -0.270983934402466
		-0.0780858993530273 -0.276713132858276
		-0.0810694694519043 -0.278963804244995
		-0.0851850509643555 -0.277148485183716
		-0.0886759757995605 -0.271273136138916
		-0.0912580490112305 -0.264797210693359
		-0.093134880065918 -0.258567571640015
		-0.0929660797119141 -0.251707792282104
		-0.0913257598876953 -0.245682001113892
		-0.0878586769104004 -0.240110874176025
		-0.084357738494873 -0.233837842941284
		-0.0804948806762695 -0.227731466293335
		-0.074927806854248 -0.222298383712769
		-0.0563206672668457 -0.215169906616211
		-0.0441403388977051 -0.214928865432739
		-0.0287599563598633 -0.215799808502197
		-0.0118660926818848 -0.219435453414917
		0.00651693344116211 -0.225900173187256
		0.0264759063720703 -0.233037233352661
		0.0472002029418945 -0.240463256835938
		0.0687074661254883 -0.247420787811279
		0.0879907608032227 -0.25345253944397
		0.10275411605835 -0.257692813873291
		0.113116264343262 -0.261159420013428
		0.121819496154785 -0.266241312026978
		0.129180431365967 -0.27150559425354
		0.134980201721191 -0.277616024017334
		0.138407230377197 -0.283980846405029
		0.139612197875977 -0.290240526199341
		0.140820503234863 -0.296051502227783
		0.139509201049805 -0.302407026290894
		0.138659477233887 -0.301776885986328
		0.138566970825195 -0.302284955978394
		0.138940334320068 -0.303348779678345
		0.13801383972168 -0.302705049514771
		0.136441230773926 -0.301114797592163
		0.136185646057129 -0.29899525642395
		0.136542797088623 -0.295439958572388
		0.135914325714111 -0.291039943695068
		0.136292934417725 -0.287924766540527
		0.137283325195312 -0.286736965179443
		0.139772891998291 -0.285691499710083
		0.14375638961792 -0.284742116928101
		0.150585174560547 -0.284840106964111
		0.159670352935791 -0.28556489944458
		0.170924186706543 -0.285479545593262
		0.184267997741699 -0.285270214080811
		0.209714889526367 -0.28423547744751
		0.22251033782959 -0.28141975402832
		0.234349250793457 -0.2767174243927
		0.243575096130371 -0.271186590194702
		0.249000072479248 -0.267449617385864
		0.251852512359619 -0.265111207962036
		0.251987934112549 -0.263451814651489
		0.250884056091309 -0.262758493423462
		0.249485969543457 -0.262547731399536
		0.247910976409912 -0.263566732406616
		0.247492790222168 -0.265493392944336
		0.248725414276123 -0.267669916152954
		0.251158714294434 -0.270594358444214
		0.255521297454834 -0.273554086685181
		0.261666774749756 -0.276744604110718
		0.269351005554199 -0.280841112136841
		0.278572082519531 -0.285514116287231
		0.299405097961426 -0.296522855758667
		0.312143325805664 -0.302227258682251
		0.325217247009277 -0.307610750198364
		0.337949275970459 -0.312054872512817
		0.349468231201172 -0.314567089080811
		0.360532760620117 -0.314177513122559
		0.370200634002686 -0.311247825622559
		0.378127574920654 -0.305584669113159
		0.383511066436768 -0.298526525497437
		0.387265682220459 -0.290677785873413
		0.387244701385498 -0.282173871994019
		0.386185169219971 -0.274831771850586
		0.384037017822266 -0.267829895019531
		0.382267951965332 -0.262994050979614
		0.380838871002197 -0.26068377494812
		0.377907752990723 -0.260178804397583
		0.375614643096924 -0.261584997177124
		0.369502544403076 -0.262701034545898
		0.365026473999023 -0.264458417892456
		0.356003761291504 -0.269674301147461
		0.345454216003418 -0.275667905807495
		0.333970546722412 -0.282252550125122
		0.321840286254883 -0.289541006088257
		0.309884548187256 -0.297092914581299
		0.299385547637939 -0.303168773651123
		0.290313243865967 -0.307686567306519
		0.281789302825928 -0.311065435409546
		0.273219108581543 -0.314868688583374
		0.262310981750488 -0.318504095077515
		0.251391410827637 -0.321002721786499
		0.240737438201904 -0.320741415023804
		0.232179164886475 -0.317836046218872
		0.227717399597168 -0.312403202056885
		0.230002403259277 -0.305433750152588
		0.254036903381348 -0.293991088867188
		0.277008533477783 -0.289056777954102
		0.304621696472168 -0.281209468841553
		0.334768295288086 -0.269120216369629
		0.363463401794434 -0.254126071929932
		0.387835502624512 -0.239358186721802
		0.405727386474609 -0.224400281906128
		0.417745590209961 -0.209673881530762
		0.423427104949951 -0.195384502410889
		0.423691749572754 -0.181973695755005
		0.418605327606201 -0.169075489044189
		0.411143779754639 -0.156472206115723
		0.404132843017578 -0.145740747451782
		0.39979076385498 -0.138320684432983
		0.397964477539062 -0.134185075759888
		0.399243354797363 -0.131262063980103
		0.404416561126709 -0.129144191741943
		0.419278621673584 -0.129027843475342
		0.4277024269104 -0.130073308944702
		0.438353538513184 -0.130678176879883
		0.44916296005249 -0.130324602127075
		0.461356163024902 -0.129501819610596
		0.474164485931396 -0.128871440887451
		0.486894130706787 -0.12805962562561
		0.500238418579102 -0.126250028610229
		0.512677192687988 -0.124185800552368
		0.524662494659424 -0.121276378631592
		0.534428596496582 -0.117805957794189
		0.54300594329834 -0.114422082901001
		0.549008369445801 -0.110936403274536
		0.552371501922607 -0.107539653778076
		0.5541090965271 -0.104978322982788
		0.553494453430176 -0.103536367416382
		0.551347255706787 -0.102737665176392
		0.545073986053467 -0.100511789321899
		0.541100978851318 -0.0985555648803711
		0.537099838256836 -0.0961718559265137
		0.532195091247559 -0.0950329303741455
		0.52634859085083 -0.0966095924377441
		0.519018173217773 -0.100193738937378
		0.5101318359375 -0.104804039001465
		0.500622272491455 -0.109034299850464
		0.491445541381836 -0.112497329711914
		0.482985019683838 -0.115975856781006
		0.472667217254639 -0.11888575553894
		0.462184429168701 -0.122554779052734
		0.454413890838623 -0.126400232315063
		0.44776725769043 -0.131272554397583
		0.442382335662842 -0.13599681854248
		0.437877655029297 -0.139255046844482
		0.433121204376221 -0.142088890075684
		0.422080993652344 -0.145957469940186
		0.416577816009521 -0.14663553237915
		0.410492897033691 -0.146164178848267
		0.404528141021729 -0.144514083862305
		0.398483753204346 -0.140771865844727
		0.393879890441895 -0.134054660797119
		0.391788482666016 -0.12442946434021
		0.395020008087158 -0.110282897949219
		0.404316425323486 -0.0924298763275146
		0.419227600097656 -0.0730030536651611
		0.436414241790771 -0.0524382591247559
		0.452496528625488 -0.0307762622833252
		0.46465015411377 -0.00885963439941406
		0.470919132232666 0.0118618011474609
		0.471738338470459 0.0295846462249756
		0.468568325042725 0.0439534187316895
		0.461705207824707 0.0554640293121338
		0.443526268005371 0.0710468292236328
		0.434700489044189 0.0755090713500977
		0.426765441894531 0.0782167911529541
		0.421051502227783 0.0801191329956055
		0.418045043945312 0.0824100971221924
		0.417571544647217 0.0852377414703369
		0.419477462768555 0.0878434181213379
		0.423949241638184 0.091031551361084
		0.430417537689209 0.0950090885162354
		0.437716960906982 0.0991506576538086
		0.445755004882812 0.103963375091553
		0.454879760742188 0.110303163528442
		0.463923454284668 0.117713212966919
		0.472463130950928 0.125356197357178
		0.481566429138184 0.133115768432617
		0.489361763000488 0.140381574630737
		0.495473861694336 0.146354675292969
		0.501782417297363 0.152403593063354
		0.49962043762207 0.150851488113403
		0.495697975158691 0.146430969238281
		0.491469860076904 0.140134811401367
		0.486589908599854 0.132877826690674
		0.481780052185059 0.122764825820923
		0.477402210235596 0.109484434127808
		0.473172664642334 0.094106912612915
		0.468643188476562 0.0785017013549805
		0.464509010314941 0.0630860328674316
		0.459725379943848 0.0476391315460205
		0.453319549560547 0.0324914455413818
		0.445653915405273 0.0188322067260742
		0.438377857208252 0.00649428367614746
		0.429794788360596 -0.00443434715270996
		0.421534538269043 -0.0143640041351318
		0.414921283721924 -0.0219359397888184
		0.397269725799561 -0.0303847789764404
		0.384975433349609 -0.0333311557769775
		0.370035648345947 -0.0354053974151611
		0.352634906768799 -0.0358033180236816
		0.332738876342773 -0.0347392559051514
		0.310945987701416 -0.0302491188049316
		0.28757381439209 -0.0235538482666016
		0.263988971710205 -0.0162003040313721
		0.241765022277832 -0.00849199295043945
		0.221742630004883 0.000783681869506836
		0.20318078994751 0.0102345943450928
		0.186397075653076 0.0195605754852295
		0.174269199371338 0.0289134979248047
		0.166467189788818 0.0388715267181396
		0.161996364593506 0.0489127635955811
		0.163612842559814 0.0599124431610107
		0.16918420791626 0.072174072265625
		0.188727855682373 0.101404428482056
		0.202877521514893 0.11634373664856
		0.217136859893799 0.129003763198853
		0.229912757873535 0.138884782791138
		0.242195129394531 0.14531397819519
		0.253225803375244 0.150682210922241
		0.262510776519775 0.155666828155518
		0.271790981292725 0.160313367843628
		0.281164169311523 0.163785696029663
		0.2886061668396 0.165462255477905
		0.294008731842041 0.16591739654541
		0.299050807952881 0.166698217391968
		0.302873134613037 0.166089057922363
		0.304895401000977 0.165116310119629
		0.305915832519531 0.163655757904053
		0.306830406188965 0.161288738250732
		0.308081150054932 0.158243179321289
		0.31202220916748 0.149340391159058
		0.314437389373779 0.144694089889526
		0.317511081695557 0.14007830619812
		0.320812225341797 0.134567975997925
		0.323647022247314 0.128568172454834
		0.324954986572266 0.122252702713013
		0.325276374816895 0.116429567337036
		0.324569702148438 0.110835313796997
		0.323738098144531 0.106825113296509
		0.323533058166504 0.103705883026123
		0.324018001556396 0.100380659103394
		0.324975967407227 0.0959620475769043
		0.326784610748291 0.0914826393127441
		0.328701496124268 0.0866022109985352
		0.331665992736816 0.0813596248626709
		0.335169315338135 0.0750961303710938
		0.33757209777832 0.0675766468048096
		0.338962078094482 0.0467574596405029
		0.336756706237793 0.0345120429992676
		0.332902908325195 0.0206060409545898
		0.328428745269775 0.00525093078613281
		0.323375225067139 -0.0104110240936279
		0.316117763519287 -0.0274648666381836
		0.309474468231201 -0.0437572002410889
		0.300365924835205 -0.0597870349884033
		0.290976524353027 -0.0738968849182129
		0.282667636871338 -0.086742639541626
		0.274199485778809 -0.0984318256378174
		0.265737056732178 -0.109603643417358
		0.257789611816406 -0.118470430374146
		0.24982213973999 -0.125035762786865
		0.242022037506104 -0.130192041397095
		0.233880043029785 -0.133731603622437
		0.224735736846924 -0.13561224937439
		0.207808971405029 -0.134838581085205
		0.19872522354126 -0.133257627487183
		0.190921306610107 -0.129929780960083
		0.185051441192627 -0.124285697937012
		0.180243492126465 -0.118795871734619
		0.177026271820068 -0.114239692687988
		0.174826622009277 -0.110117673873901
		0.172225475311279 -0.107481002807617
		0.169949054718018 -0.105882883071899
		0.167011737823486 -0.105079889297485
		0.163503646850586 -0.105352878570557
		0.161638259887695 -0.106391429901123
		0.165784358978271 -0.108232021331787
		0.174703121185303 -0.112935066223145
		0.185089111328125 -0.119543313980103
		0.196276187896729 -0.125423431396484
		0.206334114074707 -0.130500316619873
		0.215018749237061 -0.144342184066772
		0.213131904602051 -0.15262770652771
		0.205775737762451 -0.162504434585571
		0.193562507629395 -0.173283576965332
		0.177497386932373 -0.186003684997559
		0.156392097473145 -0.200410604476929
		0.134032249450684 -0.214765548706055
		0.111944198608398 -0.226467847824097
		0.0898861885070801 -0.23592472076416
		0.0696063041687012 -0.242912769317627
		0.0492334365844727 -0.247467041015625
		0.0171055793762207 -0.252387285232544
		0.00430774688720703 -0.252336740493774
		-0.00622081756591797 -0.252688646316528
		-0.0151019096374512 -0.252621173858643
		-0.0218172073364258 -0.252825736999512
		-0.027043342590332 -0.253784418106079
		-0.0339865684509277 -0.25594425201416
		-0.0364909172058105 -0.257465362548828
		-0.0377192497253418 -0.259146213531494
		-0.0388088226318359 -0.259784460067749
		-0.0404534339904785 -0.26132607460022
		-0.043067455291748 -0.263568639755249
		-0.0425143241882324 -0.259778022766113
		-0.047370433807373 -0.262283563613892
		-0.0481181144714355 -0.252684116363525
		-0.0519828796386719 -0.247211456298828
		-0.0547966957092285 -0.241640329360962
		-0.0590348243713379 -0.232613563537598
		-0.066317081451416 -0.223186731338501
		-0.0749993324279785 -0.210277080535889
		-0.0873661041259766 -0.197201490402222
		-0.102601528167725 -0.180588960647583
		-0.120834350585938 -0.161726474761963
		-0.161011219024658 -0.118717193603516
		-0.182309627532959 -0.0955238342285156
		-0.203787803649902 -0.0707340240478516
		-0.221941471099854 -0.0440220832824707
		-0.247904300689697 0.000123023986816406
		-0.257389068603516 0.0181052684783936
		-0.265834331512451 0.0338494777679443
		-0.274196147918701 0.0470576286315918
		-0.283370971679688 0.0562930107116699
		-0.290090084075928 0.0641119480133057
		-0.297959566116333 0.0692861080169678
		-0.30614447593689 0.074479341506958
		-0.313383817672729 0.0778217315673828
		-0.321587085723877 0.0794146060943604
		-0.329018592834473 0.0806443691253662
		-0.336623191833496 0.0792453289031982
		-0.344444990158081 0.0784447193145752
		-0.358558416366577 0.0796604156494141
		-0.365620374679565 0.0820145606994629
		-0.372202396392822 0.085338830947876
		-0.378693819046021 0.0917680263519287
		-0.384901285171509 0.101403474807739
		-0.391800880432129 0.113877296447754
		-0.398156881332397 0.12794041633606
		-0.405303239822388 0.144651651382446
		-0.413211822509766 0.163980007171631
		-0.422950029373169 0.186177492141724
		-0.432249546051025 0.20915699005127
		-0.443677663803101 0.234650373458862
		-0.455579280853271 0.261464357376099
		-0.4680495262146 0.288782358169556
		-0.480740547180176 0.316969394683838
		-0.494502782821655 0.343819618225098
		-0.506997585296631 0.369302988052368
		-0.532356739044189 0.41681981086731
		-0.542201995849609 0.43903374671936
		-0.548934698104858 0.460180521011353
		-0.552461862564087 0.478749513626099
		-0.554431676864624 0.494734525680542
		-0.554164409637451 0.508585214614868
		-0.551351070404053 0.52018404006958
		-0.546444892883301 0.530516386032104
		-0.540326118469238 0.538650989532471
		-0.533962488174438 0.54590106010437
		-0.528228521347046 0.5516517162323
		-0.523319005966187 0.556171655654907
		-0.51875901222229 0.559774875640869
		-0.514635801315308 0.563307762145996
		-0.51225209236145 0.567486763000488
		-0.511198759078979 0.572057485580444
		-0.509496688842773 0.57818603515625
		-0.50188136100769 0.597802400588989
		-0.496378183364868 0.610551357269287
		-0.49030065536499 0.625753879547119
		-0.483154535293579 0.642142057418823
		-0.473594903945923 0.660194158554077
		-0.462607622146606 0.679688215255737
		-0.450906038284302 0.700359106063843
		-0.438165664672852 0.722132682800293
		-0.423839330673218 0.745080947875977
		-0.409336566925049 0.768850803375244
		-0.392941474914551 0.79328727722168
		-0.377383232116699 0.81843090057373
		-0.359654188156128 0.843892097473145
		-0.341591835021973 0.868237257003784
		-0.323523998260498 0.890495538711548
		-0.306995868682861 0.910418510437012
		-0.288999557495117 0.928917646408081
		-0.250134468078613 0.960476398468018
		-0.229742050170898 0.973967552185059
		-0.208060264587402 0.985514402389526
		-0.185215473175049 0.994890213012695
		-0.160974502563477 1.00202345848083
		-0.135478496551514 1.00649857521057
		-0.108591079711914 1.00827670097351
		-0.0816740989685059 1.00731587409973
		-0.0534162521362305 1.00445103645325
		-0.0238981246948242 1.00028848648071
		0.00528669357299805 0.995312213897705
		0.0342493057250977 0.98904275894165
		0.0632443428039551 0.982847452163696
		0.0929851531982422 0.9762122631073
		0.123081207275391 0.969633340835571
		0.153232574462891 0.962374210357666
		0.183555126190186 0.955987691879272
		0.242154598236084 0.942861557006836
		0.270921230316162 0.934135675430298
		0.298911094665527 0.924891710281372
		0.324925899505615 0.916084051132202
		0.352818965911865 0.90650749206543
		0.38033390045166 0.897371292114258
		0.408624649047852 0.888093948364258
		0.437955379486084 0.877878904342651
		0.468069553375244 0.866084337234497
		0.498217582702637 0.852882146835327
		0.528214454650879 0.838371992111206
		0.558545112609863 0.821885108947754
		0.587999820709229 0.803868293762207
		0.617506980895996 0.783855676651001
		0.647718906402588 0.761553049087524
		0.674814224243164 0.738767623901367
		0.701378345489502 0.713350772857666
		0.745468616485596 0.664853811264038
		0.765552043914795 0.639255285263062
		0.78288459777832 0.613598823547363
		0.79861307144165 0.587558031082153
		0.813061237335205 0.560839176177979
		0.826841831207275 0.532722473144531
		0.839196681976318 0.503191232681274
		0.848245143890381 0.471790313720703
		0.854654788970947 0.440048933029175
		0.859573364257812 0.407224178314209
		0.863399505615234 0.373703002929688
		0.864762783050537 0.340895652770996
		0.864442348480225 0.308376550674438
		0.862275123596191 0.277302742004395
		0.858223915100098 0.248275756835938
		0.853150844573975 0.220256805419922
		0.847230434417725 0.192909955978394
		0.835236549377441 0.14272141456604
		0.828899383544922 0.119407176971436
		0.822700500488281 0.0958201885223389
		0.816460609436035 0.0714199542999268
		0.810808181762695 0.0473392009735107
		0.805733203887939 0.0222983360290527
		0.800402164459229 -0.00338029861450195
		0.794578075408936 -0.0295500755310059
		0.788138389587402 -0.055478572845459
		0.78176736831665 -0.0832867622375488
		0.774805068969727 -0.112417221069336
		0.767723083496094 -0.143109083175659
		0.760618209838867 -0.17512321472168
		0.7532639503479 -0.21000075340271
		0.745965003967285 -0.245792388916016
		0.738360404968262 -0.282887935638428
		0.730146884918213 -0.320350885391235
		0.710628986358643 -0.394152402877808
		0.698646068572998 -0.428880214691162
		0.657362937927246 -0.521860361099243
		0.64145040512085 -0.549778461456299
		0.624608993530273 -0.575902700424194
		0.607239723205566 -0.599847197532654
		0.588366508483887 -0.622284770011902
		0.568402290344238 -0.643708944320679
		0.547265529632568 -0.663846254348755
		0.52375602722168 -0.684187531471252
		0.499780654907227 -0.702359557151794
		0.473758697509766 -0.720627427101135
		0.446412563323975 -0.737960815429688
		0.417838573455811 -0.754318952560425
		0.388992309570312 -0.769166707992554
		0.359073162078857 -0.782992005348206
		0.329636573791504 -0.796103477478027
		0.271152019500732 -0.822140336036682
		0.243062019348145 -0.833965659141541
		0.21561336517334 -0.844884872436523
		0.187674522399902 -0.855868101119995
		0.158923625946045 -0.866855978965759
		0.131221294403076 -0.87742805480957
		0.102925777435303 -0.88866662979126
		0.0739636421203613 -0.899849891662598
		0.0439496040344238 -0.91117250919342
		0.0129146575927734 -0.922146797180176
		-0.0196795463562012 -0.933053135871887
		-0.0537261962890625 -0.942923069000244
		-0.0897884368896484 -0.951091289520264
		-0.127527236938477 -0.957845568656921
		-0.166604042053223 -0.962430953979492
		-0.206568717956543 -0.965288281440735
		-0.247217178344727 -0.96538507938385
		-0.329178333282471 -0.958763957023621
		-0.368557453155518 -0.950914263725281
		-0.405108451843262 -0.939173340797424
		-0.440417528152466 -0.923030614852905
		-0.473879098892212 -0.902953028678894
		-0.503445386886597 -0.880014181137085
		-0.529167890548706 -0.855117559432983
		-0.551555395126343 -0.82848048210144
		-0.569809436798096 -0.800993800163269
		-0.586248874664307 -0.773085951805115
		-0.597811222076416 -0.744176626205444
		-0.607747077941895 -0.716200709342957
		-0.613790035247803 -0.686839938163757
		-0.618688106536865 -0.655681967735291
		-0.620568752288818 -0.624021172523499
		-0.618654489517212 -0.592276453971863
		-0.615419149398804 -0.559221982955933
		0.177433013916016 0.0861220359802246
		0.309604167938232 0.15399956703186
		0.339141845703125 0.0583400726318359
		0.216389179229736 -0.13598895072937
		0.212870121002197 -0.137587070465088
		-0.0312280654907227 -0.254820346832275
		-0.140756607055664 -0.140568494796753
		-0.351674556732178 0.0785534381866455
		-0.519889354705811 0.393232107162476
		-0.506192207336426 0.586934089660645
		-0.269911766052246 0.945492267608643
		0.212356090545654 0.95012640953064
		0.724745273590088 0.688522338867188
		0.841421127319336 0.166541576385498
		0.721342086791992 -0.357373952865601
		0.300580978393555 -0.809238791465759
		-0.610964775085449 -0.489260673522949
		-0.607926607131958 -0.455189228057861
		-0.603689908981323 -0.422123908996582
		-0.599552392959595 -0.389879941940308
		-0.59548020362854 -0.357625722885132
		-0.592183589935303 -0.325899124145508
		-0.589895963668823 -0.295116424560547
		-0.588583946228027 -0.265467882156372
		-0.587278604507446 -0.238084316253662
		-0.586090326309204 -0.21272873878479
		-0.586262941360474 -0.188371419906616
		-0.587850332260132 -0.164679765701294
		-0.590389251708984 -0.143239736557007
		-0.594301700592041 -0.126609563827515
		-0.599139928817749 -0.113186597824097
		-0.605550527572632 -0.101835489273071
		-0.613922595977783 -0.0925326347351074
		-0.634068727493286 -0.0717589855194092
		-0.644924640655518 -0.0614001750946045
		-0.656250238418579 -0.0506665706634521
		-0.668896198272705 -0.0389750003814697
		-0.680670022964478 -0.0275671482086182
		-0.691154718399048 -0.0174288749694824
		-0.701662063598633 -0.00787973403930664
		-0.710356950759888 -0.00017857551574707
		-0.719061374664307 0.00759434700012207
		-0.725793123245239 0.0149052143096924
		-0.731291055679321 0.022099494934082
		-0.738020896911621 0.0284197330474854
		-0.74286413192749 0.0360815525054932
		-0.747014999389648 0.0455987453460693
		-0.750281095504761 0.0568203926086426
		-0.75363826751709 0.0686643123626709
		-0.756863832473755 0.0817265510559082
		-0.761823654174805 0.114290237426758
		-0.763055801391602 0.133702993392944
		-0.764393329620361 0.1537766456604
		-0.766040086746216 0.172672748565674
		-0.767355442047119 0.190469980239868
		-0.769161701202393 0.20570707321167
		-0.771661281585693 0.219291925430298
		-0.774086236953735 0.231238126754761
		-0.7765212059021 0.241647243499756
		-0.779036998748779 0.249555110931396
		-0.780534505844116 0.255419015884399
		-0.781241893768311 0.257972717285156
		-0.780497074127197 0.25778603553772
		-0.778975248336792 0.253654003143311
		-0.775996446609497 0.246142864227295
		-0.77303147315979 0.235913991928101
		-0.769604206085205 0.222410202026367
		-0.761847734451294 0.187525749206543
		-0.757518768310547 0.167120695114136
		-0.753512382507324 0.144575119018555
		-0.750282049179077 0.120208501815796
		-0.747298002243042 0.0944588184356689
		-0.743875026702881 0.0675256252288818
		-0.740626335144043 0.0398380756378174
		-0.736815214157104 0.01287841796875
		-0.731963157653809 -0.011357307434082
		-0.725107669830322 -0.0335919857025146
		-0.717881917953491 -0.0545296669006348
		-0.7103271484375 -0.0755658149719238
		-0.701545476913452 -0.0947704315185547
		-0.691472053527832 -0.111368894577026
		-0.680073499679565 -0.125797510147095
		-0.667577505111694 -0.137928247451782
		-0.652133226394653 -0.149919748306274
		-0.617653131484985 -0.171041250228882
		-0.598726034164429 -0.180262565612793
		-0.578066349029541 -0.190841913223267
		-0.555577516555786 -0.201057434082031
		-0.509512424468994 -0.220014095306396
		-0.485393285751343 -0.229013204574585
		-0.460012674331665 -0.238246440887451
		-0.4352867603302 -0.248354911804199
		-0.41011905670166 -0.258070468902588
		-0.384690999984741 -0.267657279968262
		-0.359653949737549 -0.276645183563232
		-0.335649013519287 -0.286207675933838
		-0.31182599067688 -0.29650354385376
		-0.289180755615234 -0.307836294174194
		-0.267637729644775 -0.320336818695068
		-0.24760103225708 -0.33472752571106
		-0.22847318649292 -0.349688053131104
		-0.19361686706543 -0.379155158996582
		-0.176737785339355 -0.393926382064819
		-0.158020496368408 -0.406778335571289
		-0.138083934783936 -0.417801856994629
		-0.119011878967285 -0.426871776580811
		-0.101283550262451 -0.434321641921997
		-0.084444522857666 -0.43945050239563
		-0.0684695243835449 -0.441160678863525
		-0.0525670051574707 -0.440855979919434
		-0.0359859466552734 -0.438445329666138
		-0.0187258720397949 -0.433384656906128
		-0.00103235244750977 -0.426134347915649
		0.0175786018371582 -0.416799068450928
		0.0368180274963379 -0.40570592880249
		0.0562801361083984 -0.393829107284546
		0.0756058692932129 -0.380057334899902
		0.0935158729553223 -0.366219997406006
		0.127132415771484 -0.337311029434204
		0.144192695617676 -0.321071624755859
		0.159880638122559 -0.302901744842529
		0.17364501953125 -0.283389329910278
		0.187992095947266 -0.262850522994995
		0.203932762145996 -0.241878032684326
		0.221642017364502 -0.219441890716553
		0.240053653717041 -0.195604085922241
		0.259304046630859 -0.171033143997192
		0.278057098388672 -0.145843029022217
		0.296329498291016 -0.119817972183228
		0.314387798309326 -0.0946147441864014
		0.330929279327393 -0.0687880516052246
		0.346407890319824 -0.0420989990234375
		0.361673355102539 -0.0143969058990479
		0.376054763793945 0.0138068199157715
		0.387606620788574 0.0414309501647949
		0.405519008636475 0.0884754657745361
		0.415902614593506 0.132177591323853
		0.416234493255615 0.151044845581055
		0.41546106338501 0.170459747314453
		0.394092082977295 0.260523319244385
		0.386957168579102 0.277479410171509
		0.380415439605713 0.294589281082153
		0.376338005065918 0.313321590423584
		0.372751235961914 0.332738637924194
		0.366763591766357 0.351131200790405
		0.358230113983154 0.367668390274048
		0.350014209747314 0.384257793426514
		0.340785503387451 0.401687145233154
		0.331520557403564 0.420798301696777
		0.323375701904297 0.441179037094116
		0.310941219329834 0.482294082641602
		0.308172702789307 0.502575397491455
		0.310308456420898 0.546392917633057
		0.311174392700195 0.568055868148804
		0.313054084777832 0.590389490127563
		0.314286708831787 0.612309217453003
		0.349265575408936 0.737952947616577
		-0.0771465301513672 0.892141580581665
		-0.103035926818848 0.898790597915649
		-0.127203941345215 0.904443979263306
		-0.152550220489502 0.909306049346924
		-0.177211761474609 0.913433074951172
		-0.199509143829346 0.915637254714966
		-0.22012996673584 0.915960550308228
		-0.239708423614502 0.914646625518799
		-0.257837295532227 0.913088321685791
		-0.275170803070068 0.910592794418335
		-0.291835784912109 0.905678749084473
		-0.307930946350098 0.899218320846558
		-0.339160203933716 0.884451150894165
		-0.35645604133606 0.877817630767822
		-0.374419689178467 0.872951984405518
		-0.39461612701416 0.867832660675049
		-0.413528680801392 0.863002300262451
		-0.434149026870728 0.858445167541504
		-0.454180955886841 0.855116605758667
		-0.474398612976074 0.850518226623535
		-0.495420932769775 0.84687876701355
		-0.519164323806763 0.843543529510498
		-0.545945405960083 0.841277599334717
		-0.573398351669312 0.839277029037476
		-0.640521287918091 0.839683055877686
		-0.675939798355103 0.841784715652466
		-0.711319923400879 0.844024896621704
		-0.745542287826538 0.845655918121338
		-0.77782940864563 0.847686767578125
		-0.835324048995972 0.848407745361328
		-0.861037731170654 0.84616494178772
		-0.884045362472534 0.84143590927124
		-0.905376434326172 0.835734367370605
		-0.924411058425903 0.82956337928772
		-0.943338871002197 0.822526931762695
		-0.959426403045654 0.81410551071167
		-0.974107503890991 0.80456280708313
		-0.987156391143799 0.793249130249023
		-1.00044560432434 0.78156590461731
		-1.01171278953552 0.767951488494873
		-1.03103733062744 0.736908674240112
		-1.03818464279175 0.719378709793091
		-1.04438638687134 0.699389934539795
		-1.05596685409546 0.655285835266113
		-1.06922245025635 0.579573392868042
		-1.07759428024292 0.553168773651123
		-1.09551954269409 0.498144865036011
		-1.10556650161743 0.470243215560913
		-1.11692070960999 0.443197011947632
		-1.12974572181702 0.417119026184082
		-1.14465951919556 0.391692399978638
		-1.16202735900879 0.367180347442627
		-1.1812846660614 0.343663454055786
		-1.2021279335022 0.320536375045776
		-1.2240252494812 0.297778129577637
		-1.24555158615112 0.275411128997803
		-1.26656818389893 0.253067493438721
		-1.28825283050537 0.23053240776062
		-1.30957126617432 0.20690131187439
		-1.32879257202148 0.183419704437256
		-1.34500527381897 0.160382032394409
		-1.35969018936157 0.138440370559692
		-1.37283277511597 0.117492437362671
		-1.393630027771 0.077899694442749
		-1.40196681022644 0.059185266494751
		-1.40856981277466 0.0402343273162842
		-1.41422247886658 0.0213611125946045
		-1.41884565353394 0.00356006622314453
		-1.42154002189636 -0.0142605304718018
		-1.42318940162659 -0.0323963165283203
		-1.42367458343506 -0.0511415004730225
		-1.42362236976624 -0.0703063011169434
		-1.42239260673523 -0.0912046432495117
		-1.41909909248352 -0.112357616424561
		-1.41440534591675 -0.134867906570435
		-1.4093804359436 -0.158769130706787
		-1.40293455123901 -0.184844255447388
		-1.39639210700989 -0.212805509567261
		-1.38781332969666 -0.27105450630188
		-1.38315677642822 -0.300517559051514
		-1.37339043617249 -0.360459327697754
		-1.36982464790344 -0.392401456832886
		-1.36742043495178 -0.424032926559448
		-1.36534738540649 -0.45495080947876
		-1.36543130874634 -0.485974550247192
		-1.36722660064697 -0.516673803329468
		-1.37010622024536 -0.54721212387085
		-1.37366080284119 -0.577129364013672
		-1.37686896324158 -0.604763627052307
		-1.37926173210144 -0.631255626678467
		-1.38275146484375 -0.655606508255005
		-1.38498687744141 -0.680518627166748
		-1.38651609420776 -0.705329537391663
		-1.38539028167725 -0.729177355766296
		-1.3840913772583 -0.751536726951599
		-1.38346815109253 -0.772741556167603
		-1.38135361671448 -0.79314661026001
		-1.37165331840515 -0.83073103427887
		-1.36466312408447 -0.849750399589539
		-1.35562539100647 -0.869269132614136
		-1.34518647193909 -0.889382719993591
		-1.33293962478638 -0.909808278083801
		-1.3187940120697 -0.930265307426453
		-1.30283188819885 -0.951046228408813
		-1.28592348098755 -0.971583247184753
		-1.26674222946167 -0.991960883140564
		-1.2476954460144 -1.01371097564697
		-1.22875738143921 -1.03751075267792
		-1.20744609832764 -1.06155121326447
		-1.18541169166565 -1.0843790769577
		-1.16442084312439 -1.10666763782501
		-1.1441810131073 -1.1282547712326
		-1.12445902824402 -1.14823436737061
		-1.10490369796753 -1.16666042804718
		-1.06659197807312 -1.20172131061554
		-1.04832196235657 -1.21831595897675
		-1.03042697906494 -1.2346156835556
		-1.01287293434143 -1.25140452384949
		-0.996163845062256 -1.26929199695587
		-0.980551719665527 -1.28842079639435
		-0.965555429458618 -1.30863332748413
		-0.950004816055298 -1.32948160171509
		-0.934775829315186 -1.34865164756775
		-0.919826745986938 -1.36704313755035
		-0.904102802276611 -1.38577842712402
		-0.886617422103882 -1.40567374229431
		-0.867335319519043 -1.42653572559357
		-0.847383499145508 -1.44705355167389
		-0.828514337539673 -1.46608257293701
		-0.811046838760376 -1.48377859592438
		-0.794135570526123 -1.50002300739288
		-0.759332180023193 -1.52780890464783
		-0.741383790969849 -1.53920316696167
		-0.723081350326538 -1.54952669143677
		-0.703518390655518 -1.55907297134399
		-0.682607173919678 -1.56704163551331
		-0.660017967224121 -1.57362425327301
		-0.636722564697266 -1.57851707935333
		-0.612234354019165 -1.58195179700851
		-0.586457014083862 -1.58453363180161
		-0.560209989547729 -1.58753657341003
		-0.533539056777954 -1.59100604057312
		-0.505252361297607 -1.59477227926254
		-0.477203845977783 -1.59917253255844
		-0.449627161026001 -1.60420197248459
		-0.422936201095581 -1.60877197980881
		-0.396540403366089 -1.61306059360504
		-0.369686603546143 -1.61795848608017
		-0.612901210784912 -0.524705648422241
		-0.623639106750488 -0.0827333927154541
		-0.759415864944458 0.0969486236572266
		-0.765902757644653 0.206015110015869
		-0.635656118392944 -0.160703897476196
		-0.210632801055908 -0.364865303039551
		0.110140800476074 -0.352065324783325
		0.397636890411377 0.0663933753967285
		0.308783054351807 0.524256467819214
		-0.323544025421143 0.891928434371948
		-0.807354927062988 0.848468542098999
		-1.08566737174988 0.525724649429321
		-1.3844850063324 0.0970406532287598
		-1.37774538993835 -0.330165386199951
		-1.37803649902344 -0.811916351318359
		-1.08558082580566 -1.1844310760498
		-0.311478137969971 -1.62600874900818
		-0.281677722930908 -1.62950885295868
		-0.251367568969727 -1.63237982988358
		-0.220885276794434 -1.63472723960876
		-0.189516544342041 -1.63752090930939
		-0.157893180847168 -1.64131784439087
		-0.126617908477783 -1.64587354660034
		-0.0958166122436523 -1.65038418769836
		-0.0655584335327148 -1.65478658676147
		-0.0352721214294434 -1.65827614068985
		-0.00374841690063477 -1.66158729791641
		0.0277552604675293 -1.66481399536133
		0.0580167770385742 -1.66786795854568
		0.0863537788391113 -1.6704740524292
		0.113113880157471 -1.67180967330933
		0.138965129852295 -1.67214679718018
		0.164598941802979 -1.6712287068367
		0.223477363586426 -1.66731441020966
		0.253528594970703 -1.66237789392471
		0.406907081604004 -1.61055964231491
		0.438739776611328 -1.59540581703186
		0.470752239227295 -1.57963824272156
		0.503418445587158 -1.5646425485611
		0.537535667419434 -1.54839432239532
		0.769270420074463 -1.4526686668396
		0.803145885467529 -1.44112813472748
		0.834123134613037 -1.42723560333252
		0.956114768981934 -1.38370990753174
		0.983589172363281 -1.3732922077179
		1.00933218002319 -1.36105251312256
		1.06125926971436 -1.33309471607208
		1.6235203742981 -0.428878784179688
		1.63295316696167 -0.404431819915771
		1.64113235473633 -0.379792451858521
		1.65468120574951 -0.328134059906006
		1.66056871414185 -0.300351619720459
		1.66580820083618 -0.270761489868164
		1.66995620727539 -0.239458084106445
		1.673424243927 -0.207259893417358
		1.67653131484985 -0.173421382904053
		1.67898845672607 -0.138564586639404
		1.68178701400757 -0.103179454803467
		1.68339967727661 -0.0660345554351807
		1.68313074111938 -0.0278937816619873
		1.68244743347168 0.00902271270751953
		1.68320274353027 0.0454325675964355
		1.68390274047852 0.0835318565368652
		1.68568277359009 0.121679782867432
		1.68696022033691 0.159290313720703
		1.68765687942505 0.196160793304443
		1.68779277801514 0.232713460922241
		1.68615627288818 0.305814981460571
		1.68452787399292 0.34220814704895
		1.68253469467163 0.378530740737915
		1.6795597076416 0.414657115936279
		1.67606544494629 0.450713634490967
		1.67270469665527 0.485814809799194
		1.66941547393799 0.519673347473145
		1.66573524475098 0.551533222198486
		1.66047954559326 0.580873727798462
		1.6543402671814 0.607470750808716
		1.64925527572632 0.631947994232178
		1.64482069015503 0.657304525375366
		1.6411190032959 0.681826591491699
		1.63750839233398 0.704970359802246
		1.62708473205566 0.747475147247314
		1.62175941467285 0.769228935241699
		1.61561012268066 0.790820837020874
		1.60143327713013 0.839084148406982
		1.59309577941895 0.865492820739746
		1.58275413513184 0.891013383865356
		1.57043600082397 0.917715311050415
		1.52076721191406 1.00522422790527
		1.48705148696899 1.06638813018799
		1.42788887023926 1.17068076133728
		1.40828990936279 1.20570063591003
		1.38775205612183 1.24042820930481
		1.34559392929077 1.31070899963379
		1.30250549316406 1.38341999053955
		1.28173542022705 1.42011833190918
		1.24328088760376 1.49331617355347
		1.22635650634766 1.52858471870422
		1.21079301834106 1.56264567375183
		0.279900550842285 2.31785464286804
		0.254583835601807 2.32567501068115
		0.206756114959717 2.34287858009338
		0.15880823135376 2.36259603500366
		0.135116100311279 2.36922979354858
		0.111289978027344 2.37606930732727
		0.0618014335632324 2.38764262199402
		-0.150369644165039 2.38737654685974
		-0.310161352157593 2.3532121181488
		-0.340095996856689 2.34732604026794
		-0.399203300476074 2.33772802352905
		-0.42923641204834 2.33288931846619
		-0.459766626358032 2.32752871513367
		-0.490379810333252 2.3218207359314
		-0.522181987762451 2.31597566604614
		-0.55480432510376 2.30905413627625
		-0.58782958984375 2.30206775665283
		-0.621176242828369 2.29491662979126
		-0.654132127761841 2.28933238983154
		-0.687326192855835 2.2845151424408
		-0.720879793167114 2.27963376045227
		-0.753679513931274 2.27425670623779
		-0.783764362335205 2.2681782245636
		-0.81511116027832 2.26283931732178
		-0.84791111946106 2.25803565979004
		-0.882334232330322 2.25269794464111
		-0.916018009185791 2.24679350852966
		-0.981632709503174 2.23131442070007
		-1.00900077819824 2.22099757194519
		-1.03934240341187 2.21077513694763
		-1.07042169570923 2.19663023948669
		-1.10250520706177 2.1812105178833
		-1.13425517082214 2.1641538143158
		-1.16610765457153 2.14611482620239
		-1.19898819923401 2.12581825256348
		-1.23128485679626 2.10582566261292
		-1.26612114906311 2.08402228355408
		-1.29942989349365 2.06244111061096
		-1.33362197875977 2.04235982894897
		-1.36534929275513 2.02273631095886
		-1.40055131912231 2.00250387191772
		-1.4348201751709 1.98262286186218
		-1.46832084655762 1.96368837356567
		-1.5029878616333 1.94602727890015
		-1.57450652122498 1.91064715385437
		-1.6095929145813 1.89277267456055
		-1.64395570755005 1.87572932243347
		-1.67663216590881 1.85897159576416
		-1.70660948753357 1.84299373626709
		-1.73975443840027 1.82700753211975
		-1.77373862266541 1.8108856678009
		-1.83015704154968 1.78078889846802
		-1.90257358551025 1.73876643180847
		-1.92771100997925 1.72396087646484
		-1.95211005210876 1.70957064628601
		-1.97498416900635 1.6944375038147
		-1.99632143974304 1.67964363098145
		-2.01756238937378 1.66498708724976
		-2.03893661499023 1.64983034133911
		-2.05983686447144 1.63298606872559
		-2.08063530921936 1.61446356773376
		-2.12348532676697 1.5724823474884
		-2.14357447624207 1.54941606521606
		-2.16593980789185 1.52381467819214
		-2.18623614311218 1.49846315383911
		-2.20717883110046 1.47089600563049
		-2.22741532325745 1.43993735313416
		-2.2462956905365 1.40983057022095
		-2.26328206062317 1.38170766830444
		-2.27943921089172 1.35371208190918
		-2.29773199558258 1.32472157478333
		-2.31566762924194 1.29507756233215
		-2.33314919471741 1.26553702354431
		-2.34915232658386 1.23751020431519
		-2.36416685581207 1.21056222915649
		-2.37859559059143 1.18387699127197
		-2.39202523231506 1.15666127204895
		-2.40671873092651 1.12935185432434
		-2.42982041835785 1.0743842124939
		-2.44235527515411 1.04626870155334
		-2.46629595756531 0.990217447280884
		-2.47793924808502 0.963125228881836
		-2.48897469043732 0.936257839202881
		-2.49852514266968 0.908730983734131
		-2.50624287128448 0.883384943008423
		-2.55507278442383 0.766805171966553
		-2.56312501430511 0.743082046508789
		-2.57129347324371 0.718043565750122
		-2.57917749881744 0.691274404525757
		-2.58634638786316 0.66340446472168
		-2.59270334243774 0.634773015975952
		-2.59945571422577 0.604812383651733
		-2.60654664039612 0.572771549224854
		-2.61368417739868 0.540310144424438
		-2.62096869945526 0.504998922348022
		-2.63374650478363 0.431916952133179
		-2.63881754875183 0.396202325820923
		-2.64365470409393 0.363004922866821
		-2.64867854118347 0.328368902206421
		-2.65313029289246 0.292894124984741
		-2.65693140029907 0.257617712020874
		-2.6605429649353 0.224954128265381
		-2.66544985771179 0.191718816757202
		-2.67079341411591 0.157835721969604
		-2.67502284049988 0.124284982681274
		-2.6784462928772 0.0910201072692871
		-2.68211209774017 0.0571565628051758
		-2.6856597661972 0.0237395763397217
		-2.68919372558594 -0.00969147682189941
		-2.6932338476181 -0.0427958965301514
		-2.69813191890717 -0.0753779411315918
		-2.70251095294952 -0.104392528533936
		-2.7126921415329 -0.166093826293945
		-2.71796214580536 -0.19374942779541
		-2.72342264652252 -0.222967624664307
		-2.72893142700195 -0.253115653991699
		-2.73447895050049 -0.281982421875
		-2.73923242092133 -0.309565782546997
		-2.74299395084381 -0.336159706115723
		-2.7451468706131 -0.362699747085571
		-2.74537551403046 -0.390228033065796
		-2.74378907680511 -0.418106317520142
		-2.74096155166626 -0.446968555450439
		-2.73668158054352 -0.477169752120972
		-2.7317430973053 -0.508008003234863
		-2.72557151317596 -0.540722131729126
		-2.71864080429077 -0.574871778488159
		-2.71061623096466 -0.609448552131653
		-2.70129454135895 -0.644609689712524
		-2.67886400222778 -0.717106461524963
		-2.6673172712326 -0.752311229705811
		-2.65463697910309 -0.789408683776855
		-2.64236986637115 -0.827803254127502
		-2.63112545013428 -0.865175843238831
		-2.62102353572845 -0.901326298713684
		-2.61064875125885 -0.937251329421997
		-2.60043942928314 -0.973786115646362
		-2.58978402614594 -1.01025009155273
		-2.57893645763397 -1.04626965522766
		-2.56782758235931 -1.08245003223419
		-2.55666899681091 -1.11859428882599
		-2.54519855976105 -1.1552015542984
		-2.53366422653198 -1.19198095798492
		-2.52290534973145 -1.22778296470642
		-2.51320350170135 -1.26251196861267
		-2.50329458713531 -1.29652106761932
		-2.48282408714294 -1.35920095443726
		-2.47191047668457 -1.38944625854492
		-2.46302127838135 -1.41858196258545
		-2.45534217357635 -1.4463963508606
		-2.44446957111359 -1.47234511375427
		-2.43424987792969 -1.49613070487976
		-2.42134249210358 -1.51895153522491
		-2.40863907337189 -1.54172730445862
		-2.39260590076447 -1.56381773948669
		-2.33537495136261 -1.63054805994034
		-2.31106078624725 -1.65425443649292
		-2.28736090660095 -1.67704099416733
		-2.25985908508301 -1.70025169849396
		-2.23019909858704 -1.72372609376907
		-2.19887137413025 -1.74912697076797
		-2.16682648658752 -1.77341520786285
		-2.13653635978699 -1.7984157204628
		-2.07474207878113 -1.85125440359116
		-2.04470062255859 -1.87600284814835
		-2.01509594917297 -1.90213578939438
		-1.98608040809631 -1.93009912967682
		-1.9574990272522 -1.95792067050934
		-1.9300754070282 -1.98432910442352
		-1.90186023712158 -2.01142889261246
		-1.87359881401062 -2.03864073753357
		-1.84519171714783 -2.06586521863937
		-1.81597661972046 -2.09307414293289
		-1.78741240501404 -2.1189076602459
		-1.76104640960693 -2.14417916536331
		-1.73467302322388 -2.1683267056942
		-1.70934295654297 -2.1912028491497
		-1.68445491790771 -2.21133920550346
		-1.65966939926147 -2.22999203205109
		-1.63541865348816 -2.24848467111588
		-1.58971524238586 -2.2849377989769
		-1.5673840045929 -2.30085781216621
		-1.54432034492493 -2.31549006700516
		-1.52030181884766 -2.32923766970634
		-1.49463629722595 -2.34254080057144
		-1.46833992004395 -2.35574577748775
		-1.44052004814148 -2.36896093189716
		-1.41103911399841 -2.38190983235836
		-1.37977242469788 -2.39502175152302
		-1.34667587280273 -2.40792129933834
		-1.31229043006897 -2.42054000496864
		-1.27611684799194 -2.43307012319565
		-1.23697113990784 -2.44605901837349
		-1.20029973983765 -2.45887637883425
		-1.16470146179199 -2.4717211201787
		-1.12725710868835 -2.48578376322985
		-1.08926844596863 -2.50131710618734
		-0.341370582580566 -1.62219375371933
		0.194170475006104 -1.67026317119598
		1.64847040176392 -0.354336023330688
		1.68733406066895 0.269269227981567
		1.60856580734253 0.814151048660278
		0.229955673217773 2.3338668346405
		-0.369425773620605 2.34252643585205
		-0.947361469268799 2.23924374580383
		-1.5411479473114 1.92815399169922
		-2.10221433639526 1.59406900405884
		-2.41758620738983 1.10244679450989
		-2.62758481502533 0.469635486602783
		-2.70839035511017 -0.137597322463989
		-2.6905277967453 -0.680629253387451
		-2.49304866790771 -1.32868719100952
		-2.10426497459412 -1.82492816448212
		0.407365798950195 -0.0268702507019043
		-0.288166522979736 -0.96311092376709
		-0.777018308639526 -1.51480090618134
		-1.61203265190125 -2.26702144742012
		-4.13223399221897 -0.512238264083862
		-1.01703119277954 -2.53395292535424
		-0.983861446380615 -2.5493841804564
		-0.951470851898193 -2.56420776620507
		-0.919610977172852 -2.57862347969785
		-0.888596773147583 -2.59209386538714
		-0.857147455215454 -2.60519089922309
		-0.82542085647583 -2.6174099855125
		-0.79365611076355 -2.62849796563387
		-0.762150764465332 -2.63885738700628
		-0.730725765228271 -2.64919175952673
		-0.700920581817627 -2.65919617563486
		-0.643120288848877 -2.67870170623064
		-0.614440441131592 -2.68613499403
		-0.58615517616272 -2.6925845593214
		-0.557061910629272 -2.69913183152676
		-0.52793550491333 -2.70639076083899
		-0.501125335693359 -2.71534219384193
		-0.44826865196228 -2.73275418579578
		-0.421224117279053 -2.74102954566479
		-0.391674041748047 -2.74908554553986
		-0.362610340118408 -2.75483372807503
		-0.331282615661621 -2.76123031973839
		-0.297548532485962 -2.76681044697762
		-0.26157283782959 -2.77313280105591
		-0.187160015106201 -2.78901851177216
		-0.146848201751709 -2.79822327196598
		-0.0599956512451172 -2.81402134895325
		-0.0185279846191406 -2.82283216714859
		0.0240025520324707 -2.8329082429409
		0.0669064521789551 -2.84278526902199
		0.109373569488525 -2.85003280639648
		0.151431560516357 -2.85946771502495
		0.191341876983643 -2.86845707893372
		0.232278347015381 -2.87615031003952
		0.310129642486572 -2.89058798551559
		0.348493099212646 -2.89715033769608
		0.385982036590576 -2.90396782755852
		0.423657894134521 -2.90918472409248
		0.459821701049805 -2.91594570875168
		0.496395111083984 -2.92049819231033
		2.29180574417114 -2.07416784763336
		2.30596208572388 -2.0442481637001
		2.3211932182312 -2.01457870006561
		2.33689594268799 -1.985171854496
		2.35356521606445 -1.95499891042709
		2.36924982070923 -1.92544519901276
		2.38502883911133 -1.89737385511398
		2.39975595474243 -1.86874735355377
		2.51012420654297 -1.08475148677826
		2.51091289520264 -0.798977017402649
		2.51673984527588 -0.387422800064087
		2.5140962600708 -0.352558374404907
		2.50971937179565 -0.319583415985107
		2.50571012496948 -0.287270545959473
		2.49907541275024 -0.254826307296753
		2.49449491500854 -0.214574813842773
		2.48898935317993 -0.171088457107544
		2.48301029205322 -0.127415180206299
		2.47722053527832 -0.0802211761474609
		2.47077655792236 -0.0294284820556641
		2.46413278579712 0.0173079967498779
		2.45852136611938 0.0667934417724609
		2.45339727401733 0.116848707199097
		2.44881820678711 0.166456937789917
		2.44529294967651 0.213187456130981
		2.44277572631836 0.260267734527588
		2.44064950942993 0.353001832962036
		2.44101619720459 0.399437665939331
		2.44167518615723 0.444752931594849
		2.44259452819824 0.489096641540527
		2.44437503814697 0.532661914825439
		2.44666957855225 0.575822114944458
		2.44977998733521 0.617964029312134
		2.45331573486328 0.656864881515503
		2.45689535140991 0.69455885887146
		2.46033096313477 0.730181455612183
		2.46403741836548 0.763455390930176
		2.46764802932739 0.796577453613281
		2.47222852706909 0.828947782516479
		2.47816514968872 0.859796047210693
		2.48332643508911 0.889948606491089
		2.48793697357178 0.918000459671021
		2.49196577072144 0.947416067123413
		2.49954605102539 1.00915813446045
		2.50288248062134 1.04421544075012
		2.50583219528198 1.08066082000732
		2.50728702545166 1.12000942230225
		2.50651407241821 1.16194200515747
		2.50352430343628 1.20583319664001
		2.49963092803955 1.25229215621948
		2.49480438232422 1.30165266990662
		2.48987007141113 1.35134553909302
		2.48564720153809 1.39978361129761
		2.48208856582642 1.45026874542236
		2.47937059402466 1.49879837036133
		2.47700786590576 1.54741811752319
		2.47508382797241 1.59475755691528
		2.47278642654419 1.64081692695618
		2.4712438583374 1.68485593795776
		2.46966457366943 1.72858452796936
		2.46754550933838 1.81110191345215
		2.46647024154663 1.85129356384277
		2.46329259872437 1.89035725593567
		2.4619574546814 1.92913150787354
		2.46200752258301 1.96401071548462
		2.45984172821045 1.99817514419556
		2.45761966705322 2.03080606460571
		2.45581293106079 2.06174731254578
		2.45387411117554 2.09077310562134
		2.45147609710693 2.11859011650085
		2.44816970825195 2.14579463005066
		2.44444227218628 2.17156004905701
		2.44025468826294 2.1965115070343
		2.43455839157104 2.22147536277771
		2.43018579483032 2.24539732933044
		2.42347049713135 2.27212691307068
		2.41743564605713 2.29834985733032
		2.40144634246826 2.35683155059814
		2.39230012893677 2.38807082176208
		2.38174676895142 2.42027902603149
		2.37012910842896 2.45140767097473
		2.35784816741943 2.48862028121948
		2.34454154968262 2.52484560012817
		2.33202362060547 2.56064414978027
		2.32121992111206 2.59442758560181
		2.31048250198364 2.62879347801208
		2.11861371994019 3.37461233139038
		1.58058500289917 3.93439912796021
		1.55937147140503 3.94429039955139
		1.45819520950317 3.99499297142029
		1.41218185424805 4.01202487945557
		1.25929546356201 4.03858375549316
		1.22367525100708 4.04181981086731
		1.10778141021729 4.05534720420837
		1.07028961181641 4.05958986282349
		1.0305814743042 4.06476664543152
		-3.82414370775223 3.79132008552551
		-4.1596665084362 2.676926612854
		-4.16670659184456 2.64075040817261
		-4.17371195554733 2.60695505142212
		-4.17738965153694 2.57142376899719
		-4.18609333783388 2.53663730621338
		-4.18670164048672 2.50735378265381
		-4.21103971451521 2.32144474983215
		-4.20935282111168 2.29540371894836
		-4.20968658477068 2.2608425617218
		-4.20620309561491 2.22475552558899
		-4.20786896348 2.19141912460327
		-4.20828974992037 2.15073347091675
		-4.20619543641806 2.11229038238525
		-4.20442977547646 2.07479500770569
		-4.2040161266923 2.02928423881531
		-4.20181374996901 1.98470664024353
		-4.20385627448559 1.93955898284912
		-4.20545345544815 1.89935827255249
		-4.20952846109867 1.85276174545288
		-4.21714520454407 1.80208969116211
		-4.22210679203272 1.7588996887207
		-4.22874741256237 1.71305060386658
		-4.23479851707816 1.6707878112793
		-4.24839610606432 1.5873019695282
		-4.25360972434282 1.5457136631012
		-4.25900623947382 1.50419664382935
		-4.26284719258547 1.46238350868225
		-4.26626331172884 1.42074084281921
		-4.26885493844748 1.37931227684021
		-4.27121603488922 1.33762645721436
		-4.27303393930197 1.29781126976013
		-4.27447614818811 1.25935435295105
		-4.2765838522464 1.22175621986389
		-4.27821468003094 1.18630862236023
		-4.27991060353816 1.15098571777344
		-4.28133000992239 1.11767983436584
		-4.28482772130519 1.08298993110657
		-4.28516953345388 1.05089569091797
		-4.28501587174833 1.0174880027771
		-4.28457326348871 0.985489845275879
		-4.28265500254929 0.916829586029053
		-4.27911493182182 0.880947351455688
		-4.27630409598351 0.843485116958618
		-4.27383713424206 0.802809000015259
		-4.26959686726332 0.761577844619751
		-4.26608921028674 0.718852996826172
		-4.26321532391012 0.674260139465332
		-4.25418167561293 0.579790353775024
		-4.24977958574891 0.530970096588135
		-4.24693186953664 0.482069253921509
		-4.24485631287098 0.433767080307007
		-4.24440364167094 0.386854648590088
		-4.24354512244463 0.340838193893433
		-4.24263399094343 0.295625686645508
		-4.24144769087434 0.25081205368042
		-4.24038485810161 0.205930233001709
		-4.23757592588663 0.117404699325562
		-4.23542648926377 0.0736122131347656
		-4.23253225535154 0.031005859375
		-4.22966364771128 -0.011249303817749
		-4.22636525332928 -0.0515420436859131
		-4.22223431617022 -0.0907320976257324
		-4.21799114346504 -0.129073143005371
		-4.21535950899124 -0.165078163146973
		-4.21366623044014 -0.196521997451782
		-4.20830386132002 -0.229782819747925
		-4.20407105237246 -0.26090407371521
		-4.19729298353195 -0.288059711456299
		-4.1834372729063 -0.349525213241577
		-4.17608794569969 -0.379807949066162
		-4.16717550158501 -0.411098957061768
		-4.15682092308998 -0.443200826644897
		-4.14527183771133 -0.477459669113159
		-4.11757835745811 -0.548268556594849
		-4.10173688828945 -0.585371851921082
		-4.08492965996265 -0.623841404914856
		-4.06741763651371 -0.665006399154663
		-2.96754837036133 -2.5100936666131
		-2.94735586643219 -2.52657172083855
		-2.87810015678406 -2.5770115358755
		-2.8514506816864 -2.59360602684319
		-2.82563555240631 -2.61183220334351
		-1.05238842964172 -2.51772248744965
		-0.474890232086182 -2.72438958287239
		0.27153205871582 -2.8836835026741
		2.44172239303589 0.307831764221191
		2.49629068374634 0.978105068206787
		2.46844100952148 1.77034568786621
		2.41002702713013 2.32722878456116
		1.385573387146 4.01973009109497
		-4.19627466797829 2.44317150115967
		-4.24120136350393 1.62881994247437
		-4.28289302438498 0.952000379562378
		-4.23921549320221 0.161624908447266
		-2.05663585662842 -2.99925199151039
		-2.03290820121765 -3.00431290268898
		-2.00595831871033 -3.00992795825005
		-1.98002099990845 -3.01537668704987
		-1.95394563674927 -3.01995036005974
		-1.92585968971252 -3.02453607320786
		-1.89684224128723 -3.02698829770088
		-1.86894369125366 -3.02812758088112
		-1.84121203422546 -3.02814793586731
		-1.81411910057068 -3.02639156579971
		-1.7867431640625 -3.02492702007294
		-1.76561403274536 -3.0225770175457
		-1.74574112892151 -3.0178214609623
		-1.72816395759583 -3.01353740692139
		-1.7135124206543 -3.01027265191078
		-1.67882466316223 -2.99871018528938
		-1.66427850723267 -2.99379333853722
		-1.65968132019043 -2.99396693706512
		-1.6573007106781 -2.99597212672234
		-1.65600156784058 -2.99835485219955
		-1.65597748756409 -3.00085905194283
		-1.65622687339783 -3.00352856516838
		-1.65692496299744 -3.00601354241371
		-1.65792679786682 -3.00868371129036
		-1.65921831130981 -3.0110998749733
		-1.66054248809814 -3.01334461569786
		-1.66207098960876 -3.01574352383614
		-1.66236090660095 -3.01731204986572
		-1.66127061843872 -3.01699897646904
		-1.66040325164795 -3.01658216118813
		-1.65868782997131 -3.01479014754295
		-1.65604138374329 -3.01179641485214
		-1.65282678604126 -3.00754314661026
		-1.64426755905151 -2.99984154105186
		-1.63774490356445 -2.99701151251793
		-1.63064527511597 -2.99456202983856
		-1.62326884269714 -2.99265360832214
		-1.6156599521637 -2.99131834506989
		-1.6071949005127 -2.99000269174576
		-1.59878039360046 -2.98852199316025
		-1.58913516998291 -2.98695829510689
		-1.5781877040863 -2.98502278327942
		-1.56599259376526 -2.98271310329437
		-1.55170798301697 -2.97940289974213
		-1.53504419326782 -2.97700735926628
		-1.51706838607788 -2.97525662183762
		-1.49450302124023 -2.97378075122833
		-1.47509765625 -2.97272634506226
		-1.4506528377533 -2.97208935022354
		-1.42367076873779 -2.97121644020081
		-1.3644654750824 -2.97231164574623
		-1.33342838287354 -2.97437763214111
		-1.30103039741516 -2.97678118944168
		-1.26802158355713 -2.97996410727501
		-1.23500442504883 -2.98277714848518
		-1.20114278793335 -2.98504650592804
		-1.16715526580811 -2.98803558945656
		-1.13260769844055 -2.99141106009483
		-1.09819149971008 -2.99458742141724
		-1.06397271156311 -2.99819800257683
		-0.998855352401733 -3.00515681505203
		-0.967853784561157 -3.00805431604385
		-0.937385559082031 -3.01055896282196
		-0.90665078163147 -3.01173716783524
		-0.874955415725708 -3.01067760586739
		-0.808577537536621 -3.00484576821327
		-0.772720813751221 -3.00011810660362
		-0.69523286819458 -2.98856514692307
		-0.653045892715454 -2.98187693953514
		-0.563559532165527 -2.96788403391838
		-0.14522123336792 -2.9391251206398
		-0.0597672462463379 -2.93881180882454
		-0.0181751251220703 -2.93933454155922
		0.105367183685303 -2.93970274925232
		0.146444320678711 -2.9394593834877
		0.186685562133789 -2.93931180238724
		0.226377964019775 -2.93883082270622
		0.265230655670166 -2.9382132589817
		0.300805568695068 -2.93776574730873
		0.335568904876709 -2.93737882375717
		0.370904922485352 -2.93704554438591
		0.405324459075928 -2.93630382418633
		0.438881397247314 -2.93404501676559
		2.17435836791992 -2.78757962584496
		2.06236982345581 -2.6830712556839
		2.05214929580688 -2.65330012887716
		2.03332185745239 -2.59877029433846
		2.02492618560791 -2.56251018494368
		1.97929382324219 -2.47538748383522
		1.94073438644409 -2.40861620008945
		1.92259407043457 -2.3872944265604
		1.90208196640015 -2.36588583886623
		1.87917232513428 -2.34837964177132
		1.85496139526367 -2.32487595081329
		1.82957315444946 -2.29801434278488
		1.80338621139526 -2.27601116895676
		1.74406623840332 -2.21913880109787
		1.7189507484436 -2.19203069806099
		1.69262170791626 -2.16593128442764
		1.64244556427002 -2.10721951723099
		1.61837863922119 -2.07457190752029
		1.54565286636353 -1.98650711774826
		1.52145719528198 -1.95610004663467
		1.44986867904663 -1.87479269504547
		1.42536926269531 -1.84347718954086
		1.4007740020752 -1.81670540571213
		1.37623357772827 -1.7889004945755
		1.35126161575317 -1.765829205513
		1.32710552215576 -1.74171191453934
		1.30432415008545 -1.71966928243637
		1.28198575973511 -1.70078784227371
		1.21338129043579 -1.63991332054138
		1.16199111938477 -1.6056923866272
		1.10488080978394 -1.57400059700012
		1.07449150085449 -1.55473792552948
		1.04306697845459 -1.53567349910736
		1.00961112976074 -1.52091157436371
		0.973335742950439 -1.5039644241333
		0.816562175750732 -1.42578864097595
		0.777291297912598 -1.40362441539764
		0.739748001098633 -1.38304674625397
		0.703005790710449 -1.36010468006134
		0.668007373809814 -1.33413589000702
		0.633259773254395 -1.30729389190674
		0.60081958770752 -1.28239107131958
		0.566814422607422 -1.25603842735291
		0.532726287841797 -1.22989284992218
		0.499220848083496 -1.20394432544708
		0.46537971496582 -1.17788088321686
		0.432822704315186 -1.15096068382263
		0.400049686431885 -1.12468898296356
		0.367897510528564 -1.09821355342865
		0.336660861968994 -1.07305634021759
		0.307440757751465 -1.04896855354309
		0.277522087097168 -1.02637577056885
		0.216916084289551 -0.985205173492432
		0.186448097229004 -0.966617584228516
		0.155266761779785 -0.947815656661987
		0.125396251678467 -0.929558396339417
		0.0959076881408691 -0.911806106567383
		0.0667314529418945 -0.893410086631775
		0.0363645553588867 -0.874421238899231
		0.00520133972167969 -0.855442523956299
		-0.0272154808044434 -0.835718870162964
		-0.0612826347351074 -0.815157532691956
		-0.0960116386413574 -0.793968319892883
		-0.130734443664551 -0.772088766098022
		-0.165922164916992 -0.749632120132446
		-0.200377941131592 -0.725830554962158
		-0.235208511352539 -0.701361775398254
		-0.269782543182373 -0.675049066543579
		-0.301742553710938 -0.648808121681213
		-0.355880260467529 -0.59538209438324
		-0.380717039108276 -0.566305637359619
		-0.404174089431763 -0.536694765090942
		-0.427075624465942 -0.507186651229858
		-0.448946237564087 -0.477012872695923
		-0.469935894012451 -0.445830583572388
		-0.48877477645874 -0.412712097167969
		-0.507504940032959 -0.379825830459595
		-0.523527383804321 -0.345473527908325
		-0.538507699966431 -0.311203002929688
		-0.552841424942017 -0.276901006698608
		-0.565301418304443 -0.242959260940552
		-0.577220916748047 -0.209362983703613
		-0.58855938911438 -0.175933361053467
		-0.59973931312561 -0.141176462173462
		-0.609078645706177 -0.109683513641357
		-0.616737127304077 -0.080751895904541
		-0.628238201141357 -0.0207855701446533
		-0.635458707809448 0.00931954383850098
		-0.643556118011475 0.0402882099151611
		-0.651140689849854 0.0719368457794189
		-0.658101558685303 0.10407543182373
		-0.664508104324341 0.136897325515747
		-0.670377731323242 0.170685052871704
		-0.675612688064575 0.206317663192749
		-0.679100513458252 0.243142604827881
		-0.681045055389404 0.281492233276367
		-0.684248924255371 0.359079122543335
		-0.682765483856201 0.398490428924561
		-0.680221557617188 0.435830116271973
		-0.675568103790283 0.47168493270874
		-0.667203187942505 0.506792306900024
		-0.656699657440186 0.542487621307373
		-0.644065856933594 0.5770263671875
		-0.547400951385498 0.724396705627441
		-0.521059513092041 0.748488187789917
		-0.492045164108276 0.770983457565308
		-0.461901903152466 0.792261600494385
		-0.430648326873779 0.812301158905029
		-0.398018360137939 0.831261157989502
		-0.364010334014893 0.848019361495972
		-0.328376531600952 0.864441156387329
		-0.255277156829834 0.891423463821411
		-0.218183517456055 0.90111255645752
		-0.180343627929688 0.908562898635864
		-0.143445491790771 0.914277315139771
		-0.10714054107666 0.91960597038269
		-0.0709714889526367 0.924352407455444
		-0.0348954200744629 0.928344964981079
		0.00151395797729492 0.932253360748291
		0.0386314392089844 0.935134887695312
		0.113154888153076 0.937446594238281
		0.150767803192139 0.936983585357666
		0.188944339752197 0.935603380203247
		0.227670669555664 0.933363676071167
		0.266463756561279 0.930252552032471
		0.305579662322998 0.925670385360718
		0.34449577331543 0.918662071228027
		0.380981922149658 0.90895938873291
		0.415079593658447 0.897632360458374
		0.448842525482178 0.883423566818237
		0.480967044830322 0.865925788879395
		0.51073694229126 0.846319675445557
		0.538800239562988 0.825078010559082
		0.564413070678711 0.802412033081055
		0.588239669799805 0.777213096618652
		0.611161231994629 0.750345945358276
		0.632898807525635 0.722244262695312
		0.671199321746826 0.662543058395386
		0.68829345703125 0.631237268447876
		0.703159332275391 0.600261926651001
		0.715634346008301 0.56950306892395
		0.726748466491699 0.538830518722534
		0.737296581268311 0.508408308029175
		0.746474742889404 0.480378389358521
		0.753448963165283 0.45435357093811
		0.759535312652588 0.426355838775635
		0.764811515808105 0.397804260253906
		0.771056175231934 0.369369745254517
		0.777851581573486 0.341900587081909
		0.784536361694336 0.313913583755493
		0.792035579681396 0.285567998886108
		0.800614356994629 0.256142377853394
		0.809704303741455 0.225502967834473
		0.819454193115234 0.194146156311035
		0.840110778808594 0.12628173828125
		0.849795341491699 0.090538501739502
		0.85797119140625 0.0544514656066895
		0.863979816436768 0.018322229385376
		0.867427825927734 -0.0165162086486816
		0.867900371551514 -0.0497832298278809
		0.865953922271729 -0.0818181037902832
		0.860862255096436 -0.112916231155396
		0.852774620056152 -0.141768455505371
		0.842184066772461 -0.169568061828613
		0.830191135406494 -0.196530818939209
		0.81524658203125 -0.222442626953125
		0.798420429229736 -0.246750593185425
		0.778918743133545 -0.270984888076782
		0.757312297821045 -0.294944286346436
		0.733702182769775 -0.317675590515137
		0.708244323730469 -0.340005397796631
		0.652328014373779 -0.382449865341187
		0.62255859375 -0.400696039199829
		0.591763973236084 -0.417586088180542
		0.561076641082764 -0.433994054794312
		0.530841827392578 -0.449265480041504
		0.499690055847168 -0.463799953460693
		0.467292785644531 -0.478108167648315
		0.43571138381958 -0.491402626037598
		0.406163692474365 -0.502818584442139
		0.377118110656738 -0.514632225036621
		0.348095893859863 -0.526409149169922
		0.318670272827148 -0.538020372390747
		0.289245128631592 -0.5503089427948
		0.259159564971924 -0.562934637069702
		0.228304386138916 -0.575451374053955
		0.196201324462891 -0.58827543258667
		0.163700103759766 -0.600040316581726
		0.0935449600219727 -0.620789408683777
		0.0567646026611328 -0.629667401313782
		0.0204238891601562 -0.635545015335083
		-0.0143508911132812 -0.637822151184082
		-0.0488944053649902 -0.635840535163879
		-0.0805091857910156 -0.632934927940369
		-0.113161563873291 -0.626247048377991
		-0.144683837890625 -0.616654515266418
		-0.174492359161377 -0.605078458786011
		-0.202998638153076 -0.591166496276855
		-0.230573654174805 -0.574578285217285
		-0.256010055541992 -0.555505990982056
		-0.280004978179932 -0.534609794616699
		-0.303425073623657 -0.511988639831543
		-0.326541662216187 -0.488833427429199
		-0.347731590270996 -0.464216947555542
		-0.368520498275757 -0.438265323638916
		-1.67060613632202 -2.99560761451721
		-1.6493091583252 -3.00330793857574
		-1.39501333236694 -2.97107955813408
		-0.735051870346069 -2.99458855390549
		2.07312345504761 -2.71348099410534
		1.57058906555176 -2.01604640483856
		0.898318290710449 -1.46577334403992
		0.247017383575439 -1.00457739830017
		-0.329594850540161 -0.622746109962463
		-0.622649669647217 -0.0509903430938721
		-0.629070043563843 0.610405921936035
		0.075739860534668 0.936861038208008
		0.652867794036865 0.69294548034668
		0.829652309417725 0.160964965820312
		0.680900573730469 -0.361942052841187
		0.128764629364014 -0.6104576587677
		-0.388209104537964 -0.412678480148315
		-0.607199907302856 0.0627813339233398
		-0.525317668914795 0.402263641357422
		-0.405617713928223 -0.387486934661865
		-0.422074317932129 -0.362639188766479
		-0.43783974647522 -0.337647438049316
		-0.45269250869751 -0.313091039657593
		-0.466138124465942 -0.291240692138672
		-0.477127313613892 -0.269887685775757
		-0.48696756362915 -0.248616218566895
		-0.49686861038208 -0.227666616439819
		-0.508135318756104 -0.207389831542969
		-0.519225835800171 -0.184927225112915
		-0.530579805374146 -0.162606954574585
		-0.540906429290771 -0.139997720718384
		-0.551109075546265 -0.116265773773193
		-0.560221910476685 -0.0920288562774658
		-0.569478034973145 -0.0673706531524658
		-0.57762885093689 -0.0420577526092529
		-0.585057258605957 -0.0160865783691406
		-0.610787391662598 0.0889711380004883
		-0.618768930435181 0.114238023757935
		-0.623031377792358 0.140683174133301
		-0.62691068649292 0.164891242980957
		-0.628286838531494 0.188154697418213
		-0.626328706741333 0.229560613632202
		-0.623257637023926 0.248366594314575
		-0.619644641876221 0.266180753707886
		-0.615277767181396 0.283860921859741
		-0.609172582626343 0.30049204826355
		-0.601079702377319 0.315871715545654
		-0.591888189315796 0.328700065612793
		-0.582172870635986 0.341063976287842
		-0.571691274642944 0.352863788604736
		-0.560601711273193 0.363513946533203
		-0.549024105072021 0.374831438064575
		-0.536946535110474 0.388329267501831
		-0.515031099319458 0.416720151901245
		-0.505024433135986 0.42948317527771
		-0.496411561965942 0.440706253051758
		-0.488390684127808 0.450682640075684
		-0.481375694274902 0.458633184432983
		-0.475879430770874 0.465291500091553
		-0.470975637435913 0.470431327819824
		-0.467100381851196 0.474532127380371
		-0.464586496353149 0.477438926696777
		-0.462545394897461 0.480718851089478
		-0.461005449295044 0.484076976776123
		-0.459953784942627 0.486122131347656
		-0.458978652954102 0.488553762435913
		-0.459135770797729 0.495852947235107
		-0.459111928939819 0.500250577926636
		-0.459519863128662 0.504960060119629
		-0.460515022277832 0.509134292602539
		-0.460334062576294 0.513065099716187
		-0.460330724716187 0.516794204711914
		-0.460944414138794 0.520808935165405
		-0.460898160934448 0.524644374847412
		-0.464481115341187 0.52683687210083
		-0.467690229415894 0.528415441513062
		-0.471284866333008 0.529098987579346
		-0.473724126815796 0.529650926589966
		-0.477516651153564 0.529351472854614
		-0.481000661849976 0.530147552490234
		-0.484831809997559 0.530839204788208
		-0.488232135772705 0.531748294830322
		-0.491442680358887 0.531158447265625
		-0.494639158248901 0.531203746795654
	};
\addlegendentry{Optitrack}
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.471813 -0.21331
		-0.441062 -0.201245
		-0.441062 -0.201245
		-0.56084 -0.268602
		-0.514195 -0.237621
		-0.514195 -0.237621
		-0.510642 -0.251453
		-0.534535 -0.265227
		-0.512931 -0.246751
		-0.518666 -0.238782
		-0.518666 -0.238782
		-0.502524 -0.245551
		-0.502524 -0.245551
		-0.54931 -0.276751
		-0.53299 -0.250344
		-0.519304 -0.226464
		-0.519408 -0.237164
		-0.492816 -0.221767
		-0.4882 -0.231752
		-0.492564 -0.222325
		-0.445873 -0.225539
		-0.506175 -0.246085
		-0.405837 -0.217529
		-0.377665 -0.2003
		-0.403763 -0.239267
		-0.407127 -0.237491
		-0.425957 -0.282793
		-0.373588 -0.247483
		-0.413719 -0.285202
		-0.401608 -0.283386
		-0.50172 -0.362715
		-0.468808 -0.340396
		-0.46353 -0.344105
		-0.381156 -0.285008
		-0.45928 -0.398183
		-0.438766 -0.389327
		-0.423699 -0.363458
		-0.485881 -0.413812
		-0.426484 -0.385278
		-0.433532 -0.389122
		-0.451602 -0.411361
		-0.411471 -0.384725
		-0.356614 -0.342059
		-0.435263 -0.417406
		-0.268326 -0.271036
		-0.285709 -0.297311
		-0.344737 -0.367372
		-0.330558 -0.352371
		-0.335563 -0.355797
		-0.339404 -0.372305
		-0.318664 -0.359519
		-0.401077 -0.503008
		-0.373213 -0.495472
		-0.323317 -0.457375
		-0.367815 -0.534798
		-0.311162 -0.462805
		-0.259467 -0.473378
		-0.272684 -0.49541
		-0.257095 -0.551586
		-0.223216 -0.521574
		-0.242335 -0.510636
		-0.183268 -0.482606
		-0.155448 -0.516001
		-0.161932 -0.504971
		-0.159442 -0.506337
		-0.122697 -0.463083
		-0.116558 -0.426165
		-0.10413 -0.436974
		-0.53013 -0.244831
		-0.480875 -0.417774
		-0.304197 -0.359362
		-0.0937639 -0.423741
		0.0923089 -0.417099
		0.21743 -0.376189
		0.30707 -0.264665
		0.465771 -0.302449
		0.33897 -0.201476
		0.522324 -0.251039
		0.506588 -0.137955
		0.338165 0.0528818
		0.539558 0.0742143
		0.365829 0.0752735
		0.310193 0.244224
		0.367389 0.282844
		-0.0889491 -0.424778
		-0.0920426 -0.424118
		-0.112805 -0.521161
		-0.0618906 -0.429483
		-0.0439408 -0.377566
		-0.0433751 -0.392044
		-0.0224507 -0.404111
		-0.01179 -0.400863
		0.0110259 -0.437361
		0.0182601 -0.400063
		0.024878 -0.399706
		0.0278348 -0.399511
		0.0409853 -0.398377
		0.0435133 -0.411703
		0.0664064 -0.464845
		0.0707469 -0.454269
		0.0939396 -0.464062
		0.101793 -0.424426
		0.104201 -0.4327
		0.114594 -0.431932
		0.145244 -0.511607
		0.13471 -0.425401
		0.134196 -0.41653
		0.145355 -0.421883
		0.151776 -0.419616
		0.148043 -0.384247
		0.167507 -0.454661
		0.145517 -0.363793
		0.152434 -0.415565
		0.183426 -0.430568
		0.17742 -0.386149
		0.207905 -0.419625
		0.228233 -0.446368
		0.20644 -0.371593
		0.244769 -0.365454
		0.198615 -0.284292
		0.270132 -0.347548
		0.298047 -0.359359
		0.296688 -0.333573
		0.286635 -0.308797
		0.32784 -0.347709
		0.283729 -0.296308
		0.254051 -0.265483
		0.257273 -0.257273
		0.273036 -0.274408
		0.273922 -0.261657
		0.270579 -0.265113
		0.333809 -0.303043
		0.341864 -0.30563
		0.342604 -0.301364
		0.314958 -0.280298
		0.33026 -0.278114
		0.268524 -0.239114
		0.274635 -0.243248
		0.280881 -0.247283
		0.248169 -0.22539
		0.297758 -0.26389
		0.254039 -0.220167
		0.266127 -0.23684
		0.350139 -0.303346
		0.419102 -0.328745
		0.42838 -0.342312
		0.439276 -0.369391
		0.399963 -0.321071
		0.421445 -0.312321
		0.452151 -0.320107
		0.450362 -0.308877
		0.456202 -0.300185
		0.468471 -0.308948
		0.474149 -0.29381
		0.477222 -0.288791
		0.448064 -0.250612
		0.451883 -0.239345
		0.453087 -0.237058
		0.451975 -0.23917
		0.45193 -0.239257
		0.449991 -0.242882
		0.451975 -0.23917
		0.449839 -0.247411
		0.450272 -0.246622
		0.449484 -0.248056
		0.446205 -0.253907
		0.4474 -0.252475
		0.448228 -0.25718
		0.391123 -0.220795
		0.341231 -0.209884
		0.414618 -0.239015
		0.403693 -0.229335
		0.413156 -0.238606
		0.597685 -0.320765
		0.531917 -0.283281
		0.536983 -0.283804
		0.556015 -0.299068
		0.671069 -0.34693
		0.661016 -0.3466
		0.5243 -0.275947
		0.532206 -0.281053
		0.558455 -0.289725
		0.484942 -0.262525
		0.560623 -0.276064
		0.453982 -0.222676
		0.489992 -0.236548
		0.424098 -0.205474
		0.443066 -0.210239
		0.445123 -0.205848
		0.420169 -0.18174
		0.423444 -0.184403
		0.471585 -0.198767
		0.529565 -0.226956
		0.50986 -0.217282
		0.50392 -0.211949
		0.50984 -0.197286
		0.518972 -0.19375
		0.543178 -0.191567
		0.5202 -0.19043
		0.493735 -0.182947
		0.527052 -0.177239
		0.532349 -0.15947
		0.484759 -0.13695
		0.446351 -0.10665
		0.453969 -0.100882
		0.437733 -0.0617069
		0.401779 -0.0438624
		0.416724 -0.0359245
		0.382217 -0.0181224
		0.366934 0.00157484
		0.365751 0.0158334
		0.35832 0.0167014
		0.356664 0.0260227
		0.470861 0.0442689
		0.433367 0.0627
		0.47375 0.0627618
		0.43202 0.0713932
		0.432872 0.0660314
		0.431627 0.0737362
		0.369237 0.0562213
		0.352383 0.0519909
		0.387989 0.0545367
		0.388872 0.0478375
		0.389275 0.0444447
		0.374801 0.0422927
		0.364457 0.0394008
		0.363722 0.0402593
		0.379876 0.037412
		0.40791 0.0443048
		0.41014 0.0416307
		0.403591 0.0377895
		0.479597 0.0484986
		0.473257 0.0457423
		0.488366 0.0452191
		0.492399 0.0545091
		0.477979 0.0515293
		0.487461 0.0629563
		0.539284 0.0761814
		0.539284 0.0761814
		0.539245 0.0764601
		0.481621 0.0721529
		0.481621 0.0721529
		0.412056 0.065307
		0.361431 0.057719
		0.361431 0.057719
		0.361631 0.0600391
		0.37247 0.0594212
		0.37247 0.0594212
		0.386473 0.0644121
		0.387354 0.0588779
		0.387354 0.0588779
		0.350337 0.0643477
		0.336975 0.0538607
		0.336975 0.0538607
		0.378085 0.0886866
		0.378085 0.0886866
		0.488875 0.142589
		0.365274 0.122781
		0.365274 0.122781
		0.419555 0.154014
		0.332385 0.148662
		0.332385 0.148662
		0.328609 0.160809
		0.32499 0.168003
		0.32499 0.168003
		0.300879 0.172298
		0.263788 0.167448
		0.263788 0.167448
		0.291566 0.199087
		0.284741 0.213237
		0.284741 0.213237
		0.323778 0.259023
		0.323778 0.259023
		0.313534 0.249402
		0.270044 0.235518
		0.270044 0.235518
		0.297822 0.254502
		0.279413 0.238249
		0.279413 0.238249
		0.273496 0.227914
		0.250313 0.195064
		0.250313 0.195064
		0.289437 0.23358
		0.289437 0.23358
		0.297647 0.230645
		0.313979 0.250915
		0.313979 0.250915
		0.404545 0.326026
		0.367389 0.282844
		0.472756 0.370751
		0.490191 0.388068
		0.490191 0.388068
		0.391749 0.309449
		0.394775 0.305579
		0.370399 0.285647
		0.365258 0.273555
		0.355552 0.267799
		0.334171 0.246684
		0.293624 0.220218
		0.303077 0.214789
		0.303321 0.219875
		0.288064 0.19372
		0.283038 0.183791
		0.301873 0.188181
		0.261397 0.173886
		0.253264 0.179807
		0.221531 0.155749
		0.241347 0.15598
		0.225474 0.149985
		0.257137 0.177493
		0.254476 0.181286
		0.257137 0.177493
		0.257302 0.177253
		0.290306 0.186717
		0.257266 0.177305
		0.25602 0.179099
		0.293182 0.204298
		0.290763 0.200066
		0.273092 0.185402
		0.270179 0.189621
		0.248579 0.187015
		0.248305 0.187378
		0.402981 0.332316
		0.225178 0.204509
		0.152317 0.140252
		0.167412 0.159841
		0.141652 0.139495
		0.143414 0.149359
		0.152169 0.157746
		0.127467 0.128127
		0.180484 0.181429
		0.123154 0.126412
		0.192787 0.191783
		0.194617 0.196677
		0.182702 0.179817
		0.178348 0.178348
		0.196759 0.191498
		0.161044 0.14519
		0.163377 0.14485
		0.165477 0.142447
		0.162863 0.143148
		0.160527 0.141742
		0.17173 0.151634
		0.161268 0.140898
		0.170841 0.15106
		0.170101 0.147836
		0.172477 0.145805
		0.171018 0.145187
		0.184908 0.15409
		0.161876 0.137298
		0.184435 0.154656
		0.184824 0.155794
		0.195727 0.165535
		0.206163 0.170543
		0.191714 0.157764
		0.216113 0.174466
		0.187521 0.146713
		0.208044 0.165992
		0.210636 0.165338
		0.203847 0.149919
		0.17519 0.109494
		0.142249 0.0866171
		0.140827 0.0806747
		0.145621 0.0808198
		0.146568 0.0790889
		0.147564 0.0781649
		0.148365 0.0756659
		0.129557 0.0522003
		0.192612 0.0589055
		0.237806 0.0577528
		0.206388 0.0503626
		0.343388 0.0499766
		0.39511 0.0309533
		0.380962 0.0157278
		0.380807 0.0191273
		0.434701 0.0177027
		0.451085 0.0222509
		0.456286 0.0245535
		0.35071 -0.00943613
		0.386393 0.00686922
		0.386322 0.010122
		0.36685 0.00800985
		0.415566 -0.00722719
		0.366906 -0.00478573
		0.385906 -0.0205816
		0.401007 -0.035331
		0.390043 -0.0381376
		0.393572 -0.0511819
		0.393342 -0.052916
		0.424022 -0.0798606
		0.421396 -0.110181
		0.331238 -0.103121
		0.376959 -0.126811
		0.303942 -0.109998
		0.259331 -0.0963229
		0.222978 -0.116481
		0.214494 -0.192659
		0.210803 -0.167711
		0.201112 -0.164242
		0.183663 -0.15238
		0.182349 -0.18346
		0.210008 -0.218972
		0.183594 -0.192495
		0.223145 -0.267479
		0.208031 -0.252411
		0.232134 -0.241749
		0.253778 -0.30227
		0.251867 -0.303865
		0.255254 -0.311608
		0.264613 -0.354034
		0.226064 -0.3184
		0.268402 -0.379598
		0.242393 -0.364501
		0.19871 -0.336151
		0.22503 -0.412223
		0.215937 -0.418007
		0.198163 -0.413985
		0.154594 -0.397798
		0.149332 -0.406409
		0.143542 -0.401918
		0.100232 -0.422546
		0.0566762 -0.380793
		0.0133657 -0.355861
		-0.0171917 -0.328205
		-0.0768416 -0.318573
		-0.0838311 -0.284737
		-0.0865507 -0.275008
		-0.0982505 -0.271969
		-0.176117 -0.342866
		-0.226198 -0.404894
		-0.228674 -0.400179
		-0.282459 -0.420067
		-0.252712 -0.378007
		-0.269701 -0.374237
		-0.243938 -0.322148
		-0.235874 -0.283733
		-0.268361 -0.291039
		-0.302639 -0.290771
		-0.307474 -0.285654
		-0.373422 -0.310435
		-0.26652 -0.201691
		-0.320543 -0.194269
		-0.274856 -0.173159
		-0.360364 -0.215143
		-0.347306 -0.19483
		-0.345857 -0.197391
		-0.349405 -0.189821
		-0.420869 -0.21735
		-0.369764 -0.181426
		-0.374789 -0.176984
		-0.36707 -0.166541
		-0.434616 -0.165661
		-0.439066 -0.153479
		-0.444678 -0.136368
		-0.443565 -0.128966
		-0.44588 -0.120719
		-0.45018 -0.11693
		-0.453061 -0.110835
		-0.422298 -0.0603283
		-0.388546 -0.0404736
		-0.504018 -0.0296481
		-0.521239 -0.00657024
		-0.544371 0.0228727
		-0.48802 0.0364496
		-0.430967 0.0393414
		-0.428758 0.0587096
		-0.487304 0.0550511
		-0.625455 0.0825068
		-0.584632 0.084585
		-0.584393 0.106932
		-0.569776 0.126078
		-0.508279 0.125984
		-0.604873 0.179897
		-0.552503 0.20091
		-0.403459 0.174658
		-0.52153 0.263033
		-0.518339 0.269267
		-0.457537 0.250843
		-0.439286 0.249905
		-0.443711 0.263085
		-0.354262 0.224157
		-0.350739 0.229632
		-0.429546 0.279301
		-0.429697 0.290961
		-0.41591 0.299229
		-0.355785 0.265221
		-0.374482 0.283438
		-0.327743 0.263719
		-0.289352 0.266986
		-0.371328 0.342346
		-0.362593 0.355341
		-0.341474 0.355556
		-0.41363 0.486074
		-0.429976 0.590216
		-0.39768 0.577523
		-0.378905 0.605733
		-0.372116 0.640572
		-0.349725 0.628492
		-0.350613 0.632127
		-0.326372 0.604033
		-0.312928 0.599579
		-0.313635 0.647668
		-0.288428 0.583833
		-0.23444 0.54069
		-0.209796 0.511504
		-0.205775 0.507444
		-0.162231 0.453188
		-0.1536 0.468029
		-0.109234 0.472751
		-0.0706288 0.612875
		-0.033467 0.500146
		-0.033467 0.500146
		-0.0167616 0.320866
		0.0230748 0.31151
		0.0230748 0.31151
		0.0507164 0.259434
		0.0956961 0.499534
		0.0956961 0.499534
		0.0844884 0.317138
		0.112211 0.438642
		0.112211 0.438642
		0.105666 0.349933
		0.205858 0.473862
		0.205858 0.473862
		0.19739 0.418604
		0.241411 0.467372
		0.389009 0.646522
		0.388266 0.639818
		0.388266 0.639818
		0.493508 0.704548
		0.571262 0.762911
		0.571262 0.762911
		0.559112 0.695481
		0.560552 0.673998
		0.560552 0.673998
		0.630707 0.689619
		0.541607 0.564292
		0.541607 0.564292
		0.462254 0.444127
		0.404357 0.373402
		0.404357 0.373402
		0.461255 0.405548
		0.541222 0.465398
		0.531748 0.410782
		0.430495 0.315831
		0.430495 0.315831
		0.49031 0.298747
		0.511078 0.312325
		0.511078 0.312325
		0.544356 0.295791
		0.53805 0.277546
		0.53805 0.277546
		0.483923 0.175214
		0.483923 0.175214
		0.537296 0.187591
		0.522923 0.140352
		0.522923 0.140352
		0.450501 0.107262
		0.445402 0.0694133
		0.445402 0.0694133
		0.444326 0.0365463
		0.428797 0.0166343
		0.457741 -0.0463535
		0.410282 -0.0566499
		0.528145 -0.139218
		0.594317 -0.201464
		0.642314 -0.246405
		0.633291 -0.271811
		0.609566 -0.288742
		0.578212 -0.309574
		0.468382 -0.290571
		0.494263 -0.301155
		0.381102 -0.265885
		0.404779 -0.310331
		0.328002 -0.281374
		0.300572 -0.276765
		0.26788 -0.269239
		0.266359 -0.298556
		0.438353 -0.542844
		0.415537 -0.548102
		0.424618 -0.607787
		0.385656 -0.559329
		0.384629 -0.666495
		0.375718 -0.671559
		0.350284 -0.642188
		0.341051 -0.679163
		0.341051 -0.679163
		0.329758 -0.719471
		0.282138 -0.68397
		0.241026 -0.635673
		0.244943 -0.734829
		0.224043 -0.800154
		0.173071 -0.736286
		0.164108 -0.741416
		0.0840718 -0.568591
		0.0797394 -0.62825
		0.0691792 -0.782026
		0.0290642 -0.829945
		-0.00606545 -0.773339
		-0.0388859 -0.759769
		-0.0804154 -0.756501
		-0.116352 -0.751813
		-0.134075 -0.785742
		-0.150141 -0.78824
		-0.157137 -0.770278
		-0.16827 -0.767922
		-0.17557 -0.777523
		-0.186281 -0.763753
		-0.197325 -0.718615
		-0.223428 -0.720928
		-0.236499 -0.721471
		0.257464 0.206933
		0.163603 0.142301
		0.197183 0.158581
		0.407076 0.0242752
		0.385599 -0.0902089
		0.251867 -0.303865
		-0.0485082 -0.349594
		-0.294657 -0.192838
		-0.467907 -0.0995548
		-0.501345 0.235414
		-0.360808 0.399605
		-0.109234 0.472751
		0.241411 0.467372
		0.541222 0.465398
		0.447503 0.0542428
		0.279362 -0.297006
		-0.267421 -0.716095
		-0.287567 -0.705577
		-0.303512 -0.712202
		-0.311565 -0.704803
		-0.328915 -0.66355
		-0.336489 -0.64774
		-0.284938 -0.516029
		-0.383614 -0.678016
		-0.370495 -0.584043
		-0.290394 -0.450611
		-0.318151 -0.441435
		-0.322715 -0.43811
		-0.323611 -0.41204
		-0.340279 -0.398238
		-0.450532 -0.489288
		-0.479104 -0.494395
		-0.571861 -0.542535
		-0.710874 -0.611351
		-0.656491 -0.532992
		-0.718401 -0.560703
		-0.692845 -0.48926
		-0.750335 -0.515417
		-0.796004 -0.554682
		-0.780995 -0.511569
		-0.740687 -0.45247
		-0.718091 -0.422581
		-0.626849 -0.341454
		-0.662262 -0.336387
		-0.748728 -0.340598
		-0.761031 -0.312142
		-0.729854 -0.269791
		-0.800525 -0.273047
		-0.741152 -0.252796
		-0.734634 -0.241096
		-0.815354 -0.224925
		-0.792439 -0.192837
		-0.787172 -0.181884
		-0.791127 -0.172501
		-0.792346 -0.16681
		-0.792942 -0.163954
		-0.831513 -0.166303
		-0.803299 -0.150996
		-0.830657 -0.14677
		-0.830117 -0.149796
		-0.811691 -0.128645
		-0.811691 -0.128645
		-0.837032 -0.13582
		-0.795778 -0.149583
		-0.795778 -0.149583
		-0.794673 -0.15535
		-0.830286 -0.172323
		-0.805816 -0.182449
		-0.785322 -0.183045
		-0.782811 -0.198668
		-0.781248 -0.199718
		-0.780457 -0.207726
		-0.77958 -0.226138
		-0.781594 -0.248553
		-0.783132 -0.266083
		-0.777479 -0.282174
		-0.757147 -0.299947
		-0.788166 -0.31344
		-0.775347 -0.343928
		-0.757306 -0.338872
		-0.755271 -0.340901
		-0.768876 -0.366418
		-0.809629 -0.396814
		-0.829857 -0.476584
		-0.817214 -0.537734
		-0.755191 -0.522067
		-0.687994 -0.729124
		-0.687994 -0.729124
		-0.687994 -0.729124
		-0.670154 -0.741287
		-0.645803 -0.746593
		-0.580209 -0.84394
		-0.580209 -0.84394
		-0.580209 -0.84394
		-0.580209 -0.84394
		-0.431 -0.734871
		-0.3974 -0.716525
		-0.3974 -0.716525
		-0.339069 -0.769184
		-0.339069 -0.769184
		-0.230127 -0.786785
		-0.156646 -0.783231
		-0.0854454 -0.670212
		-0.0631101 -0.660027
		-0.0399663 -0.666105
		-0.00257984 -0.663032
		0.0208581 -0.765792
		0.0828592 -0.760529
		0.109559 -0.724776
		0.156021 -0.713239
		0.156021 -0.713239
		0.170607 -0.716551
		0.22321 -0.734244
		0.263554 -0.765857
		0.285106 -0.759249
		0.335559 -0.69761
		0.335559 -0.69761
		0.367196 -0.674149
		0.42431 -0.611006
		0.42431 -0.611006
		0.441233 -0.563046
		0.441233 -0.563046
		0.476933 -0.556881
		0.443478 -0.498599
		0.328948 -0.334115
		0.479076 -0.450187
		0.338269 -0.306294
		0.394545 -0.32162
		0.476535 -0.33945
		0.411055 -0.29708
		0.471896 -0.299745
		0.583904 -0.322491
		0.604864 -0.26744
		0.657504 -0.196712
		0.705955 -0.157835
		0.654144 -0.118446
		0.629909 -0.0518444
		0.734676 -0.0268784
		0.669937 0.00274566
		0.578788 0.199414
		0.603645 0.253894
		0.60403 0.306042
		0.591855 0.334411
		0.664538 0.384891
		0.564068 0.360591
		0.605557 0.413007
		0.557883 0.411342
		0.560129 0.41491
		0.541476 0.441865
		0.508898 0.452353
		0.491262 0.476884
		0.469304 0.490422
		0.492186 0.559538
		0.511801 0.645567
		0.542226 0.767052
		0.550206 0.811379
		0.316001 0.876333
		-0.115895 0.858808
		-0.115895 0.858808
		-0.15484 0.865281
		-0.15484 0.865281
		-0.216861 0.852172
		-0.330836 0.931116
		-0.330836 0.931116
		-0.422995 0.984557
		-0.481239 1.00007
		-0.481239 1.00007
		-0.534289 0.929663
		-0.569491 0.945502
		-0.607155 0.920044
		-0.600819 0.87812
		-0.600819 0.87812
		-0.626357 0.870345
		-0.657303 0.877628
		-0.657303 0.877628
		-0.752293 0.916858
		-0.718475 0.860673
		-0.718475 0.860673
		-0.738304 0.807407
		-0.744758 0.798988
		-0.744758 0.798988
		-0.924433 0.810406
		-0.924433 0.810406
		-1.07017 0.904111
		-1.09954 0.913967
		-1.09954 0.913967
		-1.1394 0.878963
		-1.1394 0.878963
		-1.18701 0.844516
		-1.23204 0.837213
		-1.23204 0.837213
		-1.22092 0.821868
		-1.22092 0.821868
		-1.23639 0.817848
		-1.2652 0.763893
		-1.2652 0.763893
		-1.27638 0.736187
		-1.23076 0.689225
		-1.33077 0.691809
		-1.30574 0.652869
		-1.37097 0.623617
		-1.34773 0.524651
		-1.34664 0.515734
		-1.37117 0.481368
		-1.37669 0.465358
		-1.36894 0.456312
		-1.39284 0.430427
		-1.39757 0.424091
		-1.61149 0.454945
		-1.61885 0.428034
		-1.64857 0.412142
		-1.64792 0.384516
		-1.70663 0.376715
		-1.72623 0.344099
		-1.77425 0.292781
		-1.82634 0.17964
		-1.77459 0.144983
		-1.80685 0.136703
		-1.79418 0.11068
		-1.77892 0.0750844
		-1.77994 -0.0574174
		-1.77571 -0.0747064
		-1.76734 -0.0686347
		-1.81321 -0.0987968
		-1.80168 -0.134979
		-1.72314 -0.156142
		-1.71296 -0.178549
		-1.71059 -0.207515
		-1.7146 -0.229734
		-1.72506 -0.270597
		-1.72209 -0.288903
		-1.71624 -0.321796
		-1.69718 -0.33497
		-1.69182 -0.357348
		-1.68303 -0.38022
		-1.68584 -0.443938
		-1.67763 -0.472181
		-1.63756 -0.48581
		-1.59322 -0.50767
		-1.58471 -0.533628
		-1.55262 -0.566495
		-1.54765 -0.570463
		-1.54072 -0.649826
		-1.53012 -0.671377
		-1.52228 -0.688652
		-1.60316 -0.771278
		-1.58505 -0.776127
		-1.5223 -0.753193
		-1.64445 -0.842277
		-1.64048 -0.898496
		-1.62808 -0.936147
		-1.58277 -0.946223
		-1.55179 -0.957123
		-1.458 -0.928802
		-1.60657 -1.07105
		-1.64381 -1.12896
		-1.66138 -1.16865
		-1.50977 -1.09749
		-1.50641 -1.12254
		-1.48573 -1.13886
		-1.4678 -1.15122
		-1.52723 -1.21692
		-1.34249 -1.09547
		-1.45292 -1.26603
		-1.43348 -1.27154
		-1.41302 -1.27531
		-1.50762 -1.39763
		-1.38529 -1.28934
		-1.50144 -1.44829
		-1.51791 -1.56643
		-1.635 -1.71069
		-1.35864 -1.51172
		-1.33964 -1.50316
		-1.33775 -1.53523
		-1.25068 -1.46611
		-1.22166 -1.49579
		-1.18723 -1.53326
		-1.23481 -1.66987
		-1.22908 -1.7286
		-1.2546 -1.76322
		-1.22332 -1.79421
		-1.2769 -1.93712
		-1.25881 -1.97604
		-1.26325 -2.09274
		-1.20751 -2.03952
		-1.19088 -2.11627
		-1.15319 -2.13189
		-1.133 -2.13004
		-1.02857 -2.09336
		-0.864253 -1.81555
		-0.838656 -1.82752
		-0.915439 -2.03049
		-0.843635 -1.9575
		-0.802294 -1.89749
		-0.778789 -1.89949
		-0.687205 -1.80466
		-0.613333 -1.79872
		-0.634382 -1.81856
		-0.587905 -1.83644
		-0.587905 -1.83644
		-0.548185 -1.81139
		-0.490944 -1.8668
		-0.473212 -1.84493
		-0.45669 -1.87548
		-0.445165 -1.946
		-0.246317 -0.718178
		-0.57817 -0.53459
		-0.80894 -0.247004
		-0.805047 -0.175536
		-0.824684 -0.508555
		-0.230127 -0.786785
		0.410153 -0.629471
		0.721321 -0.145428
		0.436515 0.471789
		-0.569491 0.945502
		-1.14362 0.898898
		-1.33126 0.489226
		-1.78053 -0.0344618
		-1.66262 -0.475034
		-1.42872 -0.932931
		-1.54852 -1.67756
		-0.401667 -2.00833
		-0.342544 -1.90846
		-0.333244 -1.93158
		-0.298241 -1.93235
		-0.254637 -1.90371
		-0.239343 -1.93316
		-0.211418 -1.89672
		-0.165169 -1.92697
		-0.158565 -1.99791
		-0.102645 -2.02723
		-0.0300223 -1.90942
		0.0312621 -1.98201
		0.0627421 -1.98892
		0.108405 -2.13422
		0.169423 -2.12118
		0.187481 -2.08908
		0.267411 -2.10586
		0.369835 -1.98308
		0.377347 -2.0721
		0.527072 -1.92413
		0.591874 -2.02448
		0.687958 -2.17974
		0.689413 -2.03411
		0.702769 -2.00695
		0.960461 -2.18812
		0.864879 -1.84713
		0.757279 -1.55189
		0.883582 -1.62373
		0.908384 -1.56041
		1.21863 -1.84478
		1.51055 -2.12743
		1.93626 -0.67869
		1.95003 -0.658883
		1.86056 -0.626514
		1.83776 -0.540881
		1.90157 -0.546941
		1.98745 -0.526476
		1.83374 -0.464467
		2.03211 -0.479712
		2.00977 -0.451707
		2.06434 -0.411519
		2.06513 -0.362067
		1.87787 -0.302882
		1.91706 -0.257241
		2.0073 -0.250912
		1.91998 -0.191998
		1.91932 -0.173358
		1.94803 -0.12568
		1.93905 -0.0685839
		1.94968 -0.0376143
		1.9862 0.0191595
		1.95455 0.0754166
		2.09462 0.128795
		2.10918 0.170645
		1.93321 0.199557
		2.0355 0.256908
		1.88096 0.242705
		2.00305 0.311153
		2.06397 0.349598
		2.06102 0.382665
		2.07301 0.411901
		2.11534 0.464681
		2.1282 0.518048
		2.09839 0.55074
		2.09839 0.55074
		1.91683 0.619583
		1.91683 0.619583
		1.84633 0.729798
		1.8577 0.739289
		1.75987 0.85566
		1.67308 0.822265
		1.67308 0.822265
		1.65078 0.911971
		1.7937 1.14085
		1.74582 1.2234
		1.74582 1.2234
		1.71895 1.27428
		1.65824 1.26465
		1.52439 1.31624
		1.52439 1.31624
		1.44431 1.36705
		1.44431 1.36705
		1.33992 1.3342
		0.50805 1.71403
		0.438991 1.79344
		0.371321 1.81417
		0.423526 1.91731
		0.359703 1.85847
		0.350357 1.84881
		0.317125 1.7493
		0.0105715 1.8236
		-0.0784526 1.92769
		-0.0870736 1.76196
		-0.0660574 1.73781
		-0.144094 1.8412
		-0.145369 1.91775
		-0.137418 1.96393
		-0.180407 1.77314
		-0.169186 1.87196
		-0.157609 1.86957
		-0.159991 1.83989
		-0.175622 1.66841
		-0.18203 1.73434
		-0.338167 1.84355
		-0.55064 2.09496
		-0.640362 2.43487
		-0.625485 2.35648
		-0.707689 2.38845
		-0.693001 2.277
		-0.819185 2.47316
		-0.865241 2.35704
		-0.872424 2.31669
		-0.872424 2.31669
		-0.95834 2.39202
		-1.04328 2.49584
		-0.933372 2.29301
		-1.15899 2.38895
		-1.19091 2.38182
		-1.24918 2.41725
		-1.25237 2.39307
		-1.25396 2.373
		-1.27401 2.38777
		-1.34996 2.41182
		-1.37068 2.38023
		-1.36628 2.32834
		-1.42557 2.28569
		-1.51035 2.20324
		-1.38706 2.01301
		-1.31886 1.87938
		-1.457 1.98295
		-1.28791 1.72128
		-1.47933 1.92382
		-1.5117 1.91761
		-1.4808 1.79715
		-1.44479 1.6593
		-1.85625 1.95104
		-1.86843 1.93938
		-1.91938 1.95164
		-1.95164 1.91938
		-1.97219 1.91561
		-2.07531 1.98288
		-2.04328 1.90489
		-2.10453 1.90568
		-2.14217 1.92203
		-2.17091 1.85484
		-2.17853 1.83631
		-2.13228 1.76215
		-2.1965 1.74907
		-2.19024 1.69464
		-2.0914 1.61228
		-2.17836 1.66768
		-2.20064 1.65048
		-2.17748 1.5822
		-2.19026 1.56447
		-2.19765 1.55406
		-2.36896 1.59611
		-2.38566 1.57104
		-2.58966 1.61294
		-2.60014 1.57801
		-2.68597 1.59306
		-2.7137 1.58377
		-2.4186 1.33829
		-2.43564 1.3146
		-2.456 1.27616
		-2.50069 1.22183
		-2.50482 1.19548
		-2.51791 1.11727
		-2.52092 1.09535
		-2.65677 0.997338
		-2.67513 0.933771
		-2.67176 0.893369
		-2.6666 0.877825
		-2.68725 0.840795
		-2.66576 0.809542
		-2.67028 0.79453
		-2.67691 0.771871
		-2.7056 0.686742
		-2.69007 0.672517
		-2.70783 0.582594
		-2.6918 0.505733
		-2.69591 0.473827
		-2.75746 0.456808
		-2.74699 0.439851
		-2.76137 0.432504
		-2.80715 0.386613
		-2.86112 0.367248
		-2.92947 0.341043
		-2.93154 0.322818
		-2.93514 0.288272
		-2.90687 0.24152
		-3.16057 0.244568
		-2.82206 0.184777
		-2.91647 0.165411
		-2.92057 0.129996
		-3.17548 0.084554
		-2.88669 -0.00854035
		-2.8865 -0.0341596
		-2.88518 -0.0938964
		-2.83396 -0.117383
		-2.92532 -0.155327
		-2.8092 -0.199469
		-2.80602 -0.240043
		-2.89035 -0.264309
		-2.91566 -0.283825
		-2.89519 -0.325495
		-2.8822 -0.332562
		-2.81904 -0.383657
		-2.83424 -0.39528
		-3.43164 -0.48878
		-3.19879 -0.504571
		-3.40122 -0.588868
		-3.10242 -0.613052
		-2.83635 -0.623655
		-2.72963 -0.645186
		-2.72777 -0.653012
		-2.77061 -0.698967
		-2.83161 -0.740177
		-2.84869 -0.779276
		-2.69754 -0.768391
		-2.72451 -0.797418
		-2.67478 -0.834335
		-2.65566 -0.89334
		-2.71161 -0.951151
		-2.6984 -0.988028
		-2.66447 -1.01974
		-2.6628 -1.04375
		-2.64475 -1.06776
		-2.91965 -1.20435
		-2.70849 -1.13774
		-3.15378 -1.42268
		-3.05686 -1.42588
		-3.02339 -1.45823
		-3.02227 -1.48668
		-3.03191 -1.53077
		-2.99609 -1.57172
		-2.99037 -1.62222
		-2.90255 -1.68348
		-2.92916 -1.70868
		-2.87094 -1.80042
		-2.80418 -1.80884
		-2.77873 -1.84294
		-2.77263 -1.85162
		-2.77841 -1.9874
		-2.71501 -1.98254
		-2.73639 -2.04488
		-2.79659 -2.12541
		-2.6751 -2.11036
		-2.82123 -2.25911
		-2.72376 -2.26807
		-2.82746 -2.37246
		-2.60402 -2.21191
		-2.71104 -2.35238
		-2.57956 -2.29851
		-2.4335 -2.2331
		-2.44179 -2.28737
		-2.37057 -2.27612
		-2.29628 -2.25895
		-2.21691 -2.2813
		-2.18445 -2.28499
		-2.16601 -2.34264
		-2.25263 -2.46716
		-2.10069 -2.36789
		-2.08878 -2.38454
		-2.03356 -2.48546
		-2.11763 -2.6101
		-2.08934 -2.63865
		-1.956 -2.54279
		-1.93777 -2.56196
		-1.98723 -2.71164
		-1.95283 -2.74373
		-1.89215 -2.7797
		-1.82389 -2.75995
		-1.79839 -2.79428
		-1.79062 -2.8376
		-1.73701 -2.79265
		-1.63698 -2.67037
		-1.63698 -2.67037
		-1.49318 -2.7375
		-1.49608 -2.76915
		-1.49608 -2.76915
		-0.427138 -1.95718
		0.300696 -1.88837
		1.86124 -0.584783
		2.07119 0.0331923
		1.8577 0.739289
		0.440602 1.88511
		-0.109063 1.69543
		-0.861563 2.49774
		-1.34938 1.98601
		-2.152 1.87675
		-2.55407 1.42372
		-2.73984 0.649568
		-2.81596 0.0419042
		-2.88326 -0.597433
		-2.94104 -1.26705
		-2.75114 -2.11626
		0.234597 0.165959
		0.107959 -0.55059
		-1.04085 -2.02506
		-1.98058 -2.38942
		-4.22551 -0.341336
		-1.43769 -2.80118
		-1.43769 -2.80118
		-1.45544 -2.95972
		-1.22346 -2.63515
		-1.22346 -2.63515
		-1.19992 -2.88531
		-1.17219 -2.84932
		-1.17219 -2.84932
		-1.18432 -3.04264
		-1.16754 -3.04911
		-1.16754 -3.04911
		-1.03812 -2.96607
		-1.03812 -2.96607
		-0.989329 -2.96799
		-0.955116 -2.96637
		-0.955116 -2.96637
		-0.830433 -3.00801
		-0.780137 -2.96633
		-0.726278 -2.97774
		-0.698106 -2.95353
		-0.698106 -2.95353
		-0.613389 -3.0038
		-0.587903 -3.11682
		-0.587903 -3.11682
		-0.516492 -3.26462
		-0.516492 -3.26462
		-0.304496 -3.20673
		-0.304496 -3.20673
		-0.276924 -3.46669
		-0.222813 -3.27439
		-0.222813 -3.27439
		-0.144292 -3.03915
		-0.10414 -3.19048
		-0.10414 -3.19048
		-0.0673555 -3.2427
		-0.0661719 -3.72769
		0.0706751 -3.45298
		0.0706751 -3.45298
		0.128897 -3.36124
		0.259621 -3.25007
		2.4514 -2.68387
		2.42499 -2.54523
		2.47163 -2.55234
		2.43869 -2.44844
		2.49203 -2.49203
		2.47987 -2.37373
		2.49352 -2.4248
		2.50341 -2.39584
		2.74051 -1.72341
		2.87819 -1.38229
		2.96075 -0.810017
		2.86569 -0.745618
		2.92318 -0.767335
		2.86846 -0.659212
		2.80722 -0.604633
		2.70108 -0.555131
		2.87225 -0.544585
		2.89654 -0.501832
		2.73909 -0.425896
		2.89114 -0.433229
		2.9135 -0.399718
		2.9314 -0.365311
		2.92047 -0.345146
		2.92329 -0.310046
		2.92975 -0.240436
		3.05036 -0.175627
		2.93582 -0.0800676
		2.92409 0.00886095
		3.04129 0.0643174
		3.0485 0.119729
		3.0485 0.119729
		3.04681 0.156957
		2.92154 0.195361
		2.89989 0.202113
		2.91431 0.283459
		2.91345 0.29223
		2.87427 0.341757
		2.88066 0.40523
		2.8769 0.431095
		2.83178 0.495127
		2.89534 0.531256
		2.99249 0.594838
		2.86041 0.605424
		2.84153 0.688593
		2.85475 0.713686
		2.83973 0.771283
		2.83529 0.796332
		2.83732 0.819475
		2.94756 0.918244
		2.95349 0.978285
		2.94789 0.995029
		2.86694 1.0252
		2.8522 1.07185
		2.85524 1.09118
		2.66167 1.1076
		2.60033 1.20339
		2.59727 1.18516
		2.62299 1.2093
		2.63941 1.19116
		2.75779 1.26733
		2.50682 1.24116
		2.59363 1.36462
		2.79706 1.50469
		2.66163 1.45735
		2.74136 1.54711
		2.8006 1.62286
		2.74923 1.64769
		2.66309 1.63602
		2.66191 1.67737
		2.67264 1.68073
		2.65606 1.70681
		2.64383 1.73816
		2.56382 1.72395
		2.67664 1.82456
		2.59389 1.78048
		2.66918 1.85723
		2.57844 1.82753
		2.46023 1.81919
		2.53854 1.91064
		2.5427 1.97263
		2.51307 1.97262
		2.69568 2.19575
		2.53231 2.08706
		2.54204 2.12148
		2.34921 2.02886
		2.48008 2.17124
		2.60664 3.27894
		1.30057 2.59315
		1.30057 2.59315
		1.48741 3.3314
		1.47099 3.39458
		1.16737 2.92274
		1.39452 3.39535
		1.14705 3.13589
		1.01237 3.0371
		1.01237 3.0371
		-3.62375 3.89589
		-4.02918 2.82042
		-4.08732 2.79233
		-4.10532 2.75932
		-4.12602 2.72828
		-4.13838 2.70949
		-4.12705 2.65311
		-4.28002 2.4729
		-4.2105 2.39082
		-4.25043 2.40008
		-4.28146 2.37709
		-4.27624 2.36672
		-4.24922 2.33108
		-4.11527 2.211
		-4.12059 2.20106
		-3.58751 1.85484
		-3.63002 1.81501
		-3.63404 1.80587
		-3.64775 1.77912
		-3.60975 1.72784
		-3.61562 1.7144
		-3.63254 1.67826
		-3.6626 1.66482
		-4.22417 1.86887
		-3.66436 1.54231
		-3.57916 1.48066
		-3.61988 1.45652
		-3.66822 1.44341
		-3.66511 1.41215
		-3.69907 1.39259
		-4.07357 1.51714
		-3.7003 1.33081
		-3.80238 1.31919
		-3.70098 1.248
		-3.79688 1.23619
		-3.80333 1.21618
		-3.94697 1.22413
		-3.9534 1.20321
		-4.00713 1.16971
		-4.00947 1.14391
		-4.01552 1.12249
		-3.96706 1.04277
		-3.96756 1.00889
		-3.97292 0.987556
		-3.99102 0.957845
		-3.99614 0.93624
		-4.39162 0.975916
		-4.30197 0.901829
		-4.32606 0.747562
		-4.16612 0.65719
		-4.42383 0.685383
		-4.19342 0.626059
		-4.18271 0.57571
		-4.14053 0.558274
		-4.14053 0.500121
		-4.16829 0.477374
		-4.16467 0.440829
		-4.21432 0.387388
		-4.32897 0.363779
		-3.95927 0.287545
		-4.06498 0.249108
		-4.16151 0.197063
		-4.0626 0.181568
		-4.08337 0.147455
		-4.08828 0.0908508
		-4.03725 0.078502
		-4.03725 0.078502
		-4.04188 0
		-4.18401 -0.0699278
		-4.17799 -0.151292
		-4.03451 -0.168104
		-4.03451 -0.168104
		-4.22009 -0.270368
		-4.22551 -0.341336
		-4.25031 -0.415533
		-4.16229 -0.443045
		-4.16229 -0.443045
		-4.4676 -0.538114
		-3.33817 -2.51827
		-3.40352 -2.6218
		-3.35816 -2.72251
		-3.19608 -2.64225
		-3.07252 -2.58447
		-1.45179 -2.79262
		-0.780137 -2.96633
		-0.0673555 -3.2427
		2.97086 -0.135039
		2.82017 0.648811
		2.7695 1.31281
		2.48912 1.80788
		1.47713 3.45356
		-4.17384 2.61202
		-3.6589 1.58073
		-4.06004 1.09353
		-4.21211 0.410652
		-2.64825 -3.50613
		-2.49472 -3.39757
		-2.4698 -3.39155
		-2.43833 -3.42076
		-2.41427 -3.51276
		-2.36986 -3.46
		-2.39777 -3.5784
		-2.38801 -3.58202
		-2.291 -3.52553
		-2.06965 -3.29611
		-2.22195 -3.48496
		-2.03683 -3.29616
		-2.1927 -3.52942
		-2.16291 -3.53081
		-2.14117 -3.49532
		-1.9943 -3.3948
		-1.92503 -3.3827
		-1.9155 -3.38811
		-1.88269 -3.39992
		-1.92433 -3.37311
		-1.65837 -3.01253
		-1.73078 -3.17309
		-1.72429 -3.18013
		-1.94007 -3.61134
		-1.69749 -3.23877
		-1.91219 -3.62617
		-1.69552 -3.25582
		-1.90479 -3.63429
		-1.69552 -3.25582
		-1.75143 -3.39407
		-1.68591 -3.25734
		-1.69127 -3.25803
		-1.6737 -3.23305
		-1.77562 -3.378
		-1.77562 -3.378
		-1.68662 -3.17903
		-1.80166 -3.40558
		-1.94505 -3.65434
		-1.94995 -3.65173
		-1.94007 -3.61134
		-1.80205 -3.38567
		-1.73874 -3.23657
		-1.73205 -3.24365
		-1.70298 -3.22942
		-1.69003 -3.22454
		-1.6987 -3.23167
		-1.78186 -3.38989
		-1.90479 -3.63429
		-1.76854 -3.38519
		-1.68591 -3.25734
		-1.63527 -3.23969
		-1.61881 -3.24794
		-1.60784 -3.30965
		-1.57558 -3.32854
		-1.56474 -3.31724
		-1.51418 -3.29802
		-1.47106 -3.37604
		-1.43164 -3.40412
		-1.43548 -3.50169
		-1.34882 -3.42475
		-1.3062 -3.42351
		-1.26433 -3.40638
		-1.24427 -3.40867
		-1.14181 -3.22856
		-1.16699 -3.30982
		-1.10722 -3.26234
		-1.08081 -3.27216
		-1.06288 -3.27803
		-0.965749 -3.38521
		-0.948274 -3.6514
		-0.559454 -3.25062
		-0.422132 -3.09257
		-0.4026 -3.41204
		-0.324674 -3.44966
		-0.294996 -3.59263
		-0.285904 -3.61087
		-0.202909 -3.4596
		-0.160081 -3.63919
		-0.110021 -3.74072
		-0.0711081 -3.46399
		0.0186693 -3.2298
		0.0367762 -3.16275
		0.0839087 -3.20718
		1.93594 -2.69915
		1.9348 -2.61985
		2.03643 -2.7914
		1.8172 -2.47881
		1.832 -2.55204
		1.71689 -2.32478
		2.04718 -2.66609
		2.04718 -2.66609
		1.89799 -2.50393
		2.00485 -2.61665
		2.00485 -2.61665
		1.90081 -2.44894
		2.05691 -2.70697
		1.68773 -2.24227
		2.02762 -2.58314
		2.02762 -2.58314
		1.91602 -2.44825
		1.91602 -2.44825
		1.91129 -2.42214
		2.05027 -2.54385
		1.85721 -2.3866
		1.86508 -2.36186
		1.86508 -2.36186
		1.86487 -2.35927
		1.86487 -2.35927
		1.87359 -2.35512
		1.64166 -2.11626
		1.64166 -2.11626
		1.64659 -2.10353
		1.61264 -2.03906
		1.52172 -1.9187
		1.61292 -2.07149
		1.61292 -2.07149
		1.56542 -2.00497
		1.60649 -2.08844
		1.15994 -1.56054
		1.06747 -1.47413
		1.15569 -1.58683
		1.01575 -1.42637
		1.00779 -1.44284
		0.92562 -1.32962
		0.902242 -1.32023
		0.880452 -1.31562
		0.836983 -1.2604
		0.762903 -1.1995
		0.732902 -1.16905
		0.722641 -1.18046
		0.725612 -1.26381
		0.710975 -1.24658
		0.699102 -1.27683
		0.562801 -1.06851
		0.547881 -1.07123
		0.522358 -1.08684
		0.490717 -1.08811
		0.453457 -1.03764
		0.444816 -1.0476
		0.415922 -1.02163
		0.408715 -1.02179
		0.373178 -0.961217
		0.337963 -0.975484
		0.313302 -0.982454
		0.246844 -0.881095
		0.199602 -0.8306
		0.150652 -0.793232
		0.124568 -0.744509
		0.11018 -0.795742
		0.0744853 -0.631923
		0.0675464 -0.683258
		0.0352912 -0.571276
		0.0198559 -0.635388
		-0.0184799 -0.654718
		-0.0676023 -0.690108
		-0.102121 -0.62294
		-0.126229 -0.633774
		-0.161972 -0.621762
		-0.161169 -0.565296
		-0.169865 -0.462191
		-0.200065 -0.44869
		-0.248588 -0.497176
		-0.187927 -0.327023
		-0.271434 -0.402535
		-0.296763 -0.423088
		-0.305346 -0.389644
		-0.406204 -0.441335
		-0.449142 -0.442268
		-0.510652 -0.458809
		-0.483317 -0.313691
		-0.46186 -0.29833
		-0.396499 -0.233453
		-0.429378 -0.230446
		-0.414269 -0.222337
		-0.430858 -0.216404
		-0.423035 -0.198298
		-0.430307 -0.18198
		-0.442945 -0.141896
		-0.454481 -0.121456
		-0.398619 -0.0552708
		-0.366676 -0.033612
		-0.37398 -0.0202573
		-0.364638 -0.00151299
		-0.38851 0.0356134
		-0.509921 0.108034
		-0.517257 0.194524
		-0.485282 0.319942
		-0.393747 0.277212
		-0.409133 0.299907
		-0.400398 0.303053
		-0.344154 0.305376
		-0.337266 0.32908
		-0.290545 0.287711
		-0.314167 0.341278
		-0.22969 0.317191
		-0.236813 0.354455
		-0.222294 0.404954
		-0.206507 0.413013
		-0.233839 0.447101
		-0.176464 0.363307
		-0.173994 0.394281
		-0.168812 0.41451
		-0.101334 0.286922
		-0.111986 0.361475
		-0.113415 0.37805
		-0.100983 0.397811
		-0.0627249 0.349658
		-0.0454252 0.290278
		-0.0412272 0.294162
		-0.0228554 0.500915
		0.00135326 0.358612
		0.0161617 0.35825
		0.0443209 0.405002
		0.0313459 0.228129
		0.0502322 0.249229
		0.0559672 0.256849
		0.0881262 0.31651
		0.130161 0.39362
		0.137166 0.391234
		0.219215 0.531759
		0.221921 0.409701
		0.272896 0.468669
		0.272984 0.461519
		0.27799 0.422545
		0.281671 0.407257
		0.354188 0.480218
		0.433583 0.525401
		0.442106 0.486814
		0.483467 0.491349
		0.478657 0.468418
		0.462504 0.431827
		0.482321 0.41409
		0.462676 0.385939
		0.459076 0.370792
		0.490841 0.369299
		0.526478 0.380646
		0.464409 0.308218
		0.443193 0.274357
		0.407237 0.226816
		0.413767 0.214674
		0.419003 0.204264
		0.47345 0.210422
		0.619061 0.232148
		0.54721 0.180206
		0.716239 0.190612
		0.715758 0.146601
		0.643962 0.0905167
		0.655865 0.0522602
		0.733321 0.0119239
		0.733121 -0.0208611
		0.667757 -0.0540694
		0.664093 -0.0589115
		0.713379 -0.109308
		0.672972 -0.132966
		0.60043 -0.163754
		0.597269 -0.174932
		0.591409 -0.193823
		0.384288 -0.145932
		0.406427 -0.174183
		0.475157 -0.231271
		0.542549 -0.284656
		0.39438 -0.232205
		0.409747 -0.261113
		0.314431 -0.219947
		0.333429 -0.243725
		0.32864 -0.251115
		0.43416 -0.346869
		0.334418 -0.327303
		0.284554 -0.287565
		0.271752 -0.280614
		0.263549 -0.309251
		0.272629 -0.348177
		0.271292 -0.356175
		0.245458 -0.341438
		0.239427 -0.426479
		0.197548 -0.420704
		0.233728 -0.482064
		0.156482 -0.454181
		0.195251 -0.496435
		0.122548 -0.443772
		0.100881 -0.461726
		0.0768519 -0.428941
		0.0613667 -0.486843
		0.044972 -0.451594
		0.0216313 -0.473922
		-0.0194737 -0.517135
		-0.0483968 -0.496593
		-0.059322 -0.447785
		-2.05665 -3.55239
		-1.68689 -3.25925
		-1.73732 -3.38831
		-1.08081 -3.27216
		1.9348 -2.61985
		1.91129 -2.42214
		1.26427 -1.68354
		0.545139 -1.08196
		0.0270182 -0.574137
		-0.439767 -0.308268
		-0.527194 0.260174
		-0.0987562 0.289379
		0.155804 0.340563
		0.426479 0.271225
		0.591781 -0.136378
		0.280419 -0.341094
		-0.0742878 -0.441917
		-0.401475 -0.246925
		-0.396386 -0.0218349
		-0.0984647 -0.425442
		-0.119973 -0.425529
		-0.135651 -0.412528
		-0.186729 -0.466823
		-0.196334 -0.436531
		-0.205812 -0.424097
		-0.262624 -0.488772
		-0.288676 -0.451057
		-0.346608 -0.452516
		-0.333546 -0.411373
		-0.484059 -0.566859
		-0.462191 -0.496855
		-0.462499 -0.470808
		-0.452466 -0.44182
		-0.436091 -0.344967
		-0.398069 -0.301451
		-0.39264 -0.28285
		-0.401148 -0.208388
		-0.456885 -0.217564
		-0.416312 -0.201039
		-0.414152 -0.192096
		-0.426589 -0.178196
		-0.428185 -0.145689
		-0.429609 -0.141435
		-0.470065 -0.123908
		-0.38305 -0.0921862
		-0.455061 -0.093634
		-0.45803 -0.0788413
		-0.436497 -0.0595224
		-0.430242 -0.0466095
		-0.430937 -0.0396679
		-0.395793 -0.0343456
		-0.396041 -0.0313533
		-0.388876 -0.0242039
		-0.38914 -0.0133039
		-0.381701 -0.00327643
		-0.381701 -0.00327643
		-0.349402 0.0176912
		-0.346399 0.0278881
		-0.346399 0.0278881
		-0.347093 0.0354478
		-0.345004 0.0436714
		-0.345004 0.0436714
		-0.349566 0.0309742
		-0.342216 0.037385
		-0.342216 0.037385
		-0.347036 0.0359996
		-0.350381 0.0494314
		-0.348395 0.0753671
		-0.399723 0.116313
		-0.399723 0.116313
		-0.389916 0.109813
		-0.359362 0.113483
		-0.359362 0.113483
		-0.347961 0.121577
		-0.364375 0.130345
		-0.364375 0.130345
		-0.335712 0.136172
		-0.335933 0.137061
		-0.335933 0.137061
		-0.334908 0.139545
		-0.336959 0.134517
		-0.336959 0.134517
		-0.347046 0.134735
		-0.348411 0.131166
	};
\addlegendentry{Pred}
\addplot [draw=red, mark=o, only marks]
table{%
		x  y
		0.0348806381225586 2.39156436920166
		0.00684881210327148 2.39474391937256
		-0.0506510734558105 2.39443731307983
		-0.0847983360290527 2.39494776725769
		-0.116747379302979 2.39262461662292
		-0.183626651763916 2.38090682029724
		-0.2149658203125 2.37380695343018
		-0.245267391204834 2.3670642375946
		-0.277576446533203 2.3602819442749
		2.50666379928589 -1.00189578533173
		2.50902795791626 -0.959123849868774
		1.83770847320557 3.71651005744934
		1.51819849014282 3.96444225311279
		1.49879360198975 3.97521281242371
		0.990242958068848 4.0697455406189
		0.950779438018799 4.07549095153809
		0.912266731262207 4.08549046516418
		0.875215530395508 4.08731603622437
		0.801782608032227 4.09849834442139
		0.764955997467041 4.10351061820984
		0.728135108947754 4.10800647735596
		0.692924976348877 4.11366152763367
		0.654585838317871 4.11831283569336
		0.617834091186523 4.12234282493591
		0.578701019287109 4.12350106239319
		0.541058540344238 4.12933993339539
		0.469583034515381 4.13605856895447
		0.43604850769043 4.1387894153595
		0.406670570373535 4.14127397537231
		0.373043537139893 4.14441609382629
		0.341972351074219 4.14491891860962
		0.309821128845215 4.14388227462769
		0.277794361114502 4.14080929756165
		0.245537757873535 4.13900971412659
		0.213803291320801 4.13511061668396
		0.14548921585083 4.13243436813354
		0.110097885131836 4.12884593009949
		0.0715456008911133 4.12525463104248
		0.0320000648498535 4.12077903747559
		-0.00858640670776367 4.11617660522461
		-0.0512504577636719 4.1110565662384
		-0.0957322120666504 4.10541963577271
		-0.138855934143066 4.1009213924408
		-0.224547386169434 4.09509682655334
		-0.269137859344482 4.09284043312073
		-0.313196420669556 4.09102916717529
		-0.355009794235229 4.09032320976257
		-0.39616847038269 4.09057021141052
		-0.436958074569702 4.09112596511841
		-0.477277755737305 4.09213161468506
		-0.516749382019043 4.09348702430725
		-0.55644416809082 4.09554505348206
		-0.595999240875244 4.09798312187195
		-0.635366916656494 4.10095930099487
		-0.710631608963013 4.10780835151672
		-0.746728181838989 4.11220002174377
		-0.782769918441772 4.11697292327881
		-0.81770133972168 4.12233328819275
		-0.850539207458496 4.1285240650177
		-0.884166240692139 4.13433241844177
		-0.949852705001831 4.14455962181091
		-0.98133373260498 4.1486132144928
		-1.01424217224121 4.15104651451111
		-1.04505228996277 4.15742349624634
		-1.07655382156372 4.16180324554443
		-1.10940170288086 4.1661422252655
		-1.14253664016724 4.1702983379364
		-1.17253875732422 4.17235922813416
		-3.36154180765152 4.20306253433228
		-3.42997771501541 4.15532231330872
		-4.25797804445028 0.627000331878662
		-2.76788175106049 -2.64669377356768
		-2.73875796794891 -2.66590511798859
		-2.67853403091431 -2.69939654320478
		-2.64605629444122 -2.71739530563354
		-2.58246302604675 -2.75436447560787
		-2.21209621429443 -2.9495512843132
		-2.15789270401001 -2.96867322921753
		-2.13267469406128 -2.97837886214256
		2.50759840011597 -0.918373942375183
		0.505406856536865 4.13331317901611
		-0.181143283843994 4.09793090820312
		-0.918081521987915 4.13978624343872
		-2.08188199996948 -2.99363964796066
		-2.10686039924622 -2.98757037520409
	};
\addlegendentry{Miss}


==> tikz/vis_localize/vis_loc_test1_clean.tex <==
\addplot[draw=steelblue31119180, fill=steelblue31119180, mark=*, mark size = 0.5, only marks]
table{%
		x  y
		-0.475712776184082 0.139563798904419
		-0.48016357421875 0.13003134727478
		-0.484662771224976 0.120531320571899
		-0.488897800445557 0.11302661895752
		-0.492714405059814 0.10748553276062
		-0.49623441696167 0.103432655334473
		-0.494987010955811 0.10337495803833
		-0.484137296676636 0.113415718078613
		-0.476642370223999 0.11933422088623
		-0.467615127563477 0.125444412231445
		-0.458095788955688 0.132659435272217
		-0.448736906051636 0.139361143112183
		-0.440921068191528 0.145599126815796
		-0.434382915496826 0.151087760925293
		-0.41616678237915 0.151306629180908
		-0.408305883407593 0.146421194076538
		-0.398385524749756 0.13956618309021
		-0.386202573776245 0.130125284194946
		-0.373197555541992 0.119078874588013
		-0.360451459884644 0.10615611076355
		-0.350766658782959 0.0905110836029053
		-0.346630573272705 0.0540013313293457
		-0.34872579574585 0.0342636108398438
		-0.351482629776001 0.0158054828643799
		-0.354551792144775 -0.000281810760498047
		-0.36111044883728 -0.0232803821563721
		-0.370930194854736 -0.0325417518615723
		-0.39378809928894 -0.0262100696563721
		-0.405186414718628 -0.0147974491119385
		-0.404563903808594 -0.0129768848419189
		-0.403174161911011 -0.00988960266113281
		-0.40070366859436 -0.0061955451965332
		-0.396726369857788 -0.00256896018981934
		-0.384414911270142 -0.00140118598937988
		-0.378307580947876 -0.00747132301330566
		-0.372807741165161 -0.0177080631256104
		-0.367538690567017 -0.032109260559082
		-0.361993312835693 -0.0495333671569824
		-0.357597589492798 -0.0695714950561523
		-0.352928876876831 -0.090815544128418
		-0.349136352539062 -0.111238241195679
		-0.345038414001465 -0.12778377532959
		-0.340015172958374 -0.140910148620605
		-0.332670927047729 -0.15178108215332
		-0.325768947601318 -0.16033673286438
		-0.31738805770874 -0.172533512115479
		-0.31549859046936 -0.164752721786499
		-0.312368869781494 -0.155733108520508
		-0.305740118026733 -0.142026424407959
		-0.29944920539856 -0.13015341758728
		-0.293302536010742 -0.120808362960815
		-0.286153316497803 -0.111964702606201
		-0.277831077575684 -0.103550910949707
		-0.269028186798096 -0.0956037044525146
		-0.259313583374023 -0.089726448059082
		-0.251208305358887 -0.084907054901123
		-0.244046688079834 -0.0823824405670166
		-0.237510681152344 -0.0842549800872803
		-0.218066692352295 -0.113818645477295
		-0.209716320037842 -0.130792617797852
		-0.199263095855713 -0.148705244064331
		-0.184657573699951 -0.168038845062256
		-0.166447162628174 -0.187976121902466
		-0.149294853210449 -0.205202341079712
		-0.13410758972168 -0.215509176254272
		-0.117977142333984 -0.218178272247314
		-0.100935459136963 -0.217293262481689
		-0.0872626304626465 -0.216602325439453
		-0.0734786987304688 -0.237581968307495
		-0.0733661651611328 -0.250401496887207
		-0.0754437446594238 -0.270983934402466
		-0.0851850509643555 -0.277148485183716
		-0.0912580490112305 -0.264797210693359
		-0.0913257598876953 -0.245682001113892
		-0.0878586769104004 -0.240110874176025
		-0.074927806854248 -0.222298383712769
		-0.0563206672668457 -0.215169906616211
		-0.0441403388977051 -0.214928865432739
		-0.0287599563598633 -0.215799808502197
		-0.0118660926818848 -0.219435453414917
		0.00651693344116211 -0.225900173187256
		0.0264759063720703 -0.233037233352661
		0.0472002029418945 -0.240463256835938
		0.0687074661254883 -0.247420787811279
		0.0879907608032227 -0.25345253944397
		0.10275411605835 -0.257692813873291
		0.113116264343262 -0.261159420013428
		0.129180431365967 -0.27150559425354
		0.134980201721191 -0.277616024017334
		0.138407230377197 -0.283980846405029
		0.140823364257812 -0.300868034362793
		0.139509201049805 -0.302407026290894
		0.138659477233887 -0.301776885986328
		0.138566970825195 -0.302284955978394
		0.138940334320068 -0.303348779678345
		0.13801383972168 -0.302705049514771
		0.136441230773926 -0.301114797592163
		0.136542797088623 -0.295439958572388
		0.135914325714111 -0.291039943695068
		0.14375638961792 -0.284742116928101
		0.150585174560547 -0.284840106964111
		0.159670352935791 -0.28556489944458
		0.170924186706543 -0.285479545593262
		0.184267997741699 -0.285270214080811
		0.209714889526367 -0.28423547744751
		0.22251033782959 -0.28141975402832
		0.234349250793457 -0.2767174243927
		0.243575096130371 -0.271186590194702
		0.249485969543457 -0.262547731399536
		0.247910976409912 -0.263566732406616
		0.255521297454834 -0.273554086685181
		0.261666774749756 -0.276744604110718
		0.269351005554199 -0.280841112136841
		0.278572082519531 -0.285514116287231
		0.288749694824219 -0.290963411331177
		0.299405097961426 -0.296522855758667
		0.312143325805664 -0.302227258682251
		0.325217247009277 -0.307610750198364
		0.349468231201172 -0.314567089080811
		0.360532760620117 -0.314177513122559
		0.378127574920654 -0.305584669113159
		0.383511066436768 -0.298526525497437
		0.386185169219971 -0.274831771850586
		0.384037017822266 -0.267829895019531
		0.380838871002197 -0.26068377494812
		0.377907752990723 -0.260178804397583
		0.375614643096924 -0.261584997177124
		0.369502544403076 -0.262701034545898
		0.365026473999023 -0.264458417892456
		0.345454216003418 -0.275667905807495
		0.333970546722412 -0.282252550125122
		0.321840286254883 -0.289541006088257
		0.309884548187256 -0.297092914581299
		0.299385547637939 -0.303168773651123
		0.290313243865967 -0.307686567306519
		0.281789302825928 -0.311065435409546
		0.273219108581543 -0.314868688583374
		0.262310981750488 -0.318504095077515
		0.251391410827637 -0.321002721786499
		0.232179164886475 -0.317836046218872
		0.227717399597168 -0.312403202056885
		0.230002403259277 -0.305433750152588
		0.237928867340088 -0.298861026763916
		0.254036903381348 -0.293991088867188
		0.277008533477783 -0.289056777954102
		0.304621696472168 -0.281209468841553
		0.334768295288086 -0.269120216369629
		0.363463401794434 -0.254126071929932
		0.387835502624512 -0.239358186721802
		0.405727386474609 -0.224400281906128
		0.417745590209961 -0.209673881530762
		0.423427104949951 -0.195384502410889
		0.418605327606201 -0.169075489044189
		0.411143779754639 -0.156472206115723
		0.39979076385498 -0.138320684432983
		0.397964477539062 -0.134185075759888
		0.399243354797363 -0.131262063980103
		0.411582946777344 -0.1285240650177
		0.419278621673584 -0.129027843475342
		0.4277024269104 -0.130073308944702
		0.438353538513184 -0.130678176879883
		0.44916296005249 -0.130324602127075
		0.461356163024902 -0.129501819610596
		0.500238418579102 -0.126250028610229
		0.512677192687988 -0.124185800552368
		0.524662494659424 -0.121276378631592
		0.534428596496582 -0.117805957794189
		0.54300594329834 -0.114422082901001
		0.537099838256836 -0.0961718559265137
		0.532195091247559 -0.0950329303741455
		0.52634859085083 -0.0966095924377441
		0.5101318359375 -0.104804039001465
		0.500622272491455 -0.109034299850464
		0.491445541381836 -0.112497329711914
		0.482985019683838 -0.115975856781006
		0.44776725769043 -0.131272554397583
		0.433121204376221 -0.142088890075684
		0.428156852722168 -0.144186019897461
		0.416577816009521 -0.14663553237915
		0.410492897033691 -0.146164178848267
		0.404528141021729 -0.144514083862305
		0.393879890441895 -0.134054660797119
		0.391788482666016 -0.12442946434021
		0.395020008087158 -0.110282897949219
		0.404316425323486 -0.0924298763275146
		0.419227600097656 -0.0730030536651611
		0.436414241790771 -0.0524382591247559
		0.452496528625488 -0.0307762622833252
		0.46465015411377 -0.00885963439941406
		0.470919132232666 0.0118618011474609
		0.471738338470459 0.0295846462249756
		0.468568325042725 0.0439534187316895
		0.461705207824707 0.0554640293121338
		0.452932834625244 0.0648679733276367
		0.443526268005371 0.0710468292236328
		0.434700489044189 0.0755090713500977
		0.426765441894531 0.0782167911529541
		0.417571544647217 0.0852377414703369
		0.419477462768555 0.0878434181213379
		0.423949241638184 0.091031551361084
		0.430417537689209 0.0950090885162354
		0.437716960906982 0.0991506576538086
		0.445755004882812 0.103963375091553
		0.454879760742188 0.110303163528442
		0.463923454284668 0.117713212966919
		0.472463130950928 0.125356197357178
		0.481566429138184 0.133115768432617
		0.489361763000488 0.140381574630737
		0.495473861694336 0.146354675292969
		0.501782417297363 0.152403593063354
		0.49962043762207 0.150851488113403
		0.495697975158691 0.146430969238281
		0.491469860076904 0.140134811401367
		0.486589908599854 0.132877826690674
		0.481780052185059 0.122764825820923
		0.477402210235596 0.109484434127808
		0.473172664642334 0.094106912612915
		0.468643188476562 0.0785017013549805
		0.464509010314941 0.0630860328674316
		0.459725379943848 0.0476391315460205
		0.453319549560547 0.0324914455413818
		0.445653915405273 0.0188322067260742
		0.438377857208252 0.00649428367614746
		0.429794788360596 -0.00443434715270996
		0.414921283721924 -0.0219359397888184
		0.407365798950195 -0.0268702507019043
		0.397269725799561 -0.0303847789764404
		0.384975433349609 -0.0333311557769775
		0.370035648345947 -0.0354053974151611
		0.352634906768799 -0.0358033180236816
		0.332738876342773 -0.0347392559051514
		0.310945987701416 -0.0302491188049316
		0.28757381439209 -0.0235538482666016
		0.263988971710205 -0.0162003040313721
		0.241765022277832 -0.00849199295043945
		0.221742630004883 0.000783681869506836
		0.20318078994751 0.0102345943450928
		0.186397075653076 0.0195605754852295
		0.174269199371338 0.0289134979248047
		0.166467189788818 0.0388715267181396
		0.161996364593506 0.0489127635955811
		0.163612842559814 0.0599124431610107
		0.16918420791626 0.072174072265625
		0.177433013916016 0.0861220359802246
		0.188727855682373 0.101404428482056
		0.202877521514893 0.11634373664856
		0.217136859893799 0.129003763198853
		0.229912757873535 0.138884782791138
		0.242195129394531 0.14531397819519
		0.253225803375244 0.150682210922241
		0.262510776519775 0.155666828155518
		0.271790981292725 0.160313367843628
		0.281164169311523 0.163785696029663
		0.302873134613037 0.166089057922363
		0.304895401000977 0.165116310119629
		0.308081150054932 0.158243179321289
		0.317511081695557 0.14007830619812
		0.320812225341797 0.134567975997925
		0.323647022247314 0.128568172454834
		0.324954986572266 0.122252702713013
		0.325276374816895 0.116429567337036
		0.324569702148438 0.110835313796997
		0.323533058166504 0.103705883026123
		0.324018001556396 0.100380659103394
		0.326784610748291 0.0914826393127441
		0.335169315338135 0.0750961303710938
		0.33757209777832 0.0675766468048096
		0.339141845703125 0.0583400726318359
		0.338962078094482 0.0467574596405029
		0.332902908325195 0.0206060409545898
		0.328428745269775 0.00525093078613281
		0.323375225067139 -0.0104110240936279
		0.309474468231201 -0.0437572002410889
		0.300365924835205 -0.0597870349884033
		0.290976524353027 -0.0738968849182129
		0.282667636871338 -0.086742639541626
		0.274199485778809 -0.0984318256378174
		0.265737056732178 -0.109603643417358
		0.257789611816406 -0.118470430374146
		0.242022037506104 -0.130192041397095
		0.224735736846924 -0.13561224937439
		0.216389179229736 -0.13598895072937
		0.19872522354126 -0.133257627487183
		0.190921306610107 -0.129929780960083
		0.185051441192627 -0.124285697937012
		0.167011737823486 -0.105079889297485
		0.161638259887695 -0.106391429901123
		0.165784358978271 -0.108232021331787
		0.174703121185303 -0.112935066223145
		0.185089111328125 -0.119543313980103
		0.196276187896729 -0.125423431396484
		0.213131904602051 -0.15262770652771
		0.205775737762451 -0.162504434585571
		0.193562507629395 -0.173283576965332
		0.177497386932373 -0.186003684997559
		0.156392097473145 -0.200410604476929
		0.134032249450684 -0.214765548706055
		0.111944198608398 -0.226467847824097
		0.0898861885070801 -0.23592472076416
		0.0696063041687012 -0.242912769317627
		0.0492334365844727 -0.247467041015625
		0.0171055793762207 -0.252387285232544
		0.00430774688720703 -0.252336740493774
		-0.00622081756591797 -0.252688646316528
		-0.0151019096374512 -0.252621173858643
		-0.0364909172058105 -0.257465362548828
		-0.0388088226318359 -0.259784460067749
		-0.043067455291748 -0.263568639755249
		-0.0425143241882324 -0.259778022766113
		-0.047370433807373 -0.262283563613892
		-0.0519828796386719 -0.247211456298828
		-0.0547966957092285 -0.241640329360962
		-0.0590348243713379 -0.232613563537598
		-0.0749993324279785 -0.210277080535889
		-0.0873661041259766 -0.197201490402222
		-0.102601528167725 -0.180588960647583
		-0.120834350585938 -0.161726474761963
		-0.140756607055664 -0.140568494796753
		-0.161011219024658 -0.118717193603516
		-0.182309627532959 -0.0955238342285156
		-0.203787803649902 -0.0707340240478516
		-0.221941471099854 -0.0440220832824707
		-0.247904300689697 0.000123023986816406
		-0.257389068603516 0.0181052684783936
		-0.265834331512451 0.0338494777679443
		-0.274196147918701 0.0470576286315918
		-0.283370971679688 0.0562930107116699
		-0.290090084075928 0.0641119480133057
		-0.297959566116333 0.0692861080169678
		-0.313383817672729 0.0778217315673828
		-0.321587085723877 0.0794146060943604
		-0.329018592834473 0.0806443691253662
		-0.336623191833496 0.0792453289031982
		-0.344444990158081 0.0784447193145752
		-0.351674556732178 0.0785534381866455
		-0.358558416366577 0.0796604156494141
		-0.365620374679565 0.0820145606994629
		-0.378693819046021 0.0917680263519287
		-0.384901285171509 0.101403474807739
		-0.391800880432129 0.113877296447754
		-0.398156881332397 0.12794041633606
		-0.405303239822388 0.144651651382446
		-0.413211822509766 0.163980007171631
		-0.422950029373169 0.186177492141724
		-0.432249546051025 0.20915699005127
		-0.443677663803101 0.234650373458862
		-0.455579280853271 0.261464357376099
		-0.4680495262146 0.288782358169556
		-0.480740547180176 0.316969394683838
		-0.494502782821655 0.343819618225098
		-0.506997585296631 0.369302988052368
		-0.519889354705811 0.393232107162476
		-0.532356739044189 0.41681981086731
		-0.542201995849609 0.43903374671936
		-0.548934698104858 0.460180521011353
		-0.552461862564087 0.478749513626099
		-0.554431676864624 0.494734525680542
		-0.554164409637451 0.508585214614868
		-0.551351070404053 0.52018404006958
		-0.540326118469238 0.538650989532471
		-0.528228521347046 0.5516517162323
		-0.523319005966187 0.556171655654907
		-0.51875901222229 0.559774875640869
		-0.509496688842773 0.57818603515625
		-0.506192207336426 0.586934089660645
		-0.50188136100769 0.597802400588989
		-0.496378183364868 0.610551357269287
		-0.49030065536499 0.625753879547119
		-0.483154535293579 0.642142057418823
		-0.473594903945923 0.660194158554077
		-0.462607622146606 0.679688215255737
		-0.450906038284302 0.700359106063843
		-0.438165664672852 0.722132682800293
		-0.423839330673218 0.745080947875977
		-0.409336566925049 0.768850803375244
		-0.392941474914551 0.79328727722168
		-0.377383232116699 0.81843090057373
		-0.359654188156128 0.843892097473145
		-0.341591835021973 0.868237257003784
		-0.323523998260498 0.890495538711548
		-0.306995868682861 0.910418510437012
		-0.288999557495117 0.928917646408081
		-0.269911766052246 0.945492267608643
		-0.250134468078613 0.960476398468018
		-0.229742050170898 0.973967552185059
		-0.208060264587402 0.985514402389526
		-0.185215473175049 0.994890213012695
		-0.160974502563477 1.00202345848083
		-0.135478496551514 1.00649857521057
		-0.108591079711914 1.00827670097351
		-0.0816740989685059 1.00731587409973
		-0.0534162521362305 1.00445103645325
		-0.0238981246948242 1.00028848648071
		0.00528669357299805 0.995312213897705
		0.0342493057250977 0.98904275894165
		0.0632443428039551 0.982847452163696
		0.0929851531982422 0.9762122631073
		0.123081207275391 0.969633340835571
		0.153232574462891 0.962374210357666
		0.183555126190186 0.955987691879272
		0.212356090545654 0.95012640953064
		0.270921230316162 0.934135675430298
		0.298911094665527 0.924891710281372
		0.324925899505615 0.916084051132202
		0.352818965911865 0.90650749206543
		0.38033390045166 0.897371292114258
		0.408624649047852 0.888093948364258
		0.437955379486084 0.877878904342651
		0.468069553375244 0.866084337234497
		0.498217582702637 0.852882146835327
		0.528214454650879 0.838371992111206
		0.558545112609863 0.821885108947754
		0.587999820709229 0.803868293762207
		0.617506980895996 0.783855676651001
		0.647718906402588 0.761553049087524
		0.674814224243164 0.738767623901367
		0.701378345489502 0.713350772857666
		0.724745273590088 0.688522338867188
		0.745468616485596 0.664853811264038
		0.765552043914795 0.639255285263062
		0.78288459777832 0.613598823547363
		0.79861307144165 0.587558031082153
		0.813061237335205 0.560839176177979
		0.826841831207275 0.532722473144531
		0.839196681976318 0.503191232681274
		0.848245143890381 0.471790313720703
		0.854654788970947 0.440048933029175
		0.859573364257812 0.407224178314209
		0.863399505615234 0.373703002929688
		0.864762783050537 0.340895652770996
		0.864442348480225 0.308376550674438
		0.862275123596191 0.277302742004395
		0.858223915100098 0.248275756835938
		0.853150844573975 0.220256805419922
		0.847230434417725 0.192909955978394
		0.841421127319336 0.166541576385498
		0.835236549377441 0.14272141456604
		0.828899383544922 0.119407176971436
		0.822700500488281 0.0958201885223389
		0.816460609436035 0.0714199542999268
		0.810808181762695 0.0473392009735107
		0.805733203887939 0.0222983360290527
		0.800402164459229 -0.00338029861450195
		0.794578075408936 -0.0295500755310059
		0.788138389587402 -0.055478572845459
		0.78176736831665 -0.0832867622375488
		0.774805068969727 -0.112417221069336
		0.767723083496094 -0.143109083175659
		0.760618209838867 -0.17512321472168
		0.7532639503479 -0.21000075340271
		0.745965003967285 -0.245792388916016
		0.738360404968262 -0.282887935638428
		0.730146884918213 -0.320350885391235
		0.721342086791992 -0.357373952865601
		0.710628986358643 -0.394152402877808
		0.698646068572998 -0.428880214691162
		0.657362937927246 -0.521860361099243
		0.64145040512085 -0.549778461456299
		0.624608993530273 -0.575902700424194
		0.607239723205566 -0.599847197532654
		0.588366508483887 -0.622284770011902
		0.568402290344238 -0.643708944320679
		0.547265529632568 -0.663846254348755
		0.52375602722168 -0.684187531471252
		0.499780654907227 -0.702359557151794
		0.473758697509766 -0.720627427101135
		0.446412563323975 -0.737960815429688
		0.417838573455811 -0.754318952560425
		0.388992309570312 -0.769166707992554
		0.359073162078857 -0.782992005348206
		0.329636573791504 -0.796103477478027
		0.300580978393555 -0.809238791465759
		0.271152019500732 -0.822140336036682
		0.243062019348145 -0.833965659141541
		0.21561336517334 -0.844884872436523
		0.187674522399902 -0.855868101119995
		0.158923625946045 -0.866855978965759
		0.131221294403076 -0.87742805480957
		0.102925777435303 -0.88866662979126
		0.0739636421203613 -0.899849891662598
		0.0439496040344238 -0.91117250919342
		0.0129146575927734 -0.922146797180176
		-0.0196795463562012 -0.933053135871887
		-0.0537261962890625 -0.942923069000244
		-0.0897884368896484 -0.951091289520264
		-0.127527236938477 -0.957845568656921
		-0.166604042053223 -0.962430953979492
		-0.206568717956543 -0.965288281440735
		-0.247217178344727 -0.96538507938385
		-0.288166522979736 -0.96311092376709
		-0.329178333282471 -0.958763957023621
		-0.368557453155518 -0.950914263725281
		-0.405108451843262 -0.939173340797424
		-0.440417528152466 -0.923030614852905
		-0.473879098892212 -0.902953028678894
		-0.503445386886597 -0.880014181137085
		-0.529167890548706 -0.855117559432983
		-0.551555395126343 -0.82848048210144
		-0.569809436798096 -0.800993800163269
		-0.586248874664307 -0.773085951805115
		-0.597811222076416 -0.744176626205444
		-0.607747077941895 -0.716200709342957
		-0.613790035247803 -0.686839938163757
		-0.618688106536865 -0.655681967735291
		-0.620568752288818 -0.624021172523499
		-0.618654489517212 -0.592276453971863
		-0.615419149398804 -0.559221982955933
		-0.612901210784912 -0.524705648422241
		-0.610964775085449 -0.489260673522949
		-0.607926607131958 -0.455189228057861
		-0.603689908981323 -0.422123908996582
		-0.599552392959595 -0.389879941940308
		-0.59548020362854 -0.357625722885132
		-0.592183589935303 -0.325899124145508
		-0.589895963668823 -0.295116424560547
		-0.588583946228027 -0.265467882156372
		-0.587278604507446 -0.238084316253662
		-0.586090326309204 -0.21272873878479
		-0.587850332260132 -0.164679765701294
		-0.590389251708984 -0.143239736557007
		-0.594301700592041 -0.126609563827515
		-0.599139928817749 -0.113186597824097
		-0.605550527572632 -0.101835489273071
		-0.613922595977783 -0.0925326347351074
		-0.623639106750488 -0.0827333927154541
		-0.634068727493286 -0.0717589855194092
		-0.656250238418579 -0.0506665706634521
		-0.668896198272705 -0.0389750003814697
		-0.680670022964478 -0.0275671482086182
		-0.691154718399048 -0.0174288749694824
		-0.710356950759888 -0.00017857551574707
		-0.719061374664307 0.00759434700012207
		-0.725793123245239 0.0149052143096924
		-0.731291055679321 0.022099494934082
		-0.747014999389648 0.0455987453460693
		-0.750281095504761 0.0568203926086426
		-0.75363826751709 0.0686643123626709
		-0.756863832473755 0.0817265510559082
		-0.761823654174805 0.114290237426758
		-0.763055801391602 0.133702993392944
		-0.764393329620361 0.1537766456604
		-0.766040086746216 0.172672748565674
		-0.767355442047119 0.190469980239868
		-0.769161701202393 0.20570707321167
		-0.771661281585693 0.219291925430298
		-0.774086236953735 0.231238126754761
		-0.779036998748779 0.249555110931396
		-0.769604206085205 0.222410202026367
		-0.765902757644653 0.206015110015869
		-0.761847734451294 0.187525749206543
		-0.757518768310547 0.167120695114136
		-0.753512382507324 0.144575119018555
		-0.750282049179077 0.120208501815796
		-0.747298002243042 0.0944588184356689
		-0.743875026702881 0.0675256252288818
		-0.740626335144043 0.0398380756378174
		-0.736815214157104 0.01287841796875
		-0.731963157653809 -0.011357307434082
		-0.725107669830322 -0.0335919857025146
		-0.717881917953491 -0.0545296669006348
		-0.7103271484375 -0.0755658149719238
		-0.701545476913452 -0.0947704315185547
		-0.691472053527832 -0.111368894577026
		-0.680073499679565 -0.125797510147095
		-0.667577505111694 -0.137928247451782
		-0.652133226394653 -0.149919748306274
		-0.635656118392944 -0.160703897476196
		-0.617653131484985 -0.171041250228882
		-0.598726034164429 -0.180262565612793
		-0.578066349029541 -0.190841913223267
		-0.555577516555786 -0.201057434082031
		-0.509512424468994 -0.220014095306396
		-0.485393285751343 -0.229013204574585
		-0.460012674331665 -0.238246440887451
		-0.4352867603302 -0.248354911804199
		-0.41011905670166 -0.258070468902588
		-0.384690999984741 -0.267657279968262
		-0.359653949737549 -0.276645183563232
		-0.335649013519287 -0.286207675933838
		-0.31182599067688 -0.29650354385376
		-0.289180755615234 -0.307836294174194
		-0.267637729644775 -0.320336818695068
		-0.24760103225708 -0.33472752571106
		-0.22847318649292 -0.349688053131104
		-0.210632801055908 -0.364865303039551
		-0.19361686706543 -0.379155158996582
		-0.176737785339355 -0.393926382064819
		-0.158020496368408 -0.406778335571289
		-0.138083934783936 -0.417801856994629
		-0.119011878967285 -0.426871776580811
		-0.101283550262451 -0.434321641921997
		-0.084444522857666 -0.43945050239563
		-0.0684695243835449 -0.441160678863525
		-0.0525670051574707 -0.440855979919434
		-0.0359859466552734 -0.438445329666138
		-0.0187258720397949 -0.433384656906128
		-0.00103235244750977 -0.426134347915649
		0.0175786018371582 -0.416799068450928
		0.0368180274963379 -0.40570592880249
		0.0562801361083984 -0.393829107284546
		0.0756058692932129 -0.380057334899902
		0.0935158729553223 -0.366219997406006
		0.110140800476074 -0.352065324783325
		0.127132415771484 -0.337311029434204
		0.144192695617676 -0.321071624755859
		0.159880638122559 -0.302901744842529
		0.17364501953125 -0.283389329910278
		0.187992095947266 -0.262850522994995
		0.203932762145996 -0.241878032684326
		0.221642017364502 -0.219441890716553
		0.240053653717041 -0.195604085922241
		0.259304046630859 -0.171033143997192
		0.278057098388672 -0.145843029022217
		0.296329498291016 -0.119817972183228
		0.314387798309326 -0.0946147441864014
		0.330929279327393 -0.0687880516052246
		0.346407890319824 -0.0420989990234375
		0.361673355102539 -0.0143969058990479
		0.376054763793945 0.0138068199157715
		0.387606620788574 0.0414309501647949
		0.397636890411377 0.0663933753967285
		0.405519008636475 0.0884754657745361
		0.415902614593506 0.132177591323853
		0.416234493255615 0.151044845581055
		0.41546106338501 0.170459747314453
		0.394092082977295 0.260523319244385
		0.386957168579102 0.277479410171509
		0.380415439605713 0.294589281082153
		0.376338005065918 0.313321590423584
		0.372751235961914 0.332738637924194
		0.366763591766357 0.351131200790405
		0.358230113983154 0.367668390274048
		0.350014209747314 0.384257793426514
		0.340785503387451 0.401687145233154
		0.331520557403564 0.420798301696777
		0.323375701904297 0.441179037094116
		0.310941219329834 0.482294082641602
		0.308172702789307 0.502575397491455
		0.308783054351807 0.524256467819214
		0.310308456420898 0.546392917633057
		0.311174392700195 0.568055868148804
		0.313054084777832 0.590389490127563
		0.314286708831787 0.612309217453003
		0.349265575408936 0.737952947616577
		-0.0771465301513672 0.892141580581665
		-0.103035926818848 0.898790597915649
		-0.127203941345215 0.904443979263306
		-0.152550220489502 0.909306049346924
		-0.177211761474609 0.913433074951172
		-0.199509143829346 0.915637254714966
		-0.22012996673584 0.915960550308228
		-0.239708423614502 0.914646625518799
		-0.257837295532227 0.913088321685791
		-0.275170803070068 0.910592794418335
		-0.291835784912109 0.905678749084473
		-0.307930946350098 0.899218320846558
		-0.323544025421143 0.891928434371948
		-0.339160203933716 0.884451150894165
		-0.35645604133606 0.877817630767822
		-0.374419689178467 0.872951984405518
		-0.39461612701416 0.867832660675049
		-0.413528680801392 0.863002300262451
		-0.434149026870728 0.858445167541504
		-0.454180955886841 0.855116605758667
		-0.474398612976074 0.850518226623535
		-0.495420932769775 0.84687876701355
		-0.519164323806763 0.843543529510498
		-0.545945405960083 0.841277599334717
		-0.573398351669312 0.839277029037476
		-0.640521287918091 0.839683055877686
		-0.675939798355103 0.841784715652466
		-0.711319923400879 0.844024896621704
		-0.745542287826538 0.845655918121338
		-0.77782940864563 0.847686767578125
		-0.807354927062988 0.848468542098999
		-0.835324048995972 0.848407745361328
		-0.861037731170654 0.84616494178772
		-0.884045362472534 0.84143590927124
		-0.905376434326172 0.835734367370605
		-0.924411058425903 0.82956337928772
		-0.943338871002197 0.822526931762695
		-0.959426403045654 0.81410551071167
		-0.974107503890991 0.80456280708313
		-0.987156391143799 0.793249130249023
		-1.00044560432434 0.78156590461731
		-1.01171278953552 0.767951488494873
		-1.03818464279175 0.719378709793091
		-1.04438638687134 0.699389934539795
		-1.05596685409546 0.655285835266113
		-1.06922245025635 0.579573392868042
		-1.07759428024292 0.553168773651123
		-1.08566737174988 0.525724649429321
		-1.09551954269409 0.498144865036011
		-1.10556650161743 0.470243215560913
		-1.11692070960999 0.443197011947632
		-1.12974572181702 0.417119026184082
		-1.14465951919556 0.391692399978638
		-1.16202735900879 0.367180347442627
		-1.1812846660614 0.343663454055786
		-1.2021279335022 0.320536375045776
		-1.2240252494812 0.297778129577637
		-1.24555158615112 0.275411128997803
		-1.26656818389893 0.253067493438721
		-1.28825283050537 0.23053240776062
		-1.30957126617432 0.20690131187439
		-1.32879257202148 0.183419704437256
		-1.34500527381897 0.160382032394409
		-1.35969018936157 0.138440370559692
		-1.37283277511597 0.117492437362671
		-1.3844850063324 0.0970406532287598
		-1.393630027771 0.077899694442749
		-1.40196681022644 0.059185266494751
		-1.40856981277466 0.0402343273162842
		-1.41422247886658 0.0213611125946045
		-1.41884565353394 0.00356006622314453
		-1.42154002189636 -0.0142605304718018
		-1.42318940162659 -0.0323963165283203
		-1.42362236976624 -0.0703063011169434
		-1.42239260673523 -0.0912046432495117
		-1.41909909248352 -0.112357616424561
		-1.41440534591675 -0.134867906570435
		-1.4093804359436 -0.158769130706787
		-1.40293455123901 -0.184844255447388
		-1.39639210700989 -0.212805509567261
		-1.38781332969666 -0.27105450630188
		-1.38315677642822 -0.300517559051514
		-1.37774538993835 -0.330165386199951
		-1.37339043617249 -0.360459327697754
		-1.36982464790344 -0.392401456832886
		-1.36742043495178 -0.424032926559448
		-1.36534738540649 -0.45495080947876
		-1.36543130874634 -0.485974550247192
		-1.36722660064697 -0.516673803329468
		-1.37010622024536 -0.54721212387085
		-1.37366080284119 -0.577129364013672
		-1.37686896324158 -0.604763627052307
		-1.37926173210144 -0.631255626678467
		-1.38275146484375 -0.655606508255005
		-1.38498687744141 -0.680518627166748
		-1.38651609420776 -0.705329537391663
		-1.38539028167725 -0.729177355766296
		-1.3840913772583 -0.751536726951599
		-1.38346815109253 -0.772741556167603
		-1.38135361671448 -0.79314661026001
		-1.37803649902344 -0.811916351318359
		-1.37165331840515 -0.83073103427887
		-1.36466312408447 -0.849750399589539
		-1.35562539100647 -0.869269132614136
		-1.34518647193909 -0.889382719993591
		-1.33293962478638 -0.909808278083801
		-1.3187940120697 -0.930265307426453
		-1.30283188819885 -0.951046228408813
		-1.28592348098755 -0.971583247184753
		-1.26674222946167 -0.991960883140564
		-1.2476954460144 -1.01371097564697
		-1.22875738143921 -1.03751075267792
		-1.20744609832764 -1.06155121326447
		-1.18541169166565 -1.0843790769577
		-1.16442084312439 -1.10666763782501
		-1.1441810131073 -1.1282547712326
		-1.12445902824402 -1.14823436737061
		-1.10490369796753 -1.16666042804718
		-1.08558082580566 -1.1844310760498
		-1.06659197807312 -1.20172131061554
		-1.04832196235657 -1.21831595897675
		-1.03042697906494 -1.2346156835556
		-1.01287293434143 -1.25140452384949
		-0.996163845062256 -1.26929199695587
		-0.980551719665527 -1.28842079639435
		-0.965555429458618 -1.30863332748413
		-0.950004816055298 -1.32948160171509
		-0.934775829315186 -1.34865164756775
		-0.919826745986938 -1.36704313755035
		-0.904102802276611 -1.38577842712402
		-0.886617422103882 -1.40567374229431
		-0.867335319519043 -1.42653572559357
		-0.847383499145508 -1.44705355167389
		-0.828514337539673 -1.46608257293701
		-0.811046838760376 -1.48377859592438
		-0.794135570526123 -1.50002300739288
		-0.777018308639526 -1.51480090618134
		-0.759332180023193 -1.52780890464783
		-0.741383790969849 -1.53920316696167
		-0.723081350326538 -1.54952669143677
		-0.703518390655518 -1.55907297134399
		-0.682607173919678 -1.56704163551331
		-0.660017967224121 -1.57362425327301
		-0.636722564697266 -1.57851707935333
		-0.612234354019165 -1.58195179700851
		-0.586457014083862 -1.58453363180161
		-0.560209989547729 -1.58753657341003
		-0.533539056777954 -1.59100604057312
		-0.505252361297607 -1.59477227926254
		-0.477203845977783 -1.59917253255844
		-0.449627161026001 -1.60420197248459
		-0.422936201095581 -1.60877197980881
		-0.396540403366089 -1.61306059360504
		-0.369686603546143 -1.61795848608017
		-0.341370582580566 -1.62219375371933
		-0.311478137969971 -1.62600874900818
		-0.281677722930908 -1.62950885295868
		-0.251367568969727 -1.63237982988358
		-0.220885276794434 -1.63472723960876
		-0.189516544342041 -1.63752090930939
		-0.157893180847168 -1.64131784439087
		-0.126617908477783 -1.64587354660034
		-0.0958166122436523 -1.65038418769836
		-0.0655584335327148 -1.65478658676147
		-0.0352721214294434 -1.65827614068985
		-0.00374841690063477 -1.66158729791641
		0.0277552604675293 -1.66481399536133
		0.0580167770385742 -1.66786795854568
		0.0863537788391113 -1.6704740524292
		0.113113880157471 -1.67180967330933
		0.138965129852295 -1.67214679718018
		0.164598941802979 -1.6712287068367
		0.194170475006104 -1.67026317119598
		0.223477363586426 -1.66731441020966
		0.253528594970703 -1.66237789392471
		0.406907081604004 -1.61055964231491
		0.438739776611328 -1.59540581703186
		0.470752239227295 -1.57963824272156
		0.503418445587158 -1.5646425485611
		0.537535667419434 -1.54839432239532
		0.769270420074463 -1.4526686668396
		0.803145885467529 -1.44112813472748
		0.834123134613037 -1.42723560333252
		0.956114768981934 -1.38370990753174
		0.983589172363281 -1.3732922077179
		1.00933218002319 -1.36105251312256
		1.06125926971436 -1.33309471607208
		1.6235203742981 -0.428878784179688
		1.63295316696167 -0.404431819915771
		1.64113235473633 -0.379792451858521
		1.64847040176392 -0.354336023330688
		1.65468120574951 -0.328134059906006
		1.66056871414185 -0.300351619720459
		1.66580820083618 -0.270761489868164
		1.66995620727539 -0.239458084106445
		1.673424243927 -0.207259893417358
		1.67653131484985 -0.173421382904053
		1.67898845672607 -0.138564586639404
		1.68178701400757 -0.103179454803467
		1.68339967727661 -0.0660345554351807
		1.68313074111938 -0.0278937816619873
		1.68244743347168 0.00902271270751953
		1.68320274353027 0.0454325675964355
		1.68390274047852 0.0835318565368652
		1.68568277359009 0.121679782867432
		1.68696022033691 0.159290313720703
		1.68765687942505 0.196160793304443
		1.68779277801514 0.232713460922241
		1.68733406066895 0.269269227981567
		1.68615627288818 0.305814981460571
		1.68452787399292 0.34220814704895
		1.68253469467163 0.378530740737915
		1.6795597076416 0.414657115936279
		1.67606544494629 0.450713634490967
		1.67270469665527 0.485814809799194
		1.66941547393799 0.519673347473145
		1.66573524475098 0.551533222198486
		1.66047954559326 0.580873727798462
		1.6543402671814 0.607470750808716
		1.64925527572632 0.631947994232178
		1.64482069015503 0.657304525375366
		1.6411190032959 0.681826591491699
		1.63750839233398 0.704970359802246
		1.62708473205566 0.747475147247314
		1.62175941467285 0.769228935241699
		1.61561012268066 0.790820837020874
		1.60856580734253 0.814151048660278
		1.60143327713013 0.839084148406982
		1.59309577941895 0.865492820739746
		1.58275413513184 0.891013383865356
		1.57043600082397 0.917715311050415
		1.52076721191406 1.00522422790527
		1.48705148696899 1.06638813018799
		1.42788887023926 1.17068076133728
		1.40828990936279 1.20570063591003
		1.38775205612183 1.24042820930481
		1.34559392929077 1.31070899963379
		1.30250549316406 1.38341999053955
		1.28173542022705 1.42011833190918
		1.24328088760376 1.49331617355347
		1.22635650634766 1.52858471870422
		1.21079301834106 1.56264567375183
		0.279900550842285 2.31785464286804
		0.254583835601807 2.32567501068115
		0.229955673217773 2.3338668346405
		0.206756114959717 2.34287858009338
		0.15880823135376 2.36259603500366
		0.135116100311279 2.36922979354858
		0.111289978027344 2.37606930732727
		0.0618014335632324 2.38764262199402
		-0.150369644165039 2.38737654685974
		-0.310161352157593 2.3532121181488
		-0.340095996856689 2.34732604026794
		-0.369425773620605 2.34252643585205
		-0.399203300476074 2.33772802352905
		-0.42923641204834 2.33288931846619
		-0.459766626358032 2.32752871513367
		-0.490379810333252 2.3218207359314
		-0.522181987762451 2.31597566604614
		-0.55480432510376 2.30905413627625
		-0.58782958984375 2.30206775665283
		-0.621176242828369 2.29491662979126
		-0.654132127761841 2.28933238983154
		-0.687326192855835 2.2845151424408
		-0.720879793167114 2.27963376045227
		-0.753679513931274 2.27425670623779
		-0.783764362335205 2.2681782245636
		-0.81511116027832 2.26283931732178
		-0.84791111946106 2.25803565979004
		-0.882334232330322 2.25269794464111
		-0.916018009185791 2.24679350852966
		-0.947361469268799 2.23924374580383
		-0.981632709503174 2.23131442070007
		-1.00900077819824 2.22099757194519
		-1.03934240341187 2.21077513694763
		-1.07042169570923 2.19663023948669
		-1.10250520706177 2.1812105178833
		-1.13425517082214 2.1641538143158
		-1.16610765457153 2.14611482620239
		-1.19898819923401 2.12581825256348
		-1.23128485679626 2.10582566261292
		-1.26612114906311 2.08402228355408
		-1.29942989349365 2.06244111061096
		-1.33362197875977 2.04235982894897
		-1.36534929275513 2.02273631095886
		-1.40055131912231 2.00250387191772
		-1.4348201751709 1.98262286186218
		-1.46832084655762 1.96368837356567
		-1.5029878616333 1.94602727890015
		-1.5411479473114 1.92815399169922
		-1.57450652122498 1.91064715385437
		-1.6095929145813 1.89277267456055
		-1.64395570755005 1.87572932243347
		-1.67663216590881 1.85897159576416
		-1.70660948753357 1.84299373626709
		-1.73975443840027 1.82700753211975
		-1.77373862266541 1.8108856678009
		-1.83015704154968 1.78078889846802
		-1.90257358551025 1.73876643180847
		-1.92771100997925 1.72396087646484
		-1.95211005210876 1.70957064628601
		-1.97498416900635 1.6944375038147
		-1.99632143974304 1.67964363098145
		-2.01756238937378 1.66498708724976
		-2.03893661499023 1.64983034133911
		-2.05983686447144 1.63298606872559
		-2.08063530921936 1.61446356773376
		-2.10221433639526 1.59406900405884
		-2.12348532676697 1.5724823474884
		-2.14357447624207 1.54941606521606
		-2.16593980789185 1.52381467819214
		-2.18623614311218 1.49846315383911
		-2.20717883110046 1.47089600563049
		-2.22741532325745 1.43993735313416
		-2.2462956905365 1.40983057022095
		-2.26328206062317 1.38170766830444
		-2.27943921089172 1.35371208190918
		-2.29773199558258 1.32472157478333
		-2.31566762924194 1.29507756233215
		-2.33314919471741 1.26553702354431
		-2.34915232658386 1.23751020431519
		-2.36416685581207 1.21056222915649
		-2.37859559059143 1.18387699127197
		-2.39202523231506 1.15666127204895
		-2.40671873092651 1.12935185432434
		-2.41758620738983 1.10244679450989
		-2.42982041835785 1.0743842124939
		-2.44235527515411 1.04626870155334
		-2.46629595756531 0.990217447280884
		-2.47793924808502 0.963125228881836
		-2.48897469043732 0.936257839202881
		-2.49852514266968 0.908730983734131
		-2.50624287128448 0.883384943008423
		-2.55507278442383 0.766805171966553
		-2.56312501430511 0.743082046508789
		-2.57129347324371 0.718043565750122
		-2.57917749881744 0.691274404525757
		-2.58634638786316 0.66340446472168
		-2.59270334243774 0.634773015975952
		-2.59945571422577 0.604812383651733
		-2.60654664039612 0.572771549224854
		-2.61368417739868 0.540310144424438
		-2.62096869945526 0.504998922348022
		-2.62758481502533 0.469635486602783
		-2.63374650478363 0.431916952133179
		-2.63881754875183 0.396202325820923
		-2.64365470409393 0.363004922866821
		-2.64867854118347 0.328368902206421
		-2.65313029289246 0.292894124984741
		-2.65693140029907 0.257617712020874
		-2.6605429649353 0.224954128265381
		-2.66544985771179 0.191718816757202
		-2.67079341411591 0.157835721969604
		-2.67502284049988 0.124284982681274
		-2.6784462928772 0.0910201072692871
		-2.68211209774017 0.0571565628051758
		-2.6856597661972 0.0237395763397217
		-2.68919372558594 -0.00969147682189941
		-2.6932338476181 -0.0427958965301514
		-2.69813191890717 -0.0753779411315918
		-2.70251095294952 -0.104392528533936
		-2.70839035511017 -0.137597322463989
		-2.7126921415329 -0.166093826293945
		-2.71796214580536 -0.19374942779541
		-2.72342264652252 -0.222967624664307
		-2.72893142700195 -0.253115653991699
		-2.73447895050049 -0.281982421875
		-2.73923242092133 -0.309565782546997
		-2.74299395084381 -0.336159706115723
		-2.7451468706131 -0.362699747085571
		-2.74537551403046 -0.390228033065796
		-2.74378907680511 -0.418106317520142
		-2.74096155166626 -0.446968555450439
		-2.73668158054352 -0.477169752120972
		-2.7317430973053 -0.508008003234863
		-2.72557151317596 -0.540722131729126
		-2.71864080429077 -0.574871778488159
		-2.71061623096466 -0.609448552131653
		-2.70129454135895 -0.644609689712524
		-2.6905277967453 -0.680629253387451
		-2.67886400222778 -0.717106461524963
		-2.6673172712326 -0.752311229705811
		-2.65463697910309 -0.789408683776855
		-2.64236986637115 -0.827803254127502
		-2.63112545013428 -0.865175843238831
		-2.62102353572845 -0.901326298713684
		-2.61064875125885 -0.937251329421997
		-2.60043942928314 -0.973786115646362
		-2.58978402614594 -1.01025009155273
		-2.57893645763397 -1.04626965522766
		-2.56782758235931 -1.08245003223419
		-2.55666899681091 -1.11859428882599
		-2.54519855976105 -1.1552015542984
		-2.53366422653198 -1.19198095798492
		-2.52290534973145 -1.22778296470642
		-2.51320350170135 -1.26251196861267
		-2.50329458713531 -1.29652106761932
		-2.49304866790771 -1.32868719100952
		-2.48282408714294 -1.35920095443726
		-2.47191047668457 -1.38944625854492
		-2.46302127838135 -1.41858196258545
		-2.45534217357635 -1.4463963508606
		-2.44446957111359 -1.47234511375427
		-2.43424987792969 -1.49613070487976
		-2.42134249210358 -1.51895153522491
		-2.40863907337189 -1.54172730445862
		-2.39260590076447 -1.56381773948669
		-2.33537495136261 -1.63054805994034
		-2.31106078624725 -1.65425443649292
		-2.28736090660095 -1.67704099416733
		-2.25985908508301 -1.70025169849396
		-2.23019909858704 -1.72372609376907
		-2.19887137413025 -1.74912697076797
		-2.16682648658752 -1.77341520786285
		-2.13653635978699 -1.7984157204628
		-2.10426497459412 -1.82492816448212
		-2.07474207878113 -1.85125440359116
		-2.04470062255859 -1.87600284814835
		-2.01509594917297 -1.90213578939438
		-1.98608040809631 -1.93009912967682
		-1.9574990272522 -1.95792067050934
		-1.9300754070282 -1.98432910442352
		-1.90186023712158 -2.01142889261246
		-1.87359881401062 -2.03864073753357
		-1.84519171714783 -2.06586521863937
		-1.81597661972046 -2.09307414293289
		-1.78741240501404 -2.1189076602459
		-1.76104640960693 -2.14417916536331
		-1.73467302322388 -2.1683267056942
		-1.70934295654297 -2.1912028491497
		-1.68445491790771 -2.21133920550346
		-1.65966939926147 -2.22999203205109
		-1.63541865348816 -2.24848467111588
		-1.61203265190125 -2.26702144742012
		-1.58971524238586 -2.2849377989769
		-1.5673840045929 -2.30085781216621
		-1.54432034492493 -2.31549006700516
		-1.52030181884766 -2.32923766970634
		-1.49463629722595 -2.34254080057144
		-1.46833992004395 -2.35574577748775
		-1.44052004814148 -2.36896093189716
		-1.41103911399841 -2.38190983235836
		-1.37977242469788 -2.39502175152302
		-1.34667587280273 -2.40792129933834
		-1.31229043006897 -2.42054000496864
		-1.27611684799194 -2.43307012319565
		-1.23697113990784 -2.44605901837349
		-1.20029973983765 -2.45887637883425
		-1.16470146179199 -2.4717211201787
		-1.12725710868835 -2.48578376322985
		-1.08926844596863 -2.50131710618734
		-1.05238842964172 -2.51772248744965
		-1.01703119277954 -2.53395292535424
		-0.983861446380615 -2.5493841804564
		-0.951470851898193 -2.56420776620507
		-0.919610977172852 -2.57862347969785
		-0.888596773147583 -2.59209386538714
		-0.857147455215454 -2.60519089922309
		-0.82542085647583 -2.6174099855125
		-0.79365611076355 -2.62849796563387
		-0.762150764465332 -2.63885738700628
		-0.730725765228271 -2.64919175952673
		-0.700920581817627 -2.65919617563486
		-0.643120288848877 -2.67870170623064
		-0.614440441131592 -2.68613499403
		-0.58615517616272 -2.6925845593214
		-0.557061910629272 -2.69913183152676
		-0.52793550491333 -2.70639076083899
		-0.501125335693359 -2.71534219384193
		-0.474890232086182 -2.72438958287239
		-0.44826865196228 -2.73275418579578
		-0.421224117279053 -2.74102954566479
		-0.391674041748047 -2.74908554553986
		-0.362610340118408 -2.75483372807503
		-0.331282615661621 -2.76123031973839
		-0.297548532485962 -2.76681044697762
		-0.26157283782959 -2.77313280105591
		-0.187160015106201 -2.78901851177216
		-0.146848201751709 -2.79822327196598
		-0.0599956512451172 -2.81402134895325
		-0.0185279846191406 -2.82283216714859
		0.0240025520324707 -2.8329082429409
		0.0669064521789551 -2.84278526902199
		0.109373569488525 -2.85003280639648
		0.151431560516357 -2.85946771502495
		0.191341876983643 -2.86845707893372
		0.232278347015381 -2.87615031003952
		0.27153205871582 -2.8836835026741
		0.310129642486572 -2.89058798551559
		0.348493099212646 -2.89715033769608
		0.385982036590576 -2.90396782755852
		0.423657894134521 -2.90918472409248
		0.459821701049805 -2.91594570875168
		0.496395111083984 -2.92049819231033
		2.29180574417114 -2.07416784763336
		2.30596208572388 -2.0442481637001
		2.3211932182312 -2.01457870006561
		2.33689594268799 -1.985171854496
		2.35356521606445 -1.95499891042709
		2.36924982070923 -1.92544519901276
		2.38502883911133 -1.89737385511398
		2.39975595474243 -1.86874735355377
		2.51012420654297 -1.08475148677826
		2.51091289520264 -0.798977017402649
		2.51673984527588 -0.387422800064087
		2.5140962600708 -0.352558374404907
		2.50971937179565 -0.319583415985107
		2.50571012496948 -0.287270545959473
		2.49907541275024 -0.254826307296753
		2.49449491500854 -0.214574813842773
		2.48898935317993 -0.171088457107544
		2.48301029205322 -0.127415180206299
		2.47722053527832 -0.0802211761474609
		2.47077655792236 -0.0294284820556641
		2.46413278579712 0.0173079967498779
		2.45852136611938 0.0667934417724609
		2.45339727401733 0.116848707199097
		2.44881820678711 0.166456937789917
		2.44529294967651 0.213187456130981
		2.44277572631836 0.260267734527588
		2.44172239303589 0.307831764221191
		2.44064950942993 0.353001832962036
		2.44101619720459 0.399437665939331
		2.44167518615723 0.444752931594849
		2.44259452819824 0.489096641540527
		2.44437503814697 0.532661914825439
		2.44666957855225 0.575822114944458
		2.44977998733521 0.617964029312134
		2.45331573486328 0.656864881515503
		2.45689535140991 0.69455885887146
		2.46033096313477 0.730181455612183
		2.46403741836548 0.763455390930176
		2.46764802932739 0.796577453613281
		2.47222852706909 0.828947782516479
		2.47816514968872 0.859796047210693
		2.48332643508911 0.889948606491089
		2.48793697357178 0.918000459671021
		2.49196577072144 0.947416067123413
		2.49629068374634 0.978105068206787
		2.49954605102539 1.00915813446045
		2.50288248062134 1.04421544075012
		2.50583219528198 1.08066082000732
		2.50728702545166 1.12000942230225
		2.50651407241821 1.16194200515747
		2.50352430343628 1.20583319664001
		2.49963092803955 1.25229215621948
		2.49480438232422 1.30165266990662
		2.48987007141113 1.35134553909302
		2.48564720153809 1.39978361129761
		2.48208856582642 1.45026874542236
		2.47937059402466 1.49879837036133
		2.47700786590576 1.54741811752319
		2.47508382797241 1.59475755691528
		2.47278642654419 1.64081692695618
		2.4712438583374 1.68485593795776
		2.46966457366943 1.72858452796936
		2.46844100952148 1.77034568786621
		2.46754550933838 1.81110191345215
		2.46647024154663 1.85129356384277
		2.46329259872437 1.89035725593567
		2.4619574546814 1.92913150787354
		2.46200752258301 1.96401071548462
		2.45984172821045 1.99817514419556
		2.45761966705322 2.03080606460571
		2.45581293106079 2.06174731254578
		2.45387411117554 2.09077310562134
		2.45147609710693 2.11859011650085
		2.44816970825195 2.14579463005066
		2.44444227218628 2.17156004905701
		2.44025468826294 2.1965115070343
		2.43455839157104 2.22147536277771
		2.43018579483032 2.24539732933044
		2.42347049713135 2.27212691307068
		2.41743564605713 2.29834985733032
		2.41002702713013 2.32722878456116
		2.40144634246826 2.35683155059814
		2.39230012893677 2.38807082176208
		2.38174676895142 2.42027902603149
		2.37012910842896 2.45140767097473
		2.35784816741943 2.48862028121948
		2.34454154968262 2.52484560012817
		2.33202362060547 2.56064414978027
		2.32121992111206 2.59442758560181
		2.31048250198364 2.62879347801208
		2.11861371994019 3.37461233139038
		1.58058500289917 3.93439912796021
		1.55937147140503 3.94429039955139
		1.45819520950317 3.99499297142029
		1.41218185424805 4.01202487945557
		1.385573387146 4.01973009109497
		1.25929546356201 4.03858375549316
		1.22367525100708 4.04181981086731
		1.10778141021729 4.05534720420837
		1.07028961181641 4.05958986282349
		1.0305814743042 4.06476664543152
		-3.82414370775223 3.79132008552551
		-4.1596665084362 2.676926612854
		-4.16670659184456 2.64075040817261
		-4.17371195554733 2.60695505142212
		-4.17738965153694 2.57142376899719
		-4.18609333783388 2.53663730621338
		-4.18670164048672 2.50735378265381
		-4.19627466797829 2.44317150115967
		-4.21103971451521 2.32144474983215
		-4.20935282111168 2.29540371894836
		-4.20968658477068 2.2608425617218
		-4.20620309561491 2.22475552558899
		-4.20786896348 2.19141912460327
		-4.20828974992037 2.15073347091675
		-4.20619543641806 2.11229038238525
		-4.20442977547646 2.07479500770569
		-4.2040161266923 2.02928423881531
		-4.20181374996901 1.98470664024353
		-4.20385627448559 1.93955898284912
		-4.20545345544815 1.89935827255249
		-4.20952846109867 1.85276174545288
		-4.21714520454407 1.80208969116211
		-4.22210679203272 1.7588996887207
		-4.22874741256237 1.71305060386658
		-4.23479851707816 1.6707878112793
		-4.24120136350393 1.62881994247437
		-4.24839610606432 1.5873019695282
		-4.25360972434282 1.5457136631012
		-4.25900623947382 1.50419664382935
		-4.26284719258547 1.46238350868225
		-4.26626331172884 1.42074084281921
		-4.26885493844748 1.37931227684021
		-4.27121603488922 1.33762645721436
		-4.27303393930197 1.29781126976013
		-4.27447614818811 1.25935435295105
		-4.2765838522464 1.22175621986389
		-4.27821468003094 1.18630862236023
		-4.27991060353816 1.15098571777344
		-4.28133000992239 1.11767983436584
		-4.28482772130519 1.08298993110657
		-4.28516953345388 1.05089569091797
		-4.28501587174833 1.0174880027771
		-4.28457326348871 0.985489845275879
		-4.28289302438498 0.952000379562378
		-4.28265500254929 0.916829586029053
		-4.27911493182182 0.880947351455688
		-4.27630409598351 0.843485116958618
		-4.27383713424206 0.802809000015259
		-4.26959686726332 0.761577844619751
		-4.26608921028674 0.718852996826172
		-4.26321532391012 0.674260139465332
		-4.25418167561293 0.579790353775024
		-4.24977958574891 0.530970096588135
		-4.24693186953664 0.482069253921509
		-4.24485631287098 0.433767080307007
		-4.24440364167094 0.386854648590088
		-4.24354512244463 0.340838193893433
		-4.24263399094343 0.295625686645508
		-4.24144769087434 0.25081205368042
		-4.24038485810161 0.205930233001709
		-4.23921549320221 0.161624908447266
		-4.23757592588663 0.117404699325562
		-4.23542648926377 0.0736122131347656
		-4.23253225535154 0.031005859375
		-4.22966364771128 -0.011249303817749
		-4.22636525332928 -0.0515420436859131
		-4.22223431617022 -0.0907320976257324
		-4.21799114346504 -0.129073143005371
		-4.21535950899124 -0.165078163146973
		-4.21366623044014 -0.196521997451782
		-4.20830386132002 -0.229782819747925
		-4.20407105237246 -0.26090407371521
		-4.19729298353195 -0.288059711456299
		-4.1834372729063 -0.349525213241577
		-4.17608794569969 -0.379807949066162
		-4.16717550158501 -0.411098957061768
		-4.15682092308998 -0.443200826644897
		-4.14527183771133 -0.477459669113159
		-4.13223399221897 -0.512238264083862
		-4.11757835745811 -0.548268556594849
		-4.10173688828945 -0.585371851921082
		-4.08492965996265 -0.623841404914856
		-4.06741763651371 -0.665006399154663
		-2.96754837036133 -2.5100936666131
		-2.94735586643219 -2.52657172083855
		-2.87810015678406 -2.5770115358755
		-2.8514506816864 -2.59360602684319
		-2.82563555240631 -2.61183220334351
		-2.05663585662842 -2.99925199151039
		-2.03290820121765 -3.00431290268898
		-2.00595831871033 -3.00992795825005
		-1.98002099990845 -3.01537668704987
		-1.95394563674927 -3.01995036005974
		-1.92585968971252 -3.02453607320786
		-1.89684224128723 -3.02698829770088
		-1.86894369125366 -3.02812758088112
		-1.84121203422546 -3.02814793586731
		-1.81411910057068 -3.02639156579971
		-1.7867431640625 -3.02492702007294
		-1.76561403274536 -3.0225770175457
		-1.74574112892151 -3.0178214609623
		-1.72816395759583 -3.01353740692139
		-1.7135124206543 -3.01027265191078
		-1.67060613632202 -2.99560761451721
		-1.66427850723267 -2.99379333853722
		-1.65692496299744 -3.00601354241371
		-1.65792679786682 -3.00868371129036
		-1.66207098960876 -3.01574352383614
		-1.66236090660095 -3.01731204986572
		-1.6493091583252 -3.00330793857574
		-1.64426755905151 -2.99984154105186
		-1.63774490356445 -2.99701151251793
		-1.62326884269714 -2.99265360832214
		-1.6156599521637 -2.99131834506989
		-1.59878039360046 -2.98852199316025
		-1.5781877040863 -2.98502278327942
		-1.56599259376526 -2.98271310329437
		-1.55170798301697 -2.97940289974213
		-1.53504419326782 -2.97700735926628
		-1.51706838607788 -2.97525662183762
		-1.49450302124023 -2.97378075122833
		-1.47509765625 -2.97272634506226
		-1.4506528377533 -2.97208935022354
		-1.42367076873779 -2.97121644020081
		-1.39501333236694 -2.97107955813408
		-1.3644654750824 -2.97231164574623
		-1.33342838287354 -2.97437763214111
		-1.30103039741516 -2.97678118944168
		-1.26802158355713 -2.97996410727501
		-1.23500442504883 -2.98277714848518
		-1.20114278793335 -2.98504650592804
		-1.16715526580811 -2.98803558945656
		-1.13260769844055 -2.99141106009483
		-1.09819149971008 -2.99458742141724
		-1.06397271156311 -2.99819800257683
		-0.998855352401733 -3.00515681505203
		-0.967853784561157 -3.00805431604385
		-0.937385559082031 -3.01055896282196
		-0.90665078163147 -3.01173716783524
		-0.874955415725708 -3.01067760586739
		-0.808577537536621 -3.00484576821327
		-0.772720813751221 -3.00011810660362
		-0.735051870346069 -2.99458855390549
		-0.69523286819458 -2.98856514692307
		-0.653045892715454 -2.98187693953514
		-0.563559532165527 -2.96788403391838
		-0.14522123336792 -2.9391251206398
		-0.0597672462463379 -2.93881180882454
		-0.0181751251220703 -2.93933454155922
		0.105367183685303 -2.93970274925232
		0.146444320678711 -2.9394593834877
		0.186685562133789 -2.93931180238724
		0.226377964019775 -2.93883082270622
		0.265230655670166 -2.9382132589817
		0.300805568695068 -2.93776574730873
		0.335568904876709 -2.93737882375717
		0.370904922485352 -2.93704554438591
		0.405324459075928 -2.93630382418633
		0.438881397247314 -2.93404501676559
		2.17435836791992 -2.78757962584496
		2.07312345504761 -2.71348099410534
		2.06236982345581 -2.6830712556839
		2.05214929580688 -2.65330012887716
		2.03332185745239 -2.59877029433846
		2.02492618560791 -2.56251018494368
		1.97929382324219 -2.47538748383522
		1.94073438644409 -2.40861620008945
		1.92259407043457 -2.3872944265604
		1.90208196640015 -2.36588583886623
		1.87917232513428 -2.34837964177132
		1.85496139526367 -2.32487595081329
		1.82957315444946 -2.29801434278488
		1.80338621139526 -2.27601116895676
		1.74406623840332 -2.21913880109787
		1.7189507484436 -2.19203069806099
		1.69262170791626 -2.16593128442764
		1.64244556427002 -2.10721951723099
		1.61837863922119 -2.07457190752029
		1.57058906555176 -2.01604640483856
		1.54565286636353 -1.98650711774826
		1.52145719528198 -1.95610004663467
		1.44986867904663 -1.87479269504547
		1.42536926269531 -1.84347718954086
		1.4007740020752 -1.81670540571213
		1.37623357772827 -1.7889004945755
		1.35126161575317 -1.765829205513
		1.32710552215576 -1.74171191453934
		1.30432415008545 -1.71966928243637
		1.28198575973511 -1.70078784227371
		1.21338129043579 -1.63991332054138
		1.16199111938477 -1.6056923866272
		1.10488080978394 -1.57400059700012
		1.07449150085449 -1.55473792552948
		1.04306697845459 -1.53567349910736
		1.00961112976074 -1.52091157436371
		0.973335742950439 -1.5039644241333
		0.898318290710449 -1.46577334403992
		0.816562175750732 -1.42578864097595
		0.777291297912598 -1.40362441539764
		0.739748001098633 -1.38304674625397
		0.703005790710449 -1.36010468006134
		0.668007373809814 -1.33413589000702
		0.633259773254395 -1.30729389190674
		0.60081958770752 -1.28239107131958
		0.566814422607422 -1.25603842735291
		0.532726287841797 -1.22989284992218
		0.499220848083496 -1.20394432544708
		0.46537971496582 -1.17788088321686
		0.432822704315186 -1.15096068382263
		0.400049686431885 -1.12468898296356
		0.367897510528564 -1.09821355342865
		0.336660861968994 -1.07305634021759
		0.307440757751465 -1.04896855354309
		0.277522087097168 -1.02637577056885
		0.247017383575439 -1.00457739830017
		0.216916084289551 -0.985205173492432
		0.186448097229004 -0.966617584228516
		0.155266761779785 -0.947815656661987
		0.125396251678467 -0.929558396339417
		0.0959076881408691 -0.911806106567383
		0.0667314529418945 -0.893410086631775
		0.0363645553588867 -0.874421238899231
		0.00520133972167969 -0.855442523956299
		-0.0272154808044434 -0.835718870162964
		-0.0612826347351074 -0.815157532691956
		-0.0960116386413574 -0.793968319892883
		-0.130734443664551 -0.772088766098022
		-0.165922164916992 -0.749632120132446
		-0.200377941131592 -0.725830554962158
		-0.235208511352539 -0.701361775398254
		-0.269782543182373 -0.675049066543579
		-0.301742553710938 -0.648808121681213
		-0.329594850540161 -0.622746109962463
		-0.355880260467529 -0.59538209438324
		-0.380717039108276 -0.566305637359619
		-0.404174089431763 -0.536694765090942
		-0.427075624465942 -0.507186651229858
		-0.448946237564087 -0.477012872695923
		-0.469935894012451 -0.445830583572388
		-0.48877477645874 -0.412712097167969
		-0.507504940032959 -0.379825830459595
		-0.523527383804321 -0.345473527908325
		-0.538507699966431 -0.311203002929688
		-0.552841424942017 -0.276901006698608
		-0.565301418304443 -0.242959260940552
		-0.577220916748047 -0.209362983703613
		-0.58855938911438 -0.175933361053467
		-0.59973931312561 -0.141176462173462
		-0.609078645706177 -0.109683513641357
		-0.616737127304077 -0.080751895904541
		-0.622649669647217 -0.0509903430938721
		-0.628238201141357 -0.0207855701446533
		-0.635458707809448 0.00931954383850098
		-0.643556118011475 0.0402882099151611
		-0.651140689849854 0.0719368457794189
		-0.658101558685303 0.10407543182373
		-0.664508104324341 0.136897325515747
		-0.670377731323242 0.170685052871704
		-0.675612688064575 0.206317663192749
		-0.679100513458252 0.243142604827881
		-0.681045055389404 0.281492233276367
		-0.684248924255371 0.359079122543335
		-0.682765483856201 0.398490428924561
		-0.680221557617188 0.435830116271973
		-0.675568103790283 0.47168493270874
		-0.667203187942505 0.506792306900024
		-0.656699657440186 0.542487621307373
		-0.644065856933594 0.5770263671875
		-0.629070043563843 0.610405921936035
		-0.547400951385498 0.724396705627441
		-0.521059513092041 0.748488187789917
		-0.492045164108276 0.770983457565308
		-0.461901903152466 0.792261600494385
		-0.430648326873779 0.812301158905029
		-0.398018360137939 0.831261157989502
		-0.364010334014893 0.848019361495972
		-0.328376531600952 0.864441156387329
		-0.255277156829834 0.891423463821411
		-0.218183517456055 0.90111255645752
		-0.180343627929688 0.908562898635864
		-0.143445491790771 0.914277315139771
		-0.10714054107666 0.91960597038269
		-0.0709714889526367 0.924352407455444
		-0.0348954200744629 0.928344964981079
		0.00151395797729492 0.932253360748291
		0.0386314392089844 0.935134887695312
		0.075739860534668 0.936861038208008
		0.113154888153076 0.937446594238281
		0.150767803192139 0.936983585357666
		0.188944339752197 0.935603380203247
		0.227670669555664 0.933363676071167
		0.266463756561279 0.930252552032471
		0.305579662322998 0.925670385360718
		0.34449577331543 0.918662071228027
		0.380981922149658 0.90895938873291
		0.415079593658447 0.897632360458374
		0.448842525482178 0.883423566818237
		0.480967044830322 0.865925788879395
		0.51073694229126 0.846319675445557
		0.538800239562988 0.825078010559082
		0.564413070678711 0.802412033081055
		0.588239669799805 0.777213096618652
		0.611161231994629 0.750345945358276
		0.632898807525635 0.722244262695312
		0.652867794036865 0.69294548034668
		0.671199321746826 0.662543058395386
		0.68829345703125 0.631237268447876
		0.703159332275391 0.600261926651001
		0.715634346008301 0.56950306892395
		0.726748466491699 0.538830518722534
		0.737296581268311 0.508408308029175
		0.746474742889404 0.480378389358521
		0.753448963165283 0.45435357093811
		0.759535312652588 0.426355838775635
		0.764811515808105 0.397804260253906
		0.771056175231934 0.369369745254517
		0.777851581573486 0.341900587081909
		0.784536361694336 0.313913583755493
		0.792035579681396 0.285567998886108
		0.800614356994629 0.256142377853394
		0.809704303741455 0.225502967834473
		0.819454193115234 0.194146156311035
		0.829652309417725 0.160964965820312
		0.840110778808594 0.12628173828125
		0.849795341491699 0.090538501739502
		0.85797119140625 0.0544514656066895
		0.863979816436768 0.018322229385376
		0.867427825927734 -0.0165162086486816
		0.867900371551514 -0.0497832298278809
		0.865953922271729 -0.0818181037902832
		0.860862255096436 -0.112916231155396
		0.852774620056152 -0.141768455505371
		0.842184066772461 -0.169568061828613
		0.830191135406494 -0.196530818939209
		0.81524658203125 -0.222442626953125
		0.798420429229736 -0.246750593185425
		0.778918743133545 -0.270984888076782
		0.757312297821045 -0.294944286346436
		0.708244323730469 -0.340005397796631
		0.680900573730469 -0.361942052841187
		0.652328014373779 -0.382449865341187
		0.62255859375 -0.400696039199829
		0.591763973236084 -0.417586088180542
		0.561076641082764 -0.433994054794312
		0.530841827392578 -0.449265480041504
		0.499690055847168 -0.463799953460693
		0.467292785644531 -0.478108167648315
		0.43571138381958 -0.491402626037598
		0.406163692474365 -0.502818584442139
		0.377118110656738 -0.514632225036621
		0.348095893859863 -0.526409149169922
		0.318670272827148 -0.538020372390747
		0.289245128631592 -0.5503089427948
		0.259159564971924 -0.562934637069702
		0.228304386138916 -0.575451374053955
		0.196201324462891 -0.58827543258667
		0.163700103759766 -0.600040316581726
		0.128764629364014 -0.6104576587677
		0.0935449600219727 -0.620789408683777
		0.0567646026611328 -0.629667401313782
		0.0204238891601562 -0.635545015335083
		-0.0143508911132812 -0.637822151184082
		-0.0488944053649902 -0.635840535163879
		-0.0805091857910156 -0.632934927940369
		-0.113161563873291 -0.626247048377991
		-0.144683837890625 -0.616654515266418
		-0.174492359161377 -0.605078458786011
		-0.202998638153076 -0.591166496276855
		-0.230573654174805 -0.574578285217285
		-0.256010055541992 -0.555505990982056
		-0.280004978179932 -0.534609794616699
		-0.303425073623657 -0.511988639831543
		-0.326541662216187 -0.488833427429199
		-0.347731590270996 -0.464216947555542
		-0.368520498275757 -0.438265323638916
		-0.388209104537964 -0.412678480148315
		-0.405617713928223 -0.387486934661865
		-0.422074317932129 -0.362639188766479
		-0.43783974647522 -0.337647438049316
		-0.45269250869751 -0.313091039657593
		-0.466138124465942 -0.291240692138672
		-0.477127313613892 -0.269887685775757
		-0.48696756362915 -0.248616218566895
		-0.49686861038208 -0.227666616439819
		-0.508135318756104 -0.207389831542969
		-0.519225835800171 -0.184927225112915
		-0.530579805374146 -0.162606954574585
		-0.540906429290771 -0.139997720718384
		-0.551109075546265 -0.116265773773193
		-0.560221910476685 -0.0920288562774658
		-0.569478034973145 -0.0673706531524658
		-0.57762885093689 -0.0420577526092529
		-0.585057258605957 -0.0160865783691406
		-0.607199907302856 0.0627813339233398
		-0.610787391662598 0.0889711380004883
		-0.618768930435181 0.114238023757935
		-0.623031377792358 0.140683174133301
		-0.62691068649292 0.164891242980957
		-0.628286838531494 0.188154697418213
		-0.626328706741333 0.229560613632202
		-0.623257637023926 0.248366594314575
		-0.619644641876221 0.266180753707886
		-0.609172582626343 0.30049204826355
		-0.601079702377319 0.315871715545654
		-0.591888189315796 0.328700065612793
		-0.582172870635986 0.341063976287842
		-0.571691274642944 0.352863788604736
		-0.560601711273193 0.363513946533203
		-0.549024105072021 0.374831438064575
		-0.525317668914795 0.402263641357422
		-0.515031099319458 0.416720151901245
		-0.505024433135986 0.42948317527771
		-0.496411561965942 0.440706253051758
		-0.481375694274902 0.458633184432983
		-0.475879430770874 0.465291500091553
		-0.464586496353149 0.477438926696777
		-0.462545394897461 0.480718851089478
		-0.461005449295044 0.484076976776123
		-0.459953784942627 0.486122131347656
		-0.459135770797729 0.495852947235107
		-0.460515022277832 0.509134292602539
		-0.460334062576294 0.513065099716187
		-0.460330724716187 0.516794204711914
		-0.460898160934448 0.524644374847412
		-0.473724126815796 0.529650926589966
		-0.484831809997559 0.530839204788208
		-0.488232135772705 0.531748294830322
		-0.491442680358887 0.531158447265625
		-0.494639158248901 0.531203746795654
	};
\addlegendentry{MOCAP}
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.471813 -0.21331
		-0.441062 -0.201245
		-0.441062 -0.201245
		-0.56084 -0.268602
		-0.514195 -0.237621
		-0.514195 -0.237621
		-0.510642 -0.251453
		-0.534535 -0.265227
		-0.512931 -0.246751
		-0.518666 -0.238782
		-0.502524 -0.245551
		-0.54931 -0.276751
		-0.53299 -0.250344
		-0.519408 -0.237164
		-0.53013 -0.244831
		-0.492816 -0.221767
		-0.4882 -0.231752
		-0.492564 -0.222325
		-0.445873 -0.225539
		-0.506175 -0.246085
		-0.405837 -0.217529
		-0.377665 -0.2003
		-0.403763 -0.239267
		-0.407127 -0.237491
		-0.425957 -0.282793
		-0.373588 -0.247483
		-0.413719 -0.285202
		-0.401608 -0.283386
		-0.50172 -0.362715
		-0.468808 -0.340396
		-0.46353 -0.344105
		-0.381156 -0.285008
		-0.480875 -0.417774
		-0.45928 -0.398183
		-0.438766 -0.389327
		-0.423699 -0.363458
		-0.485881 -0.413812
		-0.426484 -0.385278
		-0.433532 -0.389122
		-0.451602 -0.411361
		-0.411471 -0.384725
		-0.356614 -0.342059
		-0.435263 -0.417406
		-0.268326 -0.271036
		-0.285709 -0.297311
		-0.330558 -0.352371
		-0.335563 -0.355797
		-0.339404 -0.372305
		-0.318664 -0.359519
		-0.304197 -0.359362
		-0.401077 -0.503008
		-0.373213 -0.495472
		-0.323317 -0.457375
		-0.367815 -0.534798
		-0.311162 -0.462805
		-0.259467 -0.473378
		-0.272684 -0.49541
		-0.257095 -0.551586
		-0.223216 -0.521574
		-0.242335 -0.510636
		-0.183268 -0.482606
		-0.155448 -0.516001
		-0.161932 -0.504971
		-0.159442 -0.506337
		-0.122697 -0.463083
		-0.116558 -0.426165
		-0.10413 -0.436974
		-0.0937638999999999 -0.423741
		-0.0889491 -0.424778
		-0.0920426000000001 -0.424118
		-0.112805 -0.521161
		-0.0618905999999999 -0.429483
		-0.0439408000000001 -0.377566
		-0.0433751 -0.392044
		-0.01179 -0.400863
		0.0110258999999999 -0.437361
		0.0182601 -0.400063
		0.024878 -0.399706
		0.0278347999999999 -0.399511
		0.0409853 -0.398377
		0.0435133000000001 -0.411703
		0.0664064 -0.464845
		0.0707469000000001 -0.454269
		0.0939395999999999 -0.464062
		0.101793 -0.424426
		0.104201 -0.4327
		0.145244 -0.511607
		0.145355 -0.421883
		0.151776 -0.419616
		0.148043 -0.384247
		0.167507 -0.454661
		0.145517 -0.363793
		0.152434 -0.415565
		0.183426 -0.430568
		0.17742 -0.386149
		0.207905 -0.419625
		0.228233 -0.446368
		0.20644 -0.371593
		0.21743 -0.376189
		0.244769 -0.365454
		0.198615 -0.284292
		0.270132 -0.347548
		0.298047 -0.359359
		0.296688 -0.333573
		0.286635 -0.308797
		0.32784 -0.347709
		0.283729 -0.296308
		0.254051 -0.265483
		0.257273 -0.257273
		0.273036 -0.274408
		0.273922 -0.261657
		0.270579 -0.265113
		0.333809 -0.303043
		0.341864 -0.30563
		0.342604 -0.301364
		0.30707 -0.264665
		0.33026 -0.278114
		0.268524 -0.239114
		0.274635 -0.243248
		0.280881 -0.247283
		0.248169 -0.22539
		0.297758 -0.26389
		0.254039 -0.220167
		0.266127 -0.23684
		0.350139 -0.303346
		0.419102 -0.328745
		0.42838 -0.342312
		0.439276 -0.369391
		0.399963 -0.321071
		0.421445 -0.312321
		0.452151 -0.320107
		0.450362 -0.308877
		0.456202 -0.300185
		0.465771 -0.302449
		0.468471 -0.308948
		0.474149 -0.29381
		0.477222 -0.288791
		0.451883 -0.239345
		0.451975 -0.23917
		0.45193 -0.239257
		0.451975 -0.23917
		0.449839 -0.247411
		0.450272 -0.246622
		0.449484 -0.248056
		0.446205 -0.253907
		0.448228 -0.25718
		0.391123 -0.220795
		0.33897 -0.201476
		0.341231 -0.209884
		0.414618 -0.239015
		0.413156 -0.238606
		0.597685 -0.320765
		0.531917 -0.283281
		0.536983 -0.283804
		0.556015 -0.299068
		0.671069 -0.34693
		0.661016 -0.3466
		0.5243 -0.275947
		0.558455 -0.289725
		0.484942 -0.262525
		0.560623 -0.276064
		0.453982 -0.222676
		0.489992 -0.236548
		0.522324 -0.251039
		0.424098 -0.205474
		0.443066 -0.210239
		0.445123 -0.205848
		0.420169 -0.18174
		0.423444 -0.184403
		0.471585 -0.198767
		0.529565 -0.226956
		0.50986 -0.217282
		0.50392 -0.211949
		0.50984 -0.197286
		0.518972 -0.19375
		0.543178 -0.191567
		0.5202 -0.19043
		0.493735 -0.182947
		0.527052 -0.177239
		0.532349 -0.15947
		0.484759 -0.13695
		0.506588 -0.137955
		0.453969 -0.100882
		0.437733 -0.0617068999999999
		0.416724 -0.0359244999999999
		0.382217 -0.0181224
		0.366934 0.00157483999999997
		0.365751 0.0158334
		0.35832 0.0167014000000001
		0.470861 0.0442689000000001
		0.433367 0.0627
		0.47375 0.0627618000000001
		0.432872 0.0660314
		0.431627 0.0737361999999999
		0.369237 0.0562213
		0.338165 0.0528818
		0.352383 0.0519909000000001
		0.387989 0.0545367000000001
		0.388872 0.0478375
		0.389275 0.0444446999999999
		0.374801 0.0422927
		0.379876 0.037412
		0.40791 0.0443047999999999
		0.41014 0.0416307
		0.403591 0.0377894999999999
		0.479597 0.0484986000000001
		0.473257 0.0457422999999999
		0.488366 0.0452191
		0.492399 0.0545091
		0.487461 0.0629563
		0.539558 0.0742143
		0.539245 0.0764601
		0.481621 0.0721529000000001
		0.481621 0.0721529000000001
		0.412056 0.065307
		0.361431 0.0577190000000001
		0.361631 0.0600391
		0.387354 0.0588778999999999
		0.365829 0.0752735
		0.378085 0.0886865999999999
		0.488875 0.142589
		0.365274 0.122781
		0.365274 0.122781
		0.419555 0.154014
		0.332385 0.148662
		0.328609 0.160809
		0.32499 0.168003
		0.32499 0.168003
		0.300879 0.172298
		0.263788 0.167448
		0.263788 0.167448
		0.291566 0.199087
		0.284741 0.213237
		0.284741 0.213237
		0.310193 0.244224
		0.323778 0.259023
		0.313534 0.249402
		0.270044 0.235518
		0.270044 0.235518
		0.297822 0.254502
		0.273496 0.227914
		0.250313 0.195064
		0.289437 0.23358
		0.313979 0.250915
		0.313979 0.250915
		0.404545 0.326026
		0.367389 0.282844
		0.367389 0.282844
		0.472756 0.370751
		0.490191 0.388068
		0.490191 0.388068
		0.391749 0.309449
		0.394775 0.305579
		0.370399 0.285647
		0.365258 0.273555
		0.334171 0.246684
		0.293624 0.220218
		0.303077 0.214789
		0.283038 0.183791
		0.301873 0.188181
		0.261397 0.173886
		0.234597 0.165959
		0.253264 0.179807
		0.241347 0.15598
		0.225474 0.149985
		0.254476 0.181286
		0.257137 0.177493
		0.257302 0.177253
		0.290306 0.186717
		0.293182 0.204298
		0.290763 0.200066
		0.273092 0.185402
		0.248579 0.187015
		0.257464 0.206933
		0.402981 0.332316
		0.225178 0.204509
		0.152317 0.140252
		0.167412 0.159841
		0.141652 0.139495
		0.143414 0.149359
		0.152169 0.157746
		0.127467 0.128127
		0.123154 0.126412
		0.192787 0.191783
		0.182702 0.179817
		0.178348 0.178348
		0.196759 0.191498
		0.161044 0.14519
		0.165477 0.142447
		0.184908 0.15409
		0.195727 0.165535
		0.206163 0.170543
		0.191714 0.157764
		0.216113 0.174466
		0.197183 0.158581
		0.187521 0.146713
		0.210636 0.165338
		0.203847 0.149919
		0.17519 0.109494
		0.142249 0.0866171
		0.140827 0.0806747000000001
		0.147564 0.0781649
		0.129557 0.0522003
		0.192612 0.0589055000000001
		0.237806 0.0577528
		0.206388 0.0503625999999999
		0.343388 0.0499765999999999
		0.39511 0.0309533
		0.407076 0.0242751999999999
		0.380962 0.0157278000000001
		0.380807 0.0191273000000001
		0.434701 0.0177027000000001
		0.451085 0.0222509
		0.456286 0.0245534999999999
		0.35071 -0.0094361300000001
		0.386393 0.00686922000000001
		0.386322 0.010122
		0.415566 -0.00722719000000005
		0.366906 -0.00478573000000004
		0.385906 -0.0205816000000001
		0.401007 -0.035331
		0.390043 -0.0381376
		0.393572 -0.0511819
		0.393342 -0.052916
		0.424022 -0.0798605999999999
		0.385599 -0.0902088999999999
		0.421396 -0.110181
		0.331238 -0.103121
		0.376959 -0.126811
		0.303942 -0.109998
		0.259331 -0.0963229000000001
		0.222978 -0.116481
		0.214494 -0.192659
		0.210803 -0.167711
		0.201112 -0.164242
		0.183663 -0.15238
		0.210008 -0.218972
		0.183594 -0.192495
		0.223145 -0.267479
		0.208031 -0.252411
		0.232134 -0.241749
		0.251867 -0.303865
		0.251867 -0.303865
		0.255254 -0.311608
		0.264613 -0.354034
		0.226064 -0.3184
		0.268402 -0.379598
		0.242393 -0.364501
		0.19871 -0.336151
		0.22503 -0.412223
		0.215937 -0.418007
		0.198163 -0.413985
		0.154594 -0.397798
		0.149332 -0.406409
		0.143542 -0.401918
		0.100232 -0.422546
		0.0566762000000001 -0.380793
		0.0133657 -0.355861
		-0.0171916999999999 -0.328205
		-0.0485082000000001 -0.349594
		-0.0768416000000001 -0.318573
		-0.0838311 -0.284737
		-0.0865507000000001 -0.275008
		-0.0982505 -0.271969
		-0.176117 -0.342866
		-0.226198 -0.404894
		-0.228674 -0.400179
		-0.282459 -0.420067
		-0.252712 -0.378007
		-0.269701 -0.374237
		-0.243938 -0.322148
		-0.235874 -0.283733
		-0.268361 -0.291039
		-0.302639 -0.290771
		-0.307474 -0.285654
		-0.373422 -0.310435
		-0.26652 -0.201691
		-0.294657 -0.192838
		-0.320543 -0.194269
		-0.274856 -0.173159
		-0.360364 -0.215143
		-0.349405 -0.189821
		-0.420869 -0.21735
		-0.369764 -0.181426
		-0.374789 -0.176984
		-0.36707 -0.166541
		-0.434616 -0.165661
		-0.439066 -0.153479
		-0.444678 -0.136368
		-0.443565 -0.128966
		-0.453061 -0.110835
		-0.467907 -0.0995547999999999
		-0.422298 -0.0603283000000001
		-0.388546 -0.0404735999999999
		-0.504018 -0.0296481
		-0.521239 -0.00657024000000006
		-0.544371 0.0228727
		-0.48802 0.0364496000000001
		-0.430967 0.0393414000000001
		-0.428758 0.0587096
		-0.487304 0.0550511
		-0.625455 0.0825068
		-0.584632 0.0845849999999999
		-0.584393 0.106932
		-0.569776 0.126078
		-0.508279 0.125984
		-0.604873 0.179897
		-0.552503 0.20091
		-0.403459 0.174658
		-0.501345 0.235414
		-0.518339 0.269267
		-0.457537 0.250843
		-0.439286 0.249905
		-0.443711 0.263085
		-0.354262 0.224157
		-0.350739 0.229632
		-0.429546 0.279301
		-0.429697 0.290961
		-0.41591 0.299229
		-0.355785 0.265221
		-0.374482 0.283438
		-0.327743 0.263719
		-0.289352 0.266986
		-0.371328 0.342346
		-0.362593 0.355341
		-0.341474 0.355556
		-0.360808 0.399605
		-0.41363 0.486074
		-0.429976 0.590216
		-0.39768 0.577523
		-0.378905 0.605733
		-0.372116 0.640572
		-0.349725 0.628492
		-0.350613 0.632127
		-0.326372 0.604033
		-0.312928 0.599579
		-0.313635 0.647668
		-0.288428 0.583833
		-0.23444 0.54069
		-0.209796 0.511504
		-0.205775 0.507444
		-0.1536 0.468029
		-0.109234 0.472751
		-0.109234 0.472751
		-0.0706287999999999 0.612875
		-0.0334669999999999 0.500146
		-0.0334669999999999 0.500146
		-0.0167615999999999 0.320866
		0.0230748000000001 0.31151
		0.0230748000000001 0.31151
		0.0507164 0.259434
		0.0956961000000001 0.499534
		0.0956961000000001 0.499534
		0.0844883999999999 0.317138
		0.112211 0.438642
		0.105666 0.349933
		0.205858 0.473862
		0.205858 0.473862
		0.19739 0.418604
		0.241411 0.467372
		0.241411 0.467372
		0.389009 0.646522
		0.388266 0.639818
		0.388266 0.639818
		0.493508 0.704548
		0.571262 0.762911
		0.571262 0.762911
		0.559112 0.695481
		0.560552 0.673998
		0.560552 0.673998
		0.630707 0.689619
		0.541607 0.564292
		0.541607 0.564292
		0.462254 0.444127
		0.404357 0.373402
		0.404357 0.373402
		0.461255 0.405548
		0.541222 0.465398
		0.541222 0.465398
		0.531748 0.410782
		0.430495 0.315831
		0.430495 0.315831
		0.49031 0.298747
		0.511078 0.312325
		0.544356 0.295791
		0.53805 0.277546
		0.53805 0.277546
		0.483923 0.175214
		0.483923 0.175214
		0.537296 0.187591
		0.522923 0.140352
		0.522923 0.140352
		0.450501 0.107262
		0.445402 0.0694132999999999
		0.445402 0.0694132999999999
		0.444326 0.0365462999999999
		0.428797 0.0166343
		0.457741 -0.0463534999999999
		0.410282 -0.0566499
		0.528145 -0.139218
		0.594317 -0.201464
		0.642314 -0.246405
		0.633291 -0.271811
		0.609566 -0.288742
		0.578212 -0.309574
		0.468382 -0.290571
		0.494263 -0.301155
		0.381102 -0.265885
		0.404779 -0.310331
		0.328002 -0.281374
		0.300572 -0.276765
		0.279362 -0.297006
		0.266359 -0.298556
		0.438353 -0.542844
		0.415537 -0.548102
		0.424618 -0.607787
		0.385656 -0.559329
		0.384629 -0.666495
		0.375718 -0.671559
		0.350284 -0.642188
		0.341051 -0.679163
		0.329758 -0.719471
		0.282138 -0.68397
		0.241026 -0.635673
		0.244943 -0.734829
		0.224043 -0.800154
		0.173071 -0.736286
		0.164108 -0.741416
		0.107959 -0.55059
		0.0840718 -0.568591
		0.0691792 -0.782026
		0.0290642000000001 -0.829945
		-0.00606544999999992 -0.773339
		-0.0388858999999999 -0.759769
		-0.0804153999999999 -0.756501
		-0.116352 -0.751813
		-0.134075 -0.785742
		-0.150141 -0.78824
		-0.157137 -0.770278
		-0.16827 -0.767922
		-0.186281 -0.763753
		-0.197325 -0.718615
		-0.223428 -0.720928
		-0.236499 -0.721471
		-0.246317 -0.718178
		-0.267421 -0.716095
		-0.287567 -0.705577
		-0.303512 -0.712202
		-0.311565 -0.704803
		-0.328915 -0.66355
		-0.336489 -0.64774
		-0.284938 -0.516029
		-0.383614 -0.678016
		-0.370495 -0.584043
		-0.290394 -0.450611
		-0.318151 -0.441435
		-0.322715 -0.43811
		-0.323611 -0.41204
		-0.340279 -0.398238
		-0.450532 -0.489288
		-0.479104 -0.494395
		-0.571861 -0.542535
		-0.57817 -0.53459
		-0.710874 -0.611351
		-0.656491 -0.532992
		-0.718401 -0.560703
		-0.692845 -0.48926
		-0.750335 -0.515417
		-0.796004 -0.554682
		-0.780995 -0.511569
		-0.740687 -0.45247
		-0.718091 -0.422581
		-0.626849 -0.341454
		-0.662262 -0.336387
		-0.748728 -0.340598
		-0.761031 -0.312142
		-0.729854 -0.269791
		-0.800525 -0.273047
		-0.741152 -0.252796
		-0.734634 -0.241096
		-0.80894 -0.247004
		-0.815354 -0.224925
		-0.792439 -0.192837
		-0.787172 -0.181884
		-0.791127 -0.172501
		-0.792942 -0.163954
		-0.831513 -0.166303
		-0.803299 -0.150996
		-0.830657 -0.14677
		-0.830117 -0.149796
		-0.811691 -0.128645
		-0.837032 -0.13582
		-0.795778 -0.149583
		-0.795778 -0.149583
		-0.794673 -0.15535
		-0.805047 -0.175536
		-0.805816 -0.182449
		-0.785322 -0.183045
		-0.782811 -0.198668
		-0.781248 -0.199718
		-0.77958 -0.226138
		-0.781594 -0.248553
		-0.783132 -0.266083
		-0.777479 -0.282174
		-0.757147 -0.299947
		-0.788166 -0.31344
		-0.775347 -0.343928
		-0.768876 -0.366418
		-0.809629 -0.396814
		-0.829857 -0.476584
		-0.824684 -0.508555
		-0.817214 -0.537734
		-0.755191 -0.522067
		-0.687994 -0.729124
		-0.687994 -0.729124
		-0.670154 -0.741287
		-0.645803 -0.746593
		-0.580209 -0.84394
		-0.431 -0.734871
		-0.3974 -0.716525
		-0.3974 -0.716525
		-0.339069 -0.769184
		-0.339069 -0.769184
		-0.230127 -0.786785
		-0.156646 -0.783231
		-0.0854454 -0.670212
		-0.0631101000000001 -0.660027
		-0.0399662999999999 -0.666105
		-0.00257984000000011 -0.663032
		0.0208581000000001 -0.765792
		0.0828591999999999 -0.760529
		0.109559 -0.724776
		0.156021 -0.713239
		0.170607 -0.716551
		0.22321 -0.734244
		0.263554 -0.765857
		0.285106 -0.759249
		0.335559 -0.69761
		0.335559 -0.69761
		0.367196 -0.674149
		0.410153 -0.629471
		0.42431 -0.611006
		0.441233 -0.563046
		0.441233 -0.563046
		0.476933 -0.556881
		0.443478 -0.498599
		0.328948 -0.334115
		0.479076 -0.450187
		0.338269 -0.306294
		0.394545 -0.32162
		0.476535 -0.33945
		0.411055 -0.29708
		0.471896 -0.299745
		0.583904 -0.322491
		0.604864 -0.26744
		0.657504 -0.196712
		0.705955 -0.157835
		0.721321 -0.145428
		0.654144 -0.118446
		0.629909 -0.0518444
		0.669937 0.00274565999999998
		0.578788 0.199414
		0.603645 0.253894
		0.60403 0.306042
		0.591855 0.334411
		0.664538 0.384891
		0.564068 0.360591
		0.605557 0.413007
		0.557883 0.411342
		0.541476 0.441865
		0.508898 0.452353
		0.491262 0.476884
		0.469304 0.490422
		0.436515 0.471789
		0.492186 0.559538
		0.511801 0.645567
		0.542226 0.767052
		0.550206 0.811379
		0.316001 0.876333
		-0.115895 0.858808
		-0.115895 0.858808
		-0.15484 0.865281
		-0.216861 0.852172
		-0.330836 0.931116
		-0.422995 0.984557
		-0.481239 1.00007
		-0.481239 1.00007
		-0.534289 0.929663
		-0.569491 0.945502
		-0.569491 0.945502
		-0.607155 0.920044
		-0.600819 0.87812
		-0.600819 0.87812
		-0.626357 0.870345
		-0.657303 0.877628
		-0.752293 0.916858
		-0.718475 0.860673
		-0.718475 0.860673
		-0.738304 0.807407
		-0.744758 0.798988
		-0.744758 0.798988
		-0.924433 0.810406
		-0.924433 0.810406
		-1.07017 0.904111
		-1.09954 0.913967
		-1.14362 0.898898
		-1.1394 0.878963
		-1.18701 0.844516
		-1.23204 0.837213
		-1.23204 0.837213
		-1.22092 0.821868
		-1.23639 0.817848
		-1.2652 0.763893
		-1.27638 0.736187
		-1.23076 0.689225
		-1.33077 0.691809
		-1.30574 0.652869
		-1.37097 0.623617
		-1.34773 0.524651
		-1.34664 0.515734
		-1.33126 0.489226
		-1.37117 0.481368
		-1.37669 0.465358
		-1.36894 0.456312
		-1.39284 0.430427
		-1.39757 0.424091
		-1.61149 0.454945
		-1.61885 0.428034
		-1.64857 0.412142
		-1.64792 0.384516
		-1.70663 0.376715
		-1.72623 0.344099
		-1.77425 0.292781
		-1.82634 0.17964
		-1.77459 0.144983
		-1.80685 0.136703
		-1.79418 0.11068
		-1.77892 0.0750843999999999
		-1.78053 -0.0344618000000001
		-1.77994 -0.0574174000000001
		-1.77571 -0.0747064
		-1.76734 -0.0686347
		-1.81321 -0.0987967999999999
		-1.80168 -0.134979
		-1.72314 -0.156142
		-1.71296 -0.178549
		-1.71059 -0.207515
		-1.7146 -0.229734
		-1.72506 -0.270597
		-1.72209 -0.288903
		-1.71624 -0.321796
		-1.69718 -0.33497
		-1.69182 -0.357348
		-1.68303 -0.38022
		-1.68584 -0.443938
		-1.67763 -0.472181
		-1.66262 -0.475034
		-1.63756 -0.48581
		-1.59322 -0.50767
		-1.58471 -0.533628
		-1.55262 -0.566495
		-1.54072 -0.649826
		-1.53012 -0.671377
		-1.52228 -0.688652
		-1.60316 -0.771278
		-1.58505 -0.776127
		-1.5223 -0.753193
		-1.64445 -0.842277
		-1.64048 -0.898496
		-1.62808 -0.936147
		-1.58277 -0.946223
		-1.55179 -0.957123
		-1.458 -0.928802
		-1.42872 -0.932931
		-1.60657 -1.07105
		-1.64381 -1.12896
		-1.66138 -1.16865
		-1.50977 -1.09749
		-1.50641 -1.12254
		-1.48573 -1.13886
		-1.4678 -1.15122
		-1.52723 -1.21692
		-1.34249 -1.09547
		-1.45292 -1.26603
		-1.43348 -1.27154
		-1.41302 -1.27531
		-1.50762 -1.39763
		-1.38529 -1.28934
		-1.50144 -1.44829
		-1.51791 -1.56643
		-1.635 -1.71069
		-1.54852 -1.67756
		-1.35864 -1.51172
		-1.33964 -1.50316
		-1.33775 -1.53523
		-1.25068 -1.46611
		-1.22166 -1.49579
		-1.18723 -1.53326
		-1.23481 -1.66987
		-1.22908 -1.7286
		-1.2546 -1.76322
		-1.22332 -1.79421
		-1.2769 -1.93712
		-1.25881 -1.97604
		-1.26325 -2.09274
		-1.20751 -2.03952
		-1.19088 -2.11627
		-1.15319 -2.13189
		-1.133 -2.13004
		-1.04085 -2.02506
		-1.02857 -2.09336
		-0.864253 -1.81555
		-0.838656 -1.82752
		-0.915439 -2.03049
		-0.843635 -1.9575
		-0.802294 -1.89749
		-0.778789 -1.89949
		-0.687205 -1.80466
		-0.613333 -1.79872
		-0.634382 -1.81856
		-0.587905 -1.83644
		-0.587905 -1.83644
		-0.548185 -1.81139
		-0.490944 -1.8668
		-0.473212 -1.84493
		-0.45669 -1.87548
		-0.445165 -1.946
		-0.427138 -1.95718
		-0.401667 -2.00833
		-0.342544 -1.90846
		-0.333244 -1.93158
		-0.298241 -1.93235
		-0.254637 -1.90371
		-0.239343 -1.93316
		-0.211418 -1.89672
		-0.165169 -1.92697
		-0.158565 -1.99791
		-0.102645 -2.02723
		-0.0300222999999999 -1.90942
		0.0312621 -1.98201
		0.0627420999999999 -1.98892
		0.108405 -2.13422
		0.169423 -2.12118
		0.187481 -2.08908
		0.267411 -2.10586
		0.300696 -1.88837
		0.369835 -1.98308
		0.377347 -2.0721
		0.527072 -1.92413
		0.591874 -2.02448
		0.687958 -2.17974
		0.689413 -2.03411
		0.702769 -2.00695
		0.960461 -2.18812
		0.864879 -1.84713
		0.757279 -1.55189
		0.883582 -1.62373
		0.908384 -1.56041
		1.21863 -1.84478
		1.51055 -2.12743
		1.93626 -0.67869
		1.95003 -0.658883
		1.86056 -0.626514
		1.86124 -0.584783
		1.83776 -0.540881
		1.90157 -0.546941
		1.98745 -0.526476
		1.83374 -0.464467
		2.03211 -0.479712
		2.00977 -0.451707
		2.06434 -0.411519
		2.06513 -0.362067
		1.87787 -0.302882
		1.91706 -0.257241
		2.0073 -0.250912
		1.91998 -0.191998
		1.91932 -0.173358
		1.94803 -0.12568
		1.93905 -0.0685838999999999
		1.94968 -0.0376143
		1.9862 0.0191595
		2.07119 0.0331923000000001
		1.95455 0.0754166000000001
		2.09462 0.128795
		2.10918 0.170645
		1.93321 0.199557
		2.0355 0.256908
		1.88096 0.242705
		2.00305 0.311153
		2.06397 0.349598
		2.06102 0.382665
		2.07301 0.411901
		2.11534 0.464681
		2.1282 0.518048
		2.09839 0.55074
		1.91683 0.619583
		1.91683 0.619583
		1.84633 0.729798
		1.8577 0.739289
		1.75987 0.85566
		1.67308 0.822265
		1.65078 0.911971
		1.7937 1.14085
		1.74582 1.2234
		1.71895 1.27428
		1.65824 1.26465
		1.52439 1.31624
		1.44431 1.36705
		1.33992 1.3342
		0.50805 1.71403
		0.438991 1.79344
		0.440602 1.88511
		0.371321 1.81417
		0.423526 1.91731
		0.359703 1.85847
		0.350357 1.84881
		0.317125 1.7493
		0.0105715 1.8236
		-0.0784526000000001 1.92769
		-0.0870736000000001 1.76196
		-0.109063 1.69543
		-0.0660574 1.73781
		-0.144094 1.8412
		-0.145369 1.91775
		-0.137418 1.96393
		-0.180407 1.77314
		-0.169186 1.87196
		-0.157609 1.86957
		-0.159991 1.83989
		-0.175622 1.66841
		-0.18203 1.73434
		-0.338167 1.84355
		-0.55064 2.09496
		-0.640362 2.43487
		-0.625485 2.35648
		-0.707689 2.38845
		-0.693001 2.277
		-0.819185 2.47316
		-0.861563 2.49774
		-0.865241 2.35704
		-0.872424 2.31669
		-0.95834 2.39202
		-1.04328 2.49584
		-0.933372 2.29301
		-1.15899 2.38895
		-1.19091 2.38182
		-1.24918 2.41725
		-1.25237 2.39307
		-1.25396 2.373
		-1.27401 2.38777
		-1.34996 2.41182
		-1.37068 2.38023
		-1.36628 2.32834
		-1.42557 2.28569
		-1.51035 2.20324
		-1.34938 1.98601
		-1.38706 2.01301
		-1.31886 1.87938
		-1.457 1.98295
		-1.28791 1.72128
		-1.47933 1.92382
		-1.5117 1.91761
		-1.4808 1.79715
		-1.44479 1.6593
		-1.85625 1.95104
		-1.86843 1.93938
		-1.91938 1.95164
		-1.95164 1.91938
		-1.97219 1.91561
		-2.07531 1.98288
		-2.04328 1.90489
		-2.10453 1.90568
		-2.14217 1.92203
		-2.152 1.87675
		-2.17091 1.85484
		-2.17853 1.83631
		-2.13228 1.76215
		-2.1965 1.74907
		-2.19024 1.69464
		-2.0914 1.61228
		-2.17836 1.66768
		-2.20064 1.65048
		-2.17748 1.5822
		-2.19026 1.56447
		-2.19765 1.55406
		-2.36896 1.59611
		-2.38566 1.57104
		-2.58966 1.61294
		-2.60014 1.57801
		-2.68597 1.59306
		-2.7137 1.58377
		-2.55407 1.42372
		-2.4186 1.33829
		-2.43564 1.3146
		-2.456 1.27616
		-2.50069 1.22183
		-2.50482 1.19548
		-2.51791 1.11727
		-2.52092 1.09535
		-2.65677 0.997338
		-2.67513 0.933771
		-2.67176 0.893369
		-2.6666 0.877825
		-2.68725 0.840795
		-2.66576 0.809542
		-2.67028 0.79453
		-2.67691 0.771871
		-2.7056 0.686742
		-2.69007 0.672517
		-2.73984 0.649568
		-2.70783 0.582594
		-2.6918 0.505733
		-2.69591 0.473827
		-2.75746 0.456808
		-2.74699 0.439851
		-2.76137 0.432504
		-2.80715 0.386613
		-2.86112 0.367248
		-2.92947 0.341043
		-2.93154 0.322818
		-2.93514 0.288272
		-2.90687 0.24152
		-3.16057 0.244568
		-2.82206 0.184777
		-2.91647 0.165411
		-2.92057 0.129996
		-3.17548 0.084554
		-2.81596 0.0419042000000001
		-2.88669 -0.00854035000000009
		-2.8865 -0.0341596
		-2.88518 -0.0938964
		-2.83396 -0.117383
		-2.92532 -0.155327
		-2.8092 -0.199469
		-2.80602 -0.240043
		-2.89035 -0.264309
		-2.91566 -0.283825
		-2.89519 -0.325495
		-2.8822 -0.332562
		-2.81904 -0.383657
		-2.83424 -0.39528
		-3.43164 -0.48878
		-3.19879 -0.504571
		-3.40122 -0.588868
		-3.10242 -0.613052
		-2.88326 -0.597433
		-2.83635 -0.623655
		-2.72777 -0.653012
		-2.77061 -0.698967
		-2.83161 -0.740177
		-2.84869 -0.779276
		-2.69754 -0.768391
		-2.72451 -0.797418
		-2.67478 -0.834335
		-2.65566 -0.89334
		-2.71161 -0.951151
		-2.6984 -0.988028
		-2.66447 -1.01974
		-2.6628 -1.04375
		-2.64475 -1.06776
		-2.91965 -1.20435
		-2.70849 -1.13774
		-2.94104 -1.26705
		-3.15378 -1.42268
		-3.05686 -1.42588
		-3.02339 -1.45823
		-3.02227 -1.48668
		-3.03191 -1.53077
		-2.99609 -1.57172
		-2.99037 -1.62222
		-2.90255 -1.68348
		-2.92916 -1.70868
		-2.87094 -1.80042
		-2.80418 -1.80884
		-2.77873 -1.84294
		-2.77263 -1.85162
		-2.77841 -1.9874
		-2.71501 -1.98254
		-2.73639 -2.04488
		-2.79659 -2.12541
		-2.75114 -2.11626
		-2.6751 -2.11036
		-2.82123 -2.25911
		-2.72376 -2.26807
		-2.82746 -2.37246
		-2.60402 -2.21191
		-2.71104 -2.35238
		-2.57956 -2.29851
		-2.4335 -2.2331
		-2.44179 -2.28737
		-2.37057 -2.27612
		-2.29628 -2.25895
		-2.21691 -2.2813
		-2.18445 -2.28499
		-2.16601 -2.34264
		-2.25263 -2.46716
		-2.10069 -2.36789
		-2.08878 -2.38454
		-1.98058 -2.38942
		-2.03356 -2.48546
		-2.11763 -2.6101
		-2.08934 -2.63865
		-1.956 -2.54279
		-1.93777 -2.56196
		-1.98723 -2.71164
		-1.95283 -2.74373
		-1.89215 -2.7797
		-1.82389 -2.75995
		-1.79839 -2.79428
		-1.79062 -2.8376
		-1.73701 -2.79265
		-1.63698 -2.67037
		-1.49318 -2.7375
		-1.49608 -2.76915
		-1.45179 -2.79262
		-1.43769 -2.80118
		-1.43769 -2.80118
		-1.45544 -2.95972
		-1.22346 -2.63515
		-1.19992 -2.88531
		-1.17219 -2.84932
		-1.18432 -3.04264
		-1.16754 -3.04911
		-1.03812 -2.96607
		-0.989329 -2.96799
		-0.955116 -2.96637
		-0.830433 -3.00801
		-0.780137 -2.96633
		-0.726278 -2.97774
		-0.698106 -2.95353
		-0.698106 -2.95353
		-0.613389 -3.0038
		-0.587903 -3.11682
		-0.587903 -3.11682
		-0.516492 -3.26462
		-0.516492 -3.26462
		-0.304496 -3.20673
		-0.304496 -3.20673
		-0.276924 -3.46669
		-0.222813 -3.27439
		-0.144292 -3.03915
		-0.10414 -3.19048
		-0.10414 -3.19048
		-0.0673554999999999 -3.2427
		-0.0673554999999999 -3.2427
		-0.0661719000000001 -3.72769
		0.0706751000000001 -3.45298
		0.0706751000000001 -3.45298
		0.128897 -3.36124
		0.259621 -3.25007
		2.4514 -2.68387
		2.42499 -2.54523
		2.47163 -2.55234
		2.43869 -2.44844
		2.49203 -2.49203
		2.47987 -2.37373
		2.49352 -2.4248
		2.50341 -2.39584
		2.74051 -1.72341
		2.87819 -1.38229
		2.96075 -0.810017
		2.86569 -0.745618
		2.92318 -0.767335
		2.86846 -0.659212
		2.80722 -0.604633
		2.70108 -0.555131
		2.87225 -0.544585
		2.89654 -0.501832
		2.73909 -0.425896
		2.89114 -0.433229
		2.9135 -0.399718
		2.9314 -0.365311
		2.92047 -0.345146
		2.92329 -0.310046
		2.92975 -0.240436
		3.05036 -0.175627
		2.97086 -0.135039
		2.93582 -0.0800676
		2.92409 0.00886095000000009
		3.04129 0.0643174
		3.0485 0.119729
		3.04681 0.156957
		2.92154 0.195361
		2.89989 0.202113
		2.91431 0.283459
		2.91345 0.29223
		2.87427 0.341757
		2.88066 0.40523
		2.8769 0.431095
		2.83178 0.495127
		2.89534 0.531256
		2.99249 0.594838
		2.86041 0.605424
		2.82017 0.648811
		2.84153 0.688593
		2.85475 0.713686
		2.83973 0.771283
		2.83529 0.796332
		2.83732 0.819475
		2.94756 0.918244
		2.95349 0.978285
		2.94789 0.995029
		2.86694 1.0252
		2.8522 1.07185
		2.85524 1.09118
		2.66167 1.1076
		2.60033 1.20339
		2.59727 1.18516
		2.62299 1.2093
		2.63941 1.19116
		2.75779 1.26733
		2.7695 1.31281
		2.50682 1.24116
		2.59363 1.36462
		2.79706 1.50469
		2.66163 1.45735
		2.74136 1.54711
		2.8006 1.62286
		2.74923 1.64769
		2.66309 1.63602
		2.66191 1.67737
		2.67264 1.68073
		2.65606 1.70681
		2.64383 1.73816
		2.56382 1.72395
		2.67664 1.82456
		2.59389 1.78048
		2.66918 1.85723
		2.57844 1.82753
		2.48912 1.80788
		2.46023 1.81919
		2.53854 1.91064
		2.5427 1.97263
		2.51307 1.97262
		2.69568 2.19575
		2.53231 2.08706
		2.54204 2.12148
		2.34921 2.02886
		2.48008 2.17124
		2.60664 3.27894
		1.30057 2.59315
		1.48741 3.3314
		1.47099 3.39458
		1.47713 3.45356
		1.16737 2.92274
		1.39452 3.39535
		1.14705 3.13589
		1.01237 3.0371
		1.01237 3.0371
		-3.62375 3.89589
		-4.02918 2.82042
		-4.08732 2.79233
		-4.10532 2.75932
		-4.12602 2.72828
		-4.13838 2.70949
		-4.12705 2.65311
		-4.17384 2.61202
		-4.28002 2.4729
		-4.2105 2.39082
		-4.25043 2.40008
		-4.27624 2.36672
		-4.24922 2.33108
		-4.11527 2.211
		-4.12059 2.20106
		-3.58751 1.85484
		-3.63002 1.81501
		-3.63404 1.80587
		-3.64775 1.77912
		-3.60975 1.72784
		-3.61562 1.7144
		-3.63254 1.67826
		-3.6626 1.66482
		-4.22417 1.86887
		-3.6589 1.58073
		-3.66436 1.54231
		-3.57916 1.48066
		-3.61988 1.45652
		-3.66822 1.44341
		-3.66511 1.41215
		-3.69907 1.39259
		-4.07357 1.51714
		-3.7003 1.33081
		-3.80238 1.31919
		-3.70098 1.248
		-3.79688 1.23619
		-3.80333 1.21618
		-3.94697 1.22413
		-3.9534 1.20321
		-4.00713 1.16971
		-4.00947 1.14391
		-4.01552 1.12249
		-4.06004 1.09353
		-3.96706 1.04277
		-3.96756 1.00889
		-3.97292 0.987556
		-3.99102 0.957845
		-3.99614 0.93624
		-4.39162 0.975916
		-4.30197 0.901829
		-4.32606 0.747562
		-4.16612 0.65719
		-4.42383 0.685383
		-4.19342 0.626059
		-4.18271 0.57571
		-4.14053 0.558274
		-4.14053 0.500121
		-4.16829 0.477374
		-4.16467 0.440829
		-4.21211 0.410652
		-4.21432 0.387388
		-4.32897 0.363779
		-3.95927 0.287545
		-4.06498 0.249108
		-4.16151 0.197063
		-4.0626 0.181568
		-4.08337 0.147455
		-4.08828 0.0908507999999999
		-4.03725 0.0785020000000001
		-4.04188 0
		-4.18401 -0.0699278000000001
		-4.17799 -0.151292
		-4.03451 -0.168104
		-4.22009 -0.270368
		-4.22551 -0.341336
		-4.25031 -0.415533
		-4.16229 -0.443045
		-4.4676 -0.538114
		-3.33817 -2.51827
		-3.40352 -2.6218
		-3.35816 -2.72251
		-3.19608 -2.64225
		-3.07252 -2.58447
		-2.64825 -3.50613
		-2.49472 -3.39757
		-2.4698 -3.39155
		-2.43833 -3.42076
		-2.41427 -3.51276
		-2.36986 -3.46
		-2.39777 -3.5784
		-2.291 -3.52553
		-2.06965 -3.29611
		-2.22195 -3.48496
		-2.03683 -3.29616
		-2.1927 -3.52942
		-2.16291 -3.53081
		-2.14117 -3.49532
		-1.9943 -3.3948
		-2.05665 -3.55239
		-1.92503 -3.3827
		-1.9155 -3.38811
		-1.88269 -3.39992
		-1.92433 -3.37311
		-1.65837 -3.01253
		-1.73078 -3.17309
		-1.72429 -3.18013
		-1.94007 -3.61134
		-1.69749 -3.23877
		-1.91219 -3.62617
		-1.69552 -3.25582
		-1.75143 -3.39407
		-1.68591 -3.25734
		-1.6737 -3.23305
		-1.77562 -3.378
		-1.77562 -3.378
		-1.68662 -3.17903
		-1.94505 -3.65434
		-1.94995 -3.65173
		-1.94007 -3.61134
		-1.80205 -3.38567
		-1.73874 -3.23657
		-1.73205 -3.24365
		-1.70298 -3.22942
		-1.69003 -3.22454
		-1.78186 -3.38989
		-1.76854 -3.38519
		-1.68591 -3.25734
		-1.73732 -3.38831
		-1.63527 -3.23969
		-1.61881 -3.24794
		-1.60784 -3.30965
		-1.57558 -3.32854
		-1.56474 -3.31724
		-1.51418 -3.29802
		-1.47106 -3.37604
		-1.43164 -3.40412
		-1.43548 -3.50169
		-1.34882 -3.42475
		-1.3062 -3.42351
		-1.26433 -3.40638
		-1.24427 -3.40867
		-1.14181 -3.22856
		-1.16699 -3.30982
		-1.10722 -3.26234
		-1.08081 -3.27216
		-1.06288 -3.27803
		-0.965749 -3.38521
		-0.948274 -3.6514
		-0.559454 -3.25062
		-0.422132 -3.09257
		-0.4026 -3.41204
		-0.324674 -3.44966
		-0.294996 -3.59263
		-0.285904 -3.61087
		-0.202909 -3.4596
		-0.160081 -3.63919
		-0.110021 -3.74072
		-0.0711081 -3.46399
		0.0186693 -3.2298
		0.0367762 -3.16275
		0.0839087000000001 -3.20718
		1.93594 -2.69915
		1.9348 -2.61985
		1.9348 -2.61985
		2.03643 -2.7914
		1.8172 -2.47881
		1.832 -2.55204
		1.71689 -2.32478
		2.04718 -2.66609
		1.89799 -2.50393
		2.00485 -2.61665
		1.90081 -2.44894
		2.05691 -2.70697
		1.68773 -2.24227
		2.02762 -2.58314
		2.02762 -2.58314
		1.91602 -2.44825
		1.91129 -2.42214
		2.05027 -2.54385
		1.85721 -2.3866
		1.86508 -2.36186
		1.86487 -2.35927
		1.86487 -2.35927
		1.87359 -2.35512
		1.64166 -2.11626
		1.64659 -2.10353
		1.61264 -2.03906
		1.52172 -1.9187
		1.61292 -2.07149
		1.61292 -2.07149
		1.56542 -2.00497
		1.60649 -2.08844
		1.26427 -1.68354
		1.15994 -1.56054
		1.06747 -1.47413
		1.15569 -1.58683
		1.01575 -1.42637
		1.00779 -1.44284
		0.92562 -1.32962
		0.902242 -1.32023
		0.880452 -1.31562
		0.836983 -1.2604
		0.762903 -1.1995
		0.732902 -1.16905
		0.722641 -1.18046
		0.725612 -1.26381
		0.710975 -1.24658
		0.699102 -1.27683
		0.562801 -1.06851
		0.547881 -1.07123
		0.545139 -1.08196
		0.522358 -1.08684
		0.490717 -1.08811
		0.453457 -1.03764
		0.444816 -1.0476
		0.415922 -1.02163
		0.408715 -1.02179
		0.373178 -0.961217
		0.337963 -0.975484
		0.313302 -0.982454
		0.246844 -0.881095
		0.199602 -0.8306
		0.150652 -0.793232
		0.124568 -0.744509
		0.11018 -0.795742
		0.0744853000000001 -0.631923
		0.0675463999999999 -0.683258
		0.0352912000000001 -0.571276
		0.0270182000000001 -0.574137
		0.0198559 -0.635388
		-0.0184799 -0.654718
		-0.0676022999999999 -0.690108
		-0.102121 -0.62294
		-0.126229 -0.633774
		-0.161972 -0.621762
		-0.161169 -0.565296
		-0.169865 -0.462191
		-0.200065 -0.44869
		-0.248588 -0.497176
		-0.187927 -0.327023
		-0.271434 -0.402535
		-0.296763 -0.423088
		-0.305346 -0.389644
		-0.406204 -0.441335
		-0.449142 -0.442268
		-0.510652 -0.458809
		-0.439767 -0.308268
		-0.483317 -0.313691
		-0.46186 -0.29833
		-0.396499 -0.233453
		-0.429378 -0.230446
		-0.414269 -0.222337
		-0.430858 -0.216404
		-0.423035 -0.198298
		-0.430307 -0.18198
		-0.442945 -0.141896
		-0.454481 -0.121456
		-0.398619 -0.0552708
		-0.366676 -0.033612
		-0.37398 -0.0202572999999999
		-0.364638 -0.00151298999999994
		-0.38851 0.0356133999999999
		-0.509921 0.108034
		-0.517257 0.194524
		-0.527194 0.260174
		-0.485282 0.319942
		-0.393747 0.277212
		-0.409133 0.299907
		-0.400398 0.303053
		-0.344154 0.305376
		-0.337266 0.32908
		-0.290545 0.287711
		-0.314167 0.341278
		-0.22969 0.317191
		-0.236813 0.354455
		-0.222294 0.404954
		-0.206507 0.413013
		-0.233839 0.447101
		-0.176464 0.363307
		-0.173994 0.394281
		-0.168812 0.41451
		-0.0987562 0.289379
		-0.111986 0.361475
		-0.113415 0.37805
		-0.100983 0.397811
		-0.0627249000000001 0.349658
		-0.0412272 0.294162
		-0.0228554000000001 0.500915
		0.00135325999999991 0.358612
		0.0161617000000001 0.35825
		0.0443209 0.405002
		0.0313459 0.228129
		0.0502321999999999 0.249229
		0.0559672 0.256849
		0.0881262 0.31651
		0.130161 0.39362
		0.137166 0.391234
		0.219215 0.531759
		0.155804 0.340563
		0.221921 0.409701
		0.272984 0.461519
		0.27799 0.422545
		0.354188 0.480218
		0.433583 0.525401
		0.442106 0.486814
		0.483467 0.491349
		0.478657 0.468418
		0.462504 0.431827
		0.482321 0.41409
		0.462676 0.385939
		0.459076 0.370792
		0.490841 0.369299
		0.526478 0.380646
		0.464409 0.308218
		0.426479 0.271225
		0.443193 0.274357
		0.407237 0.226816
		0.413767 0.214674
		0.419003 0.204264
		0.47345 0.210422
		0.619061 0.232148
		0.54721 0.180206
		0.716239 0.190612
		0.715758 0.146601
		0.643962 0.0905167
		0.655865 0.0522602000000001
		0.733321 0.0119239
		0.733121 -0.0208611000000001
		0.664093 -0.0589115
		0.713379 -0.109308
		0.672972 -0.132966
		0.591781 -0.136378
		0.60043 -0.163754
		0.597269 -0.174932
		0.591409 -0.193823
		0.384288 -0.145932
		0.406427 -0.174183
		0.475157 -0.231271
		0.542549 -0.284656
		0.39438 -0.232205
		0.409747 -0.261113
		0.314431 -0.219947
		0.333429 -0.243725
		0.43416 -0.346869
		0.334418 -0.327303
		0.284554 -0.287565
		0.271752 -0.280614
		0.263549 -0.309251
		0.280419 -0.341094
		0.272629 -0.348177
		0.271292 -0.356175
		0.245458 -0.341438
		0.239427 -0.426479
		0.197548 -0.420704
		0.233728 -0.482064
		0.156482 -0.454181
		0.195251 -0.496435
		0.122548 -0.443772
		0.0768519000000001 -0.428941
		0.0613667 -0.486843
		0.044972 -0.451594
		0.0216312999999999 -0.473922
		-0.0194737 -0.517135
		-0.0483967999999999 -0.496593
		-0.0593220000000001 -0.447785
		-0.0742878 -0.441917
		-0.119973 -0.425529
		-0.135651 -0.412528
		-0.186729 -0.466823
		-0.196334 -0.436531
		-0.205812 -0.424097
		-0.262624 -0.488772
		-0.288676 -0.451057
		-0.346608 -0.452516
		-0.333546 -0.411373
		-0.484059 -0.566859
		-0.462191 -0.496855
		-0.462499 -0.470808
		-0.452466 -0.44182
		-0.436091 -0.344967
		-0.398069 -0.301451
		-0.401475 -0.246925
		-0.401148 -0.208388
		-0.456885 -0.217564
		-0.416312 -0.201039
		-0.414152 -0.192096
		-0.426589 -0.178196
		-0.428185 -0.145689
		-0.470065 -0.123908
		-0.38305 -0.0921862
		-0.455061 -0.093634
		-0.436497 -0.0595224000000001
		-0.430242 -0.0466095
		-0.395793 -0.0343456
		-0.396041 -0.0313532999999999
		-0.396386 -0.0218349
		-0.38914 -0.0133038999999999
		-0.381701 -0.00327643000000011
		-0.381701 -0.00327643000000011
		-0.349402 0.0176912
		-0.346399 0.0278881
		-0.346399 0.0278881
		-0.347093 0.0354478
		-0.349566 0.0309742
		-0.342216 0.037385
		-0.348395 0.0753671
		-0.399723 0.116313
		-0.399723 0.116313
		-0.389916 0.109813
		-0.359362 0.113483
		-0.347961 0.121577
		-0.364375 0.130345
		-0.364375 0.130345
		-0.334908 0.139545
		-0.336959 0.134517
		-0.347046 0.134735
		-0.348411 0.131166
	};
\addlegendentry{Prediction}
\addplot [draw=red, mark=o, only marks]
table{%
		x  y
		0.0348806381225586 2.39156436920166
		0.00684881210327148 2.39474391937256
		-0.0506510734558105 2.39443731307983
		-0.0847983360290527 2.39494776725769
		-0.116747379302979 2.39262461662292
		-0.183626651763916 2.38090682029724
		-0.2149658203125 2.37380695343018
		-0.245267391204834 2.3670642375946
		-0.277576446533203 2.3602819442749
		2.50666379928589 -1.00189578533173
		2.50902795791626 -0.959123849868774
		1.83770847320557 3.71651005744934
		1.51819849014282 3.96444225311279
		1.49879360198975 3.97521281242371
		0.990242958068848 4.0697455406189
		0.950779438018799 4.07549095153809
		0.912266731262207 4.08549046516418
		0.875215530395508 4.08731603622437
		0.801782608032227 4.09849834442139
		0.764955997467041 4.10351061820984
		0.728135108947754 4.10800647735596
		0.692924976348877 4.11366152763367
		0.654585838317871 4.11831283569336
		0.617834091186523 4.12234282493591
		0.578701019287109 4.12350106239319
		0.541058540344238 4.12933993339539
		0.469583034515381 4.13605856895447
		0.43604850769043 4.1387894153595
		0.406670570373535 4.14127397537231
		0.373043537139893 4.14441609382629
		0.341972351074219 4.14491891860962
		0.309821128845215 4.14388227462769
		0.277794361114502 4.14080929756165
		0.245537757873535 4.13900971412659
		0.213803291320801 4.13511061668396
		0.14548921585083 4.13243436813354
		0.110097885131836 4.12884593009949
		0.0715456008911133 4.12525463104248
		0.0320000648498535 4.12077903747559
		-0.00858640670776367 4.11617660522461
		-0.0512504577636719 4.1110565662384
		-0.0957322120666504 4.10541963577271
		-0.138855934143066 4.1009213924408
		-0.224547386169434 4.09509682655334
		-0.269137859344482 4.09284043312073
		-0.313196420669556 4.09102916717529
		-0.355009794235229 4.09032320976257
		-0.39616847038269 4.09057021141052
		-0.436958074569702 4.09112596511841
		-0.477277755737305 4.09213161468506
		-0.516749382019043 4.09348702430725
		-0.55644416809082 4.09554505348206
		-0.595999240875244 4.09798312187195
		-0.635366916656494 4.10095930099487
		-0.710631608963013 4.10780835151672
		-0.746728181838989 4.11220002174377
		-0.782769918441772 4.11697292327881
		-0.81770133972168 4.12233328819275
		-0.850539207458496 4.1285240650177
		-0.884166240692139 4.13433241844177
		-0.949852705001831 4.14455962181091
		-0.98133373260498 4.1486132144928
		-1.01424217224121 4.15104651451111
		-1.04505228996277 4.15742349624634
		-1.07655382156372 4.16180324554443
		-1.10940170288086 4.1661422252655
		-1.14253664016724 4.1702983379364
		-1.17253875732422 4.17235922813416
		-3.36154180765152 4.20306253433228
		-3.42997771501541 4.15532231330872
		-4.25797804445028 0.627000331878662
		-2.76788175106049 -2.64669377356768
		-2.73875796794891 -2.66590511798859
		-2.67853403091431 -2.69939654320478
		-2.64605629444122 -2.71739530563354
		-2.58246302604675 -2.75436447560787
		-2.21209621429443 -2.9495512843132
		-2.15789270401001 -2.96867322921753
		-2.13267469406128 -2.97837886214256
		2.50759840011597 -0.918373942375183
		0.505406856536865 4.13331317901611
		-0.181143283843994 4.09793090820312
		-0.918081521987915 4.13978624343872
		-2.08188199996948 -2.99363964796066
		-2.10686039924622 -2.98757037520409
	};
\addlegendentry{FN}



==> tikz/vis_localize/vis_loc_test1_x_clean.tex <==
\addplot [semithick, steelblue31119180]
table {%
		0.03009033203125 -0.475712776184082
		0.470058679580688 -0.490299224853516
		1.17013049125671 -0.354551792144775
		1.70008730888367 -0.384414911270142
		2.87009000778198 -0.166447162628174
		3.07010889053345 -0.079371452331543
		3.33006143569946 -0.0851850509643555
		3.60005140304565 -0.0804948806762695
		3.80003690719604 -0.0118660926818848
		4.07007265090942 0.121819496154785
		4.3000226020813 0.139509201049805
		4.77009201049805 0.159670352935791
		5.07003974914551 0.251852512359619
		5.43010520935059 0.278572082519531
		5.97006893157959 0.380838871002197
		6.270094871521 0.321840286254883
		6.6000337600708 0.227717399597168
		6.73014068603516 0.277008533477783
		7.00003623962402 0.423691749572754
		7.2300500869751 0.404416561126709
		7.50010299682617 0.486894130706787
		7.77009582519531 0.5541090965271
		8.10003566741943 0.5101318359375
		8.63003349304199 0.398483753204346
		8.77004146575928 0.404316425323486
		8.93015098571777 0.470919132232666
		9.10003471374512 0.443526268005371
		9.29999923706055 0.419477462768555
		9.87014675140381 0.481780052185059
		10.3300876617432 0.384975433349609
		10.5000581741333 0.28757381439209
		10.7000722885132 0.174269199371338
		10.8700866699219 0.177433013916016
		11.2301368713379 0.294008731842041
		11.7300462722778 0.324569702148438
		12.4000434875488 0.282667636871338
		13.0301647186279 0.163503646850586
		13.1700344085693 0.185089111328125
		13.3300762176514 0.213131904602051
		13.4701156616211 0.156392097473145
		13.7300357818604 0.00430774688720703
		14.0000953674316 -0.0377192497253418
		14.4000635147095 -0.0873661041259766
		14.9300670623779 -0.30614447593689
		15.5701341629028 -0.455579280853271
		15.8700580596924 -0.552461862564087
		16.1000747680664 -0.528228521347046
		16.630033493042 -0.423839330673218
		16.8700637817383 -0.306995868682861
		17.2300567626953 -0.0534162521362305
		17.5000419616699 0.183555126190186
		18.0300540924072 0.647718906402588
		18.3700580596924 0.839196681976318
		18.5700817108154 0.864442348480225
		19.0700550079346 0.78176736831665
		19.5301532745361 0.64145040512085
		19.7301979064941 0.52375602722168
		19.9000701904297 0.388992309570312
		20.2300624847412 0.102925777435303
		20.4000282287598 -0.0537261962890625
		20.8301067352295 -0.529167890548706
		21.030101776123 -0.613790035247803
		21.2301235198975 -0.610964775085449
		21.7301845550537 -0.605550527572632
		22.0700759887695 -0.710356950759888
		22.3700866699219 -0.756863832473755
		22.9301166534424 -0.77303147315979
		23.4300441741943 -0.701545476913452
		23.6300277709961 -0.617653131484985
		23.6700611114502 -0.598726034164429
		23.8001384735107 -0.555577516555786
		23.8300857543945 -0.485393285751343
		23.8700408935547 -0.460012674331665
		24.0001106262207 -0.41011905670166
		24.0001392364502 -0.359653949737549
		24.0900173187256 -0.31182599067688
		24.5000457763672 -0.0684695243835449
		24.6000919342041 -0.0187258720397949
		25.0300464630127 0.203932762145996
		25.2000389099121 0.296329498291016
		25.4300575256348 0.397636890411377
		25.600040435791 0.41546106338501
		26.3701171875 0.314286708831787
		26.7300357818604 0.349265575408936
		28.3000202178955 -0.640521287918091
		28.53005027771 -0.861037731170654
		28.8300437927246 -1.01171278953552
		29.5000591278076 -1.2240252494812
		29.730052947998 -1.35969018936157
		30.030200958252 -1.42318940162659
		30.3000469207764 -1.39639210700989
		30.7302055358887 -1.37686896324158
		31.1001262664795 -1.36466312408447
		31.3300666809082 -1.26674222946167
		31.6701240539551 -1.06659197807312
		32.0301132202148 -0.886617422103882
		32.4700965881348 -0.636722564697266
		33.2701072692871 0.0580167770385742
		34.3700408935547 1.06125926971436
		35.730094909668 1.66056871414185
		36.2000427246094 1.68765687942505
		36.6000442504883 1.6543402671814
		37.0300407409668 1.57043600082397
		37.5000419616699 1.30250549316406
		37.6700859069824 1.21079301834106
		39.4001197814941 -0.150369644165039
		40.8701019287109 -1.57450652122498
		41.1300811767578 -1.83015704154968
		41.7300605773926 -2.22741532325745
		42.4000778198242 -2.5062427520752
		43.0000381469727 -2.64365482330322
		43.9000663757324 -2.73668146133423
		44.2000732421875 -2.6546368598938
		45.1301155090332 -2.31106090545654
		45.2700881958008 -2.19887137413025
		45.5300521850586 -1.9574990272522
		45.8000259399414 -1.73467302322388
		46.1300621032715 -1.49463629722595
		46.3000907897949 -1.34667587280273
		46.7700462341309 -0.857147455215454
		47.0999984741211 -0.557061910629272
		47.7000160217285 0.0669064521789551
		47.9300575256348 0.348493099212646
		48.0700187683105 0.496395111083984
		50.400074005127 2.35356521606445
		50.5000457763672 2.39975595474243
		51.5300750732422 2.51091289520264
		52.1700706481934 2.48898935317993
		52.5700874328613 2.44101619720459
		52.9700546264648 2.47816514968872
		53.3000602722168 2.50352430343628
		53.9300727844238 2.45761966705322
		54.3000564575195 2.41002702713013
		55.4000434875488 2.11861371994019
		56.600025177002 1.385573387146
		61.9700126647949 -3.82414364814758
		63.4000587463379 -4.19627475738525
		63.7700500488281 -4.20442962646484
		64.0000381469727 -4.22210693359375
		64.5000686645508 -4.27991056442261
		64.8300247192383 -4.27383708953857
		65.9301223754883 -4.1322340965271
		66.0700225830078 -4.06741762161255
		68.2301406860352 -2.82563543319702
		69.5000762939453 -1.74574112892151
		69.6700592041016 -1.67882466316223
		69.9000549316406 -1.65622687339783
		70.3701019287109 -1.63774490356445
		70.7300796508789 -1.51706838607788
		70.9000930786133 -1.39501333236694
		71.700065612793 -0.563559532165527
		72.3301467895508 0.265230655670166
		74.5000610351562 2.17435836791992
		75.6703033447266 2.02492618560791
		76.0000457763672 1.87917232513428
		76.7300643920898 1.32710552215576
		76.9700546264648 1.16199111938477
		77.3700561523438 0.739748001098633
		77.6300735473633 0.46537971496582
		78.0700988769531 0.0667314529418945
		78.6001129150391 -0.427075624465942
		78.830078125 -0.552841424942017
		79.3300857543945 -0.675612688064575
		79.6000366210938 -0.667203187942505
		79.7000732421875 -0.629070043563843
		79.9701385498047 -0.430648326873779
		80.970100402832 0.611161231994629
		81.1702117919922 0.715634346008301
		81.4301300048828 0.777851581573486
		81.9700698852539 0.842184066772461
		82.2000732421875 0.708244323730469
		83.4700469970703 -0.405617713928223
		83.7300338745117 -0.508135318756104
		84.2700271606445 -0.628286838531494
		84.5300521850586 -0.591888189315796
		85.170036315918 -0.458978652954102
		85.8000259399414 -0.494639158248901
	};
\addlegendentry{MOCAP}
\addplot [semithick, darkorange25512714]
table {%
		0.03009033203125 -0.471812963485718
		0.100090265274048 -0.441061973571777
		0.130123853683472 -0.560840010643005
		0.200061798095703 -0.514194965362549
		0.330089569091797 -0.51866602897644
		0.700080156326294 -0.492563962936401
		0.730062246322632 -0.445873022079468
		0.770052671432495 -0.50617504119873
		0.830052614212036 -0.377665042877197
		0.930162191390991 -0.425956964492798
		0.970064163208008 -0.373587965965271
		1.07016015052795 -0.501719951629639
		1.17013049125671 -0.381155967712402
		1.23006153106689 -0.480875015258789
		1.37011170387268 -0.423699021339417
		1.400066614151 -0.485880970954895
		1.43003487586975 -0.426483988761902
		1.53005766868591 -0.411471009254456
		1.57014727592468 -0.356613993644714
		1.60003757476807 -0.43526303768158
		1.63007950782776 -0.268326044082642
		1.67003083229065 -0.285709023475647
		1.73008513450623 -0.330558061599731
		1.83007526397705 -0.318664073944092
		1.87012505531311 -0.304197072982788
		1.90008497238159 -0.401077032089233
		1.97007131576538 -0.323317050933838
		2.00001835823059 -0.367815017700195
		2.07010769844055 -0.259467005729675
		2.20001912117004 -0.242334961891174
		2.27015328407288 -0.155447959899902
		2.33014225959778 -0.159441947937012
		2.43009972572327 -0.104130029678345
		2.53007888793945 -0.0920425653457642
		2.57009553909302 -0.112805008888245
		2.63014960289001 -0.0439407825469971
		2.73005795478821 -0.0117900371551514
		2.8301088809967 0.0248780250549316
		3.00006723403931 0.070746898651123
		3.07010889053345 0.0923088788986206
		3.73010635375977 0.198614954948425
		3.80003690719604 0.298047065734863
		3.87004160881042 0.286635041236877
		3.9000563621521 0.327839970588684
		3.97006511688232 0.254050970077515
		4.2300386428833 0.314957976341248
		4.53002262115479 0.266126990318298
		4.63007593154907 0.428380012512207
		4.67004489898682 0.439275979995728
		4.70004272460938 0.399963021278381
		4.83008003234863 0.456202030181885
		4.97006702423096 0.477221965789795
		5.03003168106079 0.45188295841217
		5.40004587173462 0.448228001594543
		5.4700345993042 0.338969945907593
		5.53006553649902 0.414618015289307
		5.60007095336914 0.413156032562256
		5.6300630569458 0.597684979438782
		5.70003890991211 0.536983013153076
		5.73002815246582 0.556015014648438
		5.80005931854248 0.66101598739624
		5.83004331588745 0.5242999792099
		5.90005493164062 0.558454990386963
		5.93001508712769 0.484941959381104
		5.97006893157959 0.560622930526733
		6.00006866455078 0.453981995582581
		6.07004833221436 0.522324085235596
		6.13006496429443 0.443066000938416
		6.270094871521 0.471585035324097
		6.30007362365723 0.5295649766922
		6.37004280090332 0.503920078277588
		6.50004959106445 0.52020001411438
		6.53002405166626 0.493734955787659
		6.6000337600708 0.532348990440369
		6.63010740280151 0.484758973121643
		6.67010927200317 0.506587982177734
		6.73014068603516 0.45396900177002
		7.00003623962402 0.356663942337036
		7.03002977371216 0.470860958099365
		7.07007551193237 0.433367013931274
		7.10010576248169 0.473749995231628
		7.17006015777588 0.43287205696106
		7.27005672454834 0.338165044784546
		7.37013292312622 0.388872027397156
		7.53001070022583 0.379876017570496
		7.60008239746094 0.410140037536621
		7.70007610321045 0.473257064819336
		7.97008466720581 0.539245009422302
		8.10003566741943 0.361431002616882
		8.53009033203125 0.378085017204285
		8.57003879547119 0.488875031471252
		8.63003349304199 0.365273952484131
		8.67004871368408 0.419554948806763
		8.73017692565918 0.332385063171387
		8.87004280090332 0.300879001617432
		8.93015098571777 0.263787984848022
		9.00006008148193 0.284741044044495
		9.1700325012207 0.313534021377563
		9.2300386428833 0.270043969154358
		9.29999923706055 0.279412984848022
		9.50009346008301 0.289437055587769
		9.60006141662598 0.313979029655457
		9.63005638122559 0.404545068740845
		9.70013999938965 0.367388963699341
		9.77001953125 0.490190982818604
		9.83003234863281 0.391749024391174
		9.93007469177246 0.365257978439331
		10.0000801086426 0.334171056747437
		10.0300951004028 0.293624043464661
		10.1300315856934 0.288064002990723
		10.2301397323608 0.261397004127502
		10.3300876617432 0.22153103351593
		10.470046043396 0.254476070404053
		10.8700866699219 0.257463932037354
		10.9000844955444 0.402981042861938
		10.9701023101807 0.152317047119141
		11.1300582885742 0.127467036247253
		11.170126914978 0.180484056472778
		11.2000865936279 0.123154044151306
		11.2301368713379 0.192787051200867
		11.3700733184814 0.196758985519409
		11.4300832748413 0.163377046585083
		11.9300518035889 0.195726990699768
		12.0700359344482 0.197183012962341
		12.2000694274902 0.203847050666809
		12.3000822067261 0.140826940536499
		12.4700260162354 0.129557013511658
		12.5301160812378 0.237805962562561
		12.5701103210449 0.206387996673584
		12.630054473877 0.395110011100769
		12.7000513076782 0.380962014198303
		12.8300609588623 0.456285953521729
		12.8700437545776 0.350710034370422
		12.9300317764282 0.386322021484375
		12.9700784683228 0.366850018501282
		13.000096321106 0.415565967559814
		13.0301647186279 0.366905927658081
		13.1300411224365 0.390043020248413
		13.300121307373 0.421396017074585
		13.3300762176514 0.331238031387329
		13.3701019287109 0.376958966255188
		13.4701156616211 0.222977995872498
		13.7300357818604 0.183593988418579
		13.8000545501709 0.208030939102173
		13.9000244140625 0.251867055892944
		14.1001100540161 0.242393016815186
		14.1301651000977 0.198709964752197
		14.2000827789307 0.21593701839447
		14.3700361251831 0.100232005119324
		14.5301418304443 -0.0768415927886963
		14.6300449371338 -0.0982505083084106
		14.8000459671021 -0.282459020614624
		14.8300428390503 -0.25271201133728
		14.8701000213623 -0.26970100402832
		14.9300670623779 -0.235873937606812
		15.0701026916504 -0.373422026634216
		15.1000642776489 -0.266520023345947
		15.1700954437256 -0.320543050765991
		15.2000789642334 -0.274855971336365
		15.2300262451172 -0.360363960266113
		15.3300342559814 -0.34940505027771
		15.3600482940674 -0.420868992805481
		15.4300289154053 -0.374788999557495
		15.4700508117676 -0.367069959640503
		15.53005027771 -0.439065933227539
		15.7300386428833 -0.467906951904297
		15.8000202178955 -0.388545989990234
		15.8700580596924 -0.521239042282104
		15.9000234603882 -0.544371008872986
		16.0000419616699 -0.428758025169373
		16.1000747680664 -0.58463191986084
		16.1700325012207 -0.569776058197021
		16.2000789642334 -0.508279085159302
		16.230052947998 -0.604872941970825
		16.2701244354248 -0.552502989768982
		16.3000812530518 -0.403459072113037
		16.3700828552246 -0.521529912948608
		16.4700813293457 -0.43928599357605
		16.57004737854 -0.350739002227783
		16.630033493042 -0.429697036743164
		16.6701221466064 -0.415910005569458
		16.7001190185547 -0.355785012245178
		16.7300262451172 -0.374482035636902
		16.8000431060791 -0.289351940155029
		16.8300647735596 -0.371327996253967
		16.9301643371582 -0.36080801486969
		17.0000305175781 -0.429975986480713
		17.1000518798828 -0.372115969657898
		17.2300567626953 -0.312927961349487
		17.3000545501709 -0.288428068161011
		17.3700332641602 -0.209795951843262
		17.6300449371338 -0.0334670543670654
		17.770055770874 0.0507164001464844
		17.8300304412842 0.0956960916519165
		17.8700428009033 0.0844883918762207
		17.9301071166992 0.112210988998413
		17.9700317382812 0.105666041374207
		18.0300540924072 0.205857992172241
		18.0700454711914 0.197389960289001
		18.3301162719727 0.571262001991272
		18.4301414489746 0.560552000999451
		18.4700260162354 0.630707025527954
		18.5301647186279 0.541607022285461
		18.6300468444824 0.404356956481934
		18.7300510406494 0.541221976280212
		18.7700500488281 0.531748056411743
		18.8300819396973 0.430495023727417
		18.9000053405762 0.511078000068665
		19.0300674438477 0.538049936294556
		19.1000537872314 0.483922958374023
		19.1300716400146 0.537296056747437
		19.2000923156738 0.522922992706299
		19.2301216125488 0.450500965118408
		19.4000835418701 0.428797006607056
		19.5000514984131 0.457741022109985
		19.5301532745361 0.410282015800476
		19.6300811767578 0.642313957214355
		19.7000579833984 0.60956597328186
		19.7301979064941 0.578212022781372
		19.7700462341309 0.468382000923157
		19.8000869750977 0.494262933731079
		19.8300437927246 0.381101965904236
		19.8700695037842 0.404778957366943
		19.9301109313965 0.300572037696838
		20.0000324249268 0.279361963272095
		20.0700759887695 0.438353061676025
		20.1700630187988 0.385655999183655
		20.3701095581055 0.329757928848267
		20.430082321167 0.241026043891907
		20.5000286102295 0.224043011665344
		20.6001586914062 0.107959032058716
		21.0001049041748 -0.168269991874695
		21.2001419067383 -0.246317028999329
		21.3701019287109 -0.328914999961853
		21.4302387237549 -0.284937977790833
		21.5000419616699 -0.370494961738586
		21.5300674438477 -0.290394067764282
		21.6300525665283 -0.32361102104187
		21.6700305938721 -0.34027898311615
		21.7301845550537 -0.479104042053223
		21.8300857543945 -0.710874080657959
		21.8701362609863 -0.656491041183472
		21.9000492095947 -0.718400955200195
		21.9300365447998 -0.692844986915588
		22.0300388336182 -0.780995011329651
		22.1000385284424 -0.718091011047363
		22.1301002502441 -0.626848936080933
		22.1700668334961 -0.662261962890625
		22.2300605773926 -0.761030912399292
		22.2700366973877 -0.729853987693787
		22.3000431060791 -0.800524950027466
		22.3700866699219 -0.734633922576904
		22.4300918579102 -0.815353989601135
		22.5300464630127 -0.79112696647644
		22.6000652313232 -0.792942047119141
		22.6300506591797 -0.831512928009033
		22.6700916290283 -0.803298950195312
		22.7300853729248 -0.830116987228394
		22.8000373840332 -0.811691045761108
		22.8300457000732 -0.837032079696655
		22.9301166534424 -0.794672966003418
		22.9701766967773 -0.830286026000977
		23.0700454711914 -0.785321950912476
		23.5000400543213 -0.768876075744629
		23.5700912475586 -0.829856991767883
		23.6300277709961 -0.817214012145996
		23.6700611114502 -0.755191087722778
		24.0001392364502 -0.580209016799927
		24.1600494384766 -0.339069008827209
		24.2701206207275 -0.156646013259888
		24.3300476074219 -0.0631101131439209
		24.4301490783691 0.0208580493927002
		24.5000457763672 0.109559059143066
		24.6300830841064 0.223209977149963
		24.8301296234131 0.410153031349182
		25.0300464630127 0.443477988243103
		25.0800514221191 0.328948020935059
		25.1000747680664 0.479076027870178
		25.130033493042 0.338268995285034
		25.2000389099121 0.476534962654114
		25.2300567626953 0.411054968833923
		25.270133972168 0.471895933151245
		25.3300380706787 0.604864001274109
		25.4300575256348 0.721320986747742
		25.4700870513916 0.654144048690796
		25.5300273895264 0.629909038543701
		25.5700569152832 0.734676003456116
		25.600040435791 0.669937014579773
		25.7700805664062 0.578788042068481
		25.8300552368164 0.604030013084412
		25.8700542449951 0.591855049133301
		25.9000606536865 0.664538025856018
		25.9300193786621 0.564068078994751
		25.9700489044189 0.605556964874268
		26.0300464630127 0.560128927230835
		26.2300281524658 0.436514973640442
		26.3300609588623 0.542226076126099
		26.3701171875 0.550205945968628
		27.4300785064697 -0.11589503288269
		27.4709510803223 -0.11589503288269
		27.6700706481934 -0.42299497127533
		27.7300624847412 -0.481238961219788
		27.8301124572754 -0.569491028785706
		27.9000625610352 -0.600818991661072
		28.0300788879395 -0.657302975654602
		28.0700454711914 -0.752292990684509
		28.1300525665283 -0.718474984169006
		28.2300720214844 -0.744758009910583
		28.4000396728516 -1.09953999519348
		28.5000114440918 -1.13940000534058
		28.6700305938721 -1.22091996669769
		28.8300437927246 -1.27637994289398
		28.9001083374023 -1.23075997829437
		28.9301109313965 -1.33077001571655
		28.9700050354004 -1.30573999881744
		29.0300388336182 -1.37097001075745
		29.2000350952148 -1.33125996589661
		29.2700481414795 -1.37669003009796
		29.3700866699219 -1.39757001399994
		29.4301242828369 -1.61884999275208
		29.6000823974609 -1.77425003051758
		29.630090713501 -1.82633996009827
		29.6701602935791 -1.77459001541138
		29.730052947998 -1.79418003559113
		29.8701343536377 -1.77570998668671
		29.9701480865479 -1.80167996883392
		30.030200958252 -1.71296000480652
		30.4300918579102 -1.66261994838715
		30.700080871582 -1.52227997779846
		30.7302055358887 -1.60316002368927
		30.7701511383057 -1.58504998683929
		30.8000583648682 -1.52230000495911
		30.8300552368164 -1.64444994926453
		30.9000473022461 -1.62808001041412
		31.0300216674805 -1.42871999740601
		31.1001262664795 -1.64381003379822
		31.1300449371338 -1.66138005256653
		31.2000770568848 -1.50641000270844
		31.2700939178467 -1.46780002117157
		31.3000545501709 -1.52723002433777
		31.3300666809082 -1.34248995780945
		31.370023727417 -1.45291996002197
		31.430061340332 -1.41302001476288
		31.4701442718506 -1.50761997699738
		31.5000419616699 -1.38529002666473
		31.5301399230957 -1.50144004821777
		31.5700931549072 -1.51791000366211
		31.6001319885254 -1.63499999046326
		31.7301082611084 -1.33774995803833
		31.8300380706787 -1.18722999095917
		31.930061340332 -1.25460004806519
		31.9700622558594 -1.22332000732422
		32.0000228881836 -1.27690005302429
		32.2000579833984 -1.13300001621246
		32.3300323486328 -0.838655948638916
		32.3700294494629 -0.915439009666443
		32.4301223754883 -0.802294015884399
		32.4700965881348 -0.778789043426514
		32.5301132202148 -0.613332986831665
		32.5701599121094 -0.634382009506226
		32.6301231384277 -0.587904930114746
		32.8300437927246 -0.427137970924377
		32.9700584411621 -0.298241019248962
		33.1000289916992 -0.16516900062561
		33.2000885009766 -0.0300222635269165
		33.3300857543945 0.16942298412323
		33.3700637817383 0.187481045722961
		33.4700775146484 0.369835019111633
		33.700065612793 0.591874003410339
		33.7300186157227 0.687958002090454
		33.8000793457031 0.702769041061401
		34.0301208496094 0.960461020469666
		34.1000289916992 0.757278919219971
		34.270092010498 0.908384084701538
		34.3000221252441 1.21862995624542
		34.3700408935547 1.51055002212524
		35.6000480651855 1.95002996921539
		35.6301231384277 1.86056005954742
		35.7000350952148 1.83775997161865
		35.770076751709 1.98745000362396
		35.8000717163086 1.83373999595642
		35.8300552368164 2.03210997581482
		35.8700714111328 2.00976991653442
		35.9300804138184 2.06512999534607
		35.970027923584 1.87786996364594
		36.0300636291504 2.00729990005493
		36.1000328063965 1.91931998729706
		36.1700706481934 1.93904995918274
		36.2300491333008 1.98619997501373
		36.27001953125 2.07119011878967
		36.3000564575195 1.95455002784729
		36.3300132751465 2.09461998939514
		36.3700218200684 2.10917997360229
		36.4000511169434 1.93321001529694
		36.4300575256348 2.03550004959106
		36.4700660705566 1.88095998764038
		36.5300788879395 2.06397008895874
		36.6000442504883 2.07300996780396
		36.6700553894043 2.1282000541687
		36.7300834655762 2.09839010238647
		36.8300552368164 1.91682994365692
		36.9000434875488 1.85769999027252
		37.0300407409668 1.67307996749878
		37.1300621032715 1.65077996253967
		37.2000045776367 1.7936999797821
		37.4300956726074 1.65823996067047
		37.5300903320312 1.52438998222351
		37.6700859069824 1.33992004394531
		38.8700904846191 0.508049964904785
		38.9300498962402 0.44060206413269
		38.9701118469238 0.371320962905884
		39.0300521850586 0.423526048660278
		39.1000556945801 0.350357055664062
		39.1701278686523 0.317124962806702
		39.4001197814941 0.0105714797973633
		39.6300392150879 -0.109063029289246
		39.6701812744141 -0.0660574436187744
		39.7301216125488 -0.145369052886963
		39.7700691223145 -0.137418031692505
		39.8301277160645 -0.169185996055603
		39.9300384521484 -0.17562198638916
		39.9700546264648 -0.182029962539673
		40.0702285766602 -0.640362024307251
		40.1301383972168 -0.707689046859741
		40.170108795166 -0.69300103187561
		40.2301445007324 -0.861562967300415
		40.3300247192383 -0.872424006462097
		40.400074005127 -1.04328000545502
		40.4300765991211 -0.933372020721436
		40.5000457763672 -1.1909099817276
		40.5700340270996 -1.25236999988556
		40.6300315856934 -1.27400994300842
		40.700065612793 -1.37067997455597
		40.7700881958008 -1.42557001113892
		40.8000755310059 -1.51034998893738
		40.8300895690918 -1.3493800163269
		40.8701019287109 -1.38706004619598
		40.9000244140625 -1.31886005401611
		40.9300956726074 -1.45700001716614
		40.9700927734375 -1.28790998458862
		41.0300636291504 -1.51170003414154
		41.1300811767578 -1.4447900056839
		41.2301750183105 -1.85625004768372
		41.2701034545898 -1.86843001842499
		41.400016784668 -2.07530999183655
		41.4302139282227 -2.04327988624573
		41.5300254821777 -2.15199995040894
		41.6000518798828 -2.17852997779846
		41.6300621032715 -2.13228011131287
		41.7000274658203 -2.19023990631104
		41.7300605773926 -2.0913999080658
		41.8000946044922 -2.20063996315002
		41.8300628662109 -2.1774799823761
		41.9000244140625 -2.19764995574951
		41.9301643371582 -2.36895990371704
		41.9700546264648 -2.38565993309021
		42.0300941467285 -2.60014009475708
		42.1000518798828 -2.71370005607605
		42.1700592041016 -2.41860008239746
		42.7000427246094 -2.68724989891052
		42.7700233459473 -2.67027997970581
		42.9000549316406 -2.73984003067017
		42.9702796936035 -2.69180011749268
		43.0300178527832 -2.75746011734009
		43.1001205444336 -2.76136994361877
		43.2301139831543 -2.93154001235962
		43.3000373840332 -2.90686988830566
		43.3301658630371 -3.16056990623474
		43.3700942993164 -2.82206010818481
		43.470085144043 -3.17547988891602
		43.5000495910645 -2.81595993041992
		43.5300178527832 -2.88668990135193
		43.60009765625 -2.88517999649048
		43.6300582885742 -2.83396005630493
		43.670036315918 -2.92531991004944
		43.730037689209 -2.8060200214386
		43.8000984191895 -2.91565990447998
		43.9300231933594 -2.8342399597168
		43.9700622558594 -3.43163990974426
		44.0000991821289 -3.19879007339478
		44.0301094055176 -3.40122008323669
		44.1300392150879 -2.83634996414185
		44.2000732421875 -2.72777009010315
		44.3000679016113 -2.84869003295898
		44.330135345459 -2.69754004478455
		44.3700904846191 -2.72450995445251
		44.4300308227539 -2.65565991401672
		44.5000686645508 -2.69840002059937
		44.5700492858887 -2.66280007362366
		44.6000213623047 -2.64475011825562
		44.6300430297852 -2.91965007781982
		44.6700782775879 -2.70848989486694
		44.7300300598145 -3.15377998352051
		44.8000526428223 -3.02339005470276
		44.8700637817383 -3.03190994262695
		45.0000457763672 -2.92916011810303
		45.1000137329102 -2.87093997001648
		45.1700782775879 -2.7787299156189
		45.230052947998 -2.77840995788574
		45.2700881958008 -2.71500992774963
		45.3700523376465 -2.75114011764526
		45.4000434875488 -2.67510008811951
		45.4300384521484 -2.82122993469238
		45.4700508117676 -2.72375988960266
		45.5000419616699 -2.82746005058289
		45.5300521850586 -2.60402011871338
		45.5700454711914 -2.71104001998901
		45.6300582885742 -2.43350005149841
		45.6700134277344 -2.44179010391235
		45.8000259399414 -2.18444991111755
		45.8300628662109 -2.1660099029541
		45.8700370788574 -2.25262999534607
		45.9300880432129 -2.08877992630005
		45.9700698852539 -1.98057997226715
		46.0701026916504 -2.08933997154236
		46.1300621032715 -1.93777000904083
		46.1700820922852 -1.98722994327545
		46.3701667785645 -1.73701000213623
		46.4700775146484 -1.4931800365448
		46.5302429199219 -1.4960800409317
		46.6000328063965 -1.43769001960754
		46.6700439453125 -1.45544004440308
		46.7300567626953 -1.22345995903015
		46.8300628662109 -1.17218995094299
		46.9300308227539 -1.16753995418549
		47.0300636291504 -1.03812003135681
		47.5000381469727 -0.516492009162903
		47.6301116943359 -0.304496049880981
		47.7300262451172 -0.222813010215759
		47.8000068664551 -0.104140043258667
		47.9300575256348 -0.0661718845367432
		48.0000648498535 0.0706751346588135
		48.0700187683105 0.259621024131775
		50.2700805664062 2.4514000415802
		50.3000984191895 2.42498993873596
		50.3300666809082 2.47163009643555
		50.3701324462891 2.4386899471283
		50.4300765991211 2.47987008094788
		51.5300750732422 2.87819004058838
		51.9700660705566 2.96075010299683
		52.0000534057617 2.86568999290466
		52.030086517334 2.923180103302
		52.1000480651855 2.80721998214722
		52.1300392150879 2.70108008384705
		52.2001152038574 2.89653992652893
		52.2300796508789 2.73908996582031
		52.3000144958496 2.9135000705719
		52.3700942993164 2.92046999931335
		52.4300651550293 2.92974996566772
		52.4701652526855 3.05035996437073
		52.5300521850586 2.93582010269165
		52.5700874328613 2.92408990859985
		52.6000823974609 3.04129004478455
		52.7000503540039 3.04680991172791
		52.770076751709 2.89988994598389
		52.8300971984863 2.91345000267029
		52.9000587463379 2.88066005706787
		52.9700546264648 2.83177995681763
		53.0300788879395 2.99249005317688
		53.1000595092773 2.8201699256897
		53.170051574707 2.85474991798401
		53.2700576782227 2.83732008934021
		53.3300971984863 2.9534900188446
		53.3701171875 2.94789004325867
		53.4300270080566 2.85220003128052
		53.4701385498047 2.85524010658264
		53.5301246643066 2.60033011436462
		53.6000556945801 2.62298989295959
		53.7000885009766 2.76950001716614
		53.7312927246094 2.5068199634552
		53.7701148986816 2.59363007545471
		53.800106048584 2.79706001281738
		53.8300437927246 2.66162991523743
		53.9000282287598 2.80060005187988
		54.0000343322754 2.66191005706787
		54.1000633239746 2.64383006095886
		54.130054473877 2.56381988525391
		54.1701126098633 2.67664003372192
		54.2000465393066 2.59388995170593
		54.2300910949707 2.66917991638184
		54.3300437927246 2.46023011207581
		54.400032043457 2.54270005226135
		54.4300155639648 2.51307010650635
		54.4700469970703 2.6956799030304
		54.5301246643066 2.5420401096344
		54.570068359375 2.34921002388
		54.6000900268555 2.48007988929749
		55.4000434875488 2.60664010047913
		56.3301620483398 1.30057001113892
		56.500072479248 1.48740994930267
		56.600025177002 1.47713005542755
		56.7301139831543 1.16736996173859
		56.7700653076172 1.39452004432678
		56.930046081543 1.01236999034882
		61.9700126647949 -3.62374997138977
		63.1700706481934 -4.02918004989624
		63.2300643920898 -4.10531997680664
		63.5301132202148 -4.28002023696899
		63.5700531005859 -4.21049976348877
		63.6300468444824 -4.28145980834961
		63.7000274658203 -4.24921989440918
		63.7300605773926 -4.11527013778687
		63.7700500488281 -4.12059020996094
		63.8300666809082 -3.63001990318298
		64.0300445556641 -3.66260004043579
		64.0700378417969 -4.22417020797729
		64.1300201416016 -3.66436004638672
		64.1700592041016 -3.57915997505188
		64.3000640869141 -3.69906997680664
		64.3300476074219 -4.07356977462769
		64.3700561523438 -3.70029997825623
		64.400032043457 -3.80238008499146
		64.430046081543 -3.70097994804382
		64.5700454711914 -3.9533998966217
		64.6300354003906 -4.00946998596191
		64.670036315918 -4.0155200958252
		64.7000427246094 -4.06003999710083
		64.7300491333008 -3.96706008911133
		64.8700408935547 -3.99614000320435
		64.9000854492188 -4.39162015914917
		64.930046081543 -4.3019700050354
		65.0000610351562 -4.32605981826782
		65.0300750732422 -4.16612005233765
		65.0700607299805 -4.42383003234863
		65.1300659179688 -4.18271017074585
		65.2000350952148 -4.14053010940552
		65.3700485229492 -4.32896995544434
		65.4000473022461 -3.95927000045776
		65.4700241088867 -4.16150999069214
		65.5000152587891 -4.06260013580322
		65.5700836181641 -4.08828020095825
		65.6301116943359 -4.03725004196167
		65.6700897216797 -4.04188013076782
		65.7000579833984 -4.18401002883911
		65.7700271606445 -4.1779899597168
		65.8301315307617 -4.03451013565063
		65.9000625610352 -4.22551012039185
		65.970085144043 -4.25030994415283
		66.0301055908203 -4.16229009628296
		66.0700225830078 -4.46759986877441
		68.0300979614258 -3.33817005157471
		68.0701141357422 -3.40352010726929
		68.170051574707 -3.3581600189209
		68.2301406860352 -3.0725200176239
		69.1000595092773 -2.64825010299683
		69.1300888061523 -2.49471998214722
		69.330078125 -2.38801002502441
		69.3701477050781 -2.29099988937378
		69.4000473022461 -2.06964993476868
		69.430061340332 -2.2219500541687
		69.470085144043 -2.03682994842529
		69.5000762939453 -2.19269990921021
		69.6700592041016 -1.99430000782013
		69.7000961303711 -2.05664992332458
		69.7300415039062 -1.92502999305725
		69.8300399780273 -1.92432999610901
		69.8700408935547 -1.65837001800537
		69.9700622558594 -1.94007003307343
		70.0000762939453 -1.69748997688293
		70.0300445556641 -1.91218996047974
		70.0701217651367 -1.69552004337311
		70.1000595092773 -1.90479004383087
		70.1300811767578 -1.69552004337311
		70.1700668334961 -1.75143003463745
		70.2300338745117 -1.69126999378204
		70.3000640869141 -1.68689000606537
		70.3300247192383 -1.7756199836731
		70.3701019287109 -1.7756199836731
		70.4000778198242 -1.68661999702454
		70.5000762939453 -1.9499499797821
		70.6300582885742 -1.7320499420166
		70.7300796508789 -1.69869995117188
		70.8000335693359 -1.90479004383087
		70.8701171875 -1.68590998649597
		70.9000930786133 -1.73731994628906
		70.9701843261719 -1.61881005764008
		71.1300888061523 -1.47106003761292
		71.3701171875 -1.24426996707916
		71.4000473022461 -1.14181005954742
		71.4301834106445 -1.16699004173279
		71.700065612793 -0.94827401638031
		72.2300186157227 -0.294996023178101
		72.2700500488281 -0.285903930664062
		72.3700866699219 -0.110020995140076
		72.5000686645508 0.0839086771011353
		74.5000610351562 1.93594002723694
		75.5300903320312 1.93480002880096
		75.5700378417969 2.03642988204956
		75.6301651000977 1.81719994544983
		75.6703033447266 1.83200001716614
		75.8000106811523 1.71688997745514
		75.9301834106445 2.04717993736267
		75.9700622558594 1.89798998832703
		76.0301208496094 2.00484991073608
		76.0700988769531 1.90081000328064
		76.1000061035156 2.05691003799438
		76.1700439453125 1.68772995471954
		76.2300872802734 2.02762007713318
		76.3300628662109 1.91602003574371
		76.430046081543 1.91129004955292
		76.4700469970703 2.05027008056641
		76.6000366210938 1.86507999897003
		76.7300643920898 1.87358999252319
		76.8000717163086 1.64165997505188
		76.9000549316406 1.64658999443054
		76.9700546264648 1.61264002323151
		77.0300827026367 1.52172005176544
		77.1000671386719 1.61292004585266
		77.1300201416016 1.56542003154755
		77.1700820922852 1.60649001598358
		77.2301177978516 1.26426994800568
		77.3300933837891 1.06746995449066
		77.3700561523438 1.15568995475769
		77.4300765991211 1.00778996944427
		77.5301895141602 0.880451917648315
		77.7301330566406 0.710974931716919
		77.7700958251953 0.69910192489624
		77.830078125 0.547881007194519
		77.9000549316406 0.522357940673828
		78.0300979614258 0.415921926498413
		78.1000747680664 0.373178005218506
		78.4300918579102 0.0352911949157715
		78.5300827026367 -0.0184799432754517
		78.6700668334961 -0.161972045898438
		78.770133972168 -0.200065016746521
		78.8000411987305 -0.248587965965271
		78.830078125 -0.187927007675171
		78.9000396728516 -0.296762943267822
		79.0300750732422 -0.5106520652771
		79.0700836181641 -0.439767003059387
		79.1001129150391 -0.483317017555237
		79.2300567626953 -0.414268970489502
		79.4000778198242 -0.45448100566864
		79.5300750732422 -0.373980045318604
		79.6000366210938 -0.38850998878479
		79.6300811767578 -0.509921073913574
		79.7000732421875 -0.527194023132324
		79.8300399780273 -0.485281944274902
		79.9000091552734 -0.409132957458496
		80.0300598144531 -0.290544986724854
		80.0701370239258 -0.314167022705078
		80.1301116943359 -0.229689955711365
		80.2000427246094 -0.222293972969055
		80.2700729370117 -0.23383903503418
		80.3300170898438 -0.173994064331055
		80.3701477050781 -0.168812036514282
		80.4301071166992 -0.0987561941146851
		80.5301132202148 -0.100983023643494
		80.6301345825195 -0.0412272214889526
		80.970100402832 0.137166023254395
		81.0000381469727 0.219215035438538
		81.0300369262695 0.155804038047791
		81.1300582885742 0.272984027862549
		81.200080871582 0.281671047210693
		81.3000183105469 0.442106008529663
		81.3300399780273 0.483466982841492
		81.5300369262695 0.490841031074524
		81.5700912475586 0.526478052139282
		81.6301422119141 0.426478981971741
		81.6701507568359 0.443192958831787
		81.7300567626953 0.413766980171204
		81.7700958251953 0.419003009796143
		81.800048828125 0.473449945449829
		81.8300552368164 0.61906099319458
		81.8700714111328 0.547209978103638
		81.9302062988281 0.715758085250854
		82.0000457763672 0.655864953994751
		82.0300521850586 0.733320951461792
		82.0701293945312 0.733120918273926
		82.1300354003906 0.664093017578125
		82.1700820922852 0.71337902545929
		82.2700424194336 0.600430011749268
		82.3300704956055 0.591408967971802
		82.4000473022461 0.406427025794983
		82.4701156616211 0.542549014091492
		82.5301132202148 0.409747004508972
		82.570068359375 0.314430952072144
		82.6300354003906 0.328639984130859
		82.670036315918 0.434159994125366
		82.7300720214844 0.284554004669189
		82.8700942993164 0.272629022598267
		83.170036315918 0.100880980491638
		83.5000991821289 -0.119972944259644
		83.7700958251953 -0.333546042442322
		83.8300399780273 -0.462190985679626
		83.9301300048828 -0.43609094619751
		84.0000610351562 -0.392639994621277
		84.1300048828125 -0.401147961616516
		84.1701126098633 -0.456884980201721
		84.2301177978516 -0.414152026176453
		84.4000473022461 -0.470064997673035
		84.4300384521484 -0.383049964904785
		84.5000686645508 -0.458029985427856
		84.5700607299805 -0.43024206161499
		84.700080871582 -0.388875961303711
		84.8300857543945 -0.381700992584229
		84.9000396728516 -0.346399068832397
		85.2701110839844 -0.348394989967346
		85.3301315307617 -0.399723052978516
		85.7000350952148 -0.336959004402161
		85.8000259399414 -0.348410964012146
	};
\addlegendentry{Prediction}


==> tikz/vis_localize/vis_loc_test1_y_clean.tex <==
\addplot [semithick, steelblue31119180]
table {%
		0.03009033203125 0.139563798904419
		0.330089569091797 0.0983812808990479
		0.63004732131958 0.139361143112183
		0.830052614212036 0.146421194076538
		1.00008797645569 0.0905110836029053
		1.30009770393372 -0.0325417518615723
		1.8000590801239 -0.032109260559082
		2.1300482749939 -0.170641660690308
		2.30007886886597 -0.155733108520508
		2.60006666183472 -0.0823824405670166
		2.7701268196106 -0.130792617797852
		2.97012758255005 -0.218178272247314
		3.13010787963867 -0.237581968307495
		3.33006143569946 -0.277148485183716
		3.87004160881042 -0.233037233352661
		4.3000226020813 -0.302407026290894
		5.03003168106079 -0.267449617385864
		5.40004587173462 -0.280841112136841
		5.77006244659424 -0.298526525497437
		6.03004837036133 -0.261584997177124
		6.270094871521 -0.289541006088257
		6.53002405166626 -0.320741415023804
		6.80002117156982 -0.269120216369629
		7.20003271102905 -0.131262063980103
		8.27006816864014 -0.122554779052734
		8.63003349304199 -0.140771865844727
		8.77004146575928 -0.0924298763275146
		9.0700626373291 0.0648679733276367
		9.73003196716309 0.150851488113403
		9.93007469177246 0.094106912612915
		10.3300876617432 -0.0333311557769775
		10.5300931930542 -0.0162003040313721
		10.8300457000732 0.072174072265625
		11.2000865936279 0.165462255477905
		11.5701293945312 0.14007830619812
		12.2702045440674 -0.0274648666381836
		12.500057220459 -0.118470430374146
		12.7701063156128 -0.129929780960083
		13.0700674057007 -0.106391429901123
		13.4001188278198 -0.173283576965332
		13.7000312805176 -0.252387285232544
		14.3315372467041 -0.223186731338501
		14.5000486373901 -0.140568494796753
		14.8300428390503 0.0562930107116699
		15.1301345825195 0.0785534381866455
		15.3300342559814 0.113877296447754
		15.53005027771 0.234650373458862
		16.0300636291504 0.538650989532471
		16.4700813293457 0.642142057418823
		17.1000518798828 1.00202345848083
		17.3300647735596 0.98904275894165
		17.770055770874 0.888093948364258
		18.0300540924072 0.761553049087524
		18.2701282501221 0.587558031082153
		19.7301979064941 -0.684187531471252
		20.3300838470459 -0.922146797180176
		20.6001586914062 -0.96311092376709
		20.7700901031494 -0.902953028678894
		21.170072555542 -0.559221982955933
		21.470027923584 -0.265467882156372
		21.6700305938721 -0.126609563827515
		22.0700759887695 -0.00017857551574707
		22.4701175689697 0.133702993392944
		22.6700916290283 0.231238126754761
		22.8300457000732 0.25778603553772
		22.9701766967773 0.222410202026367
		23.270092010498 0.01287841796875
		23.4700584411621 -0.111368894577026
		23.6700611114502 -0.180262565612793
		23.8300857543945 -0.229013204574585
		24.2501258850098 -0.349688053131104
		24.380126953125 -0.417801856994629
		24.5000457763672 -0.441160678863525
		24.7000942230225 -0.40570592880249
		24.9000720977783 -0.337311029434204
		25.1700534820557 -0.145843029022217
		25.5300273895264 0.132177591323853
		26.0701599121094 0.420798301696777
		26.3701171875 0.612309217453003
		26.7300357818604 0.737952947616577
		27.6700706481934 0.914646625518799
		28.1000289916992 0.850518226623535
		28.4700679779053 0.848468542098999
		28.730094909668 0.80456280708313
		28.9301109313965 0.719378709793091
		29.130126953125 0.579573392868042
		29.7000865936279 0.160382032394409
		29.9701480865479 0.00356006622314453
		30.3701496124268 -0.27105450630188
		30.8300552368164 -0.680518627166748
		32.2300567626953 -1.51480090618134
		32.5301132202148 -1.58453369140625
		33.5001449584961 -1.66237783432007
		33.8000793457031 -1.54839432239532
		34.3700408935547 -1.33309471607208
		35.9001083374023 -0.138564586639404
		36.5300788879395 0.551533222198486
		37.2000045776367 1.06638813018799
		37.6700859069824 1.56264567375183
		38.9701118469238 2.34287858009338
		39.1701278686523 2.38764262199402
		39.5701370239258 2.3532121181488
		40.4300765991211 2.1641538143158
		40.6700439453125 2.02273631095886
		41.0000267028809 1.84299373626709
		41.6700325012207 1.49846315383911
		42.3300971984863 0.936257839202881
		42.8000526428223 0.572771549224854
		43.5300178527832 -0.166093826293945
		43.8000984191895 -0.390228033065796
		44.3000679016113 -0.901326298713684
		44.7001037597656 -1.32868719100952
		44.9300346374512 -1.51895153522491
		45.2700881958008 -1.74912691116333
		45.9300880432129 -2.24848461151123
		46.8300628662109 -2.62849807739258
		48.0700187683105 -2.92049813270569
		50.3300666809082 -2.0145788192749
		50.5000457763672 -1.86874735355377
		51.3000450134277 -1.08475148677826
		51.5300750732422 -0.798977017402649
		52.2001152038574 -0.127415180206299
		52.6000823974609 0.444752931594849
		52.6701126098633 0.532661914825439
		52.8700714111328 0.763455390930176
		53.5000610351562 1.49879837036133
		53.7312927246094 1.81110191345215
		54.2000465393066 2.24539732933044
		54.6000900268555 2.62879347801208
		55.4000434875488 3.37461233139038
		56.3301620483398 3.94429039955139
		56.7700653076172 4.04181957244873
		56.930046081543 4.0647668838501
		61.9700126647949 3.79132008552551
		63.7700500488281 2.07479500770569
		64.1300201416016 1.5873019695282
		64.400032043457 1.25935435295105
		64.6300354003906 1.0174880027771
		64.8000259399414 0.843485116958618
		65.6301116943359 -0.229782819747925
		65.9000625610352 -0.477459669113159
		66.0700225830078 -0.665006399154663
		68.0701141357422 -2.52657175064087
		68.2301406860352 -2.61183214187622
		69.2300491333008 -3.01995038986206
		69.5000762939453 -3.01782155036926
		69.9300689697266 -3.00601363182068
		70.3300247192383 -2.9998414516449
		71.0700607299805 -2.98277711868286
		71.5701293945312 -2.99458861351013
		72.0000305175781 -2.93912506103516
		72.5000686645508 -2.93404507637024
		75.5300903320312 -2.68307113647461
		76.6000366210938 -1.84347724914551
		76.8000717163086 -1.70078778266907
		77.7700958251953 -1.07305634021759
		78.0000228881836 -0.929558396339417
		78.3701400756836 -0.701361775398254
		79.2000350952148 0.0719368457794189
		79.9000091552734 0.770983457565308
		80.1301116943359 0.891423463821411
		80.4701309204102 0.937446594238281
		80.7300491333008 0.897632360458374
		80.9000625610352 0.802412033081055
		81.7000579833984 0.090538501739502
		81.9302062988281 -0.141768455505371
		82.4701156616211 -0.478108167648315
		82.9300689697266 -0.635545015335083
		83.1001052856445 -0.616654515266418
		83.3000869750977 -0.511988639831543
		83.9301300048828 -0.0673706531524658
		84.2001037597656 0.140683174133301
		84.4300384521484 0.283860921859741
		84.9700469970703 0.470431327819824
		85.7700424194336 0.531158447265625
		85.8000259399414 0.531203746795654
	};
\addlegendentry{MOCAP}
\addplot [semithick, darkorange25512714]
table {%
		0.03009033203125 -0.21331000328064
		0.100090265274048 -0.201244950294495
		0.130123853683472 -0.268602013587952
		0.200061798095703 -0.237620949745178
		0.300041437149048 -0.246750950813293
		0.430106163024902 -0.245550990104675
		0.470058679580688 -0.276751041412354
		0.530123233795166 -0.226464033126831
		0.670176267623901 -0.231752038002014
		0.90015697479248 -0.237491011619568
		0.930162191390991 -0.282793045043945
		0.970064163208008 -0.247483015060425
		1.07016015052795 -0.362715005874634
		1.17013049125671 -0.285007953643799
		1.23006153106689 -0.417773962020874
		1.37011170387268 -0.363458037376404
		1.400066614151 -0.413812041282654
		1.47007870674133 -0.389122009277344
		1.50005984306335 -0.4113609790802
		1.57014727592468 -0.342059016227722
		1.60003757476807 -0.417405962944031
		1.63007950782776 -0.271036028862
		1.67003083229065 -0.297311067581177
		1.73008513450623 -0.352370977401733
		1.87012505531311 -0.359362006187439
		1.93005132675171 -0.495471954345703
		1.97007131576538 -0.457375049591064
		2.00001835823059 -0.5347980260849
		2.03002858161926 -0.462805032730103
		2.10004281997681 -0.495409965515137
		2.1300482749939 -0.551585912704468
		2.23006868362427 -0.482605934143066
		2.30007886886597 -0.504971027374268
		2.50008296966553 -0.424777984619141
		2.57009553909302 -0.521161079406738
		2.63014960289001 -0.377565979957581
		2.7701268196106 -0.437361001968384
		2.8301088809967 -0.39970600605011
		2.9300696849823 -0.411702990531921
		3.00006723403931 -0.454268932342529
		3.10007524490356 -0.424425959587097
		3.17004442214966 -0.431931972503662
		3.20006251335144 -0.511606931686401
		3.27007532119751 -0.416530013084412
		3.33006143569946 -0.419615983963013
		3.37002658843994 -0.384247064590454
		3.40004563331604 -0.454661011695862
		3.43004322052002 -0.363793015480042
		3.50008893013 -0.430567979812622
		3.5300350189209 -0.386148929595947
		3.60005140304565 -0.446367979049683
		3.630042552948 -0.371592998504639
		3.70006990432739 -0.365453958511353
		3.73010635375977 -0.284291982650757
		3.80003690719604 -0.3593590259552
		3.87004160881042 -0.308797001838684
		3.9000563621521 -0.347708940505981
		3.97006511688232 -0.265483021736145
		4.2300386428833 -0.280297994613647
		4.43007755279541 -0.225389957427979
		4.47004413604736 -0.263890027999878
		4.53002262115479 -0.236840009689331
		4.63007593154907 -0.342311978340149
		4.67004489898682 -0.369390964508057
		4.73005390167236 -0.312320947647095
		4.83008003234863 -0.300184965133667
		4.97006702423096 -0.288790941238403
		5.03003168106079 -0.239344954490662
		5.37011337280273 -0.252475023269653
		5.50009346008301 -0.20988404750824
		5.57005214691162 -0.229334950447083
		5.6300630569458 -0.320765018463135
		5.70003890991211 -0.283803939819336
		5.80005931854248 -0.34660005569458
		5.83004331588745 -0.275946974754333
		5.97006893157959 -0.276064038276672
		6.03004837036133 -0.236547946929932
		6.07004833221436 -0.251039028167725
		6.13006496429443 -0.210238933563232
		6.67010927200317 -0.137954950332642
		6.80002117156982 -0.0438623428344727
		7.20003271102905 0.0737361907958984
		7.43002223968506 0.0422927141189575
		7.73004722595215 0.0452190637588501
		8.00005435943604 0.072152853012085
		8.43009376525879 0.0538606643676758
		8.67004871368408 0.154013991355896
		8.83009624481201 0.168002963066101
		9.03005790710449 0.213237047195435
		9.13005638122559 0.259022951126099
		9.43015193939209 0.195063948631287
		9.50009346008301 0.233579993247986
		9.60006141662598 0.250915050506592
		9.63005638122559 0.32602596282959
		9.70013999938965 0.282844066619873
		9.77001953125 0.388067960739136
		9.87014675140381 0.305578947067261
		10.0700340270996 0.214789032936096
		10.2700710296631 0.165959000587463
		10.4001026153564 0.149984955787659
		10.470046043396 0.181285977363586
		10.630054473877 0.179098963737488
		10.7000722885132 0.200065970420837
		10.8700866699219 0.20693302154541
		10.9000844955444 0.332316040992737
		10.9701023101807 0.140251994132996
		11.0301065444946 0.139495015144348
		11.170126914978 0.181429028511047
		11.2000865936279 0.126412034034729
		11.2701168060303 0.196676969528198
		11.5701293945312 0.141741991043091
		12.0000715255737 0.157763957977295
		12.2000694274902 0.149919033050537
		12.2702045440674 0.086617112159729
		12.8300609588623 0.0245535373687744
		12.9000415802002 0.00686919689178467
		13.0700674057007 -0.0205816030502319
		13.4701156616211 -0.116480946540833
		13.5000820159912 -0.192659020423889
		13.6001377105713 -0.152379989624023
		13.7000312805176 -0.218971967697144
		13.7300357818604 -0.192494988441467
		13.8000545501709 -0.252411007881165
		13.9300861358643 -0.3038649559021
		13.9700546264648 -0.311607956886292
		14.0000953674316 -0.354033946990967
		14.0300750732422 -0.318400025367737
		14.1001100540161 -0.364500999450684
		14.1301651000977 -0.336151003837585
		14.2000827789307 -0.418007016181946
		14.3315372467041 -0.401917934417725
		14.3700361251831 -0.422546029090881
		14.4700679779053 -0.328204989433289
		14.5000486373901 -0.349593997001648
		14.6000595092773 -0.275007963180542
		14.8000459671021 -0.420067071914673
		14.9300670623779 -0.283733010292053
		15.0701026916504 -0.310435056686401
		15.1301345825195 -0.192837953567505
		15.4300289154053 -0.176983952522278
		15.7701148986816 -0.0603282451629639
		16.0000419616699 0.0587096214294434
		16.2000789642334 0.125983953475952
		16.2701244354248 0.200909972190857
		16.3000812530518 0.174658060073853
		16.3700828552246 0.263033032417297
		16.57004737854 0.229632019996643
		16.630033493042 0.290961027145386
		16.6701221466064 0.299229025840759
		16.7300262451172 0.283437967300415
		16.8000431060791 0.266986012458801
		16.8700637817383 0.355340957641602
		16.9301643371582 0.39960503578186
		17.0300407409668 0.577522993087769
		17.1300373077393 0.628491997718811
		17.2000579833984 0.60403299331665
		17.2700119018555 0.64766800403595
		17.3700332641602 0.511503934860229
		17.430025100708 0.453187942504883
		17.5302410125732 0.472751021385193
		17.5700664520264 0.612874984741211
		17.670108795166 0.320865988731384
		17.7300415039062 0.311509966850281
		17.770055770874 0.25943398475647
		17.8300304412842 0.499534010887146
		17.8700428009033 0.317137956619263
		17.9301071166992 0.438642024993896
		17.9700317382812 0.34993302822113
		18.0300540924072 0.473861932754517
		18.0700454711914 0.418604016304016
		18.3000621795654 0.762911081314087
		18.4301414489746 0.67399799823761
		18.4700260162354 0.689619064331055
		18.5301647186279 0.564291954040527
		18.6300468444824 0.373401999473572
		18.7300510406494 0.465398073196411
		18.8700351715088 0.298747062683105
		18.970043182373 0.295791029930115
		19.0300674438477 0.277545928955078
		19.1000537872314 0.175214052200317
		19.5301532745361 -0.056649923324585
		19.6701412200928 -0.271811008453369
		19.7301979064941 -0.309574007987976
		19.8300437927246 -0.26588499546051
		19.8700695037842 -0.310330986976624
		19.9301109313965 -0.276764988899231
		20.0000324249268 -0.297006011009216
		20.1000843048096 -0.548102021217346
		20.1300582885742 -0.607787013053894
		20.1700630187988 -0.559329032897949
		20.2300624847412 -0.671558976173401
		20.270055770874 -0.64218807220459
		20.3701095581055 -0.719470977783203
		20.430082321167 -0.635673046112061
		20.5000286102295 -0.800153970718384
		20.5300998687744 -0.736285924911499
		20.5701217651367 -0.741415977478027
		20.6302032470703 -0.568590998649597
		20.6700553894043 -0.628250002861023
		20.7300510406494 -0.829945087432861
		20.8000869750977 -0.759768962860107
		20.8700733184814 -0.751812934875488
		20.9300899505615 -0.7882399559021
		21.1300563812256 -0.720927953720093
		21.3300590515137 -0.704802989959717
		21.4000873565674 -0.647740006446838
		21.4302387237549 -0.516029000282288
		21.470027923584 -0.678015947341919
		21.5700435638428 -0.441434979438782
		21.6700305938721 -0.398237943649292
		21.7301845550537 -0.494395017623901
		21.8300857543945 -0.611351013183594
		21.8701362609863 -0.532992005348206
		21.9000492095947 -0.560703039169312
		21.9300365447998 -0.489259958267212
		22.0000438690186 -0.554682016372681
		22.1700668334961 -0.336387038230896
		22.7000408172607 -0.146770000457764
		22.8300457000732 -0.135820031166077
		23.3700428009033 -0.313439965248108
		23.4300441741943 -0.338871955871582
		23.5000400543213 -0.36641800403595
		23.6700611114502 -0.522067070007324
		23.8300857543945 -0.741286993026733
		23.8700408935547 -0.746592998504639
		24.0001392364502 -0.843940019607544
		24.1000442504883 -0.716525077819824
		24.1700801849365 -0.769183993339539
		24.2701206207275 -0.783231019973755
		24.3300476074219 -0.660027027130127
		24.4000282287598 -0.663032054901123
		24.4301490783691 -0.765792012214661
		24.7700672149658 -0.697610020637512
		25.0100517272949 -0.556880950927734
		25.0800514221191 -0.334115028381348
		25.1000747680664 -0.450186967849731
		25.130033493042 -0.306293964385986
		25.2000389099121 -0.339450001716614
		25.270133972168 -0.299744963645935
		25.3000450134277 -0.322490930557251
		25.4300575256348 -0.145427942276001
		25.600040435791 0.00274562835693359
		26.000057220459 0.411342024803162
		26.2000350952148 0.490422010421753
		26.2700366973877 0.559538006782532
		26.3701171875 0.811378955841064
		26.7300357818604 0.876332998275757
		27.570011138916 0.852172017097473
		27.6300239562988 0.931115984916687
		27.7000427246094 1.00006997585297
		27.8000164031982 0.945502042770386
		28.0300788879395 0.877628087997437
		28.0700454711914 0.916857957839966
		28.1300525665283 0.860672950744629
		28.2000617980957 0.798987984657288
		28.3300170898438 0.810405969619751
		28.4000396728516 0.91396701335907
		28.730094909668 0.817847967147827
		28.8300437927246 0.736186981201172
		29.3300266265869 0.430427074432373
		29.5300674438477 0.376714944839478
		29.6000823974609 0.292780995368958
		29.6701602935791 0.144983053207397
		29.770076751709 0.0750844478607178
		29.8301105499268 -0.0574173927307129
		30.030200958252 -0.17854905128479
		30.700080871582 -0.688652038574219
		30.7302055358887 -0.771278023719788
		30.8000583648682 -0.753193020820618
		30.8700733184814 -0.89849591255188
		30.930082321167 -0.946223020553589
		31.0000514984131 -0.928802013397217
		31.1300449371338 -1.16865003108978
		31.170129776001 -1.09748995304108
		31.3000545501709 -1.21692001819611
		31.3300666809082 -1.09546995162964
		31.4000759124756 -1.27154004573822
		31.4701442718506 -1.39762997627258
		31.5000419616699 -1.28934001922607
		31.6001319885254 -1.71069002151489
		31.6300868988037 -1.67755997180939
		31.7000675201416 -1.50315999984741
		31.7301082611084 -1.53523004055023
		31.770092010498 -1.46610999107361
		31.8300380706787 -1.53325998783112
		31.930061340332 -1.76321995258331
		31.9700622558594 -1.7942099571228
		32.0301132202148 -1.9760400056839
		32.0701713562012 -2.09274005889893
		32.1000671386719 -2.0395200252533
		32.1700553894043 -2.13189005851746
		32.2300567626953 -2.02505993843079
		32.2700653076172 -2.09335994720459
		32.3300323486328 -1.82752001285553
		32.3700294494629 -2.03048992156982
		32.4301223754883 -1.89749002456665
		32.4700965881348 -1.89948999881744
		32.5301132202148 -1.79872000217438
		32.6301231384277 -1.83643996715546
		32.6700401306152 -1.81139004230499
		32.7000579833984 -1.86679995059967
		32.7300415039062 -1.84493005275726
		32.7700424194336 -1.87548005580902
		32.8300437927246 -1.95718002319336
		32.8701133728027 -2.00833010673523
		32.9300994873047 -1.93157994747162
		33.0300979614258 -1.93315994739532
		33.0700569152832 -1.89672005176544
		33.1700706481934 -2.02723002433777
		33.2000885009766 -1.90942001342773
		33.3000679016113 -2.13421988487244
		33.4000816345215 -2.10585999488831
		33.4300880432129 -1.88837003707886
		33.5001449584961 -2.07209992408752
		33.6701507568359 -1.92412996292114
		33.7300186157227 -2.1797399520874
		33.8000793457031 -2.00694990158081
		34.0301208496094 -2.18811988830566
		34.1000289916992 -1.55189001560211
		34.2301139831543 -1.62372994422913
		34.270092010498 -1.5604100227356
		34.3000221252441 -1.84477996826172
		34.3700408935547 -2.1274299621582
		35.7000350952148 -0.540880918502808
		35.770076751709 -0.52647602558136
		35.8300552368164 -0.479712009429932
		35.9001083374023 -0.411519050598145
		36.0701103210449 -0.19199800491333
		37.0300407409668 0.822265028953552
		37.1300621032715 0.911970973014832
		37.2000045776367 1.14084994792938
		37.3700752258301 1.27427995204926
		37.4300956726074 1.26464998722076
		37.600040435791 1.36705005168915
		37.6700859069824 1.3342000246048
		38.8700904846191 1.71403002738953
		38.9300498962402 1.88511002063751
		38.9701118469238 1.81417000293732
		39.0300521850586 1.91730999946594
		39.1701278686523 1.74930000305176
		39.4001197814941 1.82360005378723
		39.5701370239258 1.92769002914429
		39.6300392150879 1.6954300403595
		39.6701812744141 1.73781001567841
		39.7700691223145 1.96393001079559
		39.8000717163086 1.77313995361328
		39.8301277160645 1.87196004390717
		39.9000663757324 1.83989000320435
		39.9300384521484 1.66840994358063
		40.0000419616699 1.84354996681213
		40.0702285766602 2.43487000465393
		40.100025177002 2.35647988319397
		40.1301383972168 2.38844990730286
		40.170108795166 2.27699995040894
		40.2301445007324 2.4977400302887
		40.3000793457031 2.31668996810913
		40.3700408935547 2.39201998710632
		40.400074005127 2.49584007263184
		40.4300765991211 2.29300999641418
		40.5000457763672 2.3818199634552
		40.530086517334 2.41724991798401
		40.6300315856934 2.38776993751526
		40.6700439453125 2.41181993484497
		40.7700881958008 2.28569006919861
		40.8000755310059 2.20323991775513
		40.8300895690918 1.98600995540619
		40.8701019287109 2.01301002502441
		40.9000244140625 1.87937998771667
		40.9300956726074 1.98294997215271
		40.9700927734375 1.72127997875214
		41.0300636291504 1.91761004924774
		41.1300811767578 1.65929996967316
		41.2301750183105 1.95104002952576
		41.3700675964355 1.91560995578766
		41.400016784668 1.98287999629974
		41.4302139282227 1.90488994121552
		41.5300254821777 1.87674999237061
		41.6000518798828 1.83631002902985
		41.6700325012207 1.74907004833221
		41.7300605773926 1.61228001117706
		41.8000946044922 1.65048003196716
		41.8700408935547 1.56447005271912
		41.9301643371582 1.59610998630524
		41.9700546264648 1.57104003429413
		42.0000839233398 1.61293995380402
		42.0300941467285 1.57800996303558
		42.1000518798828 1.58377003669739
		42.1700592041016 1.33828997612
		42.3300971984863 1.19547998905182
		42.4000778198242 1.09535002708435
		42.5700378417969 0.997338056564331
		42.6300621032715 0.89336895942688
		42.7000427246094 0.840795040130615
		42.9301414489746 0.58259391784668
		43.0300178527832 0.456807971000671
		43.1700592041016 0.367248058319092
		43.5000495910645 0.0419042110443115
		43.6300582885742 -0.117383003234863
		44.0000991821289 -0.504570960998535
		44.0701141357422 -0.613052010536194
		44.2000732421875 -0.653012037277222
		44.3000679016113 -0.779276013374329
		44.400074005127 -0.834335088729858
		44.5300598144531 -1.019739985466
		44.6000213623047 -1.06775999069214
		44.6300430297852 -1.20434999465942
		44.6700782775879 -1.13774001598358
		44.770133972168 -1.42587995529175
		45.200023651123 -1.85161995887756
		45.230052947998 -1.98740005493164
		45.2700881958008 -1.98254001140594
		45.3700523376465 -2.11626005172729
		45.5000419616699 -2.37245988845825
		45.5300521850586 -2.21191000938416
		45.5700454711914 -2.35238003730774
		45.6300582885742 -2.23309993743896
		45.7000541687012 -2.27611994743347
		45.8000259399414 -2.28499007225037
		45.8700370788574 -2.46715998649597
		45.9300880432129 -2.38454008102417
		45.9700698852539 -2.38942003250122
		46.0701026916504 -2.63864994049072
		46.1300621032715 -2.56195998191833
		46.2000770568848 -2.74373006820679
		46.2300682067871 -2.77970004081726
		46.2700881958008 -2.75994992256165
		46.3300514221191 -2.83759999275208
		46.3701667785645 -2.79264998435974
		46.4300575256348 -2.67037010192871
		46.5302429199219 -2.76915001869202
		46.6300811767578 -2.80117988586426
		46.6700439453125 -2.95971989631653
		46.7300567626953 -2.63514995574951
		46.799991607666 -2.84931993484497
		46.9000015258789 -3.0491099357605
		47.0300636291504 -2.96606993675232
		47.3700332641602 -3.00379991531372
		47.4300956726074 -3.1168200969696
		47.5300598144531 -3.26462006568909
		47.6301116943359 -3.20672988891602
		47.6700401306152 -3.46669006347656
		47.7700691223145 -3.03914999961853
		47.830135345459 -3.19047999382019
		47.9000473022461 -3.24270009994507
		47.9300575256348 -3.72768998146057
		48.0000648498535 -3.45298004150391
		48.0700187683105 -3.25007009506226
		50.2700805664062 -2.68387007713318
		50.3300666809082 -2.55234003067017
		50.3701324462891 -2.44844007492065
		50.400074005127 -2.49202990531921
		50.4300765991211 -2.37372994422913
		50.4700660705566 -2.42479991912842
		50.5000457763672 -2.39583992958069
		51.3000450134277 -1.72341001033783
		51.5300750732422 -1.3822900056839
		52.3700942993164 -0.34514594078064
		52.4701652526855 -0.175626993179321
		52.5700874328613 0.00886094570159912
		52.6701126098633 0.119729042053223
		53.5700416564941 1.18516004085541
		53.7000885009766 1.31280994415283
		53.7312927246094 1.24116003513336
		53.8300437927246 1.45735001564026
		53.9300727844238 1.64769005775452
		53.970085144043 1.63601994514465
		54.0300483703613 1.68072998523712
		54.130054473877 1.72395002841949
		54.1701126098633 1.82456004619598
		54.2000465393066 1.78048002719879
		54.2300910949707 1.85722994804382
		54.3300437927246 1.81919002532959
		54.4700469970703 2.19574999809265
		54.5001029968262 2.08705997467041
		54.5301246643066 2.12147998809814
		54.570068359375 2.02886009216309
		54.6000900268555 2.17124009132385
		55.4000434875488 3.27893996238708
		56.3301620483398 2.5931499004364
		56.500072479248 3.33139991760254
		56.600025177002 3.45356011390686
		56.7301139831543 2.92273998260498
		56.7700653076172 3.39534997940063
		56.930046081543 3.03710007667542
		61.9700126647949 3.8958899974823
		63.5301132202148 2.47289991378784
		63.6000366210938 2.40007996559143
		63.7000274658203 2.33107995986938
		63.7300605773926 2.21099996566772
		63.7700500488281 2.2010600566864
		63.8300666809082 1.81500995159149
		63.900074005127 1.77911996841431
		64.0000381469727 1.67825996875763
		64.0700378417969 1.86887001991272
		64.1300201416016 1.54230999946594
		64.2300872802734 1.44341003894806
		64.3000640869141 1.39259004592896
		64.3300476074219 1.5171400308609
		64.400032043457 1.31919002532959
		64.4700775146484 1.23618996143341
		64.930046081543 0.90182900428772
		65.0300750732422 0.657190084457397
		65.0700607299805 0.685383081436157
		65.2000350952148 0.500120997428894
		65.3700485229492 0.363779067993164
		65.4700241088867 0.197062969207764
		65.6700897216797 0
		65.7700271606445 -0.151291966438293
		65.8301315307617 -0.168103933334351
		65.9301223754883 -0.341336011886597
		66.0000228881836 -0.443045020103455
		66.0700225830078 -0.538114070892334
		68.0300979614258 -2.51827001571655
		68.0701141357422 -2.6217999458313
		68.170051574707 -2.72251009941101
		68.2301406860352 -2.58447003364563
		69.1000595092773 -3.50612998008728
		69.1300888061523 -3.39756989479065
		69.2000274658203 -3.42075991630554
		69.2300491333008 -3.51275992393494
		69.2701568603516 -3.46000003814697
		69.330078125 -3.58202004432678
		69.3701477050781 -3.52553009986877
		69.4000473022461 -3.29610991477966
		69.430061340332 -3.48496007919312
		69.470085144043 -3.29615998268127
		69.5300750732422 -3.53081011772156
		69.6700592041016 -3.39479994773865
		69.7000961303711 -3.55239009857178
		69.7300415039062 -3.38269996643066
		69.8300399780273 -3.37311005592346
		69.8700408935547 -3.01253008842468
		69.9700622558594 -3.61134004592896
		70.0000762939453 -3.23877000808716
		70.0300445556641 -3.62616991996765
		70.0701217651367 -3.25582003593445
		70.1000595092773 -3.63428997993469
		70.1300811767578 -3.25582003593445
		70.1700668334961 -3.39406991004944
		70.2300338745117 -3.25802993774414
		70.2700424194336 -3.23305010795593
		70.3000640869141 -3.2592499256134
		70.3300247192383 -3.37800002098083
		70.3701019287109 -3.37800002098083
		70.4000778198242 -3.17902994155884
		70.4700927734375 -3.65434002876282
		70.5300598144531 -3.61134004592896
		70.6300582885742 -3.24364995956421
		70.7300796508789 -3.23166990280151
		70.8000335693359 -3.63428997993469
		70.8701171875 -3.25733995437622
		70.9000930786133 -3.38830995559692
		70.930046081543 -3.23969006538391
		70.9701843261719 -3.24794006347656
		71.030029296875 -3.32854008674622
		71.1000518798828 -3.29801988601685
		71.2000579833984 -3.50168991088867
		71.2300567626953 -3.42475008964539
		71.3701171875 -3.40866994857788
		71.4000473022461 -3.22855997085571
		71.4301834106445 -3.30981993675232
		71.5300674438477 -3.27216005325317
		71.6001052856445 -3.27802991867065
		71.700065612793 -3.65140008926392
		72.0000305175781 -3.25061988830566
		72.0700378417969 -3.09257006645203
		72.1000518798828 -3.41203999519348
		72.2000427246094 -3.44966006278992
		72.2700500488281 -3.61086988449097
		72.3000335693359 -3.45959997177124
		72.3700866699219 -3.74072003364563
		72.4300689697266 -3.22979998588562
		72.4700698852539 -3.16275000572205
		72.5000686645508 -3.20718002319336
		74.5000610351562 -2.69915008544922
		75.5300903320312 -2.61984992027283
		75.5700378417969 -2.79139995574951
		75.6301651000977 -2.47881007194519
		75.6703033447266 -2.55204010009766
		75.8000106811523 -2.32477998733521
		75.9301834106445 -2.66609001159668
		75.9700622558594 -2.50393009185791
		76.0301208496094 -2.61665010452271
		76.0700988769531 -2.44894003868103
		76.1000061035156 -2.70696997642517
		76.1700439453125 -2.24226999282837
		76.2300872802734 -2.58313989639282
		76.3300628662109 -2.44825005531311
		76.430046081543 -2.42213988304138
		76.4700469970703 -2.54384994506836
		76.6000366210938 -2.36186003684998
		76.7300643920898 -2.35511994361877
		76.8000717163086 -2.11626005172729
		76.9000549316406 -2.10352993011475
		76.9700546264648 -2.03906011581421
		77.0300827026367 -1.9186999797821
		77.1000671386719 -2.07149004936218
		77.1300201416016 -2.00497007369995
		77.1700820922852 -2.08843994140625
		77.2301177978516 -1.68353998661041
		77.3300933837891 -1.47413003444672
		77.3700561523438 -1.58683001995087
		77.4300765991211 -1.44283998012543
		77.5000152587891 -1.32023000717163
		77.6700820922852 -1.18045997619629
		77.7301330566406 -1.24658000469208
		77.7700958251953 -1.27682995796204
		77.830078125 -1.07123005390167
		77.9301376342773 -1.08810997009277
		78.0000228881836 -1.04760003089905
		78.1300659179688 -0.975484013557434
		78.1701278686523 -0.982454061508179
		78.2300415039062 -0.830600023269653
		78.3000411987305 -0.744508981704712
		78.3301391601562 -0.795742034912109
		78.3701400756836 -0.631922960281372
		78.4000854492188 -0.683258056640625
		78.4300918579102 -0.571275949478149
		78.4701843261719 -0.574136972427368
		78.5300827026367 -0.654717922210693
		78.5701065063477 -0.690108060836792
		78.630241394043 -0.633774042129517
		78.6700668334961 -0.621762037277222
		78.770133972168 -0.448689937591553
		78.8000411987305 -0.497175931930542
		78.830078125 -0.327023029327393
		78.9000396728516 -0.423088073730469
		78.9300765991211 -0.389644026756287
		79.0000534057617 -0.442268013954163
		79.1001129150391 -0.313691020011902
		79.2000350952148 -0.230445981025696
		79.3300857543945 -0.181980013847351
		79.5300750732422 -0.0202573537826538
		79.6000366210938 0.0356134176254272
		79.7000732421875 0.260174036026001
		79.8300399780273 0.319941997528076
		79.8700942993164 0.277212023735046
		79.9300994873047 0.303053021430969
		80.1301116943359 0.317191004753113
		80.2700729370117 0.44710099697113
		80.3000564575195 0.363306999206543
		80.3701477050781 0.414510011672974
		80.4301071166992 0.289379000663757
		80.5301132202148 0.397810935974121
		80.6301345825195 0.294162034988403
		80.6700668334961 0.500915050506592
		80.7300491333008 0.358250021934509
		80.7700805664062 0.405001997947693
		80.8301239013672 0.249228954315186
		80.8700408935547 0.256849050521851
		81.0000381469727 0.531759023666382
		81.0300369262695 0.340563058853149
		81.1300582885742 0.461519002914429
		81.200080871582 0.407256960868835
		81.2700729370117 0.525400996208191
		81.3300399780273 0.4913489818573
		81.6000900268555 0.308218002319336
		81.7000579833984 0.226815938949585
		81.800048828125 0.210422039031982
		81.8300552368164 0.232148051261902
		82.0701293945312 -0.0208611488342285
		82.2000732421875 -0.132966041564941
		82.3300704956055 -0.193822979927063
		82.3700637817383 -0.145931959152222
		82.5301132202148 -0.261112928390503
		82.570068359375 -0.219946980476379
		82.6300354003906 -0.251114964485168
		82.7000427246094 -0.327302932739258
		82.7700500488281 -0.280614018440247
		82.9000625610352 -0.356174945831299
		83.0300521850586 -0.482064008712769
		83.0700454711914 -0.454180955886841
		83.1001052856445 -0.496434926986694
		83.129997253418 -0.443771958351135
		83.170036315918 -0.461725950241089
		83.2000350952148 -0.428941011428833
		83.2300567626953 -0.48684298992157
		83.2700347900391 -0.451593995094299
		83.3700332641602 -0.496592998504639
		83.4300384521484 -0.441916942596436
		83.5300598144531 -0.412528038024902
		83.5700454711914 -0.466822981834412
		83.6300430297852 -0.424097061157227
		83.670051574707 -0.488772034645081
		83.7700958251953 -0.411373019218445
		83.8000335693359 -0.566859006881714
		83.8700942993164 -0.470808029174805
		83.9001235961914 -0.441820025444031
		83.9701156616211 -0.301450967788696
		84.700080871582 -0.024203896522522
		85.2701110839844 0.0753670930862427
		85.3301315307617 0.116312980651855
		85.4700775146484 0.121577024459839
		85.7700424194336 0.134734988212585
		85.8000259399414 0.131165981292725
	};
\addlegendentry{Pred}


==> tikz/vis_localize/vis_loc_test2.tex <==
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.277914524078369 0.37576961517334
		-0.275003910064697 0.383870601654053
		-0.272418022155762 0.391505479812622
		-0.269741058349609 0.397460222244263
		-0.268119812011719 0.402816295623779
		-0.268088817596436 0.406571388244629
		-0.268908977508545 0.408550262451172
		-0.270450115203857 0.41128396987915
		-0.269639492034912 0.412076950073242
		-0.266358375549316 0.411823034286499
		-0.261019706726074 0.409315586090088
		-0.254870414733887 0.403332471847534
		-0.249067783355713 0.394232749938965
		-0.243528366088867 0.385250568389893
		-0.239720821380615 0.374629497528076
		-0.237747669219971 0.361641645431519
		-0.23789644241333 0.347853183746338
		-0.242003440856934 0.317989349365234
		-0.24403715133667 0.302438259124756
		-0.244656562805176 0.287178754806519
		-0.243905544281006 0.273424386978149
		-0.24237060546875 0.258841514587402
		-0.240381240844727 0.243958711624146
		-0.238692760467529 0.228465795516968
		-0.240845203399658 0.212463140487671
		-0.246352195739746 0.19645094871521
		-0.253385543823242 0.181475162506104
		-0.260647296905518 0.167635917663574
		-0.267127990722656 0.155939817428589
		-0.274684906005859 0.145185947418213
		-0.284087657928467 0.134624242782593
		-0.294699192047119 0.125189304351807
		-0.304877758026123 0.116819620132446
		-0.313113451004028 0.10960578918457
		-0.324866771697998 0.0992677211761475
		-0.328107357025146 0.0955734252929688
		-0.328493356704712 0.091015100479126
		-0.327972888946533 0.08821702003479
		-0.324159860610962 0.0864124298095703
		-0.317668676376343 0.0852720737457275
		-0.312024831771851 0.0857589244842529
		-0.307485580444336 0.087864875793457
		-0.302732229232788 0.0923888683319092
		-0.297929048538208 0.0999257564544678
		-0.293583393096924 0.109835863113403
		-0.287972450256348 0.120825529098511
		-0.285051345825195 0.131354093551636
		-0.283878326416016 0.141290664672852
		-0.284676074981689 0.149950981140137
		-0.288012981414795 0.157615184783936
		-0.292778968811035 0.164697408676147
		-0.300677299499512 0.179323673248291
		-0.301599979400635 0.187467813491821
		-0.301223278045654 0.197311878204346
		-0.29999828338623 0.205654144287109
		-0.297425746917725 0.211897373199463
		-0.293235301971436 0.217428684234619
		-0.287758350372314 0.223261594772339
		-0.281335830688477 0.227783679962158
		-0.274884700775146 0.230390310287476
		-0.268847465515137 0.230886936187744
		-0.263436317443848 0.230480194091797
		-0.258731365203857 0.229634523391724
		-0.255252361297607 0.22833776473999
		-0.253783702850342 0.225872039794922
		-0.254422187805176 0.222661018371582
		-0.25548267364502 0.217538356781006
		-0.256691932678223 0.211211919784546
		-0.239583492279053 0.333274126052856
		-0.319681644439697 0.103725671768188
		-0.297602891921997 0.171787023544312
		-0.257651805877686 0.205974817276001
		-0.206652164459229 0.166876554489136
		-0.371412038803101 0.0903289318084717
		-0.557304382324219 -0.135668516159058
		-0.210906982421875 -0.178790330886841
		-0.0921769142150879 -0.136728286743164
		-0.160892486572266 -0.0503261089324951
		0.059298038482666 0.0288634300231934
		0.16557502746582 -0.0846967697143555
		0.175269603729248 0.188712596893311
		0.184167385101318 0.243378162384033
		-0.238722324371338 0.736347198486328
		-0.829214572906494 0.540878057479858
		-0.258226871490479 0.20183801651001
		-0.257194995880127 0.199072599411011
		-0.2552490234375 0.197506189346313
		-0.251174449920654 0.19727611541748
		-0.24581241607666 0.197332859039307
		-0.239382266998291 0.196525812149048
		-0.232236862182617 0.196452379226685
		-0.2236008644104 0.196725606918335
		-0.214978694915771 0.195934772491455
		-0.207677364349365 0.195921659469604
		-0.200846195220947 0.195970058441162
		-0.195359706878662 0.193498611450195
		-0.194808006286621 0.189937353134155
		-0.196717262268066 0.185196161270142
		-0.199209690093994 0.18011474609375
		-0.201838970184326 0.174916744232178
		-0.204516410827637 0.170616626739502
		-0.2087082862854 0.163940668106079
		-0.210518360137939 0.161308288574219
		-0.212458610534668 0.159175634384155
		-0.215489387512207 0.157284021377563
		-0.21760368347168 0.155131340026855
		-0.223363399505615 0.152605056762695
		-0.229154109954834 0.149023056030273
		-0.237037658691406 0.144118785858154
		-0.247348308563232 0.138494729995728
		-0.257808685302734 0.13278341293335
		-0.269469738006592 0.127597808837891
		-0.280875682830811 0.121505260467529
		-0.292534828186035 0.115068674087524
		-0.319334030151367 0.103604316711426
		-0.333157777786255 0.0983812808990479
		-0.346196174621582 0.0942003726959229
		-0.357970952987671 0.0920331478118896
		-0.3840651512146 0.0905218124389648
		-0.653720855712891 0.122089147567749
		-0.660309076309204 0.105922937393188
		-0.661712884902954 0.0939831733703613
		-0.662400960922241 0.0808448791503906
		-0.661723136901855 0.0660829544067383
		-0.659815311431885 0.0512900352478027
		-0.656718254089355 0.0360820293426514
		-0.652273893356323 0.0210030078887939
		-0.646893978118896 0.004608154296875
		-0.639547109603882 -0.0111711025238037
		-0.630634784698486 -0.0272922515869141
		-0.619833707809448 -0.0448372364044189
		-0.607984781265259 -0.0623006820678711
		-0.595757722854614 -0.0805659294128418
		-0.583165407180786 -0.0995349884033203
		-0.570398330688477 -0.117632865905762
		-0.544569730758667 -0.154345512390137
		-0.532211065292358 -0.171351671218872
		-0.519806385040283 -0.186150312423706
		-0.507245063781738 -0.199429988861084
		-0.494518518447876 -0.210120439529419
		-0.48113489151001 -0.219118118286133
		-0.46743106842041 -0.226036310195923
		-0.454319953918457 -0.231195688247681
		-0.441144943237305 -0.234488725662231
		-0.429921865463257 -0.235854148864746
		-0.419054269790649 -0.235508918762207
		-0.408848285675049 -0.233731269836426
		-0.399264812469482 -0.230101585388184
		-0.389774799346924 -0.224617004394531
		-0.380947113037109 -0.217540502548218
		-0.372190237045288 -0.210256099700928
		-0.363263130187988 -0.201272964477539
		-0.193362712860107 -0.183841705322266
		-0.175598621368408 -0.189611673355103
		-0.15818452835083 -0.194370746612549
		-0.140665531158447 -0.195991992950439
		-0.124410152435303 -0.195259094238281
		-0.111173629760742 -0.192239284515381
		-0.101307392120361 -0.187330722808838
		-0.0941042900085449 -0.180757522583008
		-0.0888214111328125 -0.174097061157227
		-0.0854001045227051 -0.169026613235474
		-0.0830097198486328 -0.165572166442871
		-0.0816245079040527 -0.163728713989258
		-0.0798959732055664 -0.160662651062012
		-0.0802512168884277 -0.158412218093872
		-0.0814166069030762 -0.155252456665039
		-0.0833492279052734 -0.150414943695068
		-0.0872101783752441 -0.143878698348999
		-0.0972905158996582 -0.130398750305176
		-0.104498863220215 -0.125162839889526
		-0.112119674682617 -0.121433734893799
		-0.119813442230225 -0.119440793991089
		-0.127152442932129 -0.119353055953979
		-0.136002540588379 -0.119732141494751
		-0.143746376037598 -0.11943244934082
		-0.151008605957031 -0.118131160736084
		-0.157721042633057 -0.115354061126709
		-0.164333820343018 -0.111320972442627
		-0.170390605926514 -0.107547998428345
		-0.175509929656982 -0.10357403755188
		-0.178669452667236 -0.0987119674682617
		-0.180443286895752 -0.0930991172790527
		-0.180478096008301 -0.0856921672821045
		-0.178653240203857 -0.074988842010498
		-0.171958446502686 -0.0624861717224121
		-0.147720813751221 -0.0379667282104492
		-0.131465911865234 -0.0254018306732178
		-0.112082958221436 -0.0149457454681396
		-0.0917692184448242 -0.00606226921081543
		-0.0720953941345215 0.00130891799926758
		-0.0516562461853027 0.00694847106933594
		-0.0320119857788086 0.0110390186309814
		-0.0162792205810547 0.0144340991973877
		-0.00368881225585938 0.0177743434906006
		0.00761604309082031 0.0215628147125244
		0.0164546966552734 0.0251398086547852
		0.0239143371582031 0.0280828475952148
		0.0297698974609375 0.0312995910644531
		0.0342602729797363 0.034841775894165
		0.0396184921264648 0.0365960597991943
		0.0451154708862305 0.0361268520355225
		0.0516629219055176 0.0337152481079102
		0.0685520172119141 0.021864652633667
		0.0777206420898438 0.0129024982452393
		0.0862774848937988 0.00221443176269531
		0.0941362380981445 -0.00983238220214844
		0.100553512573242 -0.023557186126709
		0.105515003204346 -0.0388224124908447
		0.119484424591064 -0.135337352752686
		0.119211673736572 -0.143948554992676
		0.11967658996582 -0.151436805725098
		0.120658874511719 -0.157727479934692
		0.122608661651611 -0.160672903060913
		0.128272533416748 -0.159711599349976
		0.137197971343994 -0.156004905700684
		0.146774768829346 -0.149021148681641
		0.154118061065674 -0.138189554214478
		0.158998489379883 -0.123924732208252
		0.162104606628418 -0.106740474700928
		0.169551849365234 -0.0597004890441895
		0.17559814453125 -0.032642126083374
		0.182393550872803 -0.00373101234436035
		0.18871545791626 0.0244650840759277
		0.192722320556641 0.051316499710083
		0.193624496459961 0.077904224395752
		0.190389156341553 0.103258371353149
		0.179197788238525 0.148152589797974
		0.17380428314209 0.165935754776001
		0.169169425964355 0.179272174835205
		0.165753841400146 0.188929796218872
		0.163675785064697 0.19502067565918
		0.163528442382812 0.197766542434692
		0.165907859802246 0.198530912399292
		0.168379306793213 0.198062658309937
		0.171702861785889 0.194896697998047
		0.179773807525635 0.178441762924194
		0.183918476104736 0.166247844696045
		0.188649654388428 0.154552459716797
		0.193849563598633 0.141823053359985
		0.199704170227051 0.130581855773926
		0.205791473388672 0.120835304260254
		0.211556911468506 0.112207174301147
		0.215682506561279 0.106435537338257
		0.218117713928223 0.103313446044922
		0.218762874603271 0.102531909942627
		0.217483520507812 0.104357004165649
		0.214463710784912 0.108741998672485
		0.211386680603027 0.116566896438599
		0.208274841308594 0.128542423248291
		0.204588890075684 0.143620729446411
		0.200422763824463 0.163046360015869
		0.195801258087158 0.186198234558105
		0.178347587585449 0.274945974349976
		0.172471523284912 0.307852506637573
		0.0935778617858887 0.546064853668213
		0.0672755241394043 0.589858293533325
		0.0205011367797852 0.648478269577026
		0.00334405899047852 0.664420604705811
		-0.0146799087524414 0.678916931152344
		-0.0337276458740234 0.691680908203125
		-0.0527706146240234 0.702938318252563
		-0.0722904205322266 0.711982488632202
		-0.0930442810058594 0.719688653945923
		-0.113120079040527 0.726245164871216
		-0.132591724395752 0.73127293586731
		-0.151701927185059 0.734002113342285
		-0.172614574432373 0.734124898910522
		-0.19407320022583 0.734280347824097
		-0.216377258300781 0.735438823699951
		-0.261757850646973 0.737592220306396
		-0.285468578338623 0.739028215408325
		-0.310055255889893 0.740287065505981
		-0.336030960083008 0.741265773773193
		-0.36329197883606 0.742215394973755
		-0.391516923904419 0.743377447128296
		-0.419842481613159 0.744337320327759
		-0.44843578338623 0.744883298873901
		-0.476608514785767 0.744913578033447
		-0.505202293395996 0.743869304656982
		-0.532613277435303 0.74199652671814
		-0.560230493545532 0.739052534103394
		-0.636612415313721 0.724489688873291
		-0.68250298500061 0.708279609680176
		-0.792516469955444 0.612484693527222
		-0.804166793823242 0.596734046936035
		-0.821702480316162 0.559808254241943
		-0.834537506103516 0.522169351577759
		-0.839225292205811 0.503816604614258
		-0.840465307235718 0.485356330871582
		-0.842437505722046 0.464529275894165
		-0.844769716262817 0.443967342376709
		-0.849592924118042 0.388089418411255
		-0.853005170822144 0.3720543384552
		-0.856921911239624 0.355724334716797
		-0.860949993133545 0.341529369354248
		-0.959759712219238 0.098212718963623
		-0.976112842559814 0.0762295722961426
		-0.995194435119629 0.0539009571075439
		-1.01456260681152 0.0312232971191406
		-1.03385734558105 0.00915431976318359
		-1.05229759216309 -0.0121970176696777
		-1.0698401927948 -0.0328161716461182
		-1.08634901046753 -0.0538730621337891
		-1.13564085960388 -0.116577386856079
		-1.15089416503906 -0.136196851730347
		-1.16647338867188 -0.155740261077881
		-1.18189358711243 -0.17614221572876
		-1.19667649269104 -0.19782543182373
		-1.21087050437927 -0.220606803894043
		-1.2253429889679 -0.244003772735596
		-1.23993897438049 -0.267295122146606
		-1.25464391708374 -0.290359258651733
		-1.26926517486572 -0.313201904296875
		-1.28489875793457 -0.335656642913818
		-1.3002724647522 -0.357386350631714
		-1.3153920173645 -0.378275632858276
		-1.32886576652527 -0.399214267730713
		-1.3410964012146 -0.420318365097046
		-1.35255312919617 -0.442689657211304
		-1.36331939697266 -0.46506929397583
		-1.37888622283936 -0.507885932922363
		-1.38419413566589 -0.529788970947266
		-1.38769173622131 -0.553345203399658
		-1.39020609855652 -0.577341079711914
		-1.39093732833862 -0.602697968482971
		-1.38925623893738 -0.629052519798279
		-1.38465738296509 -0.655265927314758
		-1.37682580947876 -0.680898904800415
		-1.36653900146484 -0.705985069274902
		-1.35421657562256 -0.731403470039368
		-1.34038138389587 -0.758641242980957
		-1.32600212097168 -0.786984086036682
		-1.31065845489502 -0.815557599067688
		-1.2955470085144 -0.842177987098694
		-1.28171491622925 -0.866486549377441
		-1.26860356330872 -0.888938784599304
		-1.25459098815918 -0.910164833068848
		-1.23104214668274 -0.948655843734741
		-1.22055172920227 -0.966433167457581
		-1.21230983734131 -0.984264254570007
		-1.20609641075134 -1.00171661376953
		-1.20203185081482 -1.01882719993591
		-1.20044922828674 -1.0353969335556
		-1.19986176490784 -1.05091631412506
		-1.20200276374817 -1.06502676010132
		-1.20534944534302 -1.07807993888855
		-1.21091437339783 -1.09149968624115
		-1.2164831161499 -1.10493040084839
		-1.22399115562439 -1.11788094043732
		-1.23337912559509 -1.13042843341827
		-1.24283456802368 -1.14356100559235
		-1.25318264961243 -1.15486812591553
		-1.26245284080505 -1.16491687297821
		-1.27148461341858 -1.17476856708527
		-1.28880786895752 -1.19087469577789
		-1.29584193229675 -1.19942963123322
		-1.30305528640747 -1.20824337005615
		-1.31002974510193 -1.21720016002655
		-1.31695866584778 -1.22634041309357
		-1.32298111915588 -1.23403477668762
		-1.32748532295227 -1.24101293087006
		-1.32999658584595 -1.24770951271057
		-1.33158731460571 -1.25439536571503
		-1.33261179924011 -1.26010227203369
		-1.33137106895447 -1.26393151283264
		-1.32727575302124 -1.26638507843018
		-1.32040667533875 -1.26829326152802
		-1.3118097782135 -1.26973640918732
		-1.30072379112244 -1.27102971076965
		-1.28782987594604 -1.27334201335907
		-1.27450489997864 -1.27544581890106
		-1.24412441253662 -1.28058695793152
		-1.22928094863892 -1.28535652160645
		-1.19634604454041 -1.30898594856262
		-1.18969464302063 -1.31790268421173
		-1.18280935287476 -1.32739007472992
		-1.17535281181335 -1.3368763923645
		-1.16632890701294 -1.34616529941559
		-1.15656876564026 -1.35667419433594
		-1.14568638801575 -1.36973750591278
		-1.13331818580627 -1.38521218299866
		-1.12137508392334 -1.40149116516113
		-1.10954689979553 -1.41754627227783
		-1.09809541702271 -1.4339234828949
		-1.08424425125122 -1.45127058029175
		-1.06870937347412 -1.46602237224579
		-1.05100512504578 -1.47866702079773
		-1.03069663047791 -1.49105226993561
		-0.991294145584106 -1.51178133487701
		-0.973514556884766 -1.5204097032547
		-0.957077980041504 -1.52730321884155
		-0.940063714981079 -1.53273713588715
		-0.922473669052124 -1.53867518901825
		-0.90374493598938 -1.54427242279053
		-0.882858991622925 -1.54902696609497
		-0.858505487442017 -1.55346584320068
		-0.832416534423828 -1.5564444065094
		-0.80485987663269 -1.55800187587738
		-0.776254415512085 -1.55651497840881
		-0.749781131744385 -1.55240893363953
		-0.724327564239502 -1.54573655128479
		-0.697410106658936 -1.53377556800842
		-0.670466423034668 -1.51742672920227
		-0.643152952194214 -1.49942266941071
		-0.615800619125366 -1.48087620735168
		-0.559094905853271 -1.45412802696228
		-0.530939817428589 -1.44421637058258
		-0.503242254257202 -1.43826186656952
		-0.475287675857544 -1.43487083911896
		-0.445384979248047 -1.43234968185425
		-0.414664506912231 -1.43130505084991
		-0.380980253219604 -1.43091654777527
		-0.34503960609436 -1.43041431903839
		-0.306323289871216 -1.43204283714294
		-0.265529155731201 -1.4360214471817
		-0.224159717559814 -1.44131410121918
		-0.18022632598877 -1.44923877716064
		-0.134766578674316 -1.46014213562012
		-0.088036060333252 -1.47164249420166
		-0.0408263206481934 -1.48118901252747
		0.00507164001464844 -1.48982346057892
		0.0479178428649902 -1.49840617179871
		0.122891902923584 -1.50791537761688
		0.154507637023926 -1.50823068618774
		0.183198928833008 -1.50381076335907
		0.212789058685303 -1.49751472473145
		0.242511749267578 -1.48964643478394
		0.271658420562744 -1.48006653785706
		0.299930095672607 -1.46876990795135
		0.327905654907227 -1.45456612110138
		0.356565475463867 -1.43830156326294
		0.386484622955322 -1.41835367679596
		0.4178786277771 -1.39543557167053
		0.448380947113037 -1.36618864536285
		0.47688102722168 -1.33285450935364
		0.502026557922363 -1.29849565029144
		0.522701740264893 -1.26771581172943
		0.543740749359131 -1.24280595779419
		0.568014144897461 -1.22191202640533
		0.654234409332275 -1.17278146743774
		0.684342384338379 -1.15968525409698
		0.715023994445801 -1.14655101299286
		0.745688438415527 -1.13348603248596
		0.77711820602417 -1.12046718597412
		0.809403896331787 -1.10714292526245
		0.912381649017334 -1.06198215484619
		0.945664882659912 -1.04664981365204
		0.97785472869873 -1.03156614303589
		1.00692796707153 -1.01718664169312
		1.03428268432617 -1.00237238407135
		1.05913066864014 -0.987793326377869
		1.08167600631714 -0.971924066543579
		1.12275218963623 -0.935084700584412
		1.13949060440063 -0.91492772102356
		1.15115308761597 -0.89346182346344
		1.15871667861938 -0.869437217712402
		1.16582870483398 -0.813834309577942
		1.16874980926514 -0.783994317054749
		1.17134523391724 -0.751709938049316
		1.17438888549805 -0.719144105911255
		1.17780828475952 -0.684641718864441
		1.18082475662231 -0.648595213890076
		1.18368768692017 -0.612017512321472
		1.18810749053955 -0.57654881477356
		1.19367980957031 -0.541130542755127
		1.20135688781738 -0.507436990737915
		1.20950174331665 -0.475247859954834
		1.21814060211182 -0.443670272827148
		1.22750473022461 -0.412110328674316
		1.23639488220215 -0.381109476089478
		1.24492406845093 -0.349420547485352
		1.25454950332642 -0.316314220428467
		1.26497268676758 -0.282555103302002
		1.28720283508301 -0.212386131286621
		1.30069351196289 -0.175601482391357
		1.31554365158081 -0.138458013534546
		1.33101224899292 -0.1009361743927
		1.34755802154541 -0.0637838840484619
		1.3643012046814 -0.0268731117248535
		1.38192987442017 0.0103340148925781
		1.39972543716431 0.0486652851104736
		1.41519832611084 0.0898284912109375
		1.42902851104736 0.132864952087402
		1.44179391860962 0.175543546676636
		1.45395994186401 0.217343807220459
		1.46535778045654 0.256792545318604
		1.47516632080078 0.294201374053955
		1.48489665985107 0.329734563827515
		1.49441194534302 0.363883972167969
		1.50235223770142 0.39800763130188
		1.50231695175171 0.467626571655273
		1.49481344223022 0.502772808074951
		1.48128795623779 0.534126758575439
		1.46524572372437 0.559112310409546
		1.44973707199097 0.579289674758911
		1.43465995788574 0.597668647766113
		1.42244720458984 0.617652177810669
		1.39642190933228 0.65005350112915
		1.38611602783203 0.668458700180054
		1.37587833404541 0.690285205841064
		1.36545658111572 0.71431303024292
		1.35394096374512 0.740032196044922
		1.33936738967896 0.766297817230225
		1.32135486602783 0.792999505996704
		1.30053281784058 0.821116209030151
		1.28037548065186 0.84899377822876
		1.25910186767578 0.87829065322876
		1.21517705917358 0.941576719284058
		1.19360113143921 0.975414037704468
		1.17272520065308 1.01133465766907
		1.15340328216553 1.04729461669922
		1.1349515914917 1.08275628089905
		1.11720180511475 1.11680483818054
		1.08483028411865 1.17734718322754
		1.05749034881592 1.22486114501953
		0.528740406036377 1.91563510894775
		0.51542854309082 1.91631698608398
		0.502882480621338 1.91355156898499
		0.489019870758057 1.90758609771729
		0.473927021026611 1.90118026733398
		0.457008838653564 1.89413452148438
		0.439070224761963 1.8857729434967
		0.419692516326904 1.87804365158081
		0.398584365844727 1.87060499191284
		0.349525928497314 1.85674142837524
		0.321820259094238 1.85089731216431
		0.292811870574951 1.84480810165405
		0.26231861114502 1.83815860748291
		0.229444980621338 1.83162569999695
		0.194689273834229 1.82503867149353
		0.160228252410889 1.81991958618164
		0.123721599578857 1.81374335289001
		0.0878257751464844 1.80928683280945
		0.049893856048584 1.80878043174744
		0.0121016502380371 1.80827927589417
		-0.0252418518066406 1.80832123756409
		-0.101132869720459 1.80575013160706
		-0.142006874084473 1.79925560951233
		-0.223679542541504 1.7917697429657
		-0.290345668792725 1.7945864200592
		-0.319445610046387 1.79653334617615
		-0.347094058990479 1.79809546470642
		-0.374986171722412 1.79798603057861
		-0.40419602394104 1.79685258865356
		-0.433620452880859 1.7970175743103
		-0.525775194168091 1.79891443252563
		-0.55772852897644 1.80132818222046
		-0.591510772705078 1.80414056777954
		-0.900150060653687 1.839688539505
		-0.937129497528076 1.84108448028564
		-1.07900595664978 1.82312941551208
		-1.11122822761536 1.81740593910217
		-1.14063858985901 1.81169486045837
		-1.16588258743286 1.80447292327881
		-1.18993663787842 1.79462122917175
		-1.21050190925598 1.77912783622742
		-1.22786855697632 1.75869035720825
		-1.24272084236145 1.7332284450531
		-1.26655101776123 1.66898131370544
		-1.40675258636475 0.537503242492676
		-1.43966126441956 0.49646258354187
		-1.55778932571411 0.251029968261719
		-1.55964779853821 0.201986074447632
		-1.55779314041138 0.185920238494873
		-1.55395078659058 0.168371200561523
		-1.54841136932373 0.148701906204224
		-1.54278349876404 0.12739372253418
		-1.53607654571533 0.104254961013794
		-1.52958703041077 0.0809292793273926
		-1.52165460586548 0.0560834407806396
		-1.51535797119141 0.0302271842956543
		-1.50942587852478 0.0035548210144043
		-1.50150656700134 -0.0248394012451172
		-1.49441194534302 -0.0540707111358643
		-1.48724555969238 -0.0851426124572754
		-1.47872114181519 -0.119713306427002
		-1.46974778175354 -0.155831575393677
		-1.46372127532959 -0.190316200256348
		-1.45802640914917 -0.224709272384644
		-1.44298553466797 -0.292988300323486
		-1.43528866767883 -0.324957370758057
		-1.42665457725525 -0.358205080032349
		-1.41690230369568 -0.391166687011719
		-1.40685033798218 -0.425074100494385
		-1.3973753452301 -0.459175109863281
		-1.38502311706543 -0.492364168167114
		-1.37361288070679 -0.525559902191162
		-1.36103081703186 -0.557466268539429
		-1.34667086601257 -0.588262557983398
		-1.33012676239014 -0.618058919906616
		-1.3117663860321 -0.646023988723755
		-1.29246163368225 -0.67235791683197
		-1.23346662521362 -0.738878488540649
		-1.06192898750305 -0.854790687561035
		-1.0336377620697 -0.865420699119568
		-1.00445556640625 -0.876057386398315
		-1.37216734886169 -0.486552000045776
		-1.24150276184082 -0.930006623268127
		-1.2807469367981 -1.18326127529144
		-1.25989508628845 -1.27779948711395
		-1.01067900657654 -1.50222682952881
		-0.587999105453491 -1.46570384502411
		0.0874972343444824 -1.50444412231445
		0.595983505249023 -1.20341205596924
		1.16288661956787 -0.842788457870483
		1.27562856674194 -0.248093366622925
		1.50463008880615 0.43229079246521
		1.23722648620605 0.909407615661621
		0.374695301055908 1.86231756210327
		-0.259115219116211 1.79247093200684
		-0.861749410629272 1.8355073928833
		-1.55976057052612 0.216567277908325
		-0.946091413497925 -0.89824903011322
		-0.915157556533813 -0.911146283149719
		-0.882835865020752 -0.925284504890442
		-0.850311279296875 -0.9401615858078
		-0.817657709121704 -0.953638434410095
		-0.785905838012695 -0.966215491294861
		-0.754548788070679 -0.978294491767883
		-0.722214937210083 -0.989241719245911
		-0.688797235488892 -0.999572277069092
		-0.654980897903442 -1.00880968570709
		-0.621203422546387 -1.01825392246246
		-0.586158752441406 -1.02760255336761
		-0.550389766693115 -1.03688955307007
		-0.515504598617554 -1.04598820209503
		-0.479119062423706 -1.05159211158752
		-0.441410541534424 -1.05802917480469
		-0.403317928314209 -1.06441593170166
		-0.325944900512695 -1.0682886838913
		-0.289548873901367 -1.06584870815277
		-0.252859115600586 -1.06319272518158
		-0.218037605285645 -1.05885863304138
		-0.183183670043945 -1.05375266075134
		-0.149319171905518 -1.04818940162659
		-0.115955352783203 -1.04223024845123
		-0.0824103355407715 -1.03476870059967
		0.0155863761901855 -1.00527346134186
		0.0494132041931152 -0.994248747825623
		0.113173484802246 -0.968424677848816
		0.147118091583252 -0.956148386001587
		0.181666374206543 -0.94139564037323
		0.257551193237305 -0.909263968467712
		0.336706161499023 -0.876733660697937
		0.374966144561768 -0.861131548881531
		0.450223445892334 -0.831574201583862
		0.52379846572876 -0.801509618759155
		0.56041145324707 -0.785947442054749
		0.597454071044922 -0.76990818977356
		0.633895874023438 -0.753046870231628
		0.667784214019775 -0.734333395957947
		0.701338291168213 -0.714678883552551
		0.734431743621826 -0.694161415100098
		0.794093132019043 -0.648275017738342
		0.819271087646484 -0.623937726020813
		0.842351913452148 -0.597761511802673
		0.885119438171387 -0.548850536346436
		0.90026330947876 -0.5174241065979
		0.915440559387207 -0.489379167556763
		0.931074142456055 -0.460411548614502
		0.947207927703857 -0.430480003356934
		0.962234497070312 -0.397973775863647
		0.976572036743164 -0.364188432693481
		1.00037384033203 -0.294807434082031
		1.00885200500488 -0.254948854446411
		1.02026891708374 -0.214493036270142
		1.03311967849731 -0.176049470901489
		1.04370880126953 -0.138928174972534
		1.05272483825684 -0.102901697158813
		1.06020212173462 -0.0676677227020264
		1.06757116317749 -0.0335381031036377
		1.07419729232788 -0.000307798385620117
		1.08037281036377 0.0325901508331299
		1.08630132675171 0.0653808116912842
		1.09106206893921 0.0985817909240723
		1.09518194198608 0.131725072860718
		1.09985399246216 0.164562940597534
		1.10464382171631 0.197460412979126
		1.10961723327637 0.231368064880371
		1.11518955230713 0.26603627204895
		1.12343978881836 0.33359956741333
		1.12605762481689 0.366553068161011
		1.1283860206604 0.398186206817627
		1.12991523742676 0.431136846542358
		1.12882947921753 0.464421987533569
		1.12469577789307 0.49727463722229
		1.1186408996582 0.531249284744263
		1.11113262176514 0.564232587814331
		1.08277702331543 0.662462711334229
		1.07160091400146 0.695167303085327
		1.05993318557739 0.727816820144653
		1.04696416854858 0.760651588439941
		1.03266286849976 0.794032573699951
		1.01828527450562 0.827357769012451
		1.00089120864868 0.860113859176636
		0.980503082275391 0.894352674484253
		0.962986469268799 0.932048320770264
		0.929332256317139 1.00558090209961
		0.911039352416992 1.04221034049988
		0.892141819000244 1.08007597923279
		0.87217903137207 1.11903786659241
		0.836321830749512 1.19770646095276
		0.819808006286621 1.23536968231201
		-0.19622278213501 2.21395540237427
		-0.245086193084717 2.25039291381836
		-0.298720836639404 2.28726553916931
		-0.323575973510742 2.30481767654419
		-0.348572731018066 2.31834173202515
		-0.37579083442688 2.33057022094727
		-0.403821468353271 2.34224796295166
		-0.43004584312439 2.35452055931091
		-0.455840587615967 2.36588549613953
		-0.482459783554077 2.374760389328
		-0.586022853851318 2.40370631217957
		-0.611324787139893 2.40876054763794
		-0.636898517608643 2.41281032562256
		-0.663195133209229 2.41615533828735
		-0.743485927581787 2.42023181915283
		-0.772223949432373 2.42032670974731
		-0.79814076423645 2.42031288146973
		-0.869981527328491 2.42138504981995
		-1.18130660057068 2.43603706359863
		-1.20832514762878 2.44093346595764
		-1.23492765426636 2.4461932182312
		-1.26258540153503 2.45069766044617
		-1.28962206840515 2.45404887199402
		-1.34763288497925 2.45958685874939
		-1.37810206413269 2.46197724342346
		-1.43655300140381 2.4667592048645
		-1.51706147193909 2.46916556358337
		-1.54356670379639 2.46840763092041
		-1.57075142860413 2.46631765365601
		-1.5935230255127 2.46411490440369
		-1.64481210708618 2.45433115959167
		-1.69349145889282 2.44154191017151
		-1.71746516227722 2.4342303276062
		-1.76557040214539 2.41493272781372
		-1.79027581214905 2.40445184707642
		-1.81456160545349 2.39344477653503
		-1.8638162612915 2.36880898475647
		-1.91582250595093 2.3420672416687
		-1.94060826301575 2.32855153083801
		-1.96470475196838 2.31561851501465
		-2.01434016227722 2.29337191581726
		-2.04267382621765 2.28207278251648
		-2.07255434989929 2.2702693939209
		-2.10154128074646 2.25684332847595
		-2.16000866889954 2.23435211181641
		-2.19005465507507 2.22346138954163
		-2.21913862228394 2.21281933784485
		-2.24973273277283 2.20081210136414
		-2.28025841712952 2.18779492378235
		-2.31153643131256 2.17330002784729
		-2.34236299991608 2.15848469734192
		-2.3728449344635 2.14324069023132
		-2.40420162677765 2.12779903411865
		-2.43527221679688 2.11227250099182
		-2.46779572963715 2.09672427177429
		-2.50001692771912 2.07930207252502
		-2.52909731864929 2.06237769126892
		-2.56081962585449 2.04297494888306
		-2.58007264137268 2.02870869636536
		-2.60489082336426 2.01245951652527
		-2.62624967098236 1.99557447433472
		-2.66845166683197 1.96328783035278
		-2.69007778167725 1.94784474372864
		-2.70973861217499 1.92958474159241
		-2.72706830501556 1.90924739837646
		-2.74645042419434 1.88882327079773
		-2.76571977138519 1.86789870262146
		-2.78511047363281 1.84576153755188
		-2.80226218700409 1.82297968864441
		-2.81975698471069 1.80046057701111
		-2.83569228649139 1.7772216796875
		-2.85137045383453 1.75414323806763
		-2.86745131015778 1.73142266273499
		-2.88402533531189 1.70848727226257
		-2.90316617488861 1.68381500244141
		-2.93954348564148 1.62911558151245
		-2.95482218265533 1.6055805683136
		-2.96929132938385 1.58214282989502
		-3.01746606826782 1.51112079620361
		-3.04770684242249 1.46228671073914
		-3.08977890014648 1.38582134246826
		-3.10692059993744 1.36194014549255
		-3.12267112731934 1.33557939529419
		-3.13768661022186 1.30612730979919
		-3.15393471717834 1.27996754646301
		-3.16954720020294 1.25746083259583
		-3.1866180896759 1.2291202545166
		-3.20351207256317 1.20076036453247
		-3.22286367416382 1.16645860671997
		-3.24296236038208 1.13527202606201
		-3.26244604587555 1.10291242599487
		-3.28082573413849 1.07018446922302
		-3.29840010404587 1.03819346427917
		-3.31600266695023 1.00741124153137
		-3.33290755748749 0.974907875061035
		-3.36407256126404 0.909197568893433
		-3.37753063440323 0.876497983932495
		-3.38923466205597 0.843777418136597
		-3.39805424213409 0.812927961349487
		-3.40553867816925 0.783468961715698
		-3.41281032562256 0.75489068031311
		-3.41870957612991 0.726044178009033
		-3.42411309480667 0.697449207305908
		-3.42851662635803 0.669065237045288
		-3.43172472715378 0.64022970199585
		-3.43387365341187 0.611833572387695
		-3.4347397685051 0.584101676940918
		-3.43474948406219 0.55721116065979
		-3.43705636262894 0.526839733123779
		-3.43822127580643 0.494496822357178
		-3.43669700622559 0.464603185653687
		-3.43456965684891 0.437551259994507
		-3.4365422129631 0.378763675689697
		-3.43850862979889 0.347556114196777
		-3.44080090522766 0.316732406616211
		-3.4431928396225 0.28593897819519
		-3.44576424360275 0.254672765731812
		-3.44867873191833 0.223515748977661
		-3.45177316665649 0.191696882247925
		-3.45506072044373 0.158743381500244
		-3.45843720436096 0.125012159347534
		-3.46184128522873 0.0903043746948242
		-3.46523356437683 0.0554585456848145
		-3.46891444921494 0.0203306674957275
		-3.47204500436783 -0.0142276287078857
		-3.47590863704681 -0.0513079166412354
		-3.48035907745361 -0.0919811725616455
		-3.48161977529526 -0.131496667861938
		-3.47998875379562 -0.167396068572998
		-3.47447103261948 -0.232375144958496
		-3.47097247838974 -0.266051054000854
		-3.46644574403763 -0.300634145736694
		-3.46005737781525 -0.335422515869141
		-3.45198160409927 -0.370165109634399
		-3.44315522909164 -0.403755187988281
		-3.43409538269043 -0.436044454574585
		-3.42380207777023 -0.468412399291992
		-3.41268748044968 -0.499844551086426
		-3.39996689558029 -0.531293630599976
		-3.38667809963226 -0.563340187072754
		-3.37213838100433 -0.595449209213257
		-3.3571150302887 -0.624057531356812
		-3.34141790866852 -0.655001521110535
		-3.32591128349304 -0.684772729873657
		-3.30999851226807 -0.714697599411011
		-3.29375028610229 -0.739475607872009
		-3.26734232902527 -0.793045878410339
		-3.25367712974548 -0.825435519218445
		-3.23846209049225 -0.858538269996643
		-3.22436416149139 -0.890941858291626
		-3.2081446647644 -0.921290040016174
		-3.19458866119385 -0.95218551158905
		-3.18197989463806 -0.981675028800964
		-3.1555095911026 -1.04789161682129
		-3.14140379428864 -1.0800369977951
		-3.12641704082489 -1.11200940608978
		-3.07994282245636 -1.21052157878876
		-3.06021237373352 -1.24648082256317
		-3.04210436344147 -1.2834974527359
		-3.0218677520752 -1.31712675094604
		-2.99921452999115 -1.34790289402008
		-2.98140048980713 -1.37562072277069
		-2.96089434623718 -1.40102970600128
		-2.92002356052399 -1.45283246040344
		-2.89824247360229 -1.47874450683594
		-2.87606871128082 -1.50250637531281
		-2.8540472984314 -1.52476322650909
		-2.83277606964111 -1.54580450057983
		-2.81288230419159 -1.56750559806824
		-2.79378771781921 -1.58811640739441
		-2.77279210090637 -1.6082655787468
		-2.75166809558868 -1.62852078676224
		-2.73029482364655 -1.64835947751999
		-2.70780324935913 -1.66747826337814
		-2.68532693386078 -1.68583190441132
		-2.66274321079254 -1.70417594909668
		-2.63932800292969 -1.72032761573792
		-2.61450231075287 -1.73668175935745
		-2.58833754062653 -1.75246214866638
		-2.5624463558197 -1.76836842298508
		-0.975684642791748 -0.887036442756653
		-0.364597797393799 -1.06823217868805
		0.487151145935059 -0.816159129142761
		0.990395069122314 -0.329739093780518
		1.12084293365479 0.300183534622192
		0.946936130523682 0.968765020370483
		-0.534674882888794 2.3906843662262
		-1.6696674823761 2.44844746589661
		-2.13061833381653 2.24508094787598
		-2.64767205715179 1.97992491722107
		-2.98519551753998 1.55870747566223
		-3.34964042901993 0.942638158798218
		-3.4352662563324 0.409169435501099
		-3.47730922698975 -0.199971437454224
		-3.2802894115448 -0.764190912246704
		-2.51207566261292 -1.80423372983932
		-2.48632049560547 -1.82282418012619
		-2.46090924739838 -1.84052866697311
		-2.43648338317871 -1.85851234197617
		-2.41108787059784 -1.8779177069664
		-2.38436162471771 -1.89774787425995
		-2.35717475414276 -1.91746389865875
		-2.32966458797455 -1.93739664554596
		-2.3021252155304 -1.95721411705017
		-2.27432918548584 -1.97682863473892
		-2.24727916717529 -1.99696213006973
		-2.21946430206299 -2.01819950342178
		-2.19074535369873 -2.03955644369125
		-2.16193175315857 -2.06055390834808
		-2.13326930999756 -2.08178159594536
		-2.10351181030273 -2.10329777002335
		-2.07304453849792 -2.12380704283714
		-2.01222109794617 -2.16086426377296
		-1.98179769515991 -2.17782863974571
		-1.95189118385315 -2.19379264116287
		-1.91934061050415 -2.2077913582325
		-1.88488388061523 -2.21998143196106
		-1.85232830047607 -2.23124080896378
		-1.81905007362366 -2.24262112379074
		-1.78585290908813 -2.25429055094719
		-1.75348091125488 -2.26436007022858
		-1.7219090461731 -2.27473020553589
		-1.69067859649658 -2.2856577038765
		-1.65851235389709 -2.29659301042557
		-1.62741780281067 -2.30790463089943
		-1.59532308578491 -2.31808462738991
		-1.56192827224731 -2.32759901881218
		-1.5307035446167 -2.33660908043385
		-1.49903964996338 -2.3452306240797
		-1.43395614624023 -2.36275553703308
		-1.40116095542908 -2.37282578647137
		-1.36871361732483 -2.38361778855324
		-1.33650732040405 -2.39460724592209
		-1.30498933792114 -2.40514203906059
		-1.27354454994202 -2.41554988920689
		-1.24164271354675 -2.42633675038815
		-1.2091121673584 -2.43785780668259
		-1.17605042457581 -2.45070205628872
		-1.14237093925476 -2.46494384855032
		-1.10799789428711 -2.47965826839209
		-1.07298946380615 -2.49460106343031
		-1.03805947303772 -2.50970257073641
		-1.00288391113281 -2.52451517432928
		-0.968321561813354 -2.5392544567585
		-0.934041023254395 -2.55409646034241
		-0.899856328964233 -2.56906268279999
		-0.831038951873779 -2.59923138655722
		-0.796434879302979 -2.61408297717571
		-0.762255907058716 -2.62897242233157
		-0.729492425918579 -2.6434365734458
		-0.697430610656738 -2.65697105228901
		-0.666011333465576 -2.66896580159664
		-0.634979009628296 -2.67931958287954
		-0.604560613632202 -2.68850005418062
		-0.573789834976196 -2.69741290062666
		-0.542621850967407 -2.70544614642859
		-0.510859251022339 -2.71284830570221
		-0.478491306304932 -2.72014281153679
		-0.44575023651123 -2.727165594697
		-0.412659645080566 -2.73416940867901
		-0.379308462142944 -2.74070928990841
		-0.345607042312622 -2.74586719274521
		-0.312563419342041 -2.7504168599844
		-0.247432231903076 -2.76044636964798
		-0.214572906494141 -2.76481848955154
		-0.181426048278809 -2.76992200314999
		-0.148313045501709 -2.77595688402653
		-0.114989757537842 -2.78425669670105
		-0.0811376571655273 -2.79290406405926
		-0.0463199615478516 -2.800441801548
		-0.0110702514648438 -2.8081551194191
		0.0246763229370117 -2.8158550709486
		0.0607204437255859 -2.82358965277672
		0.0965838432312012 -2.83131216466427
		0.132359981536865 -2.83908200263977
		0.167444705963135 -2.84731617569923
		0.201561450958252 -2.85530817508698
		0.235463619232178 -2.86441379785538
		0.269999504089355 -2.87413102388382
		0.305278778076172 -2.88393640518188
		2.84257936477661 -0.211014986038208
		2.81457376480103 0.1004638671875
		2.80242395401001 0.164047718048096
		2.79462814331055 0.194010257720947
		2.78849744796753 0.227062463760376
		2.78064775466919 0.261140823364258
		2.77213573455811 0.292715549468994
		2.76582431793213 0.323065042495728
		2.76252222061157 0.355920076370239
		2.76030778884888 0.391060590744019
		2.75761318206787 0.427187442779541
		2.75471591949463 0.463705062866211
		2.75282335281372 0.499924421310425
		2.75279951095581 0.53466796875
		2.75421094894409 0.568251609802246
		2.75710344314575 0.600548028945923
		2.76139783859253 0.632907152175903
		2.7691535949707 0.698196172714233
		2.77345609664917 0.730149030685425
		2.77825212478638 0.762642860412598
		2.78289699554443 0.795141696929932
		2.7872462272644 0.827340841293335
		2.79250001907349 0.862302541732788
		2.79651737213135 0.899001359939575
		2.79398393630981 0.932919502258301
		2.79329299926758 0.961551904678345
		2.79330682754517 0.9918372631073
		2.7917013168335 1.02166938781738
		2.78791618347168 1.05705571174622
		2.78377342224121 1.09026718139648
		2.77900409698486 1.1252965927124
		2.77413654327393 1.15618705749512
		2.76660633087158 1.18758606910706
		2.75907802581787 1.21927237510681
		2.74743461608887 1.28450584411621
		2.74508905410767 1.31772017478943
		2.74361801147461 1.35084986686707
		2.74074983596802 1.38421225547791
		2.73876333236694 1.41934394836426
		2.73577117919922 1.45767974853516
		2.7325325012207 1.49440145492554
		2.72874402999878 1.5285267829895
		2.72905254364014 1.56071615219116
		2.73110485076904 1.59634184837341
		2.73241901397705 1.63182282447815
		2.73240756988525 1.66754055023193
		2.73360776901245 1.7016613483429
		2.73538970947266 1.73603010177612
		2.73796033859253 1.76927804946899
		2.74071884155273 1.80415987968445
		2.74447727203369 1.83680701255798
		2.75367593765259 1.90217614173889
		2.75852251052856 1.93256068229675
		2.76459360122681 1.96355295181274
		2.77252006530762 1.99493789672852
		2.7822208404541 2.02751851081848
		2.79284524917603 2.06441164016724
		2.79865074157715 2.1008837223053
		2.8013391494751 2.13027358055115
		2.80482721328735 2.1586058139801
		2.81136751174927 2.22044825553894
		2.81193351745605 2.24851536750793
		2.7967267036438 2.47055697441101
		-1.25423431396484 4.41702151298523
		-1.28284668922424 4.41745233535767
		-1.34642362594604 4.41757583618164
		-1.3780517578125 4.41529011726379
		-1.46747326850891 4.40644574165344
		-1.49753212928772 4.40344715118408
		-1.52495741844177 4.40060806274414
		-1.61200189590454 4.39188456535339
		-1.64092993736267 4.38759160041809
		-1.70495676994324 4.38079810142517
		-1.73913860321045 4.37614870071411
		-1.7976987361908 4.36545872688293
		-1.8305926322937 4.36523461341858
		-1.86375689506531 4.36504554748535
		-1.96089243888855 4.36458158493042
		-2.08280754089355 4.37272524833679
		-2.17093777656555 4.38751125335693
		-2.19950389862061 4.39194178581238
		-2.23015022277832 4.4000461101532
		-2.29735136032104 4.41245937347412
		-2.3642805814743 4.41809630393982
		-2.42659091949463 4.42317056655884
		-2.55515575408936 4.42500972747803
		-2.77700352668762 4.40133380889893
		-2.83530163764954 4.3861231803894
		-4.20429873466492 4.10020065307617
		-4.22010061144829 4.08039379119873
		-4.29492317698896 3.46101021766663
		-4.31000929325819 3.39911198616028
		-4.31739538908005 3.36782360076904
		-4.32703213766217 3.33652520179749
		-4.33642789721489 3.30725860595703
		-4.34849924966693 3.27134799957275
		-4.3596957847476 3.2381603717804
		-4.37124966084957 3.20386075973511
		-4.37913026660681 3.16939854621887
		-4.38626613467932 3.13728404045105
		-4.392010435462 3.10312294960022
		-4.39631663262844 3.06810808181763
		-4.40035822987556 3.03153228759766
		-4.40314587950706 2.96304535865784
		-4.40488922595978 2.92725515365601
		-4.4011113345623 2.78823852539062
		-4.39853379130363 2.75611448287964
		-4.39465756714344 2.72738265991211
		-4.38986045867205 2.69572877883911
		-4.38666721433401 2.6657600402832
		-4.38106548786163 2.56252670288086
		-4.37780532985926 2.53092908859253
		-4.37833328545094 2.49699521064758
		-4.38026493042707 2.45818686485291
		-4.38105901330709 2.42016386985779
		-4.38242050260305 2.38259887695312
		-4.3847918882966 2.35127711296082
		-4.38700991123915 2.31845045089722
		-4.38858813792467 2.28492450714111
		-4.39196179062128 2.25402641296387
		-4.39477092772722 2.22049307823181
		-4.39794144779444 2.18961191177368
		-4.40471426397562 2.12453818321228
		-4.41071511059999 2.09141445159912
		-4.41589683294296 2.05882835388184
		-4.42469291388988 2.02418804168701
		-4.43102319538593 1.99048233032227
		-4.43449854850769 1.95809984207153
		-4.43931220471859 1.92662167549133
		-4.45934599637985 1.79532742500305
		-4.46073766052723 1.75970077514648
		-4.46034848690033 1.72458982467651
		-4.45808789134026 1.65307807922363
		-4.45658256113529 1.61756777763367
		-4.45516493916512 1.58273196220398
		-4.45372633635998 1.54860162734985
		-4.45193375647068 1.51425671577454
		-4.44886103272438 1.48077583312988
		-4.44513754546642 1.44820261001587
		-4.43903480470181 1.3830738067627
		-4.4344043135643 1.35182332992554
		-4.4321563243866 1.32061576843262
		-4.43279801309109 1.2869701385498
		-4.43421801924706 1.25133943557739
		-4.43657419085503 1.21593546867371
		-4.43932144343853 1.18174433708191
		-4.44406417012215 1.14706325531006
		-4.45105755329132 1.11510062217712
		-4.45955602824688 1.0819399356842
		-4.46840590238571 1.04931497573853
		-4.47842465341091 1.01575613021851
		-4.48880562186241 0.981179475784302
		-4.49825295805931 0.948833465576172
		-4.50914753973484 0.914734840393066
		-4.51909804344177 0.883046865463257
		-4.53290510177612 0.849736452102661
		-4.5581316947937 0.781339883804321
		-4.56626176834106 0.750385761260986
		-4.57577779889107 0.716333150863647
		-4.58497714996338 0.683912992477417
		-4.59244096279144 0.652178764343262
		-4.59923928976059 0.616273641586304
		-4.60503903031349 0.582354307174683
		-4.60931822657585 0.54950475692749
		-4.61268243193626 0.515385389328003
		-4.61515274643898 0.482114791870117
		-4.61704224348068 0.449590682983398
		-4.62029728293419 0.415626287460327
		-4.62200185656548 0.384278297424316
		-4.62073856592178 0.351881980895996
		-4.62349730730057 0.320404767990112
		-4.62125924229622 0.25773024559021
		-4.62004068493843 0.224389791488647
		-4.61575084924698 0.160235404968262
		-4.61475977301598 0.128693103790283
		-4.66803827881813 -0.189714908599854
		-3.90352419018745 -1.60487282276154
		-3.60910046100616 -1.53218007087708
		-3.58334600925446 -1.52072858810425
		-3.55723333358765 -1.50785160064697
		-3.53078693151474 -1.49719512462616
		-3.50331270694733 -1.48584353923798
		-3.47518408298492 -1.47485208511353
		-3.44707757234573 -1.46545612812042
		-3.41802161931992 -1.45678246021271
		-3.38964480161667 -1.44800341129303
		-3.35970437526703 -1.43810784816742
		-3.33065295219421 -1.43012094497681
		-3.30192762613297 -1.42100524902344
		-3.27380967140198 -1.41187953948975
		-2.53768599033356 -1.78583562374115
		-2.0426971912384 -2.14299568533897
		-1.46672916412354 -2.35356555879116
		-0.865665912628174 -2.5841963738203
		-0.28018856048584 -2.75544947385788
		0.342928886413574 -2.89327621459961
		2.7653431892395 0.665658473968506
		2.75253486633301 1.25136613845825
		2.74914598464966 1.86946964263916
		-1.67482256889343 4.38534665107727
		-2.89601147174835 4.3712170124054
		-4.40217693895102 2.82323908805847
		-4.40135186910629 2.15742945671082
		-4.44310756027699 1.41467595100403
		-4.54776313900948 0.814980030059814
		-1.11919379234314 -0.0964715480804443
		-1.45046424865723 -0.259353160858154
		-2.94103753566742 -1.42703115940094
		-4.61973610520363 0.191359996795654
		0.301782131195068 -1.15168118476868
		0.103693008422852 0.279215335845947
		-1.66403460502625 4.20123672485352
		-3.21521210670471 -1.39849436283112
		-3.1865713596344 -1.39121925830841
		-3.15793740749359 -1.38318061828613
		-3.12943816184998 -1.37480044364929
		-3.09909749031067 -1.3673654794693
		-3.06734991073608 -1.35799765586853
		-3.03701293468475 -1.34549200534821
		-3.00882291793823 -1.33239769935608
		-2.97965347766876 -1.31863105297089
		-2.95066618919373 -1.30320191383362
		-2.92066764831543 -1.28523600101471
		-2.89169800281525 -1.26626873016357
		-2.86477744579315 -1.24565732479095
		-2.83690202236176 -1.22244143486023
		-2.81105995178223 -1.19838190078735
		-2.78684890270233 -1.17433416843414
		-2.76344239711761 -1.15016233921051
		-2.7184089422226 -1.09955644607544
		-2.69677650928497 -1.07208859920502
		-2.67440116405487 -1.04136502742767
		-2.65325593948364 -1.01019275188446
		-2.63146567344666 -0.980669617652893
		-2.60982489585876 -0.946884393692017
		-2.59091520309448 -0.912709951400757
		-2.57296848297119 -0.879623293876648
		-2.55188393592834 -0.846693396568298
		-2.52835249900818 -0.818550825119019
		-2.50330209732056 -0.79122269153595
		-2.47745203971863 -0.763608336448669
		-2.44934594631195 -0.732444763183594
		-2.43058657646179 -0.708453416824341
		-2.38136029243469 -0.652533292770386
		-2.35651135444641 -0.627318978309631
		-2.3328458070755 -0.60309886932373
		-2.25963997840881 -0.53263258934021
		-2.23432993888855 -0.509002685546875
		-2.20563340187073 -0.488120079040527
		-2.17600536346436 -0.464558601379395
		-2.15006589889526 -0.438178300857544
		-2.12809085845947 -0.410266399383545
		-2.10576033592224 -0.384894609451294
		-2.08376955986023 -0.359236717224121
		-2.06305289268494 -0.332146167755127
		-2.04290843009949 -0.304666042327881
		-2.0239429473877 -0.276392936706543
		-2.00612378120422 -0.248367309570312
		-1.98850655555725 -0.219738006591797
		-1.97079515457153 -0.190974950790405
		-1.95342969894409 -0.160780906677246
		-1.93699336051941 -0.129960060119629
		-1.92102193832397 -0.0983984470367432
		-1.88999128341675 -0.0309560298919678
		-1.8765594959259 0.00416159629821777
		-1.86055302619934 0.0394794940948486
		-1.84599661827087 0.0742387771606445
		-1.83171582221985 0.110515356063843
		-1.81689953804016 0.143288850784302
		-1.79959154129028 0.174514532089233
		-1.77866125106812 0.204972982406616
		-1.75677037239075 0.236977100372314
		-1.73443746566772 0.269885778427124
		-1.71265363693237 0.302143573760986
		-1.68900942802429 0.331577777862549
		-1.66547679901123 0.359428405761719
		-1.64205455780029 0.385988235473633
		-1.61738014221191 0.410605907440186
		-1.59160280227661 0.434223175048828
		-1.56518840789795 0.45696759223938
		-1.51045346260071 0.500088214874268
		-1.48287272453308 0.520118474960327
		-1.45489811897278 0.539576768875122
		-1.42418718338013 0.556799411773682
		-1.39678049087524 0.576595544815063
		-1.3745493888855 0.59682035446167
		-1.35114550590515 0.615208864212036
		-1.32780504226685 0.635141372680664
		-1.30577802658081 0.656468152999878
		-1.2826931476593 0.678339242935181
		-1.26311945915222 0.701130628585815
		-1.24088191986084 0.72329306602478
		-1.19231224060059 0.767637968063354
		-1.16723346710205 0.790067911148071
		-1.11612725257874 0.834963083267212
		-0.0431647300720215 1.15634655952454
		-0.00477313995361328 1.15637731552124
		0.0734372138977051 1.15548396110535
		0.11493444442749 1.15550422668457
		0.156240463256836 1.15547490119934
		0.197224617004395 1.15223956108093
		0.239355087280273 1.14751577377319
		0.280713558197021 1.14336776733398
		0.393359661102295 1.11055183410645
		0.429850578308105 1.09553670883179
		0.465181350708008 1.07873177528381
		0.498700618743896 1.06002998352051
		0.528893947601318 1.03945446014404
		0.555737972259521 1.01706719398499
		0.581520557403564 0.993365526199341
		0.605135440826416 0.967055559158325
		0.627744197845459 0.941199541091919
		0.649874687194824 0.91402792930603
		0.67102575302124 0.886675596237183
		0.707642078399658 0.82646918296814
		0.727741241455078 0.796602249145508
		0.750485420227051 0.770499467849731
		0.771280288696289 0.743537664413452
		0.791798114776611 0.717138528823853
		0.811149597167969 0.690264463424683
		0.82975435256958 0.66512656211853
		0.847797870635986 0.638798236846924
		0.865520477294922 0.612848997116089
		0.883092880249023 0.586136817932129
		0.901453018188477 0.55943489074707
		0.920179843902588 0.531665086746216
		0.938094139099121 0.502944707870483
		0.974667072296143 0.442760467529297
		0.992998600006104 0.411646366119385
		1.01134824752808 0.381392002105713
		1.02676868438721 0.344072103500366
		1.05940055847168 0.277475833892822
		1.06993722915649 0.244171142578125
		1.07904243469238 0.210108041763306
		1.0875449180603 0.176141262054443
		1.09378623962402 0.141998529434204
		1.09774827957153 0.107494592666626
		1.09995746612549 0.0734100341796875
		1.1002516746521 0.0401318073272705
		1.09842014312744 0.00704145431518555
		1.09559154510498 -0.0251839160919189
		1.09190988540649 -0.0559177398681641
		1.08701658248901 -0.0852518081665039
		1.080810546875 -0.114222526550293
		0.960212707519531 -0.481370210647583
		0.948887348175049 -0.514284372329712
		0.937035083770752 -0.547760963439941
		0.924861431121826 -0.582005620002747
		0.899145126342773 -0.649506330490112
		0.827256679534912 -0.825510501861572
		0.808817386627197 -0.857689023017883
		0.73979663848877 -0.940678119659424
		0.716102600097656 -0.966293334960938
		0.691353797912598 -0.989157199859619
		0.666869640350342 -1.010338306427
		0.642688751220703 -1.02959370613098
		0.61724853515625 -1.04639828205109
		0.591197490692139 -1.06121563911438
		0.564466953277588 -1.07266175746918
		0.538462162017822 -1.08243238925934
		0.513677597045898 -1.09054148197174
		0.487739086151123 -1.09425842761993
		0.459846496582031 -1.09555172920227
		0.432568550109863 -1.10253536701202
		0.407776832580566 -1.11045122146606
		0.357624530792236 -1.12734472751617
		0.332238674163818 -1.13514935970306
		0.306550979614258 -1.14023411273956
		0.281052112579346 -1.1433767080307
		0.255891799926758 -1.14623320102692
		0.230234622955322 -1.14752769470215
		0.207769870758057 -1.14956438541412
		0.187309265136719 -1.1526210308075
		0.168493747711182 -1.15689432621002
		0.150603294372559 -1.16226541996002
		0.132060527801514 -1.16833531856537
		0.114351749420166 -1.17139673233032
		0.0965490341186523 -1.17378497123718
		0.0756363868713379 -1.18040287494659
		0.0572085380554199 -1.18995928764343
		0.0446157455444336 -1.20048749446869
		0.0344123840332031 -1.21313273906708
		0.0155935287475586 -1.24252104759216
		0.00612115859985352 -1.25567853450775
		-0.00242805480957031 -1.26635670661926
		-0.0121235847473145 -1.27583789825439
		-0.0215301513671875 -1.28344988822937
		-0.0297012329101562 -1.28991317749023
		-0.0370597839355469 -1.29671406745911
		-0.0443835258483887 -1.30385673046112
		-0.0512504577636719 -1.31139993667603
		-0.0597043037414551 -1.3189594745636
		-0.0675516128540039 -1.32363784313202
		-0.0764989852905273 -1.32518410682678
		-0.090113639831543 -1.32405459880829
		-0.108784675598145 -1.32318520545959
		-0.130878925323486 -1.32353210449219
		-0.154325485229492 -1.32388532161713
		-0.179200649261475 -1.32249820232391
		-0.231256484985352 -1.3114333152771
		-0.257473468780518 -1.30180752277374
		-0.283771991729736 -1.28925204277039
		-0.307493925094604 -1.27487707138062
		-0.329721689224243 -1.25788831710815
		-0.352237939834595 -1.2392144203186
		-0.37431788444519 -1.22138142585754
		-0.393873929977417 -1.20453357696533
		-0.411863327026367 -1.18730640411377
		-0.428297519683838 -1.16887807846069
		-0.444737911224365 -1.15106201171875
		-0.459189891815186 -1.13025391101837
		-0.471837997436523 -1.10908949375153
		-0.483140707015991 -1.08830440044403
		-0.495018005371094 -1.06948029994965
		-0.505005359649658 -1.05299401283264
		-0.513897895812988 -1.03849458694458
		-0.531192541122437 -1.00704634189606
		-0.54308819770813 -0.991672158241272
		-0.552269697189331 -0.97727358341217
		-0.562112331390381 -0.961335182189941
		-0.575012683868408 -0.943560600280762
		-0.59072208404541 -0.926045894622803
		-0.608514070510864 -0.909073948860168
		-0.627354383468628 -0.893943309783936
		-0.647042989730835 -0.879947185516357
		-0.667221307754517 -0.86663031578064
		-0.687068700790405 -0.8524169921875
		-0.706599712371826 -0.838166117668152
		-0.722088813781738 -0.82431960105896
		-0.736362218856812 -0.810944199562073
		-0.749928712844849 -0.800187110900879
		-0.760092258453369 -0.794798254966736
		-0.76845383644104 -0.79436194896698
		-0.783474445343018 -0.797157764434814
		-0.788318872451782 -0.798201322555542
		-0.790523529052734 -0.799994587898254
		-0.790154933929443 -0.803003072738647
		-0.786429166793823 -0.80745804309845
		-0.779319286346436 -0.813050270080566
		-0.768954038619995 -0.81961989402771
		-0.755683660507202 -0.827946901321411
		-0.738410711288452 -0.838007807731628
		-0.716881275177002 -0.849721312522888
		-0.692207336425781 -0.862349987030029
		-0.66495680809021 -0.876645922660828
		-0.635946989059448 -0.891597509384155
		-0.604500770568848 -0.907089233398438
		-0.571570634841919 -0.922106385231018
		-0.539379119873047 -0.934856295585632
		-0.509863376617432 -0.947177886962891
		-0.453445434570312 -0.97726833820343
		-0.430291891098022 -0.993814706802368
		-0.408097267150879 -1.01165461540222
		-0.388017177581787 -1.03024351596832
		-0.368550062179565 -1.0485383272171
		-0.348654270172119 -1.06616604328156
		-0.330425500869751 -1.08242881298065
		-0.312680959701538 -1.09690487384796
		-0.297281265258789 -1.11057901382446
		-0.28343677520752 -1.1244250535965
		-0.267533779144287 -1.13790857791901
		-0.248834133148193 -1.15047705173492
		-0.228556632995605 -1.15959358215332
		-0.208854675292969 -1.1683337688446
		-0.189523220062256 -1.17654871940613
		-0.166805267333984 -1.18380606174469
		-0.141841888427734 -1.1903862953186
		-0.0904417037963867 -1.20100367069244
		-0.0621514320373535 -1.20575666427612
		-0.0310778617858887 -1.20952951908112
		0.00168323516845703 -1.21019542217255
		0.0360918045043945 -1.2074716091156
		0.0695910453796387 -1.20568192005157
		0.104830741882324 -1.2032698392868
		0.140841484069824 -1.1989837884903
		0.17212963104248 -1.19220328330994
		0.195987224578857 -1.18567633628845
		0.217358112335205 -1.17861485481262
		0.23543643951416 -1.17067837715149
		0.251672267913818 -1.16389167308807
		0.266383647918701 -1.16020596027374
		0.280211925506592 -1.15849936008453
		0.290905952453613 -1.15740156173706
		0.298315048217773 -1.15552663803101
		0.29877233505249 -1.14597022533417
		0.292807579040527 -1.14103949069977
		0.283247470855713 -1.13557350635529
		0.27116870880127 -1.12911331653595
		0.255562305450439 -1.12221300601959
		0.236757755279541 -1.11392247676849
		0.214638710021973 -1.10395288467407
		0.189376831054688 -1.09244894981384
		0.161356925964355 -1.07856893539429
		0.132272243499756 -1.06272041797638
		0.101394653320312 -1.04454636573792
		0.0699763298034668 -1.02526831626892
		0.0393834114074707 -1.00716292858124
		0.0100493431091309 -0.990828990936279
		-0.0192880630493164 -0.975882530212402
		-0.0477409362792969 -0.962546706199646
		-0.0770149230957031 -0.951367497444153
		-3.24423289299011 -1.40639495849609
		-2.74042236804962 -1.12527143955231
		-2.28314447402954 -0.554325342178345
		-1.90478777885437 -0.065068244934082
		-1.53825306892395 0.478923320770264
		0.0335893630981445 1.15593886375427
		0.689895629882812 0.858928442001343
		1.04495668411255 0.310590744018555
		0.912328720092773 -0.616129755973816
		0.382522106170654 -1.11818516254425
		0.0242424011230469 -1.22762608528137
		-0.205463886260986 -1.31866002082825
		-0.520869493484497 -1.0226012468338
		-0.776374578475952 -0.795583844184875
		-0.480547666549683 -0.961318731307983
		-0.116062164306641 -1.19577169418335
		-0.139737606048584 -0.935834050178528
		-0.171244144439697 -0.928955674171448
		-0.201854705810547 -0.922062754631042
		-0.230275630950928 -0.914840459823608
		-0.25727367401123 -0.908249258995056
		-0.282528400421143 -0.903212785720825
		-0.306378841400146 -0.899451851844788
		-0.329739332199097 -0.897916197776794
		-0.352173328399658 -0.897143602371216
		-0.376338005065918 -0.895961999893188
		-0.401447534561157 -0.894657254219055
		-0.429410219192505 -0.892661213874817
		-0.460341453552246 -0.889306306838989
		-0.494524002075195 -0.883160471916199
		-0.563714981079102 -0.868979573249817
		-0.59633469581604 -0.857339859008789
		-1.21284055709839 -0.232818841934204
		-1.22509479522705 -0.171483278274536
		-1.22740507125854 -0.139894247055054
		-1.22591137886047 -0.10886025428772
		-1.22459840774536 -0.0792357921600342
		-1.21851992607117 -0.0501852035522461
		-1.21385502815247 -0.0180635452270508
		-1.20574927330017 0.012479305267334
		-1.20286822319031 0.0413997173309326
		-1.19568467140198 0.0645697116851807
		-1.19260597229004 0.0897402763366699
		-1.18890261650085 0.139318704605103
		-1.18979620933533 0.16293740272522
		-1.19317030906677 0.186396837234497
		-1.19411087036133 0.20825719833374
		-1.19393014907837 0.228434324264526
		-1.19382524490356 0.247164249420166
		-1.19254851341248 0.261994361877441
		-1.19226694107056 0.289807796478271
		-1.19135975837708 0.299739122390747
		-1.18904876708984 0.308566570281982
		-1.18622779846191 0.321699142456055
		-1.18505859375 0.33832836151123
		-1.18447113037109 0.355790853500366
		-1.18123722076416 0.373739004135132
		-1.16909742355347 0.41967248916626
		-1.15975975990295 0.448584318161011
		-1.14965176582336 0.478830575942993
		-1.13957023620605 0.511404037475586
		-1.12785029411316 0.54493522644043
		-1.11603450775146 0.578848361968994
		-1.10163068771362 0.610631942749023
		-1.08465790748596 0.641202688217163
		-1.00886678695679 0.745638370513916
		-0.657060146331787 1.15363097190857
		-0.602487325668335 1.17550873756409
		-0.573309183120728 1.18442702293396
		-0.542730569839478 1.1920371055603
		-0.511220693588257 1.19936656951904
		-0.48034930229187 1.20702338218689
		-0.447131633758545 1.21624040603638
		-0.418034791946411 1.22655081748962
		-0.390183687210083 1.2363166809082
		-0.361660480499268 1.2460196018219
		-0.332295179367065 1.25383472442627
		-0.303332328796387 1.26068925857544
		-0.273575305938721 1.26623678207397
		-0.243466377258301 1.27206110954285
		-0.212939739227295 1.27773118019104
		-0.183267116546631 1.28299450874329
		-0.155868053436279 1.28830885887146
		-0.129417419433594 1.29340934753418
		-0.0858893394470215 1.30093908309937
		-0.0643181800842285 1.30186080932617
		-0.0418915748596191 1.30198383331299
		-0.0189332962036133 1.30376172065735
		0.00352764129638672 1.30636501312256
		0.0266714096069336 1.30821084976196
		0.0533585548400879 1.30869221687317
		0.0805072784423828 1.30846452713013
		0.108007907867432 1.30761671066284
		0.136199951171875 1.30503916740417
		0.193504333496094 1.29777312278748
		0.2219557762146 1.29172849655151
		0.251545429229736 1.28284525871277
		0.279844284057617 1.272292137146
		0.306796550750732 1.25926685333252
		0.332046508789062 1.2439866065979
		0.446691989898682 1.16754412651062
		0.51635217666626 1.13635802268982
		0.538942337036133 1.12615323066711
		0.56072473526001 1.11558651924133
		0.599546909332275 1.0926239490509
		0.643015384674072 1.05555009841919
		0.657205581665039 1.04252815246582
		0.669690608978271 1.03030276298523
		0.681671619415283 1.01776146888733
		0.692926406860352 1.00495600700378
		0.703433990478516 0.991317510604858
		0.736043930053711 0.941744327545166
		0.747417449951172 0.921402454376221
		0.758265495300293 0.90018367767334
		0.777610301971436 0.852846622467041
		0.785701274871826 0.827550649642944
		0.791847705841064 0.800203800201416
		0.795901298522949 0.770696640014648
		0.799737930297852 0.710898399353027
		0.798248767852783 0.679014682769775
		0.796547889709473 0.648887872695923
		0.79616641998291 0.617741346359253
		0.798167705535889 0.586602449417114
		0.799993515014648 0.559317350387573
		0.802294731140137 0.532225131988525
		0.806186676025391 0.504197359085083
		0.810657978057861 0.477164506912231
		0.814679145812988 0.449379444122314
		0.817949771881104 0.421698570251465
		0.821138381958008 0.394445419311523
		0.823969841003418 0.367918968200684
		0.826972961425781 0.342682838439941
		0.830242156982422 0.31749963760376
		0.834210872650146 0.292564392089844
		0.837543964385986 0.26990532875061
		0.837019443511963 0.228739738464355
		0.834843158721924 0.208525657653809
		0.832397937774658 0.190753221511841
		0.82888650894165 0.173847675323486
		0.825639724731445 0.15255069732666
		0.82374906539917 0.129616022109985
		0.821560382843018 0.106831073760986
		0.818082809448242 0.083519458770752
		0.812336444854736 0.0604681968688965
		0.804314613342285 0.0372543334960938
		0.793581962585449 0.0141868591308594
		0.780709743499756 -0.00851011276245117
		0.766463756561279 -0.0307550430297852
		0.750809669494629 -0.0517647266387939
		0.733503818511963 -0.071876049041748
		0.715365886688232 -0.0922093391418457
		0.69675350189209 -0.113544940948486
		0.665260314941406 -0.155202865600586
		0.651168823242188 -0.174505472183228
		0.638208389282227 -0.19309139251709
		0.625133037567139 -0.211330413818359
		0.612997531890869 -0.230718374252319
		0.599330902099609 -0.251935482025146
		0.589051723480225 -0.272381067276001
		0.577659130096436 -0.293827772140503
		0.565845966339111 -0.31463098526001
		0.554647445678711 -0.334999561309814
		0.542894840240479 -0.355003118515015
		0.0388383865356445 -0.741335272789001
		0.015129566192627 -0.752394080162048
		-0.00822544097900391 -0.763065218925476
		-0.0302548408508301 -0.775348305702209
		-0.0495729446411133 -0.784765243530273
		-0.0681037902832031 -0.795718669891357
		-0.102033615112305 -0.81592857837677
		-0.118130683898926 -0.824884295463562
		-0.132920265197754 -0.833081722259521
		-0.14578104019165 -0.839864134788513
		-0.160085201263428 -0.845503330230713
		-0.176154613494873 -0.850763559341431
		-0.193031311035156 -0.856585621833801
		-0.210091590881348 -0.861902236938477
		-0.22615385055542 -0.865069985389709
		-0.242024898529053 -0.864904761314392
		-0.260375499725342 -0.862035155296326
		-0.278355121612549 -0.857969045639038
		-0.296231746673584 -0.853223323822021
		-0.314008474349976 -0.847314119338989
		-0.331355094909668 -0.839377284049988
		-0.348082304000854 -0.828980445861816
		-0.364731311798096 -0.815848469734192
		-0.396506786346436 -0.781209945678711
		-0.410696268081665 -0.761560797691345
		-0.424693822860718 -0.741687536239624
		-0.437394142150879 -0.721774578094482
		-0.445772886276245 -0.7027508020401
		-0.451537609100342 -0.684049725532532
		-0.455666065216064 -0.664581537246704
		-0.458576679229736 -0.64491856098175
		-0.459955215454102 -0.624821782112122
		-0.460288286209106 -0.605255246162415
		-0.459454298019409 -0.586531281471252
		-0.457114934921265 -0.569753885269165
		-0.45353102684021 -0.554808855056763
		-0.44917893409729 -0.541997909545898
		-0.444063901901245 -0.530637264251709
		-0.438563823699951 -0.520967245101929
		-0.432770490646362 -0.512042045593262
		-0.418881177902222 -0.495677947998047
		-0.407138586044312 -0.488276481628418
		-0.396407842636108 -0.479654788970947
		-0.38745641708374 -0.471310615539551
		-0.37705659866333 -0.463324785232544
		-0.365288257598877 -0.454926252365112
		-0.353477001190186 -0.446407318115234
		-0.342907190322876 -0.437713146209717
		-0.333257675170898 -0.428781270980835
		-0.323894023895264 -0.418983221054077
		-0.315673589706421 -0.408087730407715
		-0.308763027191162 -0.396149635314941
		-0.30242657661438 -0.384101867675781
		-0.296854257583618 -0.372680187225342
		-0.291645526885986 -0.361377954483032
		-0.287078857421875 -0.349797010421753
		-0.282366275787354 -0.338062524795532
		-0.272215366363525 -0.313056468963623
		-0.266664505004883 -0.301045656204224
		-0.26079273223877 -0.289906740188599
		-0.254109859466553 -0.280073165893555
		-0.246072769165039 -0.270961761474609
		-0.237159729003906 -0.261728525161743
		-0.227141380310059 -0.252754688262939
		-0.216249942779541 -0.24431324005127
		-0.204848766326904 -0.236800909042358
		-0.192689895629883 -0.230083465576172
		-0.179750919342041 -0.225208282470703
		-0.164846897125244 -0.22139310836792
		-0.147972106933594 -0.216843843460083
		-0.129445552825928 -0.211901903152466
		-0.110036373138428 -0.205521583557129
		-0.0899624824523926 -0.198134422302246
		-0.0694217681884766 -0.190176963806152
		-0.0345239639282227 -0.173102855682373
		-0.0199680328369141 -0.166777372360229
		-0.00685691833496094 -0.161892175674438
		0.00453662872314453 -0.15779972076416
		0.0139575004577637 -0.154565095901489
		0.123301982879639 -0.07381272315979
		0.133353233337402 -0.0546555519104004
		0.140100002288818 -0.0376944541931152
		0.147955894470215 -0.0241324901580811
		0.154772281646729 -0.0120234489440918
		0.159882545471191 -0.00109410285949707
		0.162444114685059 0.00947117805480957
		0.162575721740723 0.0190322399139404
		0.160519599914551 0.0269498825073242
		0.157490730285645 0.0342843532562256
		0.154637336730957 0.039985179901123
		0.151484966278076 0.044093132019043
		0.142468929290771 0.0504040718078613
		0.136707782745361 0.0545728206634521
		0.129894733428955 0.0579440593719482
		0.124735832214355 0.0603225231170654
		0.12242317199707 0.0647997856140137
		0.120994567871094 0.0735011100769043
		0.119166851043701 0.0848557949066162
		0.117080211639404 0.097440242767334
		0.115183353424072 0.110934734344482
		0.1134352684021 0.125497579574585
		0.111397266387939 0.141303062438965
		0.108218669891357 0.159191608428955
		0.104254245758057 0.178381681442261
		0.0963058471679688 0.200126886367798
		0.0864739418029785 0.218239545822144
		0.0811862945556641 0.230682134628296
		0.0794820785522461 0.242374420166016
		0.078249454498291 0.262396097183228
		0.078188419342041 0.268656492233276
		0.0787558555603027 0.273709774017334
		0.0793972015380859 0.278515100479126
		0.0810375213623047 0.282701969146729
		0.083899974822998 0.286343812942505
		0.087313175201416 0.2889723777771
		0.0908412933349609 0.288659572601318
		0.0944013595581055 0.288135766983032
		0.0976576805114746 0.285709857940674
		0.100658893585205 0.282078742980957
		0.103667259216309 0.278978109359741
		0.105197906494141 0.276906251907349
		0.105621814727783 0.274967193603516
		0.106031894683838 0.273881435394287
		0.105300426483154 0.274158954620361
		0.104858875274658 0.274932384490967
		0.101418018341064 0.285519599914551
		0.0947113037109375 0.292232036590576
		0.074763298034668 0.297032117843628
		0.0654759407043457 0.29588770866394
		0.0576715469360352 0.294289827346802
		0.0503983497619629 0.292346477508545
		0.0440464019775391 0.289305210113525
		0.0396738052368164 0.284510135650635
		0.036984920501709 0.278688192367554
		0.035036563873291 0.271933078765869
		0.0351438522338867 0.263369560241699
		0.0376901626586914 0.253976345062256
		0.0427045822143555 0.243296146392822
		0.04888916015625 0.231685876846313
		0.0543971061706543 0.219070196151733
		0.0635647773742676 0.206120729446411
		0.0728416442871094 0.196432113647461
		-0.108039855957031 -0.942817807197571
		-1.2196102142334 -0.202438831329346
		-1.19220566749573 0.277002811431885
		-0.630638360977173 1.16545343399048
		-0.105204582214355 1.29842662811279
		0.493422985076904 1.14630746841431
		0.798702716827393 0.741109848022461
		0.838242530822754 0.249480485916138
		0.679872512817383 -0.135138273239136
		-0.0853056907653809 -0.806037068367004
		-0.38128924369812 -0.799543619155884
		-0.426846265792847 -0.503372669219971
		-0.277495861053467 -0.325661182403564
		-0.0507888793945312 -0.181404590606689
		0.147616863250732 0.0476460456848145
		0.0792436599731445 0.253770589828491
		0.0815987586975098 0.184106349945068
		0.0839347839355469 0.177815675735474
		0.084864616394043 0.171042203903198
		0.0846109390258789 0.164938449859619
		0.0830888748168945 0.15996527671814
		0.0798640251159668 0.155462265014648
		0.0746297836303711 0.150488615036011
		0.0678491592407227 0.143883228302002
		0.0594892501831055 0.134607791900635
		0.0501933097839355 0.123613834381104
		0.0398411750793457 0.11253023147583
		0.027836799621582 0.102098703384399
		0.01446533203125 0.0922648906707764
		-0.000557422637939453 0.0828537940979004
		-0.187736988067627 -0.0311923027038574
		-0.213685035705566 -0.0397756099700928
		-0.224315166473389 -0.0427324771881104
		-0.291979789733887 -0.046879768371582
		-0.298530578613281 -0.0467166900634766
		-0.303122282028198 -0.0460927486419678
		-0.307756423950195 -0.0453901290893555
		-0.389960527420044 -0.121003150939941
		-0.390766859054565 -0.143759250640869
		-0.388710975646973 -0.166485786437988
		-0.385486841201782 -0.185897827148438
		-0.383698701858521 -0.20403790473938
		-0.383737325668335 -0.221111059188843
		-0.387089967727661 -0.238704681396484
		-0.393890142440796 -0.258189678192139
		-0.404008626937866 -0.278525352478027
		-0.416037559509277 -0.299462795257568
		-0.428387641906738 -0.319905757904053
		-0.441370964050293 -0.339421987533569
		-0.454835891723633 -0.357643842697144
		-0.484662294387817 -0.390186309814453
		-0.50177001953125 -0.403891801834106
		-0.520809173583984 -0.416249752044678
		-0.541309833526611 -0.428113698959351
		-0.562495470046997 -0.439420461654663
		-0.582925319671631 -0.450322151184082
		-0.60228705406189 -0.459963083267212
		-0.620578050613403 -0.468411684036255
		-0.638140678405762 -0.477233409881592
		-0.654347658157349 -0.487643480300903
		-0.667748928070068 -0.499457597732544
		-0.678951263427734 -0.51139760017395
		-0.69033145904541 -0.522857189178467
		-0.701869010925293 -0.535581350326538
		-0.713690757751465 -0.550159215927124
		-0.72506308555603 -0.565827131271362
		-0.735092163085938 -0.582529306411743
		-0.749797344207764 -0.615846395492554
		-0.754601955413818 -0.631858944892883
		-0.75783109664917 -0.648298382759094
		-0.759751558303833 -0.665901303291321
		-0.760494470596313 -0.683921456336975
		-0.760843753814697 -0.701387166976929
		-0.760072231292725 -0.717513084411621
		-0.758500099182129 -0.731426596641541
		-0.758329391479492 -0.743111133575439
		-0.757887125015259 -0.753968715667725
		-0.758114337921143 -0.76322877407074
		-0.759844303131104 -0.771123766899109
		-0.762367963790894 -0.77870512008667
		-0.765514850616455 -0.78607714176178
		-0.768378734588623 -0.791845321655273
		-0.771888971328735 -0.795383453369141
		-0.775590658187866 -0.797245025634766
		-0.78009819984436 -0.795010328292847
		-0.780930757522583 -0.791971564292908
		-0.780750274658203 -0.788885474205017
		-0.77820873260498 -0.786558508872986
		-0.772976160049438 -0.785452961921692
		-0.766163110733032 -0.78467869758606
		-0.757642507553101 -0.784935474395752
		-0.748700141906738 -0.787457823753357
		-0.737814664840698 -0.791898250579834
		-0.72600531578064 -0.797591805458069
		-0.712883949279785 -0.80402660369873
		-0.698525428771973 -0.811575055122375
		-0.683295965194702 -0.819514393806458
		-0.66624927520752 -0.827946424484253
		-0.647917032241821 -0.837862849235535
		-0.627657413482666 -0.849101781845093
		-0.605996131896973 -0.861527919769287
		-0.557853698730469 -0.890239715576172
		-0.529401302337646 -0.905829548835754
		-0.495512723922729 -0.92119574546814
		-0.464057922363281 -0.93304967880249
		-0.436925411224365 -0.945241689682007
		-0.41058874130249 -0.959159016609192
		-0.381691932678223 -0.973583340644836
		-0.35219407081604 -0.984793186187744
		-0.322547197341919 -0.992053508758545
		-0.295402050018311 -0.998798370361328
		-0.26790189743042 -1.00387358665466
		-0.241239070892334 -1.00926995277405
		-0.215213775634766 -1.0137403011322
		-0.189555168151855 -1.01683294773102
		-0.164257049560547 -1.01862466335297
		-0.139685153961182 -1.01802289485931
		-0.115392208099365 -1.0150363445282
		-0.0691518783569336 -1.00607824325562
		-0.0457420349121094 -1.00059604644775
		-0.0225529670715332 -0.993653416633606
		0.00317192077636719 -0.986240983009338
		0.0283584594726562 -0.979088306427002
		0.0546932220458984 -0.972500562667847
		0.084205150604248 -0.966763377189636
		0.115021705627441 -0.959287166595459
		0.146191120147705 -0.952088475227356
		0.17616081237793 -0.946071982383728
		0.206294059753418 -0.940526723861694
		0.236834049224854 -0.934322118759155
		0.267406463623047 -0.927891850471497
		0.299452781677246 -0.920152068138123
		0.333450794219971 -0.911478877067566
		0.367170333862305 -0.902480959892273
		0.401196002960205 -0.893187761306763
		0.469970226287842 -0.874265551567078
		0.507074356079102 -0.862037777900696
		0.546170234680176 -0.845296144485474
		0.579728126525879 -0.826709866523743
		0.610910415649414 -0.808308959007263
		0.638806819915771 -0.789348363876343
		0.66591215133667 -0.770050764083862
		0.712863922119141 -0.726700901985168
		0.732078075408936 -0.704350709915161
		0.750754356384277 -0.682214379310608
		0.794452667236328 -0.609509110450745
		0.804858207702637 -0.584781885147095
		0.813482284545898 -0.560211896896362
		0.820796966552734 -0.534348964691162
		0.824695587158203 -0.507506608963013
		0.828262329101562 -0.480717897415161
		0.833212375640869 -0.450750827789307
		0.840239524841309 -0.396286725997925
		0.849666595458984 -0.367722749710083
		0.861075401306152 -0.337437391281128
		0.87252140045166 -0.305984735488892
		0.885688304901123 -0.275828838348389
		0.898201942443848 -0.245117425918579
		0.912219524383545 -0.214740514755249
		0.925323486328125 -0.181869029998779
		0.939818859100342 -0.149490356445312
		0.954147338867188 -0.115328311920166
		0.968924999237061 -0.0814602375030518
		0.983282089233398 -0.04693603515625
		0.997100830078125 -0.0121166706085205
		1.01074743270874 0.0232160091400146
		1.02310562133789 0.0633063316345215
		1.03198432922363 0.102896213531494
		1.03897476196289 0.140045881271362
		1.051109790802 0.209798812866211
		1.05346393585205 0.245654582977295
		1.05359649658203 0.28111720085144
		1.0523681640625 0.31537389755249
		1.05053567886353 0.349741697311401
		1.04759883880615 0.383870601654053
		1.04342985153198 0.417561769485474
		1.03795385360718 0.451553583145142
		1.03157091140747 0.485405683517456
		1.02417993545532 0.517987728118896
		1.0155200958252 0.550272941589355
		1.00656032562256 0.583091020584106
		0.996558666229248 0.615774631500244
		0.985238075256348 0.647187471389771
		0.974446773529053 0.680673122406006
		0.963448047637939 0.712829113006592
		0.953518390655518 0.744342088699341
		0.938451766967773 0.815282821655273
		0.93027400970459 0.853088855743408
		0.922322273254395 0.891509771347046
		0.915484428405762 0.929901599884033
		0.909547328948975 0.969646692276001
		0.904428482055664 1.00913023948669
		0.89959716796875 1.04875373840332
		0.89527702331543 1.0880184173584
		0.890999794006348 1.12759900093079
		0.886551380157471 1.16767978668213
		0.882192611694336 1.20822191238403
		0.878395557403564 1.25041365623474
		0.874495029449463 1.2962749004364
		0.866571426391602 1.34005856513977
		0.856096744537354 1.3804178237915
		0.846817970275879 1.41953253746033
		0.837604522705078 1.45754432678223
		0.813945770263672 1.53258228302002
		0.7995285987854 1.56949758529663
		0.783819198608398 1.60581040382385
		0.76659631729126 1.64132118225098
		0.749369621276855 1.67575097084045
		0.731455326080322 1.70944356918335
		0.713229656219482 1.74260497093201
		0.694470405578613 1.77639484405518
		0.674454689025879 1.81032395362854
		0.653285980224609 1.84310078620911
		0.634293556213379 1.87861084938049
		0.615009307861328 1.91213822364807
		0.596256732940674 1.94449043273926
		0.580290794372559 1.97979712486267
		0.565024852752686 2.01677966117859
		0.54963493347168 2.05575680732727
		0.534325122833252 2.0951611995697
		0.507808208465576 2.17390251159668
		0.496052265167236 2.21267533302307
		0.484499454498291 2.25177407264709
		0.473177433013916 2.29050779342651
		0.461001873016357 2.33013296127319
		0.448827743530273 2.36972498893738
		0.436836719512939 2.40921688079834
		0.424506664276123 2.44833755493164
		0.413651943206787 2.48991441726685
		0.401344776153564 2.53288245201111
		0.385223865509033 2.57176566123962
		0.369021415710449 2.60863351821899
		-0.217875003814697 3.24940371513367
		-0.246552467346191 3.26994204521179
		-0.303316831588745 3.31535363197327
		-0.333654642105103 3.33896040916443
		-0.362924575805664 3.36274886131287
		-0.392948150634766 3.38549327850342
		-0.424643754959106 3.40999460220337
		-1.18347120285034 3.93217301368713
		-1.29624390602112 4.00192093849182
		-1.32795166969299 4.0201108455658
		-1.3915011882782 4.05856680870056
		-1.42393732070923 4.07481980323792
		-1.45741367340088 4.09442496299744
		-1.49137496948242 4.11312985420227
		-1.52479648590088 4.13039875030518
		-1.55809330940247 4.14913511276245
		-1.6999146938324 4.21439218521118
		-1.91890859603882 4.26157784461975
		-1.95528292655945 4.26415395736694
		-2.0268383026123 4.26329231262207
		-2.06239485740662 4.26215362548828
		-2.12790489196777 4.25351309776306
		-2.16567730903625 4.24732971191406
		-2.23897290229797 4.24112248420715
		-2.26582551002502 4.23267126083374
		-2.3050936460495 4.23201394081116
		-2.33718645572662 4.22840046882629
		-2.37809193134308 4.22672843933105
		-2.65855848789215 4.24363613128662
		-2.82365846633911 4.24262523651123
		0.0780305862426758 0.190115690231323
		-0.283618450164795 -0.0466880798339844
		-0.469410419464111 -0.37454080581665
		-0.743380784988403 -0.599313497543335
		-0.778203010559082 -0.796898484230042
		-0.582801818847656 -0.875331282615662
		-0.0922799110412598 -1.01043379306793
		0.436060428619385 -0.883751034736633
		0.834952354431152 -0.422256231307983
		1.04581499099731 0.174769878387451
		0.945866584777832 0.779110908508301
		0.826606750488281 1.49510836601257
		0.520403861999512 2.13439226150513
		-0.274134159088135 3.29235863685608
		-3.93297001719475 3.7879045009613
		-3.96339324116707 3.76708340644836
		-4.14331650733948 3.6380500793457
		-4.1947211176157 3.5859808921814
		-4.27905238233507 3.46678853034973
		-4.29639540612698 3.43489789962769
		-4.309410716407 3.40455961227417
		-4.3246919773519 3.37502026557922
		-4.33771084621549 3.34030532836914
		-4.34803660959005 3.30986070632935
		-4.35750883817673 3.2743706703186
		-4.36567187309265 3.24201154708862
		-4.37683369964361 3.20461988449097
		-4.38492511212826 3.17158126831055
		-4.39310292899609 3.13798785209656
		-4.40322007238865 3.10531711578369
		-4.41340642422438 3.07091522216797
		-4.43602308630943 2.99738955497742
		-4.44531233608723 2.96080684661865
		-4.45583133399487 2.92422485351562
		-4.46550533175468 2.88711071014404
		-4.48715324699879 2.8165602684021
		-4.49448734521866 2.78023195266724
		-4.5055968016386 2.7463538646698
		-4.51347316801548 2.71088218688965
		-4.52191446721554 2.67375993728638
		-4.52901150286198 2.63604760169983
		-4.53639663755894 2.59782361984253
		-4.54663115739822 2.55873274803162
		-4.55941519141197 2.44891858100891
		-4.55823391675949 2.41090035438538
		-4.56130391359329 2.37258338928223
		-4.56291764974594 2.33149790763855
		-4.56385466456413 2.29311895370483
		-4.55870446562767 2.17376065254211
		-4.55578052997589 2.13657712936401
		-4.5508326292038 2.09760499000549
		-4.54595637321472 2.02008962631226
		-4.54092057049274 1.98181319236755
		-4.53603012859821 1.94672131538391
		-4.53110042214394 1.90975856781006
		-4.52373538911343 1.87545323371887
		-4.51978546380997 1.83823442459106
		-4.51891677081585 1.80326151847839
		-4.51372034847736 1.6814067363739
		-4.51234093308449 1.64071083068848
		-4.51297695934772 1.59907555580139
		-4.51390114426613 1.56332850456238
		-4.51563692092896 1.52465581893921
		-4.51830551028252 1.48599529266357
		-4.52075178921223 1.44682693481445
		-4.52651497721672 1.37036228179932
		-4.52925835549831 1.32887816429138
		-4.53270515799522 1.29006385803223
		-4.53835779428482 1.2509286403656
		-4.54390589892864 1.21276140213013
		-4.54368084669113 1.17218065261841
		-4.5441419929266 1.12850642204285
		-4.5458525121212 1.08800530433655
		-4.54577144980431 1.04960203170776
		-4.54629048705101 1.00828170776367
		-4.54578536748886 0.967875480651855
		-4.54313470423222 0.923189163208008
		-4.54358756542206 0.880670547485352
		-4.54231831431389 0.839977025985718
		-4.53929977118969 0.798433303833008
		-4.53871585428715 0.755667448043823
		-4.53393942117691 0.715424537658691
		-4.5286630243063 0.632451772689819
		-4.52551965415478 0.58994197845459
		-4.51618374884129 0.469233274459839
		-4.50934201478958 0.296406030654907
		-4.51083418726921 0.211812019348145
		-4.51694503426552 0.128443002700806
		-4.55139654874802 -0.162943601608276
		-4.55299171805382 -0.204670190811157
		-4.551279515028 -0.24614143371582
		-4.02382212877274 -1.74366688728333
		-3.97245144844055 -1.79454416036606
		-3.94371277093887 -1.8203467130661
		-3.91671851277351 -1.84302860498428
		-3.88668289780617 -1.86932325363159
		-3.85820871591568 -1.8912815451622
		-3.82872250676155 -1.91307520866394
		-3.80194261670113 -1.93274027109146
		-3.75150012969971 -1.98242002725601
		-3.67156702280045 -2.05859869718552
		-3.64606159925461 -2.08576083183289
		-3.62151277065277 -2.11242446303368
		-3.59757906198502 -2.13837838172913
		-3.57381939888 -2.16483741998672
		-3.54939353466034 -2.19162237644196
		-3.52537173032761 -2.21934697031975
		-3.50124663114548 -2.24589452147484
		-3.47733074426651 -2.27428308129311
		-3.45333576202393 -2.30137020349503
		-3.43016910552979 -2.3306810259819
		-3.40475672483444 -2.36064383387566
		-3.37850153446198 -2.38784867525101
		-3.35243451595306 -2.41073602437973
		-3.32477110624313 -2.44053401052952
		-3.29621243476868 -2.46576108783484
		-3.16842579841614 -2.56299112178385
		-3.13543391227722 -2.58328407723457
		-3.10135459899902 -2.60478515923023
		-3.06765425205231 -2.62332829087973
		-3.03299379348755 -2.64345582574606
		-2.99737691879272 -2.66435269266367
		-2.96185719966888 -2.6833201944828
		-2.92559409141541 -2.70058500766754
		-2.88996088504791 -2.71515870094299
		-2.85470271110535 -2.73036110401154
		-2.82013070583344 -2.7457135617733
		-2.78721952438354 -2.75631058216095
		-2.71707153320312 -2.79217636585236
		-2.6802419424057 -2.81091338396072
		-2.64295101165771 -2.83136826753616
		-2.6055052280426 -2.85059201717377
		-2.56806588172913 -2.87038141489029
		-2.49585676193237 -2.91034969687462
		-2.46035313606262 -2.92995202541351
		-2.3552770614624 -2.98854240775108
		-2.24806928634644 -3.04766669869423
		-2.21071195602417 -3.06745484471321
		-2.17365527153015 -3.08395248651505
		-2.13767433166504 -3.09946244955063
		-2.10179257392883 -3.11349731683731
		-2.06452298164368 -3.12641954421997
		-2.02474546432495 -3.13807475566864
		-1.98390173912048 -3.14681768417358
		-1.9407594203949 -3.15376573801041
		-1.89716935157776 -3.15927845239639
		-1.85325789451599 -3.16350966691971
		-1.76446127891541 -3.16971427202225
		-1.72083330154419 -3.17147719860077
		-1.67612886428833 -3.17232972383499
		-1.58740568161011 -3.17134016752243
		-1.54223299026489 -3.17227703332901
		-1.49745845794678 -3.16982191801071
		-1.45502114295959 -3.16729056835175
		-1.41264271736145 -3.16835409402847
		-1.36945748329163 -3.17247200012207
		-1.32581639289856 -3.17731326818466
		-1.28240561485291 -3.18200939893723
		-1.23884892463684 -3.18767505884171
		-1.19641518592834 -3.1915128827095
		-1.15518569946289 -3.19693201780319
		-1.11422038078308 -3.20397651195526
		-1.03807163238525 -3.19456708431244
		-0.996449947357178 -3.22233128547668
		-0.956053256988525 -3.23091667890549
		-0.916853666305542 -3.23609304428101
		-0.876659393310547 -3.24405372142792
		-0.793994665145874 -3.25187027454376
		-0.753572940826416 -3.25454133749008
		-0.713051795959473 -3.25962519645691
		-0.673753499984741 -3.25999456644058
		-0.634055614471436 -3.25969511270523
		-0.596056699752808 -3.25611644983292
		-0.555721282958984 -3.25699990987778
		-0.516140937805176 -3.2538925409317
		-0.476783990859985 -3.24990212917328
		-0.435813665390015 -3.24558299779892
		-0.396044731140137 -3.24047464132309
		-0.356666564941406 -3.23476499319077
		-0.314837455749512 -3.22965413331985
		-0.271498203277588 -3.22388970851898
		-0.229696273803711 -3.21749085187912
		-0.185202598571777 -3.21232122182846
		-0.142786979675293 -3.20569777488708
		-0.0620875358581543 -3.19375121593475
		-0.0211095809936523 -3.19395339488983
		0.0207648277282715 -3.19336593151093
		0.0628566741943359 -3.19267040491104
		0.104364395141602 -3.1920765042305
		0.144002914428711 -3.1927889585495
		0.185239315032959 -3.19562268257141
		0.227507591247559 -3.19957715272903
		2.37491416931152 -2.30922549962997
		2.44876146316528 -2.1773564517498
		2.4649977684021 -2.1441764831543
		2.48479509353638 -2.11027839779854
		2.5077657699585 -2.07683819532394
		2.52372932434082 -2.0428586602211
		2.54090547561646 -2.00905758142471
		2.56156921386719 -1.9747599363327
		2.57972955703735 -1.94098460674286
		2.62136936187744 -1.87294727563858
		2.70777130126953 -1.6848384141922
		2.75717735290527 -1.47842979431152
		2.76568841934204 -1.39536893367767
		2.76860809326172 -1.35408508777618
		2.85786437988281 0.192008972167969
		2.85634422302246 0.228513956069946
		2.85373258590698 0.265793323516846
		2.84855508804321 0.300716161727905
		2.84612607955933 0.336057662963867
		2.84673547744751 0.373656272888184
		2.84661817550659 0.413226366043091
		2.84716987609863 0.4538733959198
		2.8482837677002 0.494619607925415
		2.85047388076782 0.534889698028564
		2.85445880889893 0.573838472366333
		2.85905361175537 0.611473798751831
		2.86869096755981 0.685257434844971
		2.87447929382324 0.721235513687134
		2.88028955459595 0.75687313079834
		2.88709449768066 0.792689085006714
		2.89401245117188 0.828399419784546
		2.9037299156189 0.865922689437866
		2.91467428207397 0.903899669647217
		2.92021131515503 0.941125392913818
		2.92371273040771 0.978049516677856
		2.92993879318237 1.01631450653076
		2.93683767318726 1.09619927406311
		2.93744277954102 1.13779139518738
		2.93853044509888 1.17994260787964
		2.935378074646 1.2210693359375
		2.92083072662354 1.37201023101807
		2.91660642623901 1.40741777420044
		2.90527486801147 1.47531366348267
		2.890709400177 1.54459881782532
		2.8800106048584 1.57677745819092
		2.87378692626953 1.6095974445343
		2.87157535552979 1.64632821083069
		2.87099647521973 1.72209858894348
		2.86863899230957 1.76015734672546
		2.86899042129517 1.797682762146
		2.86707782745361 1.83340930938721
		2.86791658401489 1.86888146400452
		2.86699199676514 1.90490388870239
		2.87004327774048 1.94140148162842
		2.86941289901733 1.97789168357849
		2.86891078948975 2.01507782936096
		2.87009859085083 2.05292534828186
		2.87101030349731 2.09034872055054
		2.8718638420105 2.1271710395813
		2.87507772445679 2.16581749916077
		2.87106037139893 2.24320268630981
		2.85895156860352 2.31742310523987
		2.85384035110474 2.35589933395386
		2.81115007400513 2.58938241004944
		2.80009460449219 2.62455463409424
		2.78683996200562 2.66097569465637
		2.77733469009399 2.69660139083862
		2.76361751556396 2.72750496864319
		2.7296667098999 2.79461407661438
		2.71524000167847 2.82868361473083
		2.6989541053772 2.85878491401672
		2.68117904663086 2.88757753372192
		2.66789770126343 2.91924452781677
		2.64478778839111 2.99172782897949
		2.58808517456055 3.17231321334839
		2.55662679672241 3.28132247924805
		2.54512548446655 3.31870698928833
		2.51324272155762 3.42823791503906
		2.43456363677979 3.60847282409668
		2.4171986579895 3.64140486717224
		2.39586973190308 3.67472505569458
		2.15825176239014 3.9210410118103
		2.12908363342285 3.93671917915344
		2.06839275360107 3.96972131729126
		2.03870248794556 3.98595070838928
		2.00509595870972 4.00434827804565
		1.97539806365967 4.0162513256073
		1.94733428955078 4.03458714485168
		1.91506624221802 4.05296468734741
		1.88087940216064 4.07109093666077
		1.84514856338501 4.0894136428833
		1.80952835083008 4.10666680335999
		1.73959064483643 4.14264273643494
		1.67280101776123 4.17705988883972
		1.63879919052124 4.19552206993103
		1.60388278961182 4.21274733543396
		1.56917715072632 4.23007488250732
		1.53311014175415 4.24791836738586
		1.49794721603394 4.26189804077148
		1.4615330696106 4.28003787994385
		1.38656425476074 4.31084704399109
		1.01147365570068 4.38608193397522
		-3.87303188443184 3.82958984375
		-4.42520606517792 3.03507447242737
		-4.5615670979023 2.2546272277832
		-4.522565305233 1.40996742248535
		-4.53426498174667 0.670879125595093
		-3.77666598558426 -1.95593482255936
		-3.20176076889038 -2.53903371095657
		-2.53174531459808 -2.89029797911644
		-1.63138556480408 -3.17187261581421
		-0.834352254867554 -3.25225085020065
		-0.104713439941406 -3.19664865732193
		2.60298585891724 -1.90736126899719
		2.86371850967407 0.648694276809692
		2.89924192428589 1.51216912269592
		2.87542057037354 2.20475840568542
		2.52368211746216 3.3901801109314
		1.70664310455322 4.16231608390808
		-4.28781190142035 3.42300796508789
		-4.16802267730236 2.58314490318298
		-4.02845519781113 1.95116901397705
		-3.97852876782417 1.29072713851929
		-4.14946630597115 0.639552354812622
		-4.24721699208021 -0.0629119873046875
		-4.07036246359348 -1.22015810012817
		-3.06309103965759 -1.76182323694229
		-2.4304313659668 -1.63060188293457
		-1.86438703536987 -1.26064562797546
		-1.44160413742065 -0.894215941429138
		-1.05753898620605 -0.466533660888672
		-1.29559946060181 4.61269879341125
		-1.37559056282043 4.63076496124268
		-1.4130597114563 4.63795256614685
		-1.49455165863037 4.64759492874146
		-1.78762626647949 4.64587545394897
		-2.27300071716309 4.65301752090454
		-2.34772872924805 4.66183853149414
		-2.42698621749878 4.68191862106323
		-2.54328501224518 4.6983060836792
		-2.62138998508453 4.70752048492432
		-2.65994894504547 4.71192455291748
		-2.69729208946228 4.70599436759949
		-2.82245051860809 4.70911526679993
		-4.23999091982841 3.66129636764526
		-4.24607925489545 3.62715625762939
		-4.25239026546478 3.59513759613037
		-4.25868720561266 3.56131076812744
		-4.27058338187635 3.4935998916626
		-4.27952541038394 3.4586033821106
		-4.29417417105287 3.38643455505371
		-4.30116618098691 3.35404086112976
		-4.31371673382819 3.28272604942322
		-4.32096512615681 3.24346280097961
		-4.32518803700805 3.1681022644043
		-4.32464693486691 3.13213658332825
		-4.32279169559479 3.09304165840149
		-4.31510070711374 3.01413655281067
		-4.28759648604318 2.89460587501526
		-4.27683336474001 2.85746598243713
		-4.26667004078627 2.82028126716614
		-4.25554496794939 2.78466367721558
		-4.24314597994089 2.75018215179443
		-4.22870473563671 2.71562695503235
		-4.21463887393475 2.6810290813446
		-4.1993306428194 2.64952254295349
		-4.18373310565948 2.61518025398254
		-4.15178082883358 2.55368947982788
		-4.13792507350445 2.52309918403625
		-4.12574765086174 2.48943471908569
		-4.11309278011322 2.45494198799133
		-4.10129107534885 2.41842842102051
		-4.09020292758942 2.38270378112793
		-4.08049792051315 2.34778237342834
		-4.07193590700626 2.31321501731873
		-4.06481051445007 2.27948951721191
		-4.05937448143959 2.24639987945557
		-4.05388380587101 2.21126198768616
		-4.04847599565983 2.1759660243988
		-4.04341128468513 2.13934063911438
		-4.03808155655861 2.10271644592285
		-4.03399828076363 2.06524562835693
		-4.03035020828247 2.02861452102661
		-4.02872547507286 1.99173450469971
		-4.02544412016869 1.91340327262878
		-4.02222666144371 1.87721610069275
		-4.0193136036396 1.84034419059753
		-4.01666116714478 1.80830216407776
		-4.01274237036705 1.76624321937561
		-4.00817441940308 1.72871351242065
		-4.00273439288139 1.69208431243896
		-3.99727430939674 1.65506625175476
		-3.99231120944023 1.61896443367004
		-3.98831006884575 1.58299851417542
		-3.98564395308495 1.54717302322388
		-3.98372721672058 1.51123523712158
		-3.98256027698517 1.47486138343811
		-3.98158678412437 1.43802285194397
		-3.98043256998062 1.40123248100281
		-3.97888290882111 1.36556220054626
		-3.97903287410736 1.32728052139282
		-3.97833439707756 1.2563591003418
		-3.98115575313568 1.22094321250916
		-3.98535180091858 1.1841402053833
		-3.99072107672691 1.14653491973877
		-3.99605825543404 1.10737299919128
		-4.0029284954071 1.06973385810852
		-4.01198703050613 1.03290581703186
		-4.02261719107628 0.997755289077759
		-4.03430387377739 0.962946891784668
		-4.04721154272556 0.928728103637695
		-4.06008547544479 0.892259836196899
		-4.07302451133728 0.856697082519531
		-4.08568347990513 0.820696830749512
		-4.09867195785046 0.78463888168335
		-4.11164163053036 0.748733997344971
		-4.12567780911922 0.712336301803589
		-4.1399808973074 0.675623655319214
		-4.15896584093571 0.603645324707031
		-4.16860248148441 0.56838846206665
		-4.17636331915855 0.531500577926636
		-4.18273211270571 0.495104789733887
		-4.18890560418367 0.452875852584839
		-4.19425300508738 0.412684917449951
		-4.19804912060499 0.372173547744751
		-4.20325741916895 0.331193447113037
		-4.21106571704149 0.289340496063232
		-4.21689783036709 0.249642372131348
		-4.2225184366107 0.210363626480103
		-4.2256298661232 0.170556545257568
		-4.22913087159395 0.130983352661133
		-4.23207183927298 0.092111349105835
		-4.23849601298571 0.0522191524505615
		-4.24321653693914 0.0113778114318848
		-4.24252533912659 -0.0247721672058105
		-4.2522252202034 -0.101925373077393
		-4.25979904830456 -0.143434524536133
		-4.26624366082251 -0.183000802993774
		-4.27272154577076 -0.221892118453979
		-4.28133198991418 -0.260664463043213
		-4.28864399436861 -0.301656246185303
		-4.31462513655424 -0.427726030349731
		-4.31932611204684 -0.466691970825195
		-4.32631871849298 -0.508678913116455
		-4.33346147835255 -0.594292998313904
		-4.33655958995223 -0.638595342636108
		-4.33565010875463 -0.682178497314453
		-4.33190390467644 -0.724361658096313
		-4.32736153900623 -0.765627384185791
		-4.3205030914396 -0.805961489677429
		-4.12436370551586 -1.15932786464691
		-4.09654614329338 -1.18782424926758
		-4.043338149786 -1.24734890460968
		-4.01493975520134 -1.27250444889069
		-3.98784151673317 -1.29670178890228
		-3.95928990840912 -1.3229056596756
		-3.93076634407043 -1.34855973720551
		-3.89939099550247 -1.37964451313019
		-3.86787104606628 -1.40865087509155
		-3.83693960309029 -1.43406057357788
		-3.80543306469917 -1.45975601673126
		-3.77352094650269 -1.48527240753174
		-3.39179545640945 -1.71536839008331
		-3.35565620660782 -1.72745668888092
		-3.31959116458893 -1.73782831430435
		-3.24723029136658 -1.75442934036255
		-3.21057844161987 -1.7602264881134
		-3.17330574989319 -1.76376509666443
		-3.09741759300232 -1.76452261209488
		-3.02519679069519 -1.7592066526413
		-2.98885190486908 -1.75523942708969
		-2.95565247535706 -1.74875092506409
		-2.92090833187103 -1.74400609731674
		-2.8880627155304 -1.73840290307999
		-2.8545229434967 -1.73079758882523
		-2.81933987140656 -1.72349554300308
		-2.78343522548676 -1.71461832523346
		-2.74781048297882 -1.70637840032578
		-2.71170544624329 -1.69879055023193
		-2.67640066146851 -1.69161885976791
		-2.63994121551514 -1.68458956480026
		-2.60458433628082 -1.67618906497955
		-2.56967496871948 -1.66767877340317
		-2.5342493057251 -1.65947639942169
		-2.49851858615875 -1.64938980340958
		-2.46415948867798 -1.63993763923645
		-2.39436841011047 -1.6200076341629
		-2.35520529747009 -1.60875803232193
		-2.31709516048431 -1.59455150365829
		-2.28173542022705 -1.57849502563477
		-2.24858689308167 -1.5626460313797
		-2.18472576141357 -1.52780246734619
		-2.1537070274353 -1.50785076618195
		-2.12285566329956 -1.48744606971741
		-2.09273552894592 -1.46563458442688
		-2.06381702423096 -1.44212448596954
		-2.0360324382782 -1.41897594928741
		-2.00910758972168 -1.39702081680298
		-1.98378610610962 -1.37500655651093
		-1.96046257019043 -1.35340166091919
		-1.93742299079895 -1.33124613761902
		-1.91445112228394 -1.30818831920624
		-1.89038801193237 -1.28404033184052
		-1.84162878990173 -1.23651099205017
		-1.82075381278992 -1.21428251266479
		-1.79770517349243 -1.19187557697296
		-1.77321672439575 -1.16913676261902
		-1.74922585487366 -1.14513564109802
		-1.72442245483398 -1.12100720405579
		-1.69993138313293 -1.0984433889389
		-1.67590165138245 -1.07701814174652
		-1.6525411605835 -1.05577194690704
		-1.62922430038452 -1.03583538532257
		-1.60654878616333 -1.01764023303986
		-1.58357000350952 -0.999434947967529
		-1.56025433540344 -0.981306314468384
		-1.53724074363708 -0.963900685310364
		-1.51449966430664 -0.94619083404541
		-1.49007153511047 -0.928861975669861
		-1.46547436714172 -0.911731719970703
		-1.41630291938782 -0.876334309577942
		-1.3903443813324 -0.856740355491638
		-1.36875438690186 -0.837819933891296
		-1.34721827507019 -0.818207263946533
		-1.3238263130188 -0.796894788742065
		-1.30101227760315 -0.77394425868988
		-1.27940821647644 -0.750646829605103
		-1.25722455978394 -0.727453231811523
		-1.23586058616638 -0.704392433166504
		-1.21496295928955 -0.68113112449646
		-1.19390368461609 -0.656032204627991
		-1.17318034172058 -0.630016088485718
		-1.15255427360535 -0.604009985923767
		-1.13173460960388 -0.576488733291626
		-1.11178255081177 -0.549714088439941
		-1.09272480010986 -0.522039175033569
		-1.07402420043945 -0.494268655776978
		-1.03994178771973 -0.437890291213989
		-1.02114057540894 -0.40689754486084
		-1.00359606742859 -0.380011558532715
		-0.985740184783936 -0.352035522460938
		-0.966160297393799 -0.323455572128296
		-0.946655988693237 -0.295400381088257
		-0.928175687789917 -0.26915454864502
		-0.909447908401489 -0.243585824966431
		-0.890614986419678 -0.218994379043579
		-0.871455669403076 -0.195659875869751
		-0.852315187454224 -0.173505306243896
		-0.833538293838501 -0.152174234390259
		-0.815368413925171 -0.130190372467041
		-0.796719789505005 -0.107467889785767
		-0.777974367141724 -0.0838143825531006
		-0.758872509002686 -0.0593280792236328
		-0.738310575485229 -0.0350503921508789
		-0.695259094238281 0.0125653743743896
		-0.673020362854004 0.0344295501708984
		-0.650846242904663 0.0570385456085205
		-0.630774259567261 0.078859806060791
		-0.612360239028931 0.100586652755737
		-0.59426212310791 0.122964859008789
		-0.577320337295532 0.144001483917236
		-0.561110258102417 0.163456678390503
	};
\addlegendentry{Optitrack}
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.381783 0.0592154
		-0.364625 0.0508084
		-0.364625 0.0508084
		-0.371554 0.0672772
		-0.360835 0.0816704
		-0.36961 0.0863433
		-0.36961 0.0863433
		-0.378163 0.110492
		-0.378163 0.110492
		-0.37644 0.123912
		-0.397718 0.123143
		-0.387331 0.115548
		-0.389165 0.0976984
		-0.323527 0.0589477
		-0.285971 0.0351405
		-0.285971 0.0351405
		-0.263548 0.0260154
		-0.262932 0.0305999
		-0.263875 0.0224574
		-0.263875 0.0224574
		-0.286731 0.0301188
		-0.277912 0.0232562
		-0.277912 0.0232562
		-0.278006 0.0221009
		-0.319488 0.0079212
		-0.319488 0.0079212
		-0.273895 0.00785763
		-0.320883 -0.00798876
		-0.320883 -0.00798876
		-0.314736 0.0012899
		-0.314715 0.00386943
		-0.316422 -0.00911503
		-0.338291 -0.0110463
		-0.23237 -0.0120832
		-0.413128 -0.0351242
		-0.41601 -0.0430926
		-0.347662 -0.0429384
		-0.340086 -0.044359
		-0.445696 -0.0674759
		-0.502996 -0.0756538
		-0.45199 -0.0595213
		-0.560558 -0.065127
		-0.613496 -0.0715746
		-0.495285 -0.0208981
		-0.495285 -0.0208981
		-0.403727 0.0102642
		-0.448422 -0.0076653
		-0.462492 -0.00590419
		-0.344972 0.00143738
		-0.403799 -0.00684403
		-0.442915 -0.0300281
		-0.522387 -0.0259035
		-0.522387 -0.0259035
		-0.516037 -0.0297305
		-0.449418 -0.0255766
		-0.449418 -0.0255766
		-0.573051 -0.04426
		-0.573225 -0.0419432
		-0.573051 -0.04426
		-0.398006 -0.0180911
		-0.46082 -0.0095606
		-0.403296 -0.0235256
		-0.347038 -0.0159724
		-0.346317 -0.0042932
		-0.346317 -0.0042932
		-0.344829 -0.0100575
		-0.346153 -0.0114906
		-0.348342 -0.0173448
		-0.262932 0.0305999
		-0.404336 -0.0343768
		-0.344927 -0.00574877
		-0.343124 -0.0112963
		-0.386081 -0.0389467
		-0.414541 -0.0755308
		-0.601637 -0.275957
		-0.283811 -0.447548
		-0.0444884 -0.417804
		-0.00214159 -0.436874
		0.20302 -0.205622
		0.353353 -0.126801
		0.322988 0.132547
		0.278277 0.234264
		-0.0450356 0.804634
		-0.719545 0.55697
		-0.516037 -0.0297305
		-0.39317 -0.0177248
		-0.345246 -0.0184699
		-0.404459 -0.0268521
		-0.35645 -0.0164746
		-0.342439 0
		-0.354058 -0.0105017
		-0.328358 0.00419179
		-0.330846 0.00703929
		-0.378158 -0.0178529
		-0.370145 -0.0176259
		-0.369574 -0.0270809
		-0.345523 -0.0238292
		-0.345792 -0.0195447
		-0.330701 -0.0359457
		-0.354167 -0.0292573
		-0.332152 -0.0320498
		-0.373545 -0.0557041
		-0.366831 -0.0563118
		-0.373685 -0.0587453
		-0.366586 -0.0578821
		-0.373431 -0.060336
		-0.371192 -0.0632162
		-0.371798 -0.059552
		-0.371501 -0.0613784
		-0.372288 -0.0564073
		-0.371798 -0.059552
		-0.372524 -0.0548303
		-0.371543 -0.0611197
		-0.376095 -0.0618684
		-0.384089 -0.0626412
		-0.383615 -0.0658567
		-0.385381 -0.0545819
		-0.383156 -0.0684789
		-0.387448 -0.0774896
		-0.690576 -0.168566
		-0.712648 -0.176066
		-0.6942 -0.180383
		-0.691979 -0.188722
		-0.687993 -0.191109
		-0.702374 -0.214614
		-0.698674 -0.22637
		-0.695625 -0.23557
		-0.690454 -0.250324
		-0.686534 -0.260883
		-0.70181 -0.273877
		-0.67365 -0.289097
		-0.685673 -0.289878
		-0.665234 -0.293246
		-0.61446 -0.272261
		-0.609943 -0.267475
		-0.600253 -0.278956
		-0.611394 -0.292852
		-0.617815 -0.311503
		-0.613533 -0.323594
		-0.63428 -0.350594
		-0.646887 -0.366849
		-0.631521 -0.385619
		-0.672612 -0.42998
		-0.620987 -0.404363
		-0.685552 -0.439788
		-0.619214 -0.422878
		-0.629491 -0.439108
		-0.612355 -0.452343
		-0.540327 -0.412565
		-0.515461 -0.430872
		-0.500758 -0.440772
		-0.523819 -0.465308
		-0.263318 -0.426325
		-0.246094 -0.412868
		-0.255203 -0.440006
		-0.236754 -0.451173
		-0.193853 -0.449484
		-0.201959 -0.468993
		-0.175079 -0.431445
		-0.149675 -0.415545
		-0.121107 -0.390845
		-0.123233 -0.412733
		-0.120955 -0.461828
		-0.0858287 -0.443448
		-0.0818792 -0.444194
		-0.0765375 -0.463477
		-0.0601996 -0.452534
		-0.0536388 -0.46773
		-0.053704 -0.466151
		-0.0406578 -0.418195
		-0.0329667 -0.418871
		-0.046582 -0.472475
		-0.0487774 -0.472253
		-0.0288261 -0.434451
		-0.0305126 -0.455509
		-0.0238807 -0.455905
		-0.0364211 -0.45205
		-0.0405346 -0.472904
		-0.0407271 -0.472888
		-0.0496875 -0.47203
		-0.047031 -0.45107
		-0.0467924 -0.463468
		-0.0541481 -0.471539
		-0.0511973 -0.463002
		-0.0474118 -0.465087
		-0.0309555 -0.446644
		-0.0291375 -0.450512
		0.0553709 -0.412206
		0.160205 -0.51213
		0.0759021 -0.493364
		0.150973 -0.514927
		-0.0225035 -0.409154
		0.0498491 -0.394805
		0.136327 -0.463989
		0.0532955 -0.363879
		0.14528 -0.454586
		0.138417 -0.424181
		0.150394 -0.446553
		0.240286 -0.43732
		0.151946 -0.215367
		0.151706 -0.20101
		0.201341 -0.202759
		0.198394 -0.201093
		0.303087 -0.326552
		0.26307 -0.26307
		0.261452 -0.266293
		0.316522 -0.299565
		0.370989 -0.345549
		0.387747 -0.349186
		0.462044 -0.414845
		0.457959 -0.403203
		0.409389 -0.324541
		0.377492 -0.307214
		0.386448 -0.30147
		0.26838 -0.185596
		0.320523 -0.204114
		0.304842 -0.17587
		0.338462 -0.174113
		0.500511 -0.250255
		0.307502 -0.122404
		0.386004 -0.144752
		0.348866 -0.113546
		1.68855 0.531167
		1.58247 0.532661
		0.358422 -0.147586
		0.485784 -0.212979
		0.479852 -0.171541
		0.369553 -0.118978
		0.376475 -0.0381931
		0.328826 -0.0288725
		0.297445 0.00420911
		0.297445 0.00420911
		0.31888 0.0355959
		0.328349 0.0786187
		0.328349 0.0786187
		0.335023 0.120103
		0.322988 0.132547
		0.326771 0.147277
		0.326073 0.14458
		0.325629 0.144555
		0.307711 0.15021
		0.321487 0.158479
		0.321487 0.158479
		0.29159 0.156799
		0.29159 0.156799
		0.312992 0.181445
		0.260016 0.155252
		0.302954 0.184407
		0.302954 0.184407
		0.332277 0.233763
		0.270014 0.20592
		0.270014 0.20592
		0.272107 0.222128
		0.282939 0.274098
		0.277848 0.272206
		0.249446 0.478776
		0.251216 0.562911
		0.192968 0.69415
		0.227214 0.775556
		0.227214 0.775556
		0.184308 0.720969
		0.184308 0.720969
		0.154905 0.691731
		0.152405 0.82734
		0.152405 0.82734
		0.100509 0.848041
		0.0436584 0.739465
		0.0436584 0.739465
		-0.0285402 0.846694
		-0.0450356 0.804634
		-0.0908184 0.82676
		-0.10419 0.812068
		-0.105031 0.815533
		-0.110771 0.827706
		-0.18437 0.814299
		-0.222653 0.80521
		-0.209862 0.693342
		-0.180152 0.571212
		-0.22733 0.553024
		-0.257996 0.535181
		-0.265449 0.526751
		-0.250095 0.504159
		-0.410361 0.656577
		-0.490888 0.692853
		-0.709664 0.672667
		-0.769111 0.698225
		-0.717923 0.589386
		-0.719545 0.55697
		-0.717481 0.537372
		-0.720782 0.539098
		-0.750421 0.531675
		-0.72387 0.498402
		-0.794521 0.458986
		-0.834342 0.44171
		-0.875934 0.42251
		-0.879243 0.41558
		-0.811293 0.0928047
		-0.812322 0.0833151
		-0.843488 0.0744254
		-0.840181 0.0463335
		-0.841255 0.0184891
		-0.848627 -0.0124798
		-0.830397 -0.0513337
		-0.837298 -0.0943864
		-0.905326 -0.224703
		-0.939874 -0.192708
		-0.975514 -0.184651
		-1.01926 -0.211889
		-0.99124 -0.233649
		-1.01849 -0.244585
		-1.03403 -0.27328
		-1.12221 -0.30751
		-1.11258 -0.327461
		-1.10823 -0.3419
		-1.21266 -0.367215
		-1.19182 -0.387448
		-1.26486 -0.415661
		-1.28179 -0.437796
		-1.28868 -0.467373
		-1.28309 -0.472716
		-1.28331 -0.483502
		-1.25519 -0.492318
		-1.17685 -0.485818
		-1.31106 -0.582696
		-1.32581 -0.613364
		-1.25827 -0.597453
		-1.26506 -0.653233
		-1.25072 -0.673465
		-1.14851 -0.631051
		-1.23919 -0.708109
		-1.24751 -0.747589
		-1.15291 -0.700286
		-1.17609 -0.742792
		-1.04978 -0.685328
		-1.12446 -0.759652
		-1.04974 -0.734821
		-1.03395 -0.76842
		-1.03691 -0.797302
		-1.09546 -0.870978
		-1.13422 -0.931848
		-1.12507 -0.943919
		-1.13947 -0.991484
		-1.14927 -0.98011
		-1.16155 -1.00634
		-1.14725 -1.01699
		-1.22159 -1.09836
		-1.24911 -1.14363
		-1.26247 -1.16623
		-1.18221 -1.09248
		-1.28783 -1.21173
		-1.24905 -1.15983
		-1.26054 -1.18141
		-1.24905 -1.15983
		-1.17881 -1.10022
		-1.27198 -1.19284
		-1.21445 -1.11899
		-1.17904 -1.09666
		-1.29338 -1.21964
		-1.2432 -1.16686
		-1.23481 -1.15964
		-1.26669 -1.20558
		-1.2907 -1.22247
		-1.24658 -1.18617
		-1.2246 -1.17042
		-1.28615 -1.23516
		-1.28604 -1.23527
		-1.25581 -1.21691
		-1.29169 -1.22937
		-1.26437 -1.25318
		-1.2104 -1.2104
		-1.23297 -1.24941
		-1.16666 -1.18228
		-1.25977 -1.29896
		-1.2783 -1.35892
		-1.6774 -1.80302
		-1.67066 -1.80927
		-1.67066 -1.80927
		-1.67716 -1.80899
		-1.65465 -1.8296
		-1.63915 -1.81169
		-1.65829 -1.82631
		-1.66702 -1.81325
		-1.64771 -1.83727
		-1.61811 -1.85031
		-1.36331 -1.55198
		-1.34791 -1.57968
		-1.33175 -1.55573
		-1.21425 -1.41385
		-1.34979 -1.60209
		-1.07454 -1.35217
		-1.09806 -1.39266
		-1.13394 -1.46514
		-1.13639 -1.50186
		-1.19193 -1.59938
		-1.24933 -1.72934
		-1.35374 -1.92564
		-1.25119 -1.94004
		-1.10129 -1.7138
		-1.178 -1.84732
		-1.17274 -1.92028
		-1.12542 -1.90716
		-1.25084 -2.16403
		-1.11918 -2.00607
		-1.07621 -1.99374
		-0.995488 -1.87386
		-0.915888 -1.80685
		-0.939804 -1.92626
		-0.938994 -1.93126
		-0.911593 -1.89533
		-0.730691 -1.63429
		-0.716068 -1.64075
		-0.675666 -1.59108
		-0.679175 -1.63339
		-0.587655 -1.52161
		-0.567734 -1.56395
		-0.560093 -1.63037
		-0.527054 -1.63664
		-0.501797 -1.6689
		-0.420226 -1.60111
		-0.354562 -1.51955
		-0.302418 -1.5531
		-0.294859 -1.54547
		-0.267515 -1.51592
		-0.225302 -1.73483
		-0.211361 -1.66379
		-0.140989 -1.53073
		-0.116328 -1.68398
		-0.0623394 -1.57926
		-0.0305692 -1.55904
		0.0166054 -1.67716
		0.0693092 -1.62077
		0.118352 -1.61927
		0.173668 -1.46171
		0.188131 -1.13631
		0.21169 -1.11787
		0.243928 -1.17636
		0.284487 -1.26533
		0.292074 -1.20943
		0.33226 -1.25137
		0.331772 -1.18143
		0.552123 -1.45463
		0.571173 -1.32474
		0.627187 -1.50745
		0.672738 -1.48768
		0.644563 -1.21141
		0.670925 -1.19225
		0.737979 -1.16032
		0.754414 -1.16754
		0.880029 -1.25859
		0.795352 -1.11971
		1.00861 -1.30961
		1.1422 -1.45586
		0.894273 -1.07839
		0.928825 -1.06659
		1.30722 -1.44904
		1.09088 -1.1512
		1.43026 -1.38576
		1.34329 -1.18895
		1.37535 -1.21665
		1.17882 -0.971667
		1.12752 -0.892811
		1.19255 -0.931373
		1.14428 -0.829714
		1.14428 -0.829714
		1.03654 -0.685649
		1.06225 -0.681682
		1.06225 -0.681682
		0.954364 -0.588154
		1.04394 -0.623126
		1.04394 -0.623126
		0.792675 -0.440704
		1.13851 -0.608363
		1.13851 -0.608363
		1.21296 -0.569724
		1.33151 -0.558059
		1.283 -0.50023
		1.19526 -0.449281
		1.19526 -0.449281
		1.65952 -0.440991
		1.61718 -0.353758
		1.63789 -0.313043
		1.64824 -0.279364
		1.64544 -0.238229
		1.64544 -0.238229
		1.82886 -0.146309
		1.83244 -0.0910153
		1.83244 -0.0910153
		1.47251 -0.038497
		1.38174 -0.0315055
		1.38174 -0.0315055
		1.34339 0.00439013
		1.39397 0.022852
		1.37279 0.0855181
		1.6897 0.174023
		1.82501 0.211508
		1.82122 0.242022
		1.78481 0.261772
		1.69445 0.285261
		1.76105 0.395337
		1.71716 0.450016
		1.71348 0.527225
		1.66342 0.673567
		1.67214 0.741198
		1.63325 0.790655
		1.63325 0.790655
		1.61231 0.823429
		1.59455 0.857283
		1.59455 0.857283
		1.46841 0.927989
		1.46841 0.927989
		1.47599 0.983996
		1.34558 0.974388
		1.34558 0.974388
		1.33877 0.988391
		1.41438 1.16242
		1.19584 1.09207
		0.773188 1.63829
		0.784689 1.74565
		0.677566 1.68591
		0.215202 1.10334
		0.194579 1.14625
		0.189273 0.992158
		0.444737 1.51025
		0.67913 1.86761
		0.688654 1.86412
		0.519035 1.65285
		0.514363 1.74459
		0.31485 1.45181
		0.342553 1.64823
		0.339947 1.70489
		0.316228 1.69335
		0.309637 1.80893
		0.419484 1.98799
		0.0985986 1.24386
		0.0651912 1.13722
		0.0809465 1.13325
		0.0826989 1.21292
		0.0709654 1.24584
		-0.0819605 1.68531
		-0.0783615 1.47504
		-0.0444049 1.41651
		-0.0691895 1.47604
		-0.0827094 1.4658
		-0.0954157 1.51711
		-0.106841 1.54434
		-0.100798 1.51676
		-0.12419 1.47189
		-0.134925 1.47953
		-0.125222 1.43558
		-0.75206 1.87714
		-0.845908 1.79031
		-0.966248 1.79608
		-0.905655 1.79401
		-0.958038 1.67251
		-1.0065 1.71664
		-0.962706 1.72391
		-0.977458 1.6471
		-1.01196 1.70346
		-0.915909 1.64535
		-0.907055 1.61934
		-1.42377 0.845206
		-1.30581 0.696433
		-1.3729 0.337367
		-1.855 0.373449
		-1.8446 0.367694
		-1.79718 0.336596
		-1.37965 0.209743
		-1.39674 0.141562
		-1.55869 0.10984
		-1.545 0.0826755
		-1.33359 0.0450535
		-1.35284 0.00914075
		-1.726 -0.0396131
		-1.66049 -0.0544425
		-1.5365 -0.0668041
		-1.59249 -0.0905428
		-1.72644 -0.120851
		-1.6259 -0.151247
		-1.62515 -0.195018
		-1.29082 -0.175621
		-1.49509 -0.285974
		-1.32306 -0.282552
		-1.29197 -0.313072
		-1.30806 -0.341624
		-1.29835 -0.38636
		-1.31245 -0.425288
		-1.29803 -0.422087
		-1.18679 -0.402588
		-1.23866 -0.449619
		-1.19526 -0.464346
		-1.09835 -0.46789
		-1.08326 -0.496657
		-1.09909 -0.53948
		-1.10339 -0.626363
		-1.04235 -0.804468
		-1.04813 -0.847428
		-1.02492 -0.8645
		-1.25819 -0.484602
		-1.03985 -0.816726
		-1.17422 -1.10181
		-1.16666 -1.18228
		-1.20726 -1.46352
		-0.959369 -1.91208
		-0.258759 -1.68469
		0.4718 -1.49492
		1.32163 -1.19791
		1.21915 -0.53733
		1.34339 0.00439013
		1.58932 0.981641
		0.514561 1.55811
		-0.0574938 1.41523
		-0.545078 1.74317
		-1.76135 0.381626
		-1.11061 -1.00872
		-0.960876 -0.907246
		-1.02243 -1.00286
		-1.02249 -1.02748
		-0.973367 -1.0269
		-0.958644 -1.06136
		-0.856865 -1.02285
		-0.757564 -0.941837
		-0.786958 -0.991307
		-0.741897 -1.00325
		-0.694372 -0.972121
		-0.665576 -0.986336
		-0.657275 -0.991887
		-0.60182 -0.965183
		-0.559121 -0.961688
		-0.472299 -0.948203
		-0.432444 -0.963837
		-0.359103 -0.961234
		-0.33606 -0.946751
		-0.297999 -0.959412
		-0.25461 -0.940642
		-0.221208 -0.949053
		-0.197559 -0.973159
		-0.175208 -0.974596
		-0.12117 -1.01859
		-0.0342976 -1.02512
		0.0380602 -1.03524
		0.108453 -1.04192
		0.147509 -0.988307
		0.209058 -1.05735
		0.267483 -1.04198
		0.323302 -0.981317
		0.333885 -0.92082
		0.393053 -0.880022
		0.452488 -0.856619
		0.475831 -0.79966
		0.499095 -0.794612
		0.452434 -0.661685
		0.445757 -0.625147
		0.583597 -0.81151
		0.648884 -0.747094
		0.706477 -0.764743
		0.692397 -0.717
		0.686679 -0.659484
		0.717725 -0.59421
		0.77818 -0.621116
		0.764994 -0.572082
		0.675891 -0.478635
		0.675891 -0.478635
		0.706057 -0.457201
		0.780319 -0.473878
		0.882527 -0.466819
		0.827228 -0.402521
		0.827228 -0.402521
		0.998673 -0.379724
		1.04233 -0.295
		1.04233 -0.295
		1.03159 -0.255958
		1.02947 -0.237277
		1.02947 -0.237277
		0.84016 -0.168645
		0.853555 -0.134937
		0.853555 -0.134937
		0.87523 -0.0865611
		0.877594 -0.0578633
		0.877594 -0.0578633
		0.969341 0.0246741
		0.790304 0.0318438
		0.805164 0.0787661
		0.815981 0.101253
		0.815981 0.101253
		1.06613 0.213226
		1.11518 0.275662
		1.11518 0.275662
		1.15282 0.451483
		1.05057 0.463367
		1.16311 0.570241
		1.06999 0.564028
		1.14686 0.715098
		1.14686 0.715098
		0.989498 0.697773
		0.823625 0.62104
		0.823625 0.62104
		0.860501 0.655785
		0.866304 0.74568
		0.859771 0.767521
		0.77105 0.774721
		0.77105 0.774721
		0.779528 0.828961
		0.71543 0.84212
		0.663479 0.806651
		-0.109667 1.52104
		-0.100166 1.5168
		-0.121891 1.52832
		-0.162115 1.73619
		-0.122548 1.58332
		-0.21409 1.98033
		-0.175503 1.82084
		-0.124483 1.81313
		-0.220382 1.95444
		-0.160304 1.74783
		-0.185957 1.61639
		-0.308305 1.96617
		-0.420337 1.96157
		-0.160083 1.53491
		-0.143601 1.55089
		-0.58678 1.97207
		-0.714022 2.25991
		-0.711293 2.2084
		-0.91876 2.30793
		-0.812836 2.02884
		-1.01621 2.29752
		-1.02828 2.1475
		-1.01385 2.04096
		-0.949425 1.6978
		-0.969041 1.7362
		-0.877883 1.51359
		-1.02204 1.68637
		-1.02953 1.62096
		-1.18785 1.86391
		-1.27287 1.98002
		-1.30818 1.94892
		-1.30352 1.93873
		-1.25985 1.83989
		-1.2258 1.75457
		-1.32714 1.82795
		-1.17442 1.61
		-1.15435 1.54983
		-1.20201 1.55489
		-1.34393 1.66937
		-1.22974 1.51687
		-1.60331 1.81941
		-1.71462 1.90595
		-1.71868 1.90229
		-1.75119 1.88475
		-1.88928 1.99995
		-1.78771 1.87033
		-1.91905 1.95903
		-1.86277 1.87044
		-1.92583 1.9103
		-2.00704 1.95129
		-2.0109 1.94731
		-2.034 1.94591
		-2.14706 1.95039
		-2.16445 1.94139
		-2.19347 1.92338
		-2.25658 2.00208
		-2.17665 1.90863
		-2.18946 1.88132
		-2.13558 1.82037
		-2.19551 1.83361
		-2.26893 1.84814
		-2.48439 1.98931
		-2.41226 1.90534
		-2.31945 1.82541
		-2.34461 1.80678
		-2.48019 1.87786
		-2.46618 1.84526
		-2.56835 1.87445
		-2.64816 1.89417
		-2.66763 1.89226
		-2.67836 1.85284
		-2.78894 1.85299
		-2.66304 1.7395
		-2.82293 1.84394
		-2.76938 1.74471
		-2.73109 1.66951
		-2.95808 1.76309
		-2.83011 1.65323
		-2.97698 1.67334
		-2.94804 1.58814
		-2.97322 1.47236
		-2.74757 1.34326
		-2.71101 1.31288
		-2.72328 1.26803
		-2.59336 1.17953
		-2.58497 1.15961
		-2.59228 1.14318
		-2.61459 1.13783
		-2.63012 1.11679
		-2.76025 1.15291
		-2.81446 1.12065
		-3.04411 1.14385
		-3.07309 1.10818
		-3.01992 1.04009
		-3.19181 1.07361
		-3.19857 1.0533
		-3.24984 1.04739
		-3.18568 1.00449
		-3.42922 1.05436
		-3.31685 0.987157
		-3.33031 0.965594
		-3.27769 0.911548
		-3.05253 0.837419
		-3.26171 0.875561
		-3.29821 0.834254
		-3.27048 0.820032
		-3.29381 0.782402
		-3.17762 0.752593
		-3.19843 0.710762
		-3.11259 0.635222
		-3.2896 0.602456
		-3.37477 0.549382
		-3.37744 0.510543
		-3.16968 0.486936
		-3.23406 0.45933
		-3.38711 0.441797
		-3.22063 0.361973
		-3.34043 0.36476
		-3.24715 0.335912
		-3.2499 0.30818
		-3.3536 0.289104
		-3.35739 0.241192
		-3.53392 0.254605
		-3.40791 0.206839
		-3.43041 0.15772
		-3.41954 0.137568
		-3.37261 0.0872227
		-3.39158 0.0389838
		-3.40971 -0.00977015
		-3.38996 -0.107154
		-3.43796 -0.11855
		-3.23645 -0.139103
		-3.4041 -0.195638
		-3.2318 -0.222244
		-3.23048 -0.240666
		-3.26047 -0.280269
		-3.31243 -0.314109
		-3.39824 -0.351542
		-3.34416 -0.357613
		-3.46292 -0.411535
		-3.38523 -0.419496
		-3.47719 -0.443468
		-3.45537 -0.470732
		-3.39148 -0.505748
		-3.39154 -0.556968
		-3.24086 -0.560736
		-3.22911 -0.609626
		-3.33971 -0.662013
		-3.33971 -0.662013
		-3.4263 -0.74
		-3.33129 -0.758903
		-3.33129 -0.758903
		-2.95953 -0.759761
		-2.73446 -0.718305
		-2.63038 -0.73241
		-2.84975 -0.832608
		-2.86785 -0.886427
		-2.59338 -0.851322
		-2.56497 -0.93343
		-2.7939 -1.05202
		-2.7939 -1.05202
		-2.77837 -1.0853
		-2.77837 -1.0853
		-2.75817 -1.15215
		-2.724 -1.14649
		-2.724 -1.14649
		-2.73907 -1.22029
		-2.49734 -1.125
		-2.44624 -1.1484
		-2.44017 -1.16124
		-2.62863 -1.30578
		-2.62863 -1.30578
		-2.30749 -1.22117
		-2.51812 -1.36159
		-2.51812 -1.36159
		-2.58731 -1.4687
		-2.53155 -1.46342
		-2.53155 -1.46342
		-2.51136 -1.53378
		-2.55102 -1.5792
		-1.01747 -0.878523
		-0.384638 -0.96709
		0.443209 -0.862368
		0.780319 -0.473878
		0.789427 0.048979
		0.866304 0.74568
		-0.148618 1.80465
		-1.33831 2.04929
		-1.75102 1.87609
		-2.53339 2.03773
		-2.98117 1.71613
		-3.18987 1.07935
		-3.37297 0.539282
		-3.23932 -0.0278453
		-3.26843 -0.596007
		-2.79788 -1.82938
		-2.67977 -1.76771
		-2.67977 -1.76771
		-2.39377 -1.66186
		-2.42331 -1.71469
		-2.42331 -1.71469
		-2.41198 -1.7454
		-2.41198 -1.7454
		-2.3319 -1.74035
		-2.06808 -1.6068
		-2.06808 -1.6068
		-1.95211 -1.54421
		-1.90625 -1.54793
		-1.90625 -1.54793
		-1.97044 -1.64203
		-1.91342 -1.64217
		-1.91342 -1.64217
		-1.89897 -1.75522
		-1.89897 -1.75522
		-1.90984 -1.80973
		-1.92202 -1.85112
		-1.85257 -1.85257
		-2.06337 -2.09834
		-2.03439 -2.10394
		-2.04605 -2.12508
		-1.89461 -2.01872
		-1.84869 -2.00275
		-1.78437 -1.98441
		-1.76374 -1.99623
		-1.68978 -1.97658
		-1.67011 -2.00098
		-1.66675 -2.00803
		-1.60243 -1.97993
		-1.57283 -1.96416
		-1.54144 -2.05012
		-1.51681 -2.09538
		-1.49994 -2.12819
		-1.46954 -2.09602
		-1.48704 -2.15147
		-1.52017 -2.34395
		-1.52017 -2.34395
		-1.53164 -2.40563
		-1.38451 -2.2619
		-1.29712 -2.25415
		-1.3118 -2.28764
		-1.28638 -2.24332
		-1.09528 -2.0563
		-1.08131 -2.06368
		-1.16371 -2.25851
		-1.04885 -2.09769
		-1.08683 -2.21062
		-1.02993 -2.2377
		-1.1222 -2.35428
		-1.01845 -2.32789
		-0.967737 -2.46773
		-0.98167 -2.46222
		-0.941294 -2.47794
		-0.895692 -2.50148
		-0.891527 -2.49627
		-0.843771 -2.46763
		-0.843771 -2.46763
		-0.819914 -2.47566
		-0.78121 -2.41324
		-0.764941 -2.41845
		-0.690719 -2.39854
		-0.667272 -2.51816
		-0.669244 -2.51763
		-0.654327 -2.52155
		-0.588638 -2.54546
		-0.50348 -2.49416
		-0.494257 -2.60903
		-0.409662 -2.63003
		-0.383083 -2.5174
		-0.348755 -2.61971
		-0.301145 -2.62892
		-0.286817 -2.63052
		-0.269772 -2.63232
		-0.222295 -2.65108
		-0.196527 -2.65311
		-0.163909 -2.65533
		-0.131753 -2.65977
		-0.0992353 -2.67935
		-0.0655763 -2.66403
		-0.024477 -2.65166
		0.0326349 -2.65158
		2.69079 -0.39619
		2.67586 -0.0970099
		2.41167 -0.0292323
		2.41167 -0.0292323
		2.48704 0.0302377
		2.48585 0.0828617
		2.48585 0.0828617
		2.41226 0.176507
		2.41226 0.176507
		2.54767 0.194182
		2.42475 0.206362
		2.51972 0.238144
		2.62013 0.255623
		2.40092 0.292796
		2.40092 0.292796
		2.4052 0.315315
		2.53428 0.37087
		2.51912 0.416002
		2.52369 0.432192
		2.55485 0.46878
		2.51276 0.491793
		2.61315 0.545075
		2.63525 0.600026
		2.62353 0.631591
		2.58338 0.655844
		2.57953 0.670838
		2.64691 0.715159
		2.54771 0.76671
		2.54771 0.76671
		2.6251 0.817248
		2.7273 0.897591
		2.75524 0.950382
		2.73841 0.979242
		2.70739 1.03139
		2.73715 1.08963
		2.74171 1.17377
		2.56602 1.14687
		2.48967 1.14846
		2.43901 1.15656
		2.43901 1.15656
		2.4496 1.17327
		2.38653 1.26021
		2.38653 1.26021
		2.5062 1.39978
		2.43485 1.39718
		2.46914 1.405
		2.4855 1.46452
		2.46885 1.49805
		2.46885 1.49805
		2.42946 1.52048
		2.51279 1.578
		2.62646 1.68202
		2.48303 1.61269
		2.45377 1.61898
		2.55237 1.70745
		2.58278 1.75735
		2.54624 1.77706
		2.55956 1.80516
		2.57908 1.85258
		2.59878 1.90516
		2.54981 1.93968
		2.5407 1.9812
		2.2608 1.92002
		-0.86162 3.0329
		-0.86162 3.0329
		-0.86162 3.0329
		-0.905599 3.03591
		-0.97544 3.24218
		-0.919022 3.02583
		-1.06205 3.31053
		-1.08502 3.30307
		-1.05293 2.98759
		-1.11557 3.04805
		-1.14638 3.03659
		-1.08226 2.83682
		-1.29437 3.35359
		-1.15931 3.00368
		-1.42004 3.36638
		-1.41373 3.28571
		-1.48111 3.23151
		-1.45958 3.22643
		-1.87105 3.96854
		-1.54855 3.23346
		-1.96787 3.94775
		-1.96497 3.80205
		-2.07801 3.79412
		-2.34841 3.87731
		-2.40252 3.901
		-3.07039 3.21265
		-3.07085 3.22558
		-3.38282 2.92859
		-3.41048 2.87574
		-3.41377 2.85666
		-3.39318 2.81786
		-3.39162 2.79516
		-3.40692 2.75354
		-3.43284 2.74159
		-3.38526 2.69203
		-3.37578 2.67537
		-3.40485 2.67524
		-3.4522 2.67984
		-3.48343 2.68047
		-3.48948 2.60532
		-3.47084 2.53058
		-3.48471 2.49738
		-3.58204 2.44283
		-3.63055 2.43613
		-3.63159 2.3858
		-3.56055 2.3201
		-3.66447 2.32553
		-3.58932 2.24763
		-3.62013 2.23664
		-3.63605 2.20472
		-3.66951 2.21336
		-3.77095 2.21961
		-3.78355 2.19806
		-3.78137 2.20181
		-3.73582 2.12636
		-3.66337 2.06065
		-3.7339 2.08214
		-3.709 2.02728
		-3.7595 2.0422
		-3.72784 1.96082
		-3.68062 1.90221
		-3.67638 1.86047
		-3.78274 1.88565
		-3.70143 1.8004
		-3.73891 1.7681
		-3.76704 1.7369
		-3.81484 1.70694
		-3.68252 1.58767
		-3.75276 1.54131
		-3.75984 1.52396
		-3.78998 1.52046
		-3.76536 1.49948
		-3.78421 1.46917
		-3.78261 1.43517
		-3.74411 1.39036
		-3.76385 1.37567
		-3.8875 1.3335
		-3.90121 1.29284
		-3.91521 1.2861
		-3.93941 1.25604
		-3.94132 1.2338
		-3.9327 1.20481
		-3.93118 1.16689
		-3.92098 1.15257
		-3.88156 1.09308
		-3.88868 1.08081
		-3.82504 1.03233
		-3.80814 1.00613
		-3.84757 0.997519
		-3.87825 0.964022
		-3.93131 0.965978
		-3.84026 0.894607
		-3.93051 0.88825
		-3.9637 0.779378
		-3.92085 0.704872
		-3.92463 0.683503
		-3.93444 0.676059
		-4.05409 0.681361
		-4.05775 0.659242
		-3.99188 0.613277
		-3.99834 0.569596
		-4.0014 0.547678
		-4.00181 0.544691
		-4.00769 0.499574
		-4.0102 0.478997
		-4.0278 0.446293
		-4.04804 0.438538
		-4.0381 0.426244
		-4.04552 0.357615
		-4.05589 0.325819
		-4.04846 0.268406
		-4.0495 0.221284
		-4.08206 -0.0334597
		-3.69538 -1.25379
		-3.59904 -1.33741
		-3.40392 -1.29328
		-3.56591 -1.34809
		-3.3786 -1.30986
		-3.33536 -1.28913
		-3.39306 -1.30502
		-3.33126 -1.29549
		-3.37999 -1.3104
		-3.41547 -1.33466
		-3.1975 -1.25722
		-3.1975 -1.25722
		-3.1975 -1.25722
		-3.17 -1.25622
		-2.55102 -1.5792
		-1.86089 -1.62918
		-1.54144 -2.05012
		-1.06908 -2.21926
		-0.635527 -2.53416
		0.0334612 -2.72708
		2.53428 0.37087
		2.70739 1.03139
		2.47058 1.55462
		-1.08779 2.99574
		-2.44285 3.87616
		-3.54178 2.44301
		-3.76331 2.01482
		-3.78501 1.35731
		-3.9573 0.847196
		-0.892338 -0.18752
		-1.3059 -0.205023
		-2.77712 -1.12304
		-4.05589 0.325819
		0.100003 -1.06541
		0.202167 0.243605
		-1.11628 3.02361
		-3.17 -1.25622
		-3.18821 -1.27331
		-3.1454 -1.24058
		-2.90911 -1.15642
		-2.9154 -1.14986
		-2.75031 -1.0967
		-2.77724 -1.11609
		-2.77724 -1.11609
		-2.7794 -1.12045
		-2.75566 -1.09365
		-2.50858 -0.998713
		-2.44822 -0.985446
		-2.47562 -0.980905
		-2.47361 -0.95979
		-2.47361 -0.95979
		-2.46191 -0.941544
		-2.49977 -0.94228
		-2.49376 -0.90894
		-2.30713 -0.850755
		-2.29181 -0.840569
		-2.32947 -0.837152
		-2.23873 -0.807067
		-2.24539 -0.788351
		-2.24977 -0.775782
		-2.24759 -0.782075
		-2.24298 -0.782926
		-2.21653 -0.731872
		-2.27341 -0.741018
		-2.27223 -0.71187
		-2.27952 -0.688158
		-2.23364 -0.653235
		-2.26054 -0.591877
		-2.25927 -0.563036
		-2.04253 -0.496135
		-2.03976 -0.455417
		-2.04274 -0.441846
		-2.04508 -0.430881
		-1.92606 -0.402278
		-1.77043 -0.354085
		-1.81417 -0.341968
		-1.81726 -0.325133
		-1.86138 -0.297346
		-1.95067 -0.301524
		-1.79392 -0.260408
		-1.7754 -0.2421
		-1.77763 -0.22509
		-1.91593 -0.22178
		-1.86705 -0.196845
		-1.84798 -0.159921
		-1.84889 -0.149104
		-1.84701 -0.130657
		-1.81726 -0.0519217
		-1.83276 -0.0523646
		-1.99432 -0.0314562
		-1.90235 0.0240805
		-1.83318 0.0350289
		-1.8576 0.0844363
		-1.93221 0.139831
		-1.77916 0.174427
		-1.77603 0.203807
		-1.82403 0.234004
		-1.77764 0.249701
		-1.91049 0.301656
		-1.84947 0.332905
		-1.87861 0.378243
		-1.89791 0.450989
		-1.8878 0.489198
		-1.32214 0.388068
		-1.32072 0.435655
		-1.30061 0.457705
		-1.31609 0.52829
		-1.27822 0.52845
		-1.24456 0.525185
		-1.25114 0.562563
		-1.35696 0.629666
		-1.18715 0.615889
		-1.21606 0.630886
		-1.20077 0.634369
		-1.12789 0.656857
		-1.10181 0.699226
		-1.05757 0.7009
		-0.987958 0.684569
		-0.971186 0.727407
		-0.054006 0.82146
		-0.0607356 0.877631
		-0.00907057 0.876818
		-0.00283915 0.826174
		0.0507312 0.825791
		0.0415824 0.809471
		0.0879237 0.882269
		0.129963 0.935733
		0.145717 0.720918
		0.266995 0.792373
		0.395538 0.996307
		0.312152 0.823225
		0.297869 0.751632
		0.412592 0.888404
		0.362147 0.71068
		0.381034 0.685331
		0.390484 0.669029
		0.398873 0.653849
		0.504596 0.750888
		0.525829 0.671086
		0.575764 0.693393
		0.583922 0.676608
		0.637042 0.682085
		0.61049 0.628805
		0.66998 0.660128
		0.674138 0.629196
		0.684408 0.598058
		0.754016 0.632958
		0.862394 0.662801
		0.897249 0.657729
		0.918078 0.643407
		0.931884 0.637605
		0.927527 0.594665
		0.956697 0.554277
		0.883823 0.489072
		0.858765 0.431053
		0.903708 0.289605
		0.915702 0.249099
		0.935868 0.221465
		0.926381 0.205862
		0.927287 0.201738
		0.931147 0.162862
		0.954894 0.118911
		0.970156 0.0988461
		0.971527 0.0843212
		0.931046 0.0351338
		0.957772 -0.00362801
		1.05879 -0.0275521
		1.07804 -0.0571688
		0.967437 -0.543192
		0.967437 -0.543192
		0.819554 -0.503059
		0.859691 -0.563732
		0.762592 -0.524282
		0.818458 -0.723729
		0.751699 -0.726156
		0.685427 -0.843306
		0.653952 -0.782598
		0.653952 -0.782598
		0.644001 -0.872161
		0.658479 -0.915636
		0.658479 -0.915636
		0.615993 -0.916477
		0.591848 -0.898733
		0.581118 -0.945742
		0.57175 -0.986855
		0.56376 -0.991441
		0.56376 -0.991441
		0.483871 -1.01495
		0.44904 -1.01625
		0.425128 -1.11809
		0.431773 -1.24313
		0.373882 -1.1259
		0.3371 -1.08847
		0.33568 -1.11479
		0.33568 -1.11479
		0.284744 -1.12247
		0.23827 -1.04385
		0.23827 -1.04385
		0.195106 -0.993597
		0.184085 -1.02351
		0.184085 -1.02351
		0.145305 -1.02803
		0.126076 -1.02302
		0.0979451 -1.00394
		0.0737543 -1.051
		0.0737543 -1.051
		0.0250366 -1.01219
		0.0250366 -1.01219
		0.0104828 -1.01334
		-0.028219 -0.991189
		-0.028219 -0.991189
		-0.0445593 -0.990589
		-0.128929 -1.3077
		-0.128929 -1.3077
		-0.184322 -1.42476
		-0.184322 -1.42476
		-0.207841 -1.43968
		-0.186285 -1.25077
		-0.21496 -1.28976
		-0.271712 -1.429
		-0.284935 -1.41959
		-0.292557 -1.19604
		-0.317805 -1.18962
		-0.353933 -1.19129
		-0.361842 -1.18891
		-0.410037 -1.11828
		-0.426812 -1.14944
		-0.44968 -1.11587
		-0.52183 -1.233
		-0.487166 -1.12684
		-0.509126 -1.11583
		-0.515185 -1.1106
		-0.529779 -1.10618
		-0.531434 -1.10538
		-0.538251 -1.05204
		-0.545994 -1.04683
		-0.561103 -1.0321
		-0.580134 -1.01938
		-0.625583 -1.04839
		-0.608359 -1.02953
		-0.626075 -0.993372
		-0.669987 -1.03344
		-0.684415 -1.01363
		-0.696734 -0.9972
		-0.7017 -0.993712
		-0.689826 -0.93187
		-0.700047 -0.881827
		-0.727461 -0.867507
		-0.698076 -0.824324
		-0.70346 -0.801871
		-0.688932 -0.773291
		-0.757068 -0.828632
		-0.757068 -0.828632
		-0.715575 -0.761175
		-0.701855 -0.728849
		-0.768088 -0.782789
		-0.766025 -0.766025
		-0.792976 -0.781701
		-0.822547 -0.784289
		-0.803644 -0.773461
		-0.825807 -0.79508
		-0.799882 -0.77735
		-0.752548 -0.748981
		-0.687829 -0.704128
		-0.783481 -0.802315
		-0.719273 -0.757681
		-0.728191 -0.78978
		-0.759577 -0.831736
		-0.699921 -0.780412
		-0.675451 -0.772439
		-0.67801 -0.819262
		-0.645328 -0.77305
		-0.640708 -0.818296
		-0.625511 -0.866937
		-0.596105 -0.909249
		-0.609539 -0.980913
		-0.590943 -0.997216
		-0.576425 -1.00568
		-0.528293 -0.963358
		-0.494513 -0.973573
		-0.449776 -0.99261
		-0.442499 -0.992737
		-0.377173 -0.957723
		-0.361121 -1.01347
		-0.339418 -1.02606
		-0.300135 -0.99795
		-0.27425 -0.993229
		-0.241344 -0.965378
		-0.204745 -0.966251
		-0.18059 -0.941151
		-0.181978 -1.01016
		-0.143594 -1.00516
		-0.109568 -1.039
		-0.0815001 -1.08667
		-0.0693456 -1.07486
		-0.055797 -1.03782
		-0.0450847 -1.05198
		-0.01094 -1.0393
		0.0363997 -1.03011
		0.043978 -1.02982
		0.05514 -1.02928
		0.0626896 -1.02885
		0.0910626 -1.04722
		0.089301 -1.0344
		0.0959828 -1.02628
		0.104012 -1.03641
		0.0952516 -1.04015
		0.100615 -1.01333
		0.0843131 -1.06924
		0.0772916 -1.07822
		0.0717434 -1.05727
		0.0663996 -1.08973
		0.0651871 -1.066
		0.0668313 -1.03588
		0.0498876 -1.06683
		0.0450895 -1.03706
		-0.00786015 -1.07291
		-0.0353226 -1.0793
		-0.0595326 -1.08746
		-0.0635725 -1.1006
		-0.0728687 -1.09708
		-0.105179 -1.0882
		-0.129697 -0.972723
		-0.166402 -1.02163
		-0.203408 -1.02486
		-3.1454 -1.24058
		-2.48855 -0.935138
		-2.13539 -0.488662
		-1.7989 -0.0756816
		-1.3116 0.410156
		-0.0386263 0.855722
		0.572101 0.782529
		0.851005 0.352936
		0.859691 -0.563732
		0.469027 -1.07265
		0.0591531 -1.05366
		-0.333751 -1.18524
		-0.606162 -1.00606
		-0.791372 -0.783871
		-0.59579 -0.882652
		-0.160797 -0.997671
		-0.245628 -0.963904
		-0.271993 -0.932028
		-0.311446 -0.956851
		-0.349247 -0.94371
		-0.400779 -0.93025
		-0.439231 -0.915065
		-0.501063 -0.934313
		-0.563395 -0.964119
		-0.58473 -0.956112
		-0.570831 -0.858088
		-0.592071 -0.847904
		-0.630152 -0.85301
		-0.627349 -0.826448
		-0.692815 -0.86298
		-0.744933 -0.860171
		-0.747855 -0.801547
		-1.14505 -0.125429
		-1.15768 -0.0647655
		-1.16241 -0.0407863
		-1.18831 0
		-1.10485 0.0193156
		-1.16094 0.0369202
		-1.13234 0.060018
		-1.13188 0.0682336
		-1.21282 0.107902
		-1.14663 0.122416
		-1.17338 0.171205
		-1.13066 0.220519
		-1.14317 0.246408
		-1.0817 0.23952
		-1.18225 0.298763
		-1.2054 0.305716
		-1.19666 0.345607
		-1.17504 0.390266
		-1.16711 0.424404
		-1.19441 0.458725
		-1.18785 0.451901
		-1.18313 0.477552
		-1.17786 0.508523
		-1.17628 0.512179
		-1.14883 0.534141
		-1.00156 0.515729
		-0.929561 0.520276
		-0.915356 0.533384
		-0.907844 0.546072
		-0.945032 0.592891
		-0.952518 0.626561
		-0.94601 0.65242
		-0.875637 0.624964
		-0.826755 0.657338
		-0.623887 1.04766
		-0.538433 0.996284
		-0.449292 0.982826
		-0.453025 0.969758
		-0.453025 0.969758
		-0.384827 1.10783
		-0.261647 0.963788
		-0.261647 0.963788
		-0.207164 1.05011
		-0.186711 1.05563
		-0.186711 1.05563
		-0.142173 1.11868
		-0.142173 1.11868
		-0.175132 1.20964
		-0.12663 1.10988
		-0.113849 1.17382
		-0.113849 1.17382
		-0.0596814 1.18169
		-0.0955423 1.24205
		0.00840368 1.25215
		0.0371744 1.23089
		0.0371744 1.23089
		0.0506762 1.08592
		0.115015 1.31383
		0.115015 1.31383
		0.143123 1.25443
		0.127311 1.25613
		0.127311 1.25613
		0.305539 1.15867
		0.305539 1.15867
		0.405468 1.18774
		0.484268 1.21067
		0.484268 1.21067
		0.44666 1.04721
		0.517837 1.00238
		0.545236 0.921879
		0.574181 0.914301
		0.574181 0.914301
		0.684307 0.979337
		0.652 0.839315
		0.652 0.839315
		0.539968 0.66702
		0.610779 0.729097
		0.610779 0.729097
		0.622924 0.723501
		0.718703 0.753762
		0.762439 0.788473
		0.688898 0.675776
		0.770406 0.706205
		0.709225 0.621786
		0.693454 0.57942
		0.736512 0.580282
		0.821003 0.602977
		0.862857 0.591673
		0.88319 0.591197
		0.893172 0.576005
		0.857731 0.524362
		1.11812 0.602063
		0.870475 0.480502
		0.831837 0.412591
		0.842276 0.394185
		0.904982 0.391441
		0.895531 0.346885
		0.872628 0.296624
		0.92036 0.274303
		0.89373 0.225192
		0.907348 0.192144
		0.869877 0.16033
		0.842877 0.124628
		0.881983 0.0786264
		0.88418 0.0479788
		0.884942 0.0308701
		0.852041 0
		0.871751 -0.0134633
		0.85117 -0.0331195
		0.892058 -0.0694208
		0.895444 -0.109287
		0.69264 -0.114531
		0.676477 -0.158549
		0.648243 -0.158232
		0.629602 -0.176687
		0.504669 -0.209106
		0.603258 -0.27619
		0.68827 -0.335741
		0.686267 -0.355842
		0.555341 -0.307751
		0.746617 -0.464998
		0.713442 -0.462944
		0.657387 -0.427592
		0.58794 -0.410191
		0.641317 -0.455913
		0.633639 -0.469136
		0.629777 -0.475303
		0.598801 -0.469252
		0.631851 -0.511196
		0.593041 -0.532217
		0.515163 -0.501462
		0.038477 -0.930443
		0.0270692 -0.893285
		0.0128902 -0.828192
		-0.0218781 -0.806366
		-0.0669146 -0.747698
		-0.110229 -0.833199
		-0.183707 -0.887342
		-0.219053 -0.883058
		-0.259301 -0.891994
		-0.266922 -0.90262
		-0.308238 -0.954423
		-0.293068 -0.882653
		-0.343347 -0.940471
		-0.362365 -0.958756
		-0.402078 -0.953499
		-0.418371 -0.952957
		-0.475352 -0.970348
		-0.499773 -0.97178
		-0.519473 -0.971015
		-0.544528 -0.964935
		-0.570223 -0.913127
		-0.57319 -0.889953
		-0.571908 -0.867208
		-0.544774 -0.772041
		-0.543641 -0.734563
		-0.588826 -0.778214
		-0.5793 -0.739107
		-0.596484 -0.755772
		-0.591415 -0.704527
		-0.606634 -0.716628
		-0.614911 -0.706134
		-0.606427 -0.697899
		-0.619923 -0.701224
		-0.610028 -0.694754
		-0.630727 -0.696572
		-0.624614 -0.68673
		-0.658566 -0.72479
		-0.656009 -0.726033
		-0.66919 -0.718063
		-0.64183 -0.681272
		-0.618291 -0.652833
		-0.597885 -0.631101
		-0.627972 -0.667445
		-0.596127 -0.632761
		-0.591236 -0.631548
		-0.584573 -0.611145
		-0.582917 -0.612725
		-0.547623 -0.562585
		-0.551816 -0.557814
		-0.555262 -0.558296
		-0.497562 -0.487032
		-0.506047 -0.500663
		-0.519561 -0.508447
		-0.507458 -0.493817
		-0.522316 -0.51673
		-0.478854 -0.503765
		-0.532813 -0.521416
		-0.498416 -0.520943
		-0.504141 -0.501445
		-0.513339 -0.50506
		-0.497566 -0.511701
		-0.459504 -0.483688
		-0.469206 -0.523236
		-0.46944 -0.513364
		-0.423468 -0.495833
		-0.45212 -0.523797
		-0.387112 -0.47476
		-0.364887 -0.456109
		-0.43643 -0.519432
		-0.366496 -0.437064
		-0.377046 -0.453441
		-0.37126 -0.445994
		-0.363825 -0.461011
		-0.356852 -0.462399
		-0.30431 -0.525136
		-0.241222 -0.452578
		-0.223003 -0.434856
		-0.165194 -0.444923
		-0.0637543 -0.386169
		0.228163 -0.236666
		0.198905 -0.203847
		0.224397 -0.237098
		0.212848 -0.261094
		0.194238 -0.231055
		0.24567 -0.247159
		0.221471 -0.221471
		0.297018 -0.289904
		0.216299 -0.204781
		0.24499 -0.242073
		0.343282 -0.32532
		0.344398 -0.324139
		0.236786 -0.157858
		0.24442 -0.159813
		0.297792 -0.186947
		0.274202 -0.160688
		0.318705 -0.175467
		0.238005 -0.119646
		0.279183 -0.111103
		0.274804 -0.0897027
		0.304287 -0.0906386
		0.348224 -0.0532996
		0.281487 -0.0296302
		0.243204 -0.0117679
		0.249176 0.0265081
		0.339894 -0.0407873
		0.320732 -0.0301865
		0.24326 0.0398998
		0.26992 0.0838172
		0.234059 0.0702178
		0.219572 0.0712748
		0.25655 0.108021
		0.298082 0.165601
		0.300471 0.178057
		0.290119 0.185857
		0.279178 0.176475
		0.243641 0.16677
		0.254986 0.179033
		0.260853 0.201311
		0.273489 0.227653
		0.253279 0.227522
		0.253279 0.227522
		0.233933 0.21433
		0.277547 0.261955
		0.277547 0.261955
		0.258212 0.297815
		0.202167 0.243605
		0.202109 0.24107
		0.219954 0.263944
		0.178203 0.213207
		0.16154 0.203164
		0.16154 0.203164
		0.158939 0.208862
		0.159518 0.222457
		0.159518 0.222457
		0.172489 0.299074
		0.161647 0.297044
		0.161647 0.297044
		0.163002 0.32013
		0.158285 0.322488
		0.158285 0.322488
		0.143424 0.301874
		0.137234 0.29917
		-0.230732 -1.01679
		-1.16681 -0.110154
		-1.19913 0.430123
		-0.538433 0.996284
		-0.0955423 1.24205
		0.545236 0.921879
		0.778695 0.593133
		0.806441 0.084395
		0.604346 -0.359482
		-0.137354 -0.802271
		-0.550031 -0.794108
		-0.642393 -0.678483
		-0.486688 -0.527489
		-0.298734 -0.490421
		0.268524 -0.216311
		0.26869 0.0876779
		0.121722 0.294048
		0.111904 0.284369
		0.111904 0.284369
		0.0890537 0.249813
		0.0814723 0.23464
		0.0814723 0.23464
		0.0721868 0.237661
		0.0512868 0.192551
		0.0512868 0.192551
		0.0237053 0.209397
		0.0291396 0.213021
		0.0291396 0.213021
		-0.169421 0.258837
		-0.144279 0.202475
		0.0491863 0.18357
		0.0195709 0.251975
		0.00789693 0.276392
		-0.29618 0.210483
		-0.310561 0.196636
		-0.352857 0.20285
		-0.390597 0.228779
		-0.495474 -0.13128
		-0.528697 -0.158836
		-0.565728 -0.170922
		-0.486157 -0.153088
		-0.545205 -0.176322
		-0.489027 -0.187106
		-0.479843 -0.209538
		-0.488177 -0.243013
		-0.469034 -0.241686
		-0.476757 -0.257034
		-0.474702 -0.258928
		-0.497124 -0.284381
		-0.616212 -0.365876
		-0.659485 -0.433634
		-0.656104 -0.415923
		-0.665771 -0.442843
		-0.666207 -0.440063
		-0.698822 -0.464813
		-0.721468 -0.496423
		-0.736174 -0.489673
		-0.76109 -0.513212
		-0.785286 -0.528283
		-0.777441 -0.533607
		-0.768425 -0.526129
		-0.82941 -0.576496
		-0.82418 -0.583948
		-0.826442 -0.580743
		-0.835946 -0.593863
		-0.860902 -0.605679
		-0.888776 -0.638196
		-0.956596 -0.706865
		-0.9471 -0.697863
		-0.861038 -0.64483
		-0.936158 -0.705212
		-0.85146 -0.649799
		-0.917432 -0.73152
		-0.924134 -0.716509
		-0.917432 -0.73152
		-0.915463 -0.733983
		-0.917632 -0.763303
		-0.848418 -0.693127
		-0.853976 -0.718116
		-0.856281 -0.716796
		-0.837931 -0.708433
		-0.905664 -0.777465
		-0.842166 -0.721857
		-0.862106 -0.742369
		-0.916727 -0.795334
		-0.912845 -0.799786
		-0.900229 -0.780473
		-0.910771 -0.802147
		-0.884975 -0.783487
		-0.902474 -0.798021
		-0.832221 -0.732047
		-0.864082 -0.774834
		-0.846191 -0.774004
		-0.803727 -0.761827
		-0.790737 -0.76047
		-0.783501 -0.787304
		-0.758742 -0.780949
		-0.720778 -0.760223
		-0.711862 -0.754362
		-0.696489 -0.752771
		-0.669744 -0.741871
		-0.652273 -0.746903
		-0.6618 -0.792048
		-0.594194 -0.74194
		-0.628368 -0.846154
		-0.620671 -0.870408
		-0.597499 -0.881496
		-0.588308 -0.914313
		-0.589666 -0.960649
		-0.565938 -0.988399
		-0.492553 -0.947217
		-0.463751 -0.961995
		-0.459964 -0.961743
		-0.423838 -0.982534
		-0.389496 -0.987236
		-0.365036 -0.981035
		-0.351575 -0.985939
		-0.337915 -0.990704
		-0.302789 -1.02482
		-0.271439 -1.02759
		-0.225268 -1.01943
		-0.213122 -1.01613
		-0.159757 -1.05839
		-0.111101 -1.05943
		-0.0643052 -0.910426
		-0.0456829 -0.945286
		0.042859 -1.02862
		0.060918 -0.840027
		0.162413 -1.02993
		0.134342 -0.849792
		0.181848 -0.90587
		0.168318 -0.800251
		0.187475 -0.857935
		0.222371 -0.8637
		0.279308 -0.945349
		0.277129 -0.857168
		0.335317 -0.887405
		0.38961 -0.870694
		0.466857 -0.933714
		0.448408 -0.849258
		0.513775 -0.879207
		0.544699 -0.898017
		0.551025 -0.855926
		0.553934 -0.8238
		0.638916 -0.862152
		0.680458 -0.788883
		0.708148 -0.776312
		0.680978 -0.712089
		0.69383 -0.718114
		0.729638 -0.686293
		0.70965 -0.713216
		0.684032 -0.625401
		0.695462 -0.566074
		0.687481 -0.53789
		0.787672 -0.5681
		0.751791 -0.532241
		1.02372 -0.665419
		1.02411 -0.644955
		0.918209 -0.547902
		0.916545 -0.550681
		0.81845 -0.444302
		0.85219 -0.443416
		0.746111 -0.353734
		0.78818 -0.336908
		0.701637 -0.279029
		0.798034 -0.263965
		0.782147 -0.219238
		0.797329 -0.180527
		0.892472 -0.106564
		0.943514 -0.0698899
		0.912742 -0.0476806
		0.913586 -0.0270693
		0.89535 0.00670672
		0.936963 0.0594342
		0.929959 0.128871
		0.918916 0.161757
		1.00763 0.196981
		1.02089 0.242701
		1.00299 0.27077
		1.00657 0.330402
		0.918804 0.355552
		0.996914 0.427249
		0.944505 0.417339
		1.00757 0.493905
		0.927865 0.519604
		1.02685 0.627748
		1.11231 0.765008
		1.12629 0.78601
		0.995779 0.73825
		1.099 0.857407
		0.826253 0.737328
		0.810062 0.75508
		0.822306 0.788201
		0.767814 0.767814
		0.722038 0.756096
		0.561875 0.610499
		0.595331 0.657699
		0.672807 0.759725
		0.686165 0.792754
		0.991659 1.22321
		0.944154 1.19723
		0.753677 0.999613
		0.921277 1.29284
		0.707438 1.16749
		0.840496 1.38708
		0.682493 1.1847
		0.810361 1.4493
		0.72087 1.3749
		0.719189 1.4236
		0.710422 1.42574
		0.77552 1.71189
		0.760804 1.66146
		0.702614 1.57302
		0.705617 1.68564
		0.616183 1.53541
		0.624535 1.61956
		0.670446 1.79962
		0.620131 1.82496
		0.614791 1.87451
		0.590096 1.847
		0.101808 1.56106
		0.443404 1.90368
		0.426157 2.00108
		0.481232 1.92493
		0.427313 1.95601
		0.420823 1.9263
		0.434364 2.0648
		0.434364 2.0648
		0.454278 2.05358
		0.0893492 1.51894
		0.0893492 1.51894
		0.204751 1.86489
		-0.164023 2.25846
		-0.164023 2.25846
		-0.136936 1.98283
		-0.136936 1.98283
		-0.126954 2.30422
		-0.127655 2.30418
		-0.127655 2.30418
		-0.755189 2.83597
		-0.815065 2.886
		-0.935852 3.20997
		-0.83662 2.81851
		-0.870113 2.87807
		-0.968082 3.07456
		-0.953452 2.90254
		-0.998175 3.04753
		-1.03434 3.03288
		-1.05615 2.84664
		-1.37713 3.30121
		-1.39372 3.29425
		-1.7677 4.08024
		-1.43304 3.26576
		-1.46023 3.23957
		-1.47261 3.23396
		-1.50227 3.20678
		-1.52549 3.1958
		-1.54544 3.22783
		-1.54465 3.12743
		-2.00904 3.88653
		-1.80382 3.12727
		-2.34481 3.82702
		0.137234 0.29917
		-0.311508 0.197077
		-0.670168 -0.431478
		-0.949519 -0.691317
		-0.84143 -0.729497
		-0.65943 -0.740591
		-0.326706 -1.01512
		0.253773 -0.832499
		0.713017 -0.592507
		0.912569 -0.0508868
		1.07032 0.712051
		0.930037 1.41128
		0.577099 1.86813
		-0.104802 2.21317
		-3.12482 3.19638
		-3.12445 3.17197
		-3.25862 3.03266
		-3.33921 3.08421
		-3.40068 2.92171
		-3.40543 2.91381
		-3.40598 2.90405
		-3.40354 2.87992
		-3.39162 2.79516
		-3.40829 2.76411
		-3.42408 2.72529
		-3.43345 2.74207
		-3.38526 2.69203
		-3.37578 2.67537
		-3.44246 2.68395
		-3.47773 2.68787
		-3.4535 2.62791
		-3.47921 2.50503
		-3.60901 2.54542
		-3.63606 2.51175
		-3.64725 2.49548
		-3.72278 2.46981
		-3.7241 2.45863
		-3.65277 2.35323
		-3.68566 2.33582
		-3.69627 2.319
		-3.69362 2.27929
		-3.64113 2.22132
		-3.67874 2.19799
		-3.80284 2.17475
		-3.81375 2.14524
		-3.81375 2.14524
		-3.82327 2.13864
		-3.83773 2.09222
		-3.73125 1.94574
		-3.72875 1.94395
		-3.74436 1.90046
		-3.78423 1.84098
		-3.79113 1.79341
		-3.81808 1.78329
		-3.88383 1.77381
		-3.85029 1.747
		-3.84677 1.69947
		-3.68719 1.58023
		-3.78425 1.52046
		-3.86904 1.50653
		-3.788 1.47064
		-3.73331 1.41909
		-3.75465 1.40115
		-3.86148 1.40315
		-3.86465 1.38502
		-3.90254 1.33092
		-3.91951 1.28007
		-3.98227 1.28534
		-3.94414 1.22054
		-3.83116 1.12746
		-3.83705 1.10726
		-3.84751 1.06327
		-3.84856 1.03067
		-3.9253 1.01767
		-3.86928 0.981099
		-3.85585 0.963964
		-3.86241 0.919101
		-3.89875 0.872525
		-3.95217 0.870816
		-3.95695 0.844742
		-3.9468 0.809315
		-3.95491 0.7687
		-3.91644 0.693078
		-4.02732 0.67686
		-3.99561 0.534232
		-4.04958 0.416207
		-4.04919 0.314937
		-4.05752 0.268266
		-4.07647 -0.0675656
		-4.24039 -0.117138
		-4.24333 -0.140663
		-3.63784 -1.4486
		-3.63032 -1.46735
		-3.84667 -1.58256
		-3.63185 -1.52056
		-3.63185 -1.52056
		-3.84516 -1.69328
		-3.9728 -1.77379
		-3.9728 -1.77379
		-3.89147 -1.84905
		-3.71753 -1.86459
		-3.71753 -1.86459
		-3.57411 -1.87754
		-3.413 -1.86954
		-3.413 -1.86954
		-3.60353 -2.02627
		-3.46489 -2.02768
		-3.46489 -2.02768
		-3.59523 -2.20616
		-3.53453 -2.1875
		-3.53453 -2.1875
		-3.32055 -2.19513
		-3.28285 -2.21453
		-3.28285 -2.21453
		-3.27286 -2.23403
		-3.47241 -2.42234
		-3.20979 -2.34259
		-3.39222 -2.54417
		-3.27064 -2.49358
		-3.27064 -2.49358
		-3.094 -2.49986
		-3.1196 -2.56374
		-3.1196 -2.56374
		-3.11497 -2.60339
		-2.98065 -2.48934
		-2.98065 -2.48934
		-3.06838 -2.73132
		-3.06838 -2.73132
		-3.07533 -2.90648
		-3.07533 -2.90648
		-2.9438 -2.87371
		-2.91591 -2.95133
		-2.91591 -2.95133
		-2.84127 -3.04253
		-2.84127 -3.04253
		-2.71547 -3.14235
		-2.44072 -2.96845
		-2.39318 -3.0218
		-2.39318 -3.0218
		-2.4541 -3.19149
		-2.39122 -3.2345
		-2.43039 -3.36698
		-2.38112 -3.33122
		-2.35198 -3.43197
		-2.27795 -3.39345
		-2.22257 -3.29948
		-2.19061 -3.29733
		-1.92756 -3.04679
		-1.99642 -3.27192
		-1.99642 -3.27192
		-1.74069 -3.04622
		-1.70902 -3.0641
		-1.68195 -3.0802
		-1.66628 -3.08871
		-1.47694 -2.84241
		-1.40781 -2.8434
		-1.39067 -2.89335
		-1.37506 -2.90081
		-1.34047 -2.91695
		-1.30555 -2.93275
		-1.24943 -2.94977
		-1.21049 -2.93311
		-1.13099 -2.96301
		-1.11114 -2.97859
		-1.10293 -2.98164
		-1.09168 -2.98578
		-1.0722 -2.99283
		-1.02203 -3.01033
		-1.01778 -3.05334
		-0.923396 -3.01027
		-0.923396 -3.01027
		-0.878407 -3.01432
		-0.792151 -3.03813
		-0.74954 -3.08248
		-0.666219 -2.92248
		-0.667989 -3.09533
		-0.638218 -3.0431
		-0.609785 -3.04892
		-0.633595 -3.28677
		-0.595288 -3.29393
		-0.509816 -3.14386
		-0.445113 -3.15367
		-0.402479 -3.26892
		-0.358158 -3.49731
		-0.271773 -3.3418
		-0.258603 -3.30216
		-0.208733 -3.29996
		-0.167144 -3.45779
		-0.115278 -3.46882
		-0.0629796 -3.48488
		-0.0208671 -3.47438
		0.0216154 -3.58817
		1.98782 -2.17713
		2.16688 -2.16688
		2.05961 -1.99344
		2.12668 -2.02419
		2.17359 -2.04318
		2.53671 -2.29607
		2.14818 -1.93
		2.54886 -2.21554
		2.40599 -2.05967
		2.11539 -1.73509
		2.17206 -1.59233
		3.02877 -1.97297
		2.32616 -1.49134
		2.22966 -1.42027
		2.74131 0.0415351
		2.64859 0.0960216
		2.43456 0.132794
		2.61931 0.198433
		2.42745 0.213321
		2.57309 0.273733
		2.59422 0.301468
		2.63105 0.313795
		2.53726 0.349165
		2.57827 0.369448
		2.56629 0.406851
		2.54539 0.419059
		2.50818 0.492404
		2.60658 0.575687
		2.59174 0.622017
		2.47659 0.64208
		2.5756 0.685764
		2.5449 0.699063
		2.69944 0.762886
		2.69131 0.788108
		2.65466 0.804692
		2.83121 0.905279
		2.79819 0.976728
		2.88415 1.05874
		2.86881 1.10199
		2.89276 1.16629
		2.57227 1.21194
		2.64438 1.27133
		2.53879 1.30237
		2.47325 1.3349
		2.62185 1.47315
		2.43802 1.37695
		2.67697 1.6098
		2.66129 1.61835
		2.56541 1.60556
		2.47928 1.55695
		2.47928 1.55695
		2.66251 1.72926
		2.66942 1.77044
		2.66942 1.77044
		2.66581 1.8201
		2.6159 1.83113
		2.6159 1.83113
		2.61627 1.91434
		2.54898 1.90728
		2.54898 1.90728
		2.55204 2.02499
		2.60539 2.12045
		2.50477 2.07961
		2.34915 2.13397
		2.34915 2.13397
		2.31843 2.1857
		2.31424 2.21633
		2.31424 2.21633
		2.21586 2.24203
		2.21586 2.24203
		2.15187 2.2031
		2.12647 2.2572
		2.12647 2.2572
		1.96744 2.26814
		1.87784 2.22837
		1.93485 2.43164
		2.13041 2.72808
		2.21223 2.93273
		1.75874 2.58235
		1.75874 2.58235
		1.83095 2.71485
		1.41873 2.59564
		1.41326 2.54706
		1.43863 2.63885
		1.28759 2.43965
		1.28977 2.4727
		1.51826 2.9542
		1.39466 2.70581
		1.51686 3.00596
		1.41602 2.90329
		1.3488 2.83594
		1.302 2.81815
		1.22392 2.87832
		1.32426 3.05037
		1.37295 3.20355
		1.34885 3.21063
		1.18397 2.84319
		1.12909 2.92537
		1.03407 2.90043
		1.10234 2.95394
		0.951635 2.89664
		1.10736 4.23334
		-3.08746 3.23106
		-3.4746 2.55657
		-3.80728 2.03919
		-3.88985 1.36427
		-3.96759 0.724419
		-4.00891 -1.87995
		-3.20979 -2.34259
		-2.97736 -3.06277
		-1.8887 -3.1726
		-1.02203 -3.01033
		-0.310811 -3.32868
		2.10753 -1.81327
		2.60422 0.484321
		2.45762 1.2973
		2.53996 1.98463
		2.21223 2.93273
		1.3593 3.08169
		-3.40504 2.88118
		-3.56765 2.30916
		-3.55929 1.91229
		-3.7196 1.32374
		-3.87515 0.660537
		-4.09246 0.0687809
		-3.83267 -0.996938
		-2.98178 -1.56327
		-2.25777 -1.43176
		-1.86965 -1.26969
		-1.38553 -0.829219
		-0.941282 -0.430697
		-0.968787 3.2976
		-0.978725 3.31261
		-0.995996 3.30746
		-1.65077 4.14501
		-1.38936 3.30338
		-1.48111 3.23151
		-2.0243 3.98835
		-2.00175 3.92059
		-2.04079 3.89174
		-2.083 3.87011
		-2.22399 3.86209
		-3.33921 3.08421
		-3.34036 3.06199
		-3.36392 3.03603
		-3.34817 2.98686
		-3.36701 2.92524
		-3.40575 2.9158
		-3.40839 2.87397
		-3.39777 2.80992
		-3.38997 2.75145
		-3.41263 2.74646
		-3.38526 2.69203
		-3.41438 2.69188
		-3.46483 2.68701
		-3.41108 2.65693
		-3.51924 2.51879
		-3.50567 2.48076
		-3.49571 2.48196
		-3.44686 2.40823
		-3.58181 2.43893
		-3.47558 2.36659
		-3.49787 2.35478
		-3.51725 2.32574
		-3.53463 2.29923
		-3.65659 2.34729
		-3.6707 2.32517
		-3.55552 2.26679
		-3.5282 2.21935
		-3.56249 2.19495
		-3.59094 2.19382
		-3.59661 2.18572
		-3.62872 2.16796
		-3.61923 2.16229
		-3.70267 2.18151
		-3.6089 2.11951
		-3.57571 2.05293
		-3.5919 2.03315
		-3.68541 2.06153
		-3.58541 1.98817
		-3.59487 1.97102
		-3.6023 1.95777
		-3.55929 1.91229
		-3.59369 1.86339
		-3.58403 1.83626
		-3.58403 1.83626
		-3.4868 1.7434
		-3.54266 1.71138
		-3.54266 1.71138
		-3.74926 1.73131
		-3.65948 1.67866
		-3.65948 1.67866
		-3.56402 1.57204
		-3.53334 1.51125
		-3.53334 1.51125
		-3.5367 1.4295
		-3.57408 1.39347
		-3.57408 1.39347
		-3.67403 1.35874
		-3.7196 1.32374
		-3.75771 1.25994
		-3.80236 1.26002
		-3.80236 1.26002
		-3.74231 1.1599
		-3.81617 1.17163
		-3.81617 1.17163
		-3.84174 1.12795
		-3.69382 1.03555
		-3.69382 1.03555
		-3.66016 0.962644
		-3.68877 0.93548
		-3.68877 0.93548
		-3.67499 0.887066
		-3.72561 0.819635
		-3.72561 0.819635
		-3.87698 0.693891
		-3.87515 0.660537
		-3.8717 0.623409
		-3.86551 0.567814
		-3.86551 0.567814
		-3.89321 0.515439
		-3.87923 0.457662
		-3.87923 0.457662
		-3.98134 0.412632
		-3.9284 0.373088
		-3.9284 0.373088
		-4.06745 0.319015
		-4.06745 0.319015
		-4.06973 0.284995
		-4.06909 0.193766
		-4.06909 0.193766
		-3.96772 0.155162
		-4.09246 0.0687809
		-3.99638 0.0333958
		-3.98824 -0.0668418
		-3.98824 -0.0668418
		-3.98725 -0.111376
		-3.98017 -0.144531
		-4.1859 -0.186558
		-4.15748 -0.31268
		-4.15751 -0.347424
		-4.19738 -0.386909
		-4.24569 -0.463815
		-4.24306 -0.487298
		-4.1153 -0.531752
		-4.10929 -0.567198
		-4.10896 -0.578727
		-4.1057 -0.601399
		-3.90602 -0.931607
		-3.83459 -0.947629
		-4.11881 -1.08641
		-3.95128 -1.03376
		-4.05252 -1.12242
		-4.04947 -1.13338
		-3.84686 -1.12481
		-3.83948 -1.17443
		-3.80525 -1.19336
		-3.7086 -1.21413
		-3.63032 -1.22456
		-3.62372 -1.24396
		-3.20516 -1.47318
		-3.24496 -1.52107
		-3.23734 -1.53723
		-3.21969 -1.57384
		-3.27699 -1.62799
		-3.21868 -1.59902
		-3.23593 -1.66479
		-3.29728 -1.78289
		-3.07086 -1.69048
		-3.19473 -1.74826
		-3.15812 -1.80315
		-3.15812 -1.80315
		-2.91752 -1.68654
		-3.04402 -1.77738
		-2.97572 -1.81175
		-2.98938 -1.81607
		-2.96239 -1.80187
		-2.91862 -1.7713
		-2.89546 -1.7872
		-2.79449 -1.73451
		-2.69339 -1.67755
		-2.54599 -1.60893
		-2.67379 -1.69897
		-2.43884 -1.54968
		-2.26094 -1.43878
		-2.20013 -1.43319
		-2.17844 -1.39879
		-2.20013 -1.43319
		-2.15783 -1.43082
		-2.05002 -1.36915
		-2.14303 -1.439
		-2.09055 -1.40127
		-2.15285 -1.43262
		-2.14924 -1.43804
		-2.12838 -1.42151
		-2.13669 -1.41663
		-1.9465 -1.27604
		-1.95267 -1.30418
		-1.89348 -1.28109
		-1.90914 -1.26806
		-1.9007 -1.26947
		-1.84513 -1.24615
		-1.74827 -1.19378
		-1.81342 -1.23395
		-1.59549 -1.05184
		-1.44957 -0.953809
		-1.49257 -0.98003
		-1.49133 -0.986747
		-1.47722 -0.960752
		-1.39328 -0.881891
		-1.39328 -0.881891
		-1.42544 -0.887537
		-1.39257 -0.865083
		-1.42483 -0.881002
		-1.36349 -0.821192
		-1.29249 -0.784205
		-1.29378 -0.782063
		-1.32158 -0.789966
		-1.37526 -0.812654
		-1.25293 -0.7348
		-1.24581 -0.726722
		-1.16686 -0.677389
		-1.21405 -0.707437
		-1.21196 -0.69059
		-1.2097 -0.694544
		-1.11729 -0.641487
		-1.07621 -0.588872
		-1.07397 -0.587643
		-1.12708 -0.632368
		-1.07926 -0.582717
		-0.985021 -0.494355
		-0.967365 -0.480073
		-0.951728 -0.442501
		-0.937824 -0.436036
		-0.895819 -0.416273
		-0.962723 -0.438574
		-0.861515 -0.382896
		-0.825382 -0.365132
		-0.798746 -0.34741
		-0.816608 -0.347815
		-0.756885 -0.321958
		-0.762899 -0.307437
		-0.796579 -0.313894
		-0.756486 -0.278705
		-0.734973 -0.256964
		-0.767572 -0.253912
		-0.662044 -0.206417
		-0.73949 -0.219003
		-0.773989 -0.220708
		-0.73909 -0.193434
		-0.68152 -0.163672
		-0.647777 -0.142817
		-0.68133 -0.130922
		-0.692107 -0.119422
		-0.574355 -0.0960984
		-0.616164 -0.0890549
		-0.598278 -0.0703856
		-0.540608 -0.044003
		-0.459359 -0.0468366
		-0.543316 -0.0231646
		-0.559379 -0.0194379
		-0.551759 0.00636643
	};
\addlegendentry{Pred}
\addplot [draw=red, mark=o, only marks]
table{%
		x  y
		0.184939384460449 0.12700080871582
		-0.0627899169921875 1.80849003791809
		-0.183470249176025 1.79386591911316
		-0.463483810424805 1.79745864868164
		-0.494549512863159 1.79780626296997
		-0.626050472259521 1.80703806877136
		-0.662168979644775 1.81105661392212
		-0.699923038482666 1.81586599349976
		-0.739159822463989 1.82159113883972
		-0.779354810714722 1.82824754714966
		-0.820664882659912 1.83132147789001
		-0.973613500595093 1.84009528160095
		-1.00958442687988 1.83504176139832
		-1.04426550865173 1.82822871208191
		-0.508740186691284 2.3828272819519
		-0.560027122497559 2.39761567115784
		-0.689199924468994 2.41824746131897
		-0.715248107910156 2.4197781085968
		-0.846947431564331 2.42204546928406
		-0.896482944488525 2.42104935646057
		-0.923076868057251 2.42126417160034
		-0.950192928314209 2.42056250572205
		-1.00260257720947 2.41984128952026
		-1.02643632888794 2.41978216171265
		-1.12351655960083 2.42802119255066
		-1.40737295150757 2.46467804908752
		-1.46522879600525 2.46766376495361
		-1.49188923835754 2.46808958053589
		-1.74180388450623 2.42492341995239
		-1.8384382724762 2.38188743591309
		-1.8895218372345 2.35580134391785
		-1.98903322219849 2.30367112159729
		-1.09747457504272 2.42664790153503
		2.56631278991699 4.1558985710144
		0.18583345413208 4.45130634307861
		-0.0865716934204102 4.47834205627441
		-0.311665534973145 4.46138525009155
		-0.554606199264526 4.39847445487976
		-0.765497922897339 4.37149381637573
		-0.857213497161865 4.37468767166138
		-0.889987707138062 4.37776327133179
		-1.00627899169922 4.38773107528687
		-1.0368115901947 4.39288449287415
		-1.10242700576782 4.40288329124451
		-1.16588640213013 4.40788054466248
		-1.19683957099915 4.41242647171021
		-2.86640787124634 4.37948274612427
		-0.639804124832153 4.37901663780212
		0.354012966156006 2.64316558837891
		0.337342262268066 2.67685580253601
		0.317865371704102 2.71190762519836
		0.297689437866211 2.74566125869751
		0.276980876922607 2.77915549278259
		0.229832172393799 2.8410313129425
		0.183249473571777 2.89228129386902
		0.160796642303467 2.91698670387268
		0.137256145477295 2.94178533554077
		0.112030029296875 2.96534752845764
		0.0869851112365723 2.98773813247681
		0.06268310546875 3.00949621200562
		0.0382905006408691 3.03404140472412
		0.0138816833496094 3.05661559104919
		-0.0119738578796387 3.0767924785614
		-0.0374188423156738 3.09959626197815
		-0.0632171630859375 3.1231369972229
		-0.0892634391784668 3.14571952819824
		-0.139242172241211 3.187175989151
		-0.190523624420166 3.22986578941345
		-0.454052686691284 3.43485164642334
		-0.482349395751953 3.46012735366821
		-0.50995659828186 3.48652768135071
		-0.539922475814819 3.51195359230042
		-0.596237897872925 3.55991649627686
		-0.626880884170532 3.58152556419373
		-0.655164957046509 3.60334014892578
		-0.68376898765564 3.62514781951904
		-0.710470914840698 3.65037393569946
		-0.739860773086548 3.67483520507812
		-0.769970655441284 3.70003342628479
		-0.800036668777466 3.72414422035217
		-0.886843204498291 3.78699731826782
		-0.916602373123169 3.80544781684875
		-0.947345018386841 3.82199859619141
		-0.97872519493103 3.83761501312256
		-1.01283025741577 3.85481142997742
		-1.05009126663208 3.87340903282166
		-1.08535575866699 3.88796377182007
		-1.62772011756897 4.18571972846985
		-1.73451495170593 4.22722697257996
		-1.8450722694397 4.25348663330078
		-1.99174833297729 4.26517033576965
		0.254448413848877 2.81006598472595
		-0.86103343963623 3.76689314842224
		1.77359580993652 4.12709999084473
		1.34663152694702 4.32845544815063
		1.30881357192993 4.34236454963684
		1.18518829345703 4.36729264259338
		1.14184522628784 4.37447237968445
		1.09787511825562 4.37843489646912
		1.05463838577271 4.3830943107605
		0.969603538513184 4.38871192932129
		0.490447998046875 4.40941786766052
		0.271459102630615 4.4372661113739
		-2.14896845817566 4.63966631889343
		-0.717251062393188 -0.0104899406433105
		-0.434075117111206 0.328056335449219
		0.230428218841553 4.44654536247253
		0.151107788085938 4.46484613418579
		-0.0953121185302734 4.51950764656067
		-0.265668392181396 4.50009298324585
		-0.309620141983032 4.49742674827576
		-0.734986305236816 4.49398684501648
		-1.06163692474365 4.54810667037964
		-1.21538329124451 4.59085321426392
		-1.44999408721924 4.64009356498718
		-1.99154210090637 4.6330406665802
		-2.02605605125427 4.62743759155273
		-2.10776591300964 4.63451051712036
		-2.23209142684937 4.6476993560791
		-2.30953311920166 4.65967440605164
		-2.5863344669342 4.70303344726562
	};
\addlegendentry{Miss}


==> tikz/vis_localize/vis_loc_test2_clean.tex <==
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.277914524078369 0.37576961517334
		-0.275003910064697 0.383870601654053
		-0.272418022155762 0.391505479812622
		-0.269741058349609 0.397460222244263
		-0.268119812011719 0.402816295623779
		-0.261019706726074 0.409315586090088
		-0.254870414733887 0.403332471847534
		-0.249067783355713 0.394232749938965
		-0.243528366088867 0.385250568389893
		-0.23789644241333 0.347853183746338
		-0.239583492279053 0.333274126052856
		-0.242003440856934 0.317989349365234
		-0.24403715133667 0.302438259124756
		-0.243905544281006 0.273424386978149
		-0.240381240844727 0.243958711624146
		-0.238692760467529 0.228465795516968
		-0.246352195739746 0.19645094871521
		-0.253385543823242 0.181475162506104
		-0.294699192047119 0.125189304351807
		-0.324159860610962 0.0864124298095703
		-0.302732229232788 0.0923888683319092
		-0.297929048538208 0.0999257564544678
		-0.287972450256348 0.120825529098511
		-0.283878326416016 0.141290664672852
		-0.288012981414795 0.157615184783936
		-0.297602891921997 0.171787023544312
		-0.301599979400635 0.187467813491821
		-0.301223278045654 0.197311878204346
		-0.29999828338623 0.205654144287109
		-0.297425746917725 0.211897373199463
		-0.293235301971436 0.217428684234619
		-0.268847465515137 0.230886936187744
		-0.255252361297607 0.22833776473999
		-0.253783702850342 0.225872039794922
		-0.254422187805176 0.222661018371582
		-0.25548267364502 0.217538356781006
		-0.251174449920654 0.19727611541748
		-0.232236862182617 0.196452379226685
		-0.207677364349365 0.195921659469604
		-0.194808006286621 0.189937353134155
		-0.196717262268066 0.185196161270142
		-0.199209690093994 0.18011474609375
		-0.212458610534668 0.159175634384155
		-0.247348308563232 0.138494729995728
		-0.257808685302734 0.13278341293335
		-0.269469738006592 0.127597808837891
		-0.292534828186035 0.115068674087524
		-0.319334030151367 0.103604316711426
		-0.333157777786255 0.0983812808990479
		-0.346196174621582 0.0942003726959229
		-0.3840651512146 0.0905218124389648
		-0.653720855712891 0.122089147567749
		-0.660309076309204 0.105922937393188
		-0.661712884902954 0.0939831733703613
		-0.662400960922241 0.0808448791503906
		-0.656718254089355 0.0360820293426514
		-0.646893978118896 0.004608154296875
		-0.639547109603882 -0.0111711025238037
		-0.607984781265259 -0.0623006820678711
		-0.595757722854614 -0.0805659294128418
		-0.583165407180786 -0.0995349884033203
		-0.570398330688477 -0.117632865905762
		-0.557304382324219 -0.135668516159058
		-0.544569730758667 -0.154345512390137
		-0.532211065292358 -0.171351671218872
		-0.507245063781738 -0.199429988861084
		-0.494518518447876 -0.210120439529419
		-0.48113489151001 -0.219118118286133
		-0.454319953918457 -0.231195688247681
		-0.441144943237305 -0.234488725662231
		-0.429921865463257 -0.235854148864746
		-0.419054269790649 -0.235508918762207
		-0.408848285675049 -0.233731269836426
		-0.372190237045288 -0.210256099700928
		-0.363263130187988 -0.201272964477539
		-0.210906982421875 -0.178790330886841
		-0.193362712860107 -0.183841705322266
		-0.175598621368408 -0.189611673355103
		-0.111173629760742 -0.192239284515381
		-0.101307392120361 -0.187330722808838
		-0.0941042900085449 -0.180757522583008
		-0.0816245079040527 -0.163728713989258
		-0.0802512168884277 -0.158412218093872
		-0.0814166069030762 -0.155252456665039
		-0.0833492279052734 -0.150414943695068
		-0.0872101783752441 -0.143878698348999
		-0.104498863220215 -0.125162839889526
		-0.112119674682617 -0.121433734893799
		-0.119813442230225 -0.119440793991089
		-0.127152442932129 -0.119353055953979
		-0.143746376037598 -0.11943244934082
		-0.151008605957031 -0.118131160736084
		-0.164333820343018 -0.111320972442627
		-0.170390605926514 -0.107547998428345
		-0.175509929656982 -0.10357403755188
		-0.178669452667236 -0.0987119674682617
		-0.180443286895752 -0.0930991172790527
		-0.178653240203857 -0.074988842010498
		-0.171958446502686 -0.0624861717224121
		-0.131465911865234 -0.0254018306732178
		-0.112082958221436 -0.0149457454681396
		-0.0917692184448242 -0.00606226921081543
		-0.0720953941345215 0.00130891799926758
		-0.0516562461853027 0.00694847106933594
		-0.0320119857788086 0.0110390186309814
		-0.0162792205810547 0.0144340991973877
		0.00761604309082031 0.0215628147125244
		0.0239143371582031 0.0280828475952148
		0.0297698974609375 0.0312995910644531
		0.0516629219055176 0.0337152481079102
		0.059298038482666 0.0288634300231934
		0.0685520172119141 0.021864652633667
		0.0777206420898438 0.0129024982452393
		0.0862774848937988 0.00221443176269531
		0.100553512573242 -0.023557186126709
		0.105515003204346 -0.0388224124908447
		0.119484424591064 -0.135337352752686
		0.119211673736572 -0.143948554992676
		0.128272533416748 -0.159711599349976
		0.146774768829346 -0.149021148681641
		0.154118061065674 -0.138189554214478
		0.162104606628418 -0.106740474700928
		0.16557502746582 -0.0846967697143555
		0.169551849365234 -0.0597004890441895
		0.17559814453125 -0.032642126083374
		0.182393550872803 -0.00373101234436035
		0.18871545791626 0.0244650840759277
		0.192722320556641 0.051316499710083
		0.190389156341553 0.103258371353149
		0.179197788238525 0.148152589797974
		0.17380428314209 0.165935754776001
		0.169169425964355 0.179272174835205
		0.165753841400146 0.188929796218872
		0.168379306793213 0.198062658309937
		0.175269603729248 0.188712596893311
		0.183918476104736 0.166247844696045
		0.188649654388428 0.154552459716797
		0.193849563598633 0.141823053359985
		0.205791473388672 0.120835304260254
		0.211556911468506 0.112207174301147
		0.215682506561279 0.106435537338257
		0.218762874603271 0.102531909942627
		0.214463710784912 0.108741998672485
		0.211386680603027 0.116566896438599
		0.208274841308594 0.128542423248291
		0.204588890075684 0.143620729446411
		0.195801258087158 0.186198234558105
		0.184167385101318 0.243378162384033
		0.172471523284912 0.307852506637573
		0.0935778617858887 0.546064853668213
		0.0672755241394043 0.589858293533325
		0.0205011367797852 0.648478269577026
		0.00334405899047852 0.664420604705811
		-0.0337276458740234 0.691680908203125
		-0.0527706146240234 0.702938318252563
		-0.0930442810058594 0.719688653945923
		-0.113120079040527 0.726245164871216
		-0.132591724395752 0.73127293586731
		-0.151701927185059 0.734002113342285
		-0.172614574432373 0.734124898910522
		-0.19407320022583 0.734280347824097
		-0.216377258300781 0.735438823699951
		-0.261757850646973 0.737592220306396
		-0.310055255889893 0.740287065505981
		-0.336030960083008 0.741265773773193
		-0.36329197883606 0.742215394973755
		-0.391516923904419 0.743377447128296
		-0.419842481613159 0.744337320327759
		-0.476608514785767 0.744913578033447
		-0.505202293395996 0.743869304656982
		-0.560230493545532 0.739052534103394
		-0.636612415313721 0.724489688873291
		-0.68250298500061 0.708279609680176
		-0.792516469955444 0.612484693527222
		-0.821702480316162 0.559808254241943
		-0.839225292205811 0.503816604614258
		-0.840465307235718 0.485356330871582
		-0.844769716262817 0.443967342376709
		-0.849592924118042 0.388089418411255
		-0.959759712219238 0.098212718963623
		-0.995194435119629 0.0539009571075439
		-1.01456260681152 0.0312232971191406
		-1.03385734558105 0.00915431976318359
		-1.05229759216309 -0.0121970176696777
		-1.0698401927948 -0.0328161716461182
		-1.08634901046753 -0.0538730621337891
		-1.11919379234314 -0.0964715480804443
		-1.13564085960388 -0.116577386856079
		-1.15089416503906 -0.136196851730347
		-1.16647338867188 -0.155740261077881
		-1.18189358711243 -0.17614221572876
		-1.21087050437927 -0.220606803894043
		-1.2253429889679 -0.244003772735596
		-1.23993897438049 -0.267295122146606
		-1.25464391708374 -0.290359258651733
		-1.26926517486572 -0.313201904296875
		-1.28489875793457 -0.335656642913818
		-1.3002724647522 -0.357386350631714
		-1.3153920173645 -0.378275632858276
		-1.3410964012146 -0.420318365097046
		-1.35255312919617 -0.442689657211304
		-1.36331939697266 -0.46506929397583
		-1.37216734886169 -0.486552000045776
		-1.37888622283936 -0.507885932922363
		-1.38419413566589 -0.529788970947266
		-1.38769173622131 -0.553345203399658
		-1.39093732833862 -0.602697968482971
		-1.38925623893738 -0.629052519798279
		-1.38465738296509 -0.655265927314758
		-1.37682580947876 -0.680898904800415
		-1.35421657562256 -0.731403470039368
		-1.32600212097168 -0.786984086036682
		-1.31065845489502 -0.815557599067688
		-1.2955470085144 -0.842177987098694
		-1.28171491622925 -0.866486549377441
		-1.26860356330872 -0.888938784599304
		-1.25459098815918 -0.910164833068848
		-1.24150276184082 -0.930006623268127
		-1.22055172920227 -0.966433167457581
		-1.21230983734131 -0.984264254570007
		-1.20609641075134 -1.00171661376953
		-1.20203185081482 -1.01882719993591
		-1.19986176490784 -1.05091631412506
		-1.20200276374817 -1.06502676010132
		-1.20534944534302 -1.07807993888855
		-1.21091437339783 -1.09149968624115
		-1.2164831161499 -1.10493040084839
		-1.22399115562439 -1.11788094043732
		-1.23337912559509 -1.13042843341827
		-1.28880786895752 -1.19087469577789
		-1.30305528640747 -1.20824337005615
		-1.31002974510193 -1.21720016002655
		-1.31695866584778 -1.22634041309357
		-1.32999658584595 -1.24770951271057
		-1.33137106895447 -1.26393151283264
		-1.28782987594604 -1.27334201335907
		-1.27450489997864 -1.27544581890106
		-1.24412441253662 -1.28058695793152
		-1.22928094863892 -1.28535652160645
		-1.18280935287476 -1.32739007472992
		-1.16632890701294 -1.34616529941559
		-1.15656876564026 -1.35667419433594
		-1.14568638801575 -1.36973750591278
		-1.12137508392334 -1.40149116516113
		-1.10954689979553 -1.41754627227783
		-1.09809541702271 -1.4339234828949
		-1.08424425125122 -1.45127058029175
		-1.06870937347412 -1.46602237224579
		-1.05100512504578 -1.47866702079773
		-1.03069663047791 -1.49105226993561
		-1.01067900657654 -1.50222682952881
		-0.991294145584106 -1.51178133487701
		-0.973514556884766 -1.5204097032547
		-0.940063714981079 -1.53273713588715
		-0.922473669052124 -1.53867518901825
		-0.90374493598938 -1.54427242279053
		-0.858505487442017 -1.55346584320068
		-0.80485987663269 -1.55800187587738
		-0.776254415512085 -1.55651497840881
		-0.749781131744385 -1.55240893363953
		-0.724327564239502 -1.54573655128479
		-0.697410106658936 -1.53377556800842
		-0.670466423034668 -1.51742672920227
		-0.643152952194214 -1.49942266941071
		-0.615800619125366 -1.48087620735168
		-0.587999105453491 -1.46570384502411
		-0.559094905853271 -1.45412802696228
		-0.503242254257202 -1.43826186656952
		-0.475287675857544 -1.43487083911896
		-0.445384979248047 -1.43234968185425
		-0.414664506912231 -1.43130505084991
		-0.380980253219604 -1.43091654777527
		-0.34503960609436 -1.43041431903839
		-0.306323289871216 -1.43204283714294
		-0.265529155731201 -1.4360214471817
		-0.224159717559814 -1.44131410121918
		-0.18022632598877 -1.44923877716064
		-0.134766578674316 -1.46014213562012
		-0.088036060333252 -1.47164249420166
		-0.0408263206481934 -1.48118901252747
		0.00507164001464844 -1.48982346057892
		0.0479178428649902 -1.49840617179871
		0.0874972343444824 -1.50444412231445
		0.122891902923584 -1.50791537761688
		0.154507637023926 -1.50823068618774
		0.183198928833008 -1.50381076335907
		0.242511749267578 -1.48964643478394
		0.271658420562744 -1.48006653785706
		0.299930095672607 -1.46876990795135
		0.356565475463867 -1.43830156326294
		0.386484622955322 -1.41835367679596
		0.4178786277771 -1.39543557167053
		0.448380947113037 -1.36618864536285
		0.47688102722168 -1.33285450935364
		0.502026557922363 -1.29849565029144
		0.522701740264893 -1.26771581172943
		0.543740749359131 -1.24280595779419
		0.568014144897461 -1.22191202640533
		0.595983505249023 -1.20341205596924
		0.654234409332275 -1.17278146743774
		0.715023994445801 -1.14655101299286
		0.745688438415527 -1.13348603248596
		0.77711820602417 -1.12046718597412
		0.809403896331787 -1.10714292526245
		0.912381649017334 -1.06198215484619
		0.945664882659912 -1.04664981365204
		0.97785472869873 -1.03156614303589
		1.00692796707153 -1.01718664169312
		1.03428268432617 -1.00237238407135
		1.05913066864014 -0.987793326377869
		1.08167600631714 -0.971924066543579
		1.12275218963623 -0.935084700584412
		1.13949060440063 -0.91492772102356
		1.15115308761597 -0.89346182346344
		1.15871667861938 -0.869437217712402
		1.16288661956787 -0.842788457870483
		1.16582870483398 -0.813834309577942
		1.16874980926514 -0.783994317054749
		1.17134523391724 -0.751709938049316
		1.17780828475952 -0.684641718864441
		1.18082475662231 -0.648595213890076
		1.18810749053955 -0.57654881477356
		1.19367980957031 -0.541130542755127
		1.20950174331665 -0.475247859954834
		1.21814060211182 -0.443670272827148
		1.22750473022461 -0.412110328674316
		1.24492406845093 -0.349420547485352
		1.25454950332642 -0.316314220428467
		1.26497268676758 -0.282555103302002
		1.27562856674194 -0.248093366622925
		1.28720283508301 -0.212386131286621
		1.30069351196289 -0.175601482391357
		1.31554365158081 -0.138458013534546
		1.33101224899292 -0.1009361743927
		1.34755802154541 -0.0637838840484619
		1.3643012046814 -0.0268731117248535
		1.38192987442017 0.0103340148925781
		1.39972543716431 0.0486652851104736
		1.41519832611084 0.0898284912109375
		1.42902851104736 0.132864952087402
		1.44179391860962 0.175543546676636
		1.45395994186401 0.217343807220459
		1.46535778045654 0.256792545318604
		1.47516632080078 0.294201374053955
		1.48489665985107 0.329734563827515
		1.49441194534302 0.363883972167969
		1.50235223770142 0.39800763130188
		1.50463008880615 0.43229079246521
		1.50231695175171 0.467626571655273
		1.49481344223022 0.502772808074951
		1.48128795623779 0.534126758575439
		1.46524572372437 0.559112310409546
		1.44973707199097 0.579289674758911
		1.43465995788574 0.597668647766113
		1.39642190933228 0.65005350112915
		1.37587833404541 0.690285205841064
		1.35394096374512 0.740032196044922
		1.33936738967896 0.766297817230225
		1.32135486602783 0.792999505996704
		1.28037548065186 0.84899377822876
		1.25910186767578 0.87829065322876
		1.23722648620605 0.909407615661621
		1.21517705917358 0.941576719284058
		1.19360113143921 0.975414037704468
		1.17272520065308 1.01133465766907
		1.15340328216553 1.04729461669922
		1.11720180511475 1.11680483818054
		1.08483028411865 1.17734718322754
		1.05749034881592 1.22486114501953
		0.528740406036377 1.91563510894775
		0.489019870758057 1.90758609771729
		0.473927021026611 1.90118026733398
		0.457008838653564 1.89413452148438
		0.419692516326904 1.87804365158081
		0.398584365844727 1.87060499191284
		0.374695301055908 1.86231756210327
		0.349525928497314 1.85674142837524
		0.321820259094238 1.85089731216431
		0.292811870574951 1.84480810165405
		0.26231861114502 1.83815860748291
		0.229444980621338 1.83162569999695
		0.194689273834229 1.82503867149353
		0.160228252410889 1.81991958618164
		0.123721599578857 1.81374335289001
		0.0878257751464844 1.80928683280945
		0.049893856048584 1.80878043174744
		0.0121016502380371 1.80827927589417
		-0.0252418518066406 1.80832123756409
		-0.101132869720459 1.80575013160706
		-0.142006874084473 1.79925560951233
		-0.223679542541504 1.7917697429657
		-0.290345668792725 1.7945864200592
		-0.319445610046387 1.79653334617615
		-0.347094058990479 1.79809546470642
		-0.374986171722412 1.79798603057861
		-0.40419602394104 1.79685258865356
		-0.433620452880859 1.7970175743103
		-0.525775194168091 1.79891443252563
		-0.55772852897644 1.80132818222046
		-0.591510772705078 1.80414056777954
		-0.861749410629272 1.8355073928833
		-0.900150060653687 1.839688539505
		-0.937129497528076 1.84108448028564
		-1.07900595664978 1.82312941551208
		-1.11122822761536 1.81740593910217
		-1.14063858985901 1.81169486045837
		-1.16588258743286 1.80447292327881
		-1.18993663787842 1.79462122917175
		-1.21050190925598 1.77912783622742
		-1.22786855697632 1.75869035720825
		-1.24272084236145 1.7332284450531
		-1.26655101776123 1.66898131370544
		-1.40675258636475 0.537503242492676
		-1.43966126441956 0.49646258354187
		-1.55778932571411 0.251029968261719
		-1.55976057052612 0.216567277908325
		-1.55964779853821 0.201986074447632
		-1.55779314041138 0.185920238494873
		-1.55395078659058 0.168371200561523
		-1.54841136932373 0.148701906204224
		-1.54278349876404 0.12739372253418
		-1.52958703041077 0.0809292793273926
		-1.52165460586548 0.0560834407806396
		-1.51535797119141 0.0302271842956543
		-1.50942587852478 0.0035548210144043
		-1.50150656700134 -0.0248394012451172
		-1.49441194534302 -0.0540707111358643
		-1.48724555969238 -0.0851426124572754
		-1.47872114181519 -0.119713306427002
		-1.46974778175354 -0.155831575393677
		-1.46372127532959 -0.190316200256348
		-1.45802640914917 -0.224709272384644
		-1.45046424865723 -0.259353160858154
		-1.44298553466797 -0.292988300323486
		-1.43528866767883 -0.324957370758057
		-1.42665457725525 -0.358205080032349
		-1.40685033798218 -0.425074100494385
		-1.3973753452301 -0.459175109863281
		-1.38502311706543 -0.492364168167114
		-1.37361288070679 -0.525559902191162
		-1.36103081703186 -0.557466268539429
		-1.34667086601257 -0.588262557983398
		-1.3117663860321 -0.646023988723755
		-1.29246163368225 -0.67235791683197
		-1.23346662521362 -0.738878488540649
		-1.06192898750305 -0.854790687561035
		-1.00445556640625 -0.876057386398315
		-0.975684642791748 -0.887036442756653
		-0.946091413497925 -0.89824903011322
		-0.915157556533813 -0.911146283149719
		-0.882835865020752 -0.925284504890442
		-0.850311279296875 -0.9401615858078
		-0.817657709121704 -0.953638434410095
		-0.785905838012695 -0.966215491294861
		-0.754548788070679 -0.978294491767883
		-0.688797235488892 -0.999572277069092
		-0.654980897903442 -1.00880968570709
		-0.621203422546387 -1.01825392246246
		-0.586158752441406 -1.02760255336761
		-0.550389766693115 -1.03688955307007
		-0.515504598617554 -1.04598820209503
		-0.479119062423706 -1.05159211158752
		-0.441410541534424 -1.05802917480469
		-0.364597797393799 -1.06823217868805
		-0.325944900512695 -1.0682886838913
		-0.289548873901367 -1.06584870815277
		-0.252859115600586 -1.06319272518158
		-0.218037605285645 -1.05885863304138
		-0.183183670043945 -1.05375266075134
		-0.149319171905518 -1.04818940162659
		-0.115955352783203 -1.04223024845123
		-0.0824103355407715 -1.03476870059967
		0.0155863761901855 -1.00527346134186
		0.0494132041931152 -0.994248747825623
		0.113173484802246 -0.968424677848816
		0.147118091583252 -0.956148386001587
		0.181666374206543 -0.94139564037323
		0.257551193237305 -0.909263968467712
		0.336706161499023 -0.876733660697937
		0.374966144561768 -0.861131548881531
		0.450223445892334 -0.831574201583862
		0.487151145935059 -0.816159129142761
		0.52379846572876 -0.801509618759155
		0.56041145324707 -0.785947442054749
		0.597454071044922 -0.76990818977356
		0.633895874023438 -0.753046870231628
		0.667784214019775 -0.734333395957947
		0.701338291168213 -0.714678883552551
		0.734431743621826 -0.694161415100098
		0.794093132019043 -0.648275017738342
		0.819271087646484 -0.623937726020813
		0.842351913452148 -0.597761511802673
		0.885119438171387 -0.548850536346436
		0.90026330947876 -0.5174241065979
		0.915440559387207 -0.489379167556763
		0.931074142456055 -0.460411548614502
		0.947207927703857 -0.430480003356934
		0.962234497070312 -0.397973775863647
		0.976572036743164 -0.364188432693481
		0.990395069122314 -0.329739093780518
		1.00037384033203 -0.294807434082031
		1.00885200500488 -0.254948854446411
		1.02026891708374 -0.214493036270142
		1.03311967849731 -0.176049470901489
		1.04370880126953 -0.138928174972534
		1.05272483825684 -0.102901697158813
		1.06757116317749 -0.0335381031036377
		1.07419729232788 -0.000307798385620117
		1.08037281036377 0.0325901508331299
		1.08630132675171 0.0653808116912842
		1.09106206893921 0.0985817909240723
		1.10464382171631 0.197460412979126
		1.10961723327637 0.231368064880371
		1.11518955230713 0.26603627204895
		1.12084293365479 0.300183534622192
		1.12343978881836 0.33359956741333
		1.12605762481689 0.366553068161011
		1.1283860206604 0.398186206817627
		1.12991523742676 0.431136846542358
		1.12882947921753 0.464421987533569
		1.12469577789307 0.49727463722229
		1.1186408996582 0.531249284744263
		1.11113262176514 0.564232587814331
		1.08277702331543 0.662462711334229
		1.07160091400146 0.695167303085327
		1.05993318557739 0.727816820144653
		1.04696416854858 0.760651588439941
		1.03266286849976 0.794032573699951
		1.01828527450562 0.827357769012451
		1.00089120864868 0.860113859176636
		0.980503082275391 0.894352674484253
		0.962986469268799 0.932048320770264
		0.946936130523682 0.968765020370483
		0.929332256317139 1.00558090209961
		0.911039352416992 1.04221034049988
		0.892141819000244 1.08007597923279
		0.87217903137207 1.11903786659241
		0.836321830749512 1.19770646095276
		0.819808006286621 1.23536968231201
		-0.19622278213501 2.21395540237427
		-0.245086193084717 2.25039291381836
		-0.323575973510742 2.30481767654419
		-0.348572731018066 2.31834173202515
		-0.37579083442688 2.33057022094727
		-0.43004584312439 2.35452055931091
		-0.455840587615967 2.36588549613953
		-0.482459783554077 2.374760389328
		-0.534674882888794 2.3906843662262
		-0.586022853851318 2.40370631217957
		-0.611324787139893 2.40876054763794
		-0.636898517608643 2.41281032562256
		-0.663195133209229 2.41615533828735
		-0.743485927581787 2.42023181915283
		-0.772223949432373 2.42032670974731
		-0.79814076423645 2.42031288146973
		-0.869981527328491 2.42138504981995
		-1.18130660057068 2.43603706359863
		-1.20832514762878 2.44093346595764
		-1.26258540153503 2.45069766044617
		-1.28962206840515 2.45404887199402
		-1.34763288497925 2.45958685874939
		-1.37810206413269 2.46197724342346
		-1.43655300140381 2.4667592048645
		-1.51706147193909 2.46916556358337
		-1.57075142860413 2.46631765365601
		-1.5935230255127 2.46411490440369
		-1.64481210708618 2.45433115959167
		-1.6696674823761 2.44844746589661
		-1.71746516227722 2.4342303276062
		-1.76557040214539 2.41493272781372
		-1.79027581214905 2.40445184707642
		-1.8638162612915 2.36880898475647
		-1.91582250595093 2.3420672416687
		-1.94060826301575 2.32855153083801
		-1.96470475196838 2.31561851501465
		-2.01434016227722 2.29337191581726
		-2.07255434989929 2.2702693939209
		-2.10154128074646 2.25684332847595
		-2.13061833381653 2.24508094787598
		-2.16000866889954 2.23435211181641
		-2.19005465507507 2.22346138954163
		-2.21913862228394 2.21281933784485
		-2.24973273277283 2.20081210136414
		-2.28025841712952 2.18779492378235
		-2.31153643131256 2.17330002784729
		-2.34236299991608 2.15848469734192
		-2.3728449344635 2.14324069023132
		-2.40420162677765 2.12779903411865
		-2.43527221679688 2.11227250099182
		-2.46779572963715 2.09672427177429
		-2.50001692771912 2.07930207252502
		-2.52909731864929 2.06237769126892
		-2.58007264137268 2.02870869636536
		-2.60489082336426 2.01245951652527
		-2.62624967098236 1.99557447433472
		-2.64767205715179 1.97992491722107
		-2.66845166683197 1.96328783035278
		-2.69007778167725 1.94784474372864
		-2.72706830501556 1.90924739837646
		-2.74645042419434 1.88882327079773
		-2.76571977138519 1.86789870262146
		-2.78511047363281 1.84576153755188
		-2.80226218700409 1.82297968864441
		-2.81975698471069 1.80046057701111
		-2.83569228649139 1.7772216796875
		-2.86745131015778 1.73142266273499
		-2.88402533531189 1.70848727226257
		-2.90316617488861 1.68381500244141
		-2.93954348564148 1.62911558151245
		-2.95482218265533 1.6055805683136
		-2.98519551753998 1.55870747566223
		-3.01746606826782 1.51112079620361
		-3.04770684242249 1.46228671073914
		-3.08977890014648 1.38582134246826
		-3.10692059993744 1.36194014549255
		-3.13768661022186 1.30612730979919
		-3.15393471717834 1.27996754646301
		-3.16954720020294 1.25746083259583
		-3.1866180896759 1.2291202545166
		-3.20351207256317 1.20076036453247
		-3.22286367416382 1.16645860671997
		-3.26244604587555 1.10291242599487
		-3.28082573413849 1.07018446922302
		-3.29840010404587 1.03819346427917
		-3.33290755748749 0.974907875061035
		-3.34964042901993 0.942638158798218
		-3.36407256126404 0.909197568893433
		-3.38923466205597 0.843777418136597
		-3.39805424213409 0.812927961349487
		-3.40553867816925 0.783468961715698
		-3.41281032562256 0.75489068031311
		-3.41870957612991 0.726044178009033
		-3.42411309480667 0.697449207305908
		-3.42851662635803 0.669065237045288
		-3.43172472715378 0.64022970199585
		-3.4347397685051 0.584101676940918
		-3.43474948406219 0.55721116065979
		-3.43705636262894 0.526839733123779
		-3.43822127580643 0.494496822357178
		-3.43669700622559 0.464603185653687
		-3.4352662563324 0.409169435501099
		-3.43850862979889 0.347556114196777
		-3.44080090522766 0.316732406616211
		-3.4431928396225 0.28593897819519
		-3.44576424360275 0.254672765731812
		-3.45177316665649 0.191696882247925
		-3.45506072044373 0.158743381500244
		-3.45843720436096 0.125012159347534
		-3.46184128522873 0.0903043746948242
		-3.46523356437683 0.0554585456848145
		-3.46891444921494 0.0203306674957275
		-3.47204500436783 -0.0142276287078857
		-3.47590863704681 -0.0513079166412354
		-3.48035907745361 -0.0919811725616455
		-3.48161977529526 -0.131496667861938
		-3.47730922698975 -0.199971437454224
		-3.47447103261948 -0.232375144958496
		-3.47097247838974 -0.266051054000854
		-3.46644574403763 -0.300634145736694
		-3.45198160409927 -0.370165109634399
		-3.44315522909164 -0.403755187988281
		-3.43409538269043 -0.436044454574585
		-3.42380207777023 -0.468412399291992
		-3.41268748044968 -0.499844551086426
		-3.39996689558029 -0.531293630599976
		-3.38667809963226 -0.563340187072754
		-3.37213838100433 -0.595449209213257
		-3.3571150302887 -0.624057531356812
		-3.34141790866852 -0.655001521110535
		-3.32591128349304 -0.684772729873657
		-3.30999851226807 -0.714697599411011
		-3.29375028610229 -0.739475607872009
		-3.2802894115448 -0.764190912246704
		-3.23846209049225 -0.858538269996643
		-3.22436416149139 -0.890941858291626
		-3.2081446647644 -0.921290040016174
		-3.18197989463806 -0.981675028800964
		-3.1555095911026 -1.04789161682129
		-3.12641704082489 -1.11200940608978
		-3.07994282245636 -1.21052157878876
		-3.06021237373352 -1.24648082256317
		-3.04210436344147 -1.2834974527359
		-3.0218677520752 -1.31712675094604
		-2.99921452999115 -1.34790289402008
		-2.98140048980713 -1.37562072277069
		-2.96089434623718 -1.40102970600128
		-2.94103753566742 -1.42703115940094
		-2.92002356052399 -1.45283246040344
		-2.89824247360229 -1.47874450683594
		-2.87606871128082 -1.50250637531281
		-2.8540472984314 -1.52476322650909
		-2.83277606964111 -1.54580450057983
		-2.81288230419159 -1.56750559806824
		-2.79378771781921 -1.58811640739441
		-2.77279210090637 -1.6082655787468
		-2.75166809558868 -1.62852078676224
		-2.73029482364655 -1.64835947751999
		-2.68532693386078 -1.68583190441132
		-2.66274321079254 -1.70417594909668
		-2.63932800292969 -1.72032761573792
		-2.61450231075287 -1.73668175935745
		-2.58833754062653 -1.75246214866638
		-2.5624463558197 -1.76836842298508
		-2.53768599033356 -1.78583562374115
		-2.51207566261292 -1.80423372983932
		-2.46090924739838 -1.84052866697311
		-2.41108787059784 -1.8779177069664
		-2.38436162471771 -1.89774787425995
		-2.35717475414276 -1.91746389865875
		-2.32966458797455 -1.93739664554596
		-2.3021252155304 -1.95721411705017
		-2.27432918548584 -1.97682863473892
		-2.24727916717529 -1.99696213006973
		-2.21946430206299 -2.01819950342178
		-2.19074535369873 -2.03955644369125
		-2.16193175315857 -2.06055390834808
		-2.13326930999756 -2.08178159594536
		-2.10351181030273 -2.10329777002335
		-2.07304453849792 -2.12380704283714
		-2.01222109794617 -2.16086426377296
		-1.98179769515991 -2.17782863974571
		-1.95189118385315 -2.19379264116287
		-1.91934061050415 -2.2077913582325
		-1.88488388061523 -2.21998143196106
		-1.85232830047607 -2.23124080896378
		-1.81905007362366 -2.24262112379074
		-1.78585290908813 -2.25429055094719
		-1.75348091125488 -2.26436007022858
		-1.7219090461731 -2.27473020553589
		-1.69067859649658 -2.2856577038765
		-1.65851235389709 -2.29659301042557
		-1.59532308578491 -2.31808462738991
		-1.56192827224731 -2.32759901881218
		-1.5307035446167 -2.33660908043385
		-1.49903964996338 -2.3452306240797
		-1.43395614624023 -2.36275553703308
		-1.40116095542908 -2.37282578647137
		-1.36871361732483 -2.38361778855324
		-1.33650732040405 -2.39460724592209
		-1.30498933792114 -2.40514203906059
		-1.24164271354675 -2.42633675038815
		-1.2091121673584 -2.43785780668259
		-1.17605042457581 -2.45070205628872
		-1.14237093925476 -2.46494384855032
		-1.10799789428711 -2.47965826839209
		-1.07298946380615 -2.49460106343031
		-1.03805947303772 -2.50970257073641
		-1.00288391113281 -2.52451517432928
		-0.968321561813354 -2.5392544567585
		-0.934041023254395 -2.55409646034241
		-0.899856328964233 -2.56906268279999
		-0.865665912628174 -2.5841963738203
		-0.831038951873779 -2.59923138655722
		-0.796434879302979 -2.61408297717571
		-0.729492425918579 -2.6434365734458
		-0.697430610656738 -2.65697105228901
		-0.666011333465576 -2.66896580159664
		-0.634979009628296 -2.67931958287954
		-0.604560613632202 -2.68850005418062
		-0.542621850967407 -2.70544614642859
		-0.510859251022339 -2.71284830570221
		-0.478491306304932 -2.72014281153679
		-0.44575023651123 -2.727165594697
		-0.412659645080566 -2.73416940867901
		-0.379308462142944 -2.74070928990841
		-0.345607042312622 -2.74586719274521
		-0.312563419342041 -2.7504168599844
		-0.28018856048584 -2.75544947385788
		-0.247432231903076 -2.76044636964798
		-0.214572906494141 -2.76481848955154
		-0.181426048278809 -2.76992200314999
		-0.148313045501709 -2.77595688402653
		-0.114989757537842 -2.78425669670105
		-0.0811376571655273 -2.79290406405926
		-0.0463199615478516 -2.800441801548
		-0.0110702514648438 -2.8081551194191
		0.0246763229370117 -2.8158550709486
		0.0607204437255859 -2.82358965277672
		0.0965838432312012 -2.83131216466427
		0.132359981536865 -2.83908200263977
		0.167444705963135 -2.84731617569923
		0.201561450958252 -2.85530817508698
		0.235463619232178 -2.86441379785538
		0.269999504089355 -2.87413102388382
		0.305278778076172 -2.88393640518188
		0.342928886413574 -2.89327621459961
		2.84257936477661 -0.211014986038208
		2.81457376480103 0.1004638671875
		2.80242395401001 0.164047718048096
		2.79462814331055 0.194010257720947
		2.78849744796753 0.227062463760376
		2.78064775466919 0.261140823364258
		2.77213573455811 0.292715549468994
		2.76252222061157 0.355920076370239
		2.76030778884888 0.391060590744019
		2.75761318206787 0.427187442779541
		2.75471591949463 0.463705062866211
		2.75282335281372 0.499924421310425
		2.75279951095581 0.53466796875
		2.75421094894409 0.568251609802246
		2.75710344314575 0.600548028945923
		2.76139783859253 0.632907152175903
		2.7653431892395 0.665658473968506
		2.7691535949707 0.698196172714233
		2.77345609664917 0.730149030685425
		2.78289699554443 0.795141696929932
		2.7872462272644 0.827340841293335
		2.79250001907349 0.862302541732788
		2.79651737213135 0.899001359939575
		2.79398393630981 0.932919502258301
		2.79329299926758 0.961551904678345
		2.79330682754517 0.9918372631073
		2.7917013168335 1.02166938781738
		2.78791618347168 1.05705571174622
		2.78377342224121 1.09026718139648
		2.77413654327393 1.15618705749512
		2.75907802581787 1.21927237510681
		2.75253486633301 1.25136613845825
		2.74508905410767 1.31772017478943
		2.74361801147461 1.35084986686707
		2.73876333236694 1.41934394836426
		2.73577117919922 1.45767974853516
		2.7325325012207 1.49440145492554
		2.72874402999878 1.5285267829895
		2.72905254364014 1.56071615219116
		2.73110485076904 1.59634184837341
		2.73241901397705 1.63182282447815
		2.73240756988525 1.66754055023193
		2.73360776901245 1.7016613483429
		2.73538970947266 1.73603010177612
		2.73796033859253 1.76927804946899
		2.74071884155273 1.80415987968445
		2.74447727203369 1.83680701255798
		2.74914598464966 1.86946964263916
		2.75367593765259 1.90217614173889
		2.75852251052856 1.93256068229675
		2.76459360122681 1.96355295181274
		2.77252006530762 1.99493789672852
		2.7822208404541 2.02751851081848
		2.79284524917603 2.06441164016724
		2.79865074157715 2.1008837223053
		2.8013391494751 2.13027358055115
		2.81136751174927 2.22044825553894
		2.81193351745605 2.24851536750793
		2.7967267036438 2.47055697441101
		-1.25423431396484 4.41702151298523
		-1.28284668922424 4.41745233535767
		-1.34642362594604 4.41757583618164
		-1.3780517578125 4.41529011726379
		-1.49753212928772 4.40344715118408
		-1.52495741844177 4.40060806274414
		-1.61200189590454 4.39188456535339
		-1.64092993736267 4.38759160041809
		-1.67482256889343 4.38534665107727
		-1.70495676994324 4.38079810142517
		-1.73913860321045 4.37614870071411
		-1.7976987361908 4.36545872688293
		-1.8305926322937 4.36523461341858
		-1.86375689506531 4.36504554748535
		-1.96089243888855 4.36458158493042
		-2.08280754089355 4.37272524833679
		-2.17093777656555 4.38751125335693
		-2.23015022277832 4.4000461101532
		-2.29735136032104 4.41245937347412
		-2.3642805814743 4.41809630393982
		-2.42659091949463 4.42317056655884
		-2.55515575408936 4.42500972747803
		-2.77700352668762 4.40133380889893
		-2.83530163764954 4.3861231803894
		-2.89601147174835 4.3712170124054
		-4.20429873466492 4.10020065307617
		-4.22010061144829 4.08039379119873
		-4.29492317698896 3.46101021766663
		-4.31000929325819 3.39911198616028
		-4.31739538908005 3.36782360076904
		-4.32703213766217 3.33652520179749
		-4.33642789721489 3.30725860595703
		-4.37124966084957 3.20386075973511
		-4.37913026660681 3.16939854621887
		-4.38626613467932 3.13728404045105
		-4.39631663262844 3.06810808181763
		-4.40035822987556 3.03153228759766
		-4.40314587950706 2.96304535865784
		-4.40488922595978 2.92725515365601
		-4.40217693895102 2.82323908805847
		-4.4011113345623 2.78823852539062
		-4.39853379130363 2.75611448287964
		-4.39465756714344 2.72738265991211
		-4.38986045867205 2.69572877883911
		-4.38666721433401 2.6657600402832
		-4.38106548786163 2.56252670288086
		-4.37833328545094 2.49699521064758
		-4.38026493042707 2.45818686485291
		-4.38105901330709 2.42016386985779
		-4.38242050260305 2.38259887695312
		-4.3847918882966 2.35127711296082
		-4.38700991123915 2.31845045089722
		-4.38858813792467 2.28492450714111
		-4.39196179062128 2.25402641296387
		-4.39477092772722 2.22049307823181
		-4.39794144779444 2.18961191177368
		-4.40135186910629 2.15742945671082
		-4.40471426397562 2.12453818321228
		-4.41071511059999 2.09141445159912
		-4.41589683294296 2.05882835388184
		-4.42469291388988 2.02418804168701
		-4.43102319538593 1.99048233032227
		-4.43449854850769 1.95809984207153
		-4.43931220471859 1.92662167549133
		-4.46073766052723 1.75970077514648
		-4.46034848690033 1.72458982467651
		-4.45808789134026 1.65307807922363
		-4.45658256113529 1.61756777763367
		-4.45516493916512 1.58273196220398
		-4.45372633635998 1.54860162734985
		-4.45193375647068 1.51425671577454
		-4.44886103272438 1.48077583312988
		-4.44513754546642 1.44820261001587
		-4.44310756027699 1.41467595100403
		-4.4344043135643 1.35182332992554
		-4.4321563243866 1.32061576843262
		-4.43279801309109 1.2869701385498
		-4.43421801924706 1.25133943557739
		-4.43657419085503 1.21593546867371
		-4.43932144343853 1.18174433708191
		-4.44406417012215 1.14706325531006
		-4.45105755329132 1.11510062217712
		-4.45955602824688 1.0819399356842
		-4.46840590238571 1.04931497573853
		-4.47842465341091 1.01575613021851
		-4.48880562186241 0.981179475784302
		-4.49825295805931 0.948833465576172
		-4.50914753973484 0.914734840393066
		-4.53290510177612 0.849736452102661
		-4.5581316947937 0.781339883804321
		-4.56626176834106 0.750385761260986
		-4.57577779889107 0.716333150863647
		-4.58497714996338 0.683912992477417
		-4.59244096279144 0.652178764343262
		-4.59923928976059 0.616273641586304
		-4.60503903031349 0.582354307174683
		-4.61268243193626 0.515385389328003
		-4.61515274643898 0.482114791870117
		-4.61704224348068 0.449590682983398
		-4.62029728293419 0.415626287460327
		-4.62200185656548 0.384278297424316
		-4.62073856592178 0.351881980895996
		-4.62349730730057 0.320404767990112
		-4.62125924229622 0.25773024559021
		-4.62004068493843 0.224389791488647
		-4.61973610520363 0.191359996795654
		-4.61575084924698 0.160235404968262
		-4.61475977301598 0.128693103790283
		-4.66803827881813 -0.189714908599854
		-3.90352419018745 -1.60487282276154
		-3.60910046100616 -1.53218007087708
		-3.58334600925446 -1.52072858810425
		-3.55723333358765 -1.50785160064697
		-3.53078693151474 -1.49719512462616
		-3.47518408298492 -1.47485208511353
		-3.44707757234573 -1.46545612812042
		-3.38964480161667 -1.44800341129303
		-3.35970437526703 -1.43810784816742
		-3.33065295219421 -1.43012094497681
		-3.27380967140198 -1.41187953948975
		-3.24423289299011 -1.40639495849609
		-3.21521210670471 -1.39849436283112
		-3.15793740749359 -1.38318061828613
		-3.12943816184998 -1.37480044364929
		-3.09909749031067 -1.3673654794693
		-3.03701293468475 -1.34549200534821
		-3.00882291793823 -1.33239769935608
		-2.95066618919373 -1.30320191383362
		-2.92066764831543 -1.28523600101471
		-2.89169800281525 -1.26626873016357
		-2.86477744579315 -1.24565732479095
		-2.83690202236176 -1.22244143486023
		-2.81105995178223 -1.19838190078735
		-2.78684890270233 -1.17433416843414
		-2.76344239711761 -1.15016233921051
		-2.74042236804962 -1.12527143955231
		-2.7184089422226 -1.09955644607544
		-2.69677650928497 -1.07208859920502
		-2.67440116405487 -1.04136502742767
		-2.65325593948364 -1.01019275188446
		-2.63146567344666 -0.980669617652893
		-2.60982489585876 -0.946884393692017
		-2.59091520309448 -0.912709951400757
		-2.57296848297119 -0.879623293876648
		-2.55188393592834 -0.846693396568298
		-2.50330209732056 -0.79122269153595
		-2.47745203971863 -0.763608336448669
		-2.44934594631195 -0.732444763183594
		-2.43058657646179 -0.708453416824341
		-2.38136029243469 -0.652533292770386
		-2.35651135444641 -0.627318978309631
		-2.28314447402954 -0.554325342178345
		-2.25963997840881 -0.53263258934021
		-2.23432993888855 -0.509002685546875
		-2.17600536346436 -0.464558601379395
		-2.15006589889526 -0.438178300857544
		-2.12809085845947 -0.410266399383545
		-2.10576033592224 -0.384894609451294
		-2.08376955986023 -0.359236717224121
		-2.06305289268494 -0.332146167755127
		-2.04290843009949 -0.304666042327881
		-2.0239429473877 -0.276392936706543
		-2.00612378120422 -0.248367309570312
		-1.98850655555725 -0.219738006591797
		-1.97079515457153 -0.190974950790405
		-1.95342969894409 -0.160780906677246
		-1.93699336051941 -0.129960060119629
		-1.92102193832397 -0.0983984470367432
		-1.90478777885437 -0.065068244934082
		-1.88999128341675 -0.0309560298919678
		-1.8765594959259 0.00416159629821777
		-1.86055302619934 0.0394794940948486
		-1.84599661827087 0.0742387771606445
		-1.83171582221985 0.110515356063843
		-1.81689953804016 0.143288850784302
		-1.79959154129028 0.174514532089233
		-1.77866125106812 0.204972982406616
		-1.75677037239075 0.236977100372314
		-1.73443746566772 0.269885778427124
		-1.71265363693237 0.302143573760986
		-1.68900942802429 0.331577777862549
		-1.66547679901123 0.359428405761719
		-1.64205455780029 0.385988235473633
		-1.61738014221191 0.410605907440186
		-1.56518840789795 0.45696759223938
		-1.53825306892395 0.478923320770264
		-1.51045346260071 0.500088214874268
		-1.48287272453308 0.520118474960327
		-1.45489811897278 0.539576768875122
		-1.39678049087524 0.576595544815063
		-1.3745493888855 0.59682035446167
		-1.35114550590515 0.615208864212036
		-1.32780504226685 0.635141372680664
		-1.30577802658081 0.656468152999878
		-1.2826931476593 0.678339242935181
		-1.26311945915222 0.701130628585815
		-1.24088191986084 0.72329306602478
		-1.19231224060059 0.767637968063354
		-1.16723346710205 0.790067911148071
		-1.11612725257874 0.834963083267212
		-0.0431647300720215 1.15634655952454
		-0.00477313995361328 1.15637731552124
		0.0335893630981445 1.15593886375427
		0.0734372138977051 1.15548396110535
		0.11493444442749 1.15550422668457
		0.156240463256836 1.15547490119934
		0.197224617004395 1.15223956108093
		0.239355087280273 1.14751577377319
		0.280713558197021 1.14336776733398
		0.393359661102295 1.11055183410645
		0.429850578308105 1.09553670883179
		0.465181350708008 1.07873177528381
		0.498700618743896 1.06002998352051
		0.528893947601318 1.03945446014404
		0.555737972259521 1.01706719398499
		0.581520557403564 0.993365526199341
		0.605135440826416 0.967055559158325
		0.627744197845459 0.941199541091919
		0.649874687194824 0.91402792930603
		0.67102575302124 0.886675596237183
		0.689895629882812 0.858928442001343
		0.707642078399658 0.82646918296814
		0.727741241455078 0.796602249145508
		0.750485420227051 0.770499467849731
		0.771280288696289 0.743537664413452
		0.811149597167969 0.690264463424683
		0.82975435256958 0.66512656211853
		0.847797870635986 0.638798236846924
		0.901453018188477 0.55943489074707
		0.920179843902588 0.531665086746216
		0.938094139099121 0.502944707870483
		0.974667072296143 0.442760467529297
		0.992998600006104 0.411646366119385
		1.02676868438721 0.344072103500366
		1.04495668411255 0.310590744018555
		1.05940055847168 0.277475833892822
		1.06993722915649 0.244171142578125
		1.07904243469238 0.210108041763306
		1.0875449180603 0.176141262054443
		1.09378623962402 0.141998529434204
		1.09774827957153 0.107494592666626
		1.09995746612549 0.0734100341796875
		1.09842014312744 0.00704145431518555
		1.09190988540649 -0.0559177398681641
		1.08701658248901 -0.0852518081665039
		0.960212707519531 -0.481370210647583
		0.948887348175049 -0.514284372329712
		0.924861431121826 -0.582005620002747
		0.912328720092773 -0.616129755973816
		0.827256679534912 -0.825510501861572
		0.73979663848877 -0.940678119659424
		0.691353797912598 -0.989157199859619
		0.666869640350342 -1.010338306427
		0.642688751220703 -1.02959370613098
		0.591197490692139 -1.06121563911438
		0.564466953277588 -1.07266175746918
		0.538462162017822 -1.08243238925934
		0.513677597045898 -1.09054148197174
		0.487739086151123 -1.09425842761993
		0.432568550109863 -1.10253536701202
		0.407776832580566 -1.11045122146606
		0.357624530792236 -1.12734472751617
		0.332238674163818 -1.13514935970306
		0.281052112579346 -1.1433767080307
		0.255891799926758 -1.14623320102692
		0.230234622955322 -1.14752769470215
		0.207769870758057 -1.14956438541412
		0.187309265136719 -1.1526210308075
		0.150603294372559 -1.16226541996002
		0.114351749420166 -1.17139673233032
		0.0344123840332031 -1.21313273906708
		0.0242424011230469 -1.22762608528137
		0.0155935287475586 -1.24252104759216
		0.00612115859985352 -1.25567853450775
		-0.00242805480957031 -1.26635670661926
		-0.0215301513671875 -1.28344988822937
		-0.0512504577636719 -1.31139993667603
		-0.0597043037414551 -1.3189594745636
		-0.0675516128540039 -1.32363784313202
		-0.108784675598145 -1.32318520545959
		-0.154325485229492 -1.32388532161713
		-0.179200649261475 -1.32249820232391
		-0.205463886260986 -1.31866002082825
		-0.231256484985352 -1.3114333152771
		-0.283771991729736 -1.28925204277039
		-0.307493925094604 -1.27487707138062
		-0.352237939834595 -1.2392144203186
		-0.37431788444519 -1.22138142585754
		-0.393873929977417 -1.20453357696533
		-0.411863327026367 -1.18730640411377
		-0.428297519683838 -1.16887807846069
		-0.444737911224365 -1.15106201171875
		-0.459189891815186 -1.13025391101837
		-0.483140707015991 -1.08830440044403
		-0.495018005371094 -1.06948029994965
		-0.505005359649658 -1.05299401283264
		-0.513897895812988 -1.03849458694458
		-0.54308819770813 -0.991672158241272
		-0.562112331390381 -0.961335182189941
		-0.575012683868408 -0.943560600280762
		-0.59072208404541 -0.926045894622803
		-0.608514070510864 -0.909073948860168
		-0.647042989730835 -0.879947185516357
		-0.706599712371826 -0.838166117668152
		-0.736362218856812 -0.810944199562073
		-0.760092258453369 -0.794798254966736
		-0.788318872451782 -0.798201322555542
		-0.790523529052734 -0.799994587898254
		-0.790154933929443 -0.803003072738647
		-0.786429166793823 -0.80745804309845
		-0.768954038619995 -0.81961989402771
		-0.755683660507202 -0.827946901321411
		-0.738410711288452 -0.838007807731628
		-0.716881275177002 -0.849721312522888
		-0.692207336425781 -0.862349987030029
		-0.66495680809021 -0.876645922660828
		-0.635946989059448 -0.891597509384155
		-0.604500770568848 -0.907089233398438
		-0.571570634841919 -0.922106385231018
		-0.539379119873047 -0.934856295585632
		-0.509863376617432 -0.947177886962891
		-0.453445434570312 -0.97726833820343
		-0.430291891098022 -0.993814706802368
		-0.408097267150879 -1.01165461540222
		-0.388017177581787 -1.03024351596832
		-0.348654270172119 -1.06616604328156
		-0.330425500869751 -1.08242881298065
		-0.297281265258789 -1.11057901382446
		-0.267533779144287 -1.13790857791901
		-0.228556632995605 -1.15959358215332
		-0.208854675292969 -1.1683337688446
		-0.189523220062256 -1.17654871940613
		-0.166805267333984 -1.18380606174469
		-0.116062164306641 -1.19577169418335
		-0.0904417037963867 -1.20100367069244
		-0.0310778617858887 -1.20952951908112
		0.00168323516845703 -1.21019542217255
		0.0360918045043945 -1.2074716091156
		0.0695910453796387 -1.20568192005157
		0.104830741882324 -1.2032698392868
		0.17212963104248 -1.19220328330994
		0.195987224578857 -1.18567633628845
		0.217358112335205 -1.17861485481262
		0.23543643951416 -1.17067837715149
		0.251672267913818 -1.16389167308807
		0.280211925506592 -1.15849936008453
		0.298315048217773 -1.15552663803101
		0.301782131195068 -1.15168118476868
		0.292807579040527 -1.14103949069977
		0.236757755279541 -1.11392247676849
		0.189376831054688 -1.09244894981384
		0.161356925964355 -1.07856893539429
		0.101394653320312 -1.04454636573792
		0.0699763298034668 -1.02526831626892
		0.0393834114074707 -1.00716292858124
		-0.0192880630493164 -0.975882530212402
		-0.0477409362792969 -0.962546706199646
		-0.0770149230957031 -0.951367497444153
		-0.108039855957031 -0.942817807197571
		-0.171244144439697 -0.928955674171448
		-0.201854705810547 -0.922062754631042
		-0.230275630950928 -0.914840459823608
		-0.25727367401123 -0.908249258995056
		-0.282528400421143 -0.903212785720825
		-0.306378841400146 -0.899451851844788
		-0.352173328399658 -0.897143602371216
		-0.376338005065918 -0.895961999893188
		-0.401447534561157 -0.894657254219055
		-0.429410219192505 -0.892661213874817
		-0.460341453552246 -0.889306306838989
		-0.494524002075195 -0.883160471916199
		-0.563714981079102 -0.868979573249817
		-0.59633469581604 -0.857339859008789
		-1.21284055709839 -0.232818841934204
		-1.22509479522705 -0.171483278274536
		-1.22740507125854 -0.139894247055054
		-1.22591137886047 -0.10886025428772
		-1.22459840774536 -0.0792357921600342
		-1.21851992607117 -0.0501852035522461
		-1.21385502815247 -0.0180635452270508
		-1.20286822319031 0.0413997173309326
		-1.19568467140198 0.0645697116851807
		-1.19260597229004 0.0897402763366699
		-1.18890261650085 0.139318704605103
		-1.18979620933533 0.16293740272522
		-1.19317030906677 0.186396837234497
		-1.19411087036133 0.20825719833374
		-1.19393014907837 0.228434324264526
		-1.19382524490356 0.247164249420166
		-1.19254851341248 0.261994361877441
		-1.19226694107056 0.289807796478271
		-1.18505859375 0.33832836151123
		-1.18123722076416 0.373739004135132
		-1.16909742355347 0.41967248916626
		-1.15975975990295 0.448584318161011
		-1.14965176582336 0.478830575942993
		-1.13957023620605 0.511404037475586
		-1.12785029411316 0.54493522644043
		-1.11603450775146 0.578848361968994
		-1.08465790748596 0.641202688217163
		-1.00886678695679 0.745638370513916
		-0.657060146331787 1.15363097190857
		-0.630638360977173 1.16545343399048
		-0.602487325668335 1.17550873756409
		-0.542730569839478 1.1920371055603
		-0.511220693588257 1.19936656951904
		-0.48034930229187 1.20702338218689
		-0.447131633758545 1.21624040603638
		-0.418034791946411 1.22655081748962
		-0.390183687210083 1.2363166809082
		-0.361660480499268 1.2460196018219
		-0.332295179367065 1.25383472442627
		-0.303332328796387 1.26068925857544
		-0.273575305938721 1.26623678207397
		-0.243466377258301 1.27206110954285
		-0.212939739227295 1.27773118019104
		-0.155868053436279 1.28830885887146
		-0.129417419433594 1.29340934753418
		-0.0858893394470215 1.30093908309937
		-0.0643181800842285 1.30186080932617
		-0.0418915748596191 1.30198383331299
		-0.0189332962036133 1.30376172065735
		0.0266714096069336 1.30821084976196
		0.0805072784423828 1.30846452713013
		0.108007907867432 1.30761671066284
		0.136199951171875 1.30503916740417
		0.193504333496094 1.29777312278748
		0.251545429229736 1.28284525871277
		0.279844284057617 1.272292137146
		0.306796550750732 1.25926685333252
		0.332046508789062 1.2439866065979
		0.446691989898682 1.16754412651062
		0.493422985076904 1.14630746841431
		0.51635217666626 1.13635802268982
		0.538942337036133 1.12615323066711
		0.56072473526001 1.11558651924133
		0.599546909332275 1.0926239490509
		0.643015384674072 1.05555009841919
		0.657205581665039 1.04252815246582
		0.669690608978271 1.03030276298523
		0.681671619415283 1.01776146888733
		0.692926406860352 1.00495600700378
		0.703433990478516 0.991317510604858
		0.747417449951172 0.921402454376221
		0.758265495300293 0.90018367767334
		0.785701274871826 0.827550649642944
		0.795901298522949 0.770696640014648
		0.798702716827393 0.741109848022461
		0.799737930297852 0.710898399353027
		0.798248767852783 0.679014682769775
		0.79616641998291 0.617741346359253
		0.798167705535889 0.586602449417114
		0.802294731140137 0.532225131988525
		0.810657978057861 0.477164506912231
		0.814679145812988 0.449379444122314
		0.817949771881104 0.421698570251465
		0.826972961425781 0.342682838439941
		0.830242156982422 0.31749963760376
		0.834210872650146 0.292564392089844
		0.837543964385986 0.26990532875061
		0.837019443511963 0.228739738464355
		0.82888650894165 0.173847675323486
		0.821560382843018 0.106831073760986
		0.818082809448242 0.083519458770752
		0.812336444854736 0.0604681968688965
		0.804314613342285 0.0372543334960938
		0.780709743499756 -0.00851011276245117
		0.766463756561279 -0.0307550430297852
		0.750809669494629 -0.0517647266387939
		0.733503818511963 -0.071876049041748
		0.715365886688232 -0.0922093391418457
		0.69675350189209 -0.113544940948486
		0.651168823242188 -0.174505472183228
		0.612997531890869 -0.230718374252319
		0.599330902099609 -0.251935482025146
		0.589051723480225 -0.272381067276001
		0.577659130096436 -0.293827772140503
		0.565845966339111 -0.31463098526001
		0.542894840240479 -0.355003118515015
		0.0388383865356445 -0.741335272789001
		0.015129566192627 -0.752394080162048
		-0.00822544097900391 -0.763065218925476
		-0.0302548408508301 -0.775348305702209
		-0.0681037902832031 -0.795718669891357
		-0.0853056907653809 -0.806037068367004
		-0.118130683898926 -0.824884295463562
		-0.132920265197754 -0.833081722259521
		-0.14578104019165 -0.839864134788513
		-0.160085201263428 -0.845503330230713
		-0.176154613494873 -0.850763559341431
		-0.193031311035156 -0.856585621833801
		-0.210091590881348 -0.861902236938477
		-0.22615385055542 -0.865069985389709
		-0.260375499725342 -0.862035155296326
		-0.278355121612549 -0.857969045639038
		-0.296231746673584 -0.853223323822021
		-0.348082304000854 -0.828980445861816
		-0.38128924369812 -0.799543619155884
		-0.396506786346436 -0.781209945678711
		-0.410696268081665 -0.761560797691345
		-0.437394142150879 -0.721774578094482
		-0.445772886276245 -0.7027508020401
		-0.451537609100342 -0.684049725532532
		-0.455666065216064 -0.664581537246704
		-0.460288286209106 -0.605255246162415
		-0.459454298019409 -0.586531281471252
		-0.44917893409729 -0.541997909545898
		-0.438563823699951 -0.520967245101929
		-0.432770490646362 -0.512042045593262
		-0.426846265792847 -0.503372669219971
		-0.418881177902222 -0.495677947998047
		-0.407138586044312 -0.488276481628418
		-0.37705659866333 -0.463324785232544
		-0.365288257598877 -0.454926252365112
		-0.353477001190186 -0.446407318115234
		-0.342907190322876 -0.437713146209717
		-0.323894023895264 -0.418983221054077
		-0.308763027191162 -0.396149635314941
		-0.30242657661438 -0.384101867675781
		-0.291645526885986 -0.361377954483032
		-0.287078857421875 -0.349797010421753
		-0.26079273223877 -0.289906740188599
		-0.254109859466553 -0.280073165893555
		-0.246072769165039 -0.270961761474609
		-0.237159729003906 -0.261728525161743
		-0.227141380310059 -0.252754688262939
		-0.204848766326904 -0.236800909042358
		-0.192689895629883 -0.230083465576172
		-0.164846897125244 -0.22139310836792
		-0.129445552825928 -0.211901903152466
		-0.110036373138428 -0.205521583557129
		-0.0899624824523926 -0.198134422302246
		-0.0694217681884766 -0.190176963806152
		-0.0507888793945312 -0.181404590606689
		-0.0345239639282227 -0.173102855682373
		0.00453662872314453 -0.15779972076416
		0.0139575004577637 -0.154565095901489
		0.123301982879639 -0.07381272315979
		0.133353233337402 -0.0546555519104004
		0.140100002288818 -0.0376944541931152
		0.147955894470215 -0.0241324901580811
		0.162444114685059 0.00947117805480957
		0.162575721740723 0.0190322399139404
		0.160519599914551 0.0269498825073242
		0.157490730285645 0.0342843532562256
		0.154637336730957 0.039985179901123
		0.151484966278076 0.044093132019043
		0.147616863250732 0.0476460456848145
		0.124735832214355 0.0603225231170654
		0.12242317199707 0.0647997856140137
		0.120994567871094 0.0735011100769043
		0.119166851043701 0.0848557949066162
		0.117080211639404 0.097440242767334
		0.115183353424072 0.110934734344482
		0.1134352684021 0.125497579574585
		0.111397266387939 0.141303062438965
		0.0811862945556641 0.230682134628296
		0.0794820785522461 0.242374420166016
		0.083899974822998 0.286343812942505
		0.101418018341064 0.285519599914551
		0.0654759407043457 0.29588770866394
		0.0576715469360352 0.294289827346802
		0.0503983497619629 0.292346477508545
		0.0440464019775391 0.289305210113525
		0.0351438522338867 0.263369560241699
		0.04888916015625 0.231685876846313
		0.0543971061706543 0.219070196151733
		0.0635647773742676 0.206120729446411
		0.0780305862426758 0.190115690231323
		0.0815987586975098 0.184106349945068
		0.084864616394043 0.171042203903198
		0.0846109390258789 0.164938449859619
		0.0798640251159668 0.155462265014648
		0.0746297836303711 0.150488615036011
		0.0594892501831055 0.134607791900635
		0.0501933097839355 0.123613834381104
		-0.000557422637939453 0.0828537940979004
		-0.187736988067627 -0.0311923027038574
		-0.213685035705566 -0.0397756099700928
		-0.224315166473389 -0.0427324771881104
		-0.291979789733887 -0.046879768371582
		-0.307756423950195 -0.0453901290893555
		-0.389960527420044 -0.121003150939941
		-0.390766859054565 -0.143759250640869
		-0.383698701858521 -0.20403790473938
		-0.383737325668335 -0.221111059188843
		-0.393890142440796 -0.258189678192139
		-0.404008626937866 -0.278525352478027
		-0.416037559509277 -0.299462795257568
		-0.428387641906738 -0.319905757904053
		-0.441370964050293 -0.339421987533569
		-0.484662294387817 -0.390186309814453
		-0.520809173583984 -0.416249752044678
		-0.541309833526611 -0.428113698959351
		-0.582925319671631 -0.450322151184082
		-0.60228705406189 -0.459963083267212
		-0.620578050613403 -0.468411684036255
		-0.638140678405762 -0.477233409881592
		-0.654347658157349 -0.487643480300903
		-0.667748928070068 -0.499457597732544
		-0.701869010925293 -0.535581350326538
		-0.713690757751465 -0.550159215927124
		-0.72506308555603 -0.565827131271362
		-0.735092163085938 -0.582529306411743
		-0.749797344207764 -0.615846395492554
		-0.75783109664917 -0.648298382759094
		-0.759751558303833 -0.665901303291321
		-0.760072231292725 -0.717513084411621
		-0.758114337921143 -0.76322877407074
		-0.759844303131104 -0.771123766899109
		-0.762367963790894 -0.77870512008667
		-0.765514850616455 -0.78607714176178
		-0.768378734588623 -0.791845321655273
		-0.757642507553101 -0.784935474395752
		-0.748700141906738 -0.787457823753357
		-0.712883949279785 -0.80402660369873
		-0.698525428771973 -0.811575055122375
		-0.683295965194702 -0.819514393806458
		-0.627657413482666 -0.849101781845093
		-0.605996131896973 -0.861527919769287
		-0.582801818847656 -0.875331282615662
		-0.557853698730469 -0.890239715576172
		-0.529401302337646 -0.905829548835754
		-0.495512723922729 -0.92119574546814
		-0.464057922363281 -0.93304967880249
		-0.41058874130249 -0.959159016609192
		-0.381691932678223 -0.973583340644836
		-0.35219407081604 -0.984793186187744
		-0.322547197341919 -0.992053508758545
		-0.26790189743042 -1.00387358665466
		-0.241239070892334 -1.00926995277405
		-0.215213775634766 -1.0137403011322
		-0.189555168151855 -1.01683294773102
		-0.164257049560547 -1.01862466335297
		-0.139685153961182 -1.01802289485931
		-0.115392208099365 -1.0150363445282
		-0.0922799110412598 -1.01043379306793
		-0.0691518783569336 -1.00607824325562
		-0.0225529670715332 -0.993653416633606
		0.00317192077636719 -0.986240983009338
		0.0546932220458984 -0.972500562667847
		0.084205150604248 -0.966763377189636
		0.115021705627441 -0.959287166595459
		0.146191120147705 -0.952088475227356
		0.17616081237793 -0.946071982383728
		0.206294059753418 -0.940526723861694
		0.236834049224854 -0.934322118759155
		0.267406463623047 -0.927891850471497
		0.299452781677246 -0.920152068138123
		0.333450794219971 -0.911478877067566
		0.367170333862305 -0.902480959892273
		0.401196002960205 -0.893187761306763
		0.436060428619385 -0.883751034736633
		0.469970226287842 -0.874265551567078
		0.507074356079102 -0.862037777900696
		0.546170234680176 -0.845296144485474
		0.579728126525879 -0.826709866523743
		0.610910415649414 -0.808308959007263
		0.638806819915771 -0.789348363876343
		0.66591215133667 -0.770050764083862
		0.732078075408936 -0.704350709915161
		0.750754356384277 -0.682214379310608
		0.794452667236328 -0.609509110450745
		0.804858207702637 -0.584781885147095
		0.820796966552734 -0.534348964691162
		0.828262329101562 -0.480717897415161
		0.834952354431152 -0.422256231307983
		0.840239524841309 -0.396286725997925
		0.849666595458984 -0.367722749710083
		0.861075401306152 -0.337437391281128
		0.87252140045166 -0.305984735488892
		0.885688304901123 -0.275828838348389
		0.898201942443848 -0.245117425918579
		0.912219524383545 -0.214740514755249
		0.939818859100342 -0.149490356445312
		0.954147338867188 -0.115328311920166
		0.968924999237061 -0.0814602375030518
		0.983282089233398 -0.04693603515625
		0.997100830078125 -0.0121166706085205
		1.01074743270874 0.0232160091400146
		1.02310562133789 0.0633063316345215
		1.03198432922363 0.102896213531494
		1.03897476196289 0.140045881271362
		1.04581499099731 0.174769878387451
		1.051109790802 0.209798812866211
		1.05346393585205 0.245654582977295
		1.0523681640625 0.31537389755249
		1.05053567886353 0.349741697311401
		1.04759883880615 0.383870601654053
		1.04342985153198 0.417561769485474
		1.03795385360718 0.451553583145142
		1.03157091140747 0.485405683517456
		1.02417993545532 0.517987728118896
		1.0155200958252 0.550272941589355
		1.00656032562256 0.583091020584106
		0.996558666229248 0.615774631500244
		0.985238075256348 0.647187471389771
		0.974446773529053 0.680673122406006
		0.963448047637939 0.712829113006592
		0.953518390655518 0.744342088699341
		0.945866584777832 0.779110908508301
		0.938451766967773 0.815282821655273
		0.93027400970459 0.853088855743408
		0.922322273254395 0.891509771347046
		0.915484428405762 0.929901599884033
		0.904428482055664 1.00913023948669
		0.89959716796875 1.04875373840332
		0.89527702331543 1.0880184173584
		0.886551380157471 1.16767978668213
		0.882192611694336 1.20822191238403
		0.878395557403564 1.25041365623474
		0.874495029449463 1.2962749004364
		0.866571426391602 1.34005856513977
		0.846817970275879 1.41953253746033
		0.837604522705078 1.45754432678223
		0.826606750488281 1.49510836601257
		0.813945770263672 1.53258228302002
		0.7995285987854 1.56949758529663
		0.783819198608398 1.60581040382385
		0.76659631729126 1.64132118225098
		0.749369621276855 1.67575097084045
		0.731455326080322 1.70944356918335
		0.713229656219482 1.74260497093201
		0.694470405578613 1.77639484405518
		0.674454689025879 1.81032395362854
		0.653285980224609 1.84310078620911
		0.634293556213379 1.87861084938049
		0.615009307861328 1.91213822364807
		0.596256732940674 1.94449043273926
		0.580290794372559 1.97979712486267
		0.565024852752686 2.01677966117859
		0.54963493347168 2.05575680732727
		0.534325122833252 2.0951611995697
		0.520403861999512 2.13439226150513
		0.507808208465576 2.17390251159668
		0.496052265167236 2.21267533302307
		0.484499454498291 2.25177407264709
		0.473177433013916 2.29050779342651
		0.461001873016357 2.33013296127319
		0.448827743530273 2.36972498893738
		0.436836719512939 2.40921688079834
		0.424506664276123 2.44833755493164
		0.413651943206787 2.48991441726685
		0.401344776153564 2.53288245201111
		0.385223865509033 2.57176566123962
		0.369021415710449 2.60863351821899
		-0.217875003814697 3.24940371513367
		-0.246552467346191 3.26994204521179
		-0.274134159088135 3.29235863685608
		-0.303316831588745 3.31535363197327
		-0.333654642105103 3.33896040916443
		-0.362924575805664 3.36274886131287
		-0.392948150634766 3.38549327850342
		-0.424643754959106 3.40999460220337
		-1.18347120285034 3.93217301368713
		-1.29624390602112 4.00192093849182
		-1.32795166969299 4.0201108455658
		-1.42393732070923 4.07481980323792
		-1.45741367340088 4.09442496299744
		-1.49137496948242 4.11312985420227
		-1.52479648590088 4.13039875030518
		-1.55809330940247 4.14913511276245
		-1.66403460502625 4.20123672485352
		-1.6999146938324 4.21439218521118
		-1.91890859603882 4.26157784461975
		-1.95528292655945 4.26415395736694
		-2.0268383026123 4.26329231262207
		-2.06239485740662 4.26215362548828
		-2.12790489196777 4.25351309776306
		-2.16567730903625 4.24732971191406
		-2.23897290229797 4.24112248420715
		-2.26582551002502 4.23267126083374
		-2.3050936460495 4.23201394081116
		-2.33718645572662 4.22840046882629
		-2.37809193134308 4.22672843933105
		-2.65855848789215 4.24363613128662
		-2.82365846633911 4.24262523651123
		-3.87303188443184 3.82958984375
		-3.93297001719475 3.7879045009613
		-3.96339324116707 3.76708340644836
		-4.14331650733948 3.6380500793457
		-4.1947211176157 3.5859808921814
		-4.27905238233507 3.46678853034973
		-4.29639540612698 3.43489789962769
		-4.309410716407 3.40455961227417
		-4.3246919773519 3.37502026557922
		-4.33771084621549 3.34030532836914
		-4.35750883817673 3.2743706703186
		-4.37683369964361 3.20461988449097
		-4.38492511212826 3.17158126831055
		-4.39310292899609 3.13798785209656
		-4.40322007238865 3.10531711578369
		-4.41340642422438 3.07091522216797
		-4.42520606517792 3.03507447242737
		-4.43602308630943 2.99738955497742
		-4.44531233608723 2.96080684661865
		-4.45583133399487 2.92422485351562
		-4.46550533175468 2.88711071014404
		-4.48715324699879 2.8165602684021
		-4.49448734521866 2.78023195266724
		-4.5055968016386 2.7463538646698
		-4.51347316801548 2.71088218688965
		-4.52191446721554 2.67375993728638
		-4.53639663755894 2.59782361984253
		-4.54663115739822 2.55873274803162
		-4.55941519141197 2.44891858100891
		-4.56130391359329 2.37258338928223
		-4.56291764974594 2.33149790763855
		-4.56385466456413 2.29311895370483
		-4.5615670979023 2.2546272277832
		-4.55870446562767 2.17376065254211
		-4.55578052997589 2.13657712936401
		-4.5508326292038 2.09760499000549
		-4.54595637321472 2.02008962631226
		-4.54092057049274 1.98181319236755
		-4.53603012859821 1.94672131538391
		-4.53110042214394 1.90975856781006
		-4.52373538911343 1.87545323371887
		-4.51891677081585 1.80326151847839
		-4.51372034847736 1.6814067363739
		-4.51234093308449 1.64071083068848
		-4.51297695934772 1.59907555580139
		-4.51390114426613 1.56332850456238
		-4.51563692092896 1.52465581893921
		-4.51830551028252 1.48599529266357
		-4.52075178921223 1.44682693481445
		-4.522565305233 1.40996742248535
		-4.52651497721672 1.37036228179932
		-4.53270515799522 1.29006385803223
		-4.53835779428482 1.2509286403656
		-4.54390589892864 1.21276140213013
		-4.5441419929266 1.12850642204285
		-4.5458525121212 1.08800530433655
		-4.54577144980431 1.04960203170776
		-4.54629048705101 1.00828170776367
		-4.54578536748886 0.967875480651855
		-4.54313470423222 0.923189163208008
		-4.54358756542206 0.880670547485352
		-4.54231831431389 0.839977025985718
		-4.53929977118969 0.798433303833008
		-4.53393942117691 0.715424537658691
		-4.53426498174667 0.670879125595093
		-4.5286630243063 0.632451772689819
		-4.52551965415478 0.58994197845459
		-4.51618374884129 0.469233274459839
		-4.50934201478958 0.296406030654907
		-4.51083418726921 0.211812019348145
		-4.51694503426552 0.128443002700806
		-4.55139654874802 -0.162943601608276
		-4.55299171805382 -0.204670190811157
		-4.551279515028 -0.24614143371582
		-4.02382212877274 -1.74366688728333
		-3.97245144844055 -1.79454416036606
		-3.94371277093887 -1.8203467130661
		-3.91671851277351 -1.84302860498428
		-3.88668289780617 -1.86932325363159
		-3.85820871591568 -1.8912815451622
		-3.82872250676155 -1.91307520866394
		-3.80194261670113 -1.93274027109146
		-3.77666598558426 -1.95593482255936
		-3.75150012969971 -1.98242002725601
		-3.67156702280045 -2.05859869718552
		-3.64606159925461 -2.08576083183289
		-3.62151277065277 -2.11242446303368
		-3.59757906198502 -2.13837838172913
		-3.57381939888 -2.16483741998672
		-3.54939353466034 -2.19162237644196
		-3.50124663114548 -2.24589452147484
		-3.47733074426651 -2.27428308129311
		-3.45333576202393 -2.30137020349503
		-3.43016910552979 -2.3306810259819
		-3.40475672483444 -2.36064383387566
		-3.37850153446198 -2.38784867525101
		-3.35243451595306 -2.41073602437973
		-3.32477110624313 -2.44053401052952
		-3.29621243476868 -2.46576108783484
		-3.20176076889038 -2.53903371095657
		-3.16842579841614 -2.56299112178385
		-3.13543391227722 -2.58328407723457
		-3.06765425205231 -2.62332829087973
		-3.03299379348755 -2.64345582574606
		-2.99737691879272 -2.66435269266367
		-2.96185719966888 -2.6833201944828
		-2.92559409141541 -2.70058500766754
		-2.88996088504791 -2.71515870094299
		-2.85470271110535 -2.73036110401154
		-2.82013070583344 -2.7457135617733
		-2.78721952438354 -2.75631058216095
		-2.71707153320312 -2.79217636585236
		-2.6802419424057 -2.81091338396072
		-2.64295101165771 -2.83136826753616
		-2.6055052280426 -2.85059201717377
		-2.56806588172913 -2.87038141489029
		-2.53174531459808 -2.89029797911644
		-2.49585676193237 -2.91034969687462
		-2.46035313606262 -2.92995202541351
		-2.3552770614624 -2.98854240775108
		-2.24806928634644 -3.04766669869423
		-2.21071195602417 -3.06745484471321
		-2.17365527153015 -3.08395248651505
		-2.13767433166504 -3.09946244955063
		-2.10179257392883 -3.11349731683731
		-2.06452298164368 -3.12641954421997
		-2.02474546432495 -3.13807475566864
		-1.98390173912048 -3.14681768417358
		-1.9407594203949 -3.15376573801041
		-1.89716935157776 -3.15927845239639
		-1.85325789451599 -3.16350966691971
		-1.76446127891541 -3.16971427202225
		-1.72083330154419 -3.17147719860077
		-1.67612886428833 -3.17232972383499
		-1.63138556480408 -3.17187261581421
		-1.58740568161011 -3.17134016752243
		-1.54223299026489 -3.17227703332901
		-1.49745845794678 -3.16982191801071
		-1.45502114295959 -3.16729056835175
		-1.41264271736145 -3.16835409402847
		-1.36945748329163 -3.17247200012207
		-1.32581639289856 -3.17731326818466
		-1.28240561485291 -3.18200939893723
		-1.23884892463684 -3.18767505884171
		-1.19641518592834 -3.1915128827095
		-1.15518569946289 -3.19693201780319
		-1.11422038078308 -3.20397651195526
		-1.03807163238525 -3.19456708431244
		-0.996449947357178 -3.22233128547668
		-0.956053256988525 -3.23091667890549
		-0.916853666305542 -3.23609304428101
		-0.876659393310547 -3.24405372142792
		-0.834352254867554 -3.25225085020065
		-0.793994665145874 -3.25187027454376
		-0.753572940826416 -3.25454133749008
		-0.713051795959473 -3.25962519645691
		-0.673753499984741 -3.25999456644058
		-0.634055614471436 -3.25969511270523
		-0.596056699752808 -3.25611644983292
		-0.555721282958984 -3.25699990987778
		-0.516140937805176 -3.2538925409317
		-0.476783990859985 -3.24990212917328
		-0.435813665390015 -3.24558299779892
		-0.396044731140137 -3.24047464132309
		-0.356666564941406 -3.23476499319077
		-0.314837455749512 -3.22965413331985
		-0.271498203277588 -3.22388970851898
		-0.229696273803711 -3.21749085187912
		-0.185202598571777 -3.21232122182846
		-0.142786979675293 -3.20569777488708
		-0.104713439941406 -3.19664865732193
		-0.0620875358581543 -3.19375121593475
		-0.0211095809936523 -3.19395339488983
		0.0207648277282715 -3.19336593151093
		0.0628566741943359 -3.19267040491104
		0.104364395141602 -3.1920765042305
		0.144002914428711 -3.1927889585495
		0.185239315032959 -3.19562268257141
		0.227507591247559 -3.19957715272903
		2.37491416931152 -2.30922549962997
		2.44876146316528 -2.1773564517498
		2.4649977684021 -2.1441764831543
		2.48479509353638 -2.11027839779854
		2.5077657699585 -2.07683819532394
		2.54090547561646 -2.00905758142471
		2.56156921386719 -1.9747599363327
		2.57972955703735 -1.94098460674286
		2.60298585891724 -1.90736126899719
		2.62136936187744 -1.87294727563858
		2.70777130126953 -1.6848384141922
		2.75717735290527 -1.47842979431152
		2.76568841934204 -1.39536893367767
		2.76860809326172 -1.35408508777618
		2.85786437988281 0.192008972167969
		2.85373258590698 0.265793323516846
		2.84855508804321 0.300716161727905
		2.84673547744751 0.373656272888184
		2.84661817550659 0.413226366043091
		2.8482837677002 0.494619607925415
		2.85047388076782 0.534889698028564
		2.85445880889893 0.573838472366333
		2.86371850967407 0.648694276809692
		2.86869096755981 0.685257434844971
		2.87447929382324 0.721235513687134
		2.88709449768066 0.792689085006714
		2.89401245117188 0.828399419784546
		2.9037299156189 0.865922689437866
		2.91467428207397 0.903899669647217
		2.92021131515503 0.941125392913818
		2.92371273040771 0.978049516677856
		2.92993879318237 1.01631450653076
		2.93683767318726 1.09619927406311
		2.93744277954102 1.13779139518738
		2.93853044509888 1.17994260787964
		2.92083072662354 1.37201023101807
		2.91660642623901 1.40741777420044
		2.90527486801147 1.47531366348267
		2.89924192428589 1.51216912269592
		2.890709400177 1.54459881782532
		2.8800106048584 1.57677745819092
		2.87378692626953 1.6095974445343
		2.87157535552979 1.64632821083069
		2.87099647521973 1.72209858894348
		2.86863899230957 1.76015734672546
		2.86899042129517 1.797682762146
		2.86707782745361 1.83340930938721
		2.86791658401489 1.86888146400452
		2.86699199676514 1.90490388870239
		2.87004327774048 1.94140148162842
		2.86941289901733 1.97789168357849
		2.86891078948975 2.01507782936096
		2.87009859085083 2.05292534828186
		2.87101030349731 2.09034872055054
		2.8718638420105 2.1271710395813
		2.87542057037354 2.20475840568542
		2.87106037139893 2.24320268630981
		2.85895156860352 2.31742310523987
		2.85384035110474 2.35589933395386
		2.81115007400513 2.58938241004944
		2.80009460449219 2.62455463409424
		2.78683996200562 2.66097569465637
		2.77733469009399 2.69660139083862
		2.7296667098999 2.79461407661438
		2.6989541053772 2.85878491401672
		2.68117904663086 2.88757753372192
		2.66789770126343 2.91924452781677
		2.64478778839111 2.99172782897949
		2.58808517456055 3.17231321334839
		2.55662679672241 3.28132247924805
		2.54512548446655 3.31870698928833
		2.52368211746216 3.3901801109314
		2.51324272155762 3.42823791503906
		2.43456363677979 3.60847282409668
		2.4171986579895 3.64140486717224
		2.39586973190308 3.67472505569458
		2.15825176239014 3.9210410118103
		2.12908363342285 3.93671917915344
		2.06839275360107 3.96972131729126
		2.03870248794556 3.98595070838928
		2.00509595870972 4.00434827804565
		1.94733428955078 4.03458714485168
		1.91506624221802 4.05296468734741
		1.88087940216064 4.07109093666077
		1.84514856338501 4.0894136428833
		1.80952835083008 4.10666680335999
		1.73959064483643 4.14264273643494
		1.70664310455322 4.16231608390808
		1.67280101776123 4.17705988883972
		1.63879919052124 4.19552206993103
		1.60388278961182 4.21274733543396
		1.56917715072632 4.23007488250732
		1.53311014175415 4.24791836738586
		1.49794721603394 4.26189804077148
		1.4615330696106 4.28003787994385
		1.38656425476074 4.31084704399109
		1.01147365570068 4.38608193397522
		-1.29559946060181 4.61269879341125
		-1.37559056282043 4.63076496124268
		-1.4130597114563 4.63795256614685
		-1.49455165863037 4.64759492874146
		-1.78762626647949 4.64587545394897
		-2.27300071716309 4.65301752090454
		-2.34772872924805 4.66183853149414
		-2.42698621749878 4.68191862106323
		-2.54328501224518 4.6983060836792
		-2.62138998508453 4.70752048492432
		-2.65994894504547 4.71192455291748
		-2.69729208946228 4.70599436759949
		-2.82245051860809 4.70911526679993
		-4.24607925489545 3.62715625762939
		-4.25239026546478 3.59513759613037
		-4.25868720561266 3.56131076812744
		-4.27058338187635 3.4935998916626
		-4.27952541038394 3.4586033821106
		-4.28781190142035 3.42300796508789
		-4.29417417105287 3.38643455505371
		-4.30116618098691 3.35404086112976
		-4.31371673382819 3.28272604942322
		-4.32096512615681 3.24346280097961
		-4.32518803700805 3.1681022644043
		-4.32464693486691 3.13213658332825
		-4.32279169559479 3.09304165840149
		-4.31510070711374 3.01413655281067
		-4.28759648604318 2.89460587501526
		-4.27683336474001 2.85746598243713
		-4.26667004078627 2.82028126716614
		-4.24314597994089 2.75018215179443
		-4.22870473563671 2.71562695503235
		-4.21463887393475 2.6810290813446
		-4.1993306428194 2.64952254295349
		-4.18373310565948 2.61518025398254
		-4.16802267730236 2.58314490318298
		-4.15178082883358 2.55368947982788
		-4.13792507350445 2.52309918403625
		-4.12574765086174 2.48943471908569
		-4.11309278011322 2.45494198799133
		-4.10129107534885 2.41842842102051
		-4.08049792051315 2.34778237342834
		-4.06481051445007 2.27948951721191
		-4.05937448143959 2.24639987945557
		-4.05388380587101 2.21126198768616
		-4.04847599565983 2.1759660243988
		-4.04341128468513 2.13934063911438
		-4.03808155655861 2.10271644592285
		-4.03399828076363 2.06524562835693
		-4.03035020828247 2.02861452102661
		-4.02872547507286 1.99173450469971
		-4.02544412016869 1.91340327262878
		-4.02222666144371 1.87721610069275
		-4.0193136036396 1.84034419059753
		-4.01666116714478 1.80830216407776
		-4.01274237036705 1.76624321937561
		-4.00817441940308 1.72871351242065
		-4.00273439288139 1.69208431243896
		-3.99727430939674 1.65506625175476
		-3.99231120944023 1.61896443367004
		-3.98564395308495 1.54717302322388
		-3.98372721672058 1.51123523712158
		-3.98158678412437 1.43802285194397
		-3.98043256998062 1.40123248100281
		-3.97888290882111 1.36556220054626
		-3.97903287410736 1.32728052139282
		-3.97852876782417 1.29072713851929
		-3.97833439707756 1.2563591003418
		-3.98115575313568 1.22094321250916
		-3.98535180091858 1.1841402053833
		-3.99072107672691 1.14653491973877
		-4.0029284954071 1.06973385810852
		-4.01198703050613 1.03290581703186
		-4.02261719107628 0.997755289077759
		-4.03430387377739 0.962946891784668
		-4.04721154272556 0.928728103637695
		-4.06008547544479 0.892259836196899
		-4.07302451133728 0.856697082519531
		-4.08568347990513 0.820696830749512
		-4.09867195785046 0.78463888168335
		-4.11164163053036 0.748733997344971
		-4.12567780911922 0.712336301803589
		-4.1399808973074 0.675623655319214
		-4.14946630597115 0.639552354812622
		-4.15896584093571 0.603645324707031
		-4.16860248148441 0.56838846206665
		-4.17636331915855 0.531500577926636
		-4.18890560418367 0.452875852584839
		-4.19425300508738 0.412684917449951
		-4.19804912060499 0.372173547744751
		-4.20325741916895 0.331193447113037
		-4.21689783036709 0.249642372131348
		-4.2225184366107 0.210363626480103
		-4.2256298661232 0.170556545257568
		-4.23207183927298 0.092111349105835
		-4.23849601298571 0.0522191524505615
		-4.24321653693914 0.0113778114318848
		-4.24252533912659 -0.0247721672058105
		-4.24721699208021 -0.0629119873046875
		-4.2522252202034 -0.101925373077393
		-4.25979904830456 -0.143434524536133
		-4.27272154577076 -0.221892118453979
		-4.28133198991418 -0.260664463043213
		-4.28864399436861 -0.301656246185303
		-4.31462513655424 -0.427726030349731
		-4.31932611204684 -0.466691970825195
		-4.32631871849298 -0.508678913116455
		-4.33346147835255 -0.594292998313904
		-4.33655958995223 -0.638595342636108
		-4.33565010875463 -0.682178497314453
		-4.33190390467644 -0.724361658096313
		-4.3205030914396 -0.805961489677429
		-4.12436370551586 -1.15932786464691
		-4.09654614329338 -1.18782424926758
		-4.07036246359348 -1.22015810012817
		-4.043338149786 -1.24734890460968
		-4.01493975520134 -1.27250444889069
		-3.98784151673317 -1.29670178890228
		-3.95928990840912 -1.3229056596756
		-3.93076634407043 -1.34855973720551
		-3.89939099550247 -1.37964451313019
		-3.86787104606628 -1.40865087509155
		-3.83693960309029 -1.43406057357788
		-3.80543306469917 -1.45975601673126
		-3.77352094650269 -1.48527240753174
		-3.39179545640945 -1.71536839008331
		-3.35565620660782 -1.72745668888092
		-3.31959116458893 -1.73782831430435
		-3.24723029136658 -1.75442934036255
		-3.21057844161987 -1.7602264881134
		-3.17330574989319 -1.76376509666443
		-3.09741759300232 -1.76452261209488
		-3.06309103965759 -1.76182323694229
		-3.02519679069519 -1.7592066526413
		-2.95565247535706 -1.74875092506409
		-2.92090833187103 -1.74400609731674
		-2.8880627155304 -1.73840290307999
		-2.8545229434967 -1.73079758882523
		-2.81933987140656 -1.72349554300308
		-2.78343522548676 -1.71461832523346
		-2.74781048297882 -1.70637840032578
		-2.71170544624329 -1.69879055023193
		-2.67640066146851 -1.69161885976791
		-2.63994121551514 -1.68458956480026
		-2.60458433628082 -1.67618906497955
		-2.56967496871948 -1.66767877340317
		-2.5342493057251 -1.65947639942169
		-2.49851858615875 -1.64938980340958
		-2.46415948867798 -1.63993763923645
		-2.4304313659668 -1.63060188293457
		-2.39436841011047 -1.6200076341629
		-2.35520529747009 -1.60875803232193
		-2.31709516048431 -1.59455150365829
		-2.28173542022705 -1.57849502563477
		-2.24858689308167 -1.5626460313797
		-2.18472576141357 -1.52780246734619
		-2.1537070274353 -1.50785076618195
		-2.12285566329956 -1.48744606971741
		-2.09273552894592 -1.46563458442688
		-2.06381702423096 -1.44212448596954
		-2.0360324382782 -1.41897594928741
		-2.00910758972168 -1.39702081680298
		-1.98378610610962 -1.37500655651093
		-1.96046257019043 -1.35340166091919
		-1.91445112228394 -1.30818831920624
		-1.89038801193237 -1.28404033184052
		-1.86438703536987 -1.26064562797546
		-1.84162878990173 -1.23651099205017
		-1.82075381278992 -1.21428251266479
		-1.79770517349243 -1.19187557697296
		-1.77321672439575 -1.16913676261902
		-1.74922585487366 -1.14513564109802
		-1.72442245483398 -1.12100720405579
		-1.69993138313293 -1.0984433889389
		-1.67590165138245 -1.07701814174652
		-1.6525411605835 -1.05577194690704
		-1.62922430038452 -1.03583538532257
		-1.60654878616333 -1.01764023303986
		-1.58357000350952 -0.999434947967529
		-1.56025433540344 -0.981306314468384
		-1.53724074363708 -0.963900685310364
		-1.51449966430664 -0.94619083404541
		-1.46547436714172 -0.911731719970703
		-1.44160413742065 -0.894215941429138
		-1.41630291938782 -0.876334309577942
		-1.3903443813324 -0.856740355491638
		-1.36875438690186 -0.837819933891296
		-1.34721827507019 -0.818207263946533
		-1.3238263130188 -0.796894788742065
		-1.30101227760315 -0.77394425868988
		-1.27940821647644 -0.750646829605103
		-1.25722455978394 -0.727453231811523
		-1.23586058616638 -0.704392433166504
		-1.21496295928955 -0.68113112449646
		-1.19390368461609 -0.656032204627991
		-1.17318034172058 -0.630016088485718
		-1.13173460960388 -0.576488733291626
		-1.11178255081177 -0.549714088439941
		-1.09272480010986 -0.522039175033569
		-1.07402420043945 -0.494268655776978
		-1.05753898620605 -0.466533660888672
		-1.03994178771973 -0.437890291213989
		-1.02114057540894 -0.40689754486084
		-1.00359606742859 -0.380011558532715
		-0.985740184783936 -0.352035522460938
		-0.966160297393799 -0.323455572128296
		-0.946655988693237 -0.295400381088257
		-0.928175687789917 -0.26915454864502
		-0.909447908401489 -0.243585824966431
		-0.890614986419678 -0.218994379043579
		-0.871455669403076 -0.195659875869751
		-0.852315187454224 -0.173505306243896
		-0.833538293838501 -0.152174234390259
		-0.815368413925171 -0.130190372467041
		-0.796719789505005 -0.107467889785767
		-0.777974367141724 -0.0838143825531006
		-0.758872509002686 -0.0593280792236328
		-0.738310575485229 -0.0350503921508789
		-0.695259094238281 0.0125653743743896
		-0.650846242904663 0.0570385456085205
		-0.630774259567261 0.078859806060791
		-0.612360239028931 0.100586652755737
		-0.59426212310791 0.122964859008789
		-0.577320337295532 0.144001483917236
		-0.561110258102417 0.163456678390503
	};
\addlegendentry{MOCAP}
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.381783 0.0592154
		-0.364625 0.0508084
		-0.364625 0.0508084
		-0.371554 0.0672771999999999
		-0.360835 0.0816703999999999
		-0.36961 0.0863433
		-0.378163 0.110492
		-0.37644 0.123912
		-0.397718 0.123143
		-0.323527 0.0589477
		-0.285971 0.0351405
		-0.262932 0.0305998999999999
		-0.262932 0.0305998999999999
		-0.263875 0.0224574
		-0.263875 0.0224574
		-0.286731 0.0301187999999999
		-0.277912 0.0232562000000001
		-0.277912 0.0232562000000001
		-0.273895 0.00785762999999995
		-0.320883 -0.00798875999999993
		-0.314715 0.00386942999999995
		-0.316422 -0.00911503000000002
		-0.23237 -0.0120832
		-0.404336 -0.0343768
		-0.413128 -0.0351242
		-0.41601 -0.0430926
		-0.347662 -0.0429383999999999
		-0.340086 -0.044359
		-0.445696 -0.0674759
		-0.502996 -0.0756538
		-0.45199 -0.0595213000000001
		-0.560558 -0.0651269999999999
		-0.613496 -0.0715745999999999
		-0.403727 0.0102641999999999
		-0.448422 -0.00766529999999999
		-0.462492 -0.00590419000000009
		-0.403799 -0.00684402999999989
		-0.344927 -0.00574877000000007
		-0.522387 -0.0259035000000001
		-0.516037 -0.0297305000000001
		-0.449418 -0.0255765999999999
		-0.449418 -0.0255765999999999
		-0.573051 -0.04426
		-0.573051 -0.04426
		-0.46082 -0.00956059999999992
		-0.346317 -0.0042932
		-0.346153 -0.0114905999999999
		-0.348342 -0.0173448
		-0.516037 -0.0297305000000001
		-0.39317 -0.0177248000000001
		-0.345246 -0.0184698999999999
		-0.404459 -0.0268520999999999
		-0.328358 0.00419178999999992
		-0.370145 -0.0176259000000001
		-0.369574 -0.0270809000000001
		-0.345792 -0.0195447
		-0.330701 -0.0359457000000001
		-0.354167 -0.0292573
		-0.366586 -0.0578821
		-0.371543 -0.0611196999999999
		-0.385381 -0.0545819000000001
		-0.383156 -0.0684788999999999
		-0.414541 -0.0755307999999999
		-0.387448 -0.0774896
		-0.6942 -0.180383
		-0.698674 -0.22637
		-0.70181 -0.273877
		-0.67365 -0.289097
		-0.685673 -0.289878
		-0.665234 -0.293246
		-0.609943 -0.267475
		-0.601637 -0.275957
		-0.600253 -0.278956
		-0.613533 -0.323594
		-0.646887 -0.366849
		-0.631521 -0.385619
		-0.672612 -0.42998
		-0.685552 -0.439788
		-0.619214 -0.422878
		-0.629491 -0.439108
		-0.612355 -0.452343
		-0.540327 -0.412565
		-0.500758 -0.440772
		-0.523819 -0.465308
		-0.283811 -0.447548
		-0.263318 -0.426325
		-0.246094 -0.412868
		-0.236754 -0.451173
		-0.193853 -0.449484
		-0.201959 -0.468993
		-0.175079 -0.431445
		-0.149675 -0.415545
		-0.123233 -0.412733
		-0.120955 -0.461828
		-0.0818791999999999 -0.444194
		-0.0601996 -0.452534
		-0.0536388000000001 -0.46773
		-0.0444884000000001 -0.417804
		-0.0329667 -0.418871
		-0.0487774000000001 -0.472253
		-0.0288261000000001 -0.434451
		-0.0305126 -0.455509
		-0.0238807000000001 -0.455905
		-0.0364211000000001 -0.45205
		-0.0407271 -0.472888
		-0.0496875000000001 -0.47203
		-0.047031 -0.45107
		-0.0541480999999999 -0.471539
		-0.0511973000000001 -0.463002
		-0.0309554999999999 -0.446644
		-0.00214158999999992 -0.436874
		-0.0291375 -0.450512
		0.0553709 -0.412206
		0.0759021 -0.493364
		0.150973 -0.514927
		-0.0225035 -0.409154
		0.0498491000000001 -0.394805
		0.136327 -0.463989
		0.0532954999999999 -0.363879
		0.14528 -0.454586
		0.138417 -0.424181
		0.150394 -0.446553
		0.240286 -0.43732
		0.151946 -0.215367
		0.151706 -0.20101
		0.201341 -0.202759
		0.20302 -0.205622
		0.303087 -0.326552
		0.261452 -0.266293
		0.316522 -0.299565
		0.370989 -0.345549
		0.387747 -0.349186
		0.457959 -0.403203
		0.409389 -0.324541
		0.26838 -0.185596
		0.320523 -0.204114
		0.304842 -0.17587
		0.338462 -0.174113
		0.500511 -0.250255
		0.307502 -0.122404
		0.353353 -0.126801
		0.386004 -0.144752
		0.348866 -0.113546
		1.68855 0.531167
		1.58247 0.532661
		0.358422 -0.147586
		0.485784 -0.212979
		0.479852 -0.171541
		0.369553 -0.118978
		0.376475 -0.0381931
		0.328826 -0.0288725000000001
		0.297445 0.0042091099999999
		0.31888 0.0355958999999999
		0.328349 0.0786187
		0.335023 0.120103
		0.322988 0.132547
		0.322988 0.132547
		0.326073 0.14458
		0.29159 0.156799
		0.29159 0.156799
		0.312992 0.181445
		0.260016 0.155252
		0.302954 0.184407
		0.302954 0.184407
		0.332277 0.233763
		0.270014 0.20592
		0.278277 0.234264
		0.249446 0.478776
		0.251216 0.562911
		0.192968 0.69415
		0.227214 0.775556
		0.227214 0.775556
		0.184308 0.720969
		0.184308 0.720969
		0.154905 0.691731
		0.152405 0.82734
		0.152405 0.82734
		0.100509 0.848041
		0.0436584 0.739465
		0.0436584 0.739465
		-0.0285401999999999 0.846694
		-0.0450356000000001 0.804634
		-0.0908184000000001 0.82676
		-0.10419 0.812068
		-0.105031 0.815533
		-0.110771 0.827706
		-0.18437 0.814299
		-0.222653 0.80521
		-0.209862 0.693342
		-0.180152 0.571212
		-0.22733 0.553024
		-0.257996 0.535181
		-0.265449 0.526751
		-0.250095 0.504159
		-0.410361 0.656577
		-0.490888 0.692853
		-0.709664 0.672667
		-0.769111 0.698225
		-0.717923 0.589386
		-0.719545 0.55697
		-0.717481 0.537372
		-0.750421 0.531675
		-0.794521 0.458986
		-0.834342 0.44171
		-0.875934 0.42251
		-0.879243 0.41558
		-0.812322 0.0833151000000001
		-0.843488 0.0744254
		-0.840181 0.0463335
		-0.841255 0.0184891
		-0.848627 -0.0124797999999999
		-0.830397 -0.0513337
		-0.837298 -0.0943864000000001
		-0.892338 -0.18752
		-0.905326 -0.224703
		-0.939874 -0.192708
		-0.975514 -0.184651
		-1.01926 -0.211889
		-0.99124 -0.233649
		-1.01849 -0.244585
		-1.03403 -0.27328
		-1.12221 -0.30751
		-1.11258 -0.327461
		-1.10823 -0.3419
		-1.21266 -0.367215
		-1.26486 -0.415661
		-1.28179 -0.437796
		-1.28868 -0.467373
		-1.25819 -0.484602
		-1.25519 -0.492318
		-1.17685 -0.485818
		-1.31106 -0.582696
		-1.32581 -0.613364
		-1.25827 -0.597453
		-1.26506 -0.653233
		-1.25072 -0.673465
		-1.14851 -0.631051
		-1.23919 -0.708109
		-1.15291 -0.700286
		-1.17609 -0.742792
		-1.04978 -0.685328
		-1.12446 -0.759652
		-1.04974 -0.734821
		-1.03395 -0.76842
		-1.03691 -0.797302
		-1.03985 -0.816726
		-1.09546 -0.870978
		-1.12507 -0.943919
		-1.13947 -0.991484
		-1.14927 -0.98011
		-1.16155 -1.00634
		-1.14725 -1.01699
		-1.22159 -1.09836
		-1.24911 -1.14363
		-1.18221 -1.09248
		-1.28783 -1.21173
		-1.24905 -1.15983
		-1.26054 -1.18141
		-1.24905 -1.15983
		-1.17881 -1.10022
		-1.27198 -1.19284
		-1.17422 -1.10181
		-1.21445 -1.11899
		-1.17904 -1.09666
		-1.29338 -1.21964
		-1.24658 -1.18617
		-1.2246 -1.17042
		-1.28615 -1.23516
		-1.28604 -1.23527
		-1.25581 -1.21691
		-1.2104 -1.2104
		-1.23297 -1.24941
		-1.16666 -1.18228
		-1.25977 -1.29896
		-1.2783 -1.35892
		-1.6774 -1.80302
		-1.67066 -1.80927
		-1.66702 -1.81325
		-1.64771 -1.83727
		-1.61811 -1.85031
		-1.36331 -1.55198
		-1.34791 -1.57968
		-1.33175 -1.55573
		-1.21425 -1.41385
		-1.34979 -1.60209
		-1.20726 -1.46352
		-1.07454 -1.35217
		-1.09806 -1.39266
		-1.13394 -1.46514
		-1.13639 -1.50186
		-1.19193 -1.59938
		-1.24933 -1.72934
		-1.35374 -1.92564
		-1.25119 -1.94004
		-1.10129 -1.7138
		-1.178 -1.84732
		-1.17274 -1.92028
		-1.12542 -1.90716
		-1.25084 -2.16403
		-1.11918 -2.00607
		-1.07621 -1.99374
		-0.995488 -1.87386
		-0.915888 -1.80685
		-0.959369 -1.91208
		-0.938994 -1.93126
		-0.911593 -1.89533
		-0.730691 -1.63429
		-0.716068 -1.64075
		-0.675666 -1.59108
		-0.587655 -1.52161
		-0.567734 -1.56395
		-0.560093 -1.63037
		-0.527054 -1.63664
		-0.501797 -1.6689
		-0.420226 -1.60111
		-0.354562 -1.51955
		-0.302418 -1.5531
		-0.294859 -1.54547
		-0.267515 -1.51592
		-0.258759 -1.68469
		-0.225302 -1.73483
		-0.211361 -1.66379
		-0.140989 -1.53073
		-0.116328 -1.68398
		-0.0623393999999999 -1.57926
		-0.0305692 -1.55904
		0.0166054 -1.67716
		0.0693092 -1.62077
		0.118352 -1.61927
		0.173668 -1.46171
		0.188131 -1.13631
		0.21169 -1.11787
		0.243928 -1.17636
		0.284487 -1.26533
		0.292074 -1.20943
		0.33226 -1.25137
		0.331772 -1.18143
		0.4718 -1.49492
		0.552123 -1.45463
		0.571173 -1.32474
		0.627187 -1.50745
		0.672738 -1.48768
		0.644563 -1.21141
		0.670925 -1.19225
		0.737979 -1.16032
		0.754414 -1.16754
		0.880029 -1.25859
		0.795352 -1.11971
		1.00861 -1.30961
		1.1422 -1.45586
		0.894273 -1.07839
		0.928825 -1.06659
		1.30722 -1.44904
		1.09088 -1.1512
		1.43026 -1.38576
		1.32163 -1.19791
		1.34329 -1.18895
		1.37535 -1.21665
		1.17882 -0.971667
		1.12752 -0.892811
		1.19255 -0.931373
		1.14428 -0.829714
		1.14428 -0.829714
		1.03654 -0.685649
		1.06225 -0.681682
		1.06225 -0.681682
		0.954364 -0.588154
		1.04394 -0.623126
		1.04394 -0.623126
		0.792675 -0.440704
		1.13851 -0.608363
		1.21296 -0.569724
		1.21915 -0.53733
		1.33151 -0.558059
		1.283 -0.50023
		1.19526 -0.449281
		1.19526 -0.449281
		1.65952 -0.440991
		1.61718 -0.353758
		1.63789 -0.313043
		1.64824 -0.279364
		1.64544 -0.238229
		1.64544 -0.238229
		1.82886 -0.146309
		1.83244 -0.0910153
		1.83244 -0.0910153
		1.47251 -0.038497
		1.38174 -0.0315055
		1.34339 0.00439012999999999
		1.39397 0.0228520000000001
		1.37279 0.0855181
		1.6897 0.174023
		1.82501 0.211508
		1.82122 0.242022
		1.78481 0.261772
		1.69445 0.285261
		1.76105 0.395337
		1.71716 0.450016
		1.71348 0.527225
		1.66342 0.673567
		1.67214 0.741198
		1.63325 0.790655
		1.63325 0.790655
		1.61231 0.823429
		1.59455 0.857283
		1.59455 0.857283
		1.58932 0.981641
		1.46841 0.927989
		1.47599 0.983996
		1.34558 0.974388
		1.41438 1.16242
		1.19584 1.09207
		0.773188 1.63829
		0.784689 1.74565
		0.677566 1.68591
		0.215202 1.10334
		0.194579 1.14625
		0.189273 0.992158
		0.444737 1.51025
		0.67913 1.86761
		0.688654 1.86412
		0.514561 1.55811
		0.519035 1.65285
		0.514363 1.74459
		0.31485 1.45181
		0.342553 1.64823
		0.339947 1.70489
		0.316228 1.69335
		0.309637 1.80893
		0.419484 1.98799
		0.0985986000000001 1.24386
		0.0651912000000001 1.13722
		0.0809465 1.13325
		0.0826989 1.21292
		0.0709654 1.24584
		-0.0819605000000001 1.68531
		-0.0783615 1.47504
		-0.0574938 1.41523
		-0.0444049 1.41651
		-0.0691895 1.47604
		-0.0827093999999999 1.4658
		-0.0954157 1.51711
		-0.106841 1.54434
		-0.100798 1.51676
		-0.12419 1.47189
		-0.134925 1.47953
		-0.125222 1.43558
		-0.545078 1.74317
		-0.75206 1.87714
		-0.845908 1.79031
		-0.966248 1.79608
		-0.905655 1.79401
		-0.958038 1.67251
		-1.0065 1.71664
		-0.962706 1.72391
		-0.977458 1.6471
		-1.01196 1.70346
		-0.915909 1.64535
		-0.907055 1.61934
		-1.42377 0.845206
		-1.30581 0.696433
		-1.3729 0.337367
		-1.76135 0.381626
		-1.8446 0.367694
		-1.79718 0.336596
		-1.37965 0.209743
		-1.39674 0.141562
		-1.55869 0.10984
		-1.545 0.0826754999999999
		-1.33359 0.0450535000000001
		-1.35284 0.00914075000000003
		-1.726 -0.0396131
		-1.66049 -0.0544424999999999
		-1.5365 -0.0668040999999999
		-1.59249 -0.0905427999999999
		-1.72644 -0.120851
		-1.6259 -0.151247
		-1.62515 -0.195018
		-1.29082 -0.175621
		-1.3059 -0.205023
		-1.49509 -0.285974
		-1.32306 -0.282552
		-1.29197 -0.313072
		-1.30806 -0.341624
		-1.29835 -0.38636
		-1.31245 -0.425288
		-1.29803 -0.422087
		-1.18679 -0.402588
		-1.23866 -0.449619
		-1.19526 -0.464346
		-1.09835 -0.46789
		-1.08326 -0.496657
		-1.10339 -0.626363
		-1.04235 -0.804468
		-1.04813 -0.847428
		-1.02492 -0.8645
		-1.01747 -0.878523
		-1.11061 -1.00872
		-0.960876 -0.907246
		-1.02243 -1.00286
		-1.02249 -1.02748
		-0.973367 -1.0269
		-0.958644 -1.06136
		-0.856865 -1.02285
		-0.757564 -0.941837
		-0.786958 -0.991307
		-0.741897 -1.00325
		-0.694372 -0.972121
		-0.665576 -0.986336
		-0.657275 -0.991887
		-0.60182 -0.965183
		-0.559121 -0.961688
		-0.472299 -0.948203
		-0.432444 -0.963837
		-0.384638 -0.96709
		-0.359103 -0.961234
		-0.297999 -0.959412
		-0.25461 -0.940642
		-0.221208 -0.949053
		-0.197559 -0.973159
		-0.175208 -0.974596
		-0.12117 -1.01859
		-0.0342975999999999 -1.02512
		0.108453 -1.04192
		0.147509 -0.988307
		0.209058 -1.05735
		0.267483 -1.04198
		0.323302 -0.981317
		0.333885 -0.92082
		0.393053 -0.880022
		0.443209 -0.862368
		0.452488 -0.856619
		0.475831 -0.79966
		0.499095 -0.794612
		0.452434 -0.661685
		0.445757 -0.625147
		0.583597 -0.81151
		0.648884 -0.747094
		0.706477 -0.764743
		0.692397 -0.717
		0.686679 -0.659484
		0.717725 -0.59421
		0.77818 -0.621116
		0.764994 -0.572082
		0.675891 -0.478635
		0.675891 -0.478635
		0.706057 -0.457201
		0.780319 -0.473878
		0.882527 -0.466819
		0.827228 -0.402521
		0.827228 -0.402521
		0.998673 -0.379724
		1.04233 -0.295
		1.04233 -0.295
		1.03159 -0.255958
		1.02947 -0.237277
		0.853555 -0.134937
		0.87523 -0.0865610999999999
		0.877594 -0.0578633
		0.969341 0.0246740999999999
		0.790304 0.0318438000000001
		0.789427 0.0489790000000001
		0.805164 0.0787661
		1.06613 0.213226
		1.11518 0.275662
		1.11518 0.275662
		1.15282 0.451483
		1.05057 0.463367
		1.16311 0.570241
		1.06999 0.564028
		1.14686 0.715098
		1.14686 0.715098
		0.989498 0.697773
		0.823625 0.62104
		0.860501 0.655785
		0.866304 0.74568
		0.866304 0.74568
		0.859771 0.767521
		0.77105 0.774721
		0.77105 0.774721
		0.779528 0.828961
		0.71543 0.84212
		0.663479 0.806651
		-0.109667 1.52104
		-0.100166 1.5168
		-0.121891 1.52832
		-0.162115 1.73619
		-0.122548 1.58332
		-0.21409 1.98033
		-0.175503 1.82084
		-0.124483 1.81313
		-0.220382 1.95444
		-0.160304 1.74783
		-0.148618 1.80465
		-0.185957 1.61639
		-0.308305 1.96617
		-0.420337 1.96157
		-0.160083 1.53491
		-0.143601 1.55089
		-0.58678 1.97207
		-0.714022 2.25991
		-0.711293 2.2084
		-0.91876 2.30793
		-0.812836 2.02884
		-1.01621 2.29752
		-1.02828 2.1475
		-1.01385 2.04096
		-0.949425 1.6978
		-0.969041 1.7362
		-0.877883 1.51359
		-1.02204 1.68637
		-1.02953 1.62096
		-1.18785 1.86391
		-1.27287 1.98002
		-1.30818 1.94892
		-1.33831 2.04929
		-1.25985 1.83989
		-1.2258 1.75457
		-1.32714 1.82795
		-1.17442 1.61
		-1.15435 1.54983
		-1.20201 1.55489
		-1.34393 1.66937
		-1.22974 1.51687
		-1.60331 1.81941
		-1.71462 1.90595
		-1.75102 1.87609
		-1.88928 1.99995
		-1.78771 1.87033
		-1.91905 1.95903
		-1.86277 1.87044
		-1.92583 1.9103
		-2.0109 1.94731
		-2.034 1.94591
		-2.14706 1.95039
		-2.25658 2.00208
		-2.17665 1.90863
		-2.18946 1.88132
		-2.13558 1.82037
		-2.19551 1.83361
		-2.26893 1.84814
		-2.53339 2.03773
		-2.48439 1.98931
		-2.41226 1.90534
		-2.31945 1.82541
		-2.34461 1.80678
		-2.48019 1.87786
		-2.46618 1.84526
		-2.56835 1.87445
		-2.66763 1.89226
		-2.67836 1.85284
		-2.78894 1.85299
		-2.66304 1.7395
		-2.82293 1.84394
		-2.76938 1.74471
		-2.73109 1.66951
		-2.95808 1.76309
		-2.83011 1.65323
		-2.98117 1.71613
		-2.97698 1.67334
		-2.94804 1.58814
		-2.97322 1.47236
		-2.74757 1.34326
		-2.71101 1.31288
		-2.72328 1.26803
		-2.59336 1.17953
		-2.58497 1.15961
		-2.59228 1.14318
		-2.61459 1.13783
		-2.63012 1.11679
		-2.76025 1.15291
		-2.81446 1.12065
		-3.04411 1.14385
		-3.07309 1.10818
		-3.01992 1.04009
		-3.19181 1.07361
		-3.19857 1.0533
		-3.24984 1.04739
		-3.18568 1.00449
		-3.42922 1.05436
		-3.33031 0.965594
		-3.27769 0.911548
		-3.05253 0.837419
		-3.26171 0.875561
		-3.27048 0.820032
		-3.29381 0.782402
		-3.17762 0.752593
		-3.19843 0.710762
		-3.11259 0.635222
		-3.2896 0.602456
		-3.37477 0.549382
		-3.37297 0.539282
		-3.37744 0.510543
		-3.16968 0.486936
		-3.23406 0.45933
		-3.38711 0.441797
		-3.22063 0.361973
		-3.34043 0.36476
		-3.24715 0.335912
		-3.2499 0.30818
		-3.3536 0.289104
		-3.35739 0.241192
		-3.53392 0.254605
		-3.40791 0.206839
		-3.43041 0.15772
		-3.37261 0.0872227000000001
		-3.39158 0.0389838
		-3.40971 -0.00977015000000003
		-3.23932 -0.0278453000000001
		-3.38996 -0.107154
		-3.43796 -0.11855
		-3.23645 -0.139103
		-3.4041 -0.195638
		-3.2318 -0.222244
		-3.23048 -0.240666
		-3.31243 -0.314109
		-3.39824 -0.351542
		-3.34416 -0.357613
		-3.46292 -0.411535
		-3.38523 -0.419496
		-3.47719 -0.443468
		-3.45537 -0.470732
		-3.39148 -0.505748
		-3.39154 -0.556968
		-3.24086 -0.560736
		-3.26843 -0.596007
		-3.22911 -0.609626
		-3.33971 -0.662013
		-3.4263 -0.74
		-3.33129 -0.758903
		-3.33129 -0.758903
		-2.95953 -0.759761
		-2.73446 -0.718305
		-2.63038 -0.73241
		-2.84975 -0.832608
		-2.86785 -0.886427
		-2.59338 -0.851322
		-2.56497 -0.93343
		-2.7939 -1.05202
		-2.7939 -1.05202
		-2.77837 -1.0853
		-2.77712 -1.12304
		-2.724 -1.14649
		-2.73907 -1.22029
		-2.49734 -1.125
		-2.44624 -1.1484
		-2.44017 -1.16124
		-2.62863 -1.30578
		-2.62863 -1.30578
		-2.30749 -1.22117
		-2.51812 -1.36159
		-2.58731 -1.4687
		-2.53155 -1.46342
		-2.51136 -1.53378
		-2.55102 -1.5792
		-2.79788 -1.82938
		-2.67977 -1.76771
		-2.39377 -1.66186
		-2.42331 -1.71469
		-2.42331 -1.71469
		-2.41198 -1.7454
		-2.41198 -1.7454
		-2.3319 -1.74035
		-2.06808 -1.6068
		-1.95211 -1.54421
		-1.90625 -1.54793
		-1.90625 -1.54793
		-1.97044 -1.64203
		-1.91342 -1.64217
		-1.91342 -1.64217
		-1.86089 -1.62918
		-1.89897 -1.75522
		-1.89897 -1.75522
		-1.90984 -1.80973
		-1.92202 -1.85112
		-1.85257 -1.85257
		-2.06337 -2.09834
		-2.03439 -2.10394
		-2.04605 -2.12508
		-1.89461 -2.01872
		-1.84869 -2.00275
		-1.78437 -1.98441
		-1.76374 -1.99623
		-1.67011 -2.00098
		-1.66675 -2.00803
		-1.60243 -1.97993
		-1.57283 -1.96416
		-1.54144 -2.05012
		-1.54144 -2.05012
		-1.51681 -2.09538
		-1.49994 -2.12819
		-1.46954 -2.09602
		-1.52017 -2.34395
		-1.52017 -2.34395
		-1.53164 -2.40563
		-1.38451 -2.2619
		-1.3118 -2.28764
		-1.28638 -2.24332
		-1.09528 -2.0563
		-1.08131 -2.06368
		-1.16371 -2.25851
		-1.04885 -2.09769
		-1.08683 -2.21062
		-1.06908 -2.21926
		-1.02993 -2.2377
		-1.1222 -2.35428
		-1.01845 -2.32789
		-0.98167 -2.46222
		-0.941294 -2.47794
		-0.895692 -2.50148
		-0.891527 -2.49627
		-0.843771 -2.46763
		-0.819914 -2.47566
		-0.764941 -2.41845
		-0.690719 -2.39854
		-0.667272 -2.51816
		-0.669244 -2.51763
		-0.654327 -2.52155
		-0.635527 -2.53416
		-0.588638 -2.54546
		-0.50348 -2.49416
		-0.494257 -2.60903
		-0.409662 -2.63003
		-0.383083 -2.5174
		-0.348755 -2.61971
		-0.301145 -2.62892
		-0.269772 -2.63232
		-0.222295 -2.65108
		-0.196527 -2.65311
		-0.163909 -2.65533
		-0.131753 -2.65977
		-0.0992352999999999 -2.67935
		-0.0655763 -2.66403
		-0.0244770000000001 -2.65166
		0.0326348999999999 -2.65158
		0.0334612000000001 -2.72708
		2.69079 -0.39619
		2.67586 -0.0970099
		2.41167 -0.0292323000000001
		2.41167 -0.0292323000000001
		2.48704 0.0302377
		2.48585 0.0828617
		2.41226 0.176507
		2.41226 0.176507
		2.54767 0.194182
		2.42475 0.206362
		2.51972 0.238144
		2.62013 0.255623
		2.40092 0.292796
		2.40092 0.292796
		2.4052 0.315315
		2.53428 0.37087
		2.53428 0.37087
		2.51912 0.416002
		2.52369 0.432192
		2.55485 0.46878
		2.51276 0.491793
		2.61315 0.545075
		2.63525 0.600026
		2.62353 0.631591
		2.58338 0.655844
		2.64691 0.715159
		2.54771 0.76671
		2.54771 0.76671
		2.6251 0.817248
		2.7273 0.897591
		2.75524 0.950382
		2.73841 0.979242
		2.70739 1.03139
		2.70739 1.03139
		2.73715 1.08963
		2.74171 1.17377
		2.56602 1.14687
		2.48967 1.14846
		2.43901 1.15656
		2.4496 1.17327
		2.38653 1.26021
		2.5062 1.39978
		2.43485 1.39718
		2.46914 1.405
		2.4855 1.46452
		2.46885 1.49805
		2.42946 1.52048
		2.51279 1.578
		2.47058 1.55462
		2.62646 1.68202
		2.48303 1.61269
		2.45377 1.61898
		2.55237 1.70745
		2.58278 1.75735
		2.54624 1.77706
		2.55956 1.80516
		2.57908 1.85258
		2.59878 1.90516
		2.54981 1.93968
		2.5407 1.9812
		2.2608 1.92002
		-0.86162 3.0329
		-0.905599 3.03591
		-0.97544 3.24218
		-0.919022 3.02583
		-1.06205 3.31053
		-1.08502 3.30307
		-1.05293 2.98759
		-1.08779 2.99574
		-1.11557 3.04805
		-1.14638 3.03659
		-1.08226 2.83682
		-1.29437 3.35359
		-1.15931 3.00368
		-1.42004 3.36638
		-1.41373 3.28571
		-1.45958 3.22643
		-1.87105 3.96854
		-1.54855 3.23346
		-1.96787 3.94775
		-1.96497 3.80205
		-2.07801 3.79412
		-2.34841 3.87731
		-2.40252 3.901
		-2.44285 3.87616
		-3.07085 3.22558
		-3.38282 2.92859
		-3.41048 2.87574
		-3.41377 2.85666
		-3.39318 2.81786
		-3.39162 2.79516
		-3.40692 2.75354
		-3.43284 2.74159
		-3.37578 2.67537
		-3.40485 2.67524
		-3.4522 2.67984
		-3.48343 2.68047
		-3.48948 2.60532
		-3.47084 2.53058
		-3.48471 2.49738
		-3.54178 2.44301
		-3.58204 2.44283
		-3.63055 2.43613
		-3.63159 2.3858
		-3.56055 2.3201
		-3.66447 2.32553
		-3.58932 2.24763
		-3.62013 2.23664
		-3.66951 2.21336
		-3.77095 2.21961
		-3.78355 2.19806
		-3.73582 2.12636
		-3.66337 2.06065
		-3.7339 2.08214
		-3.709 2.02728
		-3.7595 2.0422
		-3.76331 2.01482
		-3.72784 1.96082
		-3.68062 1.90221
		-3.67638 1.86047
		-3.78274 1.88565
		-3.70143 1.8004
		-3.73891 1.7681
		-3.76704 1.7369
		-3.81484 1.70694
		-3.68252 1.58767
		-3.75276 1.54131
		-3.75984 1.52396
		-3.78998 1.52046
		-3.76536 1.49948
		-3.78421 1.46917
		-3.78261 1.43517
		-3.74411 1.39036
		-3.76385 1.37567
		-3.78501 1.35731
		-3.8875 1.3335
		-3.90121 1.29284
		-3.91521 1.2861
		-3.94132 1.2338
		-3.9327 1.20481
		-3.93118 1.16689
		-3.92098 1.15257
		-3.88156 1.09308
		-3.88868 1.08081
		-3.82504 1.03233
		-3.80814 1.00613
		-3.84757 0.997519
		-3.87825 0.964022
		-3.93131 0.965978
		-3.84026 0.894607
		-3.93051 0.88825
		-3.9573 0.847196
		-3.9637 0.779378
		-3.92085 0.704872
		-3.92463 0.683503
		-3.93444 0.676059
		-4.05409 0.681361
		-3.99188 0.613277
		-4.0014 0.547678
		-4.00181 0.544691
		-4.00769 0.499574
		-4.0102 0.478997
		-4.0278 0.446293
		-4.04804 0.438538
		-4.0381 0.426244
		-4.04552 0.357615
		-4.05589 0.325819
		-4.05589 0.325819
		-4.04846 0.268406
		-4.08206 -0.0334597000000001
		-3.69538 -1.25379
		-3.59904 -1.33741
		-3.40392 -1.29328
		-3.56591 -1.34809
		-3.3786 -1.30986
		-3.33536 -1.28913
		-3.33126 -1.29549
		-3.37999 -1.3104
		-3.41547 -1.33466
		-3.1975 -1.25722
		-3.18821 -1.27331
		-3.1454 -1.24058
		-2.90911 -1.15642
		-2.9154 -1.14986
		-2.75031 -1.0967
		-2.77724 -1.11609
		-2.7794 -1.12045
		-2.75566 -1.09365
		-2.50858 -0.998713
		-2.44822 -0.985446
		-2.47562 -0.980905
		-2.47361 -0.95979
		-2.47361 -0.95979
		-2.46191 -0.941544
		-2.49977 -0.94228
		-2.48855 -0.935138
		-2.49376 -0.90894
		-2.30713 -0.850755
		-2.32947 -0.837152
		-2.24977 -0.775782
		-2.24298 -0.782926
		-2.21653 -0.731872
		-2.27223 -0.71187
		-2.27952 -0.688158
		-2.23364 -0.653235
		-2.26054 -0.591877
		-2.25927 -0.563036
		-2.04253 -0.496135
		-2.13539 -0.488662
		-2.03976 -0.455417
		-2.04508 -0.430881
		-1.92606 -0.402278
		-1.77043 -0.354085
		-1.81417 -0.341968
		-1.81726 -0.325133
		-1.86138 -0.297346
		-1.95067 -0.301524
		-1.79392 -0.260408
		-1.7754 -0.2421
		-1.77763 -0.22509
		-1.91593 -0.22178
		-1.86705 -0.196845
		-1.84798 -0.159921
		-1.84701 -0.130657
		-1.7989 -0.0756816
		-1.83276 -0.0523646
		-1.99432 -0.0314562
		-1.90235 0.0240804999999999
		-1.83318 0.0350288999999999
		-1.8576 0.0844362999999999
		-1.93221 0.139831
		-1.77916 0.174427
		-1.77603 0.203807
		-1.82403 0.234004
		-1.77764 0.249701
		-1.91049 0.301656
		-1.84947 0.332905
		-1.87861 0.378243
		-1.89791 0.450989
		-1.8878 0.489198
		-1.32214 0.388068
		-1.3116 0.410156
		-1.30061 0.457705
		-1.31609 0.52829
		-1.27822 0.52845
		-1.24456 0.525185
		-1.25114 0.562563
		-1.35696 0.629666
		-1.18715 0.615889
		-1.21606 0.630886
		-1.20077 0.634369
		-1.12789 0.656857
		-1.10181 0.699226
		-1.05757 0.7009
		-0.987958 0.684569
		-0.971186 0.727407
		-0.054006 0.82146
		-0.0607356000000001 0.877631
		-0.0386263 0.855722
		-0.00907057 0.876818
		-0.00283915000000001 0.826174
		0.0415824 0.809471
		0.0879236999999999 0.882269
		0.129963 0.935733
		0.145717 0.720918
		0.266995 0.792373
		0.395538 0.996307
		0.312152 0.823225
		0.297869 0.751632
		0.412592 0.888404
		0.362147 0.71068
		0.381034 0.685331
		0.398873 0.653849
		0.504596 0.750888
		0.572101 0.782529
		0.525829 0.671086
		0.575764 0.693393
		0.583922 0.676608
		0.637042 0.682085
		0.61049 0.628805
		0.66998 0.660128
		0.674138 0.629196
		0.684408 0.598058
		0.754016 0.632958
		0.862394 0.662801
		0.897249 0.657729
		0.918078 0.643407
		0.931884 0.637605
		0.927527 0.594665
		0.956697 0.554277
		0.883823 0.489072
		0.858765 0.431053
		0.851005 0.352936
		0.903708 0.289605
		0.915702 0.249099
		0.935868 0.221465
		0.926381 0.205862
		0.927287 0.201738
		0.931147 0.162862
		0.954894 0.118911
		0.971527 0.0843212
		0.931046 0.0351338000000001
		0.957772 -0.0036280099999999
		1.05879 -0.0275521000000001
		1.07804 -0.0571687999999999
		0.967437 -0.543192
		0.819554 -0.503059
		0.859691 -0.563732
		0.859691 -0.563732
		0.762592 -0.524282
		0.818458 -0.723729
		0.751699 -0.726156
		0.685427 -0.843306
		0.653952 -0.782598
		0.653952 -0.782598
		0.644001 -0.872161
		0.658479 -0.915636
		0.658479 -0.915636
		0.615993 -0.916477
		0.591848 -0.898733
		0.581118 -0.945742
		0.57175 -0.986855
		0.56376 -0.991441
		0.483871 -1.01495
		0.44904 -1.01625
		0.469027 -1.07265
		0.425128 -1.11809
		0.431773 -1.24313
		0.373882 -1.1259
		0.3371 -1.08847
		0.33568 -1.11479
		0.284744 -1.12247
		0.23827 -1.04385
		0.195106 -0.993597
		0.184085 -1.02351
		0.184085 -1.02351
		0.145305 -1.02803
		0.126076 -1.02302
		0.0979451 -1.00394
		0.0737543000000001 -1.051
		0.0737543000000001 -1.051
		0.0250366 -1.01219
		0.0250366 -1.01219
		0.0104827999999999 -1.01334
		-0.028219 -0.991189
		-0.028219 -0.991189
		-0.0445593 -0.990589
		-0.128929 -1.3077
		-0.128929 -1.3077
		-0.184322 -1.42476
		-0.207841 -1.43968
		-0.186285 -1.25077
		-0.21496 -1.28976
		-0.271712 -1.429
		-0.284935 -1.41959
		-0.292557 -1.19604
		-0.317805 -1.18962
		-0.353933 -1.19129
		-0.361842 -1.18891
		-0.410037 -1.11828
		-0.426812 -1.14944
		-0.44968 -1.11587
		-0.52183 -1.233
		-0.487166 -1.12684
		-0.509126 -1.11583
		-0.529779 -1.10618
		-0.538251 -1.05204
		-0.545994 -1.04683
		-0.561103 -1.0321
		-0.580134 -1.01938
		-0.625583 -1.04839
		-0.608359 -1.02953
		-0.626075 -0.993372
		-0.669987 -1.03344
		-0.684415 -1.01363
		-0.7017 -0.993712
		-0.689826 -0.93187
		-0.700047 -0.881827
		-0.727461 -0.867507
		-0.698076 -0.824324
		-0.70346 -0.801871
		-0.688932 -0.773291
		-0.757068 -0.828632
		-0.715575 -0.761175
		-0.701855 -0.728849
		-0.766025 -0.766025
		-0.792976 -0.781701
		-0.822547 -0.784289
		-0.803644 -0.773461
		-0.825807 -0.79508
		-0.799882 -0.77735
		-0.752548 -0.748981
		-0.783481 -0.802315
		-0.719273 -0.757681
		-0.728191 -0.78978
		-0.759577 -0.831736
		-0.699921 -0.780412
		-0.675451 -0.772439
		-0.67801 -0.819262
		-0.640708 -0.818296
		-0.625511 -0.866937
		-0.59579 -0.882652
		-0.596105 -0.909249
		-0.609539 -0.980913
		-0.576425 -1.00568
		-0.528293 -0.963358
		-0.494513 -0.973573
		-0.449776 -0.99261
		-0.442499 -0.992737
		-0.377173 -0.957723
		-0.361121 -1.01347
		-0.339418 -1.02606
		-0.300135 -0.99795
		-0.27425 -0.993229
		-0.241344 -0.965378
		-0.204745 -0.966251
		-0.18059 -0.941151
		-0.181978 -1.01016
		-0.160797 -0.997671
		-0.143594 -1.00516
		-0.109568 -1.039
		-0.0815001 -1.08667
		-0.0557970000000001 -1.03782
		-0.0109399999999999 -1.0393
		0.0439780000000001 -1.02982
		0.05514 -1.02928
		0.0626895999999999 -1.02885
		0.0910625999999999 -1.04722
		0.0893010000000001 -1.0344
		0.104012 -1.03641
		0.100615 -1.01333
		0.0843130999999999 -1.06924
		0.0772915999999999 -1.07822
		0.0717433999999999 -1.05727
		0.0498875999999999 -1.06683
		0.0450895 -1.03706
		-0.00786014999999995 -1.07291
		-0.0353226 -1.0793
		-0.0635725 -1.1006
		-0.105179 -1.0882
		-0.129697 -0.972723
		-0.166402 -1.02163
		-0.203408 -1.02486
		-0.230732 -1.01679
		-0.245628 -0.963904
		-0.311446 -0.956851
		-0.349247 -0.94371
		-0.439231 -0.915065
		-0.501063 -0.934313
		-0.563395 -0.964119
		-0.58473 -0.956112
		-0.570831 -0.858088
		-0.592071 -0.847904
		-0.627349 -0.826448
		-0.692815 -0.86298
		-0.744933 -0.860171
		-0.747855 -0.801547
		-1.14505 -0.125429
		-1.16681 -0.110154
		-1.16241 -0.0407862999999999
		-1.18831 0
		-1.10485 0.0193156000000001
		-1.16094 0.0369202
		-1.13234 0.0600179999999999
		-1.13188 0.0682336000000001
		-1.21282 0.107902
		-1.14663 0.122416
		-1.17338 0.171205
		-1.13066 0.220519
		-1.14317 0.246408
		-1.0817 0.23952
		-1.18225 0.298763
		-1.2054 0.305716
		-1.19666 0.345607
		-1.17504 0.390266
		-1.19913 0.430123
		-1.16711 0.424404
		-1.19441 0.458725
		-1.18785 0.451901
		-1.18313 0.477552
		-1.17786 0.508523
		-1.17628 0.512179
		-1.14883 0.534141
		-1.00156 0.515729
		-0.929561 0.520276
		-0.915356 0.533384
		-0.907844 0.546072
		-0.945032 0.592891
		-0.952518 0.626561
		-0.94601 0.65242
		-0.875637 0.624964
		-0.826755 0.657338
		-0.623887 1.04766
		-0.538433 0.996284
		-0.449292 0.982826
		-0.453025 0.969758
		-0.453025 0.969758
		-0.384827 1.10783
		-0.261647 0.963788
		-0.261647 0.963788
		-0.207164 1.05011
		-0.186711 1.05563
		-0.186711 1.05563
		-0.142173 1.11868
		-0.175132 1.20964
		-0.12663 1.10988
		-0.113849 1.17382
		-0.0596814000000001 1.18169
		-0.0955423 1.24205
		-0.0955423 1.24205
		0.00840368000000002 1.25215
		0.0371744000000001 1.23089
		0.0506762000000001 1.08592
		0.115015 1.31383
		0.115015 1.31383
		0.143123 1.25443
		0.127311 1.25613
		0.127311 1.25613
		0.305539 1.15867
		0.405468 1.18774
		0.484268 1.21067
		0.484268 1.21067
		0.44666 1.04721
		0.517837 1.00238
		0.545236 0.921879
		0.545236 0.921879
		0.574181 0.914301
		0.684307 0.979337
		0.652 0.839315
		0.539968 0.66702
		0.610779 0.729097
		0.622924 0.723501
		0.718703 0.753762
		0.762439 0.788473
		0.688898 0.675776
		0.770406 0.706205
		0.709225 0.621786
		0.693454 0.57942
		0.736512 0.580282
		0.778695 0.593133
		0.821003 0.602977
		0.862857 0.591673
		0.88319 0.591197
		0.893172 0.576005
		0.857731 0.524362
		1.11812 0.602063
		0.870475 0.480502
		0.831837 0.412591
		0.842276 0.394185
		0.904982 0.391441
		0.895531 0.346885
		0.872628 0.296624
		0.92036 0.274303
		0.89373 0.225192
		0.869877 0.16033
		0.842877 0.124628
		0.881983 0.0786264000000001
		0.88418 0.0479788000000001
		0.884942 0.0308701
		0.852041 0
		0.85117 -0.0331195
		0.892058 -0.0694208000000001
		0.895444 -0.109287
		0.69264 -0.114531
		0.676477 -0.158549
		0.629602 -0.176687
		0.504669 -0.209106
		0.603258 -0.27619
		0.68827 -0.335741
		0.686267 -0.355842
		0.555341 -0.307751
		0.604346 -0.359482
		0.746617 -0.464998
		0.713442 -0.462944
		0.657387 -0.427592
		0.58794 -0.410191
		0.629777 -0.475303
		0.598801 -0.469252
		0.631851 -0.511196
		0.593041 -0.532217
		0.515163 -0.501462
		0.0384770000000001 -0.930443
		0.0270691999999999 -0.893285
		0.0128902 -0.828192
		-0.0218780999999999 -0.806366
		-0.0669146 -0.747698
		-0.110229 -0.833199
		-0.137354 -0.802271
		-0.183707 -0.887342
		-0.219053 -0.883058
		-0.259301 -0.891994
		-0.308238 -0.954423
		-0.293068 -0.882653
		-0.362365 -0.958756
		-0.418371 -0.952957
		-0.475352 -0.970348
		-0.499773 -0.97178
		-0.519473 -0.971015
		-0.544528 -0.964935
		-0.570223 -0.913127
		-0.571908 -0.867208
		-0.550031 -0.794108
		-0.544774 -0.772041
		-0.543641 -0.734563
		-0.588826 -0.778214
		-0.5793 -0.739107
		-0.596484 -0.755772
		-0.591415 -0.704527
		-0.606634 -0.716628
		-0.614911 -0.706134
		-0.624614 -0.68673
		-0.658566 -0.72479
		-0.656009 -0.726033
		-0.66919 -0.718063
		-0.642393 -0.678483
		-0.618291 -0.652833
		-0.597885 -0.631101
		-0.627972 -0.667445
		-0.582917 -0.612725
		-0.555262 -0.558296
		-0.497562 -0.487032
		-0.506047 -0.500663
		-0.519561 -0.508447
		-0.507458 -0.493817
		-0.522316 -0.51673
		-0.478854 -0.503765
		-0.532813 -0.521416
		-0.498416 -0.520943
		-0.497566 -0.511701
		-0.459504 -0.483688
		-0.469206 -0.523236
		-0.46944 -0.513364
		-0.423468 -0.495833
		-0.387112 -0.47476
		-0.364887 -0.456109
		-0.43643 -0.519432
		-0.366496 -0.437064
		-0.377046 -0.453441
		-0.37126 -0.445994
		-0.363825 -0.461011
		-0.356852 -0.462399
		-0.298734 -0.490421
		-0.30431 -0.525136
		-0.241222 -0.452578
		-0.223003 -0.434856
		-0.165194 -0.444923
		-0.0637543 -0.386169
		0.198905 -0.203847
		0.212848 -0.261094
		0.194238 -0.231055
		0.24567 -0.247159
		0.297018 -0.289904
		0.216299 -0.204781
		0.24499 -0.242073
		0.343282 -0.32532
		0.344398 -0.324139
		0.268524 -0.216311
		0.24442 -0.159813
		0.297792 -0.186947
		0.274202 -0.160688
		0.318705 -0.175467
		0.238005 -0.119646
		0.279183 -0.111103
		0.274804 -0.0897026999999999
		0.304287 -0.0906385999999999
		0.348224 -0.0532995999999999
		0.281487 -0.0296301999999999
		0.243204 -0.0117678999999999
		0.320732 -0.0301864999999999
		0.26869 0.0876779000000001
		0.234059 0.0702178
		0.219572 0.0712748000000001
		0.25655 0.108021
		0.290119 0.185857
		0.279178 0.176475
		0.243641 0.16677
		0.254986 0.179033
		0.260853 0.201311
		0.273489 0.227653
		0.253279 0.227522
		0.233933 0.21433
		0.277547 0.261955
		0.277547 0.261955
		0.258212 0.297815
		0.202167 0.243605
		0.202167 0.243605
		0.202109 0.24107
		0.219954 0.263944
		0.178203 0.213207
		0.16154 0.203164
		0.158939 0.208862
		0.159518 0.222457
		0.159518 0.222457
		0.172489 0.299074
		0.163002 0.32013
		0.158285 0.322488
		0.137234 0.29917
		0.137234 0.29917
		0.121722 0.294048
		0.111904 0.284369
		0.0814722999999999 0.23464
		0.0721867999999999 0.237661
		0.0512868 0.192551
		0.0291395999999999 0.213021
		-0.169421 0.258837
		-0.144279 0.202475
		0.0491862999999999 0.18357
		0.0195708999999999 0.251975
		0.00789693000000002 0.276392
		-0.29618 0.210483
		-0.310561 0.196636
		-0.352857 0.20285
		-0.390597 0.228779
		-0.495474 -0.13128
		-0.528697 -0.158836
		-0.565728 -0.170922
		-0.486157 -0.153088
		-0.545205 -0.176322
		-0.489027 -0.187106
		-0.479843 -0.209538
		-0.488177 -0.243013
		-0.469034 -0.241686
		-0.476757 -0.257034
		-0.474702 -0.258928
		-0.497124 -0.284381
		-0.616212 -0.365876
		-0.670168 -0.431478
		-0.656104 -0.415923
		-0.665771 -0.442843
		-0.666207 -0.440063
		-0.698822 -0.464813
		-0.721468 -0.496423
		-0.736174 -0.489673
		-0.76109 -0.513212
		-0.785286 -0.528283
		-0.777441 -0.533607
		-0.768425 -0.526129
		-0.82941 -0.576496
		-0.826442 -0.580743
		-0.835946 -0.593863
		-0.860902 -0.605679
		-0.888776 -0.638196
		-0.949519 -0.691317
		-0.956596 -0.706865
		-0.9471 -0.697863
		-0.85146 -0.649799
		-0.924134 -0.716509
		-0.915463 -0.733983
		-0.917632 -0.763303
		-0.848418 -0.693127
		-0.853976 -0.718116
		-0.837931 -0.708433
		-0.905664 -0.777465
		-0.842166 -0.721857
		-0.862106 -0.742369
		-0.84143 -0.729497
		-0.902474 -0.798021
		-0.832221 -0.732047
		-0.864082 -0.774834
		-0.846191 -0.774004
		-0.803727 -0.761827
		-0.790737 -0.76047
		-0.783501 -0.787304
		-0.758742 -0.780949
		-0.720778 -0.760223
		-0.711862 -0.754362
		-0.696489 -0.752771
		-0.6618 -0.792048
		-0.594194 -0.74194
		-0.628368 -0.846154
		-0.620671 -0.870408
		-0.588308 -0.914313
		-0.589666 -0.960649
		-0.565938 -0.988399
		-0.492553 -0.947217
		-0.459964 -0.961743
		-0.389496 -0.987236
		-0.337915 -0.990704
		-0.326706 -1.01512
		-0.302789 -1.02482
		-0.271439 -1.02759
		-0.225268 -1.01943
		-0.213122 -1.01613
		-0.159757 -1.05839
		-0.111101 -1.05943
		-0.0643052 -0.910426
		-0.0456829000000001 -0.945286
		0.042859 -1.02862
		0.060918 -0.840027
		0.162413 -1.02993
		0.134342 -0.849792
		0.181848 -0.90587
		0.168318 -0.800251
		0.187475 -0.857935
		0.222371 -0.8637
		0.279308 -0.945349
		0.253773 -0.832499
		0.277129 -0.857168
		0.335317 -0.887405
		0.38961 -0.870694
		0.466857 -0.933714
		0.448408 -0.849258
		0.513775 -0.879207
		0.544699 -0.898017
		0.551025 -0.855926
		0.553934 -0.8238
		0.638916 -0.862152
		0.708148 -0.776312
		0.680978 -0.712089
		0.69383 -0.718114
		0.729638 -0.686293
		0.70965 -0.713216
		0.684032 -0.625401
		0.713017 -0.592507
		0.695462 -0.566074
		0.687481 -0.53789
		0.787672 -0.5681
		0.751791 -0.532241
		1.02372 -0.665419
		1.02411 -0.644955
		0.918209 -0.547902
		0.916545 -0.550681
		0.81845 -0.444302
		0.85219 -0.443416
		0.746111 -0.353734
		0.78818 -0.336908
		0.701637 -0.279029
		0.798034 -0.263965
		0.782147 -0.219238
		0.797329 -0.180527
		0.892472 -0.106564
		0.912569 -0.0508868
		0.943514 -0.0698898999999999
		0.912742 -0.0476806000000001
		0.913586 -0.0270693
		0.89535 0.00670671999999994
		0.936963 0.0594342000000001
		0.929959 0.128871
		0.918916 0.161757
		1.00763 0.196981
		1.02089 0.242701
		1.00657 0.330402
		0.918804 0.355552
		0.996914 0.427249
		0.944505 0.417339
		1.00757 0.493905
		0.927865 0.519604
		1.02685 0.627748
		1.07032 0.712051
		1.11231 0.765008
		1.12629 0.78601
		0.995779 0.73825
		1.099 0.857407
		0.826253 0.737328
		0.810062 0.75508
		0.822306 0.788201
		0.767814 0.767814
		0.561875 0.610499
		0.595331 0.657699
		0.672807 0.759725
		0.686165 0.792754
		0.991659 1.22321
		0.944154 1.19723
		0.753677 0.999613
		0.921277 1.29284
		0.930037 1.41128
		0.707438 1.16749
		0.840496 1.38708
		0.682493 1.1847
		0.810361 1.4493
		0.72087 1.3749
		0.719189 1.4236
		0.710422 1.42574
		0.77552 1.71189
		0.760804 1.66146
		0.702614 1.57302
		0.705617 1.68564
		0.616183 1.53541
		0.624535 1.61956
		0.670446 1.79962
		0.620131 1.82496
		0.614791 1.87451
		0.590096 1.847
		0.577099 1.86813
		0.101808 1.56106
		0.443404 1.90368
		0.481232 1.92493
		0.427313 1.95601
		0.420823 1.9263
		0.434364 2.0648
		0.434364 2.0648
		0.454278 2.05358
		0.0893492 1.51894
		0.204751 1.86489
		-0.164023 2.25846
		-0.164023 2.25846
		-0.104802 2.21317
		-0.136936 1.98283
		-0.136936 1.98283
		-0.126954 2.30422
		-0.127655 2.30418
		-0.755189 2.83597
		-0.815065 2.886
		-0.935852 3.20997
		-0.83662 2.81851
		-0.870113 2.87807
		-0.968082 3.07456
		-0.953452 2.90254
		-0.998175 3.04753
		-1.03434 3.03288
		-1.11628 3.02361
		-1.05615 2.84664
		-1.37713 3.30121
		-1.39372 3.29425
		-1.7677 4.08024
		-1.43304 3.26576
		-1.47261 3.23396
		-1.52549 3.1958
		-1.54544 3.22783
		-1.54465 3.12743
		-2.00904 3.88653
		-1.80382 3.12727
		-2.34481 3.82702
		-3.08746 3.23106
		-3.12482 3.19638
		-3.25862 3.03266
		-3.33921 3.08421
		-3.40598 2.90405
		-3.40354 2.87992
		-3.39162 2.79516
		-3.40829 2.76411
		-3.42408 2.72529
		-3.43345 2.74207
		-3.38526 2.69203
		-3.37578 2.67537
		-3.44246 2.68395
		-3.47773 2.68787
		-3.4535 2.62791
		-3.4746 2.55657
		-3.47921 2.50503
		-3.60901 2.54542
		-3.63606 2.51175
		-3.64725 2.49548
		-3.72278 2.46981
		-3.7241 2.45863
		-3.65277 2.35323
		-3.68566 2.33582
		-3.69627 2.319
		-3.69362 2.27929
		-3.64113 2.22132
		-3.67874 2.19799
		-3.80284 2.17475
		-3.81375 2.14524
		-3.83773 2.09222
		-3.80728 2.03919
		-3.73125 1.94574
		-3.72875 1.94395
		-3.74436 1.90046
		-3.78423 1.84098
		-3.79113 1.79341
		-3.81808 1.78329
		-3.88383 1.77381
		-3.68719 1.58023
		-3.78425 1.52046
		-3.86904 1.50653
		-3.788 1.47064
		-3.75465 1.40115
		-3.86148 1.40315
		-3.86465 1.38502
		-3.88985 1.36427
		-3.90254 1.33092
		-3.91951 1.28007
		-3.98227 1.28534
		-3.94414 1.22054
		-3.83116 1.12746
		-3.83705 1.10726
		-3.84751 1.06327
		-3.84856 1.03067
		-3.9253 1.01767
		-3.86928 0.981099
		-3.85585 0.963964
		-3.86241 0.919101
		-3.89875 0.872525
		-3.95217 0.870816
		-3.9468 0.809315
		-3.95491 0.7687
		-3.96759 0.724419
		-3.91644 0.693078
		-4.02732 0.67686
		-3.99561 0.534232
		-4.04958 0.416207
		-4.04919 0.314937
		-4.05752 0.268266
		-4.07647 -0.0675656
		-4.24039 -0.117138
		-4.24333 -0.140663
		-3.63784 -1.4486
		-3.63032 -1.46735
		-3.84667 -1.58256
		-3.63185 -1.52056
		-3.63185 -1.52056
		-3.84516 -1.69328
		-3.9728 -1.77379
		-4.00891 -1.87995
		-3.89147 -1.84905
		-3.71753 -1.86459
		-3.71753 -1.86459
		-3.57411 -1.87754
		-3.413 -1.86954
		-3.413 -1.86954
		-3.60353 -2.02627
		-3.46489 -2.02768
		-3.59523 -2.20616
		-3.53453 -2.1875
		-3.53453 -2.1875
		-3.32055 -2.19513
		-3.28285 -2.21453
		-3.27286 -2.23403
		-3.47241 -2.42234
		-3.20979 -2.34259
		-3.20979 -2.34259
		-3.39222 -2.54417
		-3.27064 -2.49358
		-3.27064 -2.49358
		-3.094 -2.49986
		-3.1196 -2.56374
		-3.1196 -2.56374
		-3.11497 -2.60339
		-2.98065 -2.48934
		-2.98065 -2.48934
		-3.06838 -2.73132
		-3.06838 -2.73132
		-3.07533 -2.90648
		-3.07533 -2.90648
		-2.9438 -2.87371
		-2.91591 -2.95133
		-2.97736 -3.06277
		-2.84127 -3.04253
		-2.71547 -3.14235
		-2.44072 -2.96845
		-2.39318 -3.0218
		-2.39318 -3.0218
		-2.4541 -3.19149
		-2.39122 -3.2345
		-2.43039 -3.36698
		-2.38112 -3.33122
		-2.35198 -3.43197
		-2.27795 -3.39345
		-2.22257 -3.29948
		-2.19061 -3.29733
		-1.92756 -3.04679
		-1.99642 -3.27192
		-1.8887 -3.1726
		-1.74069 -3.04622
		-1.70902 -3.0641
		-1.68195 -3.0802
		-1.47694 -2.84241
		-1.40781 -2.8434
		-1.39067 -2.89335
		-1.37506 -2.90081
		-1.34047 -2.91695
		-1.30555 -2.93275
		-1.24943 -2.94977
		-1.21049 -2.93311
		-1.13099 -2.96301
		-1.09168 -2.98578
		-1.0722 -2.99283
		-1.02203 -3.01033
		-1.02203 -3.01033
		-1.01778 -3.05334
		-0.923396 -3.01027
		-0.878407 -3.01432
		-0.792151 -3.03813
		-0.74954 -3.08248
		-0.666219 -2.92248
		-0.667989 -3.09533
		-0.638218 -3.0431
		-0.609785 -3.04892
		-0.633595 -3.28677
		-0.595288 -3.29393
		-0.509816 -3.14386
		-0.445113 -3.15367
		-0.402479 -3.26892
		-0.358158 -3.49731
		-0.310811 -3.32868
		-0.271773 -3.3418
		-0.258603 -3.30216
		-0.208733 -3.29996
		-0.167144 -3.45779
		-0.115278 -3.46882
		-0.0629796 -3.48488
		-0.0208671 -3.47438
		0.0216154 -3.58817
		1.98782 -2.17713
		2.16688 -2.16688
		2.05961 -1.99344
		2.12668 -2.02419
		2.17359 -2.04318
		2.53671 -2.29607
		2.14818 -1.93
		2.54886 -2.21554
		2.40599 -2.05967
		2.10753 -1.81327
		2.11539 -1.73509
		2.17206 -1.59233
		3.02877 -1.97297
		2.32616 -1.49134
		2.22966 -1.42027
		2.74131 0.0415350999999999
		2.64859 0.0960216
		2.43456 0.132794
		2.61931 0.198433
		2.42745 0.213321
		2.57309 0.273733
		2.59422 0.301468
		2.63105 0.313795
		2.53726 0.349165
		2.57827 0.369448
		2.56629 0.406851
		2.54539 0.419059
		2.60422 0.484321
		2.50818 0.492404
		2.60658 0.575687
		2.59174 0.622017
		2.47659 0.64208
		2.5756 0.685764
		2.5449 0.699063
		2.69944 0.762886
		2.69131 0.788108
		2.65466 0.804692
		2.83121 0.905279
		2.79819 0.976728
		2.88415 1.05874
		2.86881 1.10199
		2.89276 1.16629
		2.57227 1.21194
		2.64438 1.27133
		2.53879 1.30237
		2.45762 1.2973
		2.47325 1.3349
		2.62185 1.47315
		2.43802 1.37695
		2.67697 1.6098
		2.66129 1.61835
		2.56541 1.60556
		2.47928 1.55695
		2.47928 1.55695
		2.66251 1.72926
		2.66942 1.77044
		2.66942 1.77044
		2.66581 1.8201
		2.6159 1.83113
		2.6159 1.83113
		2.61627 1.91434
		2.54898 1.90728
		2.53996 1.98463
		2.55204 2.02499
		2.60539 2.12045
		2.50477 2.07961
		2.34915 2.13397
		2.31843 2.1857
		2.31424 2.21633
		2.21586 2.24203
		2.21586 2.24203
		2.15187 2.2031
		2.12647 2.2572
		2.12647 2.2572
		1.96744 2.26814
		1.87784 2.22837
		1.93485 2.43164
		2.13041 2.72808
		2.21223 2.93273
		2.21223 2.93273
		1.75874 2.58235
		1.83095 2.71485
		1.41873 2.59564
		1.41326 2.54706
		1.43863 2.63885
		1.28759 2.43965
		1.28977 2.4727
		1.51826 2.9542
		1.39466 2.70581
		1.51686 3.00596
		1.41602 2.90329
		1.3488 2.83594
		1.302 2.81815
		1.22392 2.87832
		1.3593 3.08169
		1.32426 3.05037
		1.37295 3.20355
		1.18397 2.84319
		1.12909 2.92537
		1.03407 2.90043
		1.10234 2.95394
		0.951635 2.89664
		1.10736 4.23334
		-0.968787 3.2976
		-0.978725 3.31261
		-0.995996 3.30746
		-1.65077 4.14501
		-1.38936 3.30338
		-2.0243 3.98835
		-2.00175 3.92059
		-2.04079 3.89174
		-2.083 3.87011
		-2.22399 3.86209
		-3.33921 3.08421
		-3.34036 3.06199
		-3.36392 3.03603
		-3.34817 2.98686
		-3.36701 2.92524
		-3.40575 2.9158
		-3.40839 2.87397
		-3.39777 2.80992
		-3.40504 2.88118
		-3.41263 2.74646
		-3.41438 2.69188
		-3.46483 2.68701
		-3.41108 2.65693
		-3.50567 2.48076
		-3.49571 2.48196
		-3.44686 2.40823
		-3.58181 2.43893
		-3.47558 2.36659
		-3.51725 2.32574
		-3.53463 2.29923
		-3.6707 2.32517
		-3.56765 2.30916
		-3.55552 2.26679
		-3.5282 2.21935
		-3.56249 2.19495
		-3.59094 2.19382
		-3.59661 2.18572
		-3.62872 2.16796
		-3.61923 2.16229
		-3.70267 2.18151
		-3.6089 2.11951
		-3.5919 2.03315
		-3.68541 2.06153
		-3.6023 1.95777
		-3.55929 1.91229
		-3.59369 1.86339
		-3.55929 1.91229
		-3.58403 1.83626
		-3.4868 1.7434
		-3.54266 1.71138
		-3.74926 1.73131
		-3.65948 1.67866
		-3.56402 1.57204
		-3.53334 1.51125
		-3.5367 1.4295
		-3.57408 1.39347
		-3.67403 1.35874
		-3.75771 1.25994
		-3.7196 1.32374
		-3.80236 1.26002
		-3.80236 1.26002
		-3.74231 1.1599
		-3.81617 1.17163
		-3.69382 1.03555
		-3.69382 1.03555
		-3.68877 0.93548
		-3.67499 0.887066
		-3.72561 0.819635
		-3.87698 0.693891
		-3.8717 0.623409
		-3.87515 0.660537
		-3.86551 0.567814
		-3.89321 0.515439
		-3.87923 0.457662
		-3.87923 0.457662
		-3.98134 0.412632
		-3.9284 0.373088
		-4.06745 0.319015
		-4.06745 0.319015
		-4.06973 0.284995
		-4.06909 0.193766
		-4.06909 0.193766
		-3.96772 0.155162
		-4.09246 0.0687808999999999
		-3.99638 0.0333958000000001
		-3.98824 -0.0668418
		-3.98725 -0.111376
		-3.98017 -0.144531
		-4.1859 -0.186558
		-4.15748 -0.31268
		-4.15751 -0.347424
		-4.19738 -0.386909
		-4.24569 -0.463815
		-4.1153 -0.531752
		-4.10929 -0.567198
		-4.10896 -0.578727
		-4.1057 -0.601399
		-3.90602 -0.931607
		-3.83459 -0.947629
		-4.11881 -1.08641
		-3.95128 -1.03376
		-3.83267 -0.996938
		-4.05252 -1.12242
		-4.04947 -1.13338
		-3.84686 -1.12481
		-3.83948 -1.17443
		-3.80525 -1.19336
		-3.7086 -1.21413
		-3.63032 -1.22456
		-3.62372 -1.24396
		-3.20516 -1.47318
		-3.24496 -1.52107
		-3.23734 -1.53723
		-3.21969 -1.57384
		-3.27699 -1.62799
		-3.21868 -1.59902
		-3.23593 -1.66479
		-3.29728 -1.78289
		-3.07086 -1.69048
		-2.98178 -1.56327
		-3.19473 -1.74826
		-3.15812 -1.80315
		-3.15812 -1.80315
		-2.91752 -1.68654
		-3.04402 -1.77738
		-2.97572 -1.81175
		-2.98938 -1.81607
		-2.96239 -1.80187
		-2.91862 -1.7713
		-2.89546 -1.7872
		-2.79449 -1.73451
		-2.69339 -1.67755
		-2.54599 -1.60893
		-2.67379 -1.69897
		-2.43884 -1.54968
		-2.26094 -1.43878
		-2.20013 -1.43319
		-2.25777 -1.43176
		-2.17844 -1.39879
		-2.20013 -1.43319
		-2.15783 -1.43082
		-2.05002 -1.36915
		-2.14303 -1.439
		-2.12838 -1.42151
		-2.13669 -1.41663
		-1.9465 -1.27604
		-1.95267 -1.30418
		-1.89348 -1.28109
		-1.90914 -1.26806
		-1.84513 -1.24615
		-1.74827 -1.19378
		-1.86965 -1.26969
		-1.81342 -1.23395
		-1.59549 -1.05184
		-1.44957 -0.953809
		-1.49133 -0.986747
		-1.47722 -0.960752
		-1.39328 -0.881891
		-1.42544 -0.887537
		-1.39257 -0.865083
		-1.36349 -0.821192
		-1.29249 -0.784205
		-1.32158 -0.789966
		-1.37526 -0.812654
		-1.38553 -0.829219
		-1.24581 -0.726722
		-1.16686 -0.677389
		-1.21405 -0.707437
		-1.21196 -0.69059
		-1.2097 -0.694544
		-1.11729 -0.641487
		-1.07621 -0.588872
		-1.07397 -0.587643
		-1.12708 -0.632368
		-1.07926 -0.582717
		-0.985021 -0.494355
		-0.967365 -0.480073
		-0.937824 -0.436036
		-0.895819 -0.416273
		-0.962723 -0.438574
		-0.861515 -0.382896
		-0.941282 -0.430697
		-0.825382 -0.365132
		-0.798746 -0.34741
		-0.816608 -0.347815
		-0.756885 -0.321958
		-0.762899 -0.307437
		-0.796579 -0.313894
		-0.756486 -0.278705
		-0.767572 -0.253912
		-0.662044 -0.206417
		-0.73949 -0.219003
		-0.773989 -0.220708
		-0.73909 -0.193434
		-0.68152 -0.163672
		-0.68133 -0.130922
		-0.692107 -0.119422
		-0.574355 -0.0960984
		-0.616164 -0.0890549
		-0.598278 -0.0703856
		-0.459359 -0.0468366
		-0.543316 -0.0231646000000001
		-0.559379 -0.0194379
		-0.551759 0.00636642999999992
	};
\addlegendentry{Prediction}
\addplot [draw=red, mark=o, only marks]
table{%
		x  y
		0.184939384460449 0.12700080871582
		-0.0627899169921875 1.80849003791809
		-0.183470249176025 1.79386591911316
		-0.463483810424805 1.79745864868164
		-0.494549512863159 1.79780626296997
		-0.626050472259521 1.80703806877136
		-0.662168979644775 1.81105661392212
		-0.699923038482666 1.81586599349976
		-0.739159822463989 1.82159113883972
		-0.779354810714722 1.82824754714966
		-0.820664882659912 1.83132147789001
		-0.973613500595093 1.84009528160095
		-1.00958442687988 1.83504176139832
		-1.04426550865173 1.82822871208191
		-0.508740186691284 2.3828272819519
		-0.560027122497559 2.39761567115784
		-0.689199924468994 2.41824746131897
		-0.715248107910156 2.4197781085968
		-0.846947431564331 2.42204546928406
		-0.896482944488525 2.42104935646057
		-0.950192928314209 2.42056250572205
		-1.00260257720947 2.41984128952026
		-1.02643632888794 2.41978216171265
		-1.12351655960083 2.42802119255066
		-1.40737295150757 2.46467804908752
		-1.49188923835754 2.46808958053589
		-1.74180388450623 2.42492341995239
		-1.8384382724762 2.38188743591309
		-1.8895218372345 2.35580134391785
		-1.98903322219849 2.30367112159729
		-1.09747457504272 2.42664790153503
		2.56631278991699 4.1558985710144
		0.18583345413208 4.45130634307861
		-0.0865716934204102 4.47834205627441
		-0.311665534973145 4.46138525009155
		-0.554606199264526 4.39847445487976
		-0.765497922897339 4.37149381637573
		-0.857213497161865 4.37468767166138
		-0.889987707138062 4.37776327133179
		-1.00627899169922 4.38773107528687
		-1.0368115901947 4.39288449287415
		-1.10242700576782 4.40288329124451
		-1.16588640213013 4.40788054466248
		-1.19683957099915 4.41242647171021
		-2.86640787124634 4.37948274612427
		-0.639804124832153 4.37901663780212
		0.354012966156006 2.64316558837891
		0.317865371704102 2.71190762519836
		0.297689437866211 2.74566125869751
		0.276980876922607 2.77915549278259
		0.229832172393799 2.8410313129425
		0.183249473571777 2.89228129386902
		0.160796642303467 2.91698670387268
		0.112030029296875 2.96534752845764
		0.0869851112365723 2.98773813247681
		0.06268310546875 3.00949621200562
		0.0382905006408691 3.03404140472412
		-0.0119738578796387 3.0767924785614
		-0.0374188423156738 3.09959626197815
		-0.0892634391784668 3.14571952819824
		-0.139242172241211 3.187175989151
		-0.190523624420166 3.22986578941345
		-0.454052686691284 3.43485164642334
		-0.50995659828186 3.48652768135071
		-0.539922475814819 3.51195359230042
		-0.596237897872925 3.55991649627686
		-0.626880884170532 3.58152556419373
		-0.655164957046509 3.60334014892578
		-0.68376898765564 3.62514781951904
		-0.710470914840698 3.65037393569946
		-0.739860773086548 3.67483520507812
		-0.769970655441284 3.70003342628479
		-0.800036668777466 3.72414422035217
		-0.916602373123169 3.80544781684875
		-0.947345018386841 3.82199859619141
		-0.97872519493103 3.83761501312256
		-1.01283025741577 3.85481142997742
		-1.05009126663208 3.87340903282166
		-1.08535575866699 3.88796377182007
		-1.62772011756897 4.18571972846985
		-1.73451495170593 4.22722697257996
		-1.8450722694397 4.25348663330078
		-1.99174833297729 4.26517033576965
		0.254448413848877 2.81006598472595
		-0.86103343963623 3.76689314842224
		1.77359580993652 4.12709999084473
		1.34663152694702 4.32845544815063
		1.18518829345703 4.36729264259338
		1.14184522628784 4.37447237968445
		1.09787511825562 4.37843489646912
		1.05463838577271 4.3830943107605
		0.969603538513184 4.38871192932129
		0.490447998046875 4.40941786766052
		0.271459102630615 4.4372661113739
		-2.14896845817566 4.63966631889343
		-0.717251062393188 -0.0104899406433105
		-0.434075117111206 0.328056335449219
		0.230428218841553 4.44654536247253
		0.151107788085938 4.46484613418579
		-0.0953121185302734 4.51950764656067
		-0.265668392181396 4.50009298324585
		-0.734986305236816 4.49398684501648
		-1.06163692474365 4.54810667037964
		-1.21538329124451 4.59085321426392
		-1.44999408721924 4.64009356498718
		-1.99154210090637 4.6330406665802
		-2.02605605125427 4.62743759155273
		-2.10776591300964 4.63451051712036
		-2.23209142684937 4.6476993560791
		-2.30953311920166 4.65967440605164
		-2.5863344669342 4.70303344726562
	};
\addlegendentry{FN}


==> tikz/vis_localize/vis_loc_test2_x_clean.tex <==
\addplot [semithick, steelblue31119180]
table {%
		0.0398528575897217 -0.277914524078369
		0.839867830276489 -0.238692760467529
		1.19991421699524 -0.319681644439697
		1.42984771728516 -0.312024831771851
		1.84002876281738 -0.300677299499512
		2.13989067077637 -0.268847465515137
		2.39991331100464 -0.257651805877686
		2.66988110542297 -0.2236008644104
		2.86992263793945 -0.196717262268066
		3.36989831924438 -0.269469738006592
		4.4698543548584 -0.661723136901855
		4.72988510131836 -0.607984781265259
		5.42986917495728 -0.363263130187988
		6.26987266540527 -0.0798959732055664
		6.5698881149292 -0.119813442230225
		6.92984008789062 -0.180478096008301
		7.06984233856201 -0.147720813751221
		7.39991807937622 0.0164546966552734
		8.12986946105957 0.120658874511719
		8.42985820770264 0.169551849365234
		8.69986152648926 0.179197788238525
		8.96987915039062 0.171702861785889
		9.46986865997314 0.208274841308594
		9.69987869262695 0.172471523284912
		10.1698579788208 0.0205011367797852
		10.7699213027954 -0.36329197883606
		11.0998582839966 -0.636612415313721
		11.3999090194702 -0.792516469955444
		11.699878692627 -0.844769716262817
		11.8998603820801 -0.860949993133545
		12.3999013900757 -1.01456260681152
		12.6998586654663 -1.16647338867188
		13.3698902130127 -1.39093732833862
		13.5698432922363 -1.34038138389587
		13.8998680114746 -1.21230983734131
		14.1299076080322 -1.21091437339783
		14.3998708724976 -1.2807469367981
		14.7698440551758 -1.33137106895447
		14.9999027252197 -1.25989508628845
		15.9299030303955 -0.858505487442017
		16.1999263763428 -0.643152952194214
		16.6698665618896 -0.18022632598877
		16.929838180542 0.154507637023926
		17.1999416351318 0.386484622955322
		17.3698291778564 0.522701740264893
		17.6298694610596 0.745688438415527
		17.8698768615723 0.97785472869873
		18.0698566436768 1.12275218963623
		18.2298603057861 1.16582870483398
		18.6298713684082 1.22750473022461
		18.8999443054199 1.31554365158081
		19.3698291778564 1.50235223770142
		19.4999179840088 1.48128795623779
		20.0698585510254 1.21517705917358
		20.2998943328857 1.08483028411865
		20.3699607849121 1.05749034881592
		21.7698745727539 0.229444980621338
		22.2998847961426 -0.347094058990479
		22.4998569488525 -0.525775194168091
		23.1998767852783 -1.22786855697632
		23.2998523712158 -1.26655101776123
		24.4299068450928 -1.43966126441956
		24.9298515319824 -1.55964779853821
		25.1999034881592 -1.51535797119141
		25.7999858856201 -1.36103081703186
		26.0398941040039 -1.23346662521362
		26.4998836517334 -0.850311279296875
		27.4298725128174 0.113173484802246
		27.569881439209 0.257551193237305
		27.8698921203613 0.597454071044922
		28.0698757171631 0.794093132019043
		28.239917755127 0.90026330947876
		28.569845199585 1.03311967849731
		28.8698654174805 1.09518194198608
		29.2298393249512 1.12469577789307
		29.4698600769043 1.05993318557739
		29.7698764801025 0.911039352416992
		29.9298686981201 0.819808006286621
		32.5698547363281 -1.18130660057068
		33.1298789978027 -1.64481210708618
		33.499870300293 -1.91582250595093
		34.5998954772949 -2.78511047363281
		35.9299430847168 -3.41281032562256
		36.2998809814453 -3.43456959724426
		37.1698570251465 -3.43409538269043
		37.6998443603516 -3.2081446647644
		38.0998802185059 -3.0218677520752
		38.3998565673828 -2.83277606964111
		38.6698226928711 -2.66274309158325
		39.5299301147461 -1.95189118385315
		39.7998809814453 -1.69067859649658
		40.1998710632324 -1.30498933792114
		40.3998641967773 -1.10799789428711
		40.7698745727539 -0.729492425918579
		41.3298721313477 -0.181426048278809
		41.5698547363281 0.0607204437255859
		41.829891204834 0.342928886413574
		48.569881439209 2.84257936477661
		49.6298828125 2.7872462272644
		49.8698844909668 2.78791618347168
		50.469841003418 2.73240756988525
		50.8298873901367 2.7822208404541
		51.0698890686035 2.81193351745605
		51.2998847961426 2.7967267036438
		58.9699172973633 -1.28284668922424
		58.9699211120605 -1.34642362594604
		59.3699111938477 -1.70495676994324
		59.6298904418945 -1.96089243888855
		60.2699203491211 -2.55515575408936
		60.6298828125 -2.89601135253906
		62.5998764038086 -4.22010040283203
		63.5698471069336 -4.3484992980957
		63.7998390197754 -4.40035820007324
		64.1698913574219 -4.38666725158691
		64.5998992919922 -4.39477109909058
		65.4298629760742 -4.43903493881226
		65.6699142456055 -4.44406414031982
		66.4998626708984 -4.6234974861145
		66.6998901367188 -4.61475992202759
		67.0298385620117 -4.6680383682251
		68.9298706054688 -3.90352416038513
		69.769889831543 -3.24423289299011
		70.2298202514648 -2.83690214157104
		71.0998764038086 -2.23432993888855
		71.2998962402344 -2.08376955986023
		72.1298904418945 -1.61738014221191
		72.3698577880859 -1.42418718338013
		72.5698699951172 -1.2826931476593
		72.7998886108398 -1.11612725257874
		74.1398849487305 0.239355087280273
		74.3698577880859 0.498700618743896
		74.5698547363281 0.649874687194824
		74.9298553466797 0.865520477294922
		75.5399322509766 1.1002516746521
		75.6998977661133 1.080810546875
		76.4299163818359 0.827256679534912
		76.5999069213867 0.716102600097656
		77.2698669433594 0.207769870758057
		77.5698623657227 0.0446157455444336
		78.2298736572266 -0.205463886260986
		78.7298736572266 -0.495018005371094
		79.0698928833008 -0.608514070510864
		79.3698806762695 -0.760092258453369
		79.5998992919922 -0.786429166793823
		79.7698745727539 -0.716881275177002
		80.3298568725586 -0.297281265258789
		80.4998779296875 -0.208854675292969
		80.7699203491211 0.00168323516845703
		80.9998779296875 0.217358112335205
		81.2298889160156 0.301782131195068
		81.3998870849609 0.255562305450439
		81.5299377441406 0.161356925964355
		81.7998580932617 -0.0770149230957031
		82.0698928833008 -0.306378841400146
		82.3998870849609 -0.59633469581604
		83.569938659668 -1.22509479522705
		83.8298873901367 -1.19568467140198
		84.6698532104492 -1.10163068771362
		84.8298721313477 -1.00886678695679
		85.7299270629883 -0.602487325668335
		85.9999008178711 -0.361660480499268
		86.3298492431641 -0.0858893394470215
		86.5698547363281 0.0805072784423828
		86.8698120117188 0.332046508789062
		87.2698669433594 0.599546909332275
		87.6999053955078 0.758265495300293
		87.969856262207 0.798248767852783
		88.3000335693359 0.821138381958008
		88.6999206542969 0.82374906539917
		88.8999404907227 0.780709743499756
		89.4699020385742 0.542894840240479
		91.0298690795898 -0.331355094909668
		91.3999099731445 -0.458576679229736
		91.6998672485352 -0.432770490646362
		92.0698471069336 -0.323894023895264
		92.7698669433594 -0.147972106933594
		93.0698623657227 0.00453662872314453
		94.1698913574219 0.151484966278076
		94.8699111938477 0.078188419342041
		95.5998611450195 0.0576715469360352
		95.8298797607422 0.0376901626586914
		96.2999267578125 0.0678491592407227
		96.4998397827148 -0.000557422637939453
		96.9298629760742 -0.224315166473389
		97.2298736572266 -0.307756423950195
		98.4698791503906 -0.469410419464111
		99.0299453735352 -0.735092163085938
		99.2999114990234 -0.760072231292725
		100.029846191406 -0.712883949279785
		100.229866027832 -0.605996131896973
		100.369842529297 -0.495512723922729
		100.629875183105 -0.26790189743042
		101.09992980957 0.084205150604248
		101.699913024902 0.66591215133667
		101.969841003418 0.804858207702637
		102.999839782715 1.04342985153198
		103.36988067627 0.945866584777832
		103.729858398438 0.882192611694336
		103.969856262207 0.826606750488281
		104.499839782715 0.54963493347168
		104.969917297363 0.369021415710449
		105.999961853027 -0.392948150634766
		106.029861450195 -0.424643754959106
		107.399887084961 -1.6999146938324
		109.499870300293 -3.96339321136475
		109.899848937988 -4.27905225753784
		110.26993560791 -4.40322017669678
		110.729866027832 -4.53639650344849
		110.96989440918 -4.56291770935059
		111.429840087891 -4.51891660690308
		111.829849243164 -4.52925825119019
		112.299873352051 -4.53871583938599
		112.799850463867 -4.51694488525391
		113.099876403809 -4.55127954483032
		114.629898071289 -3.97245144844055
		115.399978637695 -3.37850141525269
		115.86986541748 -2.92559409141541
		116.299957275391 -2.46035313606262
		116.829895019531 -1.85325789451599
		118.499870300293 0.227507591247559
		120.529922485352 2.37491416931152
		121.299942016602 2.75717735290527
		121.399887084961 2.76860809326172
		123.799880981445 2.90527486801147
		124.129867553711 2.86707782745361
		124.59986114502 2.85384035110474
		124.929893493652 2.76361751556396
		125.369873046875 2.58808517456055
		125.799835205078 2.4171986579895
		126.169868469238 2.12908363342285
		126.899871826172 1.38656425476074
		130.299835205078 -2.82245063781738
		132.029846191406 -4.24607944488525
		132.599884033203 -4.31510066986084
		132.969833374023 -4.1837329864502
		133.229843139648 -4.08049774169922
		133.669876098633 -4.02222681045532
		134.329879760742 -3.99072098731995
		134.529861450195 -4.04721164703369
		135.169891357422 -4.22251844406128
		135.729888916016 -4.31932592391968
		135.96989440918 -4.32736158370972
		136.469863891602 -4.01493978500366
		136.729873657227 -3.77352094650269
		138.599884033203 -1.89038801193237
		138.899887084961 -1.67590165138245
		139.19987487793 -1.46547436714172
		139.569915771484 -1.21496295928955
		139.92985534668 -1.00359606742859
		140.269882202148 -0.815368413925171
		140.699890136719 -0.561110258102417
	};
\addlegendentry{MOCAP}
\addplot [semithick, darkorange25512714]
table {%
		0.0398528575897217 -0.381783008575439
		0.199919939041138 -0.369610071182251
		0.439872980117798 -0.389165043830872
		0.499995708465576 -0.28597092628479
		0.669878721237183 -0.263875007629395
		0.79987621307373 -0.277912020683289
		0.839867830276489 -0.278005957603455
		0.89989972114563 -0.319488048553467
		0.929943561553955 -0.273895025253296
		0.999878406524658 -0.32088303565979
		1.12990427017212 -0.338290929794312
		1.16989326477051 -0.232370018959045
		1.22988653182983 -0.413128018379211
		1.26990294456482 -0.416010022163391
		1.32991504669189 -0.340085983276367
		1.39990663528442 -0.50299596786499
		1.42984771728516 -0.451990008354187
		1.49988293647766 -0.613496065139771
		1.59985733032227 -0.403727054595947
		1.66986751556396 -0.462491989135742
		1.69989371299744 -0.344972014427185
		1.76989197731018 -0.442914962768555
		1.79995822906494 -0.344927072525024
		1.86993885040283 -0.522387027740479
		1.9698657989502 -0.449418067932129
		2.02984404563904 -0.573225021362305
		2.06986856460571 -0.573050975799561
		2.09987688064575 -0.398005962371826
		2.13989067077637 -0.460819959640503
		2.19983887672424 -0.34703803062439
		2.39991331100464 -0.343124032020569
		2.42983722686768 -0.516036987304688
		2.49990057945251 -0.345245957374573
		2.54003667831421 -0.404458999633789
		2.59984469413757 -0.342438936233521
		2.69993734359741 -0.330846071243286
		2.72984004020691 -0.37815797328949
		2.96990513801575 -0.332152009010315
		3.02985453605652 -0.373544931411743
		3.22992253303528 -0.371798038482666
		3.59989380836487 -0.383156061172485
		3.62987089157104 -0.414541006088257
		3.66988158226013 -0.387448072433472
		4.36988496780396 -0.712647914886475
		4.4698543548584 -0.687993049621582
		4.66986465454102 -0.701810002326965
		4.72988510131836 -0.685672998428345
		4.92986869812012 -0.611393928527832
		5.19988632202148 -0.685552000999451
		5.22986602783203 -0.619214057922363
		5.29988861083984 -0.61235499382019
		5.36986207962036 -0.515460968017578
		5.42986917495728 -0.523818969726562
		6.16992092132568 -0.123232960700989
		6.3698468208313 -0.0536388158798218
		6.69989013671875 -0.0364210605621338
		6.96987533569336 -0.0474117994308472
		7.02987337112427 -0.00214159488677979
		7.06984233856201 -0.0291374921798706
		7.12984228134155 0.160205006599426
		7.16992425918579 0.0759021043777466
		7.19985294342041 0.150972962379456
		7.22989892959595 -0.0225034952163696
		7.29991912841797 0.136327028274536
		7.33985614776611 0.0532954931259155
		7.39991807937622 0.13841700553894
		7.43987560272217 0.150393962860107
		7.46986532211304 0.240285992622375
		7.52987289428711 0.151705980300903
		7.59986448287964 0.198394060134888
		7.6698579788208 0.303086996078491
		7.72985887527466 0.261451959609985
		7.82990121841431 0.387747049331665
		8.06991577148438 0.457958936691284
		8.12986946105957 0.37749195098877
		8.16994094848633 0.38644802570343
		8.19985485076904 0.268379926681519
		8.22982501983643 0.320523023605347
		8.26987838745117 0.304841995239258
		8.29984188079834 0.338461995124817
		8.3298511505127 0.500510931015015
		8.36984825134277 0.307502031326294
		8.42985820770264 0.386003971099854
		8.46987533569336 0.348865985870361
		8.49985694885254 1.68854999542236
		8.53999710083008 1.58247005939484
		8.59990787506104 0.48578405380249
		8.79998779296875 0.297445058822632
		9.00005626678467 0.322988033294678
		9.22984886169434 0.321486949920654
		9.29987716674805 0.291589975357056
		9.33986663818359 0.312991976737976
		9.36986446380615 0.260015964508057
		9.42987632751465 0.302953958511353
		9.46986865997314 0.332277059555054
		9.52988815307617 0.270014047622681
		9.69987869262695 0.2778480052948
		10.0698537826538 0.251215934753418
		10.1698579788208 0.192968010902405
		10.2298450469971 0.227213978767395
		10.3298683166504 0.154904961585999
		10.3998966217041 0.152405023574829
		10.529857635498 -0.0285402536392212
		10.7298650741577 -0.11077094078064
		10.7998867034912 -0.222653031349182
		10.869873046875 -0.18015193939209
		10.9298725128174 -0.257995963096619
		10.9998807907104 -0.250095009803772
		11.1698684692383 -0.490887999534607
		11.4299058914185 -0.769110918045044
		11.5398979187012 -0.719545006752014
		11.6298732757568 -0.720782041549683
		11.6699171066284 -0.750421047210693
		11.699878692627 -0.723870038986206
		11.8998603820801 -0.879243016242981
		12.3299150466919 -0.812322020530701
		12.3999013900757 -0.840180993080139
		12.5999269485474 -0.892338037490845
		12.6698808670044 -0.939873933792114
		12.739972114563 -1.01926004886627
		12.7698669433594 -0.99124002456665
		13.1298770904541 -1.28308999538422
		13.2298717498779 -1.25519001483917
		13.2698926925659 -1.17684996128082
		13.3298358917236 -1.32580995559692
		13.3999309539795 -1.26505994796753
		13.4698486328125 -1.14850997924805
		13.5298805236816 -1.24750995635986
		13.5698432922363 -1.15290999412537
		13.5998487472534 -1.17609000205994
		13.6298599243164 -1.04978001117706
		13.6698627471924 -1.12445998191833
		13.729907989502 -1.03394997119904
		13.7998504638672 -1.03984999656677
		13.8998680114746 -1.12506997585297
		14.0398426055908 -1.14725005626678
		14.0998811721802 -1.24910998344421
		14.169885635376 -1.18220996856689
		14.1998977661133 -1.28782999515533
		14.2298536300659 -1.24905002117157
		14.2998542785645 -1.24905002117157
		14.3398628234863 -1.17881000041962
		14.3699169158936 -1.27198004722595
		14.3998708724976 -1.17421996593475
		14.4299087524414 -1.21445000171661
		14.4698686599731 -1.17903995513916
		14.4998912811279 -1.29338002204895
		14.5698471069336 -1.23480999469757
		14.6298503875732 -1.29069995880127
		14.6999492645264 -1.22459995746613
		14.729866027832 -1.2861499786377
		14.8698968887329 -1.26436996459961
		14.8998775482178 -1.21039998531342
		14.9399070739746 -1.23296999931335
		14.9999027252197 -1.16665995121002
		15.0698690414429 -1.27830004692078
		15.1998872756958 -1.6706600189209
		15.2998695373535 -1.65464997291565
		15.3698720932007 -1.65829002857208
		15.469898223877 -1.61810994148254
		15.5298519134521 -1.34791004657745
		15.5698709487915 -1.33175003528595
		15.5998830795288 -1.21424996852875
		15.6298532485962 -1.34978997707367
		15.6998300552368 -1.07454001903534
		15.8398895263672 -1.19193005561829
		15.8998908996582 -1.35373997688293
		15.9698848724365 -1.10128998756409
		15.9998579025269 -1.17799997329712
		16.0399398803711 -1.17273998260498
		16.069881439209 -1.12541997432709
		16.0998668670654 -1.25083994865417
		16.2298545837402 -0.915888071060181
		16.2698631286621 -0.959368944168091
		16.3698787689209 -0.911592960357666
		16.4298725128174 -0.716068029403687
		16.7398719787598 -0.354562044143677
		16.7998809814453 -0.294858932495117
		16.9998950958252 -0.116328001022339
		17.329833984375 0.284487009048462
		17.429838180542 0.331771969795227
		17.469877243042 0.471799969673157
		17.6298694610596 0.672738075256348
		17.6699028015137 0.644562959671021
		17.8299217224121 0.754414081573486
		17.8698768615723 0.880028963088989
		17.8999214172363 0.795351982116699
		17.9698734283447 1.14219999313354
		17.999870300293 0.894273042678833
		18.0698566436768 0.9288250207901
		18.0999088287354 1.30721998214722
		18.1298751831055 1.09088003635406
		18.1698818206787 1.43025994300842
		18.2298603057861 1.34328997135162
		18.2698135375977 1.37534999847412
		18.3298721313477 1.12751996517181
		18.3698444366455 1.19254994392395
		18.469856262207 1.03654003143311
		18.5298919677734 1.06225001811981
		18.569881439209 0.954364061355591
		18.6298713684082 1.04393994808197
		18.6699123382568 0.792675018310547
		18.7299194335938 1.13850998878479
		18.8399295806885 1.33150994777679
		18.9298648834229 1.1952600479126
		18.9998226165771 1.61717998981476
		19.1298961639404 1.64543998241425
		19.1998481750488 1.83244001865387
		19.299898147583 1.38173997402191
		19.3998489379883 1.34338998794556
		19.4298477172852 1.39397001266479
		19.4698657989502 1.37278997898102
		19.5398788452148 1.82500994205475
		19.599853515625 1.78480994701385
		19.6398544311523 1.6944500207901
		19.6998615264893 1.76104998588562
		19.7998466491699 1.66341996192932
		19.8399085998535 1.67214000225067
		19.929859161377 1.61231005191803
		20.0398406982422 1.58931994438171
		20.0998783111572 1.4684100151062
		20.2000045776367 1.34557998180389
		20.2998943328857 1.41437995433807
		20.3699607849121 1.19584000110626
		21.3298721313477 0.784688949584961
		21.3698863983154 0.677566051483154
		21.429874420166 0.194579005241394
		21.4698677062988 0.189272999763489
		21.5298595428467 0.679130077362061
		21.5699005126953 0.688653945922852
		21.6298389434814 0.5190349817276
		21.6699066162109 0.514363050460815
		21.6999435424805 0.314849972724915
		21.7698745727539 0.339946985244751
		21.8298683166504 0.309637069702148
		21.8699188232422 0.41948401927948
		21.9299163818359 0.0651911497116089
		21.9998645782471 0.0826989412307739
		22.0698509216309 0.0709654092788696
		22.0999546051025 -0.0819604396820068
		22.3399753570557 -0.0954157114028931
		22.5698795318604 -0.125221967697144
		22.7999496459961 -0.545078039169312
		22.8698616027832 -0.845907926559448
		22.9999256134033 -0.966248035430908
		23.0298728942871 -0.905655026435852
		23.0998649597168 -1.00650000572205
		23.1298637390137 -0.962706089019775
		23.1998767852783 -1.01196002960205
		23.229887008667 -0.915909051895142
		23.2998523712158 -0.907055020332336
		24.3698673248291 -1.4237699508667
		24.4299068450928 -1.30580997467041
		24.8299179077148 -1.37290000915527
		24.9298515319824 -1.85500001907349
		24.9698925018311 -1.8445999622345
		24.9998741149902 -1.79718005657196
		25.0298748016357 -1.37964999675751
		25.0699157714844 -1.3967399597168
		25.0998706817627 -1.55868995189667
		25.1398944854736 -1.54499995708466
		25.1999034881592 -1.35283994674683
		25.2298526763916 -1.72599995136261
		25.2698574066162 -1.66049003601074
		25.2999267578125 -1.53649997711182
		25.3698806762695 -1.72643995285034
		25.4998588562012 -1.30589997768402
		25.5298805236816 -1.49509000778198
		25.5999450683594 -1.29197001457214
		25.7399349212646 -1.29803001880646
		25.7699127197266 -1.18678998947144
		25.7999858856201 -1.2386599779129
		25.9298553466797 -1.09908998012543
		26.0398941040039 -1.10338997840881
		26.3698711395264 -1.01747000217438
		26.3998851776123 -1.11061000823975
		26.429838180542 -0.960875988006592
		26.4998836517334 -1.02249002456665
		26.7298641204834 -0.694371938705444
		26.8698444366455 -0.559121012687683
		26.9298343658447 -0.432443976402283
		27.169864654541 -0.197558999061584
		27.3398990631104 -0.0342975854873657
		27.4298725128174 0.108453035354614
		27.8698921203613 0.49909496307373
		27.9298229217529 0.445757031440735
		27.9999027252197 0.648884057998657
		28.0999584197998 0.692396998405457
		28.1398773193359 0.686679005622864
		28.1998901367188 0.717725038528442
		28.2698650360107 0.764994025230408
		28.3299007415771 0.675890922546387
		28.369873046875 0.706057071685791
		28.4698791503906 0.882526993751526
		28.529899597168 0.82722806930542
		28.5998191833496 1.04233002662659
		28.7298946380615 1.02946996688843
		28.799898147583 0.853554964065552
		28.9298534393311 0.877593994140625
		28.9698677062988 0.969341039657593
		28.9998569488525 0.790303945541382
		29.1298580169678 0.815980911254883
		29.1998348236084 1.11518001556396
		29.2698860168457 1.15281999111176
		29.2999324798584 1.05057001113892
		29.3998565673828 1.16311001777649
		29.4298725128174 1.06999003887177
		29.4999446868896 1.14686000347137
		29.5998783111572 0.823625087738037
		29.6698780059814 0.86630392074585
		29.7298622131348 0.859771013259888
		29.7998924255371 0.771049976348877
		29.9298686981201 0.663478970527649
		31.2999057769775 -0.109667062759399
		31.4299430847168 -0.121891021728516
		31.4698810577393 -0.162114977836609
		31.4999313354492 -0.12254798412323
		31.5298862457275 -0.21408998966217
		31.5998840332031 -0.124482989311218
		31.6298828125 -0.22038197517395
		31.6698760986328 -0.160303950309753
		31.7299213409424 -0.14861798286438
		31.7998847961426 -0.185956954956055
		31.8698673248291 -0.420336961746216
		31.8998680114746 -0.160083055496216
		31.9999332427979 -0.143600940704346
		32.0698547363281 -0.714021921157837
		32.1699104309082 -0.71129298210144
		32.5698547363281 -0.918760061264038
		32.5999298095703 -0.812835931777954
		32.6298599243164 -1.01620995998383
		32.6998672485352 -1.01384997367859
		32.8699264526367 -0.877882957458496
		32.999885559082 -1.02953004837036
		33.0699310302734 -1.27286994457245
		33.1698913574219 -1.33831000328064
		33.2999649047852 -1.22580003738403
		33.3298721313477 -1.32713997364044
		33.3698654174805 -1.17441999912262
		33.4299011230469 -1.15435004234314
		33.499870300293 -1.20201003551483
		33.5298881530762 -1.34393000602722
		33.5699005126953 -1.22974002361298
		33.6699028015137 -1.71461999416351
		33.7698745727539 -1.7510199546814
		33.8000450134277 -1.889279961586
		33.8298797607422 -1.78770995140076
		33.8698921203613 -1.91904997825623
		33.89990234375 -1.86276996135712
		33.9999198913574 -2.01090002059937
		34.0298461914062 -2.03399991989136
		34.0999145507812 -2.16444993019104
		34.1699180603027 -2.25658011436462
		34.2298545837402 -2.18946003913879
		34.2698631286621 -2.13558006286621
		34.3399391174316 -2.26892995834351
		34.369873046875 -2.53339004516602
		34.4998817443848 -2.34460997581482
		34.5998954772949 -2.56835007667542
		34.6698608398438 -2.6676299571991
		34.7298622131348 -2.78893995285034
		34.7698974609375 -2.66303992271423
		34.799919128418 -2.82293009757996
		34.8298492431641 -2.76938009262085
		34.8998680114746 -2.73109006881714
		34.9399681091309 -2.95808005332947
		34.9699440002441 -2.8301100730896
		34.999870300293 -2.98116993904114
		35.2398643493652 -2.97322010993958
		35.2999000549316 -2.71100997924805
		35.3999214172363 -2.58496999740601
		35.4998550415039 -2.63012003898621
		35.6298980712891 -3.07309007644653
		35.6698684692383 -3.01992011070251
		35.7298278808594 -3.18987011909485
		35.7698593139648 -3.19857001304626
		35.7998733520508 -3.24984002113342
		35.8298721313477 -3.18567991256714
		35.8698654174805 -3.42921996116638
		35.9299430847168 -3.33031010627747
		35.9698638916016 -3.27768993377686
		35.9998931884766 -3.05253005027771
		36.0698928833008 -3.29820990562439
		36.0999526977539 -3.27047991752625
		36.1298484802246 -3.29380989074707
		36.1998519897461 -3.19843006134033
		36.2299270629883 -3.11259007453918
		36.2998809814453 -3.37476992607117
		36.3698959350586 -3.37743997573853
		36.3998756408691 -3.16968011856079
		36.4698677062988 -3.38710999488831
		36.4999046325684 -3.22062993049622
		36.5398712158203 -3.34043002128601
		36.5998725891113 -3.24990010261536
		36.6298675537109 -3.353600025177
		36.6699371337891 -3.3573899269104
		36.6999969482422 -3.53392004966736
		36.7298316955566 -3.40791010856628
		36.7998657226562 -3.41953992843628
		36.8298530578613 -3.37261009216309
		36.8999328613281 -3.40970993041992
		36.9298629760742 -3.23932003974915
		36.9998550415039 -3.43795990943909
		37.0298614501953 -3.23644995689392
		37.0699119567871 -3.40409994125366
		37.1298484802246 -3.23047995567322
		37.1998405456543 -3.31242990493774
		37.2298469543457 -3.3982400894165
		37.2699203491211 -3.34416007995605
		37.2999000549316 -3.46291995048523
		37.3298416137695 -3.38523006439209
		37.3698997497559 -3.4771900177002
		37.4698257446289 -3.39154005050659
		37.499942779541 -3.24085998535156
		37.5398635864258 -3.26842999458313
		37.5698394775391 -3.2291100025177
		37.6298484802246 -3.33970999717712
		37.6698455810547 -3.42630004882812
		37.729850769043 -3.33129000663757
		37.7698669433594 -2.95953011512756
		37.8698921203613 -2.63037991523743
		37.8999176025391 -2.84975004196167
		37.9998931884766 -2.86785006523132
		38.0298767089844 -2.59337997436523
		38.0698699951172 -2.56497001647949
		38.1298484802246 -2.79390001296997
		38.3298950195312 -2.72399997711182
		38.3698272705078 -2.73906993865967
		38.4399185180664 -2.44623994827271
		38.5298500061035 -2.62862992286682
		38.5698509216309 -2.30749011039734
		38.6298980712891 -2.5181200504303
		38.6698226928711 -2.58731007575989
		38.7298736572266 -2.53154993057251
		38.7698783874512 -2.51135993003845
		38.8298873901367 -2.55101990699768
		38.8698539733887 -2.79787993431091
		39 -2.42331004142761
		39.0998764038086 -2.41197991371155
		39.1298675537109 -2.33189988136292
		39.1998634338379 -2.06807994842529
		39.2698860168457 -1.90625
		39.3298568725586 -1.97044003009796
		39.4298286437988 -1.8608900308609
		39.5299301147461 -1.90983998775482
		39.5698890686035 -1.92201995849609
		39.5998764038086 -1.85257005691528
		39.6298866271973 -2.06336998939514
		39.6998405456543 -2.04605007171631
		39.7698822021484 -1.84869003295898
		39.8699035644531 -1.68977999687195
		40.1998710632324 -1.4870400428772
		40.2999572753906 -1.53164005279541
		40.3698616027832 -1.29711997509003
		40.429874420166 -1.28638005256653
		40.4999084472656 -1.08131003379822
		40.5298805236816 -1.1637099981308
		40.5698776245117 -1.04885005950928
		40.6298751831055 -1.06907999515533
		40.6698455810547 -1.0299299955368
		40.6998329162598 -1.12220001220703
		40.7698745727539 -0.967736959457397
		40.8998756408691 -0.891526937484741
		41.0298690795898 -0.781209945678711
		41.0699043273926 -0.764940977096558
		41.1298828125 -0.667271971702576
		41.1998710632324 -0.654326915740967
		41.2698860168457 -0.588638067245483
		41.3699035644531 -0.409662008285522
		41.7699279785156 -0.0244770050048828
		41.829891204834 0.0334612131118774
		48.569881439209 2.69078993797302
		48.9298515319824 2.6758599281311
		48.9998970031738 2.41166996955872
		49.0698623657227 2.4858500957489
		49.1698760986328 2.41226005554199
		49.1999435424805 2.54766988754272
		49.2298927307129 2.42475008964539
		49.2998847961426 2.62013006210327
		49.3698806762695 2.40091991424561
		49.4698524475098 2.5342800617218
		49.5298652648926 2.52368998527527
		49.5699119567871 2.55485010147095
		49.5998992919922 2.51275992393494
		49.6698837280273 2.63525009155273
		49.7698783874512 2.57953000068665
		49.7998809814453 2.6469099521637
		49.8698844909668 2.54770994186401
		49.9698677062988 2.75523996353149
		50.0698699951172 2.70739006996155
		50.1298980712891 2.74170994758606
		50.1998901367188 2.48967003822327
		50.269905090332 2.43900990486145
		50.3698692321777 2.38652992248535
		50.3998870849609 2.50620007514954
		50.4298782348633 2.43484997749329
		50.4998512268066 2.48550009727478
		50.5998573303223 2.42946004867554
		50.6298446655273 2.5127899646759
		50.6698837280273 2.47058010101318
		50.6998634338379 2.62646007537842
		50.7698707580566 2.45376992225647
		50.8298873901367 2.58277988433838
		50.8999061584473 2.5595600605011
		50.9699287414551 2.59877991676331
		51.0698890686035 2.54069995880127
		51.2998847961426 2.26079988479614
		59.0099182128906 -0.905598998069763
		59.0999336242676 -0.97544002532959
		59.1398658752441 -0.919022083282471
		59.1698760986328 -1.06204998493195
		59.2698631286621 -1.08501994609833
		59.2999038696289 -1.05292999744415
		59.3998565673828 -1.14637994766235
		59.4698829650879 -1.08226001262665
		59.4999504089355 -1.29437005519867
		59.529857635498 -1.15930998325348
		59.6298904418945 -1.42004001140594
		59.7698554992676 -1.41373002529144
		59.8998756408691 -1.4595799446106
		59.9298667907715 -1.87105000019073
		59.9998512268066 -1.54855000972748
		60.0698432922363 -1.96786999702454
		60.1298675537109 -1.96496999263763
		60.2699203491211 -2.07801008224487
		60.569881439209 -2.40251994132996
		60.6298828125 -2.44285011291504
		62.5998764038086 -3.07084989547729
		63.469898223877 -3.41376996040344
		63.5398864746094 -3.39161992073059
		63.5999755859375 -3.43284010887146
		63.6698951721191 -3.37578010559082
		63.7998390197754 -3.48948001861572
		63.89990234375 -3.48470997810364
		64.0298538208008 -3.58204007148743
		64.0998764038086 -3.63158988952637
		64.1298751831055 -3.56054997444153
		64.1698913574219 -3.66446995735168
		64.269889831543 -3.58931994438171
		64.4699325561523 -3.78136992454529
		64.5299072265625 -3.66336989402771
		64.5698699951172 -3.73390007019043
		64.5998992919922 -3.70900011062622
		64.6699447631836 -3.76330995559692
		64.7699356079102 -3.67637991905212
		64.7998809814453 -3.78274011611938
		64.829948425293 -3.70143008232117
		64.9098815917969 -3.76704001426697
		65.0298919677734 -3.81484007835388
		65.0698547363281 -3.68251991271973
		65.1998901367188 -3.78997993469238
		65.2298583984375 -3.76536011695862
		65.2998580932617 -3.7826099395752
		65.3298492431641 -3.74411010742188
		65.3998794555664 -3.78501009941101
		65.4698791503906 -3.90121006965637
		65.5698623657227 -3.94131994247437
		65.6699142456055 -3.92097997665405
		65.7998657226562 -3.80814003944397
		65.8998947143555 -3.93130993843079
		65.9298095703125 -3.84026002883911
		65.9998397827148 -3.95729994773865
		66.0998764038086 -3.92462992668152
		66.1998672485352 -4.05775022506714
		66.2298736572266 -3.99187994003296
		66.6998901367188 -4.04949998855591
		67.0298385620117 -4.08205986022949
		69.329833984375 -3.59904003143311
		69.3698883056641 -3.40391993522644
		69.3998870849609 -3.56591010093689
		69.4699096679688 -3.33536005020142
		69.4998474121094 -3.39305996894836
		69.5299224853516 -3.33125996589661
		69.6000213623047 -3.41546988487244
		69.6698379516602 -3.19749999046326
		69.7999267578125 -3.17000007629395
		69.8399429321289 -3.18821001052856
		69.8698577880859 -3.14540004730225
		69.9298858642578 -2.91540002822876
		69.9698715209961 -2.75030994415283
		70.0298614501953 -2.77724003791809
		70.0999374389648 -2.75566005706787
		70.1698913574219 -2.44822001457214
		70.2298202514648 -2.47360992431641
		70.3998641967773 -2.49376010894775
		70.4298553466797 -2.3071300983429
		70.4713134765625 -2.29181003570557
		70.5099334716797 -2.32946991920471
		70.5698699951172 -2.24538993835449
		70.9298858642578 -2.25926995277405
		70.969856262207 -2.04253005981445
		71.0398635864258 -2.13539004325867
		71.0998764038086 -2.04274010658264
		71.1698760986328 -1.92605996131897
		71.1998977661133 -1.77042996883392
		71.3400421142578 -1.95067000389099
		71.3999710083008 -1.77540004253387
		71.469856262207 -1.9159300327301
		71.529914855957 -1.84798002243042
		71.5999145507812 -1.84701001644135
		71.6298522949219 -1.7989000082016
		71.6998825073242 -1.83275997638702
		71.7398681640625 -1.99432003498077
		71.7998809814453 -1.83317995071411
		71.8698959350586 -1.93220996856689
		71.9298706054688 -1.77602994441986
		71.9698715209961 -1.82403004169464
		71.9999008178711 -1.77763998508453
		72.0400466918945 -1.91049003601074
		72.0698471069336 -1.84947001934052
		72.1298904418945 -1.89790999889374
		72.1698532104492 -1.88779997825623
		72.1998596191406 -1.32213997840881
		72.4298629760742 -1.25113999843597
		72.469856262207 -1.35696005821228
		72.5299072265625 -1.21606004238129
		72.5698699951172 -1.20077002048492
		72.6298599243164 -1.10180997848511
		72.6998825073242 -1.05756998062134
		72.739860534668 -0.987957954406738
		72.7998886108398 -0.971185922622681
		73.9999542236328 -0.00907051563262939
		74.0398788452148 -0.00283920764923096
		74.0998840332031 0.0415823459625244
		74.1699295043945 0.129963040351868
		74.2699203491211 0.145717024803162
		74.3298873901367 0.395537972450256
		74.3999176025391 0.297868967056274
		74.4299240112305 0.412591934204102
		74.499885559082 0.381034016609192
		74.5698547363281 0.398872971534729
		74.6298675537109 0.57210099697113
		74.6698760986328 0.525829076766968
		74.7698669433594 0.637042045593262
		74.7999038696289 0.610490083694458
		74.8699035644531 0.674138069152832
		75.0698776245117 0.931884050369263
		75.1698532104492 0.9566969871521
		75.2298278808594 0.858765006065369
		75.269905090332 0.851005077362061
		75.3298187255859 0.915701985359192
		75.4298629760742 0.927286982536316
		75.6298522949219 0.957772016525269
		75.6998977661133 1.07804000377655
		76.1298828125 0.967437028884888
		76.1698989868164 0.819553971290588
		76.229850769043 0.859691023826599
		76.2698822021484 0.762592077255249
		76.4299163818359 0.818458080291748
		76.469856262207 0.751698970794678
		76.6698455810547 0.644001007080078
		76.7299957275391 0.658478975296021
		76.8400268554688 0.581117987632751
		76.9298858642578 0.563760042190552
		76.9998779296875 0.449039936065674
		77.0398635864258 0.469027042388916
		77.1698837280273 0.337100028991699
		77.2298431396484 0.33568000793457
		77.3698654174805 0.195106029510498
		77.4698715209961 0.145305037498474
		78.3998794555664 -0.449679970741272
		78.4298477172852 -0.521830081939697
		78.4699249267578 -0.487165927886963
		78.5698547363281 -0.529778957366943
		78.7298736572266 -0.58013391494751
		78.7998809814453 -0.608358979225159
		78.8999252319336 -0.669986963272095
		79.0999069213867 -0.727460980415344
		79.1699066162109 -0.703459978103638
		79.269905090332 -0.757067918777466
		79.3298950195312 -0.701854944229126
		79.3998718261719 -0.766025066375732
		79.4998931884766 -0.82254695892334
		79.6298370361328 -0.752547979354858
		79.6698837280273 -0.68782901763916
		79.6998825073242 -0.783481001853943
		79.7298889160156 -0.719272971153259
		79.799934387207 -0.759577035903931
		79.869873046875 -0.675451040267944
		80.0698547363281 -0.596104979515076
		80.1699066162109 -0.576425075531006
		80.2698745727539 -0.44977593421936
		80.4298858642578 -0.300135016441345
		81.0998687744141 0.0959827899932861
		81.4398956298828 0.0668313503265381
		81.4999084472656 0.0450894832611084
		81.5698471069336 -0.0353225469589233
		82.0298919677734 -0.439231038093567
		82.1298751831055 -0.58473002910614
		82.1998901367188 -0.592071056365967
		82.2998733520508 -0.692815065383911
		82.3998870849609 -0.747854948043823
		83.6299591064453 -1.1883100271225
		83.6698608398438 -1.10485005378723
		83.6999359130859 -1.1609400510788
		83.7698669433594 -1.13188004493713
		83.7998657226562 -1.21282005310059
		83.8298873901367 -1.14663004875183
		83.8698577880859 -1.17338001728058
		84.0000076293945 -1.08169996738434
		84.0698547363281 -1.20539999008179
		84.1298828125 -1.17504000663757
		84.1698760986328 -1.19913005828857
		84.1998443603516 -1.16710996627808
		84.2698593139648 -1.18784999847412
		84.3999328613281 -1.14883005619049
		84.5298461914062 -0.915355920791626
		84.5698699951172 -0.907844066619873
		84.6298599243164 -0.952517986297607
		84.6698532104492 -0.946009993553162
		84.6998596191406 -0.875637054443359
		84.8298721313477 -0.826755046844482
		85.6698684692383 -0.623887062072754
		85.7299270629883 -0.538433074951172
		85.7998580932617 -0.453024983406067
		85.8698654174805 -0.384827017784119
		85.9298553466797 -0.26164698600769
		85.9999008178711 -0.186710953712463
		86.0999450683594 -0.142173051834106
		86.1298751831055 -0.175132036209106
		86.1999588012695 -0.11384904384613
		86.2698745727539 -0.0596814155578613
		86.3298492431641 -0.095542311668396
		86.3998641967773 0.0371743440628052
		86.4698257446289 0.0506762266159058
		86.529899597168 0.115015029907227
		86.5998687744141 0.127310991287231
		86.8298645019531 0.484267950057983
		86.8698120117188 0.446660041809082
		87.1998672485352 0.574181079864502
		87.2698669433594 0.684306979179382
		87.3998641967773 0.651999950408936
		87.4298553466797 0.539968013763428
		87.4999694824219 0.610779047012329
		87.6699523925781 0.762439012527466
		87.6999053955078 0.688898086547852
		87.769889831543 0.770406007766724
		87.8298721313477 0.693454027175903
		88.0298538208008 0.893172025680542
		88.0698699951172 0.857730984687805
		88.099853515625 1.11811995506287
		88.1699142456055 0.831836938858032
		88.2298889160156 0.904981970787048
		88.3000335693359 0.872627973556519
		88.3298797607422 0.920360088348389
		88.4999237060547 0.806441068649292
		88.5298461914062 0.881983041763306
		88.5999450683594 0.884942054748535
		88.6299209594727 0.852041006088257
		88.769889831543 0.895443916320801
		88.8298950195312 0.676476955413818
		88.8999404907227 0.629601955413818
		88.9298858642578 0.504668951034546
		89.0298690795898 0.686267018318176
		89.0699005126953 0.555341005325317
		89.0999450683594 0.604346036911011
		89.1299209594727 0.746617078781128
		89.1999206542969 0.657387018203735
		89.2299041748047 0.587939977645874
		89.2999496459961 0.633638978004456
		89.3698654174805 0.598801016807556
		89.3998565673828 0.631850957870483
		89.4699020385742 0.515162944793701
		90.4698791503906 -0.0669145584106445
		90.6299133300781 -0.259300947189331
		90.7298278808594 -0.293067932128906
		90.9298400878906 -0.499773025512695
		91.0999374389648 -0.571907997131348
		91.1698684692383 -0.544774055480957
		91.2699432373047 -0.579299926757812
		91.7298278808594 -0.642392992973328
		91.7999114990234 -0.597885012626648
		91.8299026489258 -0.627972006797791
		91.9298553466797 -0.584573030471802
		92.0698471069336 -0.555262088775635
		92.0998611450195 -0.497561931610107
		92.2298812866211 -0.522315979003906
		92.269905090332 -0.478853940963745
		92.2998809814453 -0.53281307220459
		92.3299255371094 -0.486688017845154
		92.4699096679688 -0.497565984725952
		92.5298690795898 -0.469205975532532
		92.5698699951172 -0.46943998336792
		92.5998840332031 -0.423467993736267
		92.6298599243164 -0.452120065689087
		92.6999282836914 -0.364886999130249
		92.7299270629883 -0.436429977416992
		92.7998962402344 -0.37704598903656
		92.8998718261719 -0.356852054595947
		92.9298477172852 -0.298733949661255
		92.9698486328125 -0.304309964179993
		93.0998687744141 -0.0637543201446533
		93.7998580932617 0.228163003921509
		93.8298873901367 0.198904991149902
		93.8999481201172 0.212847948074341
		94.0298690795898 0.297018051147461
		94.0698471069336 0.216299057006836
		94.0998992919922 0.244989991188049
		94.1298522949219 0.343281984329224
		94.1698913574219 0.344398021697998
		94.2299270629883 0.236786007881165
		94.2698745727539 0.244420051574707
		94.2998962402344 0.297791957855225
		94.3398513793945 0.274201989173889
		94.3698501586914 0.318704962730408
		94.3998794555664 0.238005042076111
		94.4698867797852 0.274803996086121
		94.5298538208008 0.34822404384613
		94.6298828125 0.249176025390625
		94.6998901367188 0.320731997489929
		94.7298583984375 0.243260025978088
		94.7999877929688 0.26868999004364
		94.8699111938477 0.219571948051453
		94.9698715209961 0.300471067428589
		95.1299057006836 0.260853052139282
		95.1998443603516 0.253278970718384
		95.2698593139648 0.233932971954346
		95.3298873901367 0.277547001838684
		95.3698883056641 0.258211970329285
		95.4299011230469 0.20216703414917
		95.5698776245117 0.178202986717224
		95.7299270629883 0.159518003463745
		95.8298797607422 0.161646962165833
		96.0298614501953 0.137233972549438
		96.3999633789062 0.0291396379470825
		96.469856262207 -0.169420957565308
		96.4998397827148 -0.144279003143311
		96.8298797607422 0.0491863489151001
		96.9298629760742 0.00789690017700195
		97.1299362182617 -0.296180009841919
		97.1998672485352 -0.352856993675232
		97.2298736572266 -0.390596985816956
		98.0698852539062 -0.52869701385498
		98.0998840332031 -0.565727949142456
		98.1298751831055 -0.486156940460205
		98.1698760986328 -0.545204997062683
		98.2298736572266 -0.479843020439148
		98.3998947143555 -0.497123956680298
		98.4698791503906 -0.670167922973633
		98.599967956543 -0.666207075119019
		98.7298736572266 -0.761090040206909
		98.7999801635742 -0.777441024780273
		98.8998565673828 -0.824180006980896
		98.999885559082 -0.860902070999146
		99.1298370361328 -0.947099924087524
		99.1698684692383 -0.861037969589233
		99.1998596191406 -0.936157941818237
		99.229866027832 -0.851459980010986
		99.2999114990234 -0.924134016036987
		99.3999328613281 -0.917631983757019
		99.4298629760742 -0.848417997360229
		99.5298690795898 -0.837930917739868
		99.5698699951172 -0.905663967132568
		99.5999145507812 -0.842165946960449
		99.6298599243164 -0.862106084823608
		99.6698837280273 -0.841429948806763
		99.7299194335938 -0.912845015525818
		100.069885253906 -0.783501029014587
		100.269882202148 -0.659430027008057
		100.329856872559 -0.661800026893616
		100.369842529297 -0.594193935394287
		100.429840087891 -0.620671033859253
		100.599853515625 -0.492552995681763
		100.769828796387 -0.365036010742188
		100.929870605469 -0.271438956260681
		101.199897766113 0.0609179735183716
		101.229858398438 0.162413001060486
		101.269912719727 0.134341955184937
		101.329917907715 0.168318033218384
		101.399871826172 0.222370982170105
		101.429847717285 0.279307961463928
		101.469940185547 0.253772974014282
		101.529830932617 0.335317015647888
		101.699913024902 0.54469895362854
		101.799842834473 0.55393397808075
		101.82991027832 0.638916015625
		102.069854736328 0.729637980461121
		102.129875183105 0.684031963348389
		102.199851989746 0.695461988449097
		102.269874572754 0.78767204284668
		102.299865722656 0.751791000366211
		102.329849243164 1.02372002601624
		102.369857788086 1.02410995960236
		102.429908752441 0.916544914245605
		102.469856262207 0.818449974060059
		102.499893188477 0.852190017700195
		102.529861450195 0.746110916137695
		102.569900512695 0.788179993629456
		102.599876403809 0.701637029647827
		102.629898071289 0.798033952713013
		102.699951171875 0.797328948974609
		102.769874572754 0.912569046020508
		102.799873352051 0.943513989448547
		102.86988067627 0.913586020469666
		102.96989440918 0.929959058761597
		103.069931030273 1.0208899974823
		103.129898071289 1.00656998157501
		103.169860839844 0.918803930282593
		103.199913024902 0.996914029121399
		103.229873657227 0.944504976272583
		103.269859313965 1.00757002830505
		103.299865722656 0.927865028381348
		103.36988067627 1.07032001018524
		103.429878234863 1.12628996372223
		103.469909667969 0.995779037475586
		103.499931335449 1.09899997711182
		103.529914855957 0.826252937316895
		103.629867553711 0.767813920974731
		103.669883728027 0.72203803062439
		103.699928283691 0.561874985694885
		103.799964904785 0.686164975166321
		103.829895019531 0.991658926010132
		103.869873046875 0.944154024124146
		103.899940490723 0.753677010536194
		103.929847717285 0.921277046203613
		103.969856262207 0.930037021636963
		103.999877929688 0.707437992095947
		104.029846191406 0.840496063232422
		104.069854736328 0.682492971420288
		104.099868774414 0.81036102771759
		104.129844665527 0.720870018005371
		104.199821472168 0.710422039031982
		104.229866027832 0.775520086288452
		104.26985168457 0.760803937911987
		104.369926452637 0.616183042526245
		104.42985534668 0.670445919036865
		104.529838562012 0.590095996856689
		104.569847106934 0.577099084854126
		104.599891662598 0.101807951927185
		104.629844665527 0.443403959274292
		104.669868469238 0.426156997680664
		104.699859619141 0.481231927871704
		104.769905090332 0.420822978019714
		104.869911193848 0.454277992248535
		104.929885864258 0.0893491506576538
		104.969917297363 0.204751014709473
		105.829895019531 -0.164023041725159
		105.869873046875 -0.104802012443542
		105.929893493652 -0.136935949325562
		106.029861450195 -0.127655029296875
		106.999893188477 -0.815065026283264
		107.02995300293 -0.93585205078125
		107.099876403809 -0.836619973182678
		107.129890441895 -0.870113015174866
		107.199882507324 -0.953451991081238
		107.269874572754 -1.03434002399445
		107.36988067627 -1.11627995967865
		107.399887084961 -1.05614995956421
		107.629943847656 -1.39372003078461
		107.69995880127 -1.76769995689392
		107.729835510254 -1.43304002285004
		107.999923706055 -1.54464995861053
		108.029846191406 -2.00904011726379
		108.269874572754 -1.80382001399994
		108.399841308594 -2.34481000900269
		109.499870300293 -3.12444996833801
		109.969879150391 -3.40598011016846
		110.06990814209 -3.40828990936279
		110.129844665527 -3.4334499835968
		110.199897766113 -3.37578010559082
		110.26993560791 -3.47773003578186
		110.329872131348 -3.47460007667542
		110.369873046875 -3.47920989990234
		110.429901123047 -3.63605999946594
		110.469924926758 -3.6472499370575
		110.569862365723 -3.72410011291504
		110.599906921387 -3.65277004241943
		110.669906616211 -3.69626998901367
		110.729866027832 -3.64112997055054
		110.96989440918 -3.82327008247375
		111.029830932617 -3.80728006362915
		111.129867553711 -3.72874999046326
		111.299873352051 -3.81807994842529
		111.32991027832 -3.88383007049561
		111.399864196777 -3.84677004814148
		111.429840087891 -3.68719005584717
		111.569877624512 -3.86904001235962
		111.6298828125 -3.73330998420715
		111.669876098633 -3.7546501159668
		111.729858398438 -3.86465001106262
		111.899856567383 -3.94413995742798
		111.929840087891 -3.83116006851196
		112.029861450195 -3.84856009483337
		112.069900512695 -3.92529988288879
		112.129844665527 -3.85584998130798
		112.199905395508 -3.8987500667572
		112.269859313965 -3.95694994926453
		112.369857788086 -3.96759009361267
		112.399864196777 -3.9164400100708
		112.429878234863 -4.02731990814209
		112.529876708984 -3.995609998703
		112.729835510254 -4.04919004440308
		113.029846191406 -4.07646989822388
		113.099876403809 -4.24333000183105
		114.629898071289 -3.63032007217407
		114.669883728027 -3.84666991233826
		114.72989654541 -3.63185000419617
		114.799934387207 -3.9728000164032
		114.869895935059 -4.00891017913818
		114.899925231934 -3.89146995544434
		115.069885253906 -3.57411003112793
		115.129913330078 -3.41300010681152
		115.169860839844 -3.60352993011475
		115.229858398438 -3.46489000320435
		115.269859313965 -3.59523010253906
		115.429885864258 -3.28285002708435
		115.469863891602 -3.27286005020142
		115.499885559082 -3.47240996360779
		115.629905700684 -3.20978999137878
		115.669830322266 -3.39222002029419
		115.769866943359 -3.09400010108948
		115.829849243164 -3.11960005760193
		115.86986541748 -3.11496996879578
		115.929878234863 -2.98064994812012
		115.999977111816 -3.06838011741638
		116.099853515625 -3.07533001899719
		116.169868469238 -2.91591000556946
		116.229873657227 -2.97736001014709
		116.299957275391 -2.84126996994019
		116.399948120117 -2.7154700756073
		116.539855957031 -2.39317989349365
		116.599952697754 -2.45409989356995
		116.629898071289 -2.39122009277344
		116.669921875 -2.43038988113403
		116.829895019531 -2.1906099319458
		116.899948120117 -1.92755997180939
		116.969879150391 -1.9964200258255
		117.069885253906 -1.70902001857758
		117.129859924316 -1.66628003120422
		117.199913024902 -1.40780997276306
		117.299896240234 -1.34046995639801
		117.52995300293 -1.10292994976044
		117.599868774414 -1.07219994068146
		117.669914245605 -1.02202999591827
		117.999900817871 -0.609785079956055
		118.02986907959 -0.633594989776611
		118.069885253906 -0.595288038253784
		118.169906616211 -0.402478933334351
		118.469879150391 -0.0208671092987061
		118.499870300293 0.0216153860092163
		120.669898986816 2.16687989234924
		120.699882507324 2.05960988998413
		120.769897460938 2.17358994483948
		120.799865722656 2.53671002388
		120.829864501953 2.14818000793457
		120.86986541748 2.5488600730896
		120.969841003418 2.11539006233215
		121.129867553711 2.17206001281738
		121.299942016602 3.02876996994019
		121.399887084961 2.22966003417969
		122.669876098633 2.74130988121033
		122.699867248535 2.64859008789062
		122.729850769043 2.4345600605011
		122.769874572754 2.61930990219116
		122.799926757812 2.42744994163513
		122.86986541748 2.59421992301941
		122.899833679199 2.63105010986328
		122.929847717285 2.53726005554199
		122.999893188477 2.5662899017334
		123.029922485352 2.54538989067078
		123.069938659668 2.60421991348267
		123.09986114502 2.5081799030304
		123.129867553711 2.60658001899719
		123.169898986816 2.59173989295959
		123.199882507324 2.4765899181366
		123.229873657227 2.57559990882874
		123.269859313965 2.54489994049072
		123.329895019531 2.69130992889404
		123.36986541748 2.65465998649597
		123.399932861328 2.831209897995
		123.469886779785 2.79819011688232
		123.529899597168 2.86880993843079
		123.569877624512 2.89276003837585
		123.699890136719 2.57226991653442
		123.729873657227 2.64438009262085
		123.869850158691 2.47324991226196
		123.899932861328 2.62185001373291
		123.929847717285 2.43801999092102
		123.969856262207 2.6769700050354
		124.02986907959 2.66128993034363
		124.129867553711 2.4792799949646
		124.199974060059 2.66942000389099
		124.269889831543 2.66581010818481
		124.32991027832 2.61590003967285
		124.36988067627 2.61627006530762
		124.429862976074 2.54897999763489
		124.499954223633 2.55204010009766
		124.569854736328 2.6053900718689
		124.59986114502 2.50477004051208
		124.899841308594 2.31423997879028
		125.1298828125 2.12647008895874
		125.199836730957 1.96744000911713
		125.369873046875 1.87784004211426
		125.469879150391 1.93484997749329
		125.499839782715 2.13040995597839
		125.599884033203 2.21222996711731
		125.799835205078 1.75873994827271
		125.829864501953 1.83095002174377
		126.169868469238 1.41325998306274
		126.229858398438 1.43862998485565
		126.299896240234 1.28977000713348
		126.329864501953 1.51826000213623
		126.369857788086 1.39465999603271
		126.399841308594 1.51686000823975
		126.499893188477 1.30200004577637
		126.569900512695 1.22391998767853
		126.599891662598 1.35930001735687
		126.629890441895 1.32425999641418
		126.669868469238 1.3729499578476
		126.699859619141 1.34885001182556
		126.769897460938 1.1290899515152
		126.799873352051 1.03407001495361
		126.829879760742 1.10233998298645
		126.899871826172 0.951635003089905
		127.199882507324 1.10736000537872
		129.029876708984 -0.968786954879761
		129.1298828125 -0.995995998382568
		129.199890136719 -1.65076994895935
		129.429870605469 -1.38935995101929
		129.829864501953 -1.48110997676849
		129.899887084961 -2.02430009841919
		129.969863891602 -2.00174999237061
		130.129867553711 -2.08299994468689
		130.169860839844 -2.22398996353149
		130.19987487793 -3.33921003341675
		132.069885253906 -3.36701011657715
		132.099884033203 -3.40575003623962
		132.399948120117 -3.41438007354736
		132.469848632812 -3.46482992172241
		132.499923706055 -3.41107988357544
		132.529861450195 -3.51923990249634
		132.729888916016 -3.44686007499695
		132.769882202148 -3.58180999755859
		132.829849243164 -3.49786996841431
		132.899887084961 -3.53463006019592
		132.929840087891 -3.6565899848938
		132.969833374023 -3.67070007324219
		133.029830932617 -3.55552005767822
		133.069854736328 -3.52819991111755
		133.19987487793 -3.62872004508972
		133.269882202148 -3.70267009735107
		133.329864501953 -3.57571005821228
		133.369873046875 -3.59190011024475
		133.399856567383 -3.6854100227356
		133.429885864258 -3.58541011810303
		133.499862670898 -3.60229992866516
		133.529846191406 -3.55928993225098
		133.569854736328 -3.59368991851807
		133.599853515625 -3.55928993225098
		133.669876098633 -3.58402991294861
		133.699905395508 -3.48679995536804
		133.769866943359 -3.54265999794006
		133.799850463867 -3.74925994873047
		133.829895019531 -3.65948009490967
		133.869903564453 -3.65948009490967
		133.929901123047 -3.5333399772644
		133.999908447266 -3.53670001029968
		134.169845581055 -3.75770998001099
		134.199890136719 -3.7195999622345
		134.229904174805 -3.80236005783081
		134.269866943359 -3.80236005783081
		134.299819946289 -3.74231004714966
		134.329879760742 -3.81616997718811
		134.39990234375 -3.84173989295959
		134.429916381836 -3.69381999969482
		134.669876098633 -3.72561001777649
		134.729873657227 -3.87514996528625
		134.969879150391 -3.87923002243042
		134.99983215332 -3.98133993148804
		135.069854736328 -3.92840003967285
		135.129898071289 -4.06745004653931
		135.229858398438 -4.06908988952637
		135.269836425781 -3.96772003173828
		135.299926757812 -4.09246015548706
		135.329895019531 -3.9963800907135
		135.369842529297 -3.98824000358582
		135.39990234375 -4.09246015548706
		135.429870605469 -3.98824000358582
		135.499923706055 -3.98017001152039
		135.52995300293 -4.18590021133423
		135.599868774414 -4.15750980377197
		135.76985168457 -4.24306011199951
		135.869888305664 -4.10929012298584
		135.929885864258 -4.10570001602173
		135.999923706055 -3.83458995819092
		136.329986572266 -4.11881017684937
		136.400146484375 -3.83266997337341
		136.429885864258 -4.05251979827881
		136.469863891602 -4.04946994781494
		136.529891967773 -3.83947992324829
		136.569915771484 -3.8052499294281
		136.629852294922 -3.63032007217407
		136.669845581055 -3.6237199306488
		136.729873657227 -3.24496006965637
		137.1298828125 -3.2196900844574
		137.169860839844 -3.27698993682861
		137.229873657227 -3.21867990493774
		137.26985168457 -3.2359299659729
		137.299850463867 -3.29728007316589
		137.399856567383 -2.98178005218506
		137.429885864258 -3.19473004341125
		137.499893188477 -3.15811991691589
		137.529861450195 -2.91752004623413
		137.569854736328 -3.04401993751526
		137.629852294922 -2.9893798828125
		137.729843139648 -2.8954598903656
		137.799911499023 -2.69338989257812
		137.829864501953 -2.54598999023438
		137.869857788086 -2.67378997802734
		137.92985534668 -2.26094007492065
		137.96989440918 -2.20012998580933
		137.999877929688 -2.25777006149292
		138.029907226562 -2.17844009399414
		138.069900512695 -2.20012998580933
		138.099945068359 -2.15782999992371
		138.129837036133 -2.05001997947693
		138.169891357422 -2.1430299282074
		138.229919433594 -2.0905499458313
		138.299865722656 -2.14924001693726
		138.369857788086 -2.13668990135193
		138.429885864258 -1.95266997814178
		138.499908447266 -1.90913999080658
		138.569915771484 -1.84512996673584
		138.599884033203 -1.74827003479004
		138.629898071289 -1.86965000629425
		138.669845581055 -1.81342005729675
		138.729888916016 -1.44956994056702
		138.799896240234 -1.49133002758026
		138.899887084961 -1.39328002929688
		138.939834594727 -1.42543995380402
		138.969848632812 -1.39257001876831
		138.999862670898 -1.42482995986938
		139.099853515625 -1.29377996921539
		139.169937133789 -1.37525999546051
		139.19987487793 -1.25293004512787
		139.229858398438 -1.3855299949646
		139.299850463867 -1.16685998439789
		139.369903564453 -1.21195995807648
		139.469863891602 -1.07621002197266
		139.529891967773 -1.12707996368408
		139.569915771484 -1.07925999164581
		139.629898071289 -0.967365026473999
		139.729888916016 -0.895818948745728
		139.769866943359 -0.962723016738892
		139.799835205078 -0.861515045166016
		139.829879760742 -0.941282033920288
		139.899856567383 -0.7987459897995
		139.999923706055 -0.762898921966553
		140.029861450195 -0.796579003334045
		140.099868774414 -0.734972953796387
		140.129837036133 -0.767571926116943
		140.169876098633 -0.662044048309326
		140.229888916016 -0.773988962173462
		140.369842529297 -0.681329965591431
		140.469863891602 -0.574355006217957
		140.529891967773 -0.598278045654297
		140.599899291992 -0.459358930587769
		140.669845581055 -0.559378981590271
		140.699890136719 -0.551759004592896
	};
\addlegendentry{Prediction}


==> tikz/vis_localize/vis_loc_test2_y_clean.tex <==
\addplot [semithick, steelblue31119180]
table {%
		0.0398528575897217 0.37576961517334
		0.299866676330566 0.412076950073242
		0.499995708465576 0.374629497528076
		1.32991504669189 0.08821702003479
		1.56985712051392 0.109835863113403
		1.93987846374512 0.205654144287109
		2.23984622955322 0.22833776473999
		3.66988158226013 0.0905218124389648
		4.39997005462646 0.0939831733703613
		4.83985424041748 -0.117632865905762
		5.06985759735107 -0.219118118286133
		5.29988861083984 -0.230101585388184
		5.42986917495728 -0.201272964477539
		6.92984008789062 -0.0856921672821045
		7.52987289428711 0.0365960597991943
		7.72985887527466 0.00221443176269531
		7.82990121841431 -0.0388224124908447
		8.12986946105957 -0.157727479934692
		8.29984188079834 -0.138189554214478
		8.46987533569336 -0.032642126083374
		8.72989177703857 0.165935754776001
		8.92988586425781 0.198062658309937
		9.09989738464355 0.154552459716797
		9.36986446380615 0.104357004165649
		9.52988815307617 0.163046360015869
		9.66988086700439 0.274945974349976
		9.69987869262695 0.307852506637573
		10.199896812439 0.664420604705811
		10.4698495864868 0.734002113342285
		11.1698684692383 0.708279609680176
		11.6699171066284 0.464529275894165
		13.0698537826538 -0.399214267730713
		13.9998378753662 -1.0353969335556
		14.6298503875732 -1.24101293087006
		15.469898223877 -1.41754627227783
		15.6998300552368 -1.51178133487701
		16.0399398803711 -1.55651497840881
		16.1999263763428 -1.49942266941071
		16.3998355865479 -1.43487083911896
		16.6698665618896 -1.44923877716064
		16.929838180542 -1.50823068618774
		17.129861831665 -1.45456612110138
		17.269847869873 -1.36618864536285
		17.429838180542 -1.22191202640533
		18.2298603057861 -0.813834309577942
		18.3998394012451 -0.648595213890076
		18.6298713684082 -0.412110328674316
		18.8399295806885 -0.212386131286621
		19.4698657989502 0.502772808074951
		19.599853515625 0.597668647766113
		19.8698539733887 0.766297817230225
		20.3699607849121 1.22486114501953
		21.3298721313477 1.91631698608398
		21.5999813079834 1.86231756210327
		22.2398796081543 1.7945864200592
		23.0698986053467 1.81169486045837
		23.229887008667 1.7332284450531
		23.2998523712158 1.66898131370544
		24.4299068450928 0.49646258354187
		25.3698806762695 -0.119713306427002
		25.6999397277832 -0.459175109863281
		26.0398941040039 -0.738878488540649
		26.5699062347412 -0.966215491294861
		26.9298343658447 -1.06441593170166
		27.13987159729 -1.05375266075134
		27.4698829650879 -0.956148386001587
		28.0999584197998 -0.623937726020813
		28.3299007415771 -0.430480003356934
		28.4998798370361 -0.254948854446411
		28.7298946380615 -0.000307798385620117
		29.039888381958 0.300183534622192
		29.4999446868896 0.760651588439941
		29.6999053955078 0.968765020370483
		29.9298686981201 1.23536968231201
		31.4999313354492 2.31834173202515
		31.8998680114746 2.41615533828735
		33.2298622131348 2.4342303276062
		33.6999320983887 2.2702693939209
		34.2698631286621 2.02870869636536
		34.6698608398438 1.80046057701111
		35.7698593139648 0.909197568893433
		36.0398559570312 0.669065237045288
		38.3998565673828 -1.54580450057983
		39.8998870849609 -2.31808471679688
		40.429874420166 -2.49460101127625
		41.1998710632324 -2.75041675567627
		41.7298545837402 -2.86441373825073
		41.829891204834 -2.89327621459961
		48.569881439209 -0.211014986038208
		49.1698760986328 0.355920076370239
		49.5298652648926 0.730149030685425
		49.8398742675781 1.02166938781738
		50.1298980712891 1.31772017478943
		50.3698692321777 1.56071615219116
		50.7298965454102 1.93256068229675
		51.0399017333984 2.22044825553894
		51.2998847961426 2.47055697441101
		59.0099182128906 4.41528987884521
		59.7698554992676 4.37272548675537
		60.2699203491211 4.42500972747803
		60.6298828125 4.37121677398682
		62.5998764038086 4.08039379119873
		63.6298675537109 3.20386075973511
		63.89990234375 2.92725515365601
		65.0698547363281 1.75970077514648
		65.1298751831055 1.72458982467651
		65.2698822021484 1.54860162734985
		65.6699142456055 1.14706325531006
		66.4998626708984 0.320404767990112
		67.0298385620117 -0.189714908599854
		68.9298706054688 -1.60487282276154
		69.6400299072266 -1.43810784816742
		70.199951171875 -1.24565732479095
		70.5398788452148 -0.980669617652893
		70.8298568725586 -0.708453416824341
		71.7998809814453 0.110515356063843
		72.0998840332031 0.385988235473633
		72.3298645019531 0.539576768875122
		72.5698699951172 0.678339242935181
		72.7998886108398 0.834963083267212
		73.9999542236328 1.15548396110535
		74.1699295043945 1.14336776733398
		74.3999176025391 1.03945446014404
		74.7398529052734 0.770499467849731
		76.2698822021484 -0.649506330490112
		76.6298828125 -0.989157199859619
		76.8998641967773 -1.09425842761993
		77.5999069213867 -1.21313273906708
		77.8998413085938 -1.30385673046112
		78.1999130249023 -1.32249820232391
		78.3998794555664 -1.25788831710815
		79.3698806762695 -0.794798254966736
		79.6998825073242 -0.827946901321411
		80.0698547363281 -0.97726833820343
		80.4298858642578 -1.15047705173492
		80.8299026489258 -1.20568192005157
		81.2999572753906 -1.14103949069977
		81.5299377441406 -1.07856893539429
		82.0698928833008 -0.899451851844788
		82.3998870849609 -0.857339859008789
		83.5998840332031 -0.139894247055054
		83.8698577880859 0.0897402763366699
		84.1298828125 0.261994361877441
		84.4698638916016 0.41967248916626
		84.8298721313477 0.745638370513916
		85.8299560546875 1.19936656951904
		86.5698547363281 1.30846452713013
		86.8298645019531 1.25926685333252
		87.6999053955078 0.90018367767334
		87.969856262207 0.679014682769775
		88.3298797607422 0.367918968200684
		89.4699020385742 -0.355003118515015
		90.5999069213867 -0.824884295463562
		90.9298400878906 -0.857969045639038
		91.1299209594727 -0.799543619155884
		91.4698486328125 -0.605255246162415
		91.6998672485352 -0.512042045593262
		92.2998809814453 -0.338062524795532
		92.7299270629883 -0.22139310836792
		93.7998580932617 -0.07381272315979
		94.0698471069336 0.0269498825073242
		94.6298828125 0.178381681442261
		94.8699111938477 0.268656492233276
		95.1698684692383 0.282078742980957
		95.4698867797852 0.292232036590576
		95.7299270629883 0.278688192367554
		96.099853515625 0.177815675735474
		96.4998397827148 0.0828537940979004
		96.9298629760742 -0.0427324771881104
		97.2298736572266 -0.0453901290893555
		98.0698852539062 -0.143759250640869
		98.4298629760742 -0.357643842697144
		99.5298690795898 -0.78607714176178
		99.769905090332 -0.788885474205017
		100.029846191406 -0.80402660369873
		100.299880981445 -0.890239715576172
		100.629875183105 -1.00387358665466
		100.899887084961 -1.00607824325562
		101.529830932617 -0.862037777900696
		101.769874572754 -0.726700901985168
		102.39990234375 -0.214740514755249
		103.229873657227 0.647187471389771
		103.469909667969 0.891509771347046
		104.129844665527 1.67575097084045
		104.399894714355 1.94449043273926
		104.969917297363 2.60863351821899
		106.029861450195 3.40999460220337
		107.36988067627 4.20123672485352
		107.729835510254 4.26215362548828
		108.029846191406 4.22672843933105
		108.399841308594 4.24262523651123
		109.499870300293 3.76708340644836
		109.899848937988 3.46678853034973
		111.569877624512 1.64071083068848
		111.829849243164 1.32887816429138
		112.069900512695 1.04960203170776
		112.529876708984 0.469233274459839
		113.099876403809 -0.24614143371582
		114.72989654541 -1.86932325363159
		114.999847412109 -2.05859875679016
		115.499885559082 -2.46576118469238
		115.899848937988 -2.71515870094299
		116.299957275391 -2.9299521446228
		116.729843139648 -3.14681768417358
		117.069885253906 -3.17227697372437
		117.299896240234 -3.18767499923706
		117.969863891602 -3.24558305740356
		118.429862976074 -3.19278907775879
		118.499870300293 -3.19957709312439
		120.529922485352 -2.30922555923462
		120.969841003418 -1.87294721603394
		121.399887084961 -1.35408508777618
		123.329895019531 0.941125392913818
		123.499877929688 1.13779139518738
		123.729873657227 1.40741777420044
		124.269889831543 1.97789168357849
		124.869857788086 2.66097569465637
		125.1298828125 2.91924452781677
		126.129844665527 3.9210410118103
		126.499893188477 4.10666656494141
		126.899871826172 4.31084728240967
		127.199882507324 4.38608169555664
		129.429870605469 4.64587545394897
		129.969863891602 4.68191862106323
		130.299835205078 4.70911502838135
		132.099884033203 3.56131076812744
		132.529861450195 3.09304165840149
		133.329864501953 2.24639987945557
		133.569854736328 1.99173450469971
		133.829895019531 1.69208431243896
		134.169845581055 1.32728052139282
		134.629867553711 0.820696830749512
		134.899948120117 0.531500577926636
		136.329986572266 -1.15932786464691
		137.169860839844 -1.73782825469971
		137.369873046875 -1.76452255249023
		137.769866943359 -1.69161891937256
		138.169891357422 -1.5626460313797
		138.699890136719 -1.21428251266479
		139.969863891602 -0.352035522460938
		140.229888916016 -0.152174234390259
		140.499877929688 0.0344295501708984
		140.699890136719 0.163456678390503
	};
\addlegendentry{MOCAP}
\addplot [semithick, darkorange25512714]
table {%
		0.0398528575897217 0.0592154264450073
		0.129944324493408 0.067277193069458
		0.369858503341675 0.123142957687378
		0.469894170761108 0.0589476823806763
		0.569851160049438 0.0260154008865356
		0.839867830276489 0.0221009254455566
		1.12990427017212 -0.011046290397644
		1.32991504669189 -0.0443589687347412
		1.42984771728516 -0.0595213174819946
		1.49988293647766 -0.0715745687484741
		1.59985733032227 0.0102641582489014
		1.8999171257019 -0.0297305583953857
		2.39991331100464 -0.011296272277832
		2.62987303733826 -0.0105017423629761
		2.69993734359741 0.00703930854797363
		2.79987573623657 -0.0270808935165405
		2.99984097480774 -0.0389467477798462
		3.22992253303528 -0.0595519542694092
		3.66988158226013 -0.0774896144866943
		4.5998649597168 -0.250324010848999
		4.76990795135498 -0.293246030807495
		4.89986991882324 -0.278955936431885
		5.09992742538452 -0.385619044303894
		5.12984466552734 -0.429980039596558
		5.16988658905029 -0.404363036155701
		5.22986602783203 -0.42287802696228
		5.29988861083984 -0.452342987060547
		5.32987117767334 -0.412564992904663
		5.42986917495728 -0.465307950973511
		6.09986591339111 -0.415544986724854
		6.12984561920166 -0.390845060348511
		6.29987049102783 -0.4634770154953
		6.39993095397949 -0.466150999069214
		6.46986293792725 -0.418195009231567
		6.5698881149292 -0.47225296497345
		6.62990283966064 -0.455508947372437
		7.06984233856201 -0.450511932373047
		7.09984970092773 -0.412205934524536
		7.12984228134155 -0.51213002204895
		7.19985294342041 -0.51492702960968
		7.26986598968506 -0.394804954528809
		7.29991912841797 -0.463989019393921
		7.33985614776611 -0.363878965377808
		7.36987400054932 -0.454586029052734
		7.39991807937622 -0.42418098449707
		7.46986532211304 -0.437319993972778
		7.52987289428711 -0.20100998878479
		7.62983655929565 -0.205621957778931
		7.6698579788208 -0.326552033424377
		7.72985887527466 -0.266293048858643
		7.82990121841431 -0.349185943603516
		8.06991577148438 -0.403203010559082
		8.12986946105957 -0.307214021682739
		8.16994094848633 -0.301470041275024
		8.22982501983643 -0.204113960266113
		8.29984188079834 -0.174113035202026
		8.3298511505127 -0.250254988670349
		8.39985656738281 -0.126801013946533
		8.46987533569336 -0.113546013832092
		8.49985694885254 0.531167030334473
		8.53999710083008 0.532660961151123
		8.59990787506104 -0.212978959083557
		8.79998779296875 0.00420916080474854
		9.22984886169434 0.158478975296021
		9.42987632751465 0.184406995773315
		9.46986865997314 0.233762979507446
		9.52988815307617 0.205919981002808
		9.69987869262695 0.27220606803894
		10.0698537826538 0.562911033630371
		10.2298450469971 0.775556087493896
		10.3298683166504 0.691730976104736
		10.3998966217041 0.827340006828308
		10.4998607635498 0.739464998245239
		10.529857635498 0.846693992614746
		10.5999212265015 0.804633975028992
		10.7998867034912 0.805209994316101
		10.8998565673828 0.553024053573608
		10.9998807907104 0.504158973693848
		11.0998582839966 0.656576991081238
		11.1698684692383 0.692852973937988
		11.4299058914185 0.698225021362305
		11.5398979187012 0.556970000267029
		11.8998603820801 0.415580034255981
		12.6998586654663 -0.184651017189026
		13.199914932251 -0.484601974487305
		13.2698926925659 -0.485818028450012
		13.3298358917236 -0.613363981246948
		13.3698902130127 -0.597452998161316
		13.4298801422119 -0.673465013504028
		13.4698486328125 -0.631051063537598
		13.5298805236816 -0.747588992118835
		13.5698432922363 -0.700285911560059
		13.5998487472534 -0.742792010307312
		13.6298599243164 -0.685328006744385
		13.6698627471924 -0.759652018547058
		13.6998777389526 -0.734821081161499
		13.969898223877 -0.980109930038452
		14.1299076080322 -1.16622996330261
		14.169885635376 -1.09247994422913
		14.1998977661133 -1.21173000335693
		14.2298536300659 -1.1598299741745
		14.2998542785645 -1.1598299741745
		14.3398628234863 -1.10021996498108
		14.3699169158936 -1.19283998012543
		14.4299087524414 -1.11898994445801
		14.4698686599731 -1.09666001796722
		14.4998912811279 -1.21964001655579
		14.5698471069336 -1.15963995456696
		14.6298503875732 -1.22247004508972
		14.6999492645264 -1.17042005062103
		14.7698440551758 -1.23527002334595
		14.9999027252197 -1.18227994441986
		15.0698690414429 -1.35891997814178
		15.1998872756958 -1.80927002429962
		15.4298391342163 -1.8372700214386
		15.469898223877 -1.85030996799469
		15.5298519134521 -1.5796799659729
		15.5698709487915 -1.55572998523712
		15.5998830795288 -1.41384994983673
		15.6298532485962 -1.60209000110626
		15.6998300552368 -1.35216999053955
		15.7998857498169 -1.50186002254486
		15.8698463439941 -1.72933995723724
		15.9299030303955 -1.94003999233246
		15.9698848724365 -1.71379995346069
		16.0399398803711 -1.92027997970581
		16.0998668670654 -2.16403007507324
		16.1999263763428 -1.87386000156403
		16.2298545837402 -1.80684995651245
		16.2998485565186 -1.92625999450684
		16.3698787689209 -1.89532995223999
		16.4298725128174 -1.64075005054474
		16.4698753356934 -1.59107995033264
		16.4998588562012 -1.63338994979858
		16.5298538208008 -1.52161002159119
		16.6698665618896 -1.66890001296997
		16.7398719787598 -1.51954996585846
		16.7998809814453 -1.54546999931335
		16.8398914337158 -1.51592004299164
		16.8999423980713 -1.73483002185822
		16.9698734283447 -1.53073000907898
		16.9998950958252 -1.68397998809814
		17.0698890686035 -1.55903995037079
		17.0998706817627 -1.67716002464294
		17.1999416351318 -1.46170997619629
		17.229887008667 -1.13630998134613
		17.269847869873 -1.11786997318268
		17.329833984375 -1.26532995700836
		17.3698291778564 -1.20942997932434
		17.3999214172363 -1.25136995315552
		17.429838180542 -1.18142998218536
		17.469877243042 -1.49492001533508
		17.5398902893066 -1.45463001728058
		17.5698299407959 -1.32474005222321
		17.6298694610596 -1.48767995834351
		17.6998653411865 -1.19225001335144
		17.8299217224121 -1.16753995418549
		17.8698768615723 -1.25858998298645
		17.8999214172363 -1.11970996856689
		17.9698734283447 -1.45586001873016
		17.999870300293 -1.07839000225067
		18.0698566436768 -1.0665899515152
		18.0999088287354 -1.44904005527496
		18.1298751831055 -1.15120005607605
		18.1698818206787 -1.38575994968414
		18.2298603057861 -1.18894994258881
		18.2698135375977 -1.21665000915527
		18.3298721313477 -0.892811059951782
		18.3698444366455 -0.931373000144958
		18.469856262207 -0.685648918151855
		18.5298919677734 -0.681681990623474
		18.569881439209 -0.588154077529907
		18.6298713684082 -0.623126029968262
		18.6699123382568 -0.440703988075256
		18.7299194335938 -0.608362913131714
		18.7998733520508 -0.537329912185669
		18.8399295806885 -0.558058977127075
		18.9298648834229 -0.449280977249146
		18.9698715209961 -0.440991044044495
		19.0399532318115 -0.313042998313904
		19.3698291778564 0.00439012050628662
		19.4298477172852 0.0228519439697266
		19.7698440551758 0.527225017547607
		19.8399085998535 0.741198062896729
		19.929859161377 0.823428988456726
		19.9998912811279 0.857282996177673
		20.0398406982422 0.981641054153442
		20.0998783111572 0.92798900604248
		20.1298522949219 0.983995914459229
		20.229907989502 0.988390922546387
		20.2998943328857 1.16242003440857
		20.3699607849121 1.09206998348236
		21.299840927124 1.63829004764557
		21.3298721313477 1.74565005302429
		21.3698863983154 1.68590998649597
		21.429874420166 1.14625000953674
		21.4698677062988 0.992157936096191
		21.5298595428467 1.86760997772217
		21.5699005126953 1.86412000656128
		21.5999813079834 1.558109998703
		21.6699066162109 1.74459004402161
		21.6999435424805 1.45181000232697
		21.7698745727539 1.70489001274109
		21.8298683166504 1.80893003940582
		21.8699188232422 1.98799002170563
		21.9299163818359 1.13722002506256
		21.9698486328125 1.13324999809265
		21.9998645782471 1.21291995048523
		22.0698509216309 1.24583995342255
		22.0999546051025 1.68531000614166
		22.1998615264893 1.41523003578186
		22.2398796081543 1.41650998592377
		22.2998847961426 1.46580004692078
		22.3699111938477 1.5443400144577
		22.4998569488525 1.47188997268677
		22.5698795318604 1.4355800151825
		22.7999496459961 1.74317002296448
		22.8299350738525 1.87714004516602
		22.8698616027832 1.79031002521515
		23.0298728942871 1.79401004314423
		23.0698986053467 1.67251002788544
		23.1298637390137 1.72390997409821
		23.1699028015137 1.64709997177124
		23.1998767852783 1.70345997810364
		23.229887008667 1.64534997940063
		23.2998523712158 1.61933994293213
		24.3698673248291 0.845206022262573
		24.4299068450928 0.696433067321777
		24.8299179077148 0.337367057800293
		24.9298515319824 0.373448967933655
		24.9998741149902 0.336596012115479
		25.0699157714844 0.141561985015869
		25.3698806762695 -0.120851039886475
		25.6999397277832 -0.425287961959839
		25.7999858856201 -0.449619054794312
		25.8998680114746 -0.496657013893127
		25.9298553466797 -0.539479970932007
		26.3698711395264 -0.878522992134094
		26.3998851776123 -1.00872004032135
		26.429838180542 -0.907245993614197
		26.4998836517334 -1.02748000621796
		26.5699062347412 -1.06136000156403
		26.6698818206787 -0.991307020187378
		26.7699317932129 -0.98633599281311
		26.9298343658447 -0.963837027549744
		27.4698829650879 -0.988306999206543
		27.4999294281006 -1.05735003948212
		27.569881439209 -1.04198002815247
		27.8399200439453 -0.799659967422485
		27.9298229217529 -0.625146985054016
		27.9698657989502 -0.81151008605957
		27.9999027252197 -0.747093915939331
		28.0698757171631 -0.764742970466614
		28.1998901367188 -0.594210028648376
		28.239917755127 -0.621115922927856
		28.369873046875 -0.45720100402832
		28.4698791503906 -0.466819047927856
		28.529899597168 -0.402521014213562
		28.569845199585 -0.379724025726318
		28.629861831665 -0.294999957084656
		28.8998947143555 -0.0578633546829224
		29.039888381958 0.0489790439605713
		29.1698608398438 0.213225960731506
		29.2999324798584 0.463366985321045
		29.4298725128174 0.564028024673462
		29.4999446868896 0.715098023414612
		29.5398597717285 0.697772979736328
		29.5998783111572 0.621039986610413
		29.7698764801025 0.774721026420593
		29.8999252319336 0.842119932174683
		29.9298686981201 0.806650996208191
		31.3698749542236 1.5168000459671
		31.4299430847168 1.52831995487213
		31.4698810577393 1.73618996143341
		31.4999313354492 1.58332002162933
		31.5298862457275 1.98032999038696
		31.5998840332031 1.81313002109528
		31.6298828125 1.95443999767303
		31.6698760986328 1.74783003330231
		31.7299213409424 1.80464994907379
		31.7998847961426 1.61638998985291
		31.8298835754395 1.96616995334625
		31.8698673248291 1.96157002449036
		31.8998680114746 1.53490996360779
		31.9999332427979 1.55088996887207
		32.0698547363281 2.25991010665894
		32.1699104309082 2.20840001106262
		32.5698547363281 2.30792999267578
		32.5999298095703 2.02884006500244
		32.6298599243164 2.29751992225647
		32.8699264526367 1.51358997821808
		32.9698791503906 1.68637001514435
		32.999885559082 1.62095999717712
		33.0699310302734 1.98002004623413
		33.1298789978027 1.94892001152039
		33.1698913574219 2.04928994178772
		33.2298622131348 1.83989000320435
		33.2999649047852 1.75457000732422
		33.3298721313477 1.82795000076294
		33.3698654174805 1.61000001430511
		33.4299011230469 1.54982995986938
		33.499870300293 1.55489003658295
		33.5298881530762 1.66937005519867
		33.5699005126953 1.51687002182007
		33.6699028015137 1.9059499502182
		33.7698745727539 1.87609004974365
		33.8000450134277 1.99995005130768
		33.8298797607422 1.87032997608185
		33.8698921203613 1.9590300321579
		33.89990234375 1.8704400062561
		33.9999198913574 1.94730997085571
		34.1298637390137 1.92338001728058
		34.1699180603027 2.00207996368408
		34.2298545837402 1.88131999969482
		34.2999000549316 1.83361005783081
		34.3399391174316 1.848140001297
		34.3998794555664 1.98931002616882
		34.4998817443848 1.80677998065948
		34.5400466918945 1.87785995006561
		34.5699119567871 1.84526002407074
		34.6698608398438 1.89225995540619
		34.7698974609375 1.73950004577637
		34.799919128418 1.84394001960754
		34.8298492431641 1.74470996856689
		34.8998680114746 1.6695100069046
		34.9399681091309 1.7630900144577
		34.9699440002441 1.65322995185852
		34.999870300293 1.71613001823425
		35.0698928833008 1.67333996295929
		35.3298568725586 1.26803004741669
		35.3999214172363 1.15961003303528
		35.569896697998 1.12065005302429
		35.6298980712891 1.10818004608154
		35.6698684692383 1.04008996486664
		35.7298278808594 1.07934999465942
		35.8298721313477 1.00449001789093
		35.8698654174805 1.0543600320816
		35.9998931884766 0.837419033050537
		36.0398559570312 0.875560998916626
		36.3298873901367 0.539282083511353
		36.4698677062988 0.441797018051147
		36.4999046325684 0.36197304725647
		36.5698738098145 0.335911989212036
		36.9298629760742 -0.0278452634811401
		36.9998550415039 -0.118550062179565
		37.2298469543457 -0.351541996002197
		37.2699203491211 -0.35761296749115
		37.3298416137695 -0.419496059417725
		37.4298629760742 -0.50574803352356
		37.5398635864258 -0.596006989479065
		37.729850769043 -0.758903026580811
		37.7698669433594 -0.759760975837708
		37.8698921203613 -0.732409954071045
		37.8999176025391 -0.832607984542847
		37.9998931884766 -0.88642692565918
		38.0298767089844 -0.851321935653687
		38.169864654541 -1.08529996871948
		38.3698272705078 -1.22028994560242
		38.3998565673828 -1.125
		38.4698486328125 -1.16123998165131
		38.5298500061035 -1.30578005313873
		38.5698509216309 -1.22116994857788
		38.6298980712891 -1.36159002780914
		38.7000160217285 -1.4634200334549
		38.8298873901367 -1.57920002937317
		38.8698539733887 -1.82938003540039
		38.9698600769043 -1.66185998916626
		39.0298500061035 -1.71468997001648
		39.0998764038086 -1.74539995193481
		39.2299194335938 -1.5442099571228
		39.299877166748 -1.54793000221252
		39.3298568725586 -1.64203000068665
		39.4298286437988 -1.62917995452881
		39.5000152587891 -1.75522005558014
		39.5698890686035 -1.85111999511719
		39.6698608398438 -2.1039400100708
		39.7998809814453 -1.98441004753113
		39.9998893737793 -1.96415996551514
		40.0999145507812 -2.09538006782532
		40.1298561096191 -2.12819004058838
		40.169864654541 -2.09601998329163
		40.1998710632324 -2.15146994590759
		40.2698745727539 -2.34395003318787
		40.2999572753906 -2.40563011169434
		40.3698616027832 -2.25414991378784
		40.3998641967773 -2.28764009475708
		40.429874420166 -2.24331998825073
		40.4999084472656 -2.06367993354797
		40.5298805236816 -2.25851011276245
		40.5698776245117 -2.09769010543823
		40.6298751831055 -2.2192599773407
		40.6698455810547 -2.23769998550415
		40.7298469543457 -2.32788991928101
		40.7999229431152 -2.46221995353699
		40.8998756408691 -2.49626994132996
		40.9698600769043 -2.46762990951538
		41.0999603271484 -2.39854001998901
		41.1298828125 -2.51816010475159
		41.2998924255371 -2.49415993690491
		41.3699035644531 -2.63002991676331
		41.3998908996582 -2.51740002632141
		41.4698829650879 -2.62892007827759
		41.7998886108398 -2.65158009529114
		41.829891204834 -2.72708010673523
		48.569881439209 -0.39618992805481
		49.039867401123 0.0302376747131348
		49.1398811340332 0.176506996154785
		49.2998847961426 0.255622982978821
		49.8999061584473 0.817247986793518
		49.9998893737793 0.979242086410522
		50.1698684692383 1.1468700170517
		50.2998847961426 1.17326998710632
		50.4298782348633 1.39717996120453
		50.469841003418 1.40499997138977
		50.5400085449219 1.49804997444153
		50.5998573303223 1.52048003673553
		50.6298446655273 1.57799994945526
		50.6698837280273 1.55462002754211
		50.6998634338379 1.68201994895935
		50.7298965454102 1.61268997192383
		50.7698707580566 1.61898005008698
		50.8298873901367 1.75734996795654
		50.9399719238281 1.85257995128632
		50.9699287414551 1.90515995025635
		51.0698890686035 1.9811999797821
		51.2998847961426 1.9200199842453
		59.0099182128906 3.03590989112854
		59.0999336242676 3.24218010902405
		59.1398658752441 3.02583003044128
		59.1698760986328 3.31052994728088
		59.2698631286621 3.30307006835938
		59.3299140930176 2.99573993682861
		59.3998565673828 3.03659009933472
		59.4698829650879 2.83681988716125
		59.4999504089355 3.35359001159668
		59.529857635498 3.00367999076843
		59.6298904418945 3.36637997627258
		59.8998756408691 3.22642993927002
		59.9298667907715 3.96853995323181
		59.9998512268066 3.23345994949341
		60.0698432922363 3.94775009155273
		60.1298675537109 3.80205011367798
		60.2699203491211 3.79412007331848
		60.569881439209 3.90100002288818
		60.6298828125 3.87615990638733
		63.3698539733887 2.9285900592804
		63.6999473571777 2.67524003982544
		63.7698783874512 2.68046998977661
		63.8699417114258 2.53058004379272
		63.9998512268066 2.44301009178162
		64.0699081420898 2.43613004684448
		64.1698913574219 2.32553005218506
		64.3698959350586 2.21336007118225
		64.4699325561523 2.20180988311768
		64.5299072265625 2.06065011024475
		64.5698699951172 2.08213996887207
		64.6298522949219 2.04220008850098
		64.6998901367188 1.9608199596405
		64.7699356079102 1.86047005653381
		64.7998809814453 1.88565003871918
		64.8698501586914 1.76810002326965
		64.9098815917969 1.73689997196198
		65.0298919677734 1.70694005489349
		65.0698547363281 1.58766996860504
		65.9998397827148 0.847195982933044
		66.0998764038086 0.683502912521362
		66.1998672485352 0.659241914749146
		66.2998504638672 0.547677993774414
		66.6698684692383 0.26840603351593
		66.6998901367188 0.221284031867981
		67.0298385620117 -0.0334596633911133
		68.9298706054688 -1.25379002094269
		69.329833984375 -1.33740997314453
		69.3698883056641 -1.29328000545502
		69.3998870849609 -1.34809005260468
		69.4699096679688 -1.28912997245789
		69.6000213623047 -1.33466005325317
		69.6698379516602 -1.25722002983093
		69.8698577880859 -1.24057996273041
		69.9298858642578 -1.14986002445221
		69.9999237060547 -1.1160900592804
		70.0999374389648 -1.09364998340607
		70.1698913574219 -0.985445976257324
		70.7998275756836 -0.68815803527832
		70.969856262207 -0.496134996414185
		71.0698623657227 -0.455417037010193
		71.1698760986328 -0.402277946472168
		71.2298965454102 -0.341968059539795
		71.499870300293 -0.196845054626465
		71.6298522949219 -0.0756815671920776
		71.8298492431641 0.084436297416687
		71.9698715209961 0.234004020690918
		72.0998840332031 0.378242969512939
		72.1698532104492 0.489197969436646
		72.1998596191406 0.388067960739136
		72.299919128418 0.457705020904541
		72.3698577880859 0.528450012207031
		72.4298629760742 0.562562942504883
		72.4998626708984 0.615889072418213
		72.5999755859375 0.656857013702393
		72.6298599243164 0.699226021766663
		72.7998886108398 0.727406978607178
		73.8998718261719 0.821460008621216
		73.9298629760742 0.877630949020386
		74.0998840332031 0.809471011161804
		74.1699295043945 0.935733079910278
		74.2699203491211 0.720917940139771
		74.2998504638672 0.792372941970825
		74.3298873901367 0.996307015419006
		74.3999176025391 0.75163197517395
		74.4299240112305 0.888404011726379
		74.499885559082 0.685330986976624
		74.5698547363281 0.653849005699158
		74.6298675537109 0.78252899646759
		74.6999206542969 0.693392992019653
		74.9298553466797 0.632957935333252
		74.9998321533203 0.657729029655457
		75.1399307250977 0.594665050506592
		75.2298278808594 0.431053042411804
		75.3698883056641 0.221464991569519
		75.4698715209961 0.162862062454224
		75.5399322509766 0.0988460779190063
		76.1298828125 -0.543192028999329
		76.1698989868164 -0.503059029579163
		76.229850769043 -0.563732028007507
		76.2698822021484 -0.524281978607178
		76.5698699951172 -0.843306064605713
		76.6298828125 -0.78259801864624
		76.7299957275391 -0.91563606262207
		76.8400268554688 -0.945742011070251
		76.8998641967773 -0.991441011428833
		77.0398635864258 -1.07264995574951
		77.0698776245117 -1.11809003353119
		77.0999374389648 -1.24312996864319
		77.1698837280273 -1.08846998214722
		77.2298431396484 -1.11478996276855
		77.2698669433594 -1.12247002124786
		77.3298873901367 -1.04384994506836
		77.3698654174805 -0.993597030639648
		77.4298400878906 -1.02350997924805
		77.6298980712891 -1.05366003513336
		77.6999435424805 -1.01218998432159
		77.8298721313477 -0.990589022636414
		77.8998413085938 -1.30770003795624
		77.9698791503906 -1.42475998401642
		78.0298919677734 -1.25076997280121
		78.0698852539062 -1.28975999355316
		78.1298522949219 -1.41958999633789
		78.1999130249023 -1.18962001800537
		78.2998504638672 -1.18891000747681
		78.3298492431641 -1.11828005313873
		78.3699035644531 -1.14944005012512
		78.3998794555664 -1.11586999893188
		78.4298477172852 -1.23300004005432
		78.4998550415039 -1.1158299446106
		78.5998687744141 -1.10538005828857
		78.6698913574219 -1.04683005809784
		78.7298736572266 -1.01937997341156
		78.7998809814453 -1.02953004837036
		78.8698806762695 -0.993371963500977
		78.9298858642578 -1.01363003253937
		79.0298538208008 -0.931869983673096
		79.1998519897461 -0.773290991783142
		79.269905090332 -0.828631997108459
		79.3298950195312 -0.728848934173584
		79.3998718261719 -0.766025066375732
		79.5998992919922 -0.777349948883057
		79.6698837280273 -0.70412802696228
		79.6998825073242 -0.80231499671936
		79.7298889160156 -0.757681012153625
		79.799934387207 -0.831736087799072
		79.869873046875 -0.772439002990723
		79.8998641967773 -0.819262027740479
		79.9299163818359 -0.77305006980896
		80.1699066162109 -1.00567996501923
		80.229866027832 -0.973572969436646
		80.2998733520508 -0.992737054824829
		80.3298568725586 -0.957723021507263
		80.3999176025391 -1.02605998516083
		80.4998779296875 -0.965378046035767
		80.5698547363281 -0.941151022911072
		80.6299209594727 -0.997671008110046
		80.6998596191406 -1.03900003433228
		80.7299194335938 -1.08667004108429
		80.9998779296875 -1.02884995937347
		81.6998977661133 -1.08819997310638
		81.7298889160156 -0.972723007202148
		81.7998580932617 -1.02486002445221
		81.9298629760742 -0.956851005554199
		82.0698928833008 -0.934313058853149
		82.1298751831055 -0.956112027168274
		82.1998901367188 -0.847903966903687
		82.2699356079102 -0.8264479637146
		82.2998733520508 -0.862980008125305
		82.3699264526367 -0.86017107963562
		82.3998870849609 -0.801547050476074
		83.5998840332031 -0.0407862663269043
		83.6999359130859 0.0369201898574829
		83.8298873901367 0.122416019439697
		83.9699020385742 0.246407985687256
		84.3999328613281 0.534141063690186
		84.5298461914062 0.533384084701538
		84.5999145507812 0.592890977859497
		84.6698532104492 0.652420043945312
		84.6998596191406 0.624963998794556
		84.8298721313477 0.65733802318573
		85.6698684692383 1.04765999317169
		85.7299270629883 0.996284008026123
		85.8299560546875 0.969758033752441
		85.8698654174805 1.10783004760742
		85.9298553466797 0.963788032531738
		85.9999008178711 1.05562996864319
		86.1298751831055 1.20964002609253
		86.1698532104492 1.10987997055054
		86.2298583984375 1.17382001876831
		86.2698745727539 1.18168997764587
		86.3298492431641 1.24205005168915
		86.4298629760742 1.23089003562927
		86.4698257446289 1.08591997623444
		86.529899597168 1.31383001804352
		86.5998687744141 1.25612998008728
		86.729866027832 1.15866994857788
		86.8298645019531 1.21066999435425
		86.8698120117188 1.04720997810364
		87.0298919677734 1.00238001346588
		87.1299819946289 0.921879053115845
		87.1998672485352 0.914300918579102
		87.2698669433594 0.979336977005005
		87.3998641967773 0.839314937591553
		87.4298553466797 0.667020082473755
		87.4999694824219 0.729097008705139
		87.6699523925781 0.788473010063171
		87.6999053955078 0.67577600479126
		87.769889831543 0.706205010414124
		87.8298721313477 0.57941997051239
		88.0298538208008 0.576004981994629
		88.0698699951172 0.524362087249756
		88.099853515625 0.602062940597534
		88.1699142456055 0.412590980529785
		88.2698593139648 0.346884965896606
		88.4000091552734 0.19214403629303
		88.6299209594727 0
		88.7298431396484 -0.0694208145141602
		88.8699417114258 -0.158231973648071
		88.9698944091797 -0.276190042495728
		89.0298690795898 -0.355841994285583
		89.0699005126953 -0.307750940322876
		89.1699066162109 -0.462944030761719
		89.2299041748047 -0.410191059112549
		89.3298568725586 -0.475302934646606
		89.3698654174805 -0.469251990318298
		89.4298934936523 -0.532217025756836
		89.4699020385742 -0.501461982727051
		90.3298950195312 -0.930443048477173
		90.4298629760742 -0.806365966796875
		90.4698791503906 -0.747698068618774
		90.4998626708984 -0.833199024200439
		90.5298614501953 -0.802271008491516
		90.5999069213867 -0.883058071136475
		90.6698760986328 -0.902620077133179
		90.6998825073242 -0.954422950744629
		90.7298278808594 -0.882652997970581
		90.7998886108398 -0.958755970001221
		91.0298690795898 -0.913126945495605
		91.0999374389648 -0.867208003997803
		91.1698684692383 -0.772041082382202
		91.1998443603516 -0.734562993049622
		91.2298583984375 -0.778213977813721
		91.3298950195312 -0.704527020454407
		91.4299011230469 -0.697898983955383
		91.6698760986328 -0.718062996864319
		91.7698593139648 -0.652832984924316
		91.8299026489258 -0.667444944381714
		91.9298553466797 -0.61114501953125
		91.969970703125 -0.612725019454956
		92.0298919677734 -0.557814002037048
		92.0698471069336 -0.558295965194702
		92.0998611450195 -0.487031936645508
		92.2298812866211 -0.516730070114136
		92.2998809814453 -0.521415948867798
		92.6298599243164 -0.523797035217285
		92.6999282836914 -0.456109046936035
		92.7299270629883 -0.519432067871094
		92.7998962402344 -0.453441023826599
		92.9298477172852 -0.490421056747437
		92.9698486328125 -0.52513599395752
		93.0299072265625 -0.434855937957764
		93.0698623657227 -0.444923043251038
		93.0998687744141 -0.386168956756592
		93.8698806762695 -0.237097978591919
		93.8999481201172 -0.261093974113464
		93.9298629760742 -0.231055021286011
		94.0298690795898 -0.289903998374939
		94.0698471069336 -0.204781055450439
		94.1698913574219 -0.324138998985291
		94.2299270629883 -0.15785801410675
		94.3698501586914 -0.175467014312744
		94.4298706054688 -0.111103057861328
		94.6298828125 0.026508092880249
		94.6998901367188 -0.0301865339279175
		94.7698745727539 0.0838172435760498
		94.8699111938477 0.0712747573852539
		94.9998779296875 0.185857057571411
		95.0998916625977 0.179033041000366
		95.2299652099609 0.227522015571594
		95.2698593139648 0.214329957962036
		95.3298873901367 0.26195502281189
		95.3698883056641 0.297814965248108
		95.4299011230469 0.243605017662048
		95.7299270629883 0.222457051277161
		95.7998657226562 0.297044038772583
		95.9298706054688 0.322488069534302
		96.0298614501953 0.299170017242432
		96.1698684692383 0.249812960624695
		96.4298629760742 0.213021039962769
		96.469856262207 0.258836984634399
		96.4998397827148 0.20247495174408
		96.8298797607422 0.183570027351379
		96.9298629760742 0.276391983032227
		97.1698913574219 0.196635961532593
		97.2298736572266 0.228778958320618
		98.3998947143555 -0.284381031990051
		98.4698791503906 -0.431478023529053
		98.5699157714844 -0.442842960357666
		99.0299453735352 -0.638195991516113
		99.0998840332031 -0.706865072250366
		99.1698684692383 -0.644829988479614
		99.1998596191406 -0.705211997032166
		99.229866027832 -0.649798989295959
		99.2999114990234 -0.716508984565735
		99.3999328613281 -0.76330304145813
		99.4298629760742 -0.693126916885376
		99.4999542236328 -0.716795921325684
		99.5698699951172 -0.777464985847473
		99.6298599243164 -0.742368936538696
		99.6698837280273 -0.729496955871582
		99.7299194335938 -0.799785971641541
		99.8298950195312 -0.78348708152771
		99.8698959350586 -0.798021078109741
		99.8998947143555 -0.732047080993652
		99.9698944091797 -0.774003982543945
		100.269882202148 -0.740591049194336
		100.329856872559 -0.79204797744751
		100.369842529297 -0.741940021514893
		100.429840087891 -0.870408058166504
		100.499938964844 -0.914313077926636
		100.569847106934 -0.988399028778076
		100.629875183105 -0.961995005607605
		100.82984161377 -0.99070405960083
		100.929870605469 -1.02759003639221
		100.999885559082 -1.01612997055054
		101.069862365723 -1.0594300031662
		101.1298828125 -0.94528603553772
		101.169876098633 -1.02862000465393
		101.199897766113 -0.84002697467804
		101.229858398438 -1.0299299955368
		101.269912719727 -0.849792003631592
		101.299903869629 -0.905869960784912
		101.329917907715 -0.800251007080078
		101.429847717285 -0.945348978042603
		101.499885559082 -0.857167959213257
		101.529830932617 -0.887404918670654
		101.569877624512 -0.870693922042847
		101.599937438965 -0.933713912963867
		101.629844665527 -0.849257946014404
		101.699913024902 -0.898016929626465
		102.069854736328 -0.686293005943298
		102.099853515625 -0.713216066360474
		102.169876098633 -0.592507004737854
		102.229911804199 -0.537889957427979
		102.269874572754 -0.568099975585938
		102.299865722656 -0.532240986824036
		102.329849243164 -0.665418982505798
		102.369857788086 -0.644954919815063
		102.469856262207 -0.444301962852478
		102.629898071289 -0.263965010643005
		103.299865722656 0.519603967666626
		103.399871826172 0.765007972717285
		103.469909667969 0.738250017166138
		103.499931335449 0.857406973838806
		103.529914855957 0.737328052520752
		103.629867553711 0.767813920974731
		103.669883728027 0.756096005439758
		103.699928283691 0.610499024391174
		103.799964904785 0.792753934860229
		103.829895019531 1.22320997714996
		103.869873046875 1.19722998142242
		103.899940490723 0.999613046646118
		103.969856262207 1.4112800359726
		103.999877929688 1.16749000549316
		104.029846191406 1.38707995414734
		104.069854736328 1.18470001220703
		104.099868774414 1.44930005073547
		104.129844665527 1.37489998340607
		104.199821472168 1.42574000358582
		104.229866027832 1.71188998222351
		104.299858093262 1.57301998138428
		104.329833984375 1.68563997745514
		104.369926452637 1.53541004657745
		104.499839782715 1.87451004981995
		104.529838562012 1.84700000286102
		104.569847106934 1.86812996864319
		104.599891662598 1.56105995178223
		104.669868469238 2.00108003616333
		104.699859619141 1.92492997646332
		104.729858398438 1.95600998401642
		104.769905090332 1.92630004882812
		104.829895019531 2.06480002403259
		104.869911193848 2.05358004570007
		104.929885864258 1.51893997192383
		104.969917297363 1.86488997936249
		105.829895019531 2.25846004486084
		105.869873046875 2.21317005157471
		105.929893493652 1.98283004760742
		105.999961853027 2.30417990684509
		106.999893188477 2.88599991798401
		107.02995300293 3.20996999740601
		107.099876403809 2.81851005554199
		107.129890441895 2.87807011604309
		107.169952392578 3.07455992698669
		107.199882507324 2.9025399684906
		107.229919433594 3.04752993583679
		107.36988067627 3.02361011505127
		107.399887084961 2.84664011001587
		107.629943847656 3.29425001144409
		107.69995880127 4.08023977279663
		107.729835510254 3.26575994491577
		107.929908752441 3.19580006599426
		107.969879150391 3.2278299331665
		107.999923706055 3.1274299621582
		108.029846191406 3.88652992248535
		108.269874572754 3.12726998329163
		108.399841308594 3.82701992988586
		109.699851989746 3.03266000747681
		109.769905090332 3.08420991897583
		109.929870605469 2.91381001472473
		109.999855041504 2.87992000579834
		110.06990814209 2.76411008834839
		110.169868469238 2.69202995300293
		110.26993560791 2.68787002563477
		110.369873046875 2.50502991676331
		110.399932861328 2.54541993141174
		110.469924926758 2.49548006057739
		110.569862365723 2.45863008499146
		110.629844665527 2.3358199596405
		110.699920654297 2.27928996086121
		110.769920349121 2.19798994064331
		110.96989440918 2.1386399269104
		111.129867553711 1.94395005702972
		111.32991027832 1.77381002902985
		111.399864196777 1.69947004318237
		111.429840087891 1.58022999763489
		111.799850463867 1.33091998100281
		111.999862670898 1.06326997280121
		112.199905395508 0.872524976730347
		112.299873352051 0.809314966201782
		112.529876708984 0.534232020378113
		112.669868469238 0.416206955909729
		112.799850463867 0.268265962600708
		113.099876403809 -0.140663027763367
		114.699897766113 -1.52056002616882
		114.869895935059 -1.87995004653931
		114.899925231934 -1.84905004501343
		115.129913330078 -1.86953997612
		115.199928283691 -2.02767992019653
		115.299812316895 -2.1875
		115.469863891602 -2.23403000831604
		115.499885559082 -2.42233991622925
		115.629905700684 -2.34259009361267
		115.669830322266 -2.54416990280151
		115.729888916016 -2.49358010292053
		115.769866943359 -2.49986004829407
		115.829849243164 -2.56374001502991
		115.86986541748 -2.60338997840881
		115.929878234863 -2.48934006690979
		115.999977111816 -2.73131990432739
		116.099853515625 -2.90648007392883
		116.129859924316 -2.87370991706848
		116.229873657227 -3.06276988983154
		116.299957275391 -3.04253005981445
		116.399948120117 -3.1423499584198
		116.499877929688 -2.96845006942749
		116.569931030273 -3.02180004119873
		116.629898071289 -3.23449993133545
		116.669921875 -3.36698007583618
		116.699882507324 -3.33121991157532
		116.729843139648 -3.43196988105774
		116.769882202148 -3.39345002174377
		116.899948120117 -3.04678988456726
		116.969879150391 -3.27191996574402
		117.069885253906 -3.06410002708435
		117.129859924316 -3.08871006965637
		117.199913024902 -2.84340000152588
		117.269897460938 -2.90081000328064
		117.399909973145 -2.933109998703
		117.69994354248 -3.05333995819092
		117.769866943359 -3.01027011871338
		117.869888305664 -3.08247995376587
		117.899887084961 -2.92248010635376
		117.929878234863 -3.09532999992371
		117.999900817871 -3.04891991615295
		118.02986907959 -3.28677010536194
		118.069885253906 -3.29393005371094
		118.129905700684 -3.15367007255554
		118.169906616211 -3.26891994476318
		118.199920654297 -3.497309923172
		118.229866027832 -3.32868003845215
		118.269874572754 -3.34179997444153
		118.329872131348 -3.299959897995
		118.399833679199 -3.46882009506226
		118.469879150391 -3.4743800163269
		118.499870300293 -3.58817005157471
		120.529922485352 -2.17712998390198
		120.669898986816 -2.16687989234924
		120.729881286621 -2.02418994903564
		120.769897460938 -2.04317998886108
		120.799865722656 -2.29607009887695
		120.829864501953 -1.92999994754791
		120.86986541748 -2.21553993225098
		120.969841003418 -1.73509001731873
		121.129867553711 -1.59232997894287
		121.299942016602 -1.9729700088501
		121.399887084961 -1.42026996612549
		123.469886779785 0.976727962493896
		123.569877624512 1.16629004478455
		123.699890136719 1.21194005012512
		123.729873657227 1.27132999897003
		123.869850158691 1.33490002155304
		123.899932861328 1.47315001487732
		123.929847717285 1.37695002555847
		123.969856262207 1.60979998111725
		124.069862365723 1.60555994510651
		124.129867553711 1.55694997310638
		124.199974060059 1.77043998241425
		124.499954223633 2.02499008178711
		124.569854736328 2.12045001983643
		124.59986114502 2.07961010932922
		124.869857788086 2.18569993972778
		124.929893493652 2.21633005142212
		125.029876708984 2.24202990531921
		125.069862365723 2.20309996604919
		125.1298828125 2.25720000267029
		125.199836730957 2.26814007759094
		125.369873046875 2.22836995124817
		125.469879150391 2.43163990974426
		125.499839782715 2.72808003425598
		125.599884033203 2.93272995948792
		125.799835205078 2.58235001564026
		125.829864501953 2.71484994888306
		126.169868469238 2.54706001281738
		126.229858398438 2.63884997367859
		126.299896240234 2.47270011901855
		126.329864501953 2.95420002937317
		126.369857788086 2.70581007003784
		126.399841308594 3.00595998764038
		126.469886779785 2.83593988418579
		126.569900512695 2.87831997871399
		126.629890441895 3.05036997795105
		126.699859619141 3.21062994003296
		126.72989654541 2.84318995475769
		126.799873352051 2.90042996406555
		126.829879760742 2.95393991470337
		126.899871826172 2.89664006233215
		127.199882507324 4.23333978652954
		129.029876708984 3.29760003089905
		129.1298828125 3.30746006965637
		129.199890136719 4.14500999450684
		129.429870605469 3.30338001251221
		129.829864501953 3.23150992393494
		129.899887084961 3.98834991455078
		129.969863891602 3.92058992385864
		130.169860839844 3.86209011077881
		130.19987487793 3.08420991897583
		130.299835205078 3.0619900226593
		131.999923706055 3.03603005409241
		132.099884033203 2.91580009460449
		132.169860839844 2.87397003173828
		132.19987487793 2.80992007255554
		132.229858398438 2.88118004798889
		132.299850463867 2.7464599609375
		132.399948120117 2.69187998771667
		132.499923706055 2.6569299697876
		132.529861450195 2.51879000663757
		132.599884033203 2.48076009750366
		132.699905395508 2.48196005821228
		132.729888916016 2.40823006629944
		132.769882202148 2.43893003463745
		132.829849243164 2.35477995872498
		132.899887084961 2.29923009872437
		132.929840087891 2.3472900390625
		133.029830932617 2.26678991317749
		133.129852294922 2.19381999969482
		133.269882202148 2.18150997161865
		133.369873046875 2.03314995765686
		133.399856567383 2.06153011322021
		133.469879150391 1.97101998329163
		133.569854736328 1.86338996887207
		133.599853515625 1.91228997707367
		133.699905395508 1.74339997768402
		133.769866943359 1.71138000488281
		133.869903564453 1.67866003513336
		133.929901123047 1.51125001907349
		133.969879150391 1.51125001907349
		134.029861450195 1.39347004890442
		134.099822998047 1.35873997211456
		134.169845581055 1.25994002819061
		134.199890136719 1.32374000549316
		134.299819946289 1.15989995002747
		134.369903564453 1.17163002490997
		134.629867553711 0.819634914398193
		134.669876098633 0.819634914398193
		134.729873657227 0.660537004470825
		134.769866943359 0.623409032821655
		134.799850463867 0.660537004470825
		134.869873046875 0.567813992500305
		134.99983215332 0.412631988525391
		135.099868774414 0.319015026092529
		135.169891357422 0.284994959831238
		135.229858398438 0.193765997886658
		135.269836425781 0.15516197681427
		135.369842529297 -0.0668418407440186
		135.39990234375 0.0687808990478516
		135.469909667969 -0.111376047134399
		135.52995300293 -0.18655800819397
		135.599868774414 -0.347424030303955
		135.699890136719 -0.386909008026123
		135.76985168457 -0.487298011779785
		135.929885864258 -0.601398944854736
		135.999923706055 -0.947628974914551
		136.329986572266 -1.08641004562378
		136.400146484375 -0.996937990188599
		136.469863891602 -1.13338005542755
		136.669845581055 -1.24396002292633
		136.729873657227 -1.52107000350952
		137.1298828125 -1.5738400220871
		137.169860839844 -1.62799000740051
		137.229873657227 -1.59902000427246
		137.299850463867 -1.78288996219635
		137.369873046875 -1.69047999382019
		137.399856567383 -1.56326997280121
		137.469879150391 -1.80315005779266
		137.529861450195 -1.68654000759125
		137.59992980957 -1.81175005435944
		137.729843139648 -1.78719997406006
		137.829864501953 -1.60892999172211
		137.869857788086 -1.69896996021271
		137.92985534668 -1.43877995014191
		138.099945068359 -1.43081998825073
		138.129837036133 -1.36915004253387
		138.169891357422 -1.43900001049042
		138.229919433594 -1.40127003192902
		138.299865722656 -1.43804001808167
		138.369857788086 -1.41663002967834
		138.429885864258 -1.30418002605438
		138.599884033203 -1.19377994537354
		138.629898071289 -1.26969003677368
		138.669845581055 -1.23395001888275
		138.729888916016 -0.953809022903442
		138.799896240234 -0.986747026443481
		138.969848632812 -0.865082979202271
		139.1298828125 -0.789965987205505
		139.169937133789 -0.8126540184021
		139.19987487793 -0.734799981117249
		139.229858398438 -0.829218983650208
		139.299850463867 -0.677389025688171
		139.329895019531 -0.707437038421631
		139.429885864258 -0.641487002372742
		139.499877929688 -0.587643027305603
		139.529891967773 -0.632368087768555
		139.729888916016 -0.41627299785614
		139.769866943359 -0.438573956489563
		139.799835205078 -0.382895946502686
		139.829879760742 -0.430696964263916
		139.899856567383 -0.347409963607788
		140.129837036133 -0.253911972045898
		140.199905395508 -0.219002962112427
		140.669845581055 -0.0194379091262817
		140.699890136719 0.00636637210845947
	};
\addlegendentry{Prediction}


==> tikz/vis_localize/vis_loc_test3.tex <==
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.127345561981201 0.33639669418335
		-0.127067089080811 0.336051464080811
		-0.126857280731201 0.335971355438232
		-0.126943588256836 0.335843324661255
		-0.126674652099609 0.336117029190063
		-0.126482009887695 0.336321592330933
		-0.1263427734375 0.336436986923218
		-0.126259803771973 0.33642053604126
		-0.126501083374023 0.336380481719971
		-0.126931667327881 0.336288452148438
		-0.127213478088379 0.336193799972534
		-0.127379417419434 0.336082458496094
		-0.127428531646729 0.336060523986816
		-0.127238750457764 0.33616304397583
		-0.127137660980225 0.336286783218384
		-0.127051830291748 0.336385726928711
		-0.127231597900391 0.336395025253296
		-0.127309322357178 0.336313009262085
		-0.127755641937256 0.336009740829468
		-0.127657890319824 0.335921764373779
		-0.128323078155518 0.335436820983887
		-0.128292560577393 0.335200548171997
		-0.128357887268066 0.335154294967651
		-0.128033638000488 0.335654020309448
		-0.128103733062744 0.335783958435059
		-0.128036975860596 0.336326837539673
		-0.128242492675781 0.336884021759033
		-0.128693580627441 0.337846279144287
		-0.130049705505371 0.338828802108765
		-0.132980823516846 0.338552474975586
		-0.135319709777832 0.338804721832275
		-0.138466358184814 0.337401866912842
		-0.140285491943359 0.337421178817749
		-0.144243240356445 0.3355712890625
		-0.144834041595459 0.334638833999634
		-0.142208576202393 0.334274768829346
		-0.139250755310059 0.333518981933594
		-0.137133121490479 0.333959579467773
		-0.136801719665527 0.334259986877441
		-0.137418746948242 0.334198474884033
		-0.138842105865479 0.333635807037354
		-0.139020919799805 0.333207368850708
		-0.138625621795654 0.332631826400757
		-0.13801097869873 0.3323655128479
		-0.137037754058838 0.33245849609375
		-0.136043548583984 0.332458019256592
		-0.135749340057373 0.33210825920105
		-0.135772228240967 0.331512212753296
		-0.135285377502441 0.331185579299927
		-0.133986949920654 0.333990573883057
		-0.13373851776123 0.334224224090576
		-0.133357524871826 0.334911108016968
		-0.13373851776123 0.334845066070557
		-0.133326053619385 0.335404396057129
		-0.131371974945068 0.33700966835022
		-0.130611419677734 0.337652683258057
		-0.130269527435303 0.337921142578125
		-0.127150535583496 0.336419582366943
		-0.142560482025146 0.336381912231445
		-0.130171775817871 0.337992191314697
		-0.132570743560791 0.33335018157959
		-0.284072399139404 0.155272960662842
		-0.271154880523682 -0.0775504112243652
		-0.319582462310791 0.0191278457641602
		-0.165642738342285 -0.142706990242004
		-0.163980960845947 -0.125649571418762
		-0.013519287109375 -0.220731616020203
		-0.0941438674926758 -0.244161605834961
		0.0924921035766602 -0.21928858757019
		0.0640397071838379 -0.30336582660675
		-0.130343437194824 0.337821006774902
		-0.130621910095215 0.337231636047363
		-0.13059663772583 0.336978435516357
		-0.130386352539062 0.336621761322021
		-0.13006591796875 0.336508512496948
		-0.12996244430542 0.336529731750488
		-0.129973411560059 0.336352348327637
		-0.13001823425293 0.336191177368164
		-0.129636764526367 0.336391687393188
		-0.129453659057617 0.336493492126465
		-0.129319667816162 0.336454629898071
		-0.129502773284912 0.336442947387695
		-0.12939453125 0.336419105529785
		-0.129412651062012 0.336338758468628
		-0.129447937011719 0.336318492889404
		-0.129812240600586 0.336380481719971
		-0.130048274993896 0.336620092391968
		-0.130208015441895 0.336812019348145
		-0.130391120910645 0.336901187896729
		-0.130504608154297 0.33701491355896
		-0.130611419677734 0.337713241577148
		-0.130620956420898 0.338169574737549
		-0.130695343017578 0.338706254959106
		-0.130999088287354 0.339034557342529
		-0.132501125335693 0.339397430419922
		-0.134002208709717 0.338826894760132
		-0.134543418884277 0.33806324005127
		-0.134791851043701 0.337135553359985
		-0.135255813598633 0.335719108581543
		-0.135168075561523 0.334786415100098
		-0.134685039520264 0.333946943283081
		-0.133959293365479 0.333630800247192
		-0.133503913879395 0.333352565765381
		-0.13328742980957 0.333033323287964
		-0.132849216461182 0.332859039306641
		-0.132727146148682 0.332768678665161
		-0.13271427154541 0.332833766937256
		-0.132719993591309 0.332961559295654
		-0.132607936859131 0.333128929138184
		-0.132829666137695 0.333293914794922
		-0.133346080780029 0.332920789718628
		-0.134922504425049 0.331595182418823
		-0.138310432434082 0.328665256500244
		-0.144300937652588 0.323947668075562
		-0.153729915618896 0.316816329956055
		-0.165335178375244 0.308836460113525
		-0.18049955368042 0.299356460571289
		-0.194860458374023 0.288275241851807
		-0.209865570068359 0.276289463043213
		-0.224143028259277 0.26317310333252
		-0.237681865692139 0.249949216842651
		-0.250017642974854 0.235231637954712
		-0.259373188018799 0.220257759094238
		-0.267834186553955 0.206827878952026
		-0.27379322052002 0.190223455429077
		-0.280874729156494 0.174499034881592
		-0.287419319152832 0.137189626693726
		-0.288110733032227 0.119146585464478
		-0.286662101745605 0.101033449172974
		-0.285177707672119 0.0823261737823486
		-0.281112670898438 0.0637161731719971
		-0.276029109954834 0.044203519821167
		-0.272835254669189 0.0257899761199951
		-0.269052982330322 0.00666356086730957
		-0.263589382171631 -0.011359691619873
		-0.256765365600586 -0.028867244720459
		-0.249118328094482 -0.0451648235321045
		-0.242172718048096 -0.0621557235717773
		-0.238335609436035 -0.0789104700088501
		-0.239926815032959 -0.090335488319397
		-0.243424415588379 -0.094348669052124
		-0.24898624420166 -0.0919655561447144
		-0.257389068603516 -0.086189866065979
		-0.289443016052246 -0.0679054260253906
		-0.330009937286377 -0.0535423755645752
		-0.351505279541016 -0.0458657741546631
		-0.37312650680542 -0.0388782024383545
		-0.391369819641113 -0.031400203704834
		-0.404147624969482 -0.0229568481445312
		-0.412797927856445 -0.0151066780090332
		-0.419476985931396 -0.00657343864440918
		-0.423289775848389 0.00167560577392578
		-0.424114227294922 0.00839686393737793
		-0.422009944915771 0.0155158042907715
		-0.415642738342285 0.0215318202972412
		-0.404873371124268 0.0266897678375244
		-0.392663955688477 0.0302777290344238
		-0.378329277038574 0.0310306549072266
		-0.362000465393066 0.0285007953643799
		-0.34178638458252 0.0248384475708008
		-0.295982837677002 0.0126585960388184
		-0.273382186889648 0.0057227611541748
		-0.254976272583008 -0.000291347503662109
		-0.23919677734375 -0.00809168815612793
		-0.226951599121094 -0.0176470279693604
		-0.217410564422607 -0.0291993618011475
		-0.208463668823242 -0.0423965454101562
		-0.199522495269775 -0.0569124221801758
		-0.192939758300781 -0.0752726793289185
		-0.185149192810059 -0.0941650867462158
		-0.179662227630615 -0.112337470054626
		-0.172919273376465 -0.126591324806213
		-0.16869068145752 -0.137657403945923
		-0.16331148147583 -0.143073201179504
		-0.159461975097656 -0.147551774978638
		-0.154972553253174 -0.1480393409729
		-0.157015800476074 -0.146386027336121
		-0.177671909332275 -0.137000679969788
		-0.19284200668335 -0.132488608360291
		-0.210398197174072 -0.128688216209412
		-0.228511810302734 -0.125876784324646
		-0.249642848968506 -0.122074484825134
		-0.269594192504883 -0.121593475341797
		-0.283200263977051 -0.121006011962891
		-0.291861057281494 -0.120949387550354
		-0.29789924621582 -0.123217701911926
		-0.300311088562012 -0.124795079231262
		-0.295314311981201 -0.125708222389221
		-0.283912181854248 -0.12652850151062
		-0.266007423400879 -0.126245856285095
		-0.244179725646973 -0.125024318695068
		-0.220665454864502 -0.123825430870056
		-0.19743824005127 -0.121778845787048
		-0.177428245544434 -0.122844219207764
		-0.154148101806641 -0.130884408950806
		-0.144205093383789 -0.134939074516296
		-0.134428977966309 -0.141283512115479
		-0.12041711807251 -0.147732973098755
		-0.105488777160645 -0.152384996414185
		-0.0885343551635742 -0.15541934967041
		-0.0689239501953125 -0.155092716217041
		-0.0440235137939453 -0.153853297233582
		-0.0175881385803223 -0.151610612869263
		0.00612306594848633 -0.152277946472168
		0.0241775512695312 -0.156807065010071
		0.0376749038696289 -0.162075638771057
		0.0440340042114258 -0.168996095657349
		0.0435194969177246 -0.177294254302979
		0.0348596572875977 -0.187309384346008
		0.0248465538024902 -0.19659161567688
		0.00772333145141602 -0.207625508308411
		-0.0350570678710938 -0.234177947044373
		-0.0556979179382324 -0.245718240737915
		-0.0766358375549316 -0.254761338233948
		-0.096651554107666 -0.265111565589905
		-0.112179756164551 -0.273218750953674
		-0.124150276184082 -0.280424118041992
		-0.136596202850342 -0.283891320228577
		-0.143905639648438 -0.285441875457764
		-0.148105621337891 -0.284783720970154
		-0.148095607757568 -0.282817602157593
		-0.143739223480225 -0.278131365776062
		-0.138580799102783 -0.270571351051331
		-0.131194591522217 -0.264633297920227
		-0.124561309814453 -0.258047580718994
		-0.118720054626465 -0.250370144844055
		-0.110805988311768 -0.24615204334259
		-0.10306978225708 -0.244179368019104
		-0.0849523544311523 -0.240639328956604
		-0.0738344192504883 -0.236718535423279
		-0.0595850944519043 -0.230524182319641
		-0.0452413558959961 -0.221369624137878
		-0.0284314155578613 -0.213078737258911
		0.0046086311340332 -0.195339798927307
		0.0823922157287598 -0.154309988021851
		0.099827766418457 -0.148129820823669
		0.11549186706543 -0.147555232048035
		0.127522945404053 -0.149468660354614
		0.13392448425293 -0.150037884712219
		0.137029647827148 -0.151102185249329
		0.136421203613281 -0.155776381492615
		0.134178638458252 -0.161889910697937
		0.130003452301025 -0.170437455177307
		0.125154495239258 -0.180585741996765
		0.104872226715088 -0.205686807632446
		0.0831584930419922 -0.23091721534729
		0.0763993263244629 -0.241548776626587
		0.0749874114990234 -0.250195145606995
		0.0763096809387207 -0.258049130439758
		0.076683521270752 -0.267605304718018
		0.0754432678222656 -0.276083588600159
		0.0733308792114258 -0.282850980758667
		0.0684676170349121 -0.2891925573349
		0.0617537498474121 -0.293706893920898
		0.0561628341674805 -0.295415043830872
		0.0522427558898926 -0.296724438667297
		0.0496621131896973 -0.299678683280945
		0.050717830657959 -0.302342176437378
		0.0530204772949219 -0.302908658981323
		0.0563607215881348 -0.30420184135437
		0.0593900680541992 -0.306122303009033
		0.0621929168701172 -0.306800603866577
		0.0632481575012207 -0.298717856407166
		0.0646572113037109 -0.293217182159424
		0.0684065818786621 -0.287723302841187
		0.0741477012634277 -0.282844662666321
		0.089317798614502 -0.267599701881409
		0.154258251190186 -0.207270503044128
		0.188057899475098 -0.189673781394958
		0.277876377105713 -0.157894492149353
		0.271331310272217 -0.169587016105652
		0.262718200683594 -0.182254791259766
		0.23896312713623 -0.21306037902832
		0.226468086242676 -0.231433749198914
		0.215083599090576 -0.248465538024902
		0.208513259887695 -0.263208746910095
		0.202855587005615 -0.279374718666077
		0.196976661682129 -0.292702198028564
		0.190371036529541 -0.296929955482483
		0.189435005187988 -0.298970222473145
		0.195977687835693 -0.299531936645508
		0.204080581665039 -0.293481349945068
		0.211403369903564 -0.288840413093567
		0.217202663421631 -0.284569025039673
		0.222823619842529 -0.280343174934387
		0.226415634155273 -0.278469443321228
		0.228897094726562 -0.276474714279175
		0.229872226715088 -0.274652719497681
		0.230139255523682 -0.271752119064331
		0.230880737304688 -0.267615437507629
		0.232580661773682 -0.263120770454407
		0.234235763549805 -0.25724732875824
		0.236414432525635 -0.249696016311646
		0.238749027252197 -0.238720536231995
		0.240648746490479 -0.225665330886841
		0.242067813873291 -0.210521221160889
		0.247630596160889 -0.17639946937561
		0.249472141265869 -0.165167570114136
		0.251272201538086 -0.154857873916626
		0.255558490753174 -0.140889644622803
		0.257637023925781 -0.12615978717804
		0.261587619781494 -0.108753323554993
		0.266680717468262 -0.0899649858474731
		0.275506019592285 -0.0706666707992554
		0.285387516021729 -0.0525145530700684
		0.294573307037354 -0.0355722904205322
		0.30214262008667 -0.0185396671295166
		0.307894229888916 -0.00748562812805176
		0.310399532318115 -0.0055694580078125
		0.310517311096191 -0.00803828239440918
		0.306131839752197 -0.0134046077728271
		0.304028034210205 -0.020911693572998
		0.304971694946289 -0.0293946266174316
		0.332724571228027 -0.0782854557037354
		0.341250419616699 -0.0889768600463867
		0.352740287780762 -0.101634621620178
		0.363479614257812 -0.11593496799469
		0.370843410491943 -0.12634551525116
		0.373491287231445 -0.139153122901917
		0.377600193023682 -0.15196704864502
		0.37860107421875 -0.164354801177979
		0.377533912658691 -0.172898173332214
		0.377882957458496 -0.178918361663818
		0.377589702606201 -0.178051948547363
		0.376821517944336 -0.17090106010437
		0.374718189239502 -0.168509721755981
		0.37454080581665 -0.161887288093567
		0.375263690948486 -0.156908750534058
		0.374731540679932 -0.151434302330017
		0.373298168182373 -0.143836736679077
		0.3638596534729 -0.124979853630066
		0.358997821807861 -0.113800644874573
		0.35273265838623 -0.101011037826538
		0.344966411590576 -0.0886701345443726
		0.340921401977539 -0.0732778310775757
		0.333609580993652 -0.0632095336914062
		0.328624248504639 -0.0518476963043213
		0.32614803314209 -0.0395045280456543
		0.324001312255859 -0.0259950160980225
		0.323373794555664 -0.0119228363037109
		0.322394371032715 0.00493359565734863
		0.319125652313232 0.022716760635376
		0.316646099090576 0.0431790351867676
		0.314241886138916 0.0655753612518311
		0.311479568481445 0.0860886573791504
		0.304279804229736 0.105211019515991
		0.297127723693848 0.12301778793335
		0.301129341125488 0.146174669265747
		0.306344509124756 0.150805234909058
		0.312263011932373 0.150809526443481
		0.320131301879883 0.145972728729248
		0.327576160430908 0.137224197387695
		0.334969997406006 0.126255989074707
		0.345934391021729 0.115550756454468
		0.35954761505127 0.104497671127319
		0.372883796691895 0.0950582027435303
		0.403318881988525 0.0633001327514648
		0.409867286682129 0.0529162883758545
		0.416993141174316 0.0437567234039307
		0.42347526550293 0.0369217395782471
		0.428780078887939 0.0292983055114746
		0.433215618133545 0.0232694149017334
		0.438974857330322 0.0191788673400879
		0.442541599273682 0.0154011249542236
		0.446456432342529 0.0101125240325928
		0.448628902435303 0.0115163326263428
		0.450963973999023 0.0147478580474854
		0.454798221588135 0.02201247215271
		0.459031581878662 0.0279545783996582
		0.465235233306885 0.0344347953796387
		0.472632884979248 0.0409152507781982
		0.480697631835938 0.0479066371917725
		0.490830898284912 0.0555980205535889
		0.500276565551758 0.0646281242370605
		0.502219676971436 0.069892406463623
		0.507074356079102 0.0812771320343018
		0.508538722991943 0.0945429801940918
		0.511768817901611 0.114149332046509
		0.511963367462158 0.134072542190552
		0.51190185546875 0.155261754989624
		0.508926391601562 0.174934387207031
		0.496715545654297 0.216670036315918
		0.490595817565918 0.241269588470459
		0.483274459838867 0.264455080032349
		0.477270603179932 0.285759925842285
		0.472188949584961 0.305264711380005
		0.468234062194824 0.322073936462402
		0.463737010955811 0.338606595993042
		0.460882663726807 0.356423377990723
		0.459611415863037 0.374145269393921
		0.462459564208984 0.386286020278931
		0.464548110961914 0.393747329711914
		0.46444034576416 0.398537635803223
		0.462847709655762 0.398977279663086
		0.458470344543457 0.397181034088135
		0.45271110534668 0.394940376281738
		0.445829391479492 0.389979839324951
		0.426656723022461 0.379657506942749
		0.401154518127441 0.373000383377075
		0.38721227645874 0.370096921920776
		0.367719650268555 0.362842798233032
		0.34893798828125 0.357222080230713
		0.330530643463135 0.350717067718506
		0.313499450683594 0.344108819961548
		0.298742771148682 0.336133241653442
		0.288381099700928 0.322537183761597
		0.281551361083984 0.308390617370605
		0.278762340545654 0.293604850769043
		0.279944896697998 0.278062343597412
		0.27806282043457 0.262883901596069
		0.275623321533203 0.253448724746704
		0.270369052886963 0.243475675582886
		0.263097286224365 0.236979961395264
		0.253613471984863 0.231817960739136
		0.244197845458984 0.227507352828979
		0.220239162445068 0.222903490066528
		0.21048641204834 0.223798036575317
		0.202305793762207 0.22654390335083
		0.195377349853516 0.230152130126953
		0.188922882080078 0.233012437820435
		0.183437347412109 0.233025550842285
		0.177877426147461 0.232393741607666
		0.173862934112549 0.232397794723511
		0.172021389007568 0.233372926712036
		0.173356056213379 0.23404598236084
		0.177987098693848 0.235980749130249
		0.181571483612061 0.236971616744995
		0.182929039001465 0.236026525497437
		0.18595552444458 0.234527826309204
		0.187892436981201 0.230480670928955
		0.191163539886475 0.224461317062378
		0.195268154144287 0.216319799423218
		0.206107616424561 0.195353269577026
		0.2138991355896 0.185399532318115
		0.224930763244629 0.17720103263855
		0.228293895721436 0.166174650192261
		0.234451770782471 0.15834379196167
		0.23662805557251 0.149872303009033
		0.237882137298584 0.146816253662109
		0.235296249389648 0.148083209991455
		0.22999095916748 0.152985334396362
		0.221821784973145 0.161926984786987
		0.211772918701172 0.17420506477356
		0.199408531188965 0.187267541885376
		0.187984466552734 0.203916311264038
		0.177075862884521 0.221850872039795
		0.164938449859619 0.238018751144409
		0.150642871856689 0.253601789474487
		0.138581275939941 0.270908832550049
		0.110453128814697 0.304648876190186
		0.0937137603759766 0.319470882415771
		0.0803012847900391 0.336474180221558
		0.0651917457580566 0.351107120513916
		0.0489134788513184 0.36388111114502
		0.0324978828430176 0.376163244247437
		0.014441967010498 0.386840343475342
		-0.00388669967651367 0.394574165344238
		-0.0209331512451172 0.402735710144043
		-0.0390849113464355 0.411031246185303
		-0.0606465339660645 0.416812896728516
		-0.0795478820800781 0.42249321937561
		-0.10008430480957 0.425729274749756
		-0.120504856109619 0.42767333984375
		-0.141923427581787 0.431127071380615
		-0.164621353149414 0.432888984680176
		-0.185905933380127 0.430572032928467
		-0.225934982299805 0.418219566345215
		-0.241261005401611 0.408124208450317
		-0.254226207733154 0.396452665328979
		-0.262779235839844 0.383575201034546
		-0.267789363861084 0.370597839355469
		-0.2721266746521 0.357158899307251
		-0.276215076446533 0.344230175018311
		-0.279871463775635 0.334184408187866
		-0.285885810852051 0.300092458724976
		-0.287836074829102 0.277307271957397
		-0.290016651153564 0.258711338043213
		-0.294229507446289 0.239755153656006
		-0.300615787506104 0.218581914901733
		-0.310718536376953 0.197737216949463
		-0.321629524230957 0.177024126052856
		-0.333851337432861 0.155975103378296
		-0.34548807144165 0.132482528686523
		-0.370546817779541 0.0838546752929688
		-0.383539199829102 0.0578479766845703
		-0.398926734924316 0.0303187370300293
		-0.414019107818604 0.00621175765991211
		-0.424273014068604 -0.0133872032165527
		-0.433737754821777 -0.0305643081665039
		-0.442861080169678 -0.0496551990509033
		-0.451334476470947 -0.0713081359863281
		-0.459417343139648 -0.0945430994033813
		-0.467154502868652 -0.119110226631165
		-0.474080562591553 -0.144332647323608
		-0.479512691497803 -0.170464754104614
		-0.484986782073975 -0.197066068649292
		-0.490969657897949 -0.222655653953552
		-0.495134830474854 -0.247718453407288
		-0.500430583953857 -0.272140026092529
		-0.506692886352539 -0.297374248504639
		-0.513301849365234 -0.345614194869995
		-0.513943672180176 -0.367501378059387
		-0.513702869415283 -0.388545751571655
		-0.511714935302734 -0.409014821052551
		-0.506833553314209 -0.428963303565979
		-0.497222423553467 -0.449244976043701
		-0.486149787902832 -0.467885971069336
		-0.474531650543213 -0.485920667648315
		-0.462203502655029 -0.504309892654419
		-0.44971752166748 -0.522958636283875
		-0.436763763427734 -0.542275428771973
		-0.421302795410156 -0.561989307403564
		-0.405307769775391 -0.582258939743042
		-0.386942386627197 -0.602660775184631
		-0.366604328155518 -0.623126149177551
		-0.344319343566895 -0.646055102348328
		-0.320683479309082 -0.668232798576355
		-0.277768135070801 -0.692323803901672
		-0.20991325378418 -0.715116143226624
		-0.186469078063965 -0.721548438072205
		-0.165156364440918 -0.728630185127258
		0.0397253036499023 -0.786545872688293
		0.0675458908081055 -0.793713927268982
		0.095242977142334 -0.79860782623291
		0.154822826385498 -0.810104489326477
		0.20784330368042 -0.812539219856262
		0.253764629364014 -0.813935160636902
		0.615293502807617 -0.647204518318176
		0.643192768096924 -0.633183598518372
		0.670802593231201 -0.618980169296265
		0.743740558624268 -0.573930621147156
		0.895673751831055 -0.438799023628235
		1.05518579483032 -0.189391255378723
		0.000635623931884766 1.09528541564941
		-0.583347320556641 1.00973701477051
		-0.613338708877563 0.992188930511475
		-0.643503904342651 0.975106239318848
		-0.674377918243408 0.957210063934326
		-0.706018209457397 0.940574169158936
		-0.736138582229614 0.924228429794312
		-0.764584302902222 0.907700538635254
		-0.792263031005859 0.890322923660278
		-0.819040060043335 0.872730255126953
		-0.844558715820312 0.855052947998047
		-0.870155096054077 0.835649728775024
		-0.896199226379395 0.815333127975464
		-0.923820495605469 0.794034957885742
		-0.952131986618042 0.772542953491211
		-0.9785315990448 0.74986457824707
		-1.00269031524658 0.725519180297852
		-1.02757024765015 0.699961185455322
		-1.07523036003113 0.647204637527466
		-1.09437251091003 0.620078563690186
		-1.11210680007935 0.592933416366577
		-1.12839436531067 0.567307949066162
		-1.14338636398315 0.542165279388428
		-1.15677285194397 0.516873359680176
		-1.16920042037964 0.49148154258728
		-1.18140530586243 0.465245485305786
		-1.19404697418213 0.437401056289673
		-1.20642876625061 0.407347440719604
		-1.21884965896606 0.376579761505127
		-1.23109269142151 0.344305753707886
		-1.24339413642883 0.309783697128296
		-1.25547885894775 0.275645017623901
		-1.26590919494629 0.240364789962769
		-1.27537822723389 0.203698873519897
		-1.28502869606018 0.164434432983398
		-1.29956603050232 0.088996410369873
		-1.30612921714783 0.0532190799713135
		-1.31215310096741 0.0165433883666992
		-1.31711959838867 -0.0196654796600342
		-1.32039380073547 -0.0553371906280518
		-1.32277178764343 -0.0898569822311401
		-1.32418775558472 -0.124452710151672
		-1.32500529289246 -0.158437490463257
		-1.32609105110168 -0.19228720664978
		-1.32617902755737 -0.224774241447449
		-1.32651877403259 -0.258758544921875
		-1.32579970359802 -0.292041420936584
		-1.32355952262878 -0.324952721595764
		-1.31922578811646 -0.356620788574219
		-1.31426572799683 -0.387404561042786
		-1.30942845344543 -0.419981241226196
		-1.30443930625916 -0.453237771987915
		0.244743824005127 -0.192188143730164
		0.317878723144531 -0.0535197257995605
		0.368955612182617 -0.135257244110107
		0.297122001647949 0.13664722442627
		0.443462371826172 0.0108850002288818
		0.502670288085938 0.194518089294434
		0.414446353912354 0.375095367431641
		0.232686519622803 0.224810600280762
		0.199058055877686 0.205518007278442
		0.124088764190674 0.287678480148315
		-0.206937789916992 0.425435781478882
		-0.358366012573242 0.107967376708984
		-0.51127815246582 -0.322139739990234
		-0.298972129821777 -0.68138587474823
		-0.514503955841064 1.04398608207703
		-1.05309510231018 0.673888683319092
		-1.28728914260864 -0.510735273361206
		-1.27771997451782 -0.536915302276611
		-1.26819586753845 -0.562709093093872
		-1.25748014450073 -0.587427616119385
		-1.24508428573608 -0.610039234161377
		-1.23216128349304 -0.631744027137756
		-1.21963357925415 -0.653706908226013
		-1.20684671401978 -0.676852703094482
		-1.19270896911621 -0.701040267944336
		-1.17677235603333 -0.725752234458923
		-1.15970468521118 -0.751201272010803
		-1.14170575141907 -0.777201175689697
		-1.12304663658142 -0.804616689682007
		-1.10406303405762 -0.832702994346619
		-1.08358836174011 -0.8623126745224
		-1.06120085716248 -0.893404960632324
		-1.03935527801514 -0.921954274177551
		-0.997435569763184 -0.979643583297729
		-0.97650933265686 -1.01081764698029
		-0.954917192459106 -1.04151690006256
		-0.932660102844238 -1.07052993774414
		-0.909939527511597 -1.09875893592834
		-0.886212825775146 -1.12652593851089
		-0.862452268600464 -1.15353900194168
		-0.839177370071411 -1.17903697490692
		-0.815754652023315 -1.2038522362709
		-0.792101383209229 -1.22816842794418
		-0.767385959625244 -1.25185036659241
		-0.742187976837158 -1.2749205827713
		-0.716208934783936 -1.2957581281662
		-0.689436674118042 -1.31554001569748
		-0.660673379898071 -1.33487033843994
		-0.630569219589233 -1.35101294517517
		-0.600506544113159 -1.36599403619766
		-0.544595241546631 -1.39070624113083
		-0.516556262969971 -1.40400987863541
		-0.488700866699219 -1.41589421033859
		-0.462868690490723 -1.42462944984436
		-0.437064647674561 -1.43352478742599
		-0.407913684844971 -1.44261866807938
		-0.379749774932861 -1.45121031999588
		1.33056688308716 -1.01596760749817
		1.35563373565674 -0.992703557014465
		1.40142488479614 -0.947503924369812
		1.56949138641357 -0.693477153778076
		1.59641218185425 -0.615870952606201
		1.45703172683716 1.19138956069946
		1.44387340545654 1.2247428894043
		-0.289704322814941 2.70656037330627
		-0.320497512817383 2.71177887916565
		-0.385273933410645 2.71884107589722
		-0.539919853210449 2.69782757759094
		-0.564927101135254 2.69101142883301
		-0.590946674346924 2.68302369117737
		-0.617502689361572 2.67279672622681
		-0.645879983901978 2.66252136230469
		-0.675025939941406 2.65035390853882
		-0.704952478408813 2.63782215118408
		-0.735376119613647 2.62346267700195
		-0.768058300018311 2.60692429542542
		-0.802142143249512 2.58924341201782
		-0.834689855575562 2.5705680847168
		-0.862192630767822 2.55151057243347
		-0.891415357589722 2.5333309173584
		-0.921496391296387 2.51435279846191
		-0.952172040939331 2.49623608589172
		-1.01182007789612 2.46045851707458
		-1.06711292266846 2.42441987991333
		-1.22242474555969 2.33184289932251
		-1.32146668434143 2.27758526802063
		-1.57897305488586 2.04121494293213
		-1.6480188369751 1.94861459732056
		-1.67137670516968 1.91444730758667
		-2.25361108779907 0.874212026596069
		-2.26539397239685 0.797172069549561
		-2.27008938789368 0.756518125534058
		-2.27581930160522 0.715568065643311
		-2.2820155620575 0.671371698379517
		-2.28688764572144 0.62915563583374
		-2.29258489608765 0.587712049484253
		-2.30083727836609 0.545308113098145
		-2.30962038040161 0.50223970413208
		-2.31872916221619 0.459707975387573
		-2.32791781425476 0.418349027633667
		-2.33625292778015 0.378353118896484
		-2.35341095924377 0.299217224121094
		-2.36205077171326 0.259202718734741
		-2.37082481384277 0.219289779663086
		-2.37931704521179 0.17857813835144
		-2.38751935958862 0.138083457946777
		-2.39563727378845 0.0995147228240967
		-2.4016592502594 0.0617759227752686
		-2.40769982337952 0.0250015258789062
		-2.41449761390686 -0.0468127727508545
		-2.41528987884521 -0.0820958614349365
		-2.41491532325745 -0.11840283870697
		-2.41299533843994 -0.151818990707397
		-2.41100978851318 -0.184613704681396
		-2.40664196014404 -0.218201398849487
		-2.40203356742859 -0.251810908317566
		-2.3967866897583 -0.287399172782898
		-2.39388537406921 -0.322534918785095
		-2.381267786026 -0.401355266571045
		-2.37408089637756 -0.443756341934204
		-2.36735057830811 -0.487742185592651
		-2.36215329170227 -0.531498074531555
		-2.35752153396606 -0.576264142990112
		-2.35336685180664 -0.622230052947998
		-2.34855937957764 -0.667589902877808
		-2.34447503089905 -0.711048364639282
		-2.3418447971344 -0.755615472793579
		-2.3410120010376 -0.799931645393372
		-2.33989763259888 -0.843094706535339
		-2.33670544624329 -0.885925650596619
		-2.33290004730225 -0.928900361061096
		-2.32806205749512 -0.971526503562927
		-2.32050442695618 -1.01427781581879
		-2.31167984008789 -1.05693066120148
		-2.30255722999573 -1.09987038373947
		-2.28236293792725 -1.19041496515274
		-2.26996302604675 -1.23702794313431
		-2.25768184661865 -1.28114533424377
		-2.24549078941345 -1.32466202974319
		-2.23391342163086 -1.36858493089676
		-2.22111892700195 -1.4110643863678
		-2.20887303352356 -1.45023894309998
		-2.19683218002319 -1.48708492517471
		-2.18462538719177 -1.52269667387009
		-2.17144393920898 -1.55671948194504
		-2.15778207778931 -1.58942127227783
		-2.14257025718689 -1.62325593829155
		-2.12607502937317 -1.65824967622757
		-2.10942792892456 -1.69390663504601
		-2.09220862388611 -1.7306235730648
		-2.0724835395813 -1.76860895752907
		-2.05078744888306 -1.80741992592812
		-2.00400161743164 -1.88384968042374
		-1.97906064987183 -1.92237174510956
		-1.95275402069092 -1.96187348663807
		-1.92724633216858 -1.9982313066721
		-1.90249633789062 -2.0328359156847
		-1.87849926948547 -2.06690534064546
		-1.85164165496826 -2.10034058988094
		-1.82491588592529 -2.13212168961763
		-1.79769921302795 -2.16205789893866
		-1.76935219764709 -2.19062901288271
		-1.74066495895386 -2.21796932816505
		-1.7110493183136 -2.24473166465759
		-1.68170881271362 -2.27094706892967
		-1.65143728256226 -2.2974946051836
		-1.62045001983643 -2.32440593838692
		-1.58984279632568 -2.34969666600227
		-1.56005930900574 -2.37272024154663
		-1.49762749671936 -2.41797864437103
		-1.46767425537109 -2.43602341413498
		-1.44050121307373 -2.45182201266289
		-1.41324687004089 -2.46686562895775
		-1.38416886329651 -2.48116624355316
		-1.35521483421326 -2.49339607357979
		-1.32497119903564 -2.50404217839241
		-1.29381799697876 -2.51406338810921
		-1.26369762420654 -2.52342221140862
		-1.23093128204346 -2.53150218725204
		-1.16138768196106 -2.54533371329308
		-1.12258219718933 -2.55138838291168
		-0.997140645980835 -2.57278525829315
		-0.909528970718384 -2.58448070287704
		-0.866600275039673 -2.58940428495407
		-0.825949192047119 -2.59541898965836
		-0.400846004486084 -2.59659290313721
		-0.323870658874512 -2.558499366045
		-0.285403728485107 -2.54078635573387
		-0.248787403106689 -2.52475935220718
		-0.217128753662109 -2.51330947875977
		-0.185720443725586 -2.50488662719727
		-0.153455257415771 -2.49865132570267
		-0.122417449951172 -2.49272155761719
		-0.0640659332275391 -2.46941301226616
		0.0270724296569824 -2.4031730890274
		0.0581064224243164 -2.3757598400116
		0.14694881439209 -2.28924432396889
		0.177852153778076 -2.2608225941658
		0.208495616912842 -2.23119166493416
		0.238874435424805 -2.20432397723198
		0.298620223999023 -2.16592083126307
		0.32868480682373 -2.14919875562191
		0.358621120452881 -2.13479162752628
		0.416624546051025 -2.11850539594889
		0.447444915771484 -2.11314310505986
		0.479402542114258 -2.10795144736767
		0.53981351852417 -2.10506253316998
		0.568412780761719 -2.10404275357723
		0.659700870513916 -2.10751416534185
		0.687624931335449 -2.11187508702278
		1.29006958007812 -1.94416399300098
		1.3372368812561 -1.90888941287994
		1.53340673446655 -1.76066148281097
		1.55816030502319 -1.74136555194855
		1.58145189285278 -1.7212016582489
		1.60648584365845 -1.70230749249458
		1.62718296051025 -1.68331179022789
		1.64575862884521 -1.66528597474098
		1.68503618240356 -1.6324103474617
		1.70443201065063 -1.61509642004967
		1.738356590271 -1.57982692122459
		1.75437068939209 -1.55862414836884
		1.76754808425903 -1.53786581754684
		1.78147220611572 -1.51620477437973
		1.79591703414917 -1.49340116977692
		1.80657052993774 -1.4696056842804
		1.81633758544922 -1.44516170024872
		1.82488775253296 -1.41984003782272
		1.83294343948364 -1.39247667789459
		1.8410325050354 -1.36351543664932
		1.84689569473267 -1.33538049459457
		1.85570526123047 -1.30703413486481
		1.86204242706299 -1.27923280000687
		1.86887216567993 -1.25146263837814
		1.88799953460693 -1.16520243883133
		1.89627361297607 -1.13632905483246
		1.90449810028076 -1.10646677017212
		1.98085594177246 -0.784555435180664
		1.98875761032104 -0.761571168899536
		2.00995397567749 -0.719612121582031
		2.01883268356323 -0.697352886199951
		2.04478597640991 -0.574985146522522
		1.95436954498291 0.222334861755371
		1.95725011825562 0.255880117416382
		1.96000528335571 0.288040637969971
		1.9628849029541 0.320069789886475
		1.96722936630249 0.352580308914185
		1.97021436691284 0.385518312454224
		1.97024583816528 0.417383432388306
		1.96860265731812 0.447250366210938
		1.96731233596802 0.50609302520752
		1.9672679901123 0.536402940750122
		1.96639776229858 0.567726850509644
		1.96342992782593 0.600409984588623
		1.95831918716431 0.63367748260498
		1.95049524307251 0.66839075088501
		1.94130754470825 0.703469276428223
		1.93104839324951 0.739678859710693
		1.92077827453613 0.776458978652954
		1.91051340103149 0.813912630081177
		1.89990472793579 0.851215124130249
		1.89012098312378 0.888729333877563
		1.88151359558105 0.927408933639526
		1.87119102478027 0.966757297515869
		1.86127424240112 1.00381898880005
		1.85330247879028 1.04165196418762
		1.84587144851685 1.08209729194641
		1.83152008056641 1.16457676887512
		1.82439613342285 1.20593571662903
		1.81831645965576 1.24764490127563
		1.81271696090698 1.29049825668335
		1.80806350708008 1.33366131782532
		1.80342531204224 1.37706303596497
		1.79928922653198 1.42026662826538
		1.7971453666687 1.46274161338806
		1.79433917999268 1.50360155105591
		1.79073858261108 1.54185962677002
		1.78850507736206 1.57890057563782
		1.78533029556274 1.61689305305481
		1.77936553955078 1.65458941459656
		1.77215480804443 1.69134116172791
		1.76421213150024 1.72705721855164
		1.75564289093018 1.76215815544128
		1.74704170227051 1.79564142227173
		1.72739744186401 1.86128783226013
		1.71561241149902 1.89452505111694
		1.70328283309937 1.92758560180664
		1.68997430801392 1.96368288993835
		1.67693424224854 2.00393080711365
		1.66645002365112 2.04511189460754
		1.65657567977905 2.08444046974182
		1.64457130432129 2.12453842163086
		1.63191890716553 2.1675066947937
		1.62269878387451 2.21275925636292
		1.61720418930054 2.25856971740723
		1.61373615264893 2.30315804481506
		1.60957717895508 2.34642052650452
		1.60499095916748 2.38978672027588
		1.59963417053223 2.43225789070129
		1.5933313369751 2.4761049747467
		1.58933258056641 2.51898574829102
		-1.29669737815857 -0.483376026153564
		-1.01832628250122 -0.950077176094055
		-0.57034158706665 -1.37942218780518
		-0.516458511352539 2.70517754554749
		-1.18905401229858 2.34989953041077
		-2.34445548057556 0.338964462280273
		-2.38806486129761 -0.360974788665771
		-2.29243230819702 -1.14463686943054
		-2.0277144908905 -1.84598053991795
		-1.52983593940735 -2.39586943387985
		-0.362374782562256 -2.58049273490906
		0.387324810028076 -2.12533460184932
		1.66561460494995 -1.64850580692291
		1.9673752784729 0.476650714874268
		1.83908987045288 1.12314629554749
		1.58502817153931 2.60557079315186
		1.58406448364258 2.64927816390991
		1.58242988586426 2.68812775611877
		1.5798716545105 2.72636914253235
		1.51393747329712 3.02699828147888
		-0.124678611755371 4.20443820953369
		-0.160244941711426 4.22027730941772
		-0.193114280700684 4.23818707466125
		-0.227484703063965 4.25466060638428
		-0.260913372039795 4.27157402038574
		-0.403662204742432 4.3402111530304
		-0.442275047302246 4.3545069694519
		-0.485790252685547 4.36636924743652
		-0.527101516723633 4.38018202781677
		-0.565081596374512 4.39249134063721
		-0.601755142211914 4.40324831008911
		-0.63889741897583 4.40784955024719
		-0.676595449447632 4.41289401054382
		-0.714593648910522 4.41830611228943
		-0.788907051086426 4.42795085906982
		-0.826500177383423 4.42929124832153
		-0.863492012023926 4.43156766891479
		-0.901363134384155 4.43281126022339
		-1.14219951629639 4.434246301651
		-1.17949223518372 4.43559050559998
		-1.21873140335083 4.43601393699646
		-1.29791688919067 4.44250535964966
		-1.33931136131287 4.44604587554932
		-1.37961959838867 4.45002579689026
		-1.41981768608093 4.45318055152893
		-1.4564642906189 4.46156072616577
		-2.13085269927979 4.43182468414307
		-2.35638403892517 4.34141278266907
		-2.49751377105713 4.28180313110352
		-2.52496933937073 4.26759099960327
		-2.75772988796234 4.20397353172302
		-3.40758538246155 4.2420494556427
		-3.49682247638702 4.22978472709656
		-3.56490099430084 4.21172451972961
		-3.72223800420761 4.16917896270752
		-4.54988226667047 2.65141105651855
		-4.55744732171297 2.61663150787354
		-4.63490474969149 2.03544211387634
		-4.64186987280846 1.99602842330933
		-4.64891293272376 1.95807123184204
		-4.65664889663458 1.91834759712219
		-4.66422605514526 1.87747669219971
		-4.67152072489262 1.83692574501038
		-4.6764026209712 1.79753565788269
		-4.65569248050451 1.45130395889282
		-4.64606685191393 1.41955518722534
		-4.63563089817762 1.38606834411621
		-4.62575577571988 1.35111546516418
		-4.61396354995668 1.31347155570984
		-4.602758676745 1.27379202842712
		-4.59036883898079 1.23333811759949
		-4.57641697302461 1.19529986381531
		-4.56173906847835 1.15940880775452
		-4.54857661575079 1.12266421318054
		-4.5343305580318 1.08709383010864
		-4.519834831357 1.04947829246521
		-4.50518117845058 1.0110936164856
		-4.47888568043709 0.937682628631592
		-4.46760940551758 0.901084899902344
		-4.44034348428249 0.82365870475769
		-4.42624649405479 0.784178733825684
		-4.41335700452328 0.744888067245483
		-4.3994043469429 0.707567691802979
		-4.38476076722145 0.669619083404541
		-4.36960543692112 0.633818387985229
		-4.35243183374405 0.597996234893799
		-4.33569243550301 0.562502145767212
		-4.31775832176208 0.528888463973999
		-4.29749092459679 0.496784925460815
		-4.27538186311722 0.467316627502441
		-4.2514223754406 0.437769174575806
		-4.22524318099022 0.409273862838745
		-4.20040947198868 0.382643699645996
		-4.17372596263885 0.356757879257202
		-4.14584773778915 0.331774711608887
		-4.11631852388382 0.307438611984253
		-4.05589020252228 0.260846138000488
		-4.02274340391159 0.23731255531311
		-3.98701959848404 0.213740110397339
		-3.94924908876419 0.191959857940674
		-3.90749990940094 0.173275947570801
		-3.8671846985817 0.152487993240356
		-3.83298647403717 0.129753351211548
		-3.79806685447693 0.10661244392395
		-3.76082342863083 0.083491325378418
		-3.72200465202332 0.0617899894714355
		-3.68550968170166 0.0395750999450684
		-3.57727706432343 -0.0289900302886963
		-3.53887224197388 -0.0535352230072021
		-3.46355807781219 -0.103548049926758
		-3.39046704769135 -0.151049137115479
		-3.17591059207916 -0.248821377754211
		-3.13769257068634 -0.257687568664551
		-3.02755010128021 -0.2863529920578
		-2.99115383625031 -0.295754790306091
		-2.95299530029297 -0.305933475494385
		-2.91587340831757 -0.315494656562805
		-2.87696957588196 -0.3264000415802
		-2.83641052246094 -0.33561098575592
		-2.79450595378876 -0.342979073524475
		-2.750812292099 -0.348366618156433
		-2.7033611536026 -0.352126240730286
		-2.65276038646698 -0.359118103981018
		-2.60619187355042 -0.370252013206482
		-2.52297878265381 -0.394192695617676
		-2.48068761825562 -0.408087491989136
		-2.39927768707275 -0.437232136726379
		-2.35953903198242 -0.452861189842224
		-2.2826828956604 -0.48480212688446
		-2.24623084068298 -0.501744389533997
		-2.09651327133179 -0.573573231697083
		-1.84740424156189 -0.653395175933838
		-1.81103944778442 -0.660107612609863
		-1.77560305595398 -0.666983246803284
		-1.73799562454224 -0.67051088809967
		-1.70212602615356 -0.673930525779724
		-1.6637749671936 -0.676748394966125
		-1.62431788444519 -0.679673433303833
		-1.58258247375488 -0.683019280433655
		-1.54093384742737 -0.685417771339417
		-1.49897861480713 -0.687060475349426
		-1.45732927322388 -0.687062859535217
		-1.41757106781006 -0.687598347663879
		-1.37885236740112 -0.687753558158875
		-1.33969712257385 -0.688208699226379
		-1.29980087280273 -0.689888477325439
		-1.25923156738281 -0.695621013641357
		-1.10503554344177 -0.715830206871033
		-1.06684923171997 -0.722302079200745
		-1.02712726593018 -0.731185913085938
		-0.986946821212769 -0.738367915153503
		-0.946746826171875 -0.746049523353577
		-0.742647171020508 -0.769329071044922
		-0.671017408370972 -0.767243385314941
		0.141541004180908 -0.473962426185608
		0.206554412841797 -0.434712052345276
		0.336203575134277 -0.333460092544556
		0.355794429779053 -0.307351350784302
		0.425021648406982 -0.11326014995575
		0.429826259613037 -0.0840921401977539
		0.430779457092285 -0.0549068450927734
		0.432490825653076 0.00406193733215332
		0.436112403869629 0.0328750610351562
		0.44124174118042 0.0915300846099854
		0.449906349182129 0.205270528793335
		0.452280521392822 0.234741449356079
		0.452969074249268 0.265023231506348
		0.454581260681152 0.323949813842773
		0.457519054412842 0.352993726730347
		0.457813262939453 0.382885694503784
		0.458809375762939 0.414554119110107
		0.457891464233398 0.448054075241089
		0.453404903411865 0.480981588363647
		0.308011054992676 0.755092859268188
		0.28810977935791 0.766688108444214
		0.266928672790527 0.777087450027466
		0.243512630462646 0.787376403808594
		0.218341827392578 0.795889616012573
		0.192546844482422 0.805432796478271
		0.171152114868164 0.816164255142212
		0.15043830871582 0.828520536422729
		0.105767726898193 0.851438999176025
		0.0829334259033203 0.86394476890564
		0.0598263740539551 0.876285076141357
		-0.645771265029907 0.425600290298462
		-0.64622688293457 0.41634202003479
		-0.64609956741333 0.405576467514038
		-0.635387420654297 0.407418251037598
		-0.631699800491333 0.412808418273926
		-0.626741886138916 0.419063329696655
		-0.622390508651733 0.423846244812012
		-0.616232395172119 0.429705142974854
		-0.608434677124023 0.43577241897583
		-0.597229957580566 0.443042755126953
		-0.554276466369629 0.469800472259521
		-0.538060188293457 0.478265523910522
		-0.522171497344971 0.486138343811035
		-0.505465507507324 0.494146347045898
		-0.44761848449707 0.516604423522949
		-0.429244995117188 0.524779319763184
		-0.405308246612549 0.534150123596191
		-0.383967399597168 0.543862342834473
		-0.364859104156494 0.553305387496948
		-0.344911098480225 0.559716463088989
		-0.327674388885498 0.564679384231567
		-0.310309886932373 0.568539619445801
		-0.295854568481445 0.574695825576782
		-0.280683994293213 0.58046293258667
		-0.254661560058594 0.58939528465271
		-0.243091106414795 0.594078540802002
		-0.233814716339111 0.596724987030029
		-0.226614952087402 0.598632097244263
		-0.219466686248779 0.599214315414429
		-0.212057113647461 0.600447654724121
		-0.202766895294189 0.60158896446228
		1.58644485473633 2.55997228622437
		-0.0877523422241211 4.18661904335022
		-0.753582239151001 4.42287635803223
		-4.45416580140591 0.862858772277832
		-4.08704447746277 0.284059524536133
		-3.10141944885254 -0.270267963409424
		-2.13670492172241 -0.556227326393127
		-1.14369940757751 -0.710853457450867
		0.446651935577393 0.148282766342163
		0.128088474273682 0.839929819107056
		-0.468228340148926 0.509299516677856
		-0.193849563598633 0.601641893386841
		-0.151124477386475 0.669442415237427
		-0.156197071075439 0.642545461654663
		-0.173178672790527 0.648711442947388
		-0.169086456298828 0.660304307937622
		0.187442779541016 -0.296054005622864
		-1.29291844367981 0.125106334686279
		1.73746633529663 1.82906007766724
		-0.18605899810791 0.603196382522583
		-0.177406311035156 0.608280420303345
		-0.168651580810547 0.615051507949829
		-0.162323474884033 0.621321678161621
		-0.156878471374512 0.627245187759399
		-0.152524471282959 0.633376121520996
		-0.148797512054443 0.640159368515015
		-0.145305633544922 0.646092891693115
		-0.143763542175293 0.652109622955322
		-0.143428325653076 0.658360481262207
		-0.143693447113037 0.663336038589478
		-0.144739627838135 0.667201280593872
		-0.1456298828125 0.669757127761841
		-0.147010326385498 0.671627521514893
		-0.148738384246826 0.672910213470459
		-0.149610042572021 0.67240571975708
		-0.150368213653564 0.671210050582886
		-0.152036190032959 0.667159557342529
		-0.153104305267334 0.66432785987854
		-0.153993606567383 0.661499738693237
		-0.154722213745117 0.658397912979126
		-0.155334949493408 0.655032873153687
		-0.155972957611084 0.652511835098267
		-0.156762599945068 0.650664567947388
		-0.156816005706787 0.649554491043091
		-0.155936241149902 0.647962093353271
		-0.156054973602295 0.648412466049194
		-0.15577220916748 0.647952556610107
		-0.155218601226807 0.647212028503418
		-0.155232906341553 0.646515846252441
		-0.154995441436768 0.645752429962158
		-0.155182361602783 0.645328283309937
		-0.155441284179688 0.644339084625244
		-0.155731201171875 0.643541574478149
		-0.156999588012695 0.641479969024658
		-0.157299518585205 0.640864372253418
		-0.158003807067871 0.640629529953003
		-0.159074783325195 0.640942096710205
		-0.159783840179443 0.641289710998535
		-0.160358905792236 0.642080307006836
		-0.160533428192139 0.642005205154419
		-0.16222620010376 0.643749237060547
		-0.164155960083008 0.644567012786865
		-0.165218353271484 0.64490532875061
		-0.166973114013672 0.646193504333496
		-0.168387889862061 0.64797043800354
		-0.170182704925537 0.649528741836548
		-0.171244144439697 0.649488210678101
	};
\addlegendentry{Optitrack}
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.233598 0.142923
		-0.234864 0.140831
		-0.155847 0.127126
		-0.182829 0.140527
		-0.159678 0.122278
		-0.183684 0.139408
		-0.212984 0.166318
		-0.212312 0.167175
		-0.157321 0.125297
		-0.205796 0.159654
		-0.158696 0.123551
		-0.210425 0.169543
		-0.201944 0.164499
		-0.238245 0.14381
		-0.182394 0.141091
		-0.234133 0.150413
		-0.181601 0.14211
		-0.160663 0.120982
		-0.184083 0.148093
		-0.21433 0.164579
		-0.205796 0.159654
		-0.20644 0.15882
		-0.184083 0.148093
		-0.203866 0.162111
		-0.209633 0.170522
		-0.159678 0.122278
		-0.201944 0.164499
		-0.206405 0.174416
		-0.209633 0.170522
		-0.162636 0.118316
		-0.18644 0.1357
		-0.18644 0.1357
		-0.148293 0.0924178
		-0.248505 0.136027
		-0.265987 0.138994
		-0.268574 0.130957
		-0.262074 0.143191
		-0.254134 0.138195
		-0.267113 0.144451
		-0.320831 0.150172
		-0.254932 0.130224
		-0.259052 0.132863
		-0.253001 0.133937
		-0.260761 0.125992
		-0.258569 0.1338
		-0.300576 0.146636
		-0.262557 0.132958
		-0.250359 0.13813
		-0.202316 0.131754
		-0.249633 0.149155
		-0.240526 0.146128
		-0.249822 0.152444
		-0.246108 0.14557
		-0.250735 0.147295
		-0.213657 0.165453
		-0.182706 0.140687
		-0.159678 0.122278
		-0.241443 0.153182
		-0.235626 0.129613
		-0.2172 0.160773
		-0.253691 0.125467
		-0.554728 0.118637
		-0.561151 0.0297729
		-0.500336 -0.133456
		-0.196247 -0.160394
		-0.253028 -0.247871
		-0.0371643 -0.418148
		-0.0331704 -0.424965
		0.083795 -0.405212
		0.0592004 -0.41298
		-0.211774 0.167855
		-0.187544 0.13417
		-0.232158 0.138491
		-0.171913 0.163188
		-0.182394 0.141091
		-0.169223 0.165977
		-0.210301 0.169697
		-0.197427 0.138973
		-0.194332 0.143269
		-0.233746 0.132973
		-0.239527 0.141665
		-0.224419 0.133188
		-0.220901 0.138944
		-0.197991 0.138169
		-0.231677 0.136546
		-0.238126 0.144008
		-0.221593 0.137838
		-0.181346 0.111757
		-0.22422 0.133522
		-0.230115 0.139163
		-0.221086 0.13865
		-0.239631 0.14149
		-0.228872 0.141198
		-0.187744 0.116065
		-0.235924 0.139049
		-0.246108 0.14557
		-0.255313 0.140563
		-0.251759 0.133447
		-0.260026 0.134301
		-0.252334 0.134489
		-0.253633 0.139112
		-0.244407 0.132792
		-0.255068 0.122644
		-0.336126 0.111818
		-0.343221 0.116181
		-0.249247 0.121007
		-0.25688 0.122983
		-0.328805 0.106945
		-0.265585 0.123552
		-0.314323 0.110638
		-0.316187 0.108967
		-0.276032 0.123425
		-0.316791 0.151028
		-0.316934 0.165882
		-0.259591 0.128385
		-0.253001 0.123395
		-0.355145 0.156299
		-0.393158 0.124249
		-0.386988 0.159492
		-0.460709 0.14322
		-0.440341 0.128924
		-0.657503 0.204548
		-0.707248 0.162496
		-0.634471 0.191759
		-0.599427 0.16444
		-0.532988 0.105035
		-0.530434 0.117255
		-0.519706 0.0695716
		-0.503083 0.0542512
		-0.515868 0.0462122
		-0.492413 0.0383081
		-0.492256 0.0402704
		-0.561289 0.0270317
		-0.561878 -0.00832611
		-0.564651 0.0126456
		-0.631059 0.177994
		-0.651161 0.167262
		-0.640668 0.0487465
		-0.669869 -0.0203873
		-0.647414 0.193899
		-0.694 -0.0292675
		-0.653333 -0.0372826
		-0.599263 0.0428222
		-0.565444 -0.0149431
		-0.599801 -0.0295504
		-0.647563 -0.0606558
		-0.644133 -0.0620428
		-0.610607 -0.0628668
		-0.523543 -0.0346518
		-0.536319 -0.049302
		-0.521274 -0.0456628
		-0.500235 -0.102932
		-0.463405 -0.102045
		-0.562017 -0.117246
		-0.561932 -0.117656
		-0.406081 -0.081821
		-0.555166 -0.106608
		-0.594595 -0.124042
		-0.515147 -0.123187
		-0.576808 -0.168049
		-0.607967 -0.161559
		-0.616049 -0.178118
		-0.612604 -0.250899
		-0.474349 -0.217117
		-0.476837 -0.282235
		-0.386502 -0.235622
		-0.235276 -0.116846
		-0.281465 -0.173413
		-0.23185 -0.120173
		-0.217181 -0.109818
		-0.1674 -0.0945096
		-0.232429 -0.173229
		-0.203772 -0.150458
		-0.268947 -0.259629
		-0.26955 -0.259002
		-0.268932 -0.259645
		-0.268932 -0.259645
		-0.270487 -0.275119
		-0.270487 -0.275119
		-0.315192 -0.324757
		-0.292108 -0.324368
		-0.292108 -0.324368
		-0.319633 -0.365034
		-0.311521 -0.328107
		-0.311521 -0.328107
		-0.322489 -0.339469
		-0.323994 -0.338032
		-0.323994 -0.338032
		-0.378765 -0.412284
		-0.364342 -0.39823
		-0.364342 -0.39823
		-0.32678 -0.37378
		-0.293322 -0.298345
		-0.293322 -0.298345
		-0.238633 -0.257606
		-0.238633 -0.257606
		-0.228615 -0.248392
		-0.322164 -0.480925
		-0.322164 -0.480925
		-0.260178 -0.466906
		-0.222963 -0.435827
		-0.222963 -0.435827
		-0.20974 -0.445324
		-0.231802 -0.512868
		-0.223905 -0.526743
		-0.224102 -0.531999
		-0.210457 -0.505284
		-0.210457 -0.505284
		-0.102555 -0.379358
		-0.0480361 -0.387099
		-0.0480361 -0.387099
		-0.0408256 -0.393723
		-0.0408256 -0.393723
		-0.0509162 -0.627246
		-0.0480831 -0.564521
		-0.0480831 -0.564521
		-0.0479431 -0.416089
		-0.0479431 -0.416089
		-0.0876599 -0.37573
		-0.0876599 -0.37573
		-0.101199 -0.374344
		-0.108806 -0.378778
		-0.0929131 -0.375968
		-0.0929131 -0.375968
		-0.16761 -0.416794
		-0.0871783 -0.389476
		-0.0871783 -0.389476
		-0.0397894 -0.393569
		-0.0063836 -0.42621
		0.0187805 -0.41642
		0.0343487 -0.415426
		0.0252026 -0.447055
		0.083795 -0.405212
		0.0422832 -0.398818
		0.0785992 -0.417879
		0.0641273 -0.360848
		0.070356 -0.356307
		0.155261 -0.403724
		0.177035 -0.4236
		0.173007 -0.409716
		0.19768 -0.459313
		0.261577 -0.455077
		0.202645 -0.412293
		0.179326 -0.454856
		0.192885 -0.481602
		0.083795 -0.405212
		0.0713301 -0.406457
		0.0559601 -0.446169
		0.0559601 -0.446169
		0.0582743 -0.45265
		0.0330414 -0.415532
		0.0366073 -0.421918
		0.0340311 -0.375883
		0.0433059 -0.392902
		0.0515386 -0.414006
		0.0561425 -0.413407
		0.0574623 -0.413226
		0.0574623 -0.413226
		0.0356897 -0.412877
		0.0461242 -0.383517
		0.0461242 -0.383517
		0.0513499 -0.41403
		0.0561425 -0.413407
		0.0633043 -0.419529
		0.0879211 -0.455289
		0.0873973 -0.38828
		0.0874488 -0.392225
		0.191275 -0.404266
		0.0924824 -0.3601
		0.240585 -0.337621
		0.253498 -0.343278
		0.234306 -0.31901
		0.263957 -0.335484
		0.319983 -0.413892
		0.254525 -0.366595
		0.287328 -0.366475
		0.3393 -0.436995
		0.280966 -0.368568
		0.257933 -0.336553
		0.289323 -0.419511
		0.338807 -0.456493
		0.307767 -0.424194
		0.266571 -0.39325
		0.268313 -0.392063
		0.300561 -0.40878
		0.264174 -0.388951
		0.280834 -0.373823
		0.297139 -0.393963
		0.237109 -0.370986
		0.278454 -0.371679
		0.228002 -0.292476
		0.324294 -0.419338
		0.334846 -0.44572
		0.343153 -0.461172
		0.336311 -0.469414
		0.334176 -0.443069
		0.239726 -0.356399
		0.268081 -0.396134
		0.251878 -0.352949
		0.330254 -0.378069
		0.282276 -0.284577
		0.33128 -0.254433
		0.215412 -0.216204
		0.474625 -0.314209
		0.181823 -0.171912
		0.319577 -0.209481
		0.376113 -0.248017
		0.378229 -0.25392
		0.352564 -0.221547
		0.353375 -0.279335
		1.0801 -0.3217
		0.319571 -0.240339
		0.312475 -0.206874
		0.490516 -0.295169
		0.506238 -0.303881
		0.514899 -0.364933
		0.536347 -0.315058
		0.514401 -0.310393
		0.496705 -0.230419
		0.511657 -0.253048
		0.415863 -0.241406
		0.411114 -0.197066
		0.480105 -0.230137
		0.518861 -0.252663
		0.412013 -0.195179
		0.408811 -0.22155
		0.397968 -0.211846
		0.317285 -0.177438
		0.331503 -0.192217
		0.488772 -0.246396
		0.512875 -0.236486
		0.507571 -0.252973
		0.508409 -0.242771
		0.40618 -0.20781
		0.48326 -0.223436
		0.501835 -0.219987
		0.450395 -0.190194
		0.513269 -0.127891
		0.384916 -0.0876402
		0.426417 -0.124147
		0.364334 -0.0758683
		0.412047 -0.101126
		0.39248 -0.116319
		0.333115 -0.151492
		0.399838 -0.114485
		0.435975 -0.0985221
		0.416131 -0.0940378
		0.441177 -0.104136
		0.411609 -0.0928824
		0.360872 -0.0471444
		0.360405 -0.0186922
		0.368902 -0.0301791
		0.357349 -0.0132882
		0.360642 -0.0133604
		0.248603 0.0147356
		0.321936 0.0131684
		0.478126 0.0355586
		0.382963 -0.0113499
		0.48655 0.0398036
		0.466519 0.0311088
		0.409423 0.0120888
		0.406126 0.0105317
		0.386174 -0.0295996
		0.341595 -0.0298131
		0.518802 -0.0244363
		0.449747 -0.019412
		0.290192 -0.0289102
		0.56877 -0.00803693
		0.507484 0.00717098
		0.554114 0.00780201
		0.558111 0.00783043
		0.491209 -0.0223982
		0.566755 0.0298189
		0.536399 0.0262472
		0.60921 0.0509229
		0.460807 0.053338
		0.357508 0.0478207
		0.490259 0.0687845
		0.455817 0.0660192
		0.394444 0.0713189
		0.457639 0.0579927
		0.399227 0.089812
		0.500998 0.122093
		0.474152 0.114308
		0.345806 0.0867335
		0.373 0.0962466
		0.371048 0.103517
		0.468098 0.133265
		0.470827 0.123276
		0.47653 0.12523
		0.448048 0.169941
		0.528532 0.204398
		0.744448 0.352779
		0.568154 0.243595
		0.590416 0.256605
		0.232968 0.0904673
		0.368331 0.150662
		0.445892 0.238131
		0.422718 0.235906
		0.414298 0.251685
		0.47631 0.287502
		0.330057 0.205506
		0.422029 0.280576
		0.262355 0.160849
		0.295673 0.182328
		0.32467 0.196785
		0.330614 0.176844
		0.310093 0.222577
		0.270971 0.197684
		0.25307 0.199329
		0.246907 0.188303
		0.166667 0.140749
		0.362529 0.294615
		0.205654 0.185815
		0.220023 0.206122
		0.273814 0.264167
		0.256976 0.247983
		0.256976 0.247983
		0.256976 0.247983
		0.208322 0.199021
		0.257815 0.253744
		0.230492 0.226869
		0.223956 0.211748
		0.211312 0.203764
		0.232262 0.222704
		0.197043 0.182845
		0.197043 0.182845
		0.199404 0.188226
		0.199404 0.188226
		0.199084 0.184056
		0.183439 0.160368
		0.183439 0.160368
		0.194234 0.162865
		0.158774 0.127995
		0.158774 0.127995
		0.152322 0.124431
		0.152322 0.124431
		0.176876 0.144183
		0.160366 0.126898
		0.13269 0.115654
		0.13269 0.115654
		0.145552 0.122374
		0.145552 0.122374
		0.130411 0.113592
		0.133769 0.115523
		0.133769 0.115523
		0.14478 0.135086
		0.114026 0.103975
		0.116986 0.105361
		0.200711 0.221691
		0.200711 0.221691
		0.173391 0.185642
		0.169878 0.202402
		0.176021 0.217383
		0.176021 0.217383
		0.191589 0.247035
		0.191589 0.247035
		0.155756 0.209911
		0.1486 0.234126
		0.1486 0.234126
		0.186162 0.326741
		0.271618 0.521916
		0.271618 0.521916
		0.117771 0.262675
		0.11791 0.260171
		0.11791 0.260171
		0.0915629 0.279046
		0.0915629 0.279046
		0.0701679 0.230345
		0.0495476 0.165123
		0.0495476 0.165123
		0.0454165 0.162017
		0.0279323 0.123447
		0.0285945 0.216168
		-0.0160372 0.331535
		-0.0441726 0.230786
		-0.119088 0.392646
		-0.140385 0.315588
		-0.119906 0.210493
		-0.210482 0.209344
		-0.210482 0.209344
		-0.248878 0.215718
		-0.280694 0.229537
		-0.317634 0.276419
		-0.263889 0.214811
		-0.340407 0.249764
		-0.385204 0.216446
		-0.327982 0.17282
		-0.322019 0.158525
		-0.343888 0.159252
		-0.348291 0.155028
		-0.385182 0.148639
		-0.42066 0.138696
		-0.372212 0.10496
		-0.383712 0.0957104
		-0.391182 0.0876381
		-0.340604 0.0525964
		-0.335782 0.0406406
		-0.422898 0.0315039
		-0.440403 0.0144005
		-0.577517 -0.0517172
		-0.614073 -0.113415
		-0.586378 -0.166751
		-0.609864 -0.261064
		-0.641268 -0.315799
		-0.649031 -0.336013
		-0.577054 -0.323362
		-0.676517 -0.394485
		-0.693223 -0.412626
		-0.682134 -0.458931
		-0.661432 -0.466891
		-0.577209 -0.434749
		-0.573437 -0.439713
		-0.589854 -0.483501
		-0.490858 -0.411346
		-0.552487 -0.492349
		-0.55889 -0.525979
		-0.582058 -0.625257
		-0.550998 -0.715533
		-0.581012 -0.79205
		-0.577126 -0.831707
		-0.377833 -0.928873
		-0.350575 -0.962825
		-0.304502 -0.969691
		-0.189735 -0.970845
		-0.128075 -0.980886
		-0.0495586 -0.962891
		0.460911 -0.911802
		0.510836 -0.960805
		0.523272 -0.910362
		0.524725 -0.810343
		0.671745 -0.755509
		1.00235 -0.615106
		0.385628 0.911396
		-0.405152 0.946212
		-0.433129 0.933737
		-0.500094 0.977632
		-0.5016 0.929351
		-0.490058 0.871819
		-0.52079 0.88878
		-0.551174 0.857708
		-0.533462 0.834049
		-0.579056 0.864479
		-0.612776 0.877949
		-0.631097 0.858778
		-0.645441 0.852423
		-0.674166 0.853266
		-0.681789 0.791362
		-0.676805 0.73974
		-0.713472 0.725785
		-0.89106 0.805941
		-0.83553 0.729007
		-0.934983 0.756671
		-1.02987 0.783595
		-0.985615 0.739438
		-1.00029 0.73275
		-1.07169 0.749038
		-1.08549 0.708458
		-1.10329 0.680404
		-1.02329 0.589768
		-1.03626 0.565922
		-1.01611 0.519598
		-1.05603 0.528101
		-1.08848 0.522373
		-1.03807 0.477662
		-1.10125 0.485438
		-1.13362 0.459811
		-1.17076 0.419218
		-1.26467 0.279927
		-1.26962 0.260892
		-1.24023 0.221075
		-1.26679 0.189719
		-1.24642 0.177985
		-1.22163 0.146848
		-1.21048 0.119321
		-1.21638 0.103364
		-1.33104 0.0856674
		-1.31556 0.0402452
		-1.33362 0
		-1.27686 -0.0303811
		-1.38444 -0.0656557
		-1.25837 -0.0934579
		-1.29619 -0.131723
		-1.29619 -0.131723
		-1.29276 -0.162028
		0.293523 -0.434629
		0.744418 -0.273727
		0.481491 -0.227222
		0.377954 -0.0778845
		0.48739 -0.0141792
		0.3931 0.0797236
		0.446997 0.23704
		0.224472 0.211201
		0.144985 0.128122
		0.116986 0.105361
		0.124194 0.274879
		-0.241675 0.199401
		-0.493375 -0.0181492
		-0.533061 -0.522021
		-0.314026 0.917878
		-0.797056 0.746157
		-1.39012 -0.288233
		-1.32132 -0.322202
		-1.23941 -0.367356
		-1.23941 -0.367356
		-1.20877 -0.47658
		-1.18605 -0.48161
		-1.18605 -0.48161
		-1.19662 -0.528847
		-1.19662 -0.528847
		-1.14426 -0.537411
		-1.22238 -0.628905
		-1.02396 -0.554825
		-1.02396 -0.554825
		-1.05893 -0.621416
		-1.13936 -0.701703
		-1.13936 -0.701703
		-1.13202 -0.727813
		-1.06706 -0.766061
		-1.1226 -0.860561
		-1.11313 -0.868748
		-1.11313 -0.868748
		-1.1044 -0.908758
		-1.18843 -1.03968
		-1.18843 -1.03968
		-0.978945 -0.941775
		-1.1084 -1.10143
		-1.1084 -1.10143
		-1.10475 -1.1864
		-1.06233 -1.19223
		-1.06233 -1.19223
		-0.986547 -1.19649
		-0.990135 -1.25339
		-0.990135 -1.25339
		-0.98264 -1.38695
		-0.99052 -1.50776
		-0.865025 -1.51552
		-0.876944 -1.551
		-0.876944 -1.551
		-0.772228 -1.47926
		-0.771621 -1.58259
		-0.771621 -1.58259
		1.19022 -1.52142
		1.40371 -1.77806
		1.30768 -1.55847
		1.24478 -0.949681
		1.2563 -0.890952
		1.5941 0.86579
		1.6221 0.892669
		0.116072 2.67343
		0.0863476 2.55451
		-0.00829328 2.69055
		-0.218209 2.73116
		-0.233549 2.71437
		-0.257376 2.70181
		-0.299156 2.70424
		-0.350814 2.70991
		-0.456347 2.72504
		-0.467441 2.67508
		-0.504752 2.66002
		-0.542101 2.67279
		-0.562951 2.68443
		-0.598226 2.67526
		-0.644345 2.68354
		-0.660342 2.67965
		-0.635774 2.54729
		-0.706898 2.65535
		-0.691308 2.43554
		-0.856972 2.55112
		-0.995707 2.53608
		-1.12586 2.20526
		-1.30375 1.91049
		-1.36672 1.93025
		-1.37006 1.71654
		-2.16352 1.1423
		-2.23862 1.08515
		-2.23862 1.08515
		-2.19752 1.02584
		-2.51377 1.02383
		-2.51377 1.02383
		-2.41527 0.89491
		-2.50502 0.852745
		-2.50502 0.852745
		-2.54559 0.836601
		-2.492 0.758435
		-2.492 0.758435
		-2.52909 0.637199
		-2.52909 0.637199
		-2.50986 0.607025
		-2.61204 0.571461
		-2.61204 0.571461
		-2.59478 0.542011
		-2.5906 0.42576
		-2.5906 0.42576
		-2.48638 0.194948
		-2.48638 0.194948
		-2.55243 0.146247
		-2.33749 0.0919175
		-2.45295 0.0588192
		-2.61733 0.0313805
		-2.5566 -0.00763987
		-2.6171 -0.0467831
		-2.62971 -0.0781118
		-2.5469 -0.1897
		-2.62285 -0.235137
		-2.67735 -0.280027
		-2.67735 -0.280027
		-2.66477 -0.328474
		-2.57358 -0.380288
		-2.50929 -0.420034
		-2.54521 -0.489523
		-2.50663 -0.514299
		-2.41926 -0.533416
		-2.40904 -0.562413
		-2.47166 -0.645365
		-2.4577 -0.681586
		-2.53823 -0.738424
		-2.40651 -0.729583
		-2.50749 -0.813828
		-2.48391 -0.857239
		-2.52978 -0.963024
		-2.36958 -0.962908
		-2.48175 -1.06902
		-2.43782 -1.09606
		-2.51279 -1.21046
		-2.4869 -1.24612
		-2.69129 -1.37998
		-2.65956 -1.39947
		-2.8497 -1.54268
		-2.68031 -1.50982
		-2.43474 -1.44169
		-2.36913 -1.43652
		-2.33505 -1.45748
		-2.04801 -1.32237
		-2.04294 -1.35185
		-2.0974 -1.39999
		-2.03822 -1.42893
		-1.99323 -1.45571
		-2.41991 -1.84325
		-2.28564 -1.82028
		-2.27985 -1.88915
		-2.23255 -1.888
		-2.14086 -1.86315
		-2.39415 -2.13595
		-2.32886 -2.11159
		-2.36469 -2.19809
		-2.29452 -2.1685
		-2.27431 -2.18532
		-2.28786 -2.26299
		-2.41109 -2.4951
		-2.25002 -2.38588
		-2.19425 -2.38557
		-2.0954 -2.35077
		-2.18867 -2.49576
		-2.11208 -2.56828
		-2.19205 -2.6778
		-2.17133 -2.68219
		-2.0669 -2.59596
		-2.03173 -2.78565
		-1.95007 -2.74718
		-1.94774 -2.80588
		-1.95854 -2.90588
		-1.96589 -2.92187
		-1.85549 -2.86585
		-1.76206 -2.83462
		-1.66962 -2.76482
		-1.54473 -2.81365
		-1.28432 -2.54897
		-1.32003 -2.64572
		-1.26988 -2.62175
		-0.93601 -2.82077
		-0.855453 -2.86122
		-0.822457 -2.96482
		-0.793776 -3.01278
		-0.703867 -2.90824
		-0.657345 -3.04037
		-0.578784 -2.93293
		-0.542809 -2.9398
		-0.434628 -2.88036
		-0.327662 -2.80887
		-0.271032 -2.8149
		-0.177681 -2.8371
		-0.143934 -2.83901
		-0.075087 -2.78927
		-0.0085345 -2.8279
		0.091145 -2.7538
		0.119961 -2.83929
		0.127909 -2.81714
		0.177769 -2.77153
		0.265807 -2.81577
		0.265807 -2.81577
		0.350972 -2.71113
		0.398038 -2.46827
		0.513182 -2.45468
		0.561183 -2.45605
		1.35337 -2.59206
		1.40585 -2.46661
		1.52982 -2.26583
		1.59163 -2.3128
		1.43537 -2.09656
		0.770791 -1.25253
		1.75486 -2.39211
		1.68252 -2.21366
		2.18787 -2.56299
		2.20266 -2.52692
		2.2962 -2.57816
		2.15322 -2.38039
		2.23855 -2.46134
		2.22922 -2.42155
		2.2395 -2.29121
		2.34289 -2.34688
		2.2612 -2.2461
		2.34606 -2.30114
		2.48361 -2.42578
		2.40316 -2.2968
		2.28956 -2.1772
		1.852 -1.64495
		2.1767 -1.92731
		1.91307 -1.63949
		1.72879 -1.37944
		1.70291 -1.33633
		1.74554 -1.3443
		2.3806 -1.33058
		1.92795 -1.06016
		2.61059 -1.24329
		2.56344 -1.2123
		2.23932 -0.805446
		2.12332 -0.0330229
		2.9225 -0.0181236
		2.9225 -0.0181236
		2.11554 0.113291
		2.1109 0.205481
		2.11431 0.251489
		2.1908 0.254535
		2.18018 0.301223
		2.18344 0.379502
		2.12471 0.408275
		2.11307 0.455535
		2.16948 0.48677
		2.16948 0.48677
		1.89089 0.493143
		1.92807 0.535221
		1.92807 0.535221
		1.85033 0.58424
		1.92206 0.656653
		1.92206 0.656653
		2.01626 0.772643
		2.29672 0.956127
		2.29672 0.956127
		2.27867 0.993244
		2.27867 0.993244
		1.73802 0.883113
		1.69534 0.922013
		1.78323 0.981934
		2.16598 1.27795
		2.16598 1.27795
		2.16988 1.27132
		1.98874 1.22003
		2.07814 1.30282
		2.07155 1.34171
		2.01679 1.35392
		2.01679 1.35392
		2.05751 1.47942
		2.06292 1.58023
		1.98018 1.53416
		1.98018 1.53416
		1.95276 1.58504
		1.95276 1.58504
		2.03974 1.68131
		1.84972 1.64159
		1.67418 1.52962
		1.67063 1.53349
		1.69639 1.62361
		1.69639 1.62361
		1.63941 1.63504
		1.63941 1.63504
		1.56879 1.57105
		1.8085 1.91992
		1.8085 1.91992
		1.77651 1.93446
		1.76032 1.9492
		1.82232 2.02682
		1.8173 2.03131
		1.58507 1.79589
		1.58507 1.79589
		1.57113 1.8072
		-1.39012 -0.288233
		-1.06706 -0.766061
		-0.99052 -1.50776
		-0.191338 2.71544
		-0.906552 2.46592
		-2.53104 0.719864
		-2.56322 -0.14466
		-2.47957 -0.922615
		-2.00394 -1.44093
		-2.10015 -2.45755
		-0.865875 -2.71906
		0.142401 -2.92271
		1.22679 -1.78487
		2.18018 0.301223
		1.69534 0.922013
		1.37444 1.79557
		1.55365 2.0765
		1.37266 1.86524
		1.37266 1.86524
		1.22072 1.97997
		0.163256 3.74637
		0.14041 3.72851
		0.115034 3.58937
		0.0866313 3.74892
		0.0559805 3.92034
		-0.101025 3.86382
		-0.129853 3.75692
		-0.149581 3.72003
		-0.165545 3.59216
		-0.217843 3.7816
		-0.283655 3.95045
		-0.30748 3.94252
		-0.362062 3.9394
		-0.3815 3.90671
		-0.42369 3.88204
		-0.437367 3.9046
		-0.484107 3.89757
		-0.490128 3.86738
		-0.760247 3.94221
		-0.780025 3.92581
		-0.815332 3.93012
		-0.891155 3.8988
		-0.925062 3.9574
		-0.973757 3.94442
		-0.984673 3.94171
		-0.984673 3.94171
		-1.5937 3.80186
		-1.82271 3.65116
		-1.87497 3.49943
		-2.05501 3.69152
		-2.14617 3.55346
		-2.21013 2.9316
		-2.32797 2.85571
		-2.33677 2.80951
		-2.37837 2.81498
		-3.57578 2.30365
		-3.57578 2.30365
		-3.99563 2.01269
		-4.00455 1.87817
		-4.00455 1.87817
		-3.96279 1.83551
		-3.88481 1.77618
		-3.88973 1.68182
		-3.91776 1.65418
		-4.04525 1.40335
		-4.04525 1.40335
		-3.99847 1.28768
		-4.04638 1.29933
		-4.04638 1.29933
		-4.05502 1.26723
		-4.07418 1.24985
		-4.09404 1.22184
		-4.12426 1.17563
		-4.14535 1.09893
		-4.14535 1.09893
		-4.09894 1.04855
		-4.10448 1.02663
		-4.16869 0.945188
		-4.17373 0.922672
		-4.19586 0.898631
		-4.20944 0.832737
		-4.20944 0.832737
		-4.2611 0.828547
		-4.19295 0.734678
		-4.19295 0.734678
		-3.94721 0.658154
		-3.67172 0.561942
		-3.67326 0.551767
		-3.78128 0.537383
		-4.16508 0.551655
		-4.03423 0.48885
		-4.03688 0.46642
		-4.03942 0.443946
		-3.8621 0.414756
		-3.82635 0.387078
		-3.83137 0.333754
		-3.7981 0.297149
		-3.81797 0.300401
		-3.82109 0.257697
		-3.81176 0.235646
		-3.8141 0.194022
		-3.68289 0.175934
		-3.66815 0.144307
		-3.65897 0.0925362
		-3.52937 0.0395582
		-3.48172 0.039135
		-3.51654 0.019876
		-3.53253 0.00998319
		-3.53253 -0.00998319
		-3.49256 -0.0397078
		-3.58651 -0.0815524
		-3.45831 -0.238655
		-3.45683 -0.259186
		-2.72886 -0.261981
		-2.72943 -0.277917
		-2.70517 -0.276259
		-2.70353 -0.291868
		-2.70154 -0.292517
		-2.62454 -0.309049
		-2.63315 -0.318763
		-2.63315 -0.318763
		-2.62927 -0.349346
		-2.62982 -0.367142
		-2.5112 -0.365499
		-2.47196 -0.407516
		-2.37337 -0.407962
		-2.45496 -0.469268
		-2.37303 -0.475207
		-1.71547 -0.379414
		-1.73327 -0.41125
		-1.76357 -0.471757
		-1.66745 -0.589825
		-1.67568 -0.648572
		-1.56547 -0.627752
		-1.52341 -0.628281
		-1.56721 -0.665883
		-1.50834 -0.663657
		-1.49906 -0.684354
		-1.4677 -0.675113
		-1.53016 -0.722001
		-1.51089 -0.720738
		-1.52541 -0.765272
		-1.45302 -0.760578
		-1.40331 -0.781422
		-1.38654 -0.785896
		-1.37712 -0.795456
		-1.27956 -0.765276
		-1.11982 -0.771318
		-1.09109 -0.791733
		-1.05336 -0.778188
		-1.0484 -0.814786
		-1.05767 -0.853925
		-0.822754 -0.806097
		-0.755814 -0.837154
		0.122598 -0.981857
		0.217775 -0.937215
		0.380984 -0.659475
		0.368956 -0.604611
		0.447162 -0.388417
		0.253823 -0.18063
		0.253435 -0.181174
		0.366921 -0.235117
		0.513154 -0.22559
		0.496167 -0.15663
		0.478936 -0.0705557
		0.517566 -0.0477232
		0.469099 -0.0157958
		0.433852 0.044014
		0.42826 0.0661324
		0.47862 0.1108
		0.469313 0.123655
		0.489762 0.150994
		0.416644 0.147309
		0.403957 0.514735
		0.367457 0.489695
		0.435657 0.597475
		0.381813 0.544209
		0.410303 0.619306
		0.32001 0.526815
		0.343039 0.624227
		0.272485 0.521934
		0.359238 0.764124
		0.342602 0.760187
		0.30972 0.743135
		-0.517277 0.33312
		-0.517277 0.33312
		-0.531628 0.299228
		-0.584764 0.236621
		-0.584764 0.236621
		-0.588857 0.226243
		-0.563958 0.214372
		-0.563958 0.214372
		-0.552491 0.22449
		-0.554063 0.220581
		-0.50192 0.189522
		-0.50192 0.189522
		-0.487924 0.187015
		-0.393915 0.141242
		-0.370797 0.16408
		-0.367453 0.165927
		-0.362927 0.175606
		-0.385412 0.212348
		-0.384827 0.230435
		-0.403144 0.265841
		-0.403144 0.265841
		-0.35861 0.240937
		-0.328185 0.240281
		-0.328185 0.240281
		-0.278717 0.216611
		-0.278717 0.216611
		-0.274331 0.22214
		-0.240707 0.210951
		-0.240707 0.210951
		-0.234005 0.206277
		-0.23475 0.217534
		1.45936 1.89029
		0.191886 3.7011
		-0.406868 3.93502
		-4.19041 0.923713
		-3.95124 0.343221
		-3.36719 -0.271095
		-1.7778 -0.464503
		-1.13156 -0.732687
		0.533028 -0.128486
		0.281865 0.552956
		-0.378002 0.159104
		-0.235103 0.218013
		-0.226661 0.255075
		0.299404 -0.402377
		-1.15177 0.332451
		1.84972 1.64159
		-0.233412 0.219822
		-0.216138 0.216088
		-0.218498 0.227869
		-0.210212 0.218098
		-0.213284 0.218906
		-0.211345 0.217
		-0.212718 0.219456
		-0.225276 0.230054
		-0.25566 0.261357
		-0.240897 0.249109
		-0.248515 0.26816
		-0.250455 0.266349
		-0.236578 0.245905
		-0.200168 0.245873
		-0.200168 0.245873
		-0.198665 0.233351
		-0.226661 0.255075
		-0.23254 0.249728
		-0.22891 0.253059
		-0.22891 0.253059
		-0.244527 0.240622
		-0.248503 0.235666
		-0.248503 0.235666
		-0.242675 0.241288
		-0.241831 0.242959
		-0.246687 0.252995
		-0.264547 0.277064
		-0.239513 0.254935
		-0.242709 0.256941
		-0.215971 0.225233
		-0.219314 0.231155
		-0.236466 0.248986
		-0.218319 0.228717
		-0.224626 0.235325
		-0.246019 0.253645
		-0.266016 0.275654
		-0.266364 0.274504
		-0.268663 0.272627
		-0.269366 0.271932
		-0.269366 0.271932
		-0.270075 0.271228
		-0.249725 0.249544
		-0.249083 0.250185
		-0.270757 0.270547
		-0.294567 0.292844
		-0.276608 0.276393
		-0.299246 0.294513
		-0.274175 0.271195
		-0.237138 0.259739
		-0.250362 0.248905
		-0.270757 0.270547
	};
\addlegendentry{Pred}
\addplot [draw=red, mark=o, only marks]
table{%
		x  y
		-0.127206325531006 0.336211204528809
		-0.134419441223145 0.331306219100952
		-0.133753776550293 0.332391738891602
		-0.133886814117432 0.332860946655273
		-0.134137153625488 0.333293199539185
		-0.134048461914062 0.33379077911377
		-0.133165836334229 0.335495233535767
		-0.132776260375977 0.335920333862305
		-0.132369995117188 0.336314678192139
		-0.13191032409668 0.336570739746094
		-0.13095760345459 0.337332010269165
		-0.134012699127197 0.331721544265747
		-0.12944221496582 0.336433887481689
		-0.131443500518799 0.33923602104187
		-0.129917621612549 0.336459875106812
		-0.130057334899902 0.336324691772461
		-0.130042552947998 0.336323499679565
		-0.129631996154785 0.336425542831421
		-0.129331588745117 0.33652138710022
		-0.129453182220459 0.336517572402954
		-0.12966251373291 0.336363554000854
		-0.129889011383057 0.336460590362549
		-0.129928112030029 0.336501121520996
		-0.13056468963623 0.33737850189209
		-0.132200717926025 0.339166402816772
		-0.133244037628174 0.339192628860474
		1.48837184906006 -1.79680702090263
		1.51169395446777 -1.77818402647972
		1.87379026412964 -1.22246450185776
		1.96542549133301 -0.829026818275452
		1.88099431991577 -1.19361960887909
		1.56966733932495 2.84534358978271
		1.56297874450684 2.88486242294312
		1.45581245422363 3.12256407737732
		1.43606519699097 3.15328907966614
		1.41528272628784 3.18331432342529
		1.3942346572876 3.21430468559265
		1.37285947799683 3.24273252487183
		1.30512714385986 3.32663822174072
		1.28122186660767 3.35366344451904
		1.2566065788269 3.37853813171387
		1.22669887542725 3.40153908729553
		1.19250440597534 3.42830920219421
		1.13290119171143 3.47973799705505
		1.10378265380859 3.50279903411865
		1.04111480712891 3.55282711982727
		1.00658416748047 3.58054971694946
		0.975536823272705 3.60814118385315
		0.944155216217041 3.63566255569458
		0.913527011871338 3.66178846359253
		0.885063648223877 3.68749570846558
		0.856333255767822 3.71239733695984
		0.826505661010742 3.73820018768311
		0.798305511474609 3.76467323303223
		0.766876220703125 3.79016494750977
		0.736276626586914 3.81562232971191
		0.705400943756104 3.8399498462677
		0.673804759979248 3.86397790908813
		0.644132137298584 3.88783955574036
		0.61450719833374 3.90927672386169
		0.55016565322876 3.93943738937378
		0.515307903289795 3.95416188240051
		0.481907367706299 3.97110962867737
		0.447263717651367 3.98452091217041
		0.414120197296143 3.99796438217163
		0.3821120262146 4.01247310638428
		0.348891735076904 4.023517370224
		0.315462589263916 4.03659605979919
		0.281076908111572 4.04957556724548
		0.245109081268311 4.06288051605225
		0.207736968994141 4.07650637626648
		0.169685363769531 4.0901210308075
		0.128819465637207 4.10358047485352
		0.0873255729675293 4.11724829673767
		0.0501694679260254 4.13015222549438
		-0.0149927139282227 4.15698289871216
		-0.0509490966796875 4.17031574249268
		-0.294960021972656 4.28855013847351
		-0.330137252807617 4.30537080764771
		-0.3666090965271 4.32211446762085
		-0.937418699264526 4.43487882614136
		-0.976156234741211 4.4368097782135
		-1.01523780822754 4.43747448921204
		-1.05521440505981 4.43886852264404
		-1.09977555274963 4.43570065498352
		-1.53107452392578 4.47047019004822
		-1.9883930683136 4.47778487205505
		-2.02428364753723 4.4678909778595
		-2.09637141227722 4.44344329833984
		-2.54859137535095 4.26521348953247
		-2.57706809043884 4.25314140319824
		-2.60288333892822 4.24578809738159
		-2.62685918807983 4.238605260849
		-2.65104758739471 4.23094868659973
		-2.67718267440796 4.22304844856262
		-2.70208704471588 4.2170832157135
		-3.35370290279388 4.25053334236145
		-3.4366739988327 4.23933410644531
		-3.46608150005341 4.23578405380249
		-3.64101892709732 4.19075274467468
		-3.83840227127075 4.11388659477234
		-4.56400008313358 2.58181285858154
		-4.5788249084726 2.46781444549561
		-4.58145009726286 2.42833924293518
		-4.58794745849445 2.34922552108765
		-4.59265303518623 2.31213641166687
		-4.59761593677104 2.27460432052612
		-4.60220231488347 2.23346638679504
		-4.61376073583961 2.15303230285645
		-4.62103664875031 2.115314245224
		-4.62802820280194 2.07553625106812
		-4.67956501245499 1.75870227813721
		-4.68301013112068 1.72068071365356
		-4.68606703728437 1.68488693237305
		-4.68550603836775 1.6498236656189
		-4.68293036520481 1.61361503601074
		-4.67857114970684 1.57682991027832
		-4.67319777607918 1.54225659370422
		-4.66163071244955 1.48022794723511
		-4.49162828922272 0.974047183990479
		1.16172933578491 3.45492267608643
		0.581977367401123 3.92502427101135
		-1.49411177635193 4.46626806259155
		-3.3784407377243 4.24612951278687
		-4.60737638175488 2.19235944747925
		-4.66783845424652 1.5105562210083
		-0.16835880279541 0.647355794906616
	};
\addlegendentry{Miss}


==> tikz/vis_localize/vis_loc_test3_clean.tex <==
% This file was created with tikzplotlib v0.10.1.
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.127345561981201 0.33639669418335
		-0.127428531646729 0.336060523986816
		-0.128036975860596 0.336326837539673
		-0.128693580627441 0.337846279144287
		-0.130049705505371 0.338828802108765
		-0.138466358184814 0.337401866912842
		-0.144834041595459 0.334638833999634
		-0.142208576202393 0.334274768829346
		-0.137418746948242 0.334198474884033
		-0.137037754058838 0.33245849609375
		-0.136043548583984 0.332458019256592
		-0.12939453125 0.336419105529785
		-0.130695343017578 0.338706254959106
		-0.134543418884277 0.33806324005127
		-0.133503913879395 0.333352565765381
		-0.132727146148682 0.332768678665161
		-0.134922504425049 0.331595182418823
		-0.165335178375244 0.308836460113525
		-0.18049955368042 0.299356460571289
		-0.209865570068359 0.276289463043213
		-0.224143028259277 0.26317310333252
		-0.250017642974854 0.235231637954712
		-0.259373188018799 0.220257759094238
		-0.284072399139404 0.155272960662842
		-0.288110733032227 0.119146585464478
		-0.285177707672119 0.0823261737823486
		-0.281112670898438 0.0637161731719971
		-0.276029109954834 0.044203519821167
		-0.272835254669189 0.0257899761199951
		-0.256765365600586 -0.028867244720459
		-0.249118328094482 -0.0451648235321045
		-0.242172718048096 -0.0621557235717773
		-0.238335609436035 -0.0789104700088501
		-0.24898624420166 -0.0919655561447144
		-0.257389068603516 -0.086189866065979
		-0.271154880523682 -0.0775504112243652
		-0.330009937286377 -0.0535423755645752
		-0.351505279541016 -0.0458657741546631
		-0.37312650680542 -0.0388782024383545
		-0.391369819641113 -0.031400203704834
		-0.404147624969482 -0.0229568481445312
		-0.412797927856445 -0.0151066780090332
		-0.419476985931396 -0.00657343864440918
		-0.423289775848389 0.00167560577392578
		-0.422009944915771 0.0155158042907715
		-0.415642738342285 0.0215318202972412
		-0.404873371124268 0.0266897678375244
		-0.362000465393066 0.0285007953643799
		-0.34178638458252 0.0248384475708008
		-0.295982837677002 0.0126585960388184
		-0.273382186889648 0.0057227611541748
		-0.226951599121094 -0.0176470279693604
		-0.217410564422607 -0.0291993618011475
		-0.208463668823242 -0.0423965454101562
		-0.192939758300781 -0.0752726793289185
		-0.185149192810059 -0.0941650867462158
		-0.172919273376465 -0.126591324806213
		-0.16869068145752 -0.137657403945923
		-0.16331148147583 -0.143073201179504
		-0.165642738342285 -0.142706990242004
		-0.177671909332275 -0.137000679969788
		-0.210398197174072 -0.128688216209412
		-0.249642848968506 -0.122074484825134
		-0.269594192504883 -0.121593475341797
		-0.29789924621582 -0.123217701911926
		-0.295314311981201 -0.125708222389221
		-0.244179725646973 -0.125024318695068
		-0.220665454864502 -0.123825430870056
		-0.19743824005127 -0.121778845787048
		-0.163980960845947 -0.125649571418762
		-0.12041711807251 -0.147732973098755
		-0.105488777160645 -0.152384996414185
		-0.0885343551635742 -0.15541934967041
		-0.0689239501953125 -0.155092716217041
		-0.0440235137939453 -0.153853297233582
		0.00612306594848633 -0.152277946472168
		0.0440340042114258 -0.168996095657349
		0.0435194969177246 -0.177294254302979
		0.0248465538024902 -0.19659161567688
		-0.013519287109375 -0.220731616020203
		-0.0350570678710938 -0.234177947044373
		-0.0556979179382324 -0.245718240737915
		-0.0766358375549316 -0.254761338233948
		-0.112179756164551 -0.273218750953674
		-0.148095607757568 -0.282817602157593
		-0.143739223480225 -0.278131365776062
		-0.138580799102783 -0.270571351051331
		-0.10306978225708 -0.244179368019104
		-0.0941438674926758 -0.244161605834961
		-0.0595850944519043 -0.230524182319641
		0.0823922157287598 -0.154309988021851
		0.127522945404053 -0.149468660354614
		0.137029647827148 -0.151102185249329
		0.125154495239258 -0.180585741996765
		0.104872226715088 -0.205686807632446
		0.0924921035766602 -0.21928858757019
		0.0831584930419922 -0.23091721534729
		0.0763993263244629 -0.241548776626587
		0.0763096809387207 -0.258049130439758
		0.076683521270752 -0.267605304718018
		0.0754432678222656 -0.276083588600159
		0.0617537498474121 -0.293706893920898
		0.0561628341674805 -0.295415043830872
		0.0496621131896973 -0.299678683280945
		0.050717830657959 -0.302342176437378
		0.0563607215881348 -0.30420184135437
		0.0593900680541992 -0.306122303009033
		0.0621929168701172 -0.306800603866577
		0.0632481575012207 -0.298717856407166
		0.0646572113037109 -0.293217182159424
		0.0684065818786621 -0.287723302841187
		0.0741477012634277 -0.282844662666321
		0.154258251190186 -0.207270503044128
		0.188057899475098 -0.189673781394958
		0.262718200683594 -0.182254791259766
		0.23896312713623 -0.21306037902832
		0.226468086242676 -0.231433749198914
		0.208513259887695 -0.263208746910095
		0.202855587005615 -0.279374718666077
		0.196976661682129 -0.292702198028564
		0.204080581665039 -0.293481349945068
		0.211403369903564 -0.288840413093567
		0.217202663421631 -0.284569025039673
		0.226415634155273 -0.278469443321228
		0.232580661773682 -0.263120770454407
		0.238749027252197 -0.238720536231995
		0.240648746490479 -0.225665330886841
		0.242067813873291 -0.210521221160889
		0.244743824005127 -0.192188143730164
		0.247630596160889 -0.17639946937561
		0.249472141265869 -0.165167570114136
		0.251272201538086 -0.154857873916626
		0.255558490753174 -0.140889644622803
		0.257637023925781 -0.12615978717804
		0.275506019592285 -0.0706666707992554
		0.294573307037354 -0.0355722904205322
		0.310517311096191 -0.00803828239440918
		0.304028034210205 -0.020911693572998
		0.317878723144531 -0.0535197257995605
		0.370843410491943 -0.12634551525116
		0.376821517944336 -0.17090106010437
		0.375263690948486 -0.156908750534058
		0.368955612182617 -0.135257244110107
		0.3638596534729 -0.124979853630066
		0.333609580993652 -0.0632095336914062
		0.328624248504639 -0.0518476963043213
		0.324001312255859 -0.0259950160980225
		0.316646099090576 0.0431790351867676
		0.311479568481445 0.0860886573791504
		0.304279804229736 0.105211019515991
		0.297122001647949 0.13664722442627
		0.301129341125488 0.146174669265747
		0.334969997406006 0.126255989074707
		0.345934391021729 0.115550756454468
		0.372883796691895 0.0950582027435303
		0.403318881988525 0.0633001327514648
		0.409867286682129 0.0529162883758545
		0.416993141174316 0.0437567234039307
		0.42347526550293 0.0369217395782471
		0.428780078887939 0.0292983055114746
		0.433215618133545 0.0232694149017334
		0.450963973999023 0.0147478580474854
		0.454798221588135 0.02201247215271
		0.459031581878662 0.0279545783996582
		0.480697631835938 0.0479066371917725
		0.490830898284912 0.0555980205535889
		0.500276565551758 0.0646281242370605
		0.507074356079102 0.0812771320343018
		0.508538722991943 0.0945429801940918
		0.511963367462158 0.134072542190552
		0.51190185546875 0.155261754989624
		0.502670288085938 0.194518089294434
		0.496715545654297 0.216670036315918
		0.490595817565918 0.241269588470459
		0.483274459838867 0.264455080032349
		0.477270603179932 0.285759925842285
		0.472188949584961 0.305264711380005
		0.468234062194824 0.322073936462402
		0.463737010955811 0.338606595993042
		0.460882663726807 0.356423377990723
		0.462459564208984 0.386286020278931
		0.464548110961914 0.393747329711914
		0.445829391479492 0.389979839324951
		0.414446353912354 0.375095367431641
		0.401154518127441 0.373000383377075
		0.34893798828125 0.357222080230713
		0.330530643463135 0.350717067718506
		0.313499450683594 0.344108819961548
		0.298742771148682 0.336133241653442
		0.288381099700928 0.322537183761597
		0.281551361083984 0.308390617370605
		0.278762340545654 0.293604850769043
		0.279944896697998 0.278062343597412
		0.27806282043457 0.262883901596069
		0.275623321533203 0.253448724746704
		0.232686519622803 0.224810600280762
		0.220239162445068 0.222903490066528
		0.177877426147461 0.232393741607666
		0.173862934112549 0.232397794723511
		0.172021389007568 0.233372926712036
		0.173356056213379 0.23404598236084
		0.177987098693848 0.235980749130249
		0.18595552444458 0.234527826309204
		0.195268154144287 0.216319799423218
		0.199058055877686 0.205518007278442
		0.2138991355896 0.185399532318115
		0.224930763244629 0.17720103263855
		0.23662805557251 0.149872303009033
		0.221821784973145 0.161926984786987
		0.211772918701172 0.17420506477356
		0.199408531188965 0.187267541885376
		0.187984466552734 0.203916311264038
		0.177075862884521 0.221850872039795
		0.164938449859619 0.238018751144409
		0.150642871856689 0.253601789474487
		0.138581275939941 0.270908832550049
		0.110453128814697 0.304648876190186
		0.0803012847900391 0.336474180221558
		0.0651917457580566 0.351107120513916
		0.0489134788513184 0.36388111114502
		0.0324978828430176 0.376163244247437
		0.014441967010498 0.386840343475342
		-0.00388669967651367 0.394574165344238
		-0.0390849113464355 0.411031246185303
		-0.0606465339660645 0.416812896728516
		-0.0795478820800781 0.42249321937561
		-0.10008430480957 0.425729274749756
		-0.120504856109619 0.42767333984375
		-0.164621353149414 0.432888984680176
		-0.185905933380127 0.430572032928467
		-0.206937789916992 0.425435781478882
		-0.225934982299805 0.418219566345215
		-0.254226207733154 0.396452665328979
		-0.267789363861084 0.370597839355469
		-0.2721266746521 0.357158899307251
		-0.279871463775635 0.334184408187866
		-0.287836074829102 0.277307271957397
		-0.294229507446289 0.239755153656006
		-0.300615787506104 0.218581914901733
		-0.310718536376953 0.197737216949463
		-0.321629524230957 0.177024126052856
		-0.333851337432861 0.155975103378296
		-0.370546817779541 0.0838546752929688
		-0.383539199829102 0.0578479766845703
		-0.398926734924316 0.0303187370300293
		-0.433737754821777 -0.0305643081665039
		-0.451334476470947 -0.0713081359863281
		-0.459417343139648 -0.0945430994033813
		-0.467154502868652 -0.119110226631165
		-0.474080562591553 -0.144332647323608
		-0.484986782073975 -0.197066068649292
		-0.490969657897949 -0.222655653953552
		-0.495134830474854 -0.247718453407288
		-0.500430583953857 -0.272140026092529
		-0.506692886352539 -0.297374248504639
		-0.513301849365234 -0.345614194869995
		-0.513943672180176 -0.367501378059387
		-0.513702869415283 -0.388545751571655
		-0.511714935302734 -0.409014821052551
		-0.497222423553467 -0.449244976043701
		-0.486149787902832 -0.467885971069336
		-0.474531650543213 -0.485920667648315
		-0.462203502655029 -0.504309892654419
		-0.44971752166748 -0.522958636283875
		-0.436763763427734 -0.542275428771973
		-0.421302795410156 -0.561989307403564
		-0.405307769775391 -0.582258939743042
		-0.386942386627197 -0.602660775184631
		-0.366604328155518 -0.623126149177551
		-0.344319343566895 -0.646055102348328
		-0.298972129821777 -0.68138587474823
		-0.277768135070801 -0.692323803901672
		-0.186469078063965 -0.721548438072205
		-0.165156364440918 -0.728630185127258
		0.0397253036499023 -0.786545872688293
		0.095242977142334 -0.79860782623291
		0.154822826385498 -0.810104489326477
		0.20784330368042 -0.812539219856262
		0.253764629364014 -0.813935160636902
		0.643192768096924 -0.633183598518372
		0.670802593231201 -0.618980169296265
		0.743740558624268 -0.573930621147156
		0.895673751831055 -0.438799023628235
		1.05518579483032 -0.189391255378723
		0.000635623931884766 1.09528541564941
		-0.514503955841064 1.04398608207703
		-0.583347320556641 1.00973701477051
		-0.613338708877563 0.992188930511475
		-0.643503904342651 0.975106239318848
		-0.674377918243408 0.957210063934326
		-0.706018209457397 0.940574169158936
		-0.736138582229614 0.924228429794312
		-0.764584302902222 0.907700538635254
		-0.819040060043335 0.872730255126953
		-0.844558715820312 0.855052947998047
		-0.896199226379395 0.815333127975464
		-0.952131986618042 0.772542953491211
		-0.9785315990448 0.74986457824707
		-1.00269031524658 0.725519180297852
		-1.02757024765015 0.699961185455322
		-1.05309510231018 0.673888683319092
		-1.07523036003113 0.647204637527466
		-1.11210680007935 0.592933416366577
		-1.12839436531067 0.567307949066162
		-1.14338636398315 0.542165279388428
		-1.15677285194397 0.516873359680176
		-1.16920042037964 0.49148154258728
		-1.19404697418213 0.437401056289673
		-1.20642876625061 0.407347440719604
		-1.21884965896606 0.376579761505127
		-1.23109269142151 0.344305753707886
		-1.24339413642883 0.309783697128296
		-1.25547885894775 0.275645017623901
		-1.26590919494629 0.240364789962769
		-1.27537822723389 0.203698873519897
		-1.28502869606018 0.164434432983398
		-1.29291844367981 0.125106334686279
		-1.30612921714783 0.0532190799713135
		-1.31215310096741 0.0165433883666992
		-1.31711959838867 -0.0196654796600342
		-1.32039380073547 -0.0553371906280518
		-1.32277178764343 -0.0898569822311401
		-1.32500529289246 -0.158437490463257
		-1.32609105110168 -0.19228720664978
		-1.32651877403259 -0.258758544921875
		-1.32579970359802 -0.292041420936584
		-1.31922578811646 -0.356620788574219
		-1.30942845344543 -0.419981241226196
		-1.30443930625916 -0.453237771987915
		-1.29669737815857 -0.483376026153564
		-1.27771997451782 -0.536915302276611
		-1.26819586753845 -0.562709093093872
		-1.25748014450073 -0.587427616119385
		-1.24508428573608 -0.610039234161377
		-1.23216128349304 -0.631744027137756
		-1.21963357925415 -0.653706908226013
		-1.20684671401978 -0.676852703094482
		-1.19270896911621 -0.701040267944336
		-1.17677235603333 -0.725752234458923
		-1.15970468521118 -0.751201272010803
		-1.14170575141907 -0.777201175689697
		-1.10406303405762 -0.832702994346619
		-1.08358836174011 -0.8623126745224
		-1.06120085716248 -0.893404960632324
		-1.03935527801514 -0.921954274177551
		-1.01832628250122 -0.950077176094055
		-0.997435569763184 -0.979643583297729
		-0.97650933265686 -1.01081764698029
		-0.954917192459106 -1.04151690006256
		-0.932660102844238 -1.07052993774414
		-0.909939527511597 -1.09875893592834
		-0.886212825775146 -1.12652593851089
		-0.862452268600464 -1.15353900194168
		-0.815754652023315 -1.2038522362709
		-0.792101383209229 -1.22816842794418
		-0.767385959625244 -1.25185036659241
		-0.742187976837158 -1.2749205827713
		-0.716208934783936 -1.2957581281662
		-0.689436674118042 -1.31554001569748
		-0.660673379898071 -1.33487033843994
		-0.630569219589233 -1.35101294517517
		-0.600506544113159 -1.36599403619766
		-0.544595241546631 -1.39070624113083
		-0.488700866699219 -1.41589421033859
		-0.462868690490723 -1.42462944984436
		-0.437064647674561 -1.43352478742599
		-0.407913684844971 -1.44261866807938
		-0.379749774932861 -1.45121031999588
		1.33056688308716 -1.01596760749817
		1.35563373565674 -0.992703557014465
		1.40142488479614 -0.947503924369812
		1.56949138641357 -0.693477153778076
		1.59641218185425 -0.615870952606201
		1.45703172683716 1.19138956069946
		1.44387340545654 1.2247428894043
		-0.289704322814941 2.70656037330627
		-0.320497512817383 2.71177887916565
		-0.385273933410645 2.71884107589722
		-0.516458511352539 2.70517754554749
		-0.564927101135254 2.69101142883301
		-0.590946674346924 2.68302369117737
		-0.617502689361572 2.67279672622681
		-0.675025939941406 2.65035390853882
		-0.704952478408813 2.63782215118408
		-0.735376119613647 2.62346267700195
		-0.768058300018311 2.60692429542542
		-0.802142143249512 2.58924341201782
		-0.834689855575562 2.5705680847168
		-0.862192630767822 2.55151057243347
		-0.891415357589722 2.5333309173584
		-0.921496391296387 2.51435279846191
		-1.01182007789612 2.46045851707458
		-1.06711292266846 2.42441987991333
		-1.18905401229858 2.34989953041077
		-1.22242474555969 2.33184289932251
		-1.32146668434143 2.27758526802063
		-1.57897305488586 2.04121494293213
		-1.6480188369751 1.94861459732056
		-1.67137670516968 1.91444730758667
		-2.25361108779907 0.874212026596069
		-2.26539397239685 0.797172069549561
		-2.27581930160522 0.715568065643311
		-2.2820155620575 0.671371698379517
		-2.28688764572144 0.62915563583374
		-2.29258489608765 0.587712049484253
		-2.30083727836609 0.545308113098145
		-2.30962038040161 0.50223970413208
		-2.31872916221619 0.459707975387573
		-2.32791781425476 0.418349027633667
		-2.33625292778015 0.378353118896484
		-2.34445548057556 0.338964462280273
		-2.35341095924377 0.299217224121094
		-2.36205077171326 0.259202718734741
		-2.37082481384277 0.219289779663086
		-2.38751935958862 0.138083457946777
		-2.39563727378845 0.0995147228240967
		-2.4016592502594 0.0617759227752686
		-2.40769982337952 0.0250015258789062
		-2.41449761390686 -0.0468127727508545
		-2.41528987884521 -0.0820958614349365
		-2.41299533843994 -0.151818990707397
		-2.41100978851318 -0.184613704681396
		-2.40664196014404 -0.218201398849487
		-2.40203356742859 -0.251810908317566
		-2.3967866897583 -0.287399172782898
		-2.39388537406921 -0.322534918785095
		-2.38806486129761 -0.360974788665771
		-2.381267786026 -0.401355266571045
		-2.37408089637756 -0.443756341934204
		-2.36215329170227 -0.531498074531555
		-2.35752153396606 -0.576264142990112
		-2.35336685180664 -0.622230052947998
		-2.34855937957764 -0.667589902877808
		-2.34447503089905 -0.711048364639282
		-2.3418447971344 -0.755615472793579
		-2.3410120010376 -0.799931645393372
		-2.33989763259888 -0.843094706535339
		-2.33670544624329 -0.885925650596619
		-2.33290004730225 -0.928900361061096
		-2.32806205749512 -0.971526503562927
		-2.32050442695618 -1.01427781581879
		-2.31167984008789 -1.05693066120148
		-2.30255722999573 -1.09987038373947
		-2.29243230819702 -1.14463686943054
		-2.28236293792725 -1.19041496515274
		-2.26996302604675 -1.23702794313431
		-2.25768184661865 -1.28114533424377
		-2.24549078941345 -1.32466202974319
		-2.23391342163086 -1.36858493089676
		-2.22111892700195 -1.4110643863678
		-2.20887303352356 -1.45023894309998
		-2.19683218002319 -1.48708492517471
		-2.18462538719177 -1.52269667387009
		-2.17144393920898 -1.55671948194504
		-2.15778207778931 -1.58942127227783
		-2.12607502937317 -1.65824967622757
		-2.10942792892456 -1.69390663504601
		-2.0724835395813 -1.76860895752907
		-2.05078744888306 -1.80741992592812
		-2.0277144908905 -1.84598053991795
		-2.00400161743164 -1.88384968042374
		-1.97906064987183 -1.92237174510956
		-1.95275402069092 -1.96187348663807
		-1.92724633216858 -1.9982313066721
		-1.90249633789062 -2.0328359156847
		-1.87849926948547 -2.06690534064546
		-1.85164165496826 -2.10034058988094
		-1.82491588592529 -2.13212168961763
		-1.79769921302795 -2.16205789893866
		-1.76935219764709 -2.19062901288271
		-1.74066495895386 -2.21796932816505
		-1.7110493183136 -2.24473166465759
		-1.68170881271362 -2.27094706892967
		-1.65143728256226 -2.2974946051836
		-1.62045001983643 -2.32440593838692
		-1.56005930900574 -2.37272024154663
		-1.52983593940735 -2.39586943387985
		-1.49762749671936 -2.41797864437103
		-1.46767425537109 -2.43602341413498
		-1.44050121307373 -2.45182201266289
		-1.41324687004089 -2.46686562895775
		-1.38416886329651 -2.48116624355316
		-1.32497119903564 -2.50404217839241
		-1.29381799697876 -2.51406338810921
		-1.26369762420654 -2.52342221140862
		-1.23093128204346 -2.53150218725204
		-1.16138768196106 -2.54533371329308
		-1.12258219718933 -2.55138838291168
		-0.997140645980835 -2.57278525829315
		-0.909528970718384 -2.58448070287704
		-0.866600275039673 -2.58940428495407
		-0.825949192047119 -2.59541898965836
		-0.400846004486084 -2.59659290313721
		-0.362374782562256 -2.58049273490906
		-0.323870658874512 -2.558499366045
		-0.285403728485107 -2.54078635573387
		-0.217128753662109 -2.51330947875977
		-0.185720443725586 -2.50488662719727
		-0.153455257415771 -2.49865132570267
		-0.122417449951172 -2.49272155761719
		-0.0640659332275391 -2.46941301226616
		0.0270724296569824 -2.4031730890274
		0.0581064224243164 -2.3757598400116
		0.14694881439209 -2.28924432396889
		0.177852153778076 -2.2608225941658
		0.208495616912842 -2.23119166493416
		0.238874435424805 -2.20432397723198
		0.298620223999023 -2.16592083126307
		0.32868480682373 -2.14919875562191
		0.358621120452881 -2.13479162752628
		0.387324810028076 -2.12533460184932
		0.416624546051025 -2.11850539594889
		0.479402542114258 -2.10795144736767
		0.53981351852417 -2.10506253316998
		0.568412780761719 -2.10404275357723
		0.659700870513916 -2.10751416534185
		0.687624931335449 -2.11187508702278
		1.29006958007812 -1.94416399300098
		1.3372368812561 -1.90888941287994
		1.53340673446655 -1.76066148281097
		1.58145189285278 -1.7212016582489
		1.60648584365845 -1.70230749249458
		1.62718296051025 -1.68331179022789
		1.66561460494995 -1.64850580692291
		1.68503618240356 -1.6324103474617
		1.70443201065063 -1.61509642004967
		1.738356590271 -1.57982692122459
		1.75437068939209 -1.55862414836884
		1.78147220611572 -1.51620477437973
		1.80657052993774 -1.4696056842804
		1.82488775253296 -1.41984003782272
		1.8410325050354 -1.36351543664932
		1.85570526123047 -1.30703413486481
		1.86887216567993 -1.25146263837814
		1.88799953460693 -1.16520243883133
		1.89627361297607 -1.13632905483246
		1.90449810028076 -1.10646677017212
		1.98875761032104 -0.761571168899536
		2.00995397567749 -0.719612121582031
		2.01883268356323 -0.697352886199951
		2.04478597640991 -0.574985146522522
		1.95436954498291 0.222334861755371
		1.95725011825562 0.255880117416382
		1.96000528335571 0.288040637969971
		1.9628849029541 0.320069789886475
		1.96722936630249 0.352580308914185
		1.97021436691284 0.385518312454224
		1.97024583816528 0.417383432388306
		1.96860265731812 0.447250366210938
		1.96731233596802 0.50609302520752
		1.9672679901123 0.536402940750122
		1.96639776229858 0.567726850509644
		1.96342992782593 0.600409984588623
		1.95831918716431 0.63367748260498
		1.95049524307251 0.66839075088501
		1.94130754470825 0.703469276428223
		1.93104839324951 0.739678859710693
		1.92077827453613 0.776458978652954
		1.91051340103149 0.813912630081177
		1.89012098312378 0.888729333877563
		1.88151359558105 0.927408933639526
		1.86127424240112 1.00381898880005
		1.85330247879028 1.04165196418762
		1.84587144851685 1.08209729194641
		1.83908987045288 1.12314629554749
		1.82439613342285 1.20593571662903
		1.81831645965576 1.24764490127563
		1.81271696090698 1.29049825668335
		1.80806350708008 1.33366131782532
		1.80342531204224 1.37706303596497
		1.79928922653198 1.42026662826538
		1.7971453666687 1.46274161338806
		1.79433917999268 1.50360155105591
		1.79073858261108 1.54185962677002
		1.78850507736206 1.57890057563782
		1.78533029556274 1.61689305305481
		1.77936553955078 1.65458941459656
		1.77215480804443 1.69134116172791
		1.76421213150024 1.72705721855164
		1.74704170227051 1.79564142227173
		1.73746633529663 1.82906007766724
		1.72739744186401 1.86128783226013
		1.71561241149902 1.89452505111694
		1.70328283309937 1.92758560180664
		1.67693424224854 2.00393080711365
		1.66645002365112 2.04511189460754
		1.65657567977905 2.08444046974182
		1.64457130432129 2.12453842163086
		1.62269878387451 2.21275925636292
		1.61720418930054 2.25856971740723
		1.61373615264893 2.30315804481506
		1.60957717895508 2.34642052650452
		1.60499095916748 2.38978672027588
		1.59963417053223 2.43225789070129
		1.58933258056641 2.51898574829102
		1.58644485473633 2.55997228622437
		1.58502817153931 2.60557079315186
		1.58406448364258 2.64927816390991
		1.58242988586426 2.68812775611877
		1.5798716545105 2.72636914253235
		1.51393747329712 3.02699828147888
		-0.0877523422241211 4.18661904335022
		-0.124678611755371 4.20443820953369
		-0.160244941711426 4.22027730941772
		-0.193114280700684 4.23818707466125
		-0.227484703063965 4.25466060638428
		-0.260913372039795 4.27157402038574
		-0.403662204742432 4.3402111530304
		-0.442275047302246 4.3545069694519
		-0.485790252685547 4.36636924743652
		-0.527101516723633 4.38018202781677
		-0.565081596374512 4.39249134063721
		-0.601755142211914 4.40324831008911
		-0.63889741897583 4.40784955024719
		-0.676595449447632 4.41289401054382
		-0.714593648910522 4.41830611228943
		-0.753582239151001 4.42287635803223
		-0.788907051086426 4.42795085906982
		-0.826500177383423 4.42929124832153
		-0.863492012023926 4.43156766891479
		-0.901363134384155 4.43281126022339
		-1.14219951629639 4.434246301651
		-1.17949223518372 4.43559050559998
		-1.21873140335083 4.43601393699646
		-1.29791688919067 4.44250535964966
		-1.33931136131287 4.44604587554932
		-1.37961959838867 4.45002579689026
		-1.41981768608093 4.45318055152893
		-1.4564642906189 4.46156072616577
		-2.13085269927979 4.43182468414307
		-2.35638403892517 4.34141278266907
		-2.49751377105713 4.28180313110352
		-2.52496933937073 4.26759099960327
		-2.75772988796234 4.20397353172302
		-3.40758538246155 4.2420494556427
		-3.49682247638702 4.22978472709656
		-3.56490099430084 4.21172451972961
		-3.72223800420761 4.16917896270752
		-4.54988226667047 2.65141105651855
		-4.55744732171297 2.61663150787354
		-4.63490474969149 2.03544211387634
		-4.64186987280846 1.99602842330933
		-4.64891293272376 1.95807123184204
		-4.65664889663458 1.91834759712219
		-4.66422605514526 1.87747669219971
		-4.6764026209712 1.79753565788269
		-4.65569248050451 1.45130395889282
		-4.63563089817762 1.38606834411621
		-4.62575577571988 1.35111546516418
		-4.61396354995668 1.31347155570984
		-4.59036883898079 1.23333811759949
		-4.57641697302461 1.19529986381531
		-4.56173906847835 1.15940880775452
		-4.54857661575079 1.12266421318054
		-4.5343305580318 1.08709383010864
		-4.519834831357 1.04947829246521
		-4.50518117845058 1.0110936164856
		-4.47888568043709 0.937682628631592
		-4.46760940551758 0.901084899902344
		-4.44034348428249 0.82365870475769
		-4.42624649405479 0.784178733825684
		-4.41335700452328 0.744888067245483
		-4.3994043469429 0.707567691802979
		-4.38476076722145 0.669619083404541
		-4.36960543692112 0.633818387985229
		-4.35243183374405 0.597996234893799
		-4.31775832176208 0.528888463973999
		-4.29749092459679 0.496784925460815
		-4.27538186311722 0.467316627502441
		-4.2514223754406 0.437769174575806
		-4.22524318099022 0.409273862838745
		-4.20040947198868 0.382643699645996
		-4.17372596263885 0.356757879257202
		-4.14584773778915 0.331774711608887
		-4.11631852388382 0.307438611984253
		-4.08704447746277 0.284059524536133
		-4.05589020252228 0.260846138000488
		-4.02274340391159 0.23731255531311
		-3.98701959848404 0.213740110397339
		-3.94924908876419 0.191959857940674
		-3.90749990940094 0.173275947570801
		-3.8671846985817 0.152487993240356
		-3.83298647403717 0.129753351211548
		-3.79806685447693 0.10661244392395
		-3.76082342863083 0.083491325378418
		-3.72200465202332 0.0617899894714355
		-3.68550968170166 0.0395750999450684
		-3.57727706432343 -0.0289900302886963
		-3.53887224197388 -0.0535352230072021
		-3.46355807781219 -0.103548049926758
		-3.39046704769135 -0.151049137115479
		-3.17591059207916 -0.248821377754211
		-3.13769257068634 -0.257687568664551
		-3.10141944885254 -0.270267963409424
		-3.02755010128021 -0.2863529920578
		-2.99115383625031 -0.295754790306091
		-2.95299530029297 -0.305933475494385
		-2.91587340831757 -0.315494656562805
		-2.87696957588196 -0.3264000415802
		-2.83641052246094 -0.33561098575592
		-2.79450595378876 -0.342979073524475
		-2.750812292099 -0.348366618156433
		-2.7033611536026 -0.352126240730286
		-2.65276038646698 -0.359118103981018
		-2.60619187355042 -0.370252013206482
		-2.52297878265381 -0.394192695617676
		-2.48068761825562 -0.408087491989136
		-2.39927768707275 -0.437232136726379
		-2.35953903198242 -0.452861189842224
		-2.2826828956604 -0.48480212688446
		-2.24623084068298 -0.501744389533997
		-2.13670492172241 -0.556227326393127
		-2.09651327133179 -0.573573231697083
		-1.84740424156189 -0.653395175933838
		-1.81103944778442 -0.660107612609863
		-1.77560305595398 -0.666983246803284
		-1.70212602615356 -0.673930525779724
		-1.6637749671936 -0.676748394966125
		-1.62431788444519 -0.679673433303833
		-1.58258247375488 -0.683019280433655
		-1.54093384742737 -0.685417771339417
		-1.49897861480713 -0.687060475349426
		-1.45732927322388 -0.687062859535217
		-1.41757106781006 -0.687598347663879
		-1.37885236740112 -0.687753558158875
		-1.33969712257385 -0.688208699226379
		-1.29980087280273 -0.689888477325439
		-1.25923156738281 -0.695621013641357
		-1.14369940757751 -0.710853457450867
		-1.10503554344177 -0.715830206871033
		-1.06684923171997 -0.722302079200745
		-1.02712726593018 -0.731185913085938
		-0.986946821212769 -0.738367915153503
		-0.946746826171875 -0.746049523353577
		-0.742647171020508 -0.769329071044922
		-0.671017408370972 -0.767243385314941
		0.141541004180908 -0.473962426185608
		0.206554412841797 -0.434712052345276
		0.336203575134277 -0.333460092544556
		0.355794429779053 -0.307351350784302
		0.429826259613037 -0.0840921401977539
		0.430779457092285 -0.0549068450927734
		0.432490825653076 0.00406193733215332
		0.436112403869629 0.0328750610351562
		0.44124174118042 0.0915300846099854
		0.446651935577393 0.148282766342163
		0.449906349182129 0.205270528793335
		0.452280521392822 0.234741449356079
		0.452969074249268 0.265023231506348
		0.454581260681152 0.323949813842773
		0.457813262939453 0.382885694503784
		0.458809375762939 0.414554119110107
		0.453404903411865 0.480981588363647
		0.308011054992676 0.755092859268188
		0.28810977935791 0.766688108444214
		0.266928672790527 0.777087450027466
		0.243512630462646 0.787376403808594
		0.192546844482422 0.805432796478271
		0.171152114868164 0.816164255142212
		0.15043830871582 0.828520536422729
		0.128088474273682 0.839929819107056
		0.0829334259033203 0.86394476890564
		0.0598263740539551 0.876285076141357
		-0.645771265029907 0.425600290298462
		-0.64622688293457 0.41634202003479
		-0.616232395172119 0.429705142974854
		-0.608434677124023 0.43577241897583
		-0.597229957580566 0.443042755126953
		-0.554276466369629 0.469800472259521
		-0.538060188293457 0.478265523910522
		-0.522171497344971 0.486138343811035
		-0.468228340148926 0.509299516677856
		-0.44761848449707 0.516604423522949
		-0.405308246612549 0.534150123596191
		-0.383967399597168 0.543862342834473
		-0.344911098480225 0.559716463088989
		-0.327674388885498 0.564679384231567
		-0.310309886932373 0.568539619445801
		-0.295854568481445 0.574695825576782
		-0.280683994293213 0.58046293258667
		-0.254661560058594 0.58939528465271
		-0.243091106414795 0.594078540802002
		-0.233814716339111 0.596724987030029
		-0.226614952087402 0.598632097244263
		-0.219466686248779 0.599214315414429
		-0.177406311035156 0.608280420303345
		-0.168651580810547 0.615051507949829
		-0.145305633544922 0.646092891693115
		-0.143763542175293 0.652109622955322
		-0.143428325653076 0.658360481262207
		-0.143693447113037 0.663336038589478
		-0.144739627838135 0.667201280593872
		-0.147010326385498 0.671627521514893
		-0.155972957611084 0.652511835098267
		-0.155232906341553 0.646515846252441
		-0.154995441436768 0.645752429962158
		-0.160358905792236 0.642080307006836
		-0.164155960083008 0.644567012786865
		-0.173178672790527 0.648711442947388
		-0.169086456298828 0.660304307937622
	};
\addlegendentry{MOCAP}
\addplot [draw=darkorange25512714, fill=darkorange25512714, mark=*, mark size=0.5, only marks]
table{%
		x  y
		-0.233598 0.142923
		-0.155847 0.127126
		-0.159678 0.122278
		-0.158696 0.123551
		-0.238245 0.14381
		-0.234133 0.150413
		-0.160663 0.120982
		-0.209633 0.170522
		-0.235626 0.129613
		-0.248505 0.136027
		-0.265987 0.138994
		-0.320831 0.150172
		-0.260761 0.125992
		-0.258569 0.1338
		-0.300576 0.146636
		-0.262557 0.132958
		-0.202316 0.131754
		-0.250735 0.147295
		-0.187544 0.13417
		-0.171913 0.163188
		-0.169223 0.165977
		-0.197427 0.138973
		-0.194332 0.143269
		-0.239527 0.141665
		-0.197991 0.138169
		-0.181346 0.111757
		-0.230115 0.139163
		-0.246108 0.14557
		-0.260026 0.134301
		-0.253633 0.139112
		-0.244407 0.132792
		-0.255068 0.122644
		-0.343221 0.116181
		-0.249247 0.121007
		-0.25688 0.122983
		-0.328805 0.106945
		-0.265585 0.123552
		-0.253691 0.125467
		-0.276032 0.123425
		-0.253001 0.123395
		-0.355145 0.156299
		-0.393158 0.124249
		-0.386988 0.159492
		-0.460709 0.14322
		-0.440341 0.128924
		-0.657503 0.204548
		-0.707248 0.162496
		-0.634471 0.191759
		-0.599427 0.16444
		-0.530434 0.117255
		-0.503083 0.0542511999999999
		-0.515868 0.0462122
		-0.492413 0.0383081000000001
		-0.492256 0.0402704
		-0.561289 0.0270317
		-0.561878 -0.00832611000000005
		-0.564651 0.0126455999999999
		-0.631059 0.177994
		-0.651161 0.167262
		-0.640668 0.0487465
		-0.669869 -0.0203873000000001
		-0.647414 0.193899
		-0.694 -0.0292675
		-0.653333 -0.0372825999999999
		-0.599263 0.0428222
		-0.561151 0.0297729
		-0.565444 -0.0149431
		-0.599801 -0.0295504
		-0.647563 -0.0606557999999999
		-0.644133 -0.0620428
		-0.610607 -0.0628668000000001
		-0.523543 -0.0346518
		-0.536319 -0.049302
		-0.521274 -0.0456628000000001
		-0.500235 -0.102932
		-0.463405 -0.102045
		-0.406081 -0.0818209999999999
		-0.555166 -0.106608
		-0.594595 -0.124042
		-0.515147 -0.123187
		-0.576808 -0.168049
		-0.500336 -0.133456
		-0.607967 -0.161559
		-0.616049 -0.178118
		-0.612604 -0.250899
		-0.474349 -0.217117
		-0.476837 -0.282235
		-0.386502 -0.235622
		-0.235276 -0.116846
		-0.281465 -0.173413
		-0.23185 -0.120173
		-0.217181 -0.109818
		-0.1674 -0.0945096000000001
		-0.232429 -0.173229
		-0.203772 -0.150458
		-0.268947 -0.259629
		-0.315192 -0.324757
		-0.292108 -0.324368
		-0.292108 -0.324368
		-0.319633 -0.365034
		-0.322489 -0.339469
		-0.323994 -0.338032
		-0.378765 -0.412284
		-0.364342 -0.39823
		-0.364342 -0.39823
		-0.32678 -0.37378
		-0.293322 -0.298345
		-0.253028 -0.247871
		-0.228615 -0.248392
		-0.322164 -0.480925
		-0.322164 -0.480925
		-0.260178 -0.466906
		-0.222963 -0.435827
		-0.20974 -0.445324
		-0.231802 -0.512868
		-0.210457 -0.505284
		-0.102555 -0.379358
		-0.0480361 -0.387099
		-0.0371642999999999 -0.418148
		-0.0408256 -0.393723
		-0.0509162000000001 -0.627246
		-0.0480830999999999 -0.564521
		-0.0929131000000001 -0.375968
		-0.16761 -0.416794
		-0.0871782999999999 -0.389476
		-0.0331703999999999 -0.424965
		-0.00638359999999993 -0.42621
		0.0187805000000001 -0.41642
		0.0343487 -0.415426
		0.0252026000000001 -0.447055
		0.0422832 -0.398818
		0.0641273 -0.360848
		0.0703560000000001 -0.356307
		0.155261 -0.403724
		0.177035 -0.4236
		0.173007 -0.409716
		0.19768 -0.459313
		0.261577 -0.455077
		0.202645 -0.412293
		0.179326 -0.454856
		0.0837950000000001 -0.405212
		0.0713301 -0.406457
		0.0559601000000001 -0.446169
		0.0582742999999999 -0.45265
		0.0366073 -0.421918
		0.0340311 -0.375883
		0.0356897 -0.412877
		0.0461241999999999 -0.383517
		0.0513498999999999 -0.41403
		0.0879211 -0.455289
		0.0874488 -0.392225
		0.191275 -0.404266
		0.240585 -0.337621
		0.253498 -0.343278
		0.234306 -0.31901
		0.263957 -0.335484
		0.287328 -0.366475
		0.3393 -0.436995
		0.280966 -0.368568
		0.257933 -0.336553
		-0.233412 0.219822
		0.289323 -0.419511
		0.338807 -0.456493
		0.307767 -0.424194
		0.300561 -0.40878
		0.264174 -0.388951
		0.297139 -0.393963
		0.237109 -0.370986
		0.278454 -0.371679
		0.228002 -0.292476
		0.334846 -0.44572
		0.343153 -0.461172
		0.293523 -0.434629
		0.268081 -0.396134
		0.251878 -0.352949
		0.330254 -0.378069
		0.282276 -0.284577
		0.33128 -0.254433
		0.215412 -0.216204
		0.474625 -0.314209
		0.181823 -0.171912
		0.319577 -0.209481
		0.376113 -0.248017
		0.378229 -0.25392
		0.352564 -0.221547
		0.353375 -0.279335
		1.0801 -0.3217
		0.319571 -0.240339
		0.312475 -0.206874
		0.744418 -0.273727
		0.490516 -0.295169
		0.506238 -0.303881
		0.514899 -0.364933
		0.536347 -0.315058
		0.496705 -0.230419
		0.415863 -0.241406
		0.411114 -0.197066
		0.480105 -0.230137
		0.518861 -0.252663
		0.412013 -0.195179
		0.317285 -0.177438
		0.331503 -0.192217
		0.488772 -0.246396
		0.481491 -0.227222
		0.512875 -0.236486
		0.508409 -0.242771
		0.40618 -0.20781
		0.501835 -0.219987
		0.513269 -0.127891
		0.384916 -0.0876402000000001
		0.426417 -0.124147
		0.364334 -0.0758683
		0.333115 -0.151492
		0.399838 -0.114485
		0.377954 -0.0778844999999999
		0.411609 -0.0928823999999999
		0.360872 -0.0471444000000001
		0.360405 -0.0186922
		0.368902 -0.0301791
		0.357349 -0.0132882000000001
		0.360642 -0.0133604000000001
		0.248603 0.0147356000000001
		0.321936 0.0131684000000001
		0.48655 0.0398035999999999
		0.466519 0.0311087999999999
		0.406126 0.0105317
		0.386174 -0.0295996000000001
		0.341595 -0.0298130999999999
		0.48739 -0.0141792000000001
		0.290192 -0.0289102000000001
		0.56877 -0.00803693000000005
		0.507484 0.00717097999999994
		0.558111 0.00783043000000005
		0.491209 -0.0223982
		0.566755 0.0298189
		0.536399 0.0262472
		0.60921 0.0509229
		0.357508 0.0478206999999999
		0.490259 0.0687845
		0.455817 0.0660191999999999
		0.394444 0.0713189000000001
		0.457639 0.0579927
		0.500998 0.122093
		0.474152 0.114308
		0.345806 0.0867335
		0.373 0.0962466
		0.371048 0.103517
		0.468098 0.133265
		0.470827 0.123276
		0.47653 0.12523
		0.448048 0.169941
		0.528532 0.204398
		0.744448 0.352779
		0.568154 0.243595
		0.590416 0.256605
		0.232968 0.0904673
		0.368331 0.150662
		0.445892 0.238131
		0.446997 0.23704
		0.47631 0.287502
		0.330057 0.205506
		0.422029 0.280576
		0.262355 0.160849
		0.295673 0.182328
		0.330614 0.176844
		0.310093 0.222577
		0.270971 0.197684
		0.25307 0.199329
		0.246907 0.188303
		0.166667 0.140749
		0.362529 0.294615
		0.256976 0.247983
		0.208322 0.199021
		0.257815 0.253744
		0.232262 0.222704
		0.197043 0.182845
		0.197043 0.182845
		0.199084 0.184056
		0.183439 0.160368
		0.144985 0.128122
		0.194234 0.162865
		0.158774 0.127995
		0.158774 0.127995
		0.152322 0.124431
		0.176876 0.144183
		0.145552 0.122374
		0.14478 0.135086
		0.114026 0.103975
		0.116986 0.105361
		0.116986 0.105361
		0.200711 0.221691
		0.173391 0.185642
		0.176021 0.217383
		0.191589 0.247035
		0.186162 0.326741
		0.271618 0.521916
		0.11791 0.260171
		0.11791 0.260171
		0.124194 0.274879
		0.0915629 0.279046
		0.0915629 0.279046
		0.0701678999999999 0.230345
		0.0495475999999999 0.165123
		0.0279323 0.123447
		0.0285945000000001 0.216168
		-0.0160372 0.331535
		-0.0441726 0.230786
		-0.119088 0.392646
		-0.140385 0.315588
		-0.119906 0.210493
		-0.210482 0.209344
		-0.248878 0.215718
		-0.280694 0.229537
		-0.241675 0.199401
		-0.317634 0.276419
		-0.263889 0.214811
		-0.340407 0.249764
		-0.385204 0.216446
		-0.327982 0.17282
		-0.322019 0.158525
		-0.343888 0.159252
		-0.348291 0.155028
		-0.42066 0.138696
		-0.372212 0.10496
		-0.383712 0.0957104
		-0.391182 0.0876380999999999
		-0.340604 0.0525964000000001
		-0.335782 0.0406405999999999
		-0.422898 0.0315038999999999
		-0.440403 0.0144005
		-0.493375 -0.0181492000000001
		-0.577517 -0.0517171999999999
		-0.614073 -0.113415
		-0.586378 -0.166751
		-0.609864 -0.261064
		-0.641268 -0.315799
		-0.649031 -0.336013
		-0.577054 -0.323362
		-0.676517 -0.394485
		-0.693223 -0.412626
		-0.682134 -0.458931
		-0.661432 -0.466891
		-0.577209 -0.434749
		-0.573437 -0.439713
		-0.589854 -0.483501
		-0.490858 -0.411346
		-0.552487 -0.492349
		-0.55889 -0.525979
		-0.582058 -0.625257
		-0.550998 -0.715533
		-0.581012 -0.79205
		-0.577126 -0.831707
		-0.377833 -0.928873
		-0.350575 -0.962825
		-0.304502 -0.969691
		-0.189735 -0.970845
		-0.128075 -0.980886
		-0.0495585999999999 -0.962891
		0.460911 -0.911802
		0.510836 -0.960805
		0.523272 -0.910362
		0.524725 -0.810343
		0.671745 -0.755509
		1.00235 -0.615106
		0.385628 0.911396
		-0.314026 0.917878
		-0.405152 0.946212
		-0.433129 0.933737
		-0.500094 0.977632
		-0.5016 0.929351
		-0.490058 0.871819
		-0.551174 0.857708
		-0.533462 0.834049
		-0.579056 0.864479
		-0.612776 0.877949
		-0.631097 0.858778
		-0.645441 0.852423
		-0.674166 0.853266
		-0.681789 0.791362
		-0.676805 0.73974
		-0.713472 0.725785
		-0.89106 0.805941
		-0.797056 0.746157
		-0.83553 0.729007
		-0.934983 0.756671
		-1.02987 0.783595
		-0.985615 0.739438
		-1.00029 0.73275
		-1.07169 0.749038
		-1.08549 0.708458
		-1.10329 0.680404
		-1.02329 0.589768
		-1.03626 0.565922
		-1.01611 0.519598
		-1.05603 0.528101
		-1.08848 0.522373
		-1.03807 0.477662
		-1.10125 0.485438
		-1.13362 0.459811
		-1.17076 0.419218
		-0.216138 0.216088
		-1.26467 0.279927
		-1.26962 0.260892
		-1.26679 0.189719
		-1.24642 0.177985
		-1.22163 0.146848
		-1.21048 0.119321
		-1.33104 0.0856673999999999
		-1.31556 0.0402452
		-1.33362 0
		-1.27686 -0.0303811
		-1.38444 -0.0656557
		-1.25837 -0.0934579
		-1.29619 -0.131723
		-1.39012 -0.288233
		-1.32132 -0.322202
		-1.23941 -0.367356
		-1.20877 -0.47658
		-1.18605 -0.48161
		-1.19662 -0.528847
		-1.14426 -0.537411
		-1.22238 -0.628905
		-1.02396 -0.554825
		-1.05893 -0.621416
		-1.13936 -0.701703
		-1.13202 -0.727813
		-1.06706 -0.766061
		-1.06706 -0.766061
		-1.1226 -0.860561
		-1.1044 -0.908758
		-1.18843 -1.03968
		-1.18843 -1.03968
		-0.978945 -0.941775
		-1.1084 -1.10143
		-1.1084 -1.10143
		-1.10475 -1.1864
		-1.06233 -1.19223
		-1.06233 -1.19223
		-0.986547 -1.19649
		-0.990135 -1.25339
		-0.98264 -1.38695
		-0.99052 -1.50776
		-0.865025 -1.51552
		-0.876944 -1.551
		-0.772228 -1.47926
		-0.771621 -1.58259
		1.19022 -1.52142
		1.40371 -1.77806
		1.30768 -1.55847
		1.24478 -0.949681
		1.2563 -0.890952
		1.5941 0.86579
		1.6221 0.892669
		0.116072 2.67343
		0.0863476000000001 2.55451
		-0.00829327999999996 2.69055
		-0.191338 2.71544
		-0.233549 2.71437
		-0.257376 2.70181
		-0.299156 2.70424
		-0.350814 2.70991
		-0.456347 2.72504
		-0.467441 2.67508
		-0.504752 2.66002
		-0.542101 2.67279
		-0.562951 2.68443
		-0.598226 2.67526
		-0.644345 2.68354
		-0.660342 2.67965
		-0.635774 2.54729
		-0.706898 2.65535
		-0.691308 2.43554
		-0.856972 2.55112
		-0.906552 2.46592
		-0.995707 2.53608
		-1.12586 2.20526
		-1.30375 1.91049
		-1.36672 1.93025
		-1.37006 1.71654
		-2.16352 1.1423
		-2.23862 1.08515
		-2.19752 1.02584
		-2.51377 1.02383
		-2.41527 0.89491
		-2.50502 0.852745
		-2.50502 0.852745
		-2.54559 0.836601
		-2.492 0.758435
		-2.53104 0.719864
		-2.52909 0.637199
		-2.50986 0.607025
		-2.61204 0.571461
		-2.59478 0.542011
		-2.5906 0.42576
		-2.5906 0.42576
		-2.48638 0.194948
		-2.55243 0.146247
		-2.33749 0.0919175000000001
		-2.45295 0.0588192000000001
		-2.61733 0.0313805
		-2.5566 -0.00763986999999999
		-2.62971 -0.0781118000000001
		-2.56322 -0.14466
		-2.5469 -0.1897
		-2.62285 -0.235137
		-2.67735 -0.280027
		-2.67735 -0.280027
		-2.66477 -0.328474
		-2.57358 -0.380288
		-2.50929 -0.420034
		-2.54521 -0.489523
		-2.50663 -0.514299
		-2.41926 -0.533416
		-2.40904 -0.562413
		-2.47166 -0.645365
		-2.4577 -0.681586
		-2.53823 -0.738424
		-2.40651 -0.729583
		-2.50749 -0.813828
		-2.47957 -0.922615
		-2.52978 -0.963024
		-2.36958 -0.962908
		-2.48175 -1.06902
		-2.43782 -1.09606
		-2.51279 -1.21046
		-2.4869 -1.24612
		-2.69129 -1.37998
		-2.65956 -1.39947
		-2.8497 -1.54268
		-2.68031 -1.50982
		-2.43474 -1.44169
		-2.36913 -1.43652
		-2.33505 -1.45748
		-2.04801 -1.32237
		-2.04294 -1.35185
		-2.0974 -1.39999
		-2.03822 -1.42893
		-2.00394 -1.44093
		-2.41991 -1.84325
		-2.28564 -1.82028
		-2.27985 -1.88915
		-2.23255 -1.888
		-2.14086 -1.86315
		-2.39415 -2.13595
		-2.32886 -2.11159
		-2.36469 -2.19809
		-2.29452 -2.1685
		-2.27431 -2.18532
		-2.28786 -2.26299
		-2.41109 -2.4951
		-2.25002 -2.38588
		-2.19425 -2.38557
		-2.0954 -2.35077
		-2.18867 -2.49576
		-2.10015 -2.45755
		-2.11208 -2.56828
		-2.19205 -2.6778
		-2.0669 -2.59596
		-2.03173 -2.78565
		-1.95007 -2.74718
		-1.94774 -2.80588
		-1.96589 -2.92187
		-1.85549 -2.86585
		-1.76206 -2.83462
		-1.66962 -2.76482
		-1.54473 -2.81365
		-1.28432 -2.54897
		-1.32003 -2.64572
		-1.26988 -2.62175
		-0.93601 -2.82077
		-0.865875 -2.71906
		-0.855453 -2.86122
		-0.822457 -2.96482
		-0.793776 -3.01278
		-0.703867 -2.90824
		-0.657345 -3.04037
		-0.578784 -2.93293
		-0.542809 -2.9398
		-0.434628 -2.88036
		-0.327662 -2.80887
		-0.271032 -2.8149
		-0.177681 -2.8371
		-0.143934 -2.83901
		-0.0750869999999999 -2.78927
		-0.00853450000000011 -2.8279
		0.091145 -2.7538
		0.119961 -2.83929
		0.127909 -2.81714
		0.142401 -2.92271
		0.177769 -2.77153
		0.265807 -2.81577
		0.350972 -2.71113
		0.398038 -2.46827
		0.513182 -2.45468
		0.561183 -2.45605
		1.35337 -2.59206
		1.40585 -2.46661
		1.52982 -2.26583
		1.59163 -2.3128
		1.43537 -2.09656
		0.770791 -1.25253
		1.75486 -2.39211
		1.68252 -2.21366
		1.22679 -1.78487
		2.20266 -2.52692
		2.2962 -2.57816
		2.15322 -2.38039
		2.23855 -2.46134
		2.22922 -2.42155
		2.2395 -2.29121
		2.34289 -2.34688
		2.2612 -2.2461
		2.34606 -2.30114
		2.48361 -2.42578
		2.40316 -2.2968
		2.28956 -2.1772
		1.852 -1.64495
		2.1767 -1.92731
		1.91307 -1.63949
		1.72879 -1.37944
		1.74554 -1.3443
		2.3806 -1.33058
		1.92795 -1.06016
		2.61059 -1.24329
		2.56344 -1.2123
		2.23932 -0.805446
		2.12332 -0.0330229
		2.9225 -0.0181236
		2.11554 0.113291
		2.1109 0.205481
		2.11431 0.251489
		2.1908 0.254535
		2.18018 0.301223
		2.18018 0.301223
		2.18344 0.379502
		2.12471 0.408275
		2.11307 0.455535
		2.16948 0.48677
		1.89089 0.493143
		1.92807 0.535221
		1.85033 0.58424
		1.92206 0.656653
		1.92206 0.656653
		2.01626 0.772643
		2.29672 0.956127
		2.29672 0.956127
		2.27867 0.993244
		1.73802 0.883113
		1.69534 0.922013
		1.78323 0.981934
		2.16598 1.27795
		2.16988 1.27132
		1.98874 1.22003
		2.07814 1.30282
		2.07155 1.34171
		2.01679 1.35392
		2.01679 1.35392
		2.05751 1.47942
		2.06292 1.58023
		1.98018 1.53416
		1.98018 1.53416
		1.95276 1.58504
		2.03974 1.68131
		-0.218498 0.227869
		1.84972 1.64159
		1.67418 1.52962
		1.69639 1.62361
		1.69639 1.62361
		1.63941 1.63504
		1.56879 1.57105
		1.8085 1.91992
		1.8085 1.91992
		1.77651 1.93446
		1.76032 1.9492
		1.82232 2.02682
		1.8173 2.03131
		1.58507 1.79589
		1.58507 1.79589
		1.57113 1.8072
		1.45936 1.89029
		1.37444 1.79557
		1.55365 2.0765
		1.37266 1.86524
		1.37266 1.86524
		1.22072 1.97997
		0.191886 3.7011
		0.163256 3.74637
		0.14041 3.72851
		0.115034 3.58937
		0.0866313000000001 3.74892
		0.0559805 3.92034
		-0.101025 3.86382
		-0.129853 3.75692
		-0.149581 3.72003
		-0.165545 3.59216
		-0.217843 3.7816
		-0.283655 3.95045
		-0.30748 3.94252
		-0.362062 3.9394
		-0.3815 3.90671
		-0.406868 3.93502
		-0.437367 3.9046
		-0.484107 3.89757
		-0.490128 3.86738
		-0.760247 3.94221
		-0.780025 3.92581
		-0.815332 3.93012
		-0.891155 3.8988
		-0.925062 3.9574
		-0.973757 3.94442
		-0.984673 3.94171
		-0.984673 3.94171
		-1.5937 3.80186
		-1.82271 3.65116
		-1.87497 3.49943
		-2.05501 3.69152
		-2.14617 3.55346
		-2.21013 2.9316
		-2.32797 2.85571
		-2.33677 2.80951
		-2.37837 2.81498
		-3.57578 2.30365
		-3.99563 2.01269
		-4.00455 1.87817
		-3.96279 1.83551
		-3.88481 1.77618
		-3.91776 1.65418
		-4.04525 1.40335
		-4.04525 1.40335
		-3.99847 1.28768
		-4.04638 1.29933
		-4.04638 1.29933
		-4.05502 1.26723
		-4.09404 1.22184
		-4.12426 1.17563
		-4.14535 1.09893
		-4.10448 1.02663
		-4.17373 0.922672
		-4.19041 0.923713
		-4.19586 0.898631
		-4.20944 0.832737
		-4.2611 0.828547
		-4.19295 0.734678
		-3.94721 0.658154
		-3.67172 0.561942
		-3.67326 0.551767
		-3.78128 0.537383
		-4.16508 0.551655
		-4.03942 0.443946
		-3.8621 0.414756
		-3.82635 0.387078
		-3.83137 0.333754
		-3.95124 0.343221
		-3.7981 0.297149
		-3.81176 0.235646
		-3.8141 0.194022
		-3.68289 0.175934
		-3.65897 0.0925362000000001
		-3.52937 0.0395582000000001
		-3.48172 0.0391349999999999
		-3.53253 -0.00998319000000003
		-3.49256 -0.0397078
		-3.58651 -0.0815524000000001
		-3.45831 -0.238655
		-3.45683 -0.259186
		-3.36719 -0.271095
		-2.72886 -0.261981
		-2.70353 -0.291868
		-2.62454 -0.309049
		-2.63315 -0.318763
		-2.62927 -0.349346
		-2.5112 -0.365499
		-2.47196 -0.407516
		-2.37337 -0.407962
		-2.45496 -0.469268
		-2.37303 -0.475207
		-1.71547 -0.379414
		-1.73327 -0.41125
		-1.7778 -0.464503
		-1.76357 -0.471757
		-1.66745 -0.589825
		-1.67568 -0.648572
		-1.56547 -0.627752
		-1.52341 -0.628281
		-1.56721 -0.665883
		-1.50834 -0.663657
		-1.4677 -0.675113
		-1.51089 -0.720738
		-1.52541 -0.765272
		-1.45302 -0.760578
		-1.40331 -0.781422
		-1.38654 -0.785896
		-1.37712 -0.795456
		-1.27956 -0.765276
		-1.13156 -0.732687
		-1.11982 -0.771318
		-1.09109 -0.791733
		-1.05336 -0.778188
		-1.0484 -0.814786
		-1.05767 -0.853925
		-0.822754 -0.806097
		-0.755814 -0.837154
		0.122598 -0.981857
		0.217775 -0.937215
		0.380984 -0.659475
		0.368956 -0.604611
		0.447162 -0.388417
		0.253823 -0.18063
		0.253435 -0.181174
		0.366921 -0.235117
		0.513154 -0.22559
		0.496167 -0.15663
		0.533028 -0.128486
		0.478936 -0.0705556999999999
		0.517566 -0.0477232000000001
		0.469099 -0.0157958
		0.433852 0.044014
		0.42826 0.0661324000000001
		0.47862 0.1108
		0.469313 0.123655
		0.489762 0.150994
		0.416644 0.147309
		0.367457 0.489695
		0.435657 0.597475
		0.381813 0.544209
		0.410303 0.619306
		0.32001 0.526815
		0.343039 0.624227
		0.281865 0.552956
		0.359238 0.764124
		0.342602 0.760187
		0.30972 0.743135
		-0.517277 0.33312
		-0.531628 0.299228
		-0.584764 0.236621
		-0.584764 0.236621
		-0.588857 0.226243
		-0.563958 0.214372
		-0.563958 0.214372
		-0.554063 0.220581
		-0.50192 0.189522
		-0.487924 0.187015
		-0.393915 0.141242
		-0.370797 0.16408
		-0.367453 0.165927
		-0.385412 0.212348
		-0.403144 0.265841
		-0.35861 0.240937
		-0.328185 0.240281
		-0.278717 0.216611
		-0.278717 0.216611
		-0.240707 0.210951
		-0.240707 0.210951
		-0.210212 0.218098
		-0.240897 0.249109
		-0.200168 0.245873
		-0.198665 0.233351
		-0.23254 0.249728
		-0.22891 0.253059
		-0.264547 0.277064
		-0.215971 0.225233
		-0.236466 0.248986
		-0.218319 0.228717
		-0.224626 0.235325
		-0.246019 0.253645
		-0.266016 0.275654
		-0.266364 0.274504
		-0.268663 0.272627
		-0.270075 0.271228
		-0.294567 0.292844
		-0.276608 0.276393
		-0.299246 0.294513
		-0.270757 0.270547
		-1.15177 0.332451
		1.84972 1.64159
	};
\addlegendentry{Prediction}
\addplot [draw=red, mark=o, only marks]
table{%
		x  y
		-0.127206325531006 0.336211204528809
		-0.134419441223145 0.331306219100952
		-0.12944221496582 0.336433887481689
		-0.131443500518799 0.33923602104187
		-0.132200717926025 0.339166402816772
		-0.133244037628174 0.339192628860474
		1.48837184906006 -1.79680702090263
		1.51169395446777 -1.77818402647972
		1.96542549133301 -0.829026818275452
		1.88099431991577 -1.19361960887909
		1.56297874450684 2.88486242294312
		1.45581245422363 3.12256407737732
		1.43606519699097 3.15328907966614
		1.41528272628784 3.18331432342529
		1.3942346572876 3.21430468559265
		1.37285947799683 3.24273252487183
		1.28122186660767 3.35366344451904
		1.2566065788269 3.37853813171387
		1.22669887542725 3.40153908729553
		1.19250440597534 3.42830920219421
		1.13290119171143 3.47973799705505
		1.10378265380859 3.50279903411865
		1.04111480712891 3.55282711982727
		1.00658416748047 3.58054971694946
		0.975536823272705 3.60814118385315
		0.944155216217041 3.63566255569458
		0.913527011871338 3.66178846359253
		0.885063648223877 3.68749570846558
		0.856333255767822 3.71239733695984
		0.826505661010742 3.73820018768311
		0.798305511474609 3.76467323303223
		0.766876220703125 3.79016494750977
		0.736276626586914 3.81562232971191
		0.705400943756104 3.8399498462677
		0.673804759979248 3.86397790908813
		0.61450719833374 3.90927672386169
		0.55016565322876 3.93943738937378
		0.515307903289795 3.95416188240051
		0.481907367706299 3.97110962867737
		0.447263717651367 3.98452091217041
		0.3821120262146 4.01247310638428
		0.348891735076904 4.023517370224
		0.315462589263916 4.03659605979919
		0.281076908111572 4.04957556724548
		0.245109081268311 4.06288051605225
		0.207736968994141 4.07650637626648
		0.169685363769531 4.0901210308075
		0.128819465637207 4.10358047485352
		0.0873255729675293 4.11724829673767
		0.0501694679260254 4.13015222549438
		-0.0149927139282227 4.15698289871216
		-0.0509490966796875 4.17031574249268
		-0.294960021972656 4.28855013847351
		-0.330137252807617 4.30537080764771
		-0.3666090965271 4.32211446762085
		-0.937418699264526 4.43487882614136
		-0.976156234741211 4.4368097782135
		-1.01523780822754 4.43747448921204
		-1.05521440505981 4.43886852264404
		-1.09977555274963 4.43570065498352
		-1.53107452392578 4.47047019004822
		-1.9883930683136 4.47778487205505
		-2.02428364753723 4.4678909778595
		-2.09637141227722 4.44344329833984
		-2.54859137535095 4.26521348953247
		-2.57706809043884 4.25314140319824
		-2.60288333892822 4.24578809738159
		-2.62685918807983 4.238605260849
		-2.65104758739471 4.23094868659973
		-2.70208704471588 4.2170832157135
		-3.4366739988327 4.23933410644531
		-3.46608150005341 4.23578405380249
		-3.64101892709732 4.19075274467468
		-3.83840227127075 4.11388659477234
		-4.56400008313358 2.58181285858154
		-4.5788249084726 2.46781444549561
		-4.58145009726286 2.42833924293518
		-4.58794745849445 2.34922552108765
		-4.59761593677104 2.27460432052612
		-4.60220231488347 2.23346638679504
		-4.62103664875031 2.115314245224
		-4.62802820280194 2.07553625106812
		-4.67956501245499 1.75870227813721
		-4.68301013112068 1.72068071365356
		-4.68606703728437 1.68488693237305
		-4.68550603836775 1.6498236656189
		-4.68293036520481 1.61361503601074
		-4.67857114970684 1.57682991027832
		-4.66163071244955 1.48022794723511
		-4.49162828922272 0.974047183990479
		1.16172933578491 3.45492267608643
		0.581977367401123 3.92502427101135
		-1.49411177635193 4.46626806259155
		-3.3784407377243 4.24612951278687
		-4.60737638175488 2.19235944747925
		-4.66783845424652 1.5105562210083
		-0.16835880279541 0.647355794906616
	};
\addlegendentry{FN}


==> tikz/vis_localize/vis_loc_test3_x_clean.tex <==
\addplot [semithick, steelblue31119180]
table {%
0.0299980640411377 -0.127345561981201
4.37010765075684 -0.144300937652588
4.92999172210693 -0.285177707672119
5.39999961853027 -0.271154880523682
5.7000093460083 -0.419476985931396
5.87002849578857 -0.404873371124268
6.07003736495972 -0.295982837677002
6.20009326934814 -0.226951599121094
6.60002422332764 -0.157015800476074
6.80009460449219 -0.249642848968506
6.97000312805176 -0.300311088562012
7.10006523132324 -0.244179725646973
7.40005493164062 -0.105488777160645
7.54001808166504 -0.0175881385803223
7.66999912261963 0.0440340042114258
7.79998588562012 0.00772333145141602
8.12999439239502 -0.148105621337891
8.34000396728516 -0.118720054626465
8.61005973815918 -0.0284314155578613
8.97002601623535 0.137029647827148
9.20997333526611 0.0924921035766602
9.39999961853027 0.0754432678222656
9.87011909484863 0.0632481575012207
10.0399971008301 0.089317798614502
10.6400012969971 0.271331310272217
10.970025062561 0.187442779541016
12.7700366973877 0.374731540679932
13.6400098800659 0.334969997406006
14.0400524139404 0.438974857330322
14.9400491714478 0.472188949584961
15.5000524520874 0.367719650268555
15.7400064468384 0.278762340545654
15.9700078964233 0.244197845458984
16.270040512085 0.173862934112549
16.5400066375732 0.191163539886475
16.9399890899658 0.221821784973145
17.5399837493896 -0.0390849113464355
17.9000587463379 -0.254226207733154
19.2100391387939 -0.506833553314209
19.5400199890137 -0.366604328155518
21.2399921417236 0.895673751831055
21.5700740814209 1.05518579483032
23.7401161193848 0.000635623931884766
24.9700298309326 -1.07523036003113
25.4399795532227 -1.26590919494629
25.7100124359131 -1.32039380073547
26.0700798034668 -1.30942845344543
26.3700904846191 -1.21963357925415
26.5701370239258 -1.12304663658142
26.810037612915 -0.97650933265686
27.5099868774414 -0.437064647674561
29.439998626709 1.40142488479614
29.9100666046143 1.59641218185425
31.6700382232666 1.44387340545654
34.4400177001953 -0.590946674346924
35.7100219726562 -1.67137670516968
36.8099899291992 -2.26539397239685
37.7400054931641 -2.3967866897583
38.4399948120117 -2.28236293792725
38.9400329589844 -2.0724835395813
39.5100212097168 -1.62045001983643
39.8700408935547 -1.29381799697876
40.0400390625 -1.12258219718933
40.7800445556641 -0.248787403106689
41.1100158691406 0.0581064224243164
42.5400123596191 1.29006958007812
43.3400192260742 1.79591703414917
43.8100242614746 1.90449810028076
44.5100021362305 2.04478597640991
45.4399528503418 1.96722936630249
45.7400588989258 1.95831918716431
46.2099914550781 1.83152008056641
47.0400085449219 1.64457130432129
47.3101272583008 1.5933313369751
47.7800369262695 1.51393747329712
49.8800659179688 -0.442275047302246
50.0800018310547 -0.676595449447632
50.7399864196777 -1.4564642906189
51.6100769042969 -2.35638403892517
52.1100196838379 -2.75773000717163
53.2700386047363 -3.49682235717773
53.4800071716309 -3.72223806381226
55.3399887084961 -4.55744743347168
56.0400123596191 -4.67640256881714
56.5100402832031 -4.61396360397339
57.0400924682617 -4.39940452575684
57.2800064086914 -4.27538204193115
57.6400489807129 -3.94924902915955
58.5500869750977 -2.95299530029297
59.5400543212891 -1.77560305595398
59.7400512695312 -1.54093384742737
60.1100196838379 -1.10503554344177
60.4800186157227 -0.671017408370972
61.6101226806641 0.355794429779053
61.9800109863281 0.432490825653076
62.5099754333496 0.453404903411865
63.0800399780273 0.243512630462646
63.3400192260742 0.0598263740539551
65.0400619506836 -0.64622688293457
65.4099960327148 -0.616232395172119
65.5800170898438 -0.554276466369629
66.2500305175781 -0.226614952087402
66.7100448608398 -0.143428325653076
68.7802352905273 -0.169086456298828
};
\addlegendentry{MOCAP}
\addplot [semithick, darkorange25512714]
table {%
0.0299980640411377 -0.233597993850708
0.0999770164489746 -0.234863996505737
0.130005836486816 -0.155846953392029
0.170056343078613 -0.182829022407532
0.200010776519775 -0.159677982330322
0.299990892410278 -0.212311983108521
0.329993963241577 -0.157320976257324
0.37003755569458 -0.205796003341675
0.399981498718262 -0.158695936203003
0.430063962936401 -0.210425019264221
0.469975233078003 -0.20194399356842
0.49998950958252 -0.238245010375977
0.540004014968872 -0.182394027709961
0.600008487701416 -0.241443037986755
0.670019626617432 -0.16066300868988
0.770064830780029 -0.205796003341675
0.870023012161255 -0.203866004943848
0.930023431777954 -0.159677982330322
1.00003814697266 -0.20640504360199
1.03998923301697 -0.209632992744446
1.07000851631165 -0.162636041641235
1.14003682136536 -0.186439990997314
1.16999983787537 -0.148293018341064
1.2299976348877 -0.248504996299744
1.3399772644043 -0.262073993682861
1.40001010894775 -0.267112970352173
1.43002438545227 -0.320831060409546
1.5000627040863 -0.259052038192749
1.60001397132874 -0.258569002151489
1.64004039764404 -0.300575971603394
1.73010611534119 -0.202316045761108
2.10002112388611 -0.25073504447937
2.47003436088562 -0.187543988227844
2.50003480911255 -0.232157945632935
2.56999516487122 -0.182394027709961
2.67002320289612 -0.210301041603088
2.82999396324158 -0.194332003593445
2.8700065612793 -0.23374605178833
3.07002377510071 -0.220901012420654
3.10004711151123 -0.197991013526917
3.1300196647644 -0.231677055358887
3.30004215240479 -0.221593022346497
3.33001637458801 -0.18134593963623
3.39999771118164 -0.230114936828613
3.57013249397278 -0.18774402141571
3.7700035572052 -0.255313038825989
3.97003746032715 -0.255068063735962
4.02998685836792 -0.343220949172974
4.07004690170288 -0.249246954917908
4.11003112792969 -0.256880044937134
4.1300163269043 -0.328804969787598
4.20001602172852 -0.253690958023071
4.23012638092041 -0.314322948455811
4.27006721496582 -0.316187024116516
4.30002117156982 -0.276031970977783
4.37010765075684 -0.316933989524841
4.43998718261719 -0.253000974655151
4.49999523162842 -0.393157958984375
4.54004192352295 -0.386988043785095
4.57004070281982 -0.460708975791931
4.59998607635498 -0.440340995788574
4.67004585266113 -0.707247972488403
4.77001857757568 -0.53298807144165
4.80000972747803 -0.554728031158447
4.89998817443848 -0.503082990646362
4.9999942779541 -0.492255926132202
5.03003311157227 -0.561289072036743
5.10001468658447 -0.564651012420654
5.17000484466553 -0.651160955429077
5.29999971389771 -0.694000005722046
5.42998695373535 -0.565443992614746
5.60000324249268 -0.610607028007507
5.67000579833984 -0.536319017410278
5.77000999450684 -0.463405013084412
5.79998779296875 -0.56201696395874
5.84000396728516 -0.56193208694458
5.87002849578857 -0.406080961227417
5.94000339508057 -0.594594955444336
5.97000885009766 -0.515146970748901
6.00012588500977 -0.576807975769043
6.04005146026611 -0.500335931777954
6.09998035430908 -0.61604905128479
6.14000463485718 -0.612604022026062
6.20009326934814 -0.476837038993835
6.33998870849609 -0.231850028038025
6.39999675750732 -0.167400002479553
6.44004154205322 -0.232429027557373
6.47007751464844 -0.203771948814392
6.5001220703125 -0.268947005271912
6.60002422332764 -0.268931984901428
6.6300253868103 -0.196246981620789
6.70001173019409 -0.270487070083618
6.74000930786133 -0.315191984176636
6.80009460449219 -0.292108058929443
6.86998081207275 -0.311521053314209
7.00003719329834 -0.323994040489197
7.06999397277832 -0.364341974258423
7.32999420166016 -0.228615045547485
7.40005493164062 -0.322164058685303
7.49999570846558 -0.222962975502014
7.57001399993896 -0.231801986694336
7.69999504089355 -0.210456967353821
7.77001190185547 -0.0480360984802246
7.96997785568237 -0.0480830669403076
8.07002639770508 -0.047943115234375
8.1700382232666 -0.10119903087616
8.2700138092041 -0.0929131507873535
8.2999963760376 -0.167610049247742
8.4000072479248 -0.0397894382476807
8.61005973815918 0.0837949514389038
8.67000198364258 0.0422831773757935
8.87003326416016 0.070356011390686
8.94001865386963 0.177034974098206
9.00000667572021 0.197679996490479
9.03001308441162 0.261577010154724
9.1099910736084 0.179326057434082
9.170090675354 0.192885041236877
9.24007511138916 0.0837949514389038
9.43003082275391 0.0366072654724121
9.73000335693359 0.0461242198944092
10.0399971008301 0.0874488353729248
10.2300510406494 0.191275000572205
10.3000030517578 0.0924824476242065
10.7700233459473 0.319983005523682
10.8000106811523 0.254524946212769
10.8700141906738 0.339300036430359
10.9400062561035 0.257933020591736
10.970025062561 -0.233412027359009
10.999981880188 0.289322972297668
11.0401268005371 0.338806986808777
11.1400194168091 0.268312931060791
11.1699962615967 0.30056095123291
11.2400207519531 0.280833959579468
11.3000030517578 0.237108945846558
11.3400602340698 0.278454065322876
11.3700046539307 0.228001952171326
11.4000396728516 0.324293971061707
11.5399932861328 0.334176063537598
11.6100635528564 0.239726066589355
11.7100191116333 0.330253958702087
11.7400484085083 0.282276034355164
11.7700319290161 0.331279993057251
11.8000078201294 0.215412020683289
11.8399829864502 0.474624991416931
11.8701210021973 0.181823015213013
11.9400196075439 0.376112937927246
12.040020942688 0.35337495803833
12.0700225830078 1.08010005950928
12.100040435791 0.319571018218994
12.1400184631348 0.312474966049194
12.2000169754028 0.744418025016785
12.3000297546387 0.506237983703613
12.4000759124756 0.514400959014893
12.4700031280518 0.511656999588013
12.500018119812 0.415863037109375
12.5400943756104 0.411113977432251
12.6000776290894 0.518861055374146
12.6700029373169 0.408810973167419
12.7100267410278 0.397968053817749
12.7700366973877 0.331503033638
12.7999858856201 0.488772034645081
12.839994430542 0.481490969657898
12.8999948501587 0.50757098197937
12.9400062561035 0.508409023284912
12.9700174331665 0.406180024147034
13.0400819778442 0.501834988594055
13.0700349807739 0.450394988059998
13.1000957489014 0.513268947601318
13.1399765014648 0.384916067123413
13.1699829101562 0.426416993141174
13.2000198364258 0.364333987236023
13.2400064468384 0.412047028541565
13.3000154495239 0.333114981651306
13.3701410293579 0.435974955558777
13.4400310516357 0.377954006195068
13.470006942749 0.441177010536194
13.5700206756592 0.360404968261719
13.670069694519 0.360641956329346
13.7100086212158 0.248602986335754
13.8399982452393 0.478126049041748
13.8700723648071 0.382962942123413
13.900050163269 0.486549973487854
13.9399948120117 0.466518998146057
14.0000009536743 0.406126022338867
14.0700130462646 0.341594934463501
14.1000213623047 0.487390041351318
14.1700105667114 0.518801927566528
14.2400197982788 0.290192008018494
14.3100185394287 0.568769931793213
14.3400011062622 0.507483959197998
14.3999795913696 0.558110952377319
14.4401330947876 0.491209030151367
14.470009803772 0.566755056381226
14.4999990463257 0.536399006843567
14.540020942688 0.609210014343262
14.6000213623047 0.357507944107056
14.6400022506714 0.490258932113647
14.7000188827515 0.394443988800049
14.7400217056274 0.45763897895813
14.7699928283691 0.393100023269653
14.8101425170898 0.399227023124695
14.8399972915649 0.500998020172119
14.8699769973755 0.474151968955994
14.8999786376953 0.345806002616882
14.9700183868408 0.371047973632812
15.0000038146973 0.468098044395447
15.0999889373779 0.448047995567322
15.1400184631348 0.528532028198242
15.1700115203857 0.744447946548462
15.2699947357178 0.232967972755432
15.3000059127808 0.368330955505371
15.3999862670898 0.446996927261353
15.4700717926025 0.414298057556152
15.5000524520874 0.476310014724731
15.5400085449219 0.33005702495575
15.5700340270996 0.4220290184021
15.5999889373779 0.262354969978333
15.7000198364258 0.330613970756531
15.839991569519 0.246906995773315
15.8700008392334 0.166666984558105
15.9100399017334 0.362529039382935
15.9700078964233 0.220023036003113
16.0700130462646 0.256976008415222
16.1400375366211 0.256976008415222
16.1700019836426 0.208322048187256
16.210090637207 0.257815003395081
16.3100090026855 0.211312055587769
16.3399848937988 0.232262015342712
16.4000930786133 0.197042942047119
16.570011138916 0.183439016342163
16.6000118255615 0.14498496055603
16.6399993896484 0.194234013557434
16.7001514434814 0.158774018287659
16.7700462341309 0.152322053909302
16.8400745391846 0.160366058349609
16.9000434875488 0.132689952850342
17 0.130411028862
17.2000179290771 0.116986036300659
17.2700347900391 0.200711011886597
17.3399982452393 0.169878005981445
17.4999942779541 0.155755996704102
17.5701160430908 0.148599982261658
17.6700420379639 0.271618008613586
17.739990234375 0.117910027503967
17.8000011444092 0.124194025993347
17.9399700164795 0.049547553062439
18.0700225830078 0.0285944938659668
18.1700038909912 -0.0441726446151733
18.2400016784668 -0.140385031700134
18.2700653076172 -0.119905948638916
18.3399906158447 -0.210482001304626
18.3999881744385 -0.280694007873535
18.4400119781494 -0.241675019264221
18.4700260162354 -0.317633986473083
18.500020980835 -0.263889074325562
18.5701370239258 -0.385203957557678
18.640022277832 -0.322018980979919
18.7700614929199 -0.420660018920898
18.8000240325928 -0.372211933135986
18.870096206665 -0.391181945800781
18.9400653839111 -0.335782051086426
19.0000228881836 -0.440402984619141
19.1700038909912 -0.609863996505737
19.2400035858154 -0.649030923843384
19.2700042724609 -0.577054023742676
19.3400325775146 -0.693222999572754
19.4000587463379 -0.661432027816772
19.470027923584 -0.573436975479126
19.5400199890137 -0.49085795879364
19.6100177764893 -0.558889985084534
19.6399955749512 -0.533061027526855
19.6700572967529 -0.582057952880859
19.7700996398926 -0.550997972488403
19.8399791717529 -0.577126026153564
20.1700611114502 -0.304502010345459
20.2999839782715 -0.128075003623962
20.9000396728516 0.523272037506104
21.0000476837158 0.524724960327148
21.2399921417236 0.67174506187439
21.5700740814209 1.00234997272491
23.7401161193848 0.38562798500061
24.4700489044189 -0.501600027084351
24.5100288391113 -0.490057945251465
24.5700035095215 -0.55117392539978
24.6100234985352 -0.533462047576904
24.7100925445557 -0.631097078323364
24.8100719451904 -0.681788921356201
24.8700408935547 -0.713472008705139
24.9100189208984 -0.891059994697571
24.9399909973145 -0.797055959701538
25.0099868774414 -0.934983015060425
25.0399856567383 -1.02987003326416
25.0700054168701 -0.985615015029907
25.110107421875 -1.00029003620148
25.1700172424316 -1.08548998832703
25.2100028991699 -1.10328996181488
25.2700119018555 -1.03626000881195
25.3101043701172 -1.01610994338989
25.3800506591797 -1.08847999572754
25.3999786376953 -1.0380699634552
25.4999885559082 -1.17076003551483
25.5400218963623 -0.216138005256653
25.5700225830078 -1.26467001438141
25.6700077056885 -1.26679003238678
25.8100471496582 -1.21638000011444
25.8699855804443 -1.31555998325348
25.9100170135498 -1.33361995220184
25.9400081634521 -1.276859998703
25.9700164794922 -1.38443994522095
26.0100631713867 -1.25837004184723
26.0700798034668 -1.29619002342224
26.1701507568359 -1.39012002944946
26.3100185394287 -1.20877003669739
26.3700904846191 -1.18605005741119
26.4400939941406 -1.19661998748779
26.4800128936768 -1.14426004886627
26.510046005249 -1.22238004207611
26.5701370239258 -1.0239599943161
26.6099891662598 -1.05893003940582
26.669994354248 -1.13935995101929
26.7700080871582 -1.0670599937439
26.8401145935059 -1.11312997341156
26.9101181030273 -1.10440003871918
26.9700241088867 -1.18842995166779
27.0100326538086 -0.978945016860962
27.0701522827148 -1.10839998722076
27.1099796295166 -1.1047500371933
27.2100219726562 -0.986546993255615
27.3700332641602 -0.990520000457764
27.4400749206543 -0.876944065093994
27.5400924682617 -0.771620988845825
29.3400115966797 1.19021999835968
29.3700275421143 1.40371000766754
29.439998626709 1.30768001079559
29.9100666046143 1.25629997253418
31.6700382232666 1.6220999956131
34.1099853515625 0.0863475799560547
34.1700248718262 -0.0082932710647583
34.7800140380859 -0.66034197807312
34.8100280761719 -0.63577401638031
34.8400115966797 -0.706897974014282
34.9099998474121 -0.69130802154541
34.9800148010254 -0.856971979141235
35.1100120544434 -0.906552076339722
35.1400032043457 -0.995707035064697
35.2399864196777 -1.12585997581482
35.7100219726562 -1.37005996704102
36.8400497436523 -2.2386200428009
36.870059967041 -2.1975200176239
36.9400787353516 -2.51377010345459
36.9701156616211 -2.41527009010315
37.0400047302246 -2.50501990318298
37.0700416564941 -2.54558992385864
37.140079498291 -2.49200010299683
37.210033416748 -2.52908992767334
37.2700004577637 -2.50986003875732
37.3400421142578 -2.6120400428772
37.4400062561035 -2.59060001373291
37.5400009155273 -2.48638010025024
37.5700378417969 -2.55242991447449
37.6099853515625 -2.33749008178711
37.6700401306152 -2.6173300743103
37.710033416748 -2.55660009384155
37.7700080871582 -2.62970995903015
37.8400459289551 -2.54690003395081
37.9101295471191 -2.67735004425049
37.9700584411621 -2.66476988792419
38.0399932861328 -2.50928997993469
38.0699996948242 -2.54520988464355
38.1100387573242 -2.50662994384766
38.1700057983398 -2.40903997421265
38.2699928283691 -2.53822994232178
38.3100776672363 -2.4065101146698
38.3400115966797 -2.50748991966248
38.4099998474121 -2.47956991195679
38.4399948120117 -2.52977991104126
38.4700164794922 -2.36958003044128
38.5100975036621 -2.48175001144409
38.5400543212891 -2.43781995773315
38.5699996948242 -2.5127899646759
38.6101188659668 -2.48690009117126
38.6699829101562 -2.65955996513367
38.7100372314453 -2.84969997406006
38.8100357055664 -2.36912989616394
38.8400573730469 -2.33505010604858
38.8699989318848 -2.0480101108551
38.910041809082 -2.04293990135193
38.9400329589844 -2.09739995002747
39.0100250244141 -2.00394010543823
39.0700378417969 -2.41990995407104
39.140022277832 -2.27985000610352
39.2100067138672 -2.14086008071899
39.240047454834 -2.39415001869202
39.2800750732422 -2.32886004447937
39.3100395202637 -2.36469006538391
39.3699989318848 -2.27431011199951
39.4100189208984 -2.28785991668701
39.4400482177734 -2.41108989715576
39.5400123596191 -2.09540009498596
39.5800170898438 -2.18866991996765
39.640064239502 -2.11208009719849
39.6799774169922 -2.19204998016357
39.7101097106934 -2.17132997512817
39.7799987792969 -2.03172993659973
39.8400344848633 -1.94773995876312
39.9101142883301 -1.96589004993439
39.9399948120117 -1.85548996925354
40.1400413513184 -1.54472994804382
40.2100105285645 -1.2843199968338
40.2399940490723 -1.32002997398376
40.2700424194336 -1.26988005638123
40.7800445556641 -0.793776035308838
40.869987487793 -0.578783988952637
40.9800987243652 -0.434628009796143
41.2800140380859 -0.0750869512557983
41.3700256347656 0.0911450386047363
41.5100212097168 0.17776894569397
41.5699920654297 0.265807032585144
41.8100395202637 0.561182975769043
42.6100692749023 1.40585005283356
42.8801155090332 1.52981996536255
42.9100189208984 1.59162998199463
42.940113067627 1.43536996841431
42.9700164794922 0.770791053771973
43.0400199890137 1.68252003192902
43.0700073242188 1.22678995132446
43.1400146484375 2.20266008377075
43.2099761962891 2.29620003700256
43.2400207519531 2.1532199382782
43.2700042724609 2.23854994773865
43.3400192260742 2.23950004577637
43.3700752258301 2.34289002418518
43.4100227355957 2.26119995117188
43.4800186157227 2.48360991477966
43.5400390625 2.28956007957458
43.5801277160645 1.85199999809265
43.6100006103516 2.17670011520386
43.6400146484375 1.9130699634552
43.7800331115723 1.70290994644165
43.8100242614746 1.74554002285004
44.2100372314453 2.38059997558594
44.2401733398438 1.9279500246048
44.340087890625 2.5634400844574
44.5100021362305 2.23932003974915
45.3099937438965 2.12332010269165
45.3699989318848 2.92249989509583
45.4399528503418 2.11089992523193
45.4799919128418 2.11431002616882
45.5399856567383 2.18018007278442
45.610050201416 2.18343997001648
45.6800155639648 2.11307001113892
45.7400588989258 2.16948008537292
45.7800559997559 1.89089000225067
45.8400077819824 1.92806994915009
45.8799781799316 1.85032999515533
45.9800338745117 2.01625990867615
46.0400238037109 2.29672002792358
46.1100273132324 2.27867007255554
46.140022277832 1.7380199432373
46.2099914550781 1.69534003734589
46.2401275634766 1.78322994709015
46.3100242614746 2.16598010063171
46.3700218200684 1.98873996734619
46.440013885498 2.07154989242554
46.5100555419922 2.01678991317749
46.5799674987793 2.06292009353638
46.6400375366211 1.98018002510071
46.7100868225098 1.9527599811554
46.7400512695312 2.03974008560181
46.7799949645996 -0.21849799156189
46.8400192260742 1.67418003082275
46.940071105957 1.69639003276825
47.0400085449219 1.56878995895386
47.1100425720215 1.80850005149841
47.170051574707 1.76031994819641
47.2400131225586 1.81729996204376
47.3101272583008 1.58507001399994
47.4100151062012 1.37443995475769
47.4399948120117 1.55365002155304
47.5100135803223 1.37266004085541
49.5400428771973 0.191885948181152
49.7101631164551 0.0559804439544678
50.1800231933594 -0.423689961433411
50.2800407409668 -0.490128040313721
50.6800003051758 -0.973757028579712
50.7399864196777 -0.984673023223877
51.6100769042969 -1.82271003723145
51.7800064086914 -1.87496995925903
51.8100738525391 -2.05501008033752
52.1100196838379 -2.14616990089417
53.1800384521484 -2.21012997627258
53.2700386047363 -2.32797002792358
53.4800071716309 -2.3783700466156
55.3399887084961 -3.57577991485596
55.8800582885742 -4.00454998016357
55.9401359558105 -3.96279001235962
55.970043182373 -3.88480997085571
56.0400123596191 -3.91775989532471
56.4100494384766 -4.04524993896484
56.4500503540039 -3.99847006797791
56.5100402832031 -4.04638004302979
56.7099990844727 -4.14534997940063
56.7400207519531 -4.09893989562988
56.7799644470215 -4.10447978973389
56.8800163269043 -4.17372989654541
57.0400924682617 -4.26109981536865
57.1100006103516 -4.1929497718811
57.1800308227539 -3.67172002792358
57.240047454834 -3.78128004074097
57.2800064086914 -4.16508007049561
57.3399963378906 -4.0368800163269
57.3800735473633 -4.03942012786865
57.4400939941406 -3.82634997367859
57.4800453186035 -3.83137011528015
57.5101051330566 -3.95124006271362
57.5400466918945 -3.79809999465942
57.6400489807129 -3.81175994873047
57.6800346374512 -3.81410002708435
57.7400588989258 -3.66814994812012
57.7800140380859 -3.65897011756897
57.8400001525879 -3.48171997070312
57.8800621032715 -3.51654005050659
58.0100059509277 -3.5325300693512
58.0800476074219 -3.49255990982056
58.1400566101074 -3.58650994300842
58.3800582885742 -3.45683002471924
58.410083770752 -3.36718988418579
58.5100250244141 -2.72942996025085
58.7399940490723 -2.62927007675171
58.7799949645996 -2.6298201084137
58.810115814209 -2.51119995117188
58.8800010681152 -2.47196006774902
58.9100151062012 -2.37336993217468
58.9799957275391 -2.45496010780334
59.0100479125977 -2.37302994728088
59.1100425720215 -1.73327004909515
59.2400398254395 -1.76356995105743
59.510139465332 -1.67568004131317
59.5799980163574 -1.52340996265411
59.6100044250488 -1.56720995903015
59.6800422668457 -1.49906003475189
59.7100028991699 -1.46770000457764
59.7400512695312 -1.53015995025635
59.8400039672852 -1.45301997661591
60.2100524902344 -1.04840004444122
60.4800186157227 -0.755814075469971
61.6101226806641 0.368955969810486
61.8399810791016 0.44716203212738
61.9100685119629 0.253435015678406
61.9800109863281 0.366920948028564
62.010009765625 0.513154029846191
62.0800170898438 0.496166944503784
62.1401214599609 0.53302800655365
62.2100830078125 0.478935956954956
62.2400207519531 0.517565965652466
62.3400459289551 0.433851957321167
62.3799934387207 0.428259968757629
62.4399719238281 0.469313025474548
62.4800148010254 0.4897620677948
62.5099754333496 0.416643977165222
62.9799880981445 0.403957009315491
63.010009765625 0.367457032203674
63.0400123596191 0.435657024383545
63.0800399780273 0.381813049316406
63.1100273132324 0.410302996635437
63.140007019043 0.32000994682312
63.1800155639648 0.343039035797119
63.2400054931641 0.281865000724792
63.3100700378418 0.342602014541626
63.3400192260742 0.309720039367676
65.1099472045898 -0.531628012657166
65.3400192260742 -0.588856935501099
65.4500045776367 -0.552490949630737
65.6400451660156 -0.487923979759216
65.680046081543 -0.393914937973022
65.8399810791016 -0.362926959991455
65.9800796508789 -0.403144001960754
66.0501174926758 -0.328184962272644
66.3100280761719 -0.234004974365234
66.7100448608398 -0.236577987670898
66.7800140380859 -0.200168013572693
66.9500198364258 -0.228909969329834
67.1100845336914 -0.242675065994263
67.5400085449219 -0.266363978385925
67.5800857543945 0.29940402507782
67.6100692749023 -0.268662929534912
67.9400100708008 -0.274174928665161
68.0401382446289 -0.250362038612366
68.0799865722656 -0.270756959915161
68.1799926757812 -1.15176999568939
68.7802352905273 1.8497200012207
};
\addlegendentry{Prediction}


==> tikz/vis_localize/vis_loc_test3_y_clean.tex <==
\addplot [semithick, steelblue31119180]
table {%
0.0299980640411377 0.33639669418335
4.49999523162842 0.288275241851807
4.77001857757568 0.174499034881592
5.19998550415039 -0.0621557235717773
5.34006309509277 -0.0919655561447144
5.97000885009766 0.0285007953643799
6.26997756958008 -0.0423965454101562
6.57006740570068 -0.1480393409729
7.19999122619629 -0.122844219207764
7.77001190185547 -0.19659161567688
8.12999439239502 -0.284783720970154
8.54006290435791 -0.230524182319641
8.97002601623535 -0.151102185249329
9.24007511138916 -0.23091721534729
9.6099853515625 -0.299678683280945
9.9399995803833 -0.287723302841187
10.6400012969971 -0.169587016105652
10.970025062561 -0.296054005622864
11.2400207519531 -0.276474714279175
11.5000152587891 -0.225665330886841
11.8701210021973 -0.0525145530700684
12.040020942688 -0.00803828239440918
12.3400497436523 -0.101634621620178
12.6000776290894 -0.178051948547363
13.01003074646 -0.0732778310775757
13.3000154495239 0.0655753612518311
13.5400390625 0.150809526443481
14.2400197982788 0.0147478580474854
14.570013999939 0.0812771320343018
14.8399972915649 0.241269588470459
15.0400142669678 0.356423377990723
15.1700115203857 0.398537635803223
15.4700717926025 0.370096921920776
15.7400064468384 0.293604850769043
15.9700078964233 0.227507352828979
16.3399848937988 0.23404598236084
16.570011138916 0.216319799423218
16.9000434875488 0.152985334396362
17.0699977874756 0.221850872039795
17.5701160430908 0.416812896728516
17.8399982452393 0.418219566345215
18.2400016784668 0.239755153656006
19.4000587463379 -0.542275428771973
19.8399791717529 -0.728630185127258
20.3700504302979 -0.813935160636902
21.0000476837158 -0.573930621147156
21.2399921417236 -0.438799023628235
21.5700740814209 -0.189391255378723
23.7401161193848 1.09528541564941
24.3700084686279 1.00973701477051
24.7400074005127 0.815333127975464
25.3101043701172 0.376579761505127
26.1701507568359 -0.510735273361206
26.6099891662598 -0.832702994346619
27.0100326538086 -1.17903697490692
27.2701225280762 -1.35101294517517
27.5700283050537 -1.45121026039124
29.3700275421143 -0.992703557014465
29.9100666046143 -0.615870952606201
31.6700382232666 1.2247428894043
34.1099853515625 2.71177887916565
34.340087890625 2.70517754554749
34.6100311279297 2.62346267700195
35.5699729919434 2.04121494293213
35.7100219726562 1.91444730758667
36.9400787353516 0.62915563583374
37.2700004577637 0.219289779663086
37.8400459289551 -0.401355266571045
38.3699760437012 -1.09987044334412
38.6400032043457 -1.45023894309998
38.9699859619141 -1.80741989612579
39.640064239502 -2.41797876358032
39.9399948120117 -2.53150224685669
40.2700424194336 -2.59541893005371
40.6800537109375 -2.58049273490906
40.8399887084961 -2.50488662719727
40.9800987243652 -2.46941304206848
41.2800140380859 -2.23119163513184
41.4100646972656 -2.14919877052307
41.640007019043 -2.10506248474121
41.8100395202637 -2.11187505722046
42.6100692749023 -1.90888941287994
43.4800186157227 -1.39247667789459
43.8100242614746 -1.10646677017212
44.5100021362305 -0.574985146522522
46.2099914550781 1.16457676887512
46.5799674987793 1.61689305305481
46.8701095581055 1.92758560180664
47.0400085449219 2.12453842163086
47.2799682617188 2.43225789070129
47.5100135803223 2.72636914253235
47.7800369262695 3.02699828147888
49.7101631164551 4.27157402038574
50.0400047302246 4.40784931182861
50.5101127624512 4.43559074401855
50.7399864196777 4.46156072616577
51.3800468444824 4.43182468414307
51.8100738525391 4.26759099960327
52.1100196838379 4.2039737701416
53.2700386047363 4.22978496551514
53.4800071716309 4.16917896270752
55.3399887084961 2.61663150787354
56.4100494384766 1.41955518722534
56.5800437927246 1.23333811759949
56.9402008056641 0.82365870475769
57.5800971984863 0.23731255531311
57.8800621032715 0.0395750999450684
58.3400497436523 -0.248821377754211
58.9100151062012 -0.408087491989136
59.6399955749512 -0.676748394966125
60.2400360107422 -0.746049523353577
60.4800186157227 -0.767243385314941
61.4100570678711 -0.434712052345276
61.6101226806641 -0.307351350784302
62.5099754333496 0.480981588363647
63.1100273132324 0.795889616012573
63.3400192260742 0.876285076141357
65.1099472045898 0.405576467514038
65.47998046875 0.443042755126953
66.1499710083008 0.58939528465271
67.0100479125977 0.667159557342529
67.8101043701172 0.642005205154419
68.7802352905273 0.660304307937622
};
\addlegendentry{MOCAP}
\addplot [semithick, darkorange25512714]
table {%
0.0299980640411377 0.14292299747467
0.399981498718262 0.12355101108551
0.430063962936401 0.169543027877808
0.770064830780029 0.159654021263123
0.930023431777954 0.122277975082397
1.00003814697266 0.174416065216064
1.03998923301697 0.170521974563599
1.07000851631165 0.118316054344177
1.14003682136536 0.135699987411499
1.16999983787537 0.09241783618927
1.2299976348877 0.136026978492737
1.53006339073181 0.133937001228333
1.67000126838684 0.132957935333252
2.10002112388611 0.147294998168945
2.3300256729126 0.140686988830566
2.37003064155579 0.122277975082397
2.43999552726746 0.167855024337769
2.50003480911255 0.138491034507751
2.54000902175903 0.163187980651855
2.56999516487122 0.141090989112854
2.59999322891235 0.165977001190186
2.67002320289612 0.169697046279907
2.8700065612793 0.132972955703735
3.19998478889465 0.144008040428162
3.67000508308411 0.139049053192139
3.94000291824341 0.132791996002197
4.07004690170288 0.121006965637207
4.59998607635498 0.128924012184143
4.63001251220703 0.204548001289368
4.67004585266113 0.162495970726013
4.70000171661377 0.191758990287781
4.9700345993042 0.0383081436157227
5.10001468658447 0.0126456022262573
5.13002109527588 0.177994012832642
5.17000484466553 0.167261958122253
5.24001598358154 -0.0203872919082642
5.27000904083252 0.193899035453796
5.29999971389771 -0.0292675495147705
5.34006309509277 -0.0372825860977173
5.39999961853027 0.0297728776931763
5.42998695373535 -0.0149431228637695
6.09998035430908 -0.178117990493774
6.14000463485718 -0.250898957252502
6.16999626159668 -0.217116951942444
6.20009326934814 -0.282235026359558
6.24005699157715 -0.235622048377991
6.26997756958008 -0.116845965385437
6.30000591278076 -0.173413038253784
6.39999675750732 -0.0945096015930176
6.44004154205322 -0.173228979110718
6.47007751464844 -0.150457978248596
6.5001220703125 -0.259629011154175
6.60002422332764 -0.259644985198975
6.6300253868103 -0.160393953323364
6.70001173019409 -0.275119066238403
6.77004814147949 -0.324368000030518
6.84000778198242 -0.365033984184265
6.90000915527344 -0.328106999397278
7.00003719329834 -0.338032007217407
7.06999397277832 -0.398229956626892
7.13999652862549 -0.373780012130737
7.19999122619629 -0.298344969749451
7.27001762390137 -0.257606029510498
7.32999420166016 -0.24839198589325
7.40005493164062 -0.480924963951111
7.54001808166504 -0.445323944091797
7.61000728607178 -0.526742935180664
7.69999504089355 -0.505284070968628
7.77001190185547 -0.387099027633667
7.84001064300537 -0.418148040771484
7.90002155303955 -0.393723011016846
7.93998003005981 -0.627246022224426
8.07002639770508 -0.416089057922363
8.12999439239502 -0.375730037689209
8.2700138092041 -0.375967979431152
8.2999963760376 -0.416794061660767
8.37005615234375 -0.38947606086731
8.47005081176758 -0.426209926605225
8.54006290435791 -0.415426015853882
8.57003211975098 -0.447054982185364
8.61005973815918 -0.405211925506592
8.9000129699707 -0.403723955154419
9.03001308441162 -0.455076932907104
9.07000160217285 -0.412292957305908
9.170090675354 -0.48160195350647
9.24007511138916 -0.405211925506592
9.37002563476562 -0.45265007019043
9.47000217437744 -0.375882983207703
9.57014083862305 -0.41340696811676
9.90005397796631 -0.419528961181641
9.9399995803833 -0.455289006233215
9.96999931335449 -0.388280034065247
10.2300510406494 -0.404265999794006
10.3000030517578 -0.360100030899048
10.7300224304199 -0.335484027862549
10.7700233459473 -0.413892030715942
10.8399982452393 -0.366474986076355
10.8700141906738 -0.436995029449463
10.9400062561035 -0.336552977561951
10.970025062561 0.21982204914093
10.999981880188 -0.419510960578918
11.0401268005371 -0.456493020057678
11.1400194168091 -0.392063021659851
11.3400602340698 -0.371679067611694
11.3700046539307 -0.292475938796997
11.440110206604 -0.445719957351685
11.5000152587891 -0.469413995742798
11.6700534820557 -0.352949023246765
11.7100191116333 -0.378069043159485
11.7700319290161 -0.254433035850525
11.8000078201294 -0.216204047203064
11.8399829864502 -0.314208984375
11.8701210021973 -0.171911954879761
11.9700469970703 -0.253919959068298
11.9999971389771 -0.22154700756073
12.0700225830078 -0.321699976921082
12.1400184631348 -0.206874012947083
12.2000169754028 -0.273726940155029
12.3000297546387 -0.303880929946899
12.3400497436523 -0.364933013916016
12.4400100708008 -0.230419039726257
12.500018119812 -0.241405963897705
12.5400943756104 -0.197065949440002
12.6000776290894 -0.252663016319275
12.6399955749512 -0.195178985595703
12.7100267410278 -0.211845993995667
12.7700366973877 -0.192216992378235
12.7999858856201 -0.246396064758301
12.870078086853 -0.236485958099365
12.9400062561035 -0.242771029472351
12.9700174331665 -0.207810044288635
13.0400819778442 -0.219987034797668
13.2000198364258 -0.0758682489395142
13.3000154495239 -0.15149199962616
13.4000358581543 -0.0940377712249756
13.4400310516357 -0.0778845548629761
13.4999933242798 -0.0928823947906494
13.6000986099243 -0.0301791429519653
13.8399982452393 0.0355585813522339
13.8700723648071 -0.0113499164581299
13.900050163269 0.0398036241531372
14.0000009536743 0.0105316638946533
14.0700130462646 -0.0298130512237549
14.4401330947876 -0.0223982334136963
14.4999990463257 0.0262471437454224
14.6000213623047 0.0478206872940063
14.7000188827515 0.0713188648223877
14.7699928283691 0.079723596572876
15.1400184631348 0.204398036003113
15.1700115203857 0.352779030799866
15.2699947357178 0.0904673337936401
15.3700475692749 0.238131046295166
15.4700717926025 0.2516850233078
15.5000524520874 0.28750205039978
15.5400085449219 0.205505967140198
15.5700340270996 0.28057599067688
15.5999889373779 0.16084897518158
15.7400064468384 0.222576975822449
15.8099842071533 0.199329018592834
15.8700008392334 0.140748977661133
15.9100399017334 0.294615030288696
15.9700078964233 0.206122040748596
16.0700130462646 0.247982978820801
16.1400375366211 0.247982978820801
16.1700019836426 0.199020981788635
16.210090637207 0.253744006156921
16.3100090026855 0.203763961791992
16.3399848937988 0.22270393371582
16.4000930786133 0.182844996452332
16.5000038146973 0.184056043624878
16.6000118255615 0.128121972084045
16.6399993896484 0.162865042686462
16.7001514434814 0.127995014190674
17.0699977874756 0.115522980690002
17.1000080108643 0.135086059570312
17.1700439453125 0.105360984802246
17.2700347900391 0.221691012382507
17.2999744415283 0.185642004013062
17.4700317382812 0.247035026550293
17.4999942779541 0.209910988807678
17.5701160430908 0.234125971794128
17.6700420379639 0.521915912628174
17.739990234375 0.260170936584473
17.8701210021973 0.279046058654785
17.9700508117676 0.165122985839844
18.0400066375732 0.123446941375732
18.140007019043 0.3315349817276
18.1700038909912 0.230785965919495
18.2000026702881 0.392646074295044
18.310037612915 0.209344029426575
18.4400119781494 0.199401021003723
18.4700260162354 0.276419043540955
18.500020980835 0.214810967445374
18.5400562286377 0.249763965606689
18.640022277832 0.158524990081787
18.7700614929199 0.138695955276489
18.8401851654053 0.0957103967666626
19.1000175476074 -0.113415002822876
19.4000587463379 -0.466891050338745
19.470027923584 -0.439713001251221
19.5000171661377 -0.483500957489014
19.5400199890137 -0.411345958709717
19.6100177764893 -0.525979042053223
19.6700572967529 -0.625257015228271
19.7700996398926 -0.715533018112183
19.8399791717529 -0.831707000732422
20.2999839782715 -0.980885982513428
20.3700504302979 -0.962890982627869
20.840015411377 -0.911802053451538
20.8699798583984 -0.96080493927002
20.9000396728516 -0.910362005233765
21.0000476837158 -0.810343027114868
21.2399921417236 -0.75550901889801
21.5700740814209 -0.615105986595154
23.7401161193848 0.911396026611328
24.4099731445312 0.93373703956604
24.4400215148926 0.97763204574585
24.5100288391113 0.871819019317627
24.5399894714355 0.888779997825623
24.6100234985352 0.834048986434937
24.6700134277344 0.877948999404907
24.8100719451904 0.791362047195435
24.8700408935547 0.72578501701355
24.9100189208984 0.805940985679626
24.9700298309326 0.729007005691528
25.0399856567383 0.783595085144043
25.110107421875 0.732749938964844
25.2100028991699 0.6804039478302
25.2700119018555 0.565922021865845
25.3399906158447 0.528100967407227
25.3800506591797 0.522372961044312
25.3999786376953 0.477661967277527
25.4701595306396 0.459810972213745
25.4999885559082 0.419218063354492
25.5400218963623 0.216088056564331
25.5700225830078 0.279927015304565
25.6400203704834 0.221075057983398
25.7699966430664 0.11932098865509
25.84006690979 0.0856673717498779
25.9700164794922 -0.0656557083129883
26.1000328063965 -0.162027955055237
26.1701507568359 -0.288233041763306
26.2700023651123 -0.367356061935425
26.3400039672852 -0.481610059738159
26.510046005249 -0.628905057907104
26.5701370239258 -0.554825067520142
26.6999835968018 -0.727813005447388
26.9101181030273 -0.908757925033569
26.9700241088867 -1.03968000411987
27.0100326538086 -0.94177508354187
27.0701522827148 -1.10143005847931
27.1400737762451 -1.1922299861908
27.2100219726562 -1.19649004936218
27.409969329834 -1.51551997661591
27.4700450897217 -1.55099999904633
27.5099868774414 -1.47925996780396
27.5700283050537 -1.58258998394012
29.3400115966797 -1.52142000198364
29.3700275421143 -1.77805995941162
29.439998626709 -1.55847001075745
29.810037612915 -0.949681043624878
29.9100666046143 -0.890951991081238
31.6700382232666 0.892668962478638
34.0799980163574 2.6734299659729
34.1099853515625 2.55451011657715
34.1700248718262 2.69055008888245
34.5400199890137 2.72503995895386
34.6100311279297 2.66002011299133
34.7400093078613 2.6835401058197
34.7800140380859 2.67965006828308
34.8100280761719 2.54729008674622
34.8400115966797 2.65534996986389
34.9099998474121 2.43553996086121
34.9800148010254 2.5511200428009
35.1100120544434 2.46591997146606
35.1400032043457 2.53607988357544
35.2399864196777 2.20526003837585
35.5699729919434 1.91049003601074
35.6700210571289 1.93025004863739
35.7100219726562 1.71653997898102
36.8400497436523 1.08515000343323
36.870059967041 1.02584004402161
36.9400787353516 1.02383005619049
37.0099792480469 0.852745056152344
37.0700416564941 0.83660101890564
37.140079498291 0.758435010910034
37.3100395202637 0.571460962295532
37.3699836730957 0.542011022567749
37.5099639892578 0.194947957992554
37.710033416748 -0.00763988494873047
38.2699928283691 -0.738424062728882
38.3100776672363 -0.729583024978638
38.4099998474121 -0.922615051269531
38.5400543212891 -1.09606003761292
38.6400032043457 -1.37997996807098
38.6699829101562 -1.3994699716568
38.7100372314453 -1.54268002510071
38.8100357055664 -1.4365199804306
38.8400573730469 -1.45747995376587
38.8699989318848 -1.32237005233765
39.0400009155273 -1.45571005344391
39.0700378417969 -1.84325003623962
39.1100654602051 -1.82027995586395
39.1700706481934 -1.88800001144409
39.2100067138672 -1.8631500005722
39.240047454834 -2.13595008850098
39.2800750732422 -2.11158990859985
39.3100395202637 -2.19809007644653
39.3699989318848 -2.1853199005127
39.4100189208984 -2.26298999786377
39.4400482177734 -2.4951000213623
39.5100212097168 -2.38557004928589
39.5400123596191 -2.35076999664307
39.5800170898438 -2.49575996398926
39.6100387573242 -2.45755004882812
39.6799774169922 -2.67779994010925
39.7400131225586 -2.59595990180969
39.7799987792969 -2.78565001487732
39.8100357055664 -2.74717998504639
39.9101142883301 -2.92186999320984
39.9399948120117 -2.86584997177124
40.010009765625 -2.83461999893188
40.0400390625 -2.76482009887695
40.1400413513184 -2.81364989280701
40.2100105285645 -2.54896998405457
40.2399940490723 -2.6457200050354
40.2700424194336 -2.62175011634827
40.6400108337402 -2.8207700252533
40.6800537109375 -2.71905994415283
40.7400169372559 -2.96481990814209
40.7800445556641 -3.01277995109558
40.8100128173828 -2.90824007987976
40.8399887084961 -3.04036998748779
40.869987487793 -2.93292999267578
40.910026550293 -2.93980002403259
41.1100158691406 -2.81489992141724
41.2400932312012 -2.83901000022888
41.2800140380859 -2.78926992416382
41.3100547790527 -2.82789993286133
41.3700256347656 -2.75379991531372
41.4100646972656 -2.83928990364075
41.439998626709 -2.81714010238647
41.4800033569336 -2.92270994186401
41.5100212097168 -2.77152991294861
41.5699920654297 -2.81576991081238
41.640007019043 -2.71112990379333
41.6800117492676 -2.46827006340027
41.8100395202637 -2.45604991912842
42.5400123596191 -2.59206008911133
42.6100692749023 -2.46660995483398
42.8801155090332 -2.26583003997803
42.9100189208984 -2.31279993057251
42.940113067627 -2.09656000137329
42.9700164794922 -1.25252997875214
43.0100555419922 -2.39211010932922
43.0400199890137 -2.21366000175476
43.0700073242188 -1.78487002849579
43.1400146484375 -2.52692008018494
43.2099761962891 -2.57816004753113
43.2400207519531 -2.38038992881775
43.2700042724609 -2.46133995056152
43.3100204467773 -2.42155003547668
43.3400192260742 -2.29120993614197
43.3700752258301 -2.34687995910645
43.4100227355957 -2.24609994888306
43.4800186157227 -2.4257800579071
43.5400390625 -2.17720007896423
43.5801277160645 -1.64495003223419
43.6100006103516 -1.9273099899292
43.6400146484375 -1.63949000835419
43.7800331115723 -1.33633005619049
44.2100372314453 -1.33057999610901
44.2401733398438 -1.06016004085541
44.3100090026855 -1.24328994750977
44.340087890625 -1.21229994297028
44.5100021362305 -0.805446028709412
45.3699989318848 -0.0181236267089844
45.4799919128418 0.251489043235779
45.8799781799316 0.584239959716797
46.0799942016602 0.993243932723999
46.140022277832 0.883113026618958
46.2401275634766 0.981934070587158
46.3100242614746 1.27795004844666
46.3700218200684 1.22002995014191
46.440013885498 1.34170997142792
46.5100555419922 1.35391998291016
46.5799674987793 1.58022999763489
46.6400375366211 1.53416001796722
46.7400512695312 1.68131005764008
46.7799949645996 0.227869033813477
46.8400192260742 1.52962005138397
46.940071105957 1.62361001968384
47.0100440979004 1.63504004478455
47.0400085449219 1.57105004787445
47.1100425720215 1.91991996765137
47.170051574707 1.94920003414154
47.2400131225586 2.03131008148193
47.3101272583008 1.79588997364044
47.3700218200684 1.89029002189636
47.4100151062012 1.79557001590729
47.4399948120117 2.07649993896484
47.5100135803223 1.86523997783661
47.7800369262695 1.97996997833252
49.6100120544434 3.7285099029541
49.640007019043 3.58937001228333
49.7101631164551 3.92034006118774
49.8500366210938 3.86382007598877
49.950080871582 3.59215998649597
50.0400047302246 3.94251990318298
50.1400299072266 3.93501996994019
50.1800231933594 3.88204002380371
50.2500038146973 3.89756989479065
50.2800407409668 3.86737990379333
50.5399894714355 3.93011999130249
50.6099853515625 3.89879989624023
50.6399917602539 3.95740008354187
50.7399864196777 3.94170999526978
51.3800468444824 3.80186009407043
51.7800064086914 3.49942994117737
51.8100738525391 3.69151997566223
52.1100196838379 3.55345988273621
53.3400230407715 2.80950999259949
53.4800071716309 2.81498003005981
55.3399887084961 2.30364990234375
55.8400344848633 2.01269006729126
55.9100532531738 1.87817001342773
56.0400123596191 1.65418004989624
56.4100494384766 1.4033499956131
56.4799880981445 1.29932999610901
56.6400184631348 1.17562997341156
56.7400207519531 1.04855000972748
56.7799644470215 1.02663004398346
56.8800163269043 0.922672033309937
56.9402008056641 0.898630976676941
57.010066986084 0.832736968994141
57.240047454834 0.537383079528809
57.2800064086914 0.551655054092407
57.3399963378906 0.46641993522644
57.4400939941406 0.387078046798706
57.5400466918945 0.297148942947388
57.5800971984863 0.300400972366333
57.6800346374512 0.194021940231323
57.7400588989258 0.144307017326355
57.8400001525879 0.0391349792480469
57.8800621032715 0.0198760032653809
58.0100059509277 -0.00998318195343018
58.1400566101074 -0.0815523862838745
58.410083770752 -0.271095037460327
58.5500869750977 -0.276258945465088
58.810115814209 -0.365499019622803
59.0100479125977 -0.475206971168518
59.0799903869629 -0.379413962364197
59.1100425720215 -0.411249995231628
59.6800422668457 -0.684354066848755
59.8799896240234 -0.781422019004822
59.9400062561035 -0.795455932617188
60.080005645752 -0.732686996459961
60.1400451660156 -0.791733026504517
60.1800193786621 -0.778187990188599
60.2400360107422 -0.853924989700317
60.4099884033203 -0.806097030639648
60.4800186157227 -0.837153911590576
61.3500785827637 -0.981857061386108
61.4100570678711 -0.937214970588684
61.6101226806641 -0.604610919952393
61.8399810791016 -0.38841700553894
61.9100685119629 -0.181174039840698
62.010009765625 -0.225589990615845
62.2100830078125 -0.0705556869506836
62.9799880981445 0.514734983444214
63.010009765625 0.489695072174072
63.0400123596191 0.597475051879883
63.0800399780273 0.544209003448486
63.1100273132324 0.619306087493896
63.140007019043 0.526814937591553
63.1800155639648 0.624227046966553
63.2099914550781 0.521934032440186
63.2400054931641 0.552955985069275
63.3100700378418 0.760186910629272
63.3400192260742 0.74313497543335
65.8100738525391 0.165926933288574
65.9800796508789 0.265841007232666
66.0501174926758 0.240280985832214
66.3100280761719 0.206277012825012
66.7400054931641 0.245872974395752
67.5400085449219 0.274503946304321
67.5800857543945 -0.402377009391785
67.6100692749023 0.272626996040344
68.0799865722656 0.270547032356262
68.1799926757812 0.332450985908508
68.7802352905273 1.64158999919891
};
\addlegendentry{Prediction}

